On the independence ratio of distance graphs

A distance graph is an undirected graph on the integers where two integers are adjacent if their difference is in a prescribed distance set. The independence ratio of a distance graph $G$ is the maximum density of an independent set in $G$. Lih, Liu, and Zhu [Star extremal circulant graphs, SIAM J. Discrete Math. 12 (1999) 491--499] showed that the independence ratio is equal to the inverse of the fractional chromatic number, thus relating the concept to the well studied question of finding the chromatic number of distance graphs. We prove that the independence ratio of a distance graph is achieved by a periodic set, and we present a framework for discharging arguments to demonstrate upper bounds on the independence ratio. With these tools, we determine the exact independence ratio for several infinite families of distance sets of size three, determine asymptotic values for others, and present several conjectures.

==> figures/svgimac <==
#!/bin/bash

for file in $* 
do
	 java -jar /Users/dstolee/User\ Applications/batik-1.7/batik-rasterizer.jar -m application/pdf $file
done



==> tables/table-g3-a00.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$51$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$52$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$53$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$54$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$55$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$56$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$57$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$58$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$59$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$60$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 0, 0+k, 0+k+i\}$.
\end{center}


==> tables/table-g3-a01.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} \\\hline
$2$ & { 2/ 7} && { 1/ 3} && { 4/11} && { 5/13} && { 2/ 5} && { 7/17} && { 8/19} && { 3/ 7} && {10/23} && {11/25} && { 4/ 9} && {13/29} && {14/31} && { 5/11} && {16/35} && {17/37} && { 6/13} && {19/41} && {20/43} && { 7/15} && {22/47} && {23/49} && { 8/17} && {25/53} && {26/55} && { 9/19} && {28/59} && {29/61} && {10/21} && {31/65} &\\\hline
$3$ & { 1/ 3} & { 2/ 5} & { 3/ 8} & { 1/ 3} & { 2/ 5} & { 4/11} & { 2/ 5} & { 5/13} & { 5/14} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 7/18} & { 7/19} & { 2/ 5} & { 8/21} & { 2/ 5} & { 9/23} & { 3/ 8} & { 2/ 5} & { 5/13} & { 2/ 5} & {11/28} & {11/29} & { 2/ 5} & {12/31} & { 2/ 5} & {13/33} & {13/34} & { 2/ 5} & { 7/18} & { 2/ 5} & {15/38} & { 5/13} & { 2/ 5} & {16/41} & { 2/ 5} & {17/43} & {17/44} & { 2/ 5} & { 9/23} & { 2/ 5} & {19/48} & {19/49} & { 2/ 5} & {20/51} & { 2/ 5} & {21/53} & { 7/18} & { 2/ 5} & {11/28} & { 2/ 5} & {23/58} & {23/59} & { 2/ 5} & {24/61} & { 2/ 5} & {25/63} & {25/64} & { 2/ 5} \\\hline
$4$ & { 2/ 7} && { 1/ 3} && { 1/ 3} && { 6/17} && { 7/19} && { 8/21} && { 9/23} && { 2/ 5} && {11/27} && {12/29} && {13/31} && {14/33} && { 3/ 7} && {16/37} && {17/39} && {18/41} && {19/43} && { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && {31/67} && {32/69} &\\\hline
$5$ & { 4/13} & { 3/ 7} & { 2/ 5} & { 3/ 8} & { 5/12} & { 1/ 3} & { 3/ 7} & { 2/ 5} & { 3/ 7} & { 7/17} & { 9/23} & { 8/19} & { 2/ 5} & { 3/ 7} & { 9/22} & { 3/ 7} & { 5/12} & { 2/ 5} & {11/26} & {11/27} & { 3/ 7} & {12/29} & { 3/ 7} & {13/31} & {13/32} & {14/33} & { 7/17} & { 3/ 7} & { 5/12} & { 3/ 7} & { 8/19} & {16/39} & {17/40} & {17/41} & { 3/ 7} & {18/43} & { 3/ 7} & {19/45} & {\color{red} 19/46} & {20/47} & { 5/12} & { 3/ 7} & {21/50} & { 3/ 7} & {11/26} & {\color{red} 22/53} & {23/54} & {23/55} & { 3/ 7} & { 8/19} & { 3/ 7} & {25/59} & {\color{red}  5/12} & {26/61} & {13/31} & { 3/ 7} & {27/64} & { 3/ 7} & {14/33} & {\color{red} 28/67} \\\hline
$6$ & { 1/ 3} && { 4/11} && { 3/ 8} && { 1/ 3} && { 6/17} && { 7/19} && { 3/ 8} && {11/29} && {12/31} && {13/33} && { 2/ 5} && {15/37} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} &\\\hline
$7$ & { 3/10} & { 4/ 9} & { 7/19} & { 2/ 5} & { 3/ 7} & { 4/11} & { 7/16} & { 1/ 3} & { 4/ 9} & { 5/13} & { 4/ 9} & { 3/ 7} & {12/29} & {10/23} & {12/31} & {11/25} & {13/33} & { 4/ 9} & { 3/ 7} & { 4/ 9} & {13/30} & { 8/19} & { 7/16} & { 2/ 5} & {15/34} & { 3/ 7} & { 4/ 9} & {16/37} & { 4/ 9} & {17/39} & {20/47} & {18/41} & { 3/ 7} & {19/43} & {19/44} & { 4/ 9} & {10/23} & { 4/ 9} & { 7/16} & { 3/ 7} & {11/25} & {22/51} & {23/52} & {23/53} & { 4/ 9} & {24/55} & { 4/ 9} & {25/57} & {\color{red} 25/58} & {26/59} & {13/30} & {27/61} & {27/62} & { 4/ 9} & { 7/16} & { 4/ 9} & {29/66} & {\color{red} 29/67} & {15/34} & {10/23} \\\hline
$8$ & { 6/19} && { 5/13} && { 2/ 5} && { 2/ 5} && { 1/ 3} && { 8/21} && { 9/23} && { 2/ 5} && { 2/ 5} && {11/29} && {12/31} && {13/33} && { 2/ 5} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && {22/53} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} &\\\hline
$9$ & { 1/ 3} & { 5/11} & { 5/14} & { 5/12} & { 2/ 5} & { 5/13} & { 4/ 9} & { 4/11} & { 9/20} & { 1/ 3} & { 5/11} & { 3/ 8} & { 5/11} & { 7/17} & { 3/ 7} & { 4/ 9} & {15/37} & {13/29} & { 5/13} & {14/31} & {16/41} & { 5/11} & {18/43} & { 5/11} & { 4/ 9} & {10/23} & {17/38} & { 5/12} & { 9/20} & { 2/ 5} & {19/42} & {11/26} & { 5/11} & { 4/ 9} & { 5/11} & {21/47} & {25/57} & {22/49} & {25/59} & {23/51} & {26/61} & {24/53} & { 4/ 9} & { 5/11} & {25/56} & { 5/11} & {13/29} & {15/34} & { 9/20} & { 3/ 7} & {14/31} & { 4/ 9} & {29/64} & {29/65} & { 5/11} & {30/67} & { 5/11} & {31/69} & {35/79} & {32/71} \\\hline
$10$ & { 4/13} && { 2/ 5} && { 7/17} && { 5/12} && {12/31} && { 1/ 3} && { 2/ 5} && {11/27} && {12/29} && { 5/12} && {17/43} && { 2/ 5} && {15/37} && {16/39} && {17/41} && { 5/12} && { 2/ 5} && {\color{red} 19/47} && {\color{red} 20/49} && {\color{red}  7/17} && {\color{red} 22/53} && { 5/12} && {28/67} && {29/69} && {30/71} && {31/73} && {32/75} && { 3/ 7} && {34/79} && {35/81} &\\\hline
$11$ & { 8/25} & { 6/13} & { 3/ 8} & { 3/ 7} & { 5/13} & { 2/ 5} & {13/31} & { 8/21} & { 5/11} & { 5/13} & {11/24} & { 1/ 3} & { 6/13} & {10/27} & { 6/13} & { 2/ 5} & {18/41} & { 3/ 7} & {18/43} & { 5/11} & { 2/ 5} & {16/35} & { 5/13} & {17/37} & {19/49} & { 6/13} & { 7/17} & { 6/13} & {23/53} & { 4/ 9} & { 5/11} & { 3/ 7} & {21/46} & {12/29} & {11/24} & { 2/ 5} & {23/50} & {13/31} & { 6/13} & { 7/16} & { 6/13} & { 5/11} & {30/67} & {26/57} & {10/23} & {27/59} & {30/71} & {28/61} & {31/73} & {29/63} & {11/25} & { 6/13} & { 5/11} & { 6/13} & {31/68} & { 9/20} & {16/35} & {18/41} & {11/24} & { 3/ 7} \\\hline
$12$ & { 1/ 3} && {11/29} && { 8/19} && { 3/ 7} && { 3/ 7} && {14/37} && { 1/ 3} && {16/41} && {13/31} && {14/33} && { 3/ 7} && { 3/ 7} && {20/51} && {21/53} && {18/43} && {19/45} && {20/47} && { 3/ 7} && { 3/ 7} && { 2/ 5} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && { 3/ 7} && {\color{red} 28/67} && {\color{red} 29/69} && {\color{red} 30/71} && {\color{red} 31/73} &\\\hline
$13$ & { 5/16} & { 7/15} & { 7/18} & { 7/16} & { 2/ 5} & { 7/17} & { 2/ 5} & { 9/23} & {16/37} & { 2/ 5} & { 6/13} & { 2/ 5} & {13/28} & { 1/ 3} & { 7/15} & {12/31} & { 7/15} & {13/33} & {21/47} & { 5/12} & { 3/ 7} & {11/25} & { 7/17} & { 6/13} & { 2/ 5} & {19/41} & { 2/ 5} & {20/43} & {\color{red} 17/44} & { 7/15} & {24/59} & { 7/15} & {26/61} & {14/31} & { 4/ 9} & { 7/16} & { 6/13} & {14/33} & {25/54} & { 7/17} & {13/28} & { 2/ 5} & {27/58} & { 5/12} & { 7/15} & {16/37} & { 7/15} & {17/38} & { 5/11} & { 6/13} & {35/79} & {31/67} & {35/81} & {32/69} & {35/83} & {33/71} & {36/85} & {34/73} & {38/87} & { 7/15} \\\hline
$14$ & {10/31} && { 7/19} && { 3/ 7} && {10/23} && { 7/16} && {17/41} && { 3/ 8} && { 1/ 3} && {18/47} && { 3/ 7} && {16/37} && {17/39} && { 7/16} && { 8/19} && {23/59} && {24/61} && { 3/ 7} && {22/51} && {23/53} && {24/55} && { 7/16} && {31/73} && { 2/ 5} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {\color{red} 31/71} && { 7/16} && {38/89} &\\\hline
$15$ & { 1/ 3} & { 8/17} & { 2/ 5} & { 4/ 9} & { 9/22} & { 8/19} & { 7/17} & { 2/ 5} & {17/41} & {11/27} & {19/43} & { 7/17} & { 7/15} & { 9/23} & {15/32} & { 1/ 3} & { 8/17} & { 2/ 5} & { 8/17} & {15/37} & {24/53} & {\color{red} 16/39} & {24/55} & { 3/ 7} & { 8/19} & {13/29} & { 9/22} & { 7/15} & { 7/17} & {22/47} & {25/63} & {23/49} & { 2/ 5} & { 8/17} & {\color{red} 21/52} & { 8/17} & {29/69} & {16/35} & {31/71} & { 4/ 9} & {33/73} & {16/37} & { 7/15} & { 8/19} & {29/62} & { 7/17} & {15/32} & { 2/ 5} & {31/66} & {17/41} & { 8/17} & { 3/ 7} & { 8/17} & {19/43} & {40/87} & { 5/11} & {40/89} & { 7/15} & {40/91} & {36/77} \\\hline
$16$ & { 6/19} && { 8/21} && {16/39} && {11/25} && { 4/ 9} && { 4/ 9} && {19/47} && { 7/18} && { 1/ 3} && {\color{red} 14/37} && {23/55} && {18/41} && {19/43} && { 4/ 9} && { 4/ 9} && {27/65} && {\color{red}  7/18} && { 9/23} && {30/71} && {25/57} && {26/59} && {27/61} && { 4/ 9} && { 4/ 9} && {35/83} && { 2/ 5} && {37/87} && {32/73} && {\color{red} 11/25} && {\color{red} 34/77} &\\\hline
$17$ & {12/37} & { 9/19} & { 5/13} & { 9/20} & { 5/12} & { 3/ 7} & { 8/19} & { 9/22} & { 2/ 5} & {12/29} & {20/47} & {13/31} & {22/49} & { 8/19} & { 8/17} & { 5/13} & {17/36} & { 1/ 3} & { 9/19} & {11/28} & { 9/19} & {17/41} & {27/59} & {18/43} & {27/61} & { 8/19} & { 3/ 7} & { 7/16} & {\color{red}  5/12} & { 5/11} & {21/50} & { 8/17} & { 8/19} & {25/53} & {28/71} & {26/55} & {29/73} & { 9/19} & {12/29} & { 9/19} & {\color{red}  5/12} & { 6/13} & {34/79} & { 9/20} & { 4/ 9} & {18/41} & {38/83} & { 3/ 7} & { 8/17} & {\color{red} 29/69} & {33/70} & { 8/19} & {17/36} & { 2/ 5} & {35/74} & {\color{red} 31/75} & { 9/19} & {20/47} & { 9/19} & { 7/16} \\\hline
$18$ & { 1/ 3} && { 9/23} && { 2/ 5} && { 4/ 9} && {13/29} && { 9/20} && {22/51} && { 2/ 5} && { 2/ 5} && { 1/ 3} && {16/41} && {25/61} && { 4/ 9} && {21/47} && {22/49} && { 9/20} && {31/71} && {30/73} && { 2/ 5} && {\color{red} 23/59} && {33/79} && { 4/ 9} && {29/65} && {30/67} && {31/69} && { 9/20} && {40/91} && {13/31} && { 2/ 5} && {41/97} &\\\hline
$19$ & {\color{red}  7/22} & {10/21} & { 3/ 8} & { 5/11} & {11/26} & {10/23} & { 3/ 7} & { 5/12} & { 3/ 7} & { 2/ 5} & { 7/17} & {14/33} & {23/53} & { 3/ 7} & { 5/11} & { 3/ 7} & { 9/19} & { 8/21} & {19/40} & { 1/ 3} & {10/21} & {12/31} & {10/21} & {19/45} & { 6/13} & {20/47} & {30/67} & { 3/ 7} & {10/23} & { 3/ 7} & {\color{red} 11/26} & { 4/ 9} & {23/54} & {17/37} & { 3/ 7} & { 9/19} & { 3/ 7} & {28/59} & {31/79} & {29/61} & {32/81} & {10/21} & {27/64} & {10/21} & {14/33} & {20/43} & {\color{red} 29/68} & { 5/11} & {39/89} & { 4/ 9} & {41/91} & {10/23} & {43/93} & {\color{red} 32/75} & { 9/19} & { 3/ 7} & {37/78} & { 3/ 7} & {19/40} & {\color{red} 37/93} \\\hline
$20$ & {14/43} && { 2/ 5} && {11/27} && { 3/ 7} && {14/31} && { 5/11} && { 5/11} && { 8/19} && { 9/22} && {24/61} && { 1/ 3} && { 2/ 5} && {\color{red} 19/47} && {10/23} && {23/51} && {24/53} && { 5/11} && { 5/11} && {34/79} && { 9/22} && {33/83} && { 2/ 5} && {12/29} && {39/89} && {32/71} && {33/73} && {34/75} && { 5/11} && { 5/11} && {27/62} &\\\hline
$21$ & { 1/ 3} & {11/23} & { 5/13} & {11/24} & { 3/ 7} & {11/25} & {13/30} & {11/26} & {10/23} & {11/27} & { 2/ 5} & { 3/ 7} & { 8/19} & {16/37} & {26/59} & {10/23} & {28/61} & {13/31} & {10/21} & { 9/23} & {21/44} & { 1/ 3} & {11/23} & {\color{red} 18/47} & {11/23} & { 3/ 7} & {33/71} & {22/51} & {33/73} & {23/53} & {11/25} & {10/23} & { 3/ 7} & {17/39} & {25/58} & { 9/20} & {13/30} & {19/41} & {10/23} & {10/21} & {36/85} & {31/65} & {\color{red}  9/23} & {32/67} & {35/89} & {11/23} & { 3/ 7} & {11/23} & {31/72} & {22/47} & {16/37} & {11/24} & {\color{red} 33/76} & {22/49} & {\color{red} 17/39} & {11/25} & {41/90} & {\color{red} 35/81} & {41/88} & {\color{red} 36/83} \\\hline
$22$ & {\color{red}  8/25} && {19/49} && {12/29} && { 5/12} && { 5/11} && {16/35} && {11/24} && {27/61} && {\color{red} 17/41} && { 5/12} && {26/67} && { 1/ 3} && {28/71} && { 7/17} && {32/75} && { 5/11} && {26/57} && {27/59} && {11/24} && {38/85} && {37/87} && { 5/12} && {36/91} && {37/93} && {\color{red} 30/73} && {42/97} && { 5/11} && {36/79} && {37/81} && {38/83} &\\\hline
$23$ & {16/49} & {12/25} & {11/28} & { 6/13} & {22/53} & { 4/ 9} & { 7/16} & { 3/ 7} & {11/25} & {12/29} & {25/59} & { 2/ 5} & {25/61} & {17/39} & { 3/ 7} & {18/41} & {29/65} & {11/25} & {31/67} & { 7/17} & {11/23} & { 2/ 5} & {23/48} & { 1/ 3} & {12/25} & {20/51} & {12/25} & { 8/19} & {36/77} & {24/55} & {36/79} & {25/57} & { 4/ 9} & {11/25} & {36/83} & { 3/ 7} & {27/62} & {19/43} & { 7/16} & { 5/11} & {29/66} & { 7/15} & {11/25} & {11/23} & {13/31} & {34/71} & { 2/ 5} & {35/73} & {\color{red} 29/74} & {12/25} & {14/33} & {12/25} & {17/39} & { 8/17} & {\color{red}  7/16} & { 6/13} & {\color{red} 18/41} & {24/53} & {\color{red} 11/25} & {\color{red} 37/85} \\\hline
$24$ & { 1/ 3} && {\color{red} 11/29} && {13/31} && {11/26} && {26/59} && {17/37} && { 6/13} && { 6/13} && {29/67} && {19/45} && {11/26} && {\color{red}  5/13} && { 1/ 3} && {30/77} && {23/55} && {\color{red}  8/19} && {37/83} && {28/61} && {29/63} && { 6/13} && { 6/13} && {41/93} && {\color{red} 30/71} && {11/26} && {13/33} && {\color{red} 35/89} && {\color{red} 33/79} && { 3/ 7} && {35/78} && {39/85} &\\\hline
$25$ & {\color{red}  9/28} & {13/27} & { 2/ 5} & {13/28} & {13/32} & {13/29} & {15/34} & {13/30} & { 4/ 9} & {13/31} & { 4/ 9} & {\color{red} 11/27} & { 2/ 5} & {14/33} & {28/67} & {19/43} & {10/23} & { 4/ 9} & {32/71} & { 4/ 9} & {34/73} & {\color{red} 11/27} & {12/25} & {15/38} & {25/52} & { 1/ 3} & {13/27} & { 2/ 5} & {13/27} & {17/41} & {39/83} & {26/59} & {39/85} & {27/61} & {13/29} & { 4/ 9} & {39/89} & { 4/ 9} & { 3/ 7} & {10/23} & {15/34} & {21/47} & {31/70} & {11/24} & { 4/ 9} & {23/49} & { 4/ 9} & {12/25} & {\color{red} 19/46} & {37/77} & {\color{red} 18/47} & {38/79} & {\color{red}  1/99} & {13/27} & {37/88} & {13/27} & {37/84} & {26/55} & {19/43} & {13/28} \\\hline
$26$ & {18/55} && {12/31} && {14/33} && { 3/ 7} && { 3/ 7} && { 6/13} && {19/41} && {13/28} && {32/71} && {\color{red} 20/47} && { 3/ 7} && { 3/ 7} && {11/28} && {\color{red} 22/67} && {\color{red} 22/57} && {25/59} && {26/61} && {39/89} && { 6/13} && {31/67} && {32/69} && {13/28} && { 5/11} && {27/62} && { 3/ 7} && { 3/ 7} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 36/85} && {\color{red} 37/87} &\\\hline
$27$ & { 1/ 3} & {14/29} & {23/59} & { 7/15} & { 7/17} & {14/31} & { 4/ 9} & { 7/16} & {17/38} & {14/33} & {13/29} & {12/29} & {29/69} & { 2/ 5} & {\color{red}  9/22} & { 4/ 9} & {31/73} & {21/47} & {11/25} & {13/29} & { 5/11} & {17/39} & {37/79} & {12/29} & {13/27} & {16/41} & {27/56} & { 1/ 3} & {14/29} & {17/43} & {14/29} & {\color{red} 25/61} & {42/89} & { 4/ 9} & { 6/13} & {29/65} & {14/31} & {30/67} & {42/95} & {13/29} & {42/97} & { 3/ 7} & { 4/ 9} & {11/25} & {33/74} & {23/51} & {17/38} & { 6/13} & {13/29} & {25/53} & {\color{red}  3/ 7} & {13/27} & {\color{red} 12/29} & {40/83} & {\color{red}  1/99} & {41/85} & {\color{red}  1/99} & {14/29} & {\color{red} 22/53} & {14/29} \\\hline
$28$ & {\color{red} 10/31} && {13/33} && { 3/ 7} && {16/37} && {13/30} && {31/69} && {20/43} && { 7/15} && { 7/15} && {34/77} && {22/51} && {13/30} && {35/83} && { 2/ 5} && { 1/ 3} && {24/61} && { 3/ 7} && {28/65} && {\color{red} 29/67} && {44/97} && {33/71} && {34/73} && { 7/15} && { 7/15} && {35/78} && {\color{red} 35/81} && {13/30} && {\color{red} 22/53} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$29$ & {20/61} & {15/31} & {\color{red} 13/34} & {15/32} & { 5/12} & { 5/11} & {29/67} & {15/34} & { 9/20} & { 3/ 7} & {14/31} & {\color{red} 18/43} & {32/73} & {13/31} & { 2/ 5} & { 8/19} & {\color{red}  5/12} & {22/49} & {34/79} & {23/51} & { 4/ 9} & {14/31} & {38/83} & { 3/ 7} & { 8/17} & {13/31} & {14/29} & {\color{red} 12/31} & {29/60} & {\color{red}  1/99} & {15/31} & { 9/23} & {15/31} & {27/65} & { 9/19} & { 7/16} & {45/97} & {31/69} & { 5/11} & {32/71} & {41/92} & {14/31} & {38/87} & {23/52} & { 3/ 7} & {23/53} & {35/78} & { 4/ 9} & { 9/20} & { 5/11} & {37/82} & {13/28} & {14/31} & { 9/19} & {\color{red}  8/19} & {14/29} & {13/31} & {43/89} & {\color{red}  1/99} & {44/91} \\\hline
$30$ & { 1/ 3} && { 2/ 5} && {28/67} && {17/39} && { 7/16} && {32/73} && { 7/15} && {22/47} && {15/32} && {37/81} && {\color{red} 23/53} && {24/55} && { 7/16} && {37/89} && {36/91} && {\color{red}  1/99} && { 2/ 5} && {41/97} && {10/23} && {\color{red} 31/71} && {25/56} && { 7/15} && {36/77} && {37/79} && {15/32} && {\color{red} 22/49} && {\color{red} 37/85} && {\color{red} 38/87} && { 7/16} && {\color{red} 13/32} &\\\hline
$31$ & {\color{red} 11/34} & {16/33} & { 7/18} & { 8/17} & { 8/19} & {16/35} & {\color{red} 14/33} & { 4/ 9} & {19/42} & {16/37} & { 5/11} & {\color{red} 19/45} & { 5/11} & {14/33} & {33/79} & { 2/ 5} & {\color{red} 21/50} & {18/41} & {\color{red} 11/26} & {24/53} & {37/85} & { 5/11} & {13/29} & { 5/11} & {41/89} & {\color{red} 25/59} & {43/91} & {14/33} & {15/31} & {13/33} & {31/64} & {\color{red}  1/99} & {16/33} & {\color{red} 26/67} & {16/33} & {29/69} & {29/61} & {22/51} & {41/88} & {33/73} & {16/35} & {34/75} & {35/78} & { 5/11} & {37/84} & { 5/11} & {16/37} & { 3/ 7} & {\color{red} 18/41} & {25/57} & {19/42} & {13/29} & {39/86} & {27/59} & { 5/11} & { 7/15} & { 5/11} & {29/61} & {\color{red}  3/ 7} & {15/31} \\\hline
$32$ & {22/67} && { 9/23} && {\color{red} 16/39} && {18/41} && {15/34} && { 3/ 7} && {36/79} && {23/49} && { 8/17} && { 8/17} && {13/29} && {25/57} && {26/59} && {15/34} && {\color{red}  7/17} && {38/97} && {\color{red}  1/99} && {\color{red}  9/23} && {38/91} && {32/73} && {11/25} && {\color{red} 15/34} && {17/37} && {38/81} && {39/83} && { 8/17} && { 8/17} && {\color{red} 33/73} && {\color{red} 40/91} && {41/93} &\\\hline
$33$ & { 1/ 3} & {17/35} & {15/38} & {17/36} & {17/40} & {17/37} & { 3/ 7} & {17/38} & { 5/11} & {17/39} & {21/46} & {\color{red} 20/47} & {16/35} & { 3/ 7} & {36/83} & { 3/ 7} & { 2/ 5} & {18/43} & {\color{red} 23/54} & { 5/11} & { 3/ 7} & {26/57} & {40/91} & {16/35} & {14/31} & {21/47} & {44/95} & { 3/ 7} & {46/97} & { 3/ 7} & {16/33} & { 2/ 5} & {33/68} & {\color{red}  1/99} & {17/35} & {\color{red} 28/71} & {17/35} & {31/73} & {41/86} & {\color{red} 32/75} & {29/62} & { 5/11} & {17/37} & {36/79} & {37/82} & {37/81} & {43/97} & {16/35} & {\color{red}  3/ 7} & {\color{red} 20/47} & { 3/ 7} & {\color{red} 38/89} & { 5/11} & {27/61} & {41/90} & {14/31} & {21/46} & {\color{red} 43/95} & {16/35} & {\color{red} 44/95} \\\hline
$34$ & {\color{red} 12/37} && {\color{red}  5/13} && {17/41} && {19/43} && { 4/ 9} && { 4/ 9} && {37/83} && { 8/17} && {25/53} && {17/36} && { 6/13} && {41/93} && {27/61} && { 4/ 9} && { 4/ 9} && { 5/12} && {\color{red}  7/18} && {\color{red}  1/99} && {\color{red}  7/18} && {\color{red} 31/75} && {34/77} && {35/79} && { 4/ 9} && {29/64} && { 8/17} && {41/87} && {42/89} && {17/36} && {\color{red}  5/11} && {\color{red} 42/95} &\\\hline
$35$ & {24/73} & {18/37} & { 2/ 5} & { 9/19} & { 3/ 7} & { 6/13} & {19/44} & { 9/20} & { 4/ 9} & {18/41} & {11/24} & { 3/ 7} & {17/37} & {22/51} & {13/29} & {16/37} & {37/89} & { 2/ 5} & { 3/ 7} & {10/23} & {\color{red} 25/58} & {27/59} & {\color{red} 16/37} & {28/61} & {43/97} & {17/37} & { 5/11} & {11/25} & {27/58} & {16/37} & {39/82} & {\color{red} 40/97} & {17/35} & {\color{red} 22/57} & {35/72} & {\color{red}  1/99} & {18/37} & { 2/ 5} & {18/37} & { 3/ 7} & {43/90} & {\color{red} 34/79} & {31/66} & {13/29} & {\color{red} 18/41} & {38/83} & {44/97} & {39/85} & {\color{red} 37/86} & {17/37} & {\color{red} 19/44} & {\color{red} 11/25} & {\color{red} 11/26} & { 3/ 7} & {\color{red} 10/23} & {\color{red} 41/95} & {43/94} & {\color{red} 43/97} & {11/24} & { 5/11} \\\hline
$36$ & { 1/ 3} && {16/41} && {18/43} && { 4/ 9} && {21/47} && {17/38} && {38/87} && {41/89} && {26/55} && { 9/19} && { 9/19} && {44/97} && { 4/ 9} && {29/65} && {17/38} && {39/89} && { 8/19} && {15/38} && {\color{red}  1/99} && {\color{red} 30/77} && {\color{red} 33/79} && { 4/ 9} && {37/83} && {38/85} && {\color{red} 39/89} && {\color{red} 41/89} && {43/91} && {44/93} && { 9/19} && {\color{red} 44/97} &\\\hline
$37$ & {\color{red} 13/40} & {19/39} & {31/79} & {19/40} & {34/81} & {19/41} & {10/23} & {19/42} & {\color{red} 17/39} & {19/43} & {23/50} & {19/44} & { 6/13} & {23/53} & { 6/13} & {17/39} & {40/93} & {20/47} & { 2/ 5} & { 5/12} & {13/30} & {22/49} & {\color{red} 27/62} & {29/63} & {\color{red} 17/39} & { 6/13} & {25/56} & { 6/13} & {16/35} & {\color{red} 10/23} & {43/92} & {17/39} & {31/65} & {\color{red} 16/39} & {18/37} & {\color{red}  5/13} & {37/76} & {\color{red}  1/99} & {19/39} & {\color{red}  1/99} & {19/39} & {\color{red} 34/81} & {34/71} & {36/83} & {\color{red} 19/42} & {\color{red} 37/85} & {\color{red} 19/43} & {40/87} & {\color{red} 19/44} & {41/89} & {\color{red} 13/30} & { 6/13} & {\color{red} 10/23} & { 6/13} & {\color{red} 27/62} & {\color{red} 23/53} & {\color{red} 27/64} & {\color{red} 42/97} & {\color{red} 22/49} & {\color{red} 27/62} \\\hline
$38$ & {26/79} && {17/43} && {19/45} && {37/85} && {22/49} && { 9/20} && { 3/ 7} && {14/31} && { 9/19} && {28/59} && {19/40} && {27/58} && {25/56} && {30/67} && {31/69} && { 9/20} && {\color{red}  3/ 7} && {17/40} && {\color{red} 25/77} && {\color{red}  1/99} && {\color{red}  1/99} && {35/83} && {\color{red} 37/85} && {13/29} && {40/89} && { 9/20} && {\color{red} 41/90} && { 9/19} && {46/97} && {47/99} &\\\hline
$39$ & { 1/ 3} & {20/41} & {\color{red} 17/44} & {10/21} & {\color{red} 19/46} & {20/43} & { 7/16} & { 5/11} & {18/41} & { 4/ 9} & { 6/13} & {10/23} & {25/54} & {24/55} & {19/41} & {25/57} & {43/97} & {18/41} & {\color{red} 17/41} & { 2/ 5} & {23/54} & {22/51} & { 7/16} & { 6/13} & {18/41} & {31/67} & {29/66} & {19/41} & {40/89} & { 5/11} & {17/37} & {32/73} & {38/81} & {18/41} & {11/23} & {\color{red} 17/41} & {19/39} & {\color{red}  1/99} & {39/80} & {\color{red}  1/99} & {20/41} & {\color{red}  1/99} & {20/41} & {\color{red}  7/17} & {\color{red} 20/43} & {38/87} & {\color{red}  5/11} & {\color{red} 39/89} & {\color{red}  4/ 9} & { 6/13} & {\color{red} 10/23} & {43/93} & {\color{red} 41/94} & {44/95} & {\color{red}  7/16} & {\color{red} 43/97} & {\color{red} 43/98} & {\color{red} 24/55} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$40$ & {\color{red} 14/43} && { 2/ 5} && {20/47} && { 3/ 7} && {23/51} && {19/42} && {42/95} && {43/97} && {46/99} && {29/61} && {10/21} && {10/21} && {38/83} && {37/84} && {32/71} && {33/73} && {19/42} && { 3/ 7} && { 3/ 7} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {37/87} && {\color{red} 25/58} && {41/91} && {14/31} && {\color{red} 33/73} && {\color{red} 43/97} && {\color{red} 46/99} && {29/61} &\\\hline
$41$ & {28/85} & {21/43} & { 9/23} & {21/44} & { 5/12} & { 7/15} & {11/25} & {21/46} & {19/43} & {21/47} & {43/95} & { 7/16} & {13/28} & { 3/ 7} & {20/43} & {26/59} & {41/90} & {19/43} & {41/96} & {11/26} & { 2/ 5} & {\color{red} 27/65} & {29/66} & { 4/ 9} & {15/34} & {32/69} & {19/43} & {33/71} & {27/61} & {20/43} & {33/73} & {\color{red} 11/25} & { 6/13} & {34/77} & {\color{red} 37/80} & {19/43} & {35/73} & {18/43} & {20/41} & {\color{red}  1/99} & {41/84} & {\color{red}  1/99} & {21/43} & {\color{red}  1/99} & {\color{red} 21/44} & {\color{red} 37/89} & {\color{red}  7/15} & {40/91} & {\color{red} 21/46} & {\color{red} 41/93} & {\color{red} 21/47} & {\color{red} 43/95} & {\color{red}  7/16} & {45/97} & {\color{red}  3/ 7} & {46/99} & {\color{red} 11/25} & {\color{red} 33/71} & {\color{red} 15/34} & {\color{red} 13/29} \\\hline
$42$ & { 1/ 3} && {35/89} && { 3/ 7} && {22/51} && {24/53} && { 5/11} && { 5/11} && {27/62} && {26/57} && {10/21} && {31/65} && {21/44} && {37/79} && {37/82} && {43/97} && {34/75} && { 5/11} && { 5/11} && {19/44} && {\color{red} 27/65} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && { 3/ 7} && {\color{red} 40/93} && {43/95} && {44/97} && { 5/11} && {\color{red} 27/62} && {\color{red} 26/57} &\\\hline
$43$ & {\color{red} 15/46} & {22/45} & {19/48} & {11/23} & {21/50} & {22/47} & {23/52} & {11/24} & { 4/ 9} & {22/49} & { 4/ 9} & {11/25} & {27/58} & {22/51} & { 7/15} & {27/61} & { 7/15} & { 4/ 9} & {29/66} & { 4/ 9} & {19/45} & { 2/ 5} & {36/85} & { 3/ 7} & {31/70} & {26/57} & { 4/ 9} & {34/73} & { 4/ 9} & { 7/15} & {41/92} & { 7/15} & {\color{red}  9/20} & {\color{red} 35/79} & {19/41} & { 4/ 9} & {\color{red} 13/28} & { 4/ 9} & {\color{red} 10/21} & {19/45} & {21/43} & {\color{red}  1/99} & {43/88} & {\color{red}  1/99} & {22/45} & {\color{red}  1/99} & {\color{red} 11/23} & {\color{red}  1/99} & {\color{red} 22/47} & {42/95} & {\color{red} 11/24} & {43/97} & {\color{red} 22/49} & {\color{red}  4/ 9} & {\color{red} 11/25} & {27/58} & {\color{red} 22/51} & {41/88} & {\color{red} 23/52} & { 7/15} \\\hline
$44$ & {30/91} && {\color{red} 19/49} && { 8/19} && {23/53} && { 5/11} && {26/57} && {21/46} && { 3/ 7} && {35/78} && {29/62} && {32/67} && {11/23} && {11/23} && {\color{red} 43/94} && {\color{red}  7/16} && { 5/11} && {36/79} && {21/46} && {\color{red} 10/23} && {10/23} && {\color{red}  5/12} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  8/19} && {\color{red} 42/97} && { 5/11} && {41/90} && {26/57} && {\color{red} 40/91} &\\\hline
$45$ & { 1/ 3} & {23/47} & { 2/ 5} & {23/48} & {11/26} & {23/49} & { 4/ 9} & {23/50} & {25/56} & {23/51} & {21/47} & {23/52} & { 7/15} & {23/53} & {29/62} & { 4/ 9} & {22/47} & {29/65} & {41/91} & {21/47} & {\color{red} 20/47} & { 8/19} & { 2/ 5} & {\color{red} 30/71} & { 4/ 9} & {26/59} & {33/74} & { 7/15} & {21/47} & {36/77} & {18/41} & {22/47} & {43/96} & {\color{red} 21/47} & {\color{red} 19/42} & {37/83} & {20/43} & {21/47} & {\color{red} 41/88} & {\color{red} 28/65} & {\color{red} 21/44} & {20/47} & {22/45} & {\color{red}  1/99} & {45/92} & {\color{red}  1/99} & {23/47} & {\color{red}  1/99} & {\color{red} 23/48} & {\color{red}  1/99} & {\color{red} 23/49} & { 4/ 9} & {\color{red} 23/50} & {41/92} & {\color{red} 23/51} & {\color{red} 25/56} & {\color{red} 23/52} & { 7/15} & {\color{red} 23/53} & {43/92} \\\hline
$46$ & {\color{red} 16/49} && {20/51} && {\color{red} 22/53} && {24/55} && {25/56} && {27/59} && {11/24} && {37/84} && {34/77} && {29/63} && {11/23} && {34/71} && {23/48} && {41/87} && {\color{red} 22/49} && {11/25} && {37/81} && {38/83} && {11/24} && {\color{red} 37/84} && { 7/16} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {27/62} && {\color{red} 25/56} && {16/35} && {38/83} &\\\hline
$47$ & {\color{red}  8/25} & {24/49} & {13/33} & {12/25} & {23/54} & { 8/17} & {38/87} & { 6/13} & {13/29} & {24/53} & {22/49} & { 4/ 9} & {39/85} & {24/55} & {15/32} & { 3/ 7} & {23/49} & {30/67} & {41/89} & {22/49} & {17/39} & {26/59} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 23/56} & {\color{red} 32/75} & {17/38} & {\color{red} 34/77} & {35/78} & {37/79} & {22/49} & {38/81} & {19/43} & {23/49} & {\color{red} 39/88} & {\color{red} 38/85} & {\color{red}  5/11} & {13/29} & { 7/15} & {22/49} & {\color{red} 43/92} & {\color{red}  3/ 7} & {\color{red} 11/23} & { 3/ 7} & {23/47} & {\color{red}  1/99} & {47/96} & {\color{red}  1/99} & {24/49} & {\color{red}  1/99} & {\color{red} 12/25} & {\color{red}  1/99} & {\color{red}  8/17} & {\color{red} 38/87} & {\color{red}  6/13} & {30/67} & {\color{red} 24/53} & {\color{red} 35/78} & {\color{red}  4/ 9} & {\color{red} 39/85} \\\hline
$48$ & { 1/ 3} && {21/53} && {23/55} && {25/57} && {\color{red} 11/25} && {28/61} && {23/50} && {37/82} && {10/23} && {29/64} && { 8/17} && {35/73} && {12/25} && {12/25} && {\color{red} 41/89} && {\color{red} 23/52} && {\color{red} 29/66} && {39/85} && {40/87} && {23/50} && {\color{red} 40/91} && {11/25} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 29/66} && {39/85} &\\\hline
$49$ & {\color{red} 17/52} & {25/51} & {\color{red}  7/18} & {25/52} & { 3/ 7} & {25/53} & {\color{red} 25/58} & {25/54} & { 9/20} & { 5/11} & {23/51} & {25/56} & {37/82} & {25/57} & {31/66} & {\color{red} 22/51} & { 8/17} & {31/69} & { 8/17} & {32/71} & {29/65} & {23/51} & {\color{red} 22/51} & {13/31} & {\color{red}  1/99} & { 3/ 7} & {41/93} & { 7/16} & { 9/20} & {\color{red} 37/81} & {23/51} & {39/83} & {43/97} & { 8/17} & { 4/ 9} & { 8/17} & {\color{red} 41/92} & {\color{red} 40/89} & {\color{red} 21/46} & {41/91} & {22/47} & {23/51} & {\color{red} 15/32} & {\color{red} 22/51} & {\color{red} 23/48} & {\color{red}  1/99} & {24/49} & {\color{red}  1/99} & {25/51} & {\color{red}  1/99} & {25/51} & {\color{red}  1/99} & {\color{red} 25/52} & {\color{red}  1/99} & {\color{red} 25/53} & {\color{red}  1/99} & {\color{red} 25/54} & {40/89} & {\color{red}  5/11} & {41/91} \\\hline
$50$ & {\color{red} 17/53} && { 2/ 5} && { 8/19} && {26/59} && {23/52} && {29/63} && { 6/13} && { 6/13} && {\color{red} 30/71} && {29/65} && {\color{red} 45/98} && {12/25} && {37/77} && {25/52} && {\color{red} 43/93} && {\color{red} 24/53} && { 4/ 9} && {\color{red} 13/29} && {41/89} && { 6/13} && { 6/13} && {42/95} && {23/52} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & { 1/ 3} & {26/53} & {11/28} & {13/27} & {27/64} & {26/55} & {13/30} & {13/28} & {14/31} & {26/57} & {24/53} & {13/29} & { 4/ 9} & {26/59} & { 8/17} & {\color{red} 23/53} & {33/70} & {27/61} & {25/53} & {33/73} & {\color{red} 40/89} & {24/53} & {\color{red} 23/53} & {\color{red} 18/43} & {\color{red} 22/53} & {\color{red}  1/99} & {\color{red} 29/70} & {\color{red} 35/81} & {37/82} & {\color{red}  4/ 9} & {19/42} & { 8/17} & {\color{red} 43/95} & {41/87} & {\color{red} 10/23} & {25/53} & {21/47} & {\color{red} 31/68} & {\color{red} 43/96} & {14/31} & {\color{red} 11/24} & {43/95} & {23/49} & {24/53} & {\color{red} 39/83} & {\color{red}  1/99} & {\color{red} 12/25} & {\color{red}  1/99} & {25/51} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {\color{red} 13/27} & {\color{red}  1/99} & {\color{red} 26/55} & {\color{red}  1/99} & {\color{red} 13/28} & {37/82} \\\hline
$52$ & {\color{red} 18/55} && {28/71} && {25/59} && {27/61} && { 4/ 9} && { 6/13} && {31/67} && {25/54} && {18/41} && {11/25} && {37/81} && {\color{red} 36/77} && {38/79} && {13/27} && {13/27} && {\color{red} 32/69} && {\color{red} 25/56} && {\color{red} 40/93} && { 6/13} && {43/93} && {25/54} && {\color{red}  4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & {\color{red}  9/28} & {27/55} & {23/58} & {27/56} & {\color{red}  5/12} & { 9/19} & {27/62} & {27/58} & {29/64} & {27/59} & { 5/11} & { 9/20} & { 5/11} & {27/61} & {19/41} & {\color{red} 24/55} & {17/36} & { 3/ 7} & {26/55} & {34/75} & {\color{red}  5/11} & { 5/11} & {\color{red}  7/16} & { 5/11} & {24/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/95} & {\color{red} 37/85} & {39/86} & {\color{red} 13/29} & { 5/11} & {42/89} & { 5/11} & {43/91} & {\color{red}  7/16} & {26/55} & {22/49} & {\color{red} 25/56} & {\color{red}  9/20} & {44/97} & {\color{red} 23/50} & { 5/11} & { 8/17} & { 5/11} & {\color{red} 41/87} & {\color{red}  1/99} & {\color{red} 25/52} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {\color{red} 27/56} & {\color{red}  1/99} & {\color{red}  9/19} & {\color{red}  1/99} \\\hline
$54$ & { 1/ 3} && {\color{red} 23/59} && {26/61} && { 4/ 9} && {29/65} && {\color{red} 30/67} && {32/69} && {13/28} && {\color{red}  4/ 9} && {\color{red}  3/ 7} && {\color{red} 35/79} && {\color{red} 43/93} && {13/27} && {40/83} && {27/56} && {\color{red} 33/71} && {\color{red} 26/57} && {\color{red}  3/ 7} && {\color{red} 35/81} && {44/95} && {45/97} && {13/28} && {\color{red} 35/78} && {25/56} && {\color{red}  3/ 7} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & {\color{red} 19/58} & {\color{red} 27/56} & { 2/ 5} & {\color{red} 28/61} & {13/31} & {28/59} & { 7/16} & {\color{red} 27/59} & { 5/11} & {28/61} & {31/68} & {14/31} & {26/57} & {\color{red} 31/71} & {37/81} & {\color{red} 32/73} & {35/74} & {\color{red} 25/57} & { 9/19} & { 5/11} & { 9/19} & {36/79} & {\color{red} 13/29} & {26/57} & {\color{red} 25/57} & {10/23} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {38/87} & { 5/11} & { 4/ 9} & {41/90} & {\color{red}  6/13} & {26/57} & {44/93} & {\color{red} 38/87} & { 9/19} & {\color{red} 11/25} & { 9/19} & {23/51} & { 5/11} & {\color{red} 33/73} & {41/90} & {\color{red}  6/13} & {26/57} & {25/53} & {\color{red} 25/57} & {\color{red} 17/36} & {\color{red}  1/99} & {\color{red} 13/27} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & {\color{red} 14/29} & {\color{red}  1/99} \\\hline
$56$ & {\color{red} 19/59} && {24/61} && { 3/ 7} && {39/89} && {30/67} && {\color{red} 13/29} && {33/71} && {27/58} && {\color{red} 13/29} && { 3/ 7} && { 4/ 9} && {\color{red} 37/83} && {\color{red} 39/83} && {41/85} && {14/29} && {14/29} && {\color{red} 41/88} && {\color{red}  9/20} && {\color{red} 43/99} && {\color{red} 43/96} && {46/99} && {27/58} && {27/58} && {\color{red} 30/67} && {13/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & {\color{red}  1/99} & {\color{red} 14/29} & {32/81} & {\color{red} 29/63} & {27/64} & {29/61} & {29/66} & {29/62} & {43/96} & {29/63} & {16/35} & {29/64} & {27/59} & {29/65} & {41/91} & {\color{red} 11/25} & { 9/19} & {\color{red} 37/84} & {37/78} & {\color{red} 35/81} & {28/59} & {37/81} & {\color{red}  5/11} & {27/59} & {\color{red} 37/84} & {\color{red} 26/59} & {\color{red} 25/58} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/45} & {\color{red} 40/91} & {21/46} & {\color{red} 25/56} & {43/94} & { 9/19} & {\color{red} 29/66} & {46/97} & {\color{red} 43/98} & {28/59} & {\color{red} 23/52} & {\color{red} 35/76} & {24/53} & {26/57} & {\color{red} 44/97} & {16/35} & {\color{red} 25/54} & {27/59} & {26/55} & {\color{red} 37/84} & {\color{red} 44/93} & {\color{red}  1/99} & {\color{red} 27/56} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} \\\hline
$58$ & {\color{red}  1/99} && {25/63} && {\color{red} 27/65} && {\color{red} 29/67} && {31/69} && { 9/20} && {34/73} && { 7/15} && { 7/15} && {\color{red} 43/99} && {\color{red} 36/83} && {\color{red} 38/85} && {\color{red} 33/71} && {14/29} && {43/89} && {29/60} && {\color{red} 43/92} && {\color{red} 41/95} && {14/31} && {\color{red}  1/99} && {\color{red} 41/90} && {41/88} && { 7/15} && { 7/15} && {40/89} && { 9/20} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & {\color{red}  1/99} & {\color{red} 10/21} & {\color{red} 25/64} & {\color{red}  6/13} & {14/33} & {\color{red} 30/67} & {15/34} & {\color{red} 10/23} & {\color{red} 27/61} & {\color{red} 30/71} & {11/24} & {\color{red} 31/73} & {28/61} & {\color{red} 26/61} & {\color{red} 43/98} & {\color{red} 34/77} & {\color{red}  6/13} & {\color{red} 27/61} & {19/40} & {\color{red}  9/22} & {29/61} & {38/83} & {\color{red} 28/61} & {39/85} & {\color{red} 19/43} & {\color{red} 40/89} & {\color{red} 27/61} & {\color{red} 23/54} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {41/93} & {\color{red} 21/47} & {\color{red} 42/95} & {11/24} & {\color{red} 44/97} & {28/61} & {47/99} & {\color{red} 27/61} & {29/61} & {\color{red}  1/99} & {29/61} & {\color{red}  4/ 9} & {\color{red} 14/31} & { 5/11} & {38/83} & {\color{red} 41/90} & {39/85} & {\color{red} 13/28} & {\color{red} 34/77} & { 9/19} & {\color{red}  1/99} & {\color{red} 46/97} & {\color{red}  1/99} & {\color{red} 14/29} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {30/61} & {\color{red}  1/99} \\\hline
$60$ & {\color{red}  1/99} && { 2/ 5} && {\color{red} 28/67} && {10/23} && {32/71} && {14/31} && { 7/15} && {36/77} && {\color{red} 39/85} && {21/47} && {\color{red} 36/83} && {13/29} && {\color{red} 27/59} && {\color{red} 42/89} && {44/91} && {15/31} && {15/31} && {\color{red} 37/79} && {\color{red} 43/99} && {\color{red} 37/85} && {\color{red}  1/99} && { 7/15} && {43/92} && {29/62} && {\color{red} 14/31} && {37/82} && {\color{red} 10/23} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 1+k, 1+k+i\}$.
\end{center}


==> tables/table-g3-a02.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 2/ 5} & { 2/ 5} & { 4/11} & { 1/ 3} & { 5/14} & { 2/ 5} & { 2/ 5} & { 3/ 8} & { 6/17} & { 7/19} & { 2/ 5} & { 2/ 5} & { 8/21} & { 4/11} & { 3/ 8} & { 2/ 5} & { 2/ 5} & { 5/13} & {10/27} & {11/29} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & {13/34} & { 2/ 5} & { 2/ 5} & { 7/18} & {14/37} & { 5/13} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {17/44} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & {19/49} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & { 7/18} & { 2/ 5} & { 2/ 5} & {11/28} & {22/57} & {23/59} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & {25/64} & { 2/ 5} & { 2/ 5} \\\hline
$2$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$3$ & { 4/11} & { 1/ 3} & { 2/ 5} & { 3/ 7} & { 1/ 3} & { 5/13} & { 3/ 7} & { 7/18} & { 3/ 8} & { 7/17} & { 3/ 7} & { 7/19} & { 2/ 5} & { 3/ 7} & { 2/ 5} & { 9/23} & { 5/12} & { 3/ 7} & { 5/13} & {11/27} & { 3/ 7} & {13/32} & { 2/ 5} & {13/31} & { 3/ 7} & {13/33} & { 7/17} & { 3/ 7} & {16/39} & {15/37} & { 8/19} & { 3/ 7} & { 2/ 5} & {17/41} & { 3/ 7} & {19/46} & { 9/22} & {19/45} & { 3/ 7} & {19/47} & { 5/12} & { 3/ 7} & {22/53} & { 7/17} & {11/26} & { 3/ 7} & {\color{red} 11/27} & {23/55} & { 3/ 7} & { 5/12} & {12/29} & {25/59} & { 3/ 7} & {\color{red} 25/61} & {13/31} & { 3/ 7} & {28/67} & {27/65} & {14/33} & { 3/ 7} \\\hline
$4$ & { 5/13} && { 2/ 5} && { 7/17} && { 8/19} && { 3/ 7} && {10/23} && {11/25} && { 4/ 9} && {13/29} && {14/31} && { 5/11} && {16/35} && {17/37} && { 6/13} && {19/41} && {20/43} && { 7/15} && {22/47} && {23/49} && { 8/17} && {25/53} && {26/55} && { 9/19} && {28/59} && {29/61} && {10/21} && {31/65} && {32/67} && {11/23} && {34/71} &\\\hline
$5$ & { 2/ 5} & { 5/16} & { 6/17} & { 4/ 9} & { 3/ 7} & { 2/ 5} & { 1/ 3} & { 9/22} & { 4/ 9} & { 8/19} & { 2/ 5} & { 5/13} & { 4/ 9} & {10/23} & { 5/12} & { 2/ 5} & {13/31} & { 4/ 9} & { 3/ 7} & {12/29} & { 2/ 5} & { 4/ 9} & { 7/16} & {14/33} & { 7/17} & {17/40} & { 4/ 9} & {16/37} & { 8/19} & {\color{red} 16/39} & { 4/ 9} & {18/41} & { 3/ 7} & {18/43} & { 3/ 7} & { 4/ 9} & {10/23} & {20/47} & {\color{red}  5/12} & { 4/ 9} & {11/25} & {22/51} & {11/26} & {25/58} & { 4/ 9} & {24/55} & { 3/ 7} & {\color{red}  8/19} & { 4/ 9} & {26/59} & {13/30} & {26/61} & {29/67} & { 4/ 9} & { 7/16} & {28/65} & {\color{red} 14/33} & { 4/ 9} & {15/34} & {10/23} \\\hline
$6$ & { 4/11} && { 5/13} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 8/21} && { 9/23} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {12/31} && {13/33} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {16/41} && {17/43} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {20/51} && {21/53} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {24/61} && {25/63} && { 2/ 5} && { 2/ 5} && { 2/ 5} &\\\hline
$7$ & { 7/19} & { 4/13} & { 3/ 7} & { 5/11} & { 4/11} & { 3/ 8} & { 4/ 9} & {11/26} & { 1/ 3} & { 3/ 7} & { 5/11} & { 2/ 5} & {12/31} & {11/25} & { 5/11} & {13/34} & { 3/ 7} & {13/29} & {16/37} & {15/38} & { 7/16} & { 5/11} & {17/41} & { 3/ 7} & { 4/ 9} & { 5/11} & { 2/ 5} & {17/39} & { 9/20} & { 7/16} & { 3/ 7} & {19/43} & { 5/11} & {11/26} & {10/23} & {21/47} & { 5/11} & { 3/ 7} & {11/25} & {23/51} & {26/59} & {23/53} & { 4/ 9} & { 5/11} & { 3/ 7} & {25/57} & {13/29} & { 5/11} & {13/30} & {27/61} & {14/31} & {31/70} & { 7/16} & {29/65} & { 5/11} & {\color{red} 29/67} & {15/34} & {31/69} & { 5/11} & {\color{red} 31/71} \\\hline
$8$ & { 8/21} && { 9/23} && { 2/ 5} && {11/27} && {12/29} && {13/31} && {14/33} && { 3/ 7} && {16/37} && {17/39} && {18/41} && {19/43} && { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && {31/67} && {32/69} && {33/71} && {34/73} && { 7/15} && {36/77} && {37/79} &\\\hline
$9$ & { 9/23} & { 1/ 3} & { 3/ 8} & { 6/13} & { 4/ 9} & { 7/19} & { 5/13} & {13/30} & { 5/11} & {13/32} & { 1/ 3} & { 7/17} & { 6/13} & { 4/ 9} & {14/37} & {15/38} & { 6/13} & {14/31} & {17/41} & { 5/13} & {19/43} & {16/35} & { 4/ 9} & { 9/23} & {20/47} & { 6/13} & { 9/20} & {21/50} & { 7/17} & { 6/13} & { 5/11} & { 4/ 9} & { 2/ 5} & {25/56} & {11/24} & {22/49} & {25/59} & {13/30} & { 6/13} & {24/53} & { 4/ 9} & {27/64} & { 6/13} & {26/57} & {13/29} & {29/68} & {31/69} & {28/61} & {14/31} & { 4/ 9} & {32/73} & { 6/13} & { 5/11} & {30/67} & { 3/ 7} & { 6/13} & {16/35} & {32/71} & { 4/ 9} & {37/82} \\\hline
$10$ & { 2/ 5} && { 7/17} && { 8/19} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {11/27} && {12/29} && {13/31} && {14/33} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 29/69} && {30/71} && {31/73} &\\\hline
$11$ & { 3/ 8} & { 9/28} & {12/29} & { 7/15} & { 2/ 5} & { 8/21} & { 5/11} & {15/34} & { 2/ 5} & { 2/ 5} & { 6/13} & { 8/19} & { 1/ 3} & {17/40} & { 7/15} & {17/42} & { 3/ 8} & { 5/11} & { 7/15} & { 2/ 5} & {19/47} & {17/37} & {22/49} & { 2/ 5} & {22/51} & {19/41} & {23/53} & { 7/18} & { 5/11} & { 7/15} & { 8/19} & {12/29} & {11/24} & { 7/15} & {25/61} & {27/62} & { 6/13} & {29/64} & { 2/ 5} & { 5/11} & {13/28} & {15/34} & {29/69} & {27/59} & { 7/15} & {31/72} & {32/73} & {29/63} & { 7/15} & { 8/19} & { 5/11} & {31/67} & {36/79} & {17/40} & {16/35} & {33/71} & {37/83} & {37/84} & {17/37} & { 7/15} \\\hline
$12$ & {11/29} && {12/31} && {13/33} && { 2/ 5} && {15/37} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} && {34/75} && { 5/11} && {36/79} && {37/81} && {38/83} && {39/85} && {40/87} &\\\hline
$13$ & {12/31} & { 6/19} & { 2/ 5} & { 8/17} & { 3/ 7} & { 9/23} & { 7/17} & {17/38} & { 6/13} & {11/27} & {16/41} & { 3/ 7} & { 7/15} & { 7/17} & { 1/ 3} & {19/46} & { 8/17} & { 7/16} & { 7/18} & {15/37} & { 8/17} & { 6/13} & { 2/ 5} & { 7/17} & { 5/11} & {20/43} & { 8/19} & {23/58} & {26/59} & {22/47} & {27/61} & {\color{red} 19/49} & { 3/ 7} & { 8/17} & { 6/13} & { 9/22} & {28/67} & { 8/17} & {13/28} & { 3/ 7} & { 7/17} & {11/24} & { 7/15} & {33/74} & { 2/ 5} & {17/38} & {15/32} & { 6/13} & {33/79} & { 7/16} & { 8/17} & {32/69} & {36/83} & { 3/ 7} & { 8/17} & {34/73} & {13/29} & {37/88} & {41/89} & {36/77} \\\hline
$14$ & {13/33} && { 3/ 7} && {10/23} && {11/25} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {20/47} && { 3/ 7} && {16/37} && {17/39} && {18/41} && {19/43} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 10/23} && {31/71} && {32/73} && {11/25} && {34/77} &\\\hline
$15$ & { 2/ 5} & { 1/ 3} & {15/37} & { 9/19} & { 5/12} & { 2/ 5} & {18/41} & {19/42} & { 8/19} & {12/29} & { 7/15} & {10/23} & {18/47} & { 8/19} & { 8/17} & {21/50} & { 1/ 3} & {11/26} & { 9/19} & {\color{red} 16/39} & { 2/ 5} & {25/56} & { 9/19} & {18/43} & { 9/22} & { 7/15} & {28/61} & { 8/19} & { 5/12} & {23/49} & {29/65} & {13/33} & {29/67} & {25/53} & {10/23} & { 2/ 5} & {32/71} & { 9/19} & {31/73} & {\color{red} 24/59} & { 7/15} & { 9/19} & {\color{red} 13/31} & {11/26} & {15/32} & {37/80} & { 8/19} & {18/41} & { 8/17} & {19/42} & { 2/ 5} & {39/86} & {17/36} & {39/88} & {37/89} & { 7/15} & { 9/19} & {10/23} & {40/93} & {37/79} \\\hline
$16$ & { 8/21} && { 9/23} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && {22/53} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} && {35/79} && { 4/ 9} && {37/83} && {38/85} && {13/29} && {40/89} && {41/91} && {14/31} && {43/95} &\\\hline
$17$ & { 5/13} & {13/40} & { 5/12} & {10/21} & {18/43} & {17/44} & { 3/ 7} & {21/46} & {21/47} & {13/31} & { 3/ 7} & {11/25} & { 8/17} & { 3/ 7} & { 8/21} & {23/54} & { 9/19} & { 3/ 7} & { 1/ 3} & {\color{red} 17/41} & {10/21} & {13/30} & {24/61} & {19/45} & {10/21} & {29/64} & { 5/12} & { 3/ 7} & {31/67} & { 8/17} & {11/26} & { 3/ 7} & {32/71} & {26/55} & { 3/ 7} & {29/74} & {11/25} & {28/59} & {34/77} & {31/78} & {34/79} & {10/21} & {37/81} & {\color{red} 27/65} & {\color{red} 14/33} & {10/21} & { 8/17} & {\color{red} 29/69} & { 3/ 7} & {41/88} & {17/36} & {13/30} & { 3/ 7} & {21/46} & { 9/19} & {21/47} & { 2/ 5} & {43/96} & {19/40} & {45/98} \\\hline
$18$ & {16/41} && {18/43} && { 4/ 9} && {13/29} && {14/31} && { 5/11} && { 5/11} && { 5/11} && {25/57} && {25/59} && {26/61} && { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && { 5/11} && { 5/11} && {35/79} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} && {34/75} && { 5/11} && { 5/11} && { 5/11} &\\\hline
$19$ & {17/43} & { 8/25} & { 2/ 5} & {11/23} & { 3/ 7} & {11/29} & { 3/ 7} & {23/50} & {10/23} & {14/33} & {24/53} & { 4/ 9} & {23/55} & {16/37} & { 9/19} & {25/58} & { 9/23} & {10/23} & {10/21} & {13/31} & { 1/ 3} & {27/64} & {11/23} & {20/47} & {26/67} & {15/34} & {11/23} & {22/51} & {11/26} & {11/24} & {34/73} & {10/23} & { 3/ 7} & { 9/19} & { 5/11} & {11/26} & {13/30} & {29/61} & { 4/ 9} & {\color{red}  9/23} & {\color{red} 10/23} & {31/65} & {37/85} & {17/43} & {13/29} & {11/23} & {\color{red}  3/ 7} & {\color{red} 30/71} & { 6/13} & {11/23} & {\color{red} 16/37} & {32/75} & { 9/19} & {15/32} & {10/23} & {\color{red} 34/79} & {19/40} & {23/50} & {23/54} & {15/34} \\\hline
$20$ & { 2/ 5} && {11/27} && {12/29} && { 5/12} && { 5/12} && { 2/ 5} && {\color{red} 15/37} && {16/39} && {17/41} && { 5/12} && {\color{red}  5/12} && {28/67} && {29/69} && {30/71} && {31/73} && {32/75} && { 3/ 7} && {34/79} && {35/81} && {36/83} && {37/85} && {38/87} && {39/89} && {40/91} && {41/93} && {42/95} && {43/97} && {\color{red} 38/87} && {41/92} && {25/56} &\\\hline
$21$ & {\color{red}  5/13} & { 1/ 3} & { 3/ 7} & {12/25} & { 7/17} & {12/31} & { 7/16} & {25/54} & {24/55} & { 3/ 7} & {11/25} & {13/29} & {27/59} & {17/39} & {25/61} & {27/62} & {10/21} & {11/25} & { 2/ 5} & {14/33} & {11/23} & {29/68} & { 1/ 3} & { 3/ 7} & {12/25} & {31/72} & {\color{red}  5/13} & {23/53} & {12/25} & {17/38} & { 3/ 7} & {25/57} & {37/79} & {37/80} & {13/30} & {11/25} & {38/83} & {10/21} & { 7/16} & {18/43} & {13/29} & {32/67} & {11/25} & { 2/ 5} & {40/91} & {34/71} & {41/93} & {\color{red} 34/87} & {\color{red} 16/37} & {12/25} & {44/97} & { 3/ 7} & {\color{red} 17/39} & {12/25} & {27/58} & {\color{red} 35/81} & {\color{red} 18/41} & {41/87} & {10/21} & {\color{red} 37/85} \\\hline
$22$ & {19/49} && { 7/17} && {23/53} && { 5/11} && {16/35} && {17/37} && { 6/13} && { 6/13} && { 6/13} && {30/67} && {10/23} && {30/71} && {31/73} && {11/25} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && { 6/13} && { 6/13} && {14/31} && {42/95} && {43/97} && { 5/11} && {36/79} && {37/81} && {38/83} && {39/85} &\\\hline
$23$ & {20/51} & {17/52} & { 2/ 5} & {13/27} & { 7/16} & {13/33} & { 8/19} & {27/58} & { 4/ 9} & { 5/12} & {27/61} & {14/31} & { 4/ 9} & {18/41} & { 6/13} & {29/66} & {11/27} & { 4/ 9} & {11/23} & { 3/ 7} & {28/71} & { 4/ 9} & {12/25} & {31/74} & { 1/ 3} & { 8/19} & {13/27} & {24/55} & {11/28} & { 7/16} & {13/27} & {26/59} & {35/83} & {19/42} & { 8/17} & { 4/ 9} & { 7/16} & {41/88} & {41/89} & { 4/ 9} & {15/34} & {11/23} & {14/31} & {\color{red}  7/17} & { 4/ 9} & {35/73} & {43/97} & {\color{red} 17/44} & { 4/ 9} & {37/77} & {\color{red} 17/39} & {\color{red}  1/99} & {25/56} & {13/27} & {\color{red} 18/41} & {31/73} & {38/83} & {13/27} & {\color{red} 19/43} & {\color{red} 38/87} \\\hline
$24$ & {21/53} && {13/31} && {14/33} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 2/ 5} && {18/43} && {19/45} && {20/47} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 23/55} && {\color{red}  8/19} && {\color{red} 25/59} && {\color{red} 26/61} && { 3/ 7} && {\color{red}  3/ 7} && { 3/ 7} && {40/93} && {41/95} && {42/97} && {43/99} && {27/62} && {38/87} && {39/89} && {29/66} && {37/84} && {34/77} &\\\hline
$25$ & { 2/ 5} & {\color{red} 10/31} & { 8/19} & {14/29} & { 7/17} & { 2/ 5} & { 4/ 9} & {29/62} & { 3/ 7} & {16/39} & {13/29} & { 5/11} & {30/67} & {19/43} & {10/23} & {31/70} & {33/71} & {21/47} & {12/29} & {16/37} & {12/25} & {13/29} & {30/77} & {11/26} & {13/27} & {17/40} & {\color{red}  1/99} & {35/82} & {14/29} & { 3/ 7} & { 2/ 5} & {27/61} & {14/29} & {39/88} & {37/89} & {29/65} & {43/91} & {21/46} & {15/34} & {13/29} & {44/95} & {15/32} & { 4/ 9} & {43/98} & { 5/11} & {12/25} & {17/38} & {\color{red} 12/29} & {25/56} & {38/79} & {13/29} & {\color{red}  1/99} & {29/66} & {40/83} & {37/84} & {\color{red}  1/99} & {\color{red} 19/43} & {14/29} & {37/82} & {\color{red}  1/99} \\\hline
$26$ & {\color{red} 12/31} && {24/59} && {26/61} && { 4/ 9} && { 6/13} && {19/41} && {20/43} && { 7/15} && { 7/15} && { 7/15} && { 5/11} && {35/79} && {35/81} && {35/83} && {36/85} && {38/87} && {40/89} && { 6/13} && {31/67} && {32/69} && {33/71} && {34/73} && { 7/15} && { 7/15} && { 7/15} && {\color{red} 21/47} && {40/89} && {34/77} && {\color{red} 11/25} && {33/73} &\\\hline
$27$ & {23/59} & { 1/ 3} & { 7/17} & {15/31} & { 4/ 9} & {25/64} & {\color{red} 13/31} & {31/66} & { 9/20} & {17/41} & {10/23} & {16/35} & {14/31} & { 4/ 9} & {33/73} & {33/74} & {32/75} & {22/49} & {36/77} & {17/39} & {13/31} & {14/31} & {13/27} & {35/82} & {\color{red} 12/31} & {37/84} & {14/29} & {\color{red} 13/31} & {\color{red}  1/99} & {37/88} & {15/31} & { 4/ 9} & {36/91} & {10/23} & {15/31} & {30/67} & {\color{red}  7/17} & {43/96} & {46/97} & {32/71} & { 4/ 9} & {23/50} & {27/58} & {14/31} & {17/38} & {41/87} & {16/35} & {23/53} & { 9/20} & {13/27} & {40/89} & {\color{red} 13/31} & {14/31} & {41/85} & {\color{red} 27/64} & {\color{red}  1/99} & {43/97} & {43/89} & { 4/ 9} & {\color{red}  1/99} \\\hline
$28$ & {24/61} && { 3/ 7} && {16/37} && {17/39} && { 7/16} && { 7/16} && {31/73} && { 2/ 5} && { 3/ 7} && {22/51} && {23/53} && {24/55} && { 7/16} && { 7/16} && {38/89} && { 3/ 7} && {28/65} && {\color{red} 29/67} && {\color{red} 10/23} && {31/71} && {\color{red}  7/16} && { 7/16} && { 3/ 7} && {\color{red} 34/79} && {\color{red} 35/81} && {\color{red} 36/83} && {\color{red} 37/85} && {\color{red} 38/87} && {\color{red}  7/16} && {\color{red}  7/16} &\\\hline
$29$ & {25/63} & {21/64} & {27/65} & {16/33} & { 8/19} & {\color{red}  5/13} & { 9/20} & {33/70} & {\color{red} 14/33} & {18/43} & { 5/11} & {17/37} & {11/25} & {33/76} & { 5/11} & {35/78} & {36/79} & {23/51} & {\color{red} 11/26} & {18/41} & {39/83} & { 5/11} & {14/33} & {37/86} & {14/29} & { 5/11} & {13/33} & {\color{red} 14/33} & {15/31} & {39/92} & {\color{red}  1/99} & {20/47} & {16/33} & {41/96} & {\color{red} 13/34} & {31/69} & {16/33} & {11/25} & {\color{red}  5/12} & {33/73} & {39/82} & {33/73} & {39/89} & { 5/11} & {43/92} & {25/54} & { 9/20} & { 5/11} & {17/37} & {44/93} & {19/42} & {\color{red} 41/96} & {\color{red} 37/86} & {14/29} & { 5/11} & {\color{red}  1/99} & {\color{red} 19/45} & {44/91} & { 5/11} & {\color{red}  1/99} \\\hline
$30$ & { 2/ 5} && {\color{red} 15/37} && {29/69} && {31/71} && {33/73} && { 7/15} && {22/47} && {23/49} && { 8/17} && { 8/17} && { 8/17} && {40/87} && {40/89} && {40/91} && {40/93} && { 8/19} && {41/97} && {43/99} && {41/92} && {26/57} && { 7/15} && {36/77} && {37/79} && {38/81} && {39/83} && { 8/17} && { 8/17} && { 8/17} && {\color{red} 24/53} && {\color{red} 24/53} &\\\hline
$31$ & {\color{red}  7/18} & {\color{red} 12/37} & { 8/19} & {17/35} & {31/71} & {16/41} & { 3/ 7} & {35/74} & { 5/11} & {19/45} & { 3/ 7} & { 6/13} & {16/35} & { 3/ 7} & { 4/ 9} & {37/82} & {37/83} & {24/53} & {39/85} & {19/43} & { 3/ 7} & {26/57} & {42/89} & {13/30} & { 3/ 7} & {16/35} & {15/31} & { 3/ 7} & { 2/ 5} & { 7/16} & {16/33} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 29/69} & {17/35} & {15/34} & {\color{red}  1/99} & {29/67} & {\color{red} 35/74} & {34/75} & {\color{red}  8/19} & { 4/ 9} & {\color{red}  6/13} & {36/79} & {\color{red} 17/40} & {41/90} & {\color{red} 37/82} & {16/35} & {19/42} & {\color{red} 39/85} & {\color{red} 27/61} & {\color{red}  7/16} & { 5/11} & {\color{red} 42/89} & {\color{red} 13/30} & { 3/ 7} & {21/46} & {15/31} & {\color{red} 20/47} & {\color{red}  1/99} \\\hline
$32$ & { 9/23} && {30/71} && {18/41} && {19/43} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {35/83} && { 2/ 5} && {37/87} && {25/57} && {26/59} && {27/61} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 35/83} && {\color{red} 30/71} && {\color{red} 32/73} && {\color{red} 11/25} && {\color{red} 34/77} && {\color{red} 35/79} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 23/54} && {\color{red} 39/89} && {\color{red} 40/91} && {\color{red} 41/93} && {\color{red} 42/95} &\\\hline
$33$ & {28/71} & { 1/ 3} & {30/73} & {18/37} & { 3/ 7} & {17/43} & { 5/11} & {37/78} & {16/37} & {20/47} & {11/24} & {19/41} & {36/83} & {22/51} & {17/37} & {39/86} & {13/29} & { 5/11} & {39/89} & { 4/ 9} & { 6/13} & {27/59} & {16/37} & {41/94} & { 9/19} & {17/37} & {41/97} & {28/65} & {16/33} & { 9/20} & {\color{red}  1/99} & {16/37} & {17/35} & {11/26} & {\color{red}  1/99} & {\color{red}  8/19} & {18/37} & {\color{red} 32/75} & {\color{red}  1/99} & { 5/11} & {\color{red} 37/78} & {\color{red} 36/83} & {17/40} & {37/81} & {\color{red} 19/41} & {13/29} & {\color{red}  3/ 7} & {39/85} & {\color{red} 39/86} & {\color{red} 41/91} & { 5/11} & {\color{red}  9/20} & {\color{red}  4/ 9} & {\color{red}  6/13} & {21/46} & {\color{red} 40/93} & {\color{red} 41/94} & {\color{red}  9/19} & {11/24} & {\color{red}  1/99} \\\hline
$34$ & {29/73} && {17/41} && {\color{red} 18/43} && {34/79} && { 4/ 9} && {38/83} && { 8/17} && {25/53} && {26/55} && { 9/19} && { 9/19} && { 9/19} && {45/97} && { 5/11} && {41/92} && {38/87} && {\color{red}  3/ 7} && {\color{red}  8/19} && {\color{red} 39/94} && {\color{red} 20/47} && {\color{red} 34/79} && {\color{red} 22/49} && {\color{red} 38/83} && { 8/17} && {41/87} && {42/89} && {43/91} && {44/93} && { 9/19} && {\color{red} 45/97} &\\\hline
$35$ & { 2/ 5} & {25/76} & { 3/ 7} & {19/39} & {34/79} & { 2/ 5} & {10/23} & {39/82} & {11/24} & { 3/ 7} & {17/39} & {20/43} & { 6/13} & {23/53} & {39/89} & {41/90} & { 6/13} & {41/92} & {14/31} & {21/47} & {\color{red} 13/30} & {28/61} & {45/97} & {43/98} & {17/39} & { 6/13} & {29/61} & {\color{red} 29/67} & {\color{red} 16/39} & { 6/13} & {17/35} & {17/39} & {\color{red}  1/99} & {\color{red} 41/95} & {18/37} & {\color{red} 38/91} & {\color{red}  1/99} & { 3/ 7} & {19/39} & {\color{red} 34/79} & {\color{red}  1/99} & {\color{red} 35/81} & {\color{red} 39/82} & {38/83} & {\color{red}  1/99} & {\color{red} 39/89} & {\color{red} 20/43} & {40/87} & {\color{red} 19/44} & {14/31} & {\color{red} 41/90} & { 6/13} & {\color{red} 41/92} & {\color{red} 44/97} & {\color{red} 21/47} & {\color{red} 41/95} & {11/24} & {\color{red} 45/97} & {\color{red} 43/98} & {\color{red} 43/99} \\\hline
$36$ & {\color{red} 16/41} && {33/79} && { 4/ 9} && {21/47} && {22/49} && { 9/20} && { 9/20} && {40/91} && {13/31} && { 2/ 5} && {41/97} && { 4/ 9} && {29/65} && {30/67} && {31/69} && { 9/20} && { 9/20} && {\color{red} 22/51} && {\color{red} 26/63} && {\color{red} 41/97} && { 4/ 9} && {37/83} && {38/85} && {13/29} && {40/89} && {\color{red} 40/89} && {\color{red} 34/77} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$37$ & {31/79} & {\color{red} 14/43} & {\color{red}  9/22} & {20/41} & {10/23} & {11/28} & {38/85} & {41/86} & {18/41} & {37/88} & { 6/13} & { 7/15} & { 3/ 7} & {24/55} & {19/41} & {43/94} & {42/95} & {\color{red} 18/41} & {44/97} & {22/49} & { 5/11} & {29/63} & { 7/16} & {15/34} & {41/88} & {31/67} & {18/41} & {\color{red} 10/23} & {41/86} & {19/41} & {\color{red} 17/41} & {\color{red} 32/73} & {18/37} & {\color{red} 42/97} & {\color{red}  1/99} & {18/41} & {19/39} & {\color{red} 37/89} & {\color{red}  1/99} & {\color{red} 11/27} & {20/41} & {\color{red} 36/83} & {\color{red}  1/99} & {\color{red} 38/85} & {\color{red} 41/86} & {\color{red} 38/87} & {\color{red}  1/99} & {41/89} & {\color{red}  7/15} & {\color{red} 42/95} & {10/23} & {43/93} & {\color{red} 43/94} & { 5/11} & {\color{red}  7/16} & {\color{red} 25/54} & {\color{red} 22/49} & {\color{red} 26/57} & {23/50} & {\color{red} 27/62} \\\hline
$38$ & {32/81} && {19/45} && {20/47} && { 3/ 7} && {39/89} && {41/91} && {43/93} && { 9/19} && {28/59} && {29/61} && {10/21} && {10/21} && {10/21} && {43/92} && {\color{red}  5/11} && {41/91} && {\color{red} 10/23} && {10/23} && {\color{red}  3/ 7} && { 3/ 7} && {\color{red} 35/83} && {\color{red} 31/73} && {\color{red} 23/53} && {\color{red} 39/89} && {\color{red}  5/11} && {\color{red} 43/93} && { 9/19} && {46/97} && {47/99} && {29/61} &\\\hline
$39$ & {33/83} & { 1/ 3} & {36/85} & {21/43} & {37/87} & {\color{red} 19/49} & {11/25} & {43/90} & { 6/13} & {\color{red} 22/53} & {19/43} & {22/47} & {13/28} & {25/57} & {42/97} & {45/98} & {20/43} & {19/43} & {41/92} & {23/51} & {25/56} & { 6/13} & {16/35} & {43/97} & {15/34} & {32/69} & {\color{red} 17/37} & {\color{red} 31/71} & {19/43} & {20/43} & {\color{red} 35/74} & {11/25} & {\color{red}  1/99} & {\color{red} 25/56} & {19/39} & {19/43} & {\color{red}  1/99} & {13/30} & {20/41} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {21/43} & {\color{red} 36/83} & {\color{red}  1/99} & {\color{red} 39/89} & {\color{red} 43/90} & { 6/13} & {\color{red}  1/99} & {\color{red} 41/93} & {\color{red} 22/47} & {44/95} & {\color{red}  7/16} & {\color{red} 41/92} & {\color{red} 45/98} & {46/99} & {\color{red}  1/99} & {16/35} & {\color{red} 23/51} & {\color{red} 25/56} \\\hline
$40$ & { 2/ 5} && {12/29} && {39/89} && {23/51} && {24/53} && { 5/11} && { 5/11} && { 5/11} && {27/62} && {38/91} && {\color{red}  1/99} && {\color{red} 20/49} && {37/84} && {32/71} && {33/73} && {34/75} && { 5/11} && { 5/11} && { 5/11} && {\color{red} 27/62} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 39/89} && {41/91} && {14/31} && {43/95} && {44/97} && { 5/11} && {\color{red} 27/62} && { 5/11} &\\\hline
$41$ & {\color{red}  9/23} & {\color{red} 15/47} & { 5/12} & {22/45} & {11/25} & {20/51} & {41/93} & {45/94} & { 4/ 9} & {23/55} & {13/28} & {23/49} & { 4/ 9} & {26/59} & { 7/15} & {41/89} & {38/87} & { 4/ 9} & { 7/15} & {24/53} & {35/78} & {44/97} & {\color{red} 15/34} & {41/92} & {17/37} & {33/71} & { 4/ 9} & {25/57} & {\color{red}  6/13} & { 7/15} & { 4/ 9} & {\color{red} 34/77} & {\color{red} 37/78} & { 7/15} & {\color{red}  1/99} & { 4/ 9} & {20/41} & {\color{red} 37/84} & {\color{red}  1/99} & { 4/ 9} & {21/43} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {22/45} & {\color{red} 40/91} & {\color{red}  1/99} & {\color{red} 41/93} & {\color{red} 45/94} & {\color{red} 42/95} & {\color{red}  1/99} & {45/97} & {\color{red} 23/49} & { 4/ 9} & {\color{red}  1/99} & {27/58} & {\color{red} 41/89} & {\color{red} 35/78} & {\color{red}  1/99} & { 7/15} \\\hline
$42$ & {35/89} && { 3/ 7} && {22/51} && {23/53} && {\color{red} 10/23} && { 4/ 9} && {41/90} && {41/88} && {10/21} && {31/65} && {32/67} && {11/23} && {11/23} && {11/23} && {\color{red} 11/24} && {\color{red} 11/24} && {\color{red} 43/96} && {\color{red} 11/25} && {11/25} && {\color{red} 10/23} && {10/23} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 41/95} && {\color{red} 26/59} && {\color{red}  4/ 9} && {\color{red} 41/90} && {\color{red} 41/88} && {10/21} &\\\hline
$43$ & {36/91} & {\color{red}  1/ 4} & {13/31} & {23/47} & {\color{red} 11/26} & {21/53} & { 4/ 9} & {47/98} & { 5/11} & { 8/19} & {21/47} & { 8/17} & { 7/15} & {27/61} & { 3/ 7} & {43/93} & {22/47} & {29/65} & {37/84} & { 5/11} & {\color{red} 21/47} & {\color{red} 21/47} & {\color{red} 33/74} & {\color{red} 24/55} & { 4/ 9} & {34/73} & { 6/13} & {\color{red} 40/93} & {21/47} & {36/77} & {\color{red} 19/41} & {\color{red} 35/79} & {\color{red}  3/ 7} & {22/47} & {\color{red} 39/82} & {37/83} & {\color{red}  1/99} & {\color{red} 34/77} & {21/43} & {21/47} & {\color{red}  1/99} & {\color{red}  1/99} & {22/45} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {23/47} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 47/98} & {\color{red}  5/11} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  8/17} & {41/88} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 43/93} & {43/92} \\\hline
$44$ & {37/93} && {\color{red}  7/17} && {42/97} && { 5/11} && {26/57} && {27/59} && {11/24} && {11/24} && {40/89} && {16/37} && {\color{red}  5/12} && {\color{red}  1/99} && {\color{red}  1/99} && {38/87} && { 5/11} && {36/79} && {37/81} && {38/83} && {11/24} && {11/24} && {\color{red}  7/16} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && { 5/11} && {41/90} && {26/57} && {16/35} && {38/83} &\\\hline
$45$ & { 2/ 5} & {\color{red}  1/99} & {11/26} & {\color{red} 45/94} & { 4/ 9} & { 2/ 5} & {27/62} & {\color{red} 23/49} & {13/29} & {25/59} & { 7/15} & {25/53} & {22/49} & { 4/ 9} & {15/32} & {32/69} & {16/37} & {30/67} & {23/49} & {26/57} & {\color{red} 17/39} & {22/49} & {\color{red} 37/83} & {\color{red} 25/57} & {\color{red} 35/78} & { 7/15} & {17/38} & {\color{red} 35/81} & {19/41} & {37/79} & {22/49} & { 4/ 9} & {\color{red} 20/43} & {23/49} & {\color{red}  3/ 7} & {38/85} & {\color{red} 41/86} & {\color{red} 22/49} & {\color{red}  1/99} & {22/49} & {22/45} & {15/34} & {\color{red}  1/99} & {\color{red}  3/ 7} & {23/47} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {24/49} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/77} & {\color{red}  1/99} & {\color{red}  1/99} & { 7/15} & {\color{red} 25/53} & {\color{red}  1/99} & {\color{red}  1/99} & {29/62} \\\hline
$46$ & {\color{red} 20/51} && {14/33} && {24/55} && {25/57} && {\color{red} 11/25} && {\color{red} 11/25} && {40/89} && {\color{red}  5/11} && {\color{red} 31/67} && {11/23} && {34/71} && {35/73} && {12/25} && {12/25} && {12/25} && {\color{red}  6/13} && {\color{red}  6/13} && {\color{red} 33/73} && {\color{red}  4/ 9} && { 4/ 9} && {\color{red} 40/91} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 29/66} && {\color{red} 40/89} &\\\hline
$47$ & {13/33} & {\color{red}  1/99} & {37/89} & {\color{red} 47/98} & { 3/ 7} & {\color{red} 28/71} & {13/29} & {\color{red}  8/17} & {35/78} & {26/61} & {23/51} & {26/55} & {15/32} & {\color{red} 28/65} & {27/61} & {33/71} & { 8/17} & {31/69} & {17/39} & {\color{red} 31/73} & { 8/17} & {23/51} & {\color{red} 18/41} & {\color{red} 26/59} & {\color{red} 17/38} & {\color{red}  5/11} & {\color{red} 37/82} & {\color{red} 34/79} & { 9/20} & {38/81} & {20/43} & {\color{red} 22/51} & {23/51} & { 8/17} & {\color{red}  7/15} & {13/29} & {\color{red}  1/99} & { 8/17} & {\color{red} 43/90} & {41/91} & {\color{red}  1/99} & {\color{red} 43/97} & {23/47} & {23/51} & {\color{red}  1/99} & {\color{red}  1/99} & {24/49} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {25/51} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 38/79} & {\color{red} 35/78} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 26/55} & {37/79} \\\hline
$48$ & {21/53} && {23/55} && { 3/ 7} && {35/78} && {28/61} && {29/63} && { 6/13} && { 6/13} && { 6/13} && {\color{red} 41/93} && {\color{red} 23/54} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 37/83} && {39/85} && {40/87} && {41/89} && { 6/13} && { 6/13} && { 6/13} && {\color{red} 41/92} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {39/85} && {17/37} &\\\hline
$49$ & {39/98} & {\color{red}  1/99} & { 3/ 7} & {\color{red} 37/77} & {\color{red} 25/58} & {\color{red} 23/59} & {\color{red} 13/30} & {\color{red} 25/53} & {14/31} & { 3/ 7} & {\color{red} 29/64} & {\color{red} 32/69} & {24/53} & {\color{red} 29/67} & { 8/17} & {\color{red} 10/23} & { 3/ 7} & {32/71} & {\color{red} 41/87} & {\color{red} 31/69} & {18/41} & {24/53} & {\color{red} 24/53} & {\color{red} 27/61} & {\color{red} 19/43} & {\color{red} 35/79} & { 9/20} & {\color{red} 35/81} & {\color{red} 39/86} & {39/83} & {19/42} & {\color{red} 14/33} & { 7/15} & {41/87} & {\color{red} 42/97} & {40/89} & {\color{red} 22/47} & {25/53} & {\color{red}  1/99} & {14/31} & {\color{red} 45/94} & {\color{red} 41/92} & {\color{red}  1/99} & {24/53} & {24/49} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {25/51} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 40/83} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 29/63} \\\hline
$50$ & { 2/ 5} && {37/88} && {26/59} && {27/61} && { 4/ 9} && {\color{red}  4/ 9} && { 4/ 9} && {44/97} && {\color{red} 11/24} && {\color{red} 34/73} && {12/25} && {37/77} && {38/79} && {13/27} && {13/27} && {13/27} && {\color{red} 13/28} && {\color{red} 13/28} && {\color{red} 41/90} && {\color{red} 13/29} && {13/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & {\color{red} 11/28} & {\color{red}  1/99} & {\color{red} 12/29} & {\color{red} 38/79} & {13/30} & {\color{red}  1/99} & {14/31} & {\color{red} 29/63} & {\color{red} 43/98} & {\color{red} 27/65} & { 5/11} & {\color{red} 33/71} & { 8/17} & {10/23} & { 5/11} & {\color{red} 31/71} & {17/36} & {33/73} & {\color{red} 16/37} & {\color{red} 40/93} & {26/55} & { 5/11} & {\color{red} 19/43} & {\color{red} 25/59} & {\color{red} 14/31} & { 5/11} & {\color{red}  4/ 9} & {\color{red} 36/83} & {19/42} & { 8/17} & {\color{red} 41/90} & {\color{red}  1/99} & { 5/11} & {42/89} & {22/47} & {\color{red}  1/99} & { 5/11} & {26/55} & {\color{red} 23/49} & {43/95} & {\color{red}  1/99} & {\color{red}  5/11} & {\color{red} 47/98} & { 5/11} & {\color{red}  1/99} & {\color{red}  1/99} & {25/51} & {\color{red} 38/91} & {\color{red}  1/99} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/85} & {\color{red}  1/99} \\\hline
$52$ & {28/71} && {25/59} && {\color{red} 26/61} && {\color{red} 39/89} && { 6/13} && {31/67} && {32/69} && {13/28} && {13/28} && {\color{red} 25/56} && {19/43} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 39/89} && { 6/13} && {43/93} && {44/95} && {45/97} && {\color{red}  5/11} && {13/28} && {\color{red} 25/56} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & {23/58} & {\color{red}  1/99} & {31/73} & {\color{red} 40/83} & {\color{red}  3/ 7} & {\color{red}  1/99} & { 7/16} & {\color{red}  6/13} & { 5/11} & {\color{red} 28/67} & {\color{red} 13/29} & {\color{red} 26/57} & {\color{red} 36/79} & {31/71} & {17/36} & {\color{red} 32/73} & {\color{red} 10/23} & {34/75} & { 9/19} & {\color{red}  3/ 7} & {\color{red} 17/39} & {36/79} & { 9/19} & {\color{red} 34/81} & {\color{red}  4/ 9} & {\color{red} 41/92} & {\color{red}  4/ 9} & {\color{red} 37/85} & {\color{red} 21/47} & {\color{red} 40/87} & { 5/11} & {\color{red}  1/99} & {\color{red} 43/94} & {43/91} & {\color{red} 41/92} & {\color{red}  1/99} & {23/49} & { 9/19} & {\color{red}  7/16} & {44/97} & {\color{red}  8/17} & { 9/19} & {\color{red}  1/99} & {41/90} & {\color{red} 37/77} & {\color{red} 38/87} & {\color{red}  1/99} & {\color{red}  3/ 7} & {26/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$54$ & {\color{red} 23/59} && {\color{red} 40/97} && { 4/ 9} && {29/65} && {30/67} && {13/29} && {\color{red} 13/29} && {\color{red} 34/77} && {\color{red} 33/73} && {\color{red}  6/13} && {\color{red} 37/79} && {13/27} && {40/83} && {41/85} && {14/29} && {14/29} && {14/29} && {\color{red} 27/58} && {\color{red} 13/29} && {\color{red} 42/97} && {\color{red}  4/ 9} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & { 2/ 5} & {\color{red}  1/99} & {13/31} & {\color{red} 41/85} & { 7/16} & {\color{red}  1/99} & { 5/11} & {\color{red} 31/67} & {\color{red} 37/84} & {29/69} & {16/35} & {\color{red} 32/71} & {\color{red} 11/24} & {32/73} & {\color{red} 35/78} & {\color{red} 11/25} & { 9/19} & { 5/11} & {\color{red}  1/99} & {\color{red} 34/79} & {\color{red} 46/97} & {37/81} & {\color{red} 18/41} & {\color{red} 35/83} & {\color{red} 41/90} & {\color{red} 35/78} & {\color{red} 21/47} & {\color{red} 38/87} & { 5/11} & {\color{red} 40/89} & {\color{red} 22/49} & {\color{red}  1/99} & {21/46} & {44/93} & {\color{red} 45/98} & {\color{red}  1/99} & {\color{red} 25/56} & {46/97} & { 8/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/90} & {\color{red} 25/53} & {26/57} & {\color{red}  1/99} & {\color{red} 39/89} & {\color{red} 38/79} & {\color{red} 35/78} & {\color{red}  1/99} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} \\\hline
$56$ & {\color{red} 24/61} && { 3/ 7} && {28/65} && {18/41} && {\color{red} 31/69} && {33/71} && {34/73} && { 7/15} && { 7/15} && { 7/15} && {\color{red} 35/78} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 44/97} && {46/99} && {27/58} && {41/88} && { 7/15} && {\color{red} 35/78} && {\color{red} 25/58} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & {\color{red} 23/59} & {\color{red}  1/99} & {\color{red} 37/89} & {\color{red} 31/65} & {\color{red} 23/54} & {\color{red}  1/99} & {15/34} & {\color{red} 32/69} & {16/35} & {30/71} & {\color{red} 23/52} & {\color{red} 33/73} & {\color{red} 11/24} & {11/25} & { 9/19} & {\color{red} 34/77} & {\color{red} 38/87} & {\color{red} 35/79} & {19/40} & {\color{red} 35/81} & {\color{red}  1/99} & {38/83} & {\color{red} 41/88} & {\color{red} 36/85} & {\color{red}  1/99} & {\color{red} 39/85} & {\color{red} 26/57} & {\color{red} 38/89} & {22/49} & {\color{red} 41/92} & {21/46} & {\color{red}  1/99} & {\color{red} 23/51} & { 9/19} & {11/24} & {\color{red}  1/99} & {\color{red} 41/89} & {47/99} & {\color{red} 11/25} & {\color{red}  1/99} & {25/53} & {\color{red} 41/88} & {\color{red}  1/99} & {16/35} & {\color{red} 26/55} & {\color{red} 29/66} & {\color{red}  1/99} & {39/85} & {\color{red} 40/83} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/73} & {28/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$58$ & {\color{red}  9/23} && {\color{red}  5/16} && {\color{red} 29/67} && {31/69} && {32/71} && {\color{red} 23/51} && {14/31} && { 4/ 9} && {\color{red} 37/83} && {\color{red} 41/90} && {\color{red} 38/83} && {\color{red}  8/17} && {14/29} && {43/89} && {44/91} && {15/31} && {\color{red}  9/19} && {\color{red} 45/97} && {\color{red}  5/11} && {\color{red} 41/92} && {\color{red} 38/87} && {\color{red}  3/ 7} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & {\color{red} 25/64} & {\color{red}  1/99} & {14/33} & {\color{red} 32/67} & {15/34} & {\color{red}  1/99} & {\color{red} 31/70} & {\color{red} 33/71} & { 4/ 9} & {31/73} & {17/37} & {\color{red} 34/75} & {\color{red} 44/97} & {34/77} & {\color{red} 23/50} & {\color{red} 35/79} & {19/40} & { 4/ 9} & {\color{red}  1/99} & {\color{red} 36/83} & {10/21} & {39/85} & {\color{red}  1/99} & {\color{red} 37/87} & {10/21} & {\color{red} 23/50} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red} 40/89} & {\color{red} 17/38} & {23/51} & {\color{red}  1/99} & {11/24} & {\color{red} 45/97} & {\color{red} 24/53} & {\color{red}  1/99} & {23/50} & {29/61} & {\color{red} 43/93} & {\color{red}  1/99} & {\color{red} 23/52} & {10/21} & {26/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 40/89} & {\color{red}  9/19} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 27/61} & {\color{red} 41/85} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {30/61} & {\color{red}  1/99} \\\hline
$60$ & { 2/ 5} && {\color{red} 28/67} && {10/23} && {\color{red} 31/71} && {\color{red} 25/56} && { 7/15} && {36/77} && {37/79} && {\color{red} 22/47} && {\color{red} 43/94} && {\color{red} 22/49} && {22/49} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && { 7/15} && {43/92} && {29/62} && {37/79} && {\color{red} 29/63} && {\color{red} 43/97} && {\color{red} 17/39} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 2+k, 2+k+i\}$.
\end{center}


==> tables/table-g3-a03.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 3/ 8} & { 1/ 3} & { 3/10} & { 1/ 3} & { 5/13} & { 3/ 7} & { 3/ 7} & { 2/ 5} & { 3/ 8} & { 6/17} & { 7/19} & { 2/ 5} & { 3/ 7} & { 3/ 7} & { 9/22} & { 9/23} & { 3/ 8} & { 5/13} & {11/27} & { 3/ 7} & { 3/ 7} & {12/29} & { 2/ 5} & {12/31} & {13/33} & { 7/17} & { 3/ 7} & { 3/ 7} & { 5/12} & {15/37} & {15/38} & { 2/ 5} & {17/41} & { 3/ 7} & { 3/ 7} & {18/43} & { 9/22} & { 2/ 5} & {19/47} & { 5/12} & { 3/ 7} & { 3/ 7} & {21/50} & { 7/17} & {21/52} & {11/27} & {23/55} & { 3/ 7} & { 3/ 7} & { 8/19} & {12/29} & {24/59} & {25/61} & {13/31} & { 3/ 7} & { 3/ 7} & {27/64} & {27/65} & { 9/22} & { 7/17} \\\hline
$2$ & { 1/ 3} && { 4/13} && { 1/ 3} && { 3/ 8} && { 7/19} && { 8/21} && { 9/23} && { 2/ 5} && {11/27} && {12/29} && {13/31} && {14/33} && { 3/ 7} && {16/37} && {17/39} && {18/41} && {19/43} && { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && {31/67} && {32/69} &\\\hline
$3$ & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} &\\\hline
$4$ & { 2/ 5} && { 4/13} && { 2/ 5} && { 1/ 3} && { 7/19} && { 2/ 5} && {10/27} && { 2/ 5} && {12/31} && {13/33} && { 2/ 5} && {15/37} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} &\\\hline
$5$ & { 7/17} & { 4/11} & { 6/19} & { 2/ 5} & { 7/16} & { 5/11} & { 9/23} & { 1/ 3} & { 2/ 5} & { 3/ 7} & { 5/11} & { 3/ 7} & {11/29} & { 2/ 5} & {11/26} & { 4/ 9} & { 5/11} & { 7/17} & { 2/ 5} & {13/31} & { 7/16} & { 5/11} & {17/39} & { 2/ 5} & { 5/12} & {16/37} & {17/38} & { 5/11} & {19/45} & {17/41} & { 3/ 7} & {19/43} & { 5/11} & {11/25} & {\color{red} 19/46} & {20/47} & { 7/16} & {22/49} & { 5/11} & { 3/ 7} & {11/26} & {23/53} & { 4/ 9} & { 5/11} & {27/61} & {\color{red}  8/19} & {25/58} & {26/59} & { 9/20} & { 5/11} & {29/67} & { 3/ 7} & { 7/16} & {29/65} & { 5/11} & { 4/ 9} & {\color{red} 29/68} & {10/23} & {31/70} & {32/71} \\\hline
$6$ & { 8/19} &&&& {10/23} && {11/25} &&&& {13/29} && {14/31} &&&& {16/35} && {17/37} &&&& {19/41} && {20/43} &&&& {22/47} && {23/49} &&&& {25/53} && {26/55} &&&& {28/59} && {29/61} &&&& {31/65} && {32/67} &&&& {34/71} && {35/73} &&&& {37/77} &\\\hline
$7$ & { 3/ 7} & { 5/13} & { 5/16} & { 5/13} & { 2/ 5} & { 6/13} & { 9/20} & { 3/ 7} & {11/29} & { 1/ 3} & {\color{red} 12/31} & { 7/16} & { 6/13} & { 4/ 9} & { 3/ 7} & { 7/18} & { 5/13} & { 8/19} & { 6/13} & { 5/11} & {15/34} & { 3/ 7} & {17/43} & { 9/22} & { 4/ 9} & { 6/13} & { 9/20} & {18/41} & { 3/ 7} & { 2/ 5} & {22/51} & { 6/13} & {21/46} & {21/47} & { 7/16} & { 3/ 7} & { 8/19} & {13/29} & { 6/13} & {24/53} & { 4/ 9} & {24/55} & { 3/ 7} & { 7/16} & { 6/13} & {27/59} & { 9/20} & {27/61} & {27/62} & { 3/ 7} & {32/71} & { 6/13} & { 5/11} & {30/67} & {15/34} & {\color{red} 10/23} & {34/77} & { 6/13} & {11/24} & {33/73} \\\hline
$8$ & { 2/ 5} && { 8/25} && {10/27} && { 3/ 7} && { 9/23} && { 1/ 3} && { 3/ 7} && {12/29} && {12/31} && {16/41} && { 3/ 7} && {15/37} && { 5/13} && { 3/ 7} && {18/43} && {\color{red}  2/ 5} && { 2/ 5} && { 3/ 7} && {\color{red}  7/17} && {25/61} && { 3/ 7} && {\color{red}  8/19} && {28/67} && {29/69} && { 3/ 7} && {31/73} && {32/75} && { 3/ 7} && {34/79} && {35/81} &\\\hline
$9$ & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & { 9/23} && { 2/ 5} & { 2/ 5} && {11/28} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & {15/38} && { 2/ 5} & { 2/ 5} && {17/43} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & {21/53} && { 2/ 5} & { 2/ 5} && {\color{red} 23/58} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} && { 2/ 5} & {27/68} && { 2/ 5} & { 2/ 5} && {\color{red} 29/73} & { 2/ 5} &\\\hline
$10$ & {11/27} && { 6/19} && { 3/ 7} && { 3/ 8} && { 2/ 5} && { 7/16} && { 1/ 3} && {13/31} && {18/43} && { 2/ 5} && {16/37} && {19/49} && {17/41} && { 7/16} && { 2/ 5} && {20/47} && {25/59} && { 7/17} && {23/53} && { 2/ 5} && {\color{red}  8/19} && { 7/16} && {\color{red} 25/61} && {\color{red}  3/ 7} && {32/75} && {\color{red} 28/67} && {\color{red} 10/23} && {34/81} && {\color{red} 31/73} && { 7/16} &\\\hline
$11$ & {12/29} & { 7/17} & {10/31} & { 7/17} & { 5/11} & { 8/17} & { 2/ 5} & { 7/18} & { 5/13} & { 8/19} & {13/28} & { 9/20} & { 2/ 5} & { 1/ 3} & {13/32} & { 5/11} & { 8/17} & {10/23} & { 7/17} & {\color{red} 14/37} & { 3/ 7} & { 6/13} & { 8/17} & {11/26} & {21/53} & {11/27} & { 5/11} & { 7/15} & {26/57} & {12/29} & {23/59} & {13/30} & {23/50} & { 8/17} & { 4/ 9} & { 7/17} & {27/65} & { 5/11} & {13/28} & { 8/17} & {10/23} & { 2/ 5} & {31/71} & {28/61} & {29/62} & {17/37} & {32/75} & { 8/19} & { 5/11} & {31/67} & { 8/17} & { 9/20} & {34/81} & {18/41} & {11/24} & {34/73} & { 8/17} & {19/43} & {37/87} & { 5/11} \\\hline
$12$ & {13/31} &&&& { 3/ 7} && {16/37} &&&& {18/41} && {19/43} &&&& {21/47} && {22/49} &&&& {24/53} && { 5/11} &&&& {27/59} && {28/61} &&&& { 6/13} && {31/67} &&&& {33/71} && {34/73} &&&& {36/77} && {37/79} &&&& {39/83} && { 8/17} &&&& {42/89} &\\\hline
$13$ & {14/33} & { 8/19} & { 7/22} & { 8/19} & {15/37} & { 9/19} & { 6/13} & { 2/ 5} & {11/28} & { 8/21} & {\color{red}  2/ 5} & { 5/11} & {15/32} & {10/23} & { 7/17} & { 1/ 3} & { 5/12} & {11/25} & { 9/19} & { 6/13} & { 8/19} & {16/41} & { 8/19} & { 3/ 7} & { 9/19} & { 7/15} & {26/59} & {\color{red} 19/47} & {24/61} & {13/31} & {29/63} & { 8/17} & { 6/13} & {14/33} & {\color{red}  7/18} & {\color{red} 23/55} & {31/69} & { 9/19} & {27/58} & { 4/ 9} & {30/73} & { 8/19} & {11/25} & { 9/19} & {15/32} & { 6/13} & {34/79} & { 2/ 5} & {35/81} & {19/41} & {33/70} & {33/71} & {38/85} & {18/43} & {37/87} & { 5/11} & { 9/19} & {36/77} & { 6/13} & {10/23} \\\hline
$14$ & { 3/ 7} && {12/37} && { 2/ 5} && { 4/ 9} && {11/29} && { 2/ 5} && { 9/20} && { 3/ 7} && { 1/ 3} && {23/53} && {18/41} && {22/57} && {24/59} && {21/47} && { 3/ 7} && { 2/ 5} && { 9/20} && {24/55} && {28/71} && {32/73} && {27/61} && { 3/ 7} && {33/79} && {30/67} && {\color{red} 10/23} && { 2/ 5} && { 9/20} && {\color{red} 11/25} && { 3/ 7} && {41/93} &\\\hline
$15$ & { 9/22} & { 3/ 7} && { 3/ 7} & {11/26} && { 3/ 7} & {12/29} && {13/31} & { 3/ 7} && { 3/ 7} & { 3/ 7} && { 3/ 7} & { 8/19} && {17/40} & { 3/ 7} && {18/43} & { 3/ 7} && { 3/ 7} & {20/47} && { 3/ 7} & {21/50} && {11/26} & { 3/ 7} && { 3/ 7} & { 3/ 7} && { 3/ 7} & {25/59} && {26/61} & { 3/ 7} && {\color{red} 27/64} & { 3/ 7} && { 3/ 7} & {29/68} && { 3/ 7} & {\color{red} 30/71} && {31/73} & { 3/ 7} && { 3/ 7} & { 3/ 7} && { 3/ 7} & {17/40} &\\\hline
$16$ & {16/39} && {\color{red}  8/25} && { 4/ 9} && { 9/22} && {12/31} && { 5/11} && {20/51} && {22/53} && { 5/11} && { 1/ 3} && {19/43} && {26/61} && {18/47} && {22/49} && { 9/22} && {29/69} && { 5/11} && {29/73} && {26/59} && { 5/11} && {31/79} && {29/65} && {36/83} && {36/85} && {32/71} && {37/89} && {11/25} && { 5/11} && {\color{red} 37/93} && { 4/ 9} &\\\hline
$17$ & {17/41} & {10/23} & {14/43} & {10/23} & { 4/ 9} & {11/23} & {19/47} & { 5/12} & {19/49} & { 2/ 5} & { 8/17} & { 6/13} & { 5/12} & { 9/23} & { 8/19} & { 3/ 7} & {19/40} & {13/29} & { 3/ 7} & { 1/ 3} & {19/44} & {14/31} & {11/23} & { 7/16} & {10/23} & {13/33} & {10/23} & { 8/17} & {11/23} & { 3/ 7} & {30/71} & {23/55} & {32/73} & { 9/19} & { 7/15} & {\color{red} 25/59} & {\color{red}  9/23} & {26/61} & {36/79} & {10/21} & {37/81} & {28/65} & {33/83} & {\color{red} 29/67} & { 8/17} & {11/23} & {13/29} & {10/23} & {\color{red}  5/12} & { 4/ 9} & {35/74} & {11/23} & {41/93} & {20/47} & {\color{red} 11/26} & {11/24} & {19/40} & {23/49} & {43/99} & {\color{red}  1/99} \\\hline
$18$ & {18/43} &&&& {20/47} && { 3/ 7} &&&& {23/53} && {24/55} &&&& {26/59} && {27/61} &&&& {29/65} && {30/67} &&&& {32/71} && {33/73} &&&& { 5/11} && {36/79} &&&& {38/83} && {39/85} &&&& {41/89} && { 6/13} &&&& {44/95} && {45/97} &&&& {27/58} &\\\hline
$19$ & {19/45} & {11/25} & { 9/28} & {11/25} & {20/49} & {12/25} & {23/51} & {11/26} & {\color{red} 13/34} & {11/27} & { 2/ 5} & {13/28} & { 9/19} & {12/29} & {17/40} & { 2/ 5} & { 3/ 7} & {14/31} & {21/44} & { 7/16} & {10/23} & { 1/ 3} & { 7/16} & {15/34} & {12/25} & {16/35} & {11/25} & { 7/18} & {11/25} & {16/37} & {12/25} & { 9/19} & { 3/ 7} & {25/59} & {33/79} & {\color{red} 26/61} & {38/81} & {10/21} & {37/83} & {28/65} & { 2/ 5} & {29/67} & {40/87} & {11/23} & {41/89} & {\color{red} 31/71} & {\color{red}  7/18} & {\color{red} 32/73} & {14/31} & {12/25} & { 9/19} & {\color{red} 11/25} & {\color{red} 11/26} & {11/25} & {\color{red} 17/40} & {12/25} & {39/82} & {23/51} & {\color{red}  3/ 7} & {11/26} \\\hline
$20$ & {20/47} && {16/49} && {13/31} && { 5/11} && { 2/ 5} && {11/26} && { 6/13} && {17/41} && {\color{red}  5/13} && { 6/13} && {29/67} && { 1/ 3} && {31/71} && {24/53} && { 2/ 5} && {\color{red}  8/19} && {27/59} && {\color{red} 25/61} && {11/26} && { 6/13} && {38/87} && {35/89} && { 6/13} && {33/73} && {\color{red}  1/99} && {43/97} && {36/79} && {37/89} && {\color{red} 19/45} && {39/85} &\\\hline
$21$ & { 3/ 7} & { 4/ 9} && { 4/ 9} & { 7/16} && {15/34} & { 3/ 7} && {16/37} & { 4/ 9} && { 4/ 9} & {18/41} && {19/43} & {\color{red} 19/44} && {10/23} & { 4/ 9} && { 4/ 9} & {11/25} && {23/52} & {\color{red} 23/53} && {24/55} & { 4/ 9} && { 4/ 9} & {26/59} && {27/61} & {\color{red} 27/62} && { 7/16} & { 4/ 9} && { 4/ 9} & {15/34} && {31/70} & {\color{red} 31/71} && {32/73} & { 4/ 9} && { 4/ 9} & {34/77} && {35/79} & {\color{red}  7/16} && {18/41} & { 4/ 9} && { 4/ 9} & {19/43} &\\\hline
$22$ & {12/29} && {\color{red} 10/31} && { 5/11} && { 3/ 7} && {23/59} && { 6/13} && { 3/ 7} && {18/43} && {13/28} && {11/28} && { 3/ 7} && {33/73} && { 1/ 3} && { 5/11} && {\color{red} 34/79} && {32/81} && {28/61} && { 3/ 7} && {\color{red} 27/65} && {31/67} && { 3/ 7} && {\color{red} 40/93} && {13/28} && {\color{red}  1/99} && { 5/11} && {41/90} && {\color{red}  1/99} && {38/83} && {\color{red} 41/96} && {\color{red}  1/99} &\\\hline
$23$ & {22/53} & {13/29} & {18/55} & {13/29} & {25/57} & {14/29} & {12/29} & {13/30} & {15/38} & {13/31} & {29/63} & {15/32} & { 2/ 5} & {12/29} & {28/67} & { 7/17} & {11/23} & {16/35} & { 7/16} & { 7/18} & {11/25} & {16/37} & {25/52} & {17/38} & { 4/ 9} & { 1/ 3} & {25/56} & { 9/20} & {14/29} & {18/41} & {13/29} & {24/61} & {13/29} & {20/43} & {14/29} & {19/44} & {39/89} & {19/45} & { 3/ 7} & {11/23} & {44/93} & {\color{red} 31/71} & {\color{red} 12/29} & {32/73} & {43/97} & {12/25} & {46/99} & {\color{red} 34/77} & {\color{red}  1/99} & {35/79} & {\color{red}  9/20} & {13/27} & {16/35} & {37/83} & {\color{red}  1/99} & {\color{red} 38/85} & {29/62} & {14/29} & {41/91} & {13/29} \\\hline
$24$ & {23/55} &&&& {25/59} && {26/61} &&&& {28/65} && {29/67} &&&& {31/71} && {32/73} &&&& {34/77} && {35/79} &&&& {37/83} && {38/85} &&&& {40/89} && {41/91} &&&& {43/95} && {44/97} &&&& {41/90} && {\color{red} 44/97} &&&& {\color{red} 41/90} && {\color{red} 26/57} &&&& {\color{red} 38/83} &\\\hline
$25$ & { 8/19} & {14/31} & {\color{red} 11/34} & {14/31} & { 5/12} & {15/31} & { 4/ 9} & { 7/16} & { 2/ 5} & {14/33} & {\color{red} 13/31} & { 8/17} & {32/69} & { 2/ 5} & {\color{red} 19/46} & {13/31} & {31/73} & {17/37} & {12/25} & { 8/19} & {23/52} & {12/31} & { 4/ 9} & { 9/20} & {27/56} & {18/41} & {13/29} & {\color{red}  1/99} & { 9/20} & {19/43} & {15/31} & { 5/11} & {14/31} & { 2/ 5} & {14/31} & {10/23} & {15/31} & {22/47} & {42/95} & { 5/12} & {42/97} & { 3/ 7} & {47/99} & {12/25} & {27/62} & {34/77} & {\color{red}  9/22} & {\color{red} 35/79} & { 7/15} & {13/27} & {\color{red} 18/41} & {37/83} & {\color{red}  1/99} & {38/85} & {\color{red} 19/43} & {14/29} & {\color{red}  5/11} & {40/89} & {\color{red}  1/99} & {41/91} \\\hline
$26$ & {25/59} && {20/61} && {16/37} && { 6/13} && {16/41} && { 7/16} && { 7/15} && {20/47} && {31/75} && {15/32} && {23/53} && {32/81} && {38/83} && {\color{red}  7/16} && {\color{red}  1/99} && {39/89} && { 6/13} && {\color{red} 26/67} && {\color{red} 10/23} && {33/71} && {\color{red} 31/73} && { 7/16} && {36/77} && {\color{red} 34/79} && {\color{red} 32/79} && {15/32} && {\color{red} 43/98} && {\color{red}  1/99} && {\color{red} 23/51} && { 6/13} &\\\hline
$27$ & {26/61} & { 5/11} && { 5/11} & {17/38} && { 9/20} & {15/34} && { 3/ 7} & { 5/11} && { 5/11} & {21/47} && {22/49} & { 5/11} && {35/79} & {24/53} && { 5/11} & {25/56} && {13/29} & { 5/11} && { 5/11} & {14/31} && {29/64} & {29/65} && {30/67} & { 5/11} && { 5/11} & {32/71} && {33/73} & {\color{red} 33/74} && {17/38} & { 5/11} && { 5/11} & { 9/20} && {37/82} & { 5/11} && {\color{red} 38/85} & {39/86} && { 5/11} & {40/89} && {41/91} & { 5/11} &\\\hline
$28$ & { 3/ 7} && {\color{red} 12/37} && {30/67} && {18/41} && {17/43} && { 7/15} && {15/34} && { 3/ 7} && { 8/17} && {\color{red}  7/17} && {24/55} && { 8/17} && {34/87} && {15/34} && {41/91} && {\color{red}  1/99} && {43/95} && {\color{red} 10/23} && {\color{red}  1/99} && {34/73} && {11/25} && { 3/ 7} && {37/79} && {\color{red} 41/95} && {36/83} && { 8/17} && {\color{red}  1/99} && {\color{red} 39/89} && {\color{red} 41/91} && {\color{red}  1/99} &\\\hline
$29$ & {\color{red}  5/12} & {16/35} & {22/67} & {16/35} & {10/23} & {17/35} & { 3/ 7} & { 4/ 9} & {17/44} & {16/37} & {34/75} & { 9/19} & { 3/ 7} & { 3/ 7} & {21/50} & { 2/ 5} & {38/81} & {19/41} & {35/83} & { 3/ 7} & {37/85} & { 8/19} & {14/29} & { 5/11} & { 9/20} & { 2/ 5} & {14/31} & {\color{red} 10/23} & {31/64} & {21/47} & { 5/11} & {\color{red}  1/99} & {31/68} & {22/49} & {17/35} & {11/25} & {16/35} & {\color{red}  1/99} & {16/35} & {\color{red} 34/75} & {\color{red}  9/19} & {\color{red}  3/ 7} & {\color{red} 11/26} & {\color{red}  1/99} & {\color{red} 18/43} & {\color{red} 38/81} & {\color{red} 19/41} & { 3/ 7} & { 3/ 7} & {\color{red} 37/85} & {10/23} & {14/29} & {\color{red}  5/11} & {40/89} & {\color{red}  1/99} & {41/91} & {\color{red} 43/98} & {15/31} & {\color{red} 21/47} & {43/95} \\\hline
$30$ & {28/67} &&&& {30/71} && {31/73} &&&& { 3/ 7} && {34/79} &&&& {36/83} && {37/85} &&&& {39/89} && {40/91} &&&& {42/95} && {43/97} &&&& {\color{red} 42/95} && {\color{red} 43/97} &&&& {\color{red} 42/95} && {\color{red} 43/97} &&&& {\color{red} 42/95} && {\color{red} 43/97} &&&& {\color{red} 42/95} && {\color{red} 43/97} &&&& {\color{red} 42/95} &\\\hline
$31$ & {29/69} & {17/37} & {\color{red} 13/40} & {17/37} & { 3/ 7} & {18/37} & {11/25} & {17/38} & { 9/23} & {17/39} & {16/37} & {19/40} & {37/81} & {17/41} & {11/26} & {16/37} & { 2/ 5} & {20/43} & {41/87} & { 8/19} & {\color{red} 25/58} & {19/45} & {40/91} & {21/46} & {15/31} & { 3/ 7} & {29/64} & {\color{red} 31/81} & { 5/11} & {22/49} & {33/68} & {11/25} & {16/35} & {\color{red}  1/99} & {11/24} & {\color{red}  3/ 7} & {18/37} & {\color{red}  4/ 9} & {17/37} & {\color{red}  1/99} & {\color{red} 17/38} & {\color{red} 34/79} & {\color{red} 19/40} & {\color{red} 37/81} & {\color{red} 17/40} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red} 41/95} & {\color{red} 20/43} & {\color{red} 41/87} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 40/91} & {\color{red} 21/46} & {15/31} & {11/25} & {43/95} & {\color{red}  1/99} & {44/97} \\\hline
$32$ & {30/71} && {24/73} && {19/43} && { 5/11} && {31/79} && {17/38} && { 8/17} && {\color{red} 22/53} && {38/87} && { 9/19} && {26/59} && { 8/19} && { 9/19} && {29/65} && {\color{red}  1/99} && {\color{red} 37/82} && {17/38} && {\color{red}  1/99} && {\color{red} 11/25} && {\color{red}  5/11} && {\color{red}  1/99} && { 4/ 9} && {39/83} && {\color{red}  1/99} && {\color{red} 38/87} && {42/89} && {40/91} && {\color{red}  1/99} && { 9/19} && {43/97} &\\\hline
$33$ & {31/73} & { 6/13} && { 6/13} & { 5/11} && {21/46} & { 9/20} && {18/41} & {23/50} && { 6/13} & {19/43} && { 5/11} & { 6/13} && { 6/13} & {27/59} && {28/61} & {42/95} && {43/97} & { 6/13} && { 6/13} & {31/68} && {16/35} & { 6/13} && {\color{red} 42/95} & {17/37} && {35/76} & { 5/11} && {36/79} & { 6/13} && {\color{red}  9/20} & {38/83} && {39/85} & {\color{red} 19/43} && { 5/11} & {41/89} && { 6/13} & {21/46} && {43/94} & {\color{red} 24/53} && { 6/13} & {45/98} &\\\hline
$34$ & {32/75} && {\color{red} 14/43} && {35/79} && {21/47} && {\color{red} 19/49} && { 8/17} && { 9/20} && {23/55} && { 9/19} && {40/93} && {27/61} && {19/40} && {17/40} && {30/67} && {\color{red} 39/86} && {\color{red}  1/99} && { 9/20} && {\color{red} 19/43} && {\color{red}  1/99} && {\color{red} 43/96} && {\color{red}  4/ 9} && {\color{red}  1/99} && { 8/17} && {13/29} && {\color{red}  1/99} && {43/91} && { 9/20} && {42/95} && {46/97} && {\color{red}  1/99} &\\\hline
$35$ & { 3/ 7} & {19/41} & {\color{red}  7/22} & {19/41} & {35/81} & {20/41} & { 7/16} & {19/42} & { 2/ 5} & {19/43} & {13/29} & {21/44} & {18/41} & {24/55} & { 3/ 7} & {\color{red} 17/41} & {43/93} & {22/47} & { 2/ 5} & {18/41} & {27/62} & { 3/ 7} & {47/99} & {23/50} & {27/62} & {\color{red} 17/41} & {25/56} & {\color{red} 10/23} & {17/35} & {\color{red} 11/25} & {11/24} & {\color{red}  1/99} & {17/37} & {\color{red} 18/41} & {37/76} & {\color{red} 23/53} & { 6/13} & {\color{red}  1/99} & {37/80} & {13/29} & {20/41} & {\color{red} 36/83} & {19/41} & {\color{red}  1/99} & {\color{red} 19/42} & {\color{red} 14/31} & {\color{red} 21/44} & {\color{red} 39/89} & {\color{red} 13/30} & {\color{red}  1/99} & {\color{red} 19/45} & {\color{red} 43/93} & {\color{red} 22/47} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 47/99} & {\color{red} 23/50} & {\color{red}  1/99} \\\hline
$36$ & {\color{red} 18/43} &&&& {\color{red} 20/47} && { 3/ 7} &&&& {\color{red}  3/ 7} && { 3/ 7} &&&& {41/95} && {42/97} &&&& {27/62} && {38/87} &&&& {\color{red} 41/95} && {\color{red} 42/97} &&&& {\color{red} 29/66} && {\color{red} 38/87} &&&& {\color{red} 27/61} && {\color{red} 37/84} &&&& {\color{red} 27/62} && {\color{red} 38/87} &&&& {\color{red} 41/95} && {\color{red} 38/87} &&&& {\color{red} 27/62} &\\\hline
$37$ & {34/81} & {20/43} & {\color{red} 15/46} & {20/43} & { 7/16} & {21/43} & {38/87} & { 5/11} & {35/89} & { 4/ 9} & {19/43} & {11/23} & {14/31} & {20/47} & {\color{red}  8/19} & {26/59} & {41/97} & {23/49} & {46/99} & {\color{red}  1/99} & { 7/16} & {19/43} & {\color{red} 38/91} & {\color{red} 29/67} & {10/21} & {10/23} & {\color{red} 19/43} & {\color{red}  5/12} & {40/89} & {\color{red}  3/ 7} & {18/37} & {\color{red} 11/25} & {35/76} & {\color{red}  1/99} & { 6/13} & {\color{red} 11/26} & {39/80} & {\color{red} 19/43} & {19/41} & {\color{red}  1/99} & {13/28} & {\color{red} 37/85} & {21/43} & {14/31} & {20/43} & {\color{red}  1/99} & {\color{red}  5/11} & {\color{red} 40/91} & {\color{red} 11/23} & {\color{red}  5/11} & {\color{red} 10/23} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red} 23/49} & {\color{red} 46/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$38$ & {35/83} && {\color{red} 15/47} && {22/49} && {40/89} && {21/53} && { 5/11} && { 9/19} && {25/59} && { 5/11} && {10/21} && {38/87} && {\color{red} 19/44} && {21/44} && {32/71} && {\color{red} 37/90} && {\color{red} 43/94} && { 5/11} && {\color{red}  1/99} && {\color{red} 21/47} && { 5/11} && {\color{red}  1/99} && {\color{red} 13/29} && {\color{red} 40/89} && {\color{red}  1/99} && {14/31} && { 9/19} && {\color{red}  1/99} && { 5/11} && {29/61} && {\color{red}  1/99} &\\\hline
$39$ & {36/85} & { 7/15} && { 7/15} & {40/89} && { 6/13} & {21/46} && {21/47} & {13/28} && {27/58} & { 3/ 7} && {11/25} & { 7/15} && { 7/15} & { 6/13} && {31/67} & {\color{red}  4/ 9} && {\color{red} 34/77} & {33/71} && {34/73} & {\color{red} 33/76} && {\color{red} 17/38} & { 7/15} && { 7/15} & {37/80} && {19/41} & {\color{red} 40/89} && {\color{red} 29/66} & {20/43} && {41/88} & {\color{red} 40/89} && { 6/13} & { 7/15} && {\color{red} 21/46} & {44/95} && {45/97} & {\color{red}  7/16} && {\color{red} 11/25} & {27/58} && {41/88} & { 6/13} &\\\hline
$40$ & {37/87} && {\color{red}  1/99} && {40/91} && {24/53} && { 2/ 5} && {45/97} && {21/46} && {26/61} && {10/21} && {30/67} && {\color{red} 29/67} && {11/23} && {10/23} && {33/73} && {11/23} && {\color{red}  1/99} && {36/79} && {\color{red} 45/98} && {\color{red}  1/99} && {21/46} && {\color{red} 23/52} && {\color{red}  1/99} && {\color{red} 40/91} && {14/31} && {\color{red}  1/99} && {\color{red} 45/97} && { 5/11} && {\color{red}  1/99} && {39/82} && {\color{red} 30/67} &\\\hline
$41$ & {38/89} & {22/47} & {\color{red}  1/99} & {22/47} & {40/93} & {\color{red} 21/44} & { 4/ 9} & {11/24} & {11/28} & {22/49} & { 4/ 9} & {\color{red} 22/47} & {21/47} & {27/61} & {13/31} & {\color{red} 20/47} & {16/35} & {25/53} & {\color{red} 12/29} & {21/47} & {15/34} & {\color{red}  1/99} & {\color{red} 35/76} & {\color{red} 11/25} & {\color{red}  1/99} & {\color{red} 20/47} & {33/74} & {11/25} & {\color{red}  9/19} & {\color{red} 23/53} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red}  9/20} & { 4/ 9} & {20/41} & {\color{red}  3/ 7} & {13/28} & {\color{red}  1/99} & {20/43} & {21/47} & {43/88} & {\color{red} 38/89} & { 7/15} & {\color{red}  1/99} & {43/92} & {\color{red}  4/ 9} & {23/47} & {\color{red}  1/99} & {22/47} & {\color{red}  1/99} & {\color{red} 11/24} & {16/35} & {\color{red} 12/25} & {\color{red}  1/99} & {\color{red} 15/34} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 17/37} & {\color{red} 25/53} & {\color{red}  1/99} \\\hline
$42$ & { 3/ 7} &&&& {23/53} && {24/55} &&&& {\color{red}  7/16} && {\color{red}  7/16} &&&& {\color{red} 28/65} && {\color{red} 29/67} &&&& {\color{red} 31/71} && {\color{red}  7/16} &&&& {\color{red}  7/16} && {\color{red} 34/79} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  7/16} && {\color{red}  3/ 7} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} &\\\hline
$43$ & {\color{red} 21/50} & {23/49} & {\color{red}  1/99} & {23/49} & { 4/ 9} & {\color{red} 11/23} & {43/99} & {23/50} & {23/58} & {23/51} & {22/49} & {\color{red} 23/49} & {30/67} & {\color{red}  3/ 7} & {27/64} & {29/65} & {\color{red}  3/ 7} & {\color{red} 22/49} & {17/37} & { 3/ 7} & {31/70} & {22/49} & {\color{red}  1/99} & {\color{red} 32/73} & {\color{red} 37/80} & {\color{red}  1/99} & {17/38} & {\color{red}  3/ 7} & {\color{red}  1/99} & {\color{red} 34/79} & {\color{red} 19/40} & { 4/ 9} & {\color{red} 22/49} & {\color{red}  1/99} & {\color{red} 19/42} & {\color{red} 36/85} & {21/43} & {13/29} & {41/88} & {\color{red}  1/99} & { 7/15} & {\color{red}  3/ 7} & {45/92} & {22/49} & {22/47} & {\color{red}  1/99} & {15/32} & {\color{red}  1/99} & {24/49} & {\color{red} 30/67} & {23/49} & {\color{red}  1/99} & {\color{red} 23/50} & {\color{red}  1/99} & {\color{red} 25/52} & {17/37} & {\color{red} 23/52} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$44$ & { 8/19} && {\color{red}  1/99} && { 5/11} && {41/92} && {\color{red}  1/99} && {28/61} && {43/92} && {\color{red} 27/65} && {23/50} && {11/23} && {31/71} && {\color{red} 32/73} && {12/25} && { 5/11} && {11/25} && {12/25} && {38/83} && {\color{red}  1/99} && {\color{red} 43/93} && {23/50} && {\color{red}  1/99} && {\color{red} 23/53} && {\color{red} 11/25} && {\color{red}  1/99} && { 5/11} && {\color{red} 41/92} && {\color{red}  1/99} && {16/35} && {\color{red} 43/92} && {\color{red}  1/99} &\\\hline
$45$ & {41/97} & { 8/17} && { 8/17} & {\color{red} 32/73} && {26/57} & { 6/13} && {\color{red} 22/51} & {29/62} && {15/32} & {24/55} && {\color{red} 27/67} & { 8/17} && { 8/17} & {\color{red} 31/71} && {\color{red} 33/73} & { 8/17} && {\color{red} 23/51} & {36/77} && {37/79} & {\color{red} 40/91} && {\color{red}  3/ 7} & {39/83} && { 8/17} & {\color{red} 39/88} && {\color{red}  5/11} & { 8/17} && { 8/17} & {43/92} && {22/47} & {\color{red}  4/ 9} && {\color{red}  4/ 9} & {23/49} && {39/83} & {\color{red} 41/92} && {\color{red} 26/57} & { 8/17} && {\color{red}  6/13} & {43/92} && {29/62} & {\color{red}  4/ 9} &\\\hline
$46$ & {14/33} && {\color{red}  1/99} && {\color{red}  3/ 7} && {27/59} && {\color{red}  1/99} && {\color{red} 39/86} && { 6/13} && {\color{red} 28/67} && {11/23} && { 6/13} && {32/73} && {12/25} && {34/77} && {\color{red} 35/79} && {25/52} && {\color{red} 35/83} && {39/85} && {\color{red} 13/29} && {\color{red}  1/99} && { 6/13} && {\color{red} 40/93} && {\color{red}  1/99} && { 6/13} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {16/35} && {\color{red}  1/99} && {\color{red} 39/85} && {17/37} &\\\hline
$47$ & {23/54} & {25/53} & {\color{red}  1/99} & {\color{red}  8/17} & {\color{red} 25/58} & {\color{red} 12/25} & { 9/20} & {\color{red} 23/52} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red} 33/76} & {\color{red}  6/13} & {\color{red} 33/73} & {30/67} & {29/68} & {\color{red} 23/53} & {\color{red} 17/38} & {\color{red} 32/71} & {\color{red} 37/86} & {33/73} & {\color{red} 16/37} & {\color{red}  1/99} & {19/41} & {\color{red} 34/77} & {\color{red}  1/99} & {\color{red} 19/43} & { 9/20} & {\color{red}  1/99} & {\color{red} 41/88} & {\color{red} 36/83} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 14/31} & {13/29} & {\color{red} 21/44} & {\color{red} 38/89} & {\color{red} 41/92} & {\color{red}  1/99} & {\color{red} 21/46} & {14/31} & {23/47} & {\color{red} 41/95} & {15/32} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {25/51} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {41/87} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {25/53} & {\color{red}  1/99} & {\color{red} 25/54} & {\color{red}  1/99} & {\color{red} 27/56} & {\color{red}  1/99} \\\hline
$48$ & {41/96} &&&& {26/59} && {27/61} &&&& { 4/ 9} && {\color{red}  4/ 9} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red} 34/77} && {\color{red} 35/79} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} &\\\hline
$49$ & { 3/ 7} & {26/55} & {\color{red}  1/99} & {\color{red} 26/57} & { 9/20} & {\color{red} 25/52} & {\color{red} 27/62} & {\color{red}  4/ 9} & {\color{red}  1/99} & {\color{red}  8/19} & { 5/11} & {\color{red} 31/67} & {\color{red}  7/16} & {\color{red} 10/23} & { 3/ 7} & {32/71} & { 5/11} & {\color{red} 33/73} & {\color{red}  9/20} & {\color{red}  8/19} & {\color{red} 33/76} & { 5/11} & {\color{red}  1/99} & {\color{red} 35/79} & {20/43} & {\color{red}  1/99} & {37/82} & { 5/11} & {\color{red}  1/99} & {\color{red} 37/85} & {\color{red} 43/92} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red} 11/23} & {14/31} & { 5/11} & {\color{red}  1/99} & {\color{red} 11/24} & {\color{red}  1/99} & {24/49} & { 5/11} & {39/83} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {26/53} & {\color{red}  1/99} & {25/53} & {\color{red}  1/99} & {17/36} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {\color{red} 13/28} & {\color{red}  1/99} \\\hline
$50$ & {\color{red}  8/19} && {\color{red}  1/99} && {\color{red} 27/61} && {\color{red} 10/23} && {\color{red}  1/99} && {31/67} && {\color{red} 43/94} && {\color{red} 30/71} && {13/28} && {12/25} && {34/77} && {\color{red} 41/92} && {13/27} && {37/83} && {\color{red} 37/83} && {27/56} && {41/89} && {\color{red}  1/99} && {\color{red} 14/31} && {44/95} && {\color{red}  1/99} && {\color{red} 43/99} && {\color{red} 41/92} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & {\color{red} 32/77} & { 9/19} && {\color{red} 27/59} & {\color{red}  7/16} && {\color{red} 37/83} & {\color{red}  3/ 7} && {\color{red} 28/67} & { 8/17} && {33/70} & {\color{red} 21/50} && {\color{red} 37/88} & {35/74} && { 9/19} & { 7/16} && {\color{red}  7/16} & {\color{red} 45/97} && { 9/19} & {\color{red} 38/83} && { 8/17} & {\color{red} 44/97} && {\color{red} 41/92} & {42/89} && {43/91} & {\color{red}  1/99} && {\color{red}  1/99} & { 9/19} && {\color{red} 45/97} & {\color{red}  9/20} && {\color{red} 23/50} & {\color{red} 41/92} && {\color{red} 38/87} & {41/87} && {25/53} & {\color{red} 37/88} && {\color{red}  1/99} & {26/55} && {44/93} & {\color{red}  1/99} && {\color{red} 33/73} & { 9/19} &\\\hline
$52$ & {36/85} && {\color{red}  1/99} && {10/23} && { 6/13} && {\color{red}  1/99} && {\color{red} 11/25} && {33/71} && {\color{red}  1/99} && {\color{red}  7/15} && {\color{red} 26/57} && {35/79} && {13/27} && {\color{red} 37/83} && {38/85} && {14/29} && {13/29} && { 6/13} && {\color{red} 43/93} && {\color{red}  1/99} && {45/97} && {\color{red}  4/ 9} && {\color{red}  1/99} && {\color{red} 26/57} && {\color{red}  3/ 7} && {\color{red}  1/99} && {\color{red} 27/64} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & {31/73} & {28/59} & {\color{red}  1/99} & {\color{red} 28/61} & { 7/16} & {\color{red} 31/65} & { 5/11} & {\color{red} 28/65} & {\color{red}  1/99} & {\color{red} 10/23} & {\color{red} 11/25} & {\color{red} 33/71} & {\color{red} 16/35} & {\color{red} 32/73} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red} 39/88} & {\color{red}  5/11} & {\color{red} 37/85} & {36/79} & { 7/16} & {\color{red}  1/99} & {\color{red}  5/11} & {\color{red} 37/83} & {\color{red}  1/99} & {\color{red} 16/35} & {39/86} & {\color{red}  1/99} & {22/47} & {\color{red} 39/89} & {\color{red}  1/99} & {\color{red}  1/99} & {21/46} & {\color{red}  1/99} & {\color{red} 39/83} & {\color{red} 41/95} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 16/35} & { 5/11} & {\color{red} 12/25} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  6/13} & {16/35} & {26/53} & {\color{red}  1/99} & {17/36} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {46/97} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} \\\hline
$54$ & {\color{red} 37/88} &&&& {29/65} && {30/67} &&&& {\color{red} 22/49} && { 9/20} &&&& {\color{red} 35/82} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} &\\\hline
$55$ & {\color{red} 13/31} & {29/61} & {\color{red}  1/99} & {\color{red} 29/63} & { 5/11} & {\color{red} 32/67} & {15/34} & {\color{red} 29/67} & {\color{red}  1/99} & {\color{red} 29/69} & {11/24} & {\color{red} 34/73} & {\color{red} 42/95} & {\color{red} 11/25} & {\color{red}  1/99} & { 5/11} & {\color{red} 37/83} & {\color{red} 36/79} & {\color{red} 41/92} & {\color{red} 17/41} & {18/41} & {38/83} & {\color{red}  1/99} & {\color{red} 38/85} & {\color{red} 21/46} & {\color{red}  1/99} & { 5/11} & {\color{red} 21/47} & {\color{red}  1/99} & {\color{red} 40/91} & {23/49} & {\color{red}  1/99} & {43/94} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 42/97} & {\color{red} 41/87} & {\color{red}  1/99} & {\color{red} 41/91} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 25/52} & {\color{red}  1/99} & {\color{red} 44/97} & {\color{red}  1/99} & {\color{red} 25/54} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {44/93} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {28/59} & {\color{red}  1/99} & {19/40} & {\color{red}  1/99} \\\hline
$56$ & { 3/ 7} && {\color{red}  1/99} && {\color{red} 42/95} && {11/25} && {\color{red}  1/99} && {34/73} && {\color{red} 24/53} && {\color{red}  1/99} && {\color{red} 43/92} && {\color{red} 38/81} && {\color{red}  1/99} && {\color{red} 43/96} && {14/29} && {40/89} && {41/91} && {15/31} && {\color{red} 14/31} && {\color{red}  1/99} && {\color{red} 46/99} && {27/58} && {\color{red}  1/99} && {\color{red} 30/67} && {43/92} && {\color{red}  1/99} && {\color{red} 16/37} && {\color{red} 27/61} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & {\color{red} 27/64} & {10/21} && {\color{red}  6/13} & {\color{red}  3/ 7} && {\color{red}  4/ 9} & {\color{red} 10/23} && {\color{red} 31/73} & {\color{red} 17/37} && { 9/19} & {\color{red}  3/ 7} && {\color{red} 31/79} & {19/40} && {39/82} & {\color{red}  1/99} && {\color{red}  1/99} & {\color{red} 39/82} && {\color{red} 43/92} & {\color{red} 39/89} && {\color{red} 41/91} & {\color{red} 25/56} && {\color{red} 38/83} & { 9/19} && {46/97} & {\color{red}  1/99} && {\color{red}  1/99} & {29/61} && {39/82} & {\color{red}  1/99} && {\color{red}  1/99} & {\color{red} 43/92} && {\color{red} 39/85} & {\color{red}  1/99} && {\color{red} 13/28} & {\color{red} 27/61} && {\color{red} 10/23} & {46/97} && {28/59} & {\color{red}  1/99} && {\color{red}  1/99} & {29/61} &\\\hline
$58$ & {\color{red} 23/55} && {\color{red}  1/99} && {\color{red} 10/23} && {\color{red} 32/71} && {\color{red}  1/99} && {\color{red}  4/ 9} && {36/77} && {\color{red}  1/99} && {\color{red} 32/69} && {15/32} && {\color{red}  1/99} && {14/29} && {\color{red} 40/89} && {41/91} && {15/31} && {43/95} && {\color{red} 43/95} && {\color{red} 47/99} && {\color{red}  1/99} && {41/88} && {\color{red} 16/35} && {\color{red}  1/99} && {29/62} && {\color{red} 34/77} && {\color{red}  1/99} && {\color{red} 33/73} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & {\color{red} 33/79} & {31/65} & {\color{red}  1/99} & {\color{red} 31/67} & {31/70} & {\color{red} 34/71} & {11/24} & {\color{red} 31/71} & {\color{red}  1/99} & {\color{red} 32/75} & {\color{red} 41/92} & {\color{red} 36/77} & { 6/13} & {\color{red} 10/23} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 38/83} & { 6/13} & {39/85} & {19/43} & {\color{red}  1/99} & {\color{red}  9/20} & {\color{red} 40/89} & {\color{red}  1/99} & { 6/13} & {\color{red} 41/92} & {\color{red}  1/99} & {\color{red} 23/50} & {\color{red} 42/95} & {\color{red}  1/99} & { 6/13} & {45/98} & {\color{red}  1/99} & {25/53} & {\color{red} 27/62} & {\color{red}  1/99} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red} 44/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red} 27/56} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 27/58} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {19/40} & {\color{red}  1/99} & {\color{red} 19/40} & {\color{red}  1/99} & {31/63} & {\color{red}  1/99} \\\hline
$60$ & {\color{red} 12/29} &&&& {32/71} && {33/73} &&&& { 5/11} && { 5/11} &&&& { 5/11} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 3, 3+k, 3+k+i\}$.
\end{center}


==> tables/table-g3-a04.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 2/ 5} & { 4/11} & { 1/ 3} & { 4/13} & { 1/ 3} & { 3/ 8} & { 7/17} & { 4/ 9} & { 4/ 9} & { 8/19} & { 2/ 5} & { 8/21} & { 4/11} & { 3/ 8} & { 2/ 5} & {11/26} & { 4/ 9} & { 4/ 9} & { 3/ 7} & {12/29} & { 2/ 5} & {12/31} & {13/33} & { 7/17} & { 3/ 7} & { 4/ 9} & { 4/ 9} & {16/37} & { 8/19} & {16/39} & { 2/ 5} & {17/42} & {18/43} & {19/44} & { 4/ 9} & { 4/ 9} & {10/23} & {20/47} & { 5/12} & {20/49} & { 7/17} & {11/26} & {23/53} & { 4/ 9} & { 4/ 9} & {24/55} & { 3/ 7} & { 8/19} & {12/29} & { 5/12} & {26/61} & {27/62} & { 4/ 9} & { 4/ 9} & { 7/16} & {28/65} & {14/33} & {28/67} & {29/69} & { 3/ 7} \\\hline
$2$ & { 4/11} && { 2/ 5} && { 2/ 5} && {\color{red}  7/19} && { 2/ 5} && { 8/21} && { 2/ 5} && { 2/ 5} && {\color{red} 11/29} && { 2/ 5} && {12/31} && { 2/ 5} && { 2/ 5} && {\color{red}  5/13} && { 2/ 5} && {16/41} && { 2/ 5} && { 2/ 5} && {\color{red} 19/49} && { 2/ 5} && {20/51} && { 2/ 5} && { 2/ 5} && {\color{red} 23/59} && { 2/ 5} && {24/61} && { 2/ 5} && { 2/ 5} && {\color{red}  9/23} && { 2/ 5} &\\\hline
$3$ & { 1/ 3} & { 3/ 8} & { 3/ 7} & { 1/ 3} & { 8/19} & { 7/17} & { 1/ 3} & { 5/11} & { 2/ 5} & {\color{red}  3/ 8} & { 5/11} & { 9/23} & {11/27} & {11/25} & { 5/13} & {13/30} & { 3/ 7} & {11/29} & { 5/11} & {13/31} & { 2/ 5} & { 5/11} & { 7/17} & { 8/19} & { 4/ 9} & {15/37} & {18/41} & {17/39} & {\color{red}  2/ 5} & { 5/11} & { 3/ 7} & {19/46} & { 5/11} & {19/45} & { 3/ 7} & {21/47} & { 5/12} & {23/52} & {11/25} & {\color{red}  7/17} & { 5/11} & {23/53} & { 8/19} & { 5/11} & { 3/ 7} & {13/30} & {13/29} & {25/59} & { 4/ 9} & {27/61} & {\color{red} 13/31} & { 5/11} & { 7/16} & {29/68} & { 5/11} & {29/67} & {31/71} & {31/69} & { 3/ 7} & {33/74} \\\hline
$4$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$5$ & { 5/13} & { 2/ 5} & { 3/ 7} & { 7/22} & { 4/ 9} & {\color{red}  3/ 8} & { 2/ 5} & { 6/13} & { 1/ 3} & {10/23} & {12/29} & { 2/ 5} & { 6/13} & { 5/13} & { 3/ 7} & {15/34} & { 2/ 5} & {14/31} & {15/37} & {14/33} & { 6/13} & { 2/ 5} & { 4/ 9} & { 3/ 7} & { 8/19} & { 6/13} & { 2/ 5} & {18/41} & {21/47} & {18/43} & { 5/11} & {21/50} & {10/23} & { 6/13} & { 5/12} & {22/49} & {24/55} & {22/51} & { 6/13} & {\color{red} 22/53} & { 4/ 9} & { 9/20} & { 3/ 7} & {26/57} & { 3/ 7} & {26/59} & { 6/13} & {26/61} & {14/31} & {15/34} & { 7/16} & { 6/13} & {\color{red} 14/33} & {30/67} & {33/73} & {10/23} & {16/35} & {33/76} & { 4/ 9} & { 6/13} \\\hline
$6$ & { 3/ 7} && { 7/17} && { 2/ 5} && { 3/ 7} && { 9/23} && { 3/ 7} && {11/27} && { 3/ 7} && {13/31} && {16/39} && { 3/ 7} && {15/37} && { 3/ 7} && {17/41} && { 3/ 7} && {19/45} && {22/53} && { 3/ 7} && {\color{red}  7/17} && { 3/ 7} && {23/55} && { 3/ 7} && {25/59} && {28/67} && { 3/ 7} && {\color{red} 27/65} && { 3/ 7} && {29/69} && { 3/ 7} && {31/73} &\\\hline
$7$ & {10/23} & { 3/ 8} & { 2/ 5} & { 6/19} & { 2/ 5} & { 3/ 7} & { 5/11} & { 7/15} & {13/31} & { 2/ 5} & { 1/ 3} & {13/34} & { 3/ 7} & {13/29} & { 7/15} & {17/38} & {16/39} & { 2/ 5} & {16/41} & { 3/ 7} & { 4/ 9} & {17/37} & { 7/15} & {10/23} & {19/47} & {19/48} & { 3/ 7} & {19/43} & { 5/11} & { 7/15} & {24/53} & {23/54} & { 2/ 5} & { 3/ 7} & {11/25} & {23/51} & { 6/13} & { 7/15} & {27/61} & {13/31} & { 3/ 7} & {25/57} & {13/29} & {27/59} & { 7/15} & {31/68} & {10/23} & { 3/ 7} & { 7/16} & {29/65} & { 5/11} & {31/67} & { 7/15} & {17/38} & { 3/ 7} & {31/71} & { 4/ 9} & {33/73} & {17/37} & { 7/15} \\\hline
$8$ & {11/25} && { 4/ 9} && {13/29} && {14/31} && { 5/11} && {16/35} && {17/37} && { 6/13} && {19/41} && {20/43} && { 7/15} && {22/47} && {23/49} && { 8/17} && {25/53} && {26/55} && { 9/19} && {28/59} && {29/61} && {10/21} && {31/65} && {32/67} && {11/23} && {34/71} && {35/73} && {12/25} && {37/77} && {38/79} && {13/27} && {40/83} &\\\hline
$9$ & { 4/ 9} & {11/28} & { 2/ 5} & { 1/ 3} & {12/31} & { 9/23} & {14/33} & { 8/17} & { 6/13} & { 4/ 9} & { 7/17} & {11/29} & { 1/ 3} & { 7/17} & {17/41} & {19/42} & { 8/17} & {16/35} & { 4/ 9} & {19/46} & {18/47} & {19/48} & {20/49} & {11/25} & { 8/17} & {20/43} & { 5/11} & { 4/ 9} & {23/55} & {11/28} & { 7/17} & {25/58} & {27/59} & { 8/17} & { 6/13} & {24/53} & { 4/ 9} & {27/64} & { 2/ 5} & {14/33} & {30/67} & { 8/17} & { 7/15} & {28/61} & {14/31} & { 4/ 9} & {31/73} & {31/74} & {11/25} & {35/76} & { 8/17} & {32/69} & {16/35} & {32/71} & { 4/ 9} & {35/82} & {36/83} & {19/42} & { 8/17} & {36/77} \\\hline
$10$ & { 8/19} && {13/31} && {10/23} && { 2/ 5} && { 4/ 9} && {12/29} && { 4/ 9} && {14/33} && { 4/ 9} && {16/37} && { 3/ 7} && {18/41} && {\color{red} 18/43} && { 4/ 9} && {20/47} && { 4/ 9} && {22/51} && { 4/ 9} && {24/55} && {29/67} && {26/59} && {\color{red} 26/61} && { 4/ 9} && {28/65} && { 4/ 9} && {10/23} && { 4/ 9} && {32/73} && {37/85} && {34/77} &\\\hline
$11$ & { 2/ 5} & { 8/21} & { 5/11} & {11/34} & { 3/ 7} & { 5/12} & {14/37} & { 9/19} & { 8/19} & {12/29} & { 7/15} & {12/31} & {18/43} & { 5/11} & { 1/ 3} & {21/46} & {20/47} & { 8/19} & { 9/19} & {16/39} & { 7/17} & {19/41} & { 8/21} & { 4/ 9} & { 5/11} & {11/28} & { 9/19} & {25/58} & { 5/12} & {23/49} & {\color{red} 25/61} & {27/62} & { 6/13} & {25/64} & { 6/13} & { 5/11} & { 8/19} & { 9/19} & {10/23} & { 3/ 7} & { 7/15} & { 5/12} & {33/73} & {29/63} & { 2/ 5} & { 9/19} & { 5/11} & {\color{red} 11/26} & { 8/17} & { 7/16} & { 4/ 9} & {33/71} & {35/83} & {13/28} & {17/37} & { 8/19} & { 9/19} & { 5/11} & {39/89} & {37/79} \\\hline
$12$ & { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} &\\\hline
$13$ & { 3/ 7} & { 7/18} & {16/37} & { 8/25} & { 6/13} & {11/27} & { 3/ 7} & {10/21} & { 8/21} & {19/44} & {19/45} & {13/33} & { 8/17} & { 3/ 7} & { 3/ 7} & {23/50} & { 1/ 3} & { 6/13} & {22/53} & {17/41} & {10/21} & { 3/ 7} & {25/57} & {13/29} & { 9/23} & {22/47} & { 5/12} & { 3/ 7} & {10/21} & {25/64} & { 6/13} & {29/66} & {\color{red} 11/27} & {26/55} & { 3/ 7} & {31/70} & {33/71} & {\color{red} 23/59} & { 7/15} & {16/37} & {\color{red} 32/75} & {10/21} & { 3/ 7} & { 6/13} & {36/79} & {33/80} & { 8/17} & {\color{red} 35/82} & {37/83} & {10/21} & { 2/ 5} & {34/73} & {13/29} & {19/44} & { 9/19} & { 3/ 7} & { 6/13} & {43/92} & {13/31} & {38/81} \\\hline
$14$ & {16/37} && {11/25} && {17/41} && {13/29} && { 2/ 5} && { 5/11} && { 3/ 7} && { 5/11} && {17/39} && { 5/11} && {19/43} && {26/59} && {21/47} && { 3/ 7} && {23/51} && {23/53} && { 5/11} && {25/57} && { 5/11} && {27/61} && { 5/11} && {29/65} && { 4/ 9} && {31/69} && {\color{red} 31/71} && {33/73} && {\color{red} 11/25} && { 5/11} && {35/79} && { 5/11} &\\\hline
$15$ & {17/39} & { 2/ 5} & {17/41} & { 1/ 3} & { 3/ 7} & { 9/22} & { 7/15} & {11/23} & {20/47} & {14/33} & { 9/23} & { 2/ 5} & {10/23} & {23/52} & { 9/19} & {25/54} & {23/55} & {10/23} & { 1/ 3} & {18/43} & {25/59} & { 7/15} & {11/23} & {14/31} & {\color{red}  5/12} & {27/64} & { 2/ 5} & {22/51} & {30/67} & {25/53} & {11/23} & {31/70} & { 3/ 7} & {\color{red}  9/23} & {12/29} & {\color{red} 10/23} & { 7/15} & {29/61} & {36/77} & {17/39} & {10/23} & { 2/ 5} & {\color{red} 14/33} & {37/82} & { 8/17} & {11/23} & {39/85} & {37/86} & {37/87} & {\color{red} 30/73} & {39/89} & { 7/15} & { 9/19} & {11/23} & {14/31} & {\color{red} 34/79} & { 2/ 5} & {41/96} & {44/97} & {39/83} \\\hline
$16$ & {18/41} && {19/43} && { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && {31/67} && {32/69} && {33/71} && {34/73} && { 7/15} && {36/77} && {37/79} && {38/81} && {39/83} && { 8/17} && {41/87} && {42/89} && {43/91} && {44/93} && {\color{red} 41/87} && {46/97} && {47/99} &\\\hline
$17$ & {19/43} & {17/44} & { 3/ 7} & {15/46} & {19/47} & {13/31} & { 3/ 7} & {12/25} & { 8/17} & {11/26} & {11/25} & { 7/18} & { 2/ 5} & {17/39} & { 8/19} & {27/58} & {10/21} & { 9/20} & {26/61} & {19/45} & { 1/ 3} & {11/25} & {\color{red}  5/12} & { 5/11} & {12/25} & { 8/17} & {10/23} & {23/53} & {28/71} & { 5/12} & { 3/ 7} & {33/74} & {12/25} & {28/59} & { 5/11} & {11/25} & {13/31} & { 2/ 5} & { 7/16} & {18/41} & {39/83} & {32/67} & { 8/17} & {19/43} & {\color{red}  3/ 7} & {35/88} & {11/25} & {13/30} & { 6/13} & {12/25} & { 9/19} & {43/94} & {\color{red} 17/39} & {\color{red} 33/79} & {41/97} & {\color{red} 35/81} & { 5/11} & {12/25} & {10/21} & { 8/17} \\\hline
$18$ & { 4/ 9} && {20/47} && {14/31} && { 7/17} && {16/35} && { 2/ 5} && { 6/13} && {25/59} && { 6/13} && { 4/ 9} && { 6/13} && {22/49} && {31/69} && {24/53} && {32/73} && {26/57} && { 3/ 7} && {28/61} && { 4/ 9} && { 6/13} && {30/67} && { 6/13} && {32/71} && { 6/13} && {34/75} && {43/95} && {36/79} && { 4/ 9} && {38/83} && {\color{red} 38/85} &\\\hline
$19$ & { 3/ 7} & {19/48} & {22/49} & {\color{red} 10/31} & {22/51} & {21/52} & {11/27} & {13/27} & { 4/ 9} & {16/37} & { 9/19} & { 5/13} & {25/59} & {13/30} & {24/61} & {29/62} & { 4/ 9} & { 4/ 9} & {11/23} & {20/47} & {28/67} & {31/68} & { 1/ 3} & {16/35} & {30/71} & { 4/ 9} & {13/27} & {24/55} & { 3/ 7} & { 9/19} & {30/77} & {35/78} & {35/79} & {33/80} & {13/27} & { 4/ 9} & { 7/16} & {31/65} & {14/33} & {19/43} & {40/87} & {35/88} & {42/89} & { 4/ 9} & { 4/ 9} & {35/73} & {\color{red} 16/37} & {41/94} & { 9/19} & {\color{red}  1/99} & {45/97} & {22/49} & { 4/ 9} & {13/27} & {\color{red} 18/41} & {\color{red} 36/83} & {10/21} & {\color{red} 36/85} & {16/35} & {43/93} \\\hline
$20$ & { 3/ 7} && {13/31} && {14/33} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 19/45} && {20/47} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {25/59} && {26/61} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 31/73} && {32/75} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 37/87} &\\\hline
$21$ & {22/51} & {12/31} & {23/53} & { 1/ 3} & { 5/11} & { 3/ 7} & { 4/ 9} & {14/29} & {12/29} & {\color{red}  5/12} & {26/61} & {16/41} & {10/21} & {19/43} & {13/29} & {31/66} & {26/67} & {15/34} & {\color{red} 29/69} & { 3/ 7} & {12/25} & {13/29} & {31/73} & {17/37} & { 1/ 3} & {35/76} & { 3/ 7} & {25/57} & {14/29} & { 7/16} & {35/81} & {37/82} & {\color{red} 12/31} & {10/21} & { 7/16} & {29/65} & {14/29} & {12/29} & {40/89} & { 4/ 9} & { 3/ 7} & {34/71} & { 4/ 9} & {13/29} & { 9/19} & {\color{red}  1/99} & {45/97} & {43/98} & {17/39} & {38/79} & {13/29} & {\color{red} 35/81} & {41/88} & {\color{red}  1/99} & {10/21} & {\color{red} 37/85} & {\color{red} 19/43} & {14/29} & {37/84} & { 5/11} \\\hline
$22$ & {23/53} && { 5/11} && { 8/19} && {17/37} && {25/61} && {19/41} && { 2/ 5} && { 7/15} && {29/69} && { 7/15} && {32/73} && { 7/15} && { 5/11} && {36/79} && {27/59} && {37/83} && {29/63} && {38/87} && {31/67} && { 3/ 7} && {33/71} && {42/95} && { 7/15} && { 5/11} && { 7/15} && {37/81} && { 7/15} && {39/85} && {39/85} && {41/89} &\\\hline
$23$ & {24/55} & {11/28} & { 8/19} & {19/58} & { 4/ 9} & {\color{red} 15/37} & {28/61} & {15/31} & { 3/ 7} & {18/41} & {13/31} & {17/43} & {14/31} & {29/68} & {11/23} & {33/70} & {30/71} & {22/49} & {\color{red} 12/31} & {31/74} & {11/25} & {17/38} & {13/27} & { 6/13} & {\color{red} 13/31} & {14/31} & {\color{red}  1/99} & {26/59} & {35/83} & {13/28} & {15/31} & {39/86} & { 7/16} & {19/44} & {\color{red} 13/33} & {30/67} & {40/91} & {11/23} & {15/31} & {21/47} & { 4/ 9} & {\color{red} 33/79} & {41/97} & {14/31} & { 5/11} & {37/77} & {29/61} & {\color{red} 20/47} & { 9/20} & {\color{red}  1/99} & {18/41} & {43/97} & {43/92} & {41/85} & {29/62} & {\color{red} 38/87} & {14/31} & {\color{red}  1/99} & { 4/ 9} & {17/38} \\\hline
$24$ & {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} && {34/75} && { 5/11} && {36/79} && {37/81} && {38/83} && {39/85} && {40/87} && {41/89} && { 6/13} && {43/93} && {44/95} && {45/97} && {46/99} && {27/58} && {41/88} && { 7/15} && {43/92} && {29/62} && {\color{red} 41/88} && {\color{red}  7/15} && {\color{red} 43/92} &\\\hline
$25$ & {26/59} & { 2/ 5} & { 4/ 9} & {\color{red} 12/37} & { 8/19} & {27/64} & {28/65} & {16/33} & {31/67} & {\color{red} 18/43} & { 5/11} & { 2/ 5} & {14/33} & {21/47} & {31/73} & {35/74} & {12/25} & {33/76} & { 5/11} & {22/53} & {13/33} & { 5/11} & {\color{red} 14/33} & {19/41} & {14/29} & {19/42} & {36/85} & {27/61} & {\color{red}  1/99} & { 5/11} & {38/89} & {41/90} & {16/33} & {43/92} & {40/93} & {31/69} & {\color{red}  1/99} & {\color{red} 41/96} & { 4/ 9} & {22/49} & {16/33} & {12/25} & {41/92} & { 5/11} & {\color{red} 16/39} & {\color{red}  1/99} & { 9/20} & {\color{red}  3/ 7} & {41/86} & {40/83} & {\color{red} 19/42} & { 5/11} & {19/43} & {\color{red}  1/99} & { 5/11} & {\color{red} 38/89} & {31/66} & {44/91} & {\color{red} 43/92} & {\color{red} 40/93} \\\hline
$26$ & {27/61} && { 3/ 7} && { 6/13} && {28/67} && {20/43} && {\color{red}  7/17} && {22/47} && { 2/ 5} && { 8/17} && {33/79} && { 8/17} && {36/83} && { 8/17} && {13/29} && {41/89} && { 6/13} && {14/31} && {32/69} && {43/97} && {34/73} && {27/62} && {36/77} && { 3/ 7} && {38/81} && {\color{red} 36/83} && { 8/17} && {\color{red} 13/29} && { 8/17} && { 6/13} && { 8/17} &\\\hline
$27$ & { 4/ 9} & {25/64} & {29/65} & { 1/ 3} & {29/67} & {17/41} & { 3/ 7} & {17/35} & { 5/11} & { 4/ 9} & {34/73} & {29/74} & {32/75} & { 3/ 7} & { 3/ 7} & {37/78} & {16/35} & {24/53} & {13/27} & {23/55} & { 3/ 7} & {37/84} & { 2/ 5} & {20/43} & {38/87} & {16/35} & {15/31} & { 4/ 9} & { 3/ 7} & {21/46} & {\color{red}  1/99} & {43/94} & { 8/19} & {43/96} & {17/35} & {32/71} & { 4/ 9} & {39/83} & {\color{red}  1/99} & {23/51} & {38/87} & { 3/ 7} & {\color{red} 37/78} & {36/79} & { 9/20} & {13/27} & {\color{red}  1/99} & {41/92} & {\color{red} 37/84} & {\color{red}  1/99} & {43/90} & {16/35} & { 5/11} & {43/89} & { 4/ 9} & {\color{red}  3/ 7} & {\color{red} 21/46} & {\color{red}  1/99} & {\color{red} 43/94} & {\color{red} 36/83} \\\hline
$28$ & {\color{red} 16/37} && {17/39} && {18/41} && {19/43} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 32/73} && {11/25} && {34/77} && {35/79} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 40/91} && {41/93} && {42/95} &\\\hline
$29$ & {29/67} & {27/68} & {10/23} & {23/70} & {32/71} & { 5/12} & { 5/11} & {18/37} & {16/37} & {20/47} & { 3/ 7} & {\color{red} 19/49} & {37/79} & {23/51} & {17/37} & {39/82} & {35/83} & {\color{red} 16/37} & { 3/ 7} & { 8/19} & {14/29} & {27/59} & {40/89} & { 7/15} & {36/91} & {41/92} & {16/37} & {\color{red} 41/94} & {16/33} & {17/37} & {\color{red} 17/41} & {\color{red}  4/ 9} & {\color{red}  1/99} & {23/50} & {\color{red}  5/12} & {33/73} & {18/37} & {\color{red} 38/89} & {\color{red}  3/ 7} & {\color{red} 43/98} & {\color{red}  1/99} & {\color{red} 37/79} & { 9/20} & {37/81} & {\color{red} 39/82} & {\color{red} 40/93} & {\color{red} 10/23} & {\color{red} 36/85} & {\color{red}  1/99} & {14/29} & { 5/11} & {\color{red} 11/24} & {\color{red}  7/15} & {\color{red}  1/99} & {\color{red} 41/92} & {\color{red} 40/93} & {\color{red} 41/94} & {46/95} & {11/24} & {\color{red} 23/52} \\\hline
$30$ & {10/23} && {32/71} && {\color{red} 31/73} && { 7/15} && { 8/19} && {23/49} && {\color{red}  8/19} && {25/53} && { 2/ 5} && { 9/19} && {37/89} && { 9/19} && {40/93} && { 9/19} && {43/97} && {46/99} && {\color{red} 32/71} && {\color{red} 19/42} && { 7/15} && {\color{red} 37/84} && {37/79} && {\color{red} 10/23} && {39/83} && {10/23} && {41/87} && {\color{red}  1/99} && {43/91} && {\color{red} 40/93} && { 9/19} && {\color{red} 43/97} &\\\hline
$31$ & {31/71} & {\color{red} 16/41} & {\color{red}  3/ 7} & {\color{red} 14/43} & { 5/11} & {19/45} & { 5/11} & {19/39} & {34/79} & { 7/16} & {17/39} & {20/51} & { 6/13} & {23/53} & { 8/17} & {41/86} & {\color{red}  3/ 7} & {26/57} & {\color{red} 37/89} & {25/59} & { 6/13} & {\color{red} 17/39} & {15/31} & {22/47} & {17/39} & { 6/13} & {\color{red}  1/99} & {29/67} & {43/99} & { 9/20} & {17/35} & {41/89} & {\color{red} 37/89} & { 6/13} & {\color{red}  1/99} & {34/75} & {\color{red}  8/19} & {\color{red}  5/11} & {19/39} & {\color{red} 15/34} & {\color{red}  7/16} & {\color{red} 43/99} & {\color{red}  1/99} & {38/83} & {\color{red} 10/23} & {\color{red}  8/17} & {\color{red} 41/86} & {\color{red} 37/87} & { 5/11} & {\color{red}  1/99} & {\color{red}  1/99} & { 6/13} & {\color{red} 11/25} & {15/31} & {\color{red} 22/47} & {\color{red} 41/95} & {11/24} & {\color{red}  1/99} & {\color{red}  1/99} & { 6/13} \\\hline
$32$ & {32/73} && {11/25} && {34/77} && {35/79} && { 4/ 9} && {37/83} && {38/85} && {13/29} && {40/89} && {41/91} && {14/31} && {43/95} && {44/97} && { 5/11} && {41/90} && {26/57} && {\color{red} 44/97} && {\color{red}  5/11} && {\color{red} 41/90} && {\color{red} 26/57} && {\color{red} 16/35} && {\color{red} 38/83} && {\color{red} 14/31} && {\color{red} 26/57} && {\color{red} 16/35} && {\color{red} 38/83} && {\color{red} 41/90} && {\color{red} 26/57} && {\color{red} 16/35} && {\color{red} 38/83} &\\\hline
$33$ & {11/25} & {15/38} & { 5/11} & { 1/ 3} & {10/23} & {\color{red} 33/80} & {35/81} & {20/41} & {38/83} & {22/51} & { 6/13} & {21/53} & {18/41} & { 5/11} & {\color{red}  3/ 7} & {43/90} & {43/91} & {\color{red} 18/41} & {19/41} & {26/61} & {\color{red} 17/41} & {29/63} & { 7/16} & {23/49} & {16/33} & {11/25} & {\color{red} 31/71} & {10/23} & {\color{red}  1/99} & {19/41} & {18/41} & {\color{red} 22/49} & {18/37} & {\color{red} 37/83} & {\color{red} 33/79} & { 5/11} & {\color{red}  1/99} & {\color{red} 41/92} & {\color{red}  1/99} & {\color{red} 35/81} & {20/41} & {\color{red} 38/83} & {\color{red}  1/99} & {39/85} & {\color{red}  1/99} & {\color{red}  1/99} & { 5/11} & {\color{red} 38/89} & {\color{red} 43/90} & {\color{red} 43/91} & {\color{red} 10/23} & {43/93} & {\color{red}  1/99} & {\color{red}  1/99} & {11/24} & {\color{red} 42/97} & {\color{red} 23/49} & {16/33} & {\color{red}  4/ 9} & {\color{red} 41/92} \\\hline
$34$ & {34/77} && {34/79} && {37/81} && { 3/ 7} && { 8/17} && { 3/ 7} && {26/55} && { 3/ 7} && {28/59} && {\color{red} 13/33} && {10/21} && {\color{red} 27/65} && {10/21} && {41/96} && {10/21} && {\color{red} 20/47} && {\color{red} 21/46} && {\color{red} 21/47} && {\color{red} 21/46} && {\color{red} 37/81} && {\color{red} 41/92} && { 8/17} && {\color{red} 11/25} && {42/89} && {11/25} && {44/93} && {\color{red}  1/99} && {46/97} && {\color{red}  1/99} && {29/61} &\\\hline
$35$ & {35/79} & { 2/ 5} & { 4/ 9} & {\color{red} 15/47} & {36/83} & { 3/ 7} & {11/25} & {21/43} & { 6/13} & {19/44} & {41/89} & { 2/ 5} & { 3/ 7} & {25/57} & {19/43} & {45/94} & {20/43} & {28/61} & {46/97} & { 3/ 7} & { 7/16} & {\color{red} 19/43} & {\color{red} 18/43} & { 8/17} & {26/57} & {32/69} & {17/35} & {31/71} & {19/43} & { 4/ 9} & {\color{red}  1/99} & {\color{red} 23/51} & {\color{red} 20/47} & {20/43} & {19/39} & {\color{red} 35/79} & {\color{red}  1/99} & {\color{red} 40/89} & {\color{red}  1/99} & {\color{red} 41/92} & {\color{red}  1/99} & {\color{red} 38/87} & {21/43} & {40/87} & {\color{red} 19/44} & {\color{red} 41/89} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red}  1/99} & {\color{red} 41/93} & {\color{red} 45/94} & {44/95} & {11/24} & {\color{red} 46/97} & {\color{red}  1/99} & {\color{red} 43/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  8/17} & {\color{red} 13/28} \\\hline
$36$ & { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && { 5/11} && { 5/11} && { 5/11} && { 5/11} && {\color{red} 29/65} && {30/67} && {31/69} && {32/71} && {33/73} && {34/75} && { 5/11} && { 5/11} && { 5/11} && { 5/11} && { 5/11} && {\color{red} 13/29} && {40/89} && {41/91} && {14/31} && {43/95} && {44/97} && { 5/11} && {\color{red} 24/53} && { 5/11} &\\\hline
$37$ & {\color{red} 10/23} & {11/28} & {37/85} & {\color{red}  7/23} & {13/29} & {\color{red}  7/17} & { 6/13} & {22/45} & { 4/ 9} & {24/55} & {40/93} & {37/94} & {44/95} & {43/96} & { 7/15} & {47/98} & { 4/ 9} & { 4/ 9} & {\color{red}  7/16} & {\color{red} 35/83} & {39/82} & {31/67} & { 7/15} & {25/53} & {\color{red}  2/ 5} & { 4/ 9} & { 4/ 9} & {32/73} & {18/37} & { 7/15} & {\color{red} 43/98} & {\color{red} 34/77} & {\color{red}  1/99} & {13/29} & { 4/ 9} & { 4/ 9} & {20/41} & { 7/15} & {\color{red}  1/99} & {\color{red} 37/85} & {\color{red}  1/99} & {\color{red} 43/95} & {\color{red}  1/99} & {41/89} & {22/45} & {\color{red} 27/61} & {\color{red}  1/99} & {\color{red} 40/93} & {\color{red}  1/99} & {\color{red} 44/95} & {\color{red} 43/96} & {45/97} & {\color{red} 47/98} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 39/82} & { 6/13} & { 7/15} \\\hline
$38$ & {37/85} && {13/29} && {\color{red} 22/51} && { 6/13} && {10/23} && { 9/19} && {10/23} && {29/61} && {23/54} && {31/65} && {\color{red}  1/99} && {11/23} && {\color{red}  1/99} && {11/23} && {\color{red} 32/75} && {11/23} && {\color{red} 34/79} && {\color{red} 21/46} && {\color{red} 23/53} && {\color{red} 23/50} && {\color{red} 24/53} && {\color{red}  9/20} && {\color{red}  6/13} && {\color{red}  4/ 9} && { 9/19} && {\color{red}  1/99} && {47/99} && {\color{red}  1/99} && {39/82} && {\color{red}  1/99} &\\\hline
$39$ & {38/87} & {35/88} & {11/25} & {\color{red}  1/99} & { 6/13} & {39/92} & {14/31} & {\color{red} 41/86} & {41/95} & {\color{red} 41/96} & {21/47} & {\color{red} 23/59} & { 7/15} & {27/61} & {\color{red} 16/35} & {\color{red} 22/47} & {\color{red}  7/16} & { 6/13} & {\color{red} 20/47} & {\color{red} 28/67} & {22/47} & {21/47} & {31/65} & {\color{red} 41/89} & { 4/ 9} & {34/73} & {\color{red} 26/71} & {11/25} & {\color{red}  4/ 9} & {\color{red} 37/85} & {19/39} & {\color{red} 35/79} & {21/47} & {22/47} & {\color{red}  1/99} & {37/83} & {\color{red}  1/99} & {14/31} & {21/43} & {\color{red} 38/87} & {\color{red}  1/99} & {\color{red} 21/47} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red} 41/90} & {23/47} & {\color{red} 41/95} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {46/99} & {\color{red}  1/99} & {\color{red} 27/58} & {\color{red} 37/77} & {\color{red} 38/87} & { 6/13} & {\color{red}  1/99} & {\color{red}  1/99} & {43/92} \\\hline
$40$ & {39/89} && {40/91} && {41/93} && {42/95} && {43/97} && { 4/ 9} && {41/92} && {25/56} && {\color{red} 43/97} && {\color{red} 40/91} && {\color{red} 41/92} && {\color{red} 25/56} && {\color{red} 30/67} && {\color{red} 40/91} && {\color{red} 41/92} && {\color{red} 42/95} && {\color{red} 30/67} && {\color{red}  4/ 9} && {\color{red} 40/89} && {\color{red} 44/97} && {\color{red} 37/82} && {\color{red} 35/78} && {\color{red} 29/64} && {\color{red} 44/97} && {\color{red}  5/11} && {\color{red} 41/90} && {\color{red} 29/64} && {\color{red} 44/97} && {\color{red} 37/82} && {\color{red} 33/73} &\\\hline
$41$ & {40/91} & {\color{red} 20/51} & {14/31} & {\color{red}  1/99} & { 4/ 9} & {\color{red} 23/55} & {42/97} & {\color{red} 43/90} & { 5/11} & {26/59} & { 7/15} & {\color{red} 10/29} & {22/49} & {\color{red} 40/93} & { 3/ 7} & {\color{red} 23/49} & {\color{red} 17/37} & {30/67} & {23/49} & {\color{red} 29/69} & {\color{red}  3/ 7} & {33/71} & { 4/ 9} & {\color{red} 43/93} & {\color{red} 35/74} & {22/49} & {\color{red} 22/49} & {34/77} & {\color{red}  1/99} & {37/79} & {22/49} & {\color{red}  4/ 9} & {20/41} & {\color{red} 40/91} & {\color{red}  1/99} & {38/85} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {\color{red} 25/57} & {22/45} & { 5/11} & {\color{red}  1/99} & {\color{red} 14/31} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} & {\color{red} 42/97} & {24/49} & {\color{red} 38/83} & {\color{red}  1/99} & {27/58} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 38/79} & {\color{red} 43/92} & {\color{red}  1/99} & {29/62} \\\hline
$42$ & {41/93} && {\color{red} 23/53} && {44/97} && {25/57} && {\color{red} 27/59} && {11/25} && {10/21} && {11/25} && {32/67} && {\color{red}  1/99} && {34/71} && {\color{red}  1/99} && {12/25} && {\color{red}  1/99} && {12/25} && {\color{red}  1/99} && {12/25} && {\color{red}  1/99} && {\color{red} 25/54} && {\color{red} 39/89} && {\color{red} 25/54} && {\color{red} 41/93} && {\color{red} 44/97} && {\color{red} 27/59} && {\color{red} 37/85} && {\color{red} 27/58} && {\color{red}  1/99} && {10/21} && {\color{red}  1/99} && {31/65} &\\\hline
$43$ & {42/95} & {19/48} & {43/97} & {\color{red}  1/99} & {\color{red} 43/99} & {21/50} & {13/29} & {\color{red} 45/94} & { 7/15} & {\color{red} 26/61} & {16/35} & {\color{red}  1/99} & {\color{red} 22/51} & {29/65} & {\color{red}  9/20} & {\color{red}  8/17} & { 8/17} & {\color{red} 31/69} & {\color{red}  6/13} & {30/71} & { 4/ 9} & {23/51} & {\color{red} 34/79} & {\color{red} 34/75} & { 8/17} & {36/77} & {\color{red} 37/78} & {35/79} & { 9/20} & {\color{red} 41/95} & {\color{red}  1/99} & {\color{red} 37/83} & {\color{red} 41/92} & { 8/17} & {21/43} & {13/29} & {23/51} & {\color{red} 43/97} & {\color{red}  1/99} & {\color{red} 40/91} & {\color{red}  1/99} & { 8/17} & {23/47} & {\color{red} 23/51} & {\color{red}  1/99} & {\color{red} 43/97} & {\color{red}  1/99} & {\color{red} 43/99} & {\color{red}  1/99} & {\color{red} 41/92} & {25/51} & {41/88} & {\color{red}  1/99} & {\color{red} 16/35} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 40/83} & {37/79} \\\hline
$44$ & {43/97} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && { 6/13} && { 6/13} && { 6/13} && { 6/13} && {\color{red} 23/52} && { 5/11} && {36/79} && {37/81} && {38/83} && {39/85} && {40/87} && {41/89} && { 6/13} && {\color{red} 14/31} && { 6/13} && { 6/13} && { 6/13} && {\color{red} 41/90} && {26/57} && {16/35} && {38/83} && {39/85} && {17/37} &\\\hline
$45$ & { 4/ 9} & { 2/ 5} & {27/62} & {\color{red}  1/99} & {\color{red} 29/66} & {25/59} & { 7/15} & {\color{red} 47/98} & {14/31} & { 4/ 9} & {\color{red} 29/67} & {\color{red}  1/99} & {17/37} & {\color{red} 29/67} & { 8/17} & {\color{red} 25/53} & {\color{red} 43/97} & {32/71} & { 4/ 9} & {\color{red}  1/99} & {\color{red} 19/41} & { 7/15} & {25/53} & {\color{red}  5/11} & {\color{red}  1/99} & {\color{red} 43/97} & { 9/20} & { 4/ 9} & {\color{red} 39/82} & {39/83} & {\color{red} 41/91} & {\color{red} 38/85} & {\color{red}  1/99} & {\color{red}  1/99} & {24/53} & {40/89} & {22/45} & {25/53} & {\color{red}  1/99} & {\color{red} 41/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 43/97} & {24/49} & {\color{red} 24/53} & {\color{red}  1/99} & {\color{red} 27/62} & {\color{red}  1/99} & {\color{red}  2/ 5} & {\color{red}  1/99} & { 7/15} & {26/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 43/93} & {\color{red}  1/99} & {38/81} \\\hline
$46$ & {\color{red} 24/55} && {25/56} && {26/59} && {\color{red} 19/42} && { 4/ 9} && {\color{red}  6/13} && { 4/ 9} && {11/23} && { 4/ 9} && {35/73} && {\color{red}  1/99} && {37/77} && {\color{red}  1/99} && {13/27} && {\color{red}  1/99} && {13/27} && {\color{red}  1/99} && {13/27} && {\color{red}  1/99} && {\color{red} 14/31} && {\color{red}  1/99} && {\color{red} 27/58} && {\color{red}  4/ 9} && {\color{red} 27/62} && {\color{red} 25/56} && {\color{red}  1/99} && {\color{red} 38/83} && {\color{red}  1/99} && {\color{red} 37/79} && {\color{red}  1/99} &\\\hline
$47$ & {38/87} & {\color{red} 33/85} & {13/29} & {\color{red}  1/99} & {\color{red}  9/20} & {\color{red}  5/12} & {\color{red} 31/70} & {\color{red} 37/77} & {\color{red} 27/62} & {\color{red} 28/65} & { 5/11} & {\color{red}  1/99} & { 8/17} & {31/69} & { 6/13} & {\color{red} 33/71} & {\color{red}  1/99} & {\color{red} 32/73} & { 5/11} & {32/75} & {\color{red} 42/89} & { 5/11} & {\color{red} 20/43} & {\color{red} 36/79} & { 9/20} & {38/81} & {\color{red}  1/99} & {\color{red} 36/83} & {\color{red} 44/97} & { 5/11} & {\color{red} 41/86} & {\color{red} 13/29} & { 5/11} & {42/89} & {\color{red}  1/99} & {41/91} & {\color{red}  1/99} & {\color{red}  1/99} & {23/47} & {\color{red} 42/95} & {\color{red}  1/99} & {\color{red} 44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {\color{red}  1/99} & {25/51} & {\color{red} 38/87} & {\color{red}  1/99} & {\color{red} 31/69} & {\color{red}  1/99} & {\color{red}  5/13} & {\color{red}  1/99} & { 6/13} & {27/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {31/66} \\\hline
$48$ & {\color{red} 42/97} && {\color{red} 43/99} && {\color{red} 27/62} && {\color{red} 38/87} && {\color{red} 39/89} && {\color{red} 29/66} && {\color{red}  3/ 7} && {\color{red} 38/87} && {\color{red} 39/89} && {\color{red} 43/99} && {\color{red} 27/62} && {\color{red} 41/95} && {\color{red} 42/97} && {\color{red} 43/99} && {\color{red} 40/93} && {\color{red} 41/95} && {\color{red} 38/89} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$49$ & {\color{red} 16/37} & {\color{red}  1/99} & {\color{red} 35/79} & {\color{red}  1/99} & {14/31} & { 3/ 7} & {\color{red}  7/16} & {\color{red} 38/79} & {\color{red} 33/74} & {\color{red} 29/67} & { 8/17} & {\color{red}  1/99} & {\color{red} 41/90} & {\color{red} 31/71} & {\color{red} 30/71} & {\color{red} 34/73} & {19/41} & {34/75} & { 9/19} & {\color{red}  1/99} & {\color{red} 17/39} & {\color{red} 36/79} & { 9/20} & {\color{red} 37/81} & {\color{red}  7/15} & {\color{red} 41/90} & { 9/19} & {\color{red}  1/99} & {\color{red}  1/99} & {41/87} & { 5/11} & {\color{red} 40/89} & {\color{red} 43/90} & {\color{red}  1/99} & {\color{red} 10/23} & {14/31} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {\color{red} 43/97} & {24/49} & {\color{red}  1/99} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {\color{red} 27/73} & {\color{red}  1/99} & {\color{red} 39/89} & {26/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {28/57} & {\color{red} 33/73} & {\color{red}  1/99} & {39/83} \\\hline
$50$ & {\color{red} 29/67} && {27/61} && {\color{red} 41/92} && {29/65} && {\color{red} 21/46} && {\color{red} 30/67} && {\color{red} 33/71} && {13/29} && {12/25} && {\color{red}  1/99} && {38/79} && {\color{red}  1/99} && {40/83} && {\color{red}  1/99} && {14/29} && {\color{red}  1/99} && {\color{red} 43/91} && {\color{red}  1/99} && {\color{red} 44/95} && {\color{red}  1/99} && {\color{red}  5/11} && {\color{red}  1/99} && {\color{red} 25/56} && {\color{red}  1/99} && {\color{red} 29/66} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  6/13} &\\\hline
$51$ & {\color{red} 41/94} & {\color{red}  1/99} & {\color{red} 17/39} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red} 27/65} & { 5/11} & {\color{red} 32/67} & { 8/17} & {10/23} & {\color{red} 35/78} & {\color{red}  1/99} & {\color{red} 11/25} & {33/73} & {\color{red} 37/81} & {\color{red}  7/15} & { 9/19} & {\color{red} 11/25} & {20/43} & {\color{red}  1/99} & {\color{red}  1/99} & {37/81} & {\color{red} 18/41} & {\color{red} 38/83} & {\color{red} 27/58} & { 8/17} & {\color{red} 22/47} & {\color{red}  1/99} & { 5/11} & {\color{red} 43/96} & {\color{red}  1/99} & {\color{red} 41/91} & {\color{red} 41/90} & {44/93} & {\color{red} 45/94} & {43/95} & {\color{red} 43/96} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} & {\color{red} 27/58} & {25/51} & {26/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/84} & {27/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {29/59} & { 8/17} \\\hline
$52$ & {\color{red} 38/87} && {\color{red}  4/ 9} && { 6/13} && {31/67} && {32/69} && {33/71} && {34/73} && { 7/15} && {\color{red} 41/88} && { 7/15} && {\color{red} 39/86} && { 7/15} && {\color{red} 21/47} && {\color{red} 38/87} && {\color{red} 40/89} && { 6/13} && {43/93} && {44/95} && {45/97} && {46/99} && {27/58} && {41/88} && { 7/15} && {\color{red} 38/83} && {\color{red} 40/89} && {\color{red} 34/77} && {\color{red} 27/61} && {\color{red} 33/73} && {\color{red} 22/57} && {\color{red}  9/29} &\\\hline
$53$ & {\color{red} 27/62} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red} 18/41} & {\color{red}  1/99} & {\color{red} 31/68} & {\color{red} 11/23} & {16/35} & {\color{red} 30/71} & {\color{red} 19/43} & {\color{red}  1/99} & {\color{red} 37/82} & {\color{red} 11/25} & { 9/19} & {\color{red} 36/77} & {\color{red} 11/24} & {36/79} & {\color{red}  1/99} & {\color{red}  1/99} & { 7/15} & {\color{red} 37/83} & {\color{red} 47/99} & {\color{red} 39/85} & {\color{red}  1/99} & {\color{red} 11/24} & { 5/11} & {\color{red}  1/99} & {\color{red} 23/49} & {43/91} & {\color{red} 38/83} & {\color{red} 14/31} & {\color{red}  1/99} & {\color{red}  1/99} & {11/24} & {44/97} & {\color{red} 47/98} & {47/99} & {\color{red}  1/99} & {\color{red} 41/92} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  3/ 7} & {16/35} & {26/53} & {\color{red} 38/83} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  7/22} & {28/57} & {\color{red} 43/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/67} \\\hline
$54$ & { 4/ 9} && {\color{red} 32/73} && {30/67} && {\color{red}  9/20} && {32/71} && {\color{red} 23/50} && {14/31} && {\color{red} 36/77} && {\color{red}  7/16} && {13/27} && {\color{red}  1/99} && {41/85} && {\color{red}  1/99} && {43/89} && {\color{red}  1/99} && {15/31} && {\color{red}  1/99} && {\color{red} 46/97} && {\color{red}  1/99} && {\color{red} 27/58} && {\color{red}  1/99} && {\color{red} 16/35} && {\color{red}  1/99} && {\color{red} 40/89} && {\color{red}  1/99} && {\color{red} 22/59} && {\color{red}  1/99} && {\color{red}  4/ 9} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & {\color{red}  7/16} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {\color{red} 40/89} & {\color{red}  1/99} & {\color{red} 19/43} & {\color{red} 34/71} & { 4/ 9} & {32/73} & {17/37} & {\color{red}  1/99} & { 9/19} & { 5/11} & {\color{red} 39/86} & {\color{red} 37/79} & {\color{red}  1/99} & { 4/ 9} & {\color{red} 38/85} & {\color{red}  1/99} & {10/21} & {39/85} & {22/47} & {\color{red} 40/87} & {\color{red}  1/99} & {\color{red} 41/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/92} & {\color{red} 38/93} & {\color{red}  8/17} & {\color{red} 43/95} & {11/24} & {46/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/77} & {\color{red} 25/56} & {\color{red}  1/99} & {10/21} & {\color{red}  1/99} & {38/83} & {\color{red}  1/99} & {\color{red}  1/99} & {27/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/82} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {29/59} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$56$ & {\color{red} 36/83} && {\color{red} 29/67} && {\color{red} 10/23} && {\color{red} 31/71} && {\color{red} 10/23} && {\color{red} 17/39} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & {\color{red} 18/41} & {\color{red}  1/99} & {\color{red} 43/97} & {\color{red}  1/99} & {16/35} & {\color{red}  1/99} & { 4/ 9} & {\color{red} 35/73} & {\color{red}  4/ 9} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & { 6/13} & {35/79} & {\color{red} 41/92} & {\color{red} 38/81} & {\color{red} 41/90} & {38/83} & {10/21} & {\color{red}  1/99} & { 6/13} & {\color{red} 41/92} & {\color{red}  1/99} & {\color{red} 41/89} & {23/49} & { 6/13} & {\color{red} 37/79} & {\color{red}  1/99} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {\color{red} 44/97} & {\color{red} 25/53} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red}  1/99} & {\color{red}  1/99} & {39/82} & {\color{red}  1/99} & {\color{red} 30/67} & {\color{red} 38/79} & {\color{red}  1/99} & {\color{red}  1/99} & {39/85} & {\color{red}  1/99} & {\color{red} 37/79} & {\color{red}  1/99} & {\color{red}  1/99} & {28/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 33/89} & {\color{red}  1/99} & {\color{red}  1/99} & {30/61} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$58$ & {\color{red} 11/25} && {31/69} && {\color{red} 35/79} && {33/73} && {\color{red} 44/97} && { 5/11} && {\color{red} 36/79} && { 5/11} && {\color{red} 39/83} && { 5/11} && {14/29} && {\color{red}  1/99} && {44/91} && {\color{red}  1/99} && {46/95} && {\color{red}  1/99} && {16/33} && {\color{red}  1/99} && {\color{red} 39/82} && {\color{red}  1/99} && {\color{red} 43/92} && {\color{red}  1/99} && {\color{red} 17/37} && {\color{red}  1/99} && {\color{red} 33/73} && {\color{red}  1/99} && {\color{red} 41/92} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & {\color{red} 40/93} & {\color{red}  1/99} & {\color{red} 19/43} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {17/37} & {\color{red} 12/25} & {\color{red} 35/76} & {34/77} & {\color{red} 21/47} & {\color{red}  1/99} & {\color{red} 38/85} & {\color{red}  4/ 9} & {\color{red} 41/89} & {\color{red} 39/83} & {10/21} & {\color{red} 38/85} & {\color{red} 43/94} & {\color{red}  1/99} & {\color{red}  1/99} & {41/89} & {\color{red}  4/ 9} & {\color{red}  6/13} & {\color{red} 43/92} & {\color{red} 14/31} & { 8/17} & {\color{red}  1/99} & {11/24} & {\color{red} 43/93} & {\color{red}  1/99} & {\color{red}  5/11} & {\color{red} 40/89} & {29/61} & {\color{red} 26/55} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {31/65} & {\color{red} 40/83} & {17/37} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  6/13} & {29/59} & {43/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 11/25} & {31/63} & {\color{red}  1/99} \\\hline
$60$ & {19/43} && {\color{red} 31/71} && {\color{red} 33/73} && { 7/15} && {36/77} && {37/79} && {38/81} && {39/83} && { 8/17} && {\color{red} 23/49} && { 8/17} && {\color{red} 40/91} && {\color{red} 40/93} && {\color{red} 24/53} && {\color{red} 15/34} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 26/57} && { 7/15} && {43/92} && {29/62} && {37/79} && {38/81} && {31/66} && {39/83} && { 8/17} && {\color{red} 31/67} && {\color{red} 41/90} && {\color{red} 31/84} && {\color{red} 41/93} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g3-a05.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 5/12} & { 5/13} & {\color{red}  4/11} & { 1/ 3} & { 5/16} & { 1/ 3} & {\color{red}  7/19} & { 2/ 5} & { 3/ 7} & { 5/11} & { 5/11} & {10/23} & { 5/12} & { 2/ 5} & { 5/13} & {10/27} & {11/29} & { 2/ 5} & {13/31} & { 7/16} & { 5/11} & { 5/11} & {15/34} & { 3/ 7} & { 5/12} & {15/37} & {15/38} & { 2/ 5} & {17/41} & { 3/ 7} & {19/43} & { 5/11} & { 5/11} & { 4/ 9} & {10/23} & {20/47} & { 5/12} & {20/49} & { 7/17} & {11/26} & {23/53} & { 4/ 9} & { 5/11} & { 5/11} & {25/56} & {25/57} & {25/58} & {25/59} & { 5/12} & {13/31} & { 3/ 7} & { 7/16} & {29/65} & { 5/11} & { 5/11} & {30/67} & {15/34} & {10/23} & { 3/ 7} & {30/71} \\\hline
$2$ & { 5/13} && { 1/ 3} && { 6/19} && { 1/ 3} && { 9/23} && { 5/12} && { 2/ 5} && {11/29} && {12/31} && {13/33} && { 2/ 5} && { 5/12} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} &\\\hline
$3$ & {\color{red}  5/14} & { 1/ 3} & { 7/16} & { 2/ 5} & { 1/ 3} & { 8/19} & {10/23} & { 1/ 3} & { 9/22} & { 6/13} & { 5/13} & { 2/ 5} & { 6/13} & { 2/ 5} & {11/28} & {13/29} & {14/33} & {12/31} & { 7/16} & { 4/ 9} & {\color{red} 13/34} & { 3/ 7} & { 6/13} & { 2/ 5} & { 8/19} & { 6/13} & {18/43} & {17/41} & {19/42} & {10/23} & { 9/22} & { 4/ 9} & {22/49} & {\color{red} 19/47} & { 7/16} & { 6/13} & {22/53} & {22/51} & { 6/13} & { 3/ 7} & {23/54} & { 5/11} & {26/59} & { 8/19} & {13/29} & {14/31} & {\color{red}  5/12} & {27/61} & { 6/13} & {14/33} & { 7/16} & { 6/13} & {10/23} & {29/67} & {31/68} & { 4/ 9} & { 3/ 7} & {32/71} & {34/75} & {\color{red} 31/73} \\\hline
$4$ & { 1/ 3} && { 3/ 7} && { 6/19} && { 3/ 7} && { 1/ 3} && { 2/ 5} && {12/31} && {11/29} && { 3/ 7} && {14/37} && { 3/ 7} && {16/41} && {16/39} && { 2/ 5} && {19/47} && { 3/ 7} && { 7/17} && { 3/ 7} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} &\\\hline
$5$ & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} && { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} &\\\hline
$6$ & { 3/ 8} && { 8/19} && { 1/ 3} && {12/29} && { 2/ 5} && { 1/ 3} && { 7/16} && {12/31} && { 5/13} && { 3/ 7} && {14/37} && {19/45} && {17/41} && {19/49} && { 7/16} && {\color{red} 19/47} && { 2/ 5} && {22/51} && {24/59} && {26/61} && {\color{red}  8/19} && {27/65} && { 7/16} && {29/69} && {30/71} && {\color{red} 29/67} && {32/75} && { 3/ 7} && {34/79} && {35/81} &\\\hline
$7$ & { 7/17} & { 5/13} & { 4/ 9} & { 3/ 7} & { 7/22} & { 2/ 5} & {11/24} & { 2/ 5} & { 7/17} & { 8/17} & { 3/ 7} & { 1/ 3} & {16/37} & {14/31} & { 5/13} & {\color{red}  2/ 5} & { 8/17} & { 3/ 7} & {17/43} & { 5/11} & {17/38} & { 9/23} & {20/47} & {19/41} & { 3/ 7} & { 7/17} & { 8/17} & { 4/ 9} & {21/53} & { 4/ 9} & {11/24} & { 3/ 7} & { 8/19} & { 8/17} & {23/52} & { 2/ 5} & {28/61} & { 5/11} & { 3/ 7} & { 7/16} & {27/58} & {26/59} & {28/67} & { 8/17} & {14/31} & { 3/ 7} & {32/71} & { 6/13} & {29/66} & {16/37} & { 8/17} & {31/69} & { 3/ 7} & { 6/13} & {11/24} & {32/73} & { 4/ 9} & { 7/15} & {17/38} & { 3/ 7} \\\hline
$8$ & { 4/ 9} && { 7/18} && {10/31} && { 2/ 5} && { 4/ 9} && {15/37} && { 1/ 3} && {13/33} && { 3/ 7} && { 4/ 9} && { 7/18} && {16/41} && {18/43} && { 4/ 9} && {23/55} && {\color{red} 19/49} && { 7/17} && {23/53} && { 4/ 9} && { 2/ 5} && {\color{red} 24/59} && {\color{red} 26/61} && { 4/ 9} && {31/73} && {31/75} && {\color{red} 29/69} && {\color{red} 31/71} && { 4/ 9} && {35/83} && {36/85} &\\\hline
$9$ & {13/29} & { 2/ 5} & { 9/22} & {\color{red}  3/ 8} & { 1/ 3} & { 2/ 5} & { 2/ 5} & { 4/ 9} & {13/28} & { 9/19} & {17/39} & { 2/ 5} & { 8/19} & { 1/ 3} & {13/34} & { 8/19} & { 4/ 9} & {17/37} & { 9/19} & {11/24} & { 3/ 7} & {17/41} & {20/51} & { 5/13} & {22/53} & { 4/ 9} & {21/46} & {22/47} & { 9/19} & {13/29} & {25/59} & { 8/19} & {24/61} & {13/31} & { 4/ 9} & { 5/11} & {13/28} & { 9/19} & {31/67} & {15/34} & {29/69} & { 2/ 5} & {30/71} & { 4/ 9} & {29/64} & { 6/13} & {31/66} & { 9/19} & { 5/11} & {17/39} & {\color{red}  8/19} & {17/40} & { 4/ 9} & {33/73} & {17/37} & { 7/15} & { 9/19} & {20/43} & {13/29} & {19/44} \\\hline
$10$ & {14/31} && { 5/11} &&&& {17/37} && { 6/13} && {19/41} && {20/43} &&&& {22/47} && {23/49} && { 8/17} && {25/53} &&&& { 9/19} && {28/59} && {29/61} && {10/21} &&&& {32/67} && {11/23} && {34/71} && {35/73} &&&& {37/77} && {38/79} && {13/27} && {40/83} &&&& {14/29} && {43/89} &\\\hline
$11$ & { 5/11} & { 7/17} & { 3/ 7} & { 2/ 5} & {12/37} & { 8/21} & { 3/ 7} & { 2/ 5} & {18/41} & {10/21} & {15/32} & { 5/11} & {19/45} & { 3/ 7} & { 7/18} & { 1/ 3} & { 3/ 7} & {16/39} & {22/51} & { 6/13} & {10/21} & {20/43} & { 5/11} & { 3/ 7} & {19/46} & {\color{red} 18/47} & {23/59} & { 3/ 7} & {26/61} & {14/31} & {10/21} & {25/53} & {25/54} & { 5/11} & {29/67} & { 7/17} & { 9/23} & { 3/ 7} & {\color{red} 30/71} & { 4/ 9} & {34/73} & {10/21} & {15/32} & { 6/13} & { 5/11} & {17/39} & {33/79} & { 2/ 5} & { 3/ 7} & {18/41} & {38/83} & {10/21} & {35/74} & { 7/15} & {35/76} & { 5/11} & {39/89} & {19/45} & { 3/ 7} & {10/23} \\\hline
$12$ & {10/23} && { 2/ 5} && { 1/ 3} && {16/41} && {18/43} && { 5/11} && { 3/ 7} && {19/49} && { 1/ 3} && { 9/22} && { 5/11} && { 4/ 9} && {20/47} && {24/61} && {25/63} && {28/65} && { 5/11} && {25/57} && {25/59} && {29/73} && {31/75} && { 5/11} && {30/67} && {\color{red} 10/23} && {\color{red} 30/71} && { 2/ 5} && {38/87} && { 5/11} && {\color{red} 35/79} && {\color{red} 35/81} &\\\hline
$13$ & { 5/12} & { 2/ 5} & { 6/13} & { 2/ 5} & {\color{red}  9/28} & { 3/ 7} & {19/43} & { 9/23} & { 2/ 5} & {11/23} & {10/23} & { 3/ 7} & {17/36} & {15/37} & {15/38} & { 6/13} & {23/53} & { 1/ 3} & {24/55} & {13/28} & { 8/19} & {10/23} & {11/23} & {20/47} & { 5/12} & {23/49} & { 3/ 7} & {20/51} & { 6/13} & { 5/11} & {\color{red}  9/23} & {15/34} & {11/23} & {10/23} & {\color{red} 25/58} & {28/59} & {\color{red} 31/73} & {\color{red} 25/61} & {29/62} & {17/38} & {\color{red} 25/64} & { 6/13} & {37/79} & {17/40} & { 4/ 9} & {11/23} & {\color{red}  3/ 7} & {\color{red}  3/ 7} & {17/36} & {19/43} & {\color{red} 12/29} & { 7/15} & {41/89} & { 2/ 5} & { 6/13} & {11/23} & {10/23} & {21/47} & {39/82} & { 7/16} \\\hline
$14$ & { 2/ 5} && {18/41} && {14/43} && {14/31} && {18/47} && { 3/ 7} && {\color{red}  7/17} && { 5/13} && {11/24} && { 1/ 3} && { 4/ 9} && { 5/12} && { 3/ 7} && {29/65} && {\color{red} 26/67} && { 5/11} && {28/71} && {26/59} && {32/75} && { 3/ 7} && {11/24} && {32/81} && {31/69} && { 5/12} && {32/73} && {40/89} && { 3/ 7} && {36/79} && {\color{red}  1/99} && {37/83} &\\\hline
$15$ & { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} && { 2/ 5} & { 2/ 5} & { 2/ 5} & { 2/ 5} &\\\hline
$16$ & {11/26} && {13/29} && {10/31} && { 3/ 7} && {11/26} && { 5/13} && { 6/13} && {16/41} && {18/43} && { 4/ 9} && { 1/ 3} && { 6/13} && {28/67} && {11/26} && { 5/11} && {\color{red} 22/57} && {11/25} && {27/61} && {31/79} && { 6/13} && {35/83} && {\color{red} 36/85} && {32/71} && {\color{red} 28/73} && { 6/13} && {34/77} && {11/26} && {37/81} && {14/33} && {41/92} &\\\hline
$17$ & { 4/ 9} & {11/27} & {21/47} & { 5/12} & {16/49} & {11/27} & { 8/17} & { 3/ 7} & { 4/ 9} & {13/27} & { 2/ 5} & {11/28} & {25/57} & {13/29} & {23/59} & {18/43} & {21/44} & { 4/ 9} & { 4/ 9} & {15/32} & {28/65} & { 1/ 3} & {29/67} & { 8/17} & {11/26} & {23/53} & {13/27} & { 4/ 9} & {\color{red} 30/73} & {17/37} & {34/75} & {15/38} & { 3/ 7} & {29/61} & {27/62} & { 4/ 9} & {13/27} & {18/41} & {33/83} & {19/42} & { 8/17} & {\color{red} 29/69} & {\color{red}  3/ 7} & {34/71} & { 4/ 9} & { 4/ 9} & {43/91} & {21/46} & {\color{red}  1/99} & {21/47} & {37/78} & {\color{red} 34/79} & {\color{red}  7/16} & {13/27} & { 4/ 9} & {21/50} & {27/58} & { 8/17} & {\color{red}  1/99} & {23/52} \\\hline
$18$ & {21/47} && { 3/ 7} && { 1/ 3} && { 3/ 7} && {17/37} && { 8/19} && {11/28} && {17/43} && { 4/ 9} && {13/28} && { 3/ 7} && { 1/ 3} && {22/53} && { 5/11} && {34/75} && { 3/ 7} && {\color{red} 24/61} && { 4/ 9} && { 6/13} && {37/85} && {\color{red} 11/28} && {37/89} && {33/73} && {13/28} && { 3/ 7} && {\color{red}  1/99} && { 4/ 9} && {38/83} && {26/57} && { 3/ 7} &\\\hline
$19$ & {22/49} & {12/29} & { 7/16} & {12/29} & {\color{red} 11/34} & { 3/ 7} & {23/55} & { 3/ 7} & { 9/19} & {14/29} & {26/59} & { 2/ 5} & {13/29} & {12/31} & {17/44} & { 4/ 9} & {27/65} & { 5/11} & {23/48} & { 8/17} & {10/23} & {22/51} & {31/71} & { 1/ 3} & {23/54} & {13/29} & {11/25} & { 9/19} & {14/29} & { 6/13} & {34/79} & {27/61} & {\color{red} 12/29} & {\color{red} 16/41} & { 7/16} & { 3/ 7} & {39/85} & {32/67} & {14/29} & { 5/11} & {\color{red}  3/ 7} & {13/29} & {\color{red}  1/99} & {\color{red} 31/73} & {33/74} & {21/47} & { 9/19} & {37/77} & {46/97} & {22/49} & {\color{red}  7/16} & {\color{red}  3/ 7} & {\color{red}  1/99} & {\color{red} 36/83} & {13/29} & { 6/13} & {41/86} & {14/29} & {43/92} & {\color{red} 38/89} \\\hline
$20$ & {23/51} && {24/53} &&&& {26/57} && {27/59} && {28/61} && {29/63} &&&& {31/67} && {32/69} && {33/71} && {34/73} &&&& {36/77} && {37/79} && {38/81} && {39/83} &&&& {41/87} && {42/89} && {43/91} && {44/93} &&&& {46/97} && {47/99} && {29/61} && {\color{red} 44/93} &&&& {\color{red} 46/97} && {\color{red} 47/99} &\\\hline
$21$ & {24/53} & {13/31} & {24/55} & { 3/ 7} & { 1/ 3} & {13/31} & {17/38} & {13/31} & {27/61} & {15/31} & {10/21} & { 7/16} & { 2/ 5} & { 4/ 9} & { 9/23} & {\color{red} 12/31} & {14/31} & { 3/ 7} & {31/71} & {17/36} & {25/52} & {17/37} & {32/75} & {14/31} & { 3/ 7} & {\color{red}  1/99} & {34/79} & {26/59} & {35/81} & {19/41} & {15/31} & {10/21} & {38/85} & {19/43} & {29/66} & {\color{red} 26/67} & {13/31} & {31/69} & { 3/ 7} & {21/46} & {15/31} & {35/73} & {44/95} & { 7/16} & {17/38} & { 3/ 7} & {\color{red}  1/99} & {14/31} & {\color{red}  7/16} & {23/51} & {39/82} & {40/83} & {10/21} & {24/53} & {14/31} & {\color{red} 38/87} & {\color{red}  1/99} & {\color{red} 41/96} & {\color{red}  4/ 9} & {25/56} \\\hline
$22$ & { 5/11} && { 3/ 7} && {\color{red} 12/37} && {\color{red} 25/61} && { 3/ 7} && {20/43} && { 7/16} && { 9/23} && {28/71} && {22/51} && {15/32} && { 5/11} && { 8/19} && {\color{red}  1/99} && { 7/16} && {39/85} && { 6/13} && {29/67} && {\color{red}  9/23} && {\color{red} 32/77} && {42/95} && { 7/15} && { 5/11} && {\color{red} 33/79} && {\color{red}  1/99} && {\color{red} 36/83} && {15/32} && {40/87} && {\color{red} 38/89} && {\color{red}  1/99} &\\\hline
$23$ & {15/34} & {14/33} & {27/59} & {14/33} & {20/61} & {\color{red} 14/33} & { 4/ 9} & {14/33} & {27/65} & {16/33} & { 5/11} & { 4/ 9} & {11/23} & { 2/ 5} & {19/48} & { 4/ 9} & {32/73} & {13/33} & {\color{red} 31/75} & { 9/19} & { 5/11} & { 5/11} & {27/56} & {25/57} & {\color{red} 34/81} & {19/41} & {36/83} & {\color{red}  1/99} & {37/85} & {20/43} & {\color{red} 37/87} & { 5/11} & {16/33} & {30/67} & {15/34} & {11/23} & {\color{red} 40/93} & {\color{red}  1/99} & {43/95} & {11/24} & {\color{red}  2/ 5} & { 3/ 7} & {16/33} & { 5/11} & {35/78} & {38/79} & {\color{red}  7/16} & {\color{red} 34/81} & {\color{red} 19/41} & {\color{red}  7/16} & {\color{red}  1/99} & { 4/ 9} & {\color{red} 20/43} & { 5/11} & { 5/11} & {43/89} & {\color{red}  4/ 9} & {40/91} & {11/23} & {\color{red} 23/53} \\\hline
$24$ & { 3/ 7} && {27/61} && { 1/ 3} && {19/41} && { 7/17} && {15/34} && {20/47} && {19/49} && { 8/17} && {30/77} && {35/79} && {25/57} && {25/59} && { 8/17} && {\color{red}  1/99} && { 6/13} && {15/34} && {\color{red} 10/23} && {43/95} && {\color{red}  1/99} && { 7/15} && {\color{red}  7/17} && {\color{red} 35/79} && {\color{red} 35/81} && {\color{red}  1/99} && { 8/17} && {\color{red}  1/99} && {41/89} && {\color{red} 40/91} && {\color{red}  1/99} &\\\hline
$25$ & { 3/ 7} & { 3/ 7} & { 3/ 7} & { 3/ 7} && { 3/ 7} & { 3/ 7} & { 3/ 7} & { 3/ 7} && { 3/ 7} & {20/47} & { 3/ 7} & { 3/ 7} && { 3/ 7} & { 3/ 7} & { 3/ 7} & {\color{red} 23/54} && { 3/ 7} & { 3/ 7} & { 3/ 7} & { 3/ 7} && {26/61} & { 3/ 7} & { 3/ 7} & { 3/ 7} && { 3/ 7} & { 3/ 7} & {\color{red} 29/68} & { 3/ 7} && { 3/ 7} & { 3/ 7} & { 3/ 7} & { 3/ 7} && { 3/ 7} & { 3/ 7} & { 3/ 7} & { 3/ 7} && { 3/ 7} & {\color{red} 35/82} & { 3/ 7} & { 3/ 7} && { 3/ 7} & { 3/ 7} & { 3/ 7} & {\color{red} 38/89} && { 3/ 7} & { 3/ 7} & { 3/ 7} & { 3/ 7} &\\\hline
$26$ & { 4/ 9} && { 6/13} && {22/67} && {10/23} && { 4/ 9} && { 5/12} && {23/49} && {20/51} && {23/53} && { 4/ 9} && {\color{red}  7/18} && {17/36} && {26/61} && { 4/ 9} && { 6/13} && {\color{red}  1/99} && {44/95} && {31/71} && { 4/ 9} && { 7/15} && {\color{red}  1/99} && {\color{red} 18/41} && { 4/ 9} && {\color{red}  1/99} && { 8/17} && {\color{red}  1/99} && {\color{red} 39/89} && { 6/13} && {\color{red}  1/99} && {\color{red} 44/95} &\\\hline
$27$ & {29/65} & {16/37} & {30/67} & {16/37} & { 1/ 3} & {16/37} & {33/71} & { 4/ 9} & {21/46} & {18/37} & {31/75} & { 8/19} & {34/77} & {17/39} & {31/79} & { 2/ 5} & {13/27} & { 5/11} & {17/37} & {10/21} & {\color{red} 12/29} & {17/43} & {38/87} & { 5/11} & {13/31} & { 4/ 9} & {31/64} & {17/37} & {41/93} & {22/47} & {\color{red} 41/95} & {\color{red}  1/99} & {\color{red} 42/97} & {\color{red} 33/71} & { 4/ 9} & {33/73} & {18/37} & {\color{red} 41/93} & {16/37} & {\color{red} 21/47} & {\color{red} 17/39} & {\color{red}  1/99} & {\color{red} 41/97} & {13/27} & {37/82} & {38/83} & {\color{red} 10/21} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 38/87} & {\color{red}  5/11} & {\color{red}  1/99} & { 4/ 9} & {44/91} & {21/46} & {\color{red} 23/51} & {\color{red} 22/47} & {\color{red} 41/95} & {\color{red}  1/99} & {\color{red} 42/97} \\\hline
$28$ & {30/67} && {10/23} && {\color{red} 14/43} && { 4/ 9} && {22/47} && { 3/ 7} && { 8/19} && {21/53} && {17/38} && { 9/19} && {26/59} && {\color{red} 15/38} && { 3/ 7} && {14/31} && { 9/19} && {17/38} && {\color{red}  1/99} && {32/73} && { 7/15} && {\color{red} 39/86} && {\color{red}  8/19} && {\color{red}  1/99} && {37/83} && { 8/17} && {\color{red}  7/16} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 14/31} && { 9/19} && {\color{red}  1/99} &\\\hline
$29$ & {31/69} & {17/39} & {19/42} & {17/39} & {24/73} & {\color{red} 17/39} & {32/75} & {17/39} & {36/77} & {19/39} & {35/79} & {17/40} & { 6/13} & {\color{red} 17/41} & {\color{red}  7/18} & { 5/11} & { 2/ 5} & {19/43} & {14/29} & {21/44} & {39/89} & {19/45} & { 6/13} & {\color{red}  1/99} & {27/64} & { 6/13} & {\color{red} 14/33} & {11/24} & {33/68} & {\color{red}  5/11} & {\color{red} 43/99} & {32/71} & {\color{red} 19/44} & {\color{red}  1/99} & {\color{red} 16/37} & { 6/13} & {\color{red} 33/76} & {\color{red} 36/77} & {19/39} & {\color{red} 22/49} & {\color{red} 17/39} & {37/81} & {17/39} & {\color{red}  1/99} & {19/42} & {\color{red} 19/44} & {\color{red} 19/43} & {14/29} & {\color{red} 21/44} & {\color{red} 39/89} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red}  1/99} & {43/94} & {\color{red}  1/99} & {\color{red} 11/24} & {47/97} & {\color{red} 23/49} & {\color{red} 43/99} \\\hline
$30$ & {32/71} && {33/73} &&&& { 5/11} && {36/79} && {37/81} && {38/83} &&&& {40/87} && {41/89} && { 6/13} && {43/93} &&&& {45/97} && {46/99} && {\color{red}  6/13} && {\color{red} 43/93} &&&& {\color{red} 45/97} && {\color{red} 46/99} && {\color{red} 27/58} && {\color{red} 41/88} &&&& {\color{red} 45/97} && {\color{red} 41/89} && {\color{red} 27/58} && {\color{red} 43/93} &&&& {\color{red} 45/97} && {\color{red} 46/99} &\\\hline
$31$ & {33/73} & {18/41} & {11/25} & {18/41} & {\color{red} 15/46} & {18/41} & {11/24} & {18/41} & { 4/ 9} & {20/41} & {39/83} & { 3/ 7} & {\color{red} 17/41} & { 5/11} & {11/28} & {\color{red} 17/41} & {19/41} & { 2/ 5} & {40/91} & {11/23} & {15/31} & {21/47} & {27/64} & { 6/13} & {14/33} & {\color{red}  1/99} & { 5/11} & {\color{red} 10/23} & {\color{red} 27/62} & {\color{red} 21/46} & {35/72} & {\color{red} 33/73} & {\color{red} 16/37} & {19/41} & {\color{red} 33/76} & {\color{red}  1/99} & {\color{red} 17/39} & {36/79} & {\color{red}  7/16} & {\color{red} 23/51} & {20/41} & {\color{red} 39/83} & {\color{red} 18/41} & {\color{red} 10/23} & {39/86} & {\color{red}  1/99} & {\color{red}  1/99} & {41/89} & {\color{red}  1/99} & {\color{red} 40/91} & {\color{red} 11/23} & {15/31} & {\color{red} 21/47} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 43/93} & {\color{red}  1/99} & {\color{red} 27/62} \\\hline
$32$ & {34/75} && { 4/ 9} && {\color{red} 15/47} && { 3/ 7} && {36/83} && {25/53} && {19/42} && {\color{red} 35/89} && { 3/ 7} && {27/61} && {10/21} && {43/97} && {\color{red} 28/67} && {\color{red}  1/99} && {32/71} && {10/21} && {\color{red} 34/75} && {34/77} && {\color{red}  1/99} && {19/42} && {\color{red} 43/94} && { 8/17} && {13/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 41/93} && { 9/19} && {\color{red}  9/20} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$33$ & { 5/11} & {19/43} & {36/79} & {19/43} & { 1/ 3} & {19/43} & {37/83} & {19/43} & {36/85} & {21/43} & {25/54} & { 5/11} & {42/89} & {19/45} & {23/58} & {10/23} & {41/93} & {\color{red} 18/43} & {\color{red} 29/74} & {23/48} & {20/43} & { 6/13} & {16/33} & {\color{red} 37/89} & {29/68} & {23/51} & {\color{red} 38/87} & {\color{red}  1/99} & {\color{red} 31/72} & {\color{red} 11/24} & {\color{red} 11/25} & {20/43} & {37/76} & { 5/11} & {\color{red} 17/39} & {\color{red} 36/79} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red} 18/41} & {\color{red} 24/53} & {\color{red} 37/84} & {\color{red} 35/78} & {21/43} & {40/87} & { 5/11} & {\color{red} 42/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 15/34} & {\color{red} 41/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/48} & {45/97} & {45/98} & {16/33} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/51} & {\color{red} 38/87} \\\hline
$34$ & { 4/ 9} && { 4/ 9} && {\color{red}  4/15} && { 8/17} && {19/44} && { 5/11} && { 3/ 7} && {\color{red} 23/59} && {29/61} && {41/97} && { 5/11} && {30/67} && {29/69} && {21/44} && {\color{red}  1/99} && {\color{red} 41/92} && { 5/11} && {35/79} && {\color{red} 45/98} && {\color{red}  1/99} && { 8/17} && { 5/11} && {40/89} && {\color{red} 22/49} && {\color{red}  1/99} && { 9/19} && {\color{red}  1/99} && { 5/11} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$35$ & { 4/ 9} & { 4/ 9} & {\color{red}  7/16} & { 4/ 9} && { 4/ 9} & {23/52} & { 4/ 9} & { 4/ 9} && { 4/ 9} & {\color{red} 25/57} & { 4/ 9} & {26/59} && {27/61} & { 4/ 9} & { 4/ 9} & { 4/ 9} && {\color{red} 29/66} & { 4/ 9} & {15/34} & { 4/ 9} && { 4/ 9} & { 4/ 9} & { 4/ 9} & { 4/ 9} && { 4/ 9} & {34/77} & { 4/ 9} & {35/79} && { 4/ 9} & { 4/ 9} & { 4/ 9} & {\color{red} 37/84} && {19/43} & { 4/ 9} & {39/88} & { 4/ 9} && { 4/ 9} & { 4/ 9} & {\color{red} 41/93} & { 4/ 9} && {\color{red}  7/16} & {43/97} & {\color{red} 43/98} & { 4/ 9} && {\color{red} 15/34} & {\color{red} 15/34} & {\color{red} 43/97} & {23/52} &\\\hline
$36$ & {37/83} && {39/85} && {\color{red}  1/99} && {39/89} && { 5/11} && {10/23} && {28/59} && {\color{red}  7/19} && { 4/ 9} && {21/46} && {\color{red} 19/46} && {11/23} && {30/71} && {33/73} && {\color{red} 16/37} && {\color{red}  1/99} && {11/23} && { 4/ 9} && {21/46} && {\color{red} 39/85} && {\color{red}  1/99} && {\color{red} 41/89} && {41/91} && {\color{red} 10/23} && { 9/19} && {\color{red}  1/99} && {\color{red}  4/ 9} && {41/90} && {\color{red}  1/99} && {10/21} &\\\hline
$37$ & {38/85} & {21/47} & {13/29} & {21/47} & {\color{red}  1/99} & {21/47} & { 6/13} & {21/47} & {13/28} & {23/47} & {20/47} & { 7/16} & {43/97} & { 3/ 7} & {\color{red}  1/99} & {21/50} & {29/61} & { 6/13} & {22/47} & {\color{red} 22/47} & {\color{red}  1/99} & {20/47} & {\color{red} 42/97} & { 4/ 9} & {\color{red}  5/12} & {\color{red}  1/99} & {18/37} & { 7/15} & {\color{red} 38/85} & {\color{red}  5/11} & {\color{red} 17/39} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red} 41/91} & {18/41} & {\color{red} 37/83} & {41/84} & {22/47} & {\color{red} 19/43} & {\color{red} 13/29} & {\color{red} 39/88} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  6/13} & {\color{red} 41/92} & {43/93} & {23/47} & {\color{red} 23/52} & {\color{red}  1/99} & {\color{red} 14/31} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 29/61} & {41/89} & {41/88} & {\color{red} 25/52} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 29/66} \\\hline
$38$ & {13/29} && {39/89} && {\color{red}  1/99} && { 5/11} && { 9/19} && {42/97} && { 7/16} && {\color{red}  1/99} && {11/24} && {32/67} && {31/69} && {\color{red}  1/99} && {31/73} && {\color{red} 39/89} && {23/48} && {36/79} && {\color{red}  1/99} && {\color{red} 36/83} && {\color{red} 38/85} && {\color{red} 11/24} && {11/24} && {\color{red}  1/99} && {14/31} && { 9/19} && {\color{red} 24/53} && {\color{red}  1/99} && {\color{red}  1/99} && {26/57} && {10/21} && {\color{red}  1/99} &\\\hline
$39$ & {40/89} & {22/49} & { 6/13} & {22/49} & {\color{red}  1/99} & {22/49} & {\color{red} 41/95} & {22/49} & {45/97} & {\color{red} 21/44} & { 4/ 9} & {11/25} & {29/62} & {\color{red} 22/51} & {\color{red}  1/99} & { 6/13} & { 3/ 7} & {23/53} & {41/86} & {\color{red} 23/49} & {\color{red} 43/99} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {\color{red} 31/74} & { 7/15} & {\color{red}  1/99} & {13/29} & {19/39} & {\color{red} 36/79} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red} 38/85} & {\color{red}  1/99} & {37/84} & {23/49} & {\color{red}  1/99} & {\color{red} 44/97} & {43/88} & {\color{red} 40/89} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 21/47} & {\color{red} 22/49} & {\color{red}  1/99} & {\color{red} 45/97} & {24/49} & {\color{red}  4/ 9} & {\color{red}  1/99} & {27/58} & {\color{red}  1/99} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/86} & {\color{red} 13/27} & {\color{red} 37/84} \\\hline
$40$ & {41/91} && {14/31} &&&& {44/97} && { 5/11} && {41/90} && {26/57} &&&& {\color{red} 44/97} && {\color{red}  5/11} && {\color{red} 41/90} && {\color{red} 14/31} &&&& {\color{red} 44/97} && {\color{red}  5/11} && {\color{red} 41/90} && {\color{red} 26/57} &&&& {\color{red} 44/97} && {\color{red} 39/85} && {\color{red} 41/90} && {\color{red} 26/57} &&&& {\color{red} 38/83} && {\color{red}  5/11} && {\color{red} 41/90} && {\color{red} 29/63} &&&& {\color{red} 38/83} && {\color{red} 39/85} &\\\hline
$41$ & {14/31} & {23/51} & {42/95} & {23/51} & {\color{red}  1/99} & {23/51} & {27/58} & {23/51} & {41/92} & {\color{red} 11/23} & {\color{red} 11/24} & {23/52} & {\color{red} 37/86} & {24/53} & {\color{red}  1/99} & {\color{red} 22/51} & { 8/17} & {\color{red}  1/99} & {\color{red} 27/62} & {\color{red} 33/71} & {\color{red} 17/36} & {\color{red} 36/83} & {\color{red}  1/99} & { 7/15} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {\color{red} 22/51} & {\color{red} 37/81} & {20/41} & {14/31} & {\color{red}  1/99} & { 8/17} & {19/43} & {\color{red}  1/99} & {\color{red} 39/88} & {\color{red} 39/89} & {\color{red}  1/99} & {\color{red} 41/91} & {45/92} & {\color{red} 26/57} & {\color{red}  1/99} & { 8/17} & {43/96} & {\color{red}  1/99} & {\color{red}  1/99} & {46/99} & {\color{red}  1/99} & {\color{red} 41/92} & {25/51} & {\color{red} 41/88} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 24/53} & {\color{red}  1/99} & {\color{red}  1/99} & {29/62} & {\color{red}  1/99} & {\color{red} 34/77} \\\hline
$42$ & {43/95} && { 5/11} && {\color{red}  1/99} && {26/59} && {\color{red} 31/72} && {10/21} && { 6/13} && {\color{red}  1/99} && {23/52} && {\color{red} 31/71} && {35/73} && { 6/13} && {\color{red}  1/99} && {\color{red}  1/99} && {37/81} && {25/52} && {\color{red} 36/85} && {\color{red}  1/99} && {\color{red}  1/99} && { 6/13} && {\color{red}  6/13} && {\color{red} 43/95} && {44/97} && {\color{red}  1/99} && {\color{red}  3/ 7} && {\color{red} 38/87} && {10/21} && {38/83} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$43$ & {44/97} & {24/53} & { 5/11} & {24/53} & {\color{red}  1/99} & {\color{red} 23/51} & {25/56} & {\color{red} 11/25} & {23/53} & {\color{red} 23/48} & {15/32} & {\color{red} 42/97} & {\color{red} 35/76} & {\color{red} 41/99} & {\color{red}  1/99} & {\color{red} 29/69} & {\color{red} 38/87} & {\color{red} 42/97} & {\color{red}  1/99} & {\color{red} 34/73} & {25/53} & { 7/15} & {\color{red}  9/19} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 39/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 38/83} & {\color{red} 24/53} & { 8/17} & {21/43} & {\color{red}  1/99} & {39/88} & {\color{red} 39/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 14/31} & {\color{red}  1/99} & {\color{red} 43/95} & {47/96} & {\color{red} 44/97} & {22/49} & {\color{red} 39/85} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 25/56} & {\color{red}  1/99} & {\color{red} 23/53} & {26/53} & {43/92} & {\color{red}  1/99} & {\color{red} 29/62} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$44$ & { 5/11} && {41/92} && {\color{red}  1/99} && {\color{red} 28/61} && { 4/ 9} && { 6/13} && {16/37} && {\color{red}  1/99} && {34/71} && { 4/ 9} && {\color{red} 44/97} && { 5/11} && {\color{red}  1/99} && {13/27} && {\color{red}  1/99} && {\color{red}  1/99} && {40/87} && {\color{red} 39/89} && {\color{red}  6/13} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 44/97} && { 5/11} && {\color{red} 41/92} && {\color{red}  1/99} && {\color{red}  7/17} && {\color{red} 28/71} && {39/85} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$45$ & {\color{red} 25/56} & { 5/11} & {13/29} & { 5/11} && {\color{red} 11/25} & {14/31} & {\color{red}  4/ 9} & {29/64} && { 5/11} & {\color{red} 30/67} & {\color{red} 44/97} & {31/69} && {32/71} & {\color{red} 39/86} & {33/73} & {\color{red} 33/74} && { 5/11} & { 5/11} & {\color{red} 35/78} & {\color{red} 39/86} && {\color{red} 44/97} & {37/82} & {\color{red} 37/83} & {19/42} && {39/86} & { 5/11} & { 5/11} & {\color{red} 40/89} && {41/91} & {\color{red} 41/92} & {14/31} & {\color{red} 44/97} && {\color{red} 43/96} & {44/97} & { 5/11} & { 5/11} && {\color{red} 41/92} & {23/51} & {\color{red} 25/56} & {33/73} && {24/53} & {\color{red} 35/78} & {44/97} & { 5/11} && {\color{red} 41/91} & { 5/11} & {\color{red} 23/55} & { 5/11} &\\\hline
$46$ & {\color{red} 11/25} && {\color{red} 37/82} && {\color{red}  1/99} && {\color{red} 33/76} && { 6/13} && {\color{red} 41/92} && {11/23} && {\color{red}  1/99} && {\color{red}  1/99} && {13/28} && {\color{red}  3/ 7} && {38/79} && {\color{red}  1/99} && {38/83} && {\color{red} 25/56} && {\color{red}  1/99} && {\color{red} 42/89} && {40/91} && {43/93} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 19/48} && {\color{red} 41/92} && {\color{red} 25/56} && {\color{red} 16/35} && {\color{red}  1/99} && {\color{red} 22/53} && {17/37} && {\color{red}  1/99} && {11/23} &\\\hline
$47$ & {\color{red} 19/43} & {26/57} & {35/78} & {26/57} & {\color{red}  1/99} & {\color{red} 44/97} & {17/37} & {\color{red}  3/ 7} & {31/66} & {\color{red} 25/52} & {\color{red}  7/16} & {\color{red} 10/23} & {\color{red}  3/ 7} & {\color{red} 38/91} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 13/28} & {\color{red} 34/75} & { 9/19} & {\color{red} 36/77} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 10/21} & { 8/17} & { 9/19} & {\color{red} 40/87} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {23/47} & { 9/19} & {\color{red} 43/96} & {\color{red} 44/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/49} & {\color{red} 23/51} & {\color{red} 25/56} & {26/53} & {\color{red} 30/67} & {\color{red}  1/99} & {\color{red} 35/78} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 11/27} & {\color{red}  1/99} & {38/81} & {28/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$48$ & {\color{red} 15/34} && {\color{red} 27/61} && {\color{red}  1/99} && { 6/13} && {\color{red} 31/67} && {17/39} && {13/29} && {\color{red}  1/99} && {\color{red} 46/99} && {37/77} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 41/92} && {14/29} && {41/89} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 45/97} && {46/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  7/17} && {\color{red} 35/78} && {\color{red} 37/84} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 31/66} && {\color{red}  1/99} &\\\hline
$49$ & {\color{red}  4/ 9} & {27/59} & {\color{red} 14/31} & {27/59} & {\color{red}  1/99} & {\color{red} 27/61} & {\color{red} 29/66} & {\color{red}  3/ 7} & { 6/13} & {\color{red} 11/23} & {\color{red} 37/84} & {\color{red} 30/71} & {17/36} & {\color{red} 32/73} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red} 31/73} & {\color{red}  1/99} & {\color{red} 41/88} & {\color{red} 37/79} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  9/19} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 21/44} & {\color{red} 41/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 42/95} & {\color{red}  1/99} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {\color{red}  1/99} & {24/49} & {\color{red}  5/11} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 20/51} & {\color{red}  1/99} & {\color{red} 11/26} & {27/55} & {\color{red} 40/89} & {\color{red}  1/99} & {\color{red} 17/37} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 46/99} & {29/59} & {\color{red} 21/58} \\\hline
$50$ & {\color{red} 41/92} && {\color{red} 25/56} &&&& {\color{red} 35/78} && {\color{red}  4/ 9} && {\color{red} 35/81} && {\color{red} 25/56} &&&& {\color{red} 35/78} && {\color{red} 40/89} && {\color{red} 41/92} && {\color{red} 41/93} &&&& {\color{red} 43/97} && {\color{red} 40/89} && {\color{red} 40/91} && {\color{red} 41/93} &&&& {\color{red} 43/97} && {\color{red}  4/ 9} && {\color{red} 41/92} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 41/91} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & {\color{red}  4/ 9} & {28/61} & {\color{red}  7/16} & {28/61} & {\color{red}  1/99} & {\color{red}  4/ 9} & { 8/17} & {\color{red} 28/65} & {\color{red} 27/62} & {\color{red} 34/71} & {19/41} & {\color{red} 13/31} & {\color{red} 34/77} & {\color{red} 10/23} & {\color{red}  1/99} & {\color{red} 34/77} & {37/78} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 38/81} & {\color{red} 43/92} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  7/15} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  6/13} & {\color{red} 11/23} & {\color{red}  1/99} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 16/35} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/90} & {25/51} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  7/15} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 11/27} & {28/57} & {\color{red} 37/82} & {\color{red}  1/99} & {\color{red} 43/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 12/29} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$52$ & {\color{red} 21/47} && { 6/13} && {\color{red}  1/99} && {31/69} && {18/41} && {\color{red} 34/73} && { 7/15} && {\color{red}  1/99} && {14/31} && {\color{red}  1/99} && {40/83} && {\color{red}  5/11} && {\color{red}  1/99} && {\color{red}  1/99} && { 6/13} && {15/31} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {27/58} && {\color{red} 41/88} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  7/18} && {\color{red} 23/55} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & {\color{red} 38/85} & {29/63} & {\color{red} 17/38} & {29/63} & {\color{red}  1/99} & {\color{red} 29/65} & {\color{red} 38/87} & {\color{red} 31/71} & { 4/ 9} & {\color{red} 35/73} & {35/74} & {\color{red}  7/16} & {20/43} & {\color{red}  3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {\color{red} 39/83} & {10/21} & {\color{red} 39/85} & {\color{red} 15/32} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 43/93} & {10/21} & { 9/19} & {\color{red} 23/48} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 26/57} & {\color{red} 23/52} & {10/21} & {26/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red}  3/ 7} & {29/59} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$54$ & {\color{red} 29/65} && {\color{red} 37/84} && {\color{red}  1/99} && {\color{red} 45/98} && {33/73} && { 7/15} && {\color{red}  1/99} && {\color{red}  1/99} && {13/27} && {\color{red} 18/41} && {15/32} && {\color{red}  1/99} && {\color{red}  1/99} && {44/91} && {\color{red}  1/99} && {\color{red}  7/16} && {45/97} && {\color{red}  1/99} && {\color{red} 29/61} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 21/52} && {\color{red}  1/99} && {\color{red} 17/37} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 23/57} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & { 5/11} & { 6/13} & {31/68} & { 6/13} && {\color{red} 30/67} & {11/24} & {\color{red} 10/23} & {17/37} && {35/76} & { 5/11} & { 6/13} & {36/79} && {37/81} & {\color{red} 41/89} & {38/83} & {\color{red} 41/89} && {\color{red} 13/29} & {40/87} & { 6/13} & {41/89} && { 6/13} & {21/46} & {\color{red} 14/31} & {43/94} && {11/24} & {\color{red} 22/49} & {45/98} & {\color{red}  5/11} && {\color{red} 41/90} & {41/89} & {\color{red} 26/57} & { 6/13} && {\color{red} 29/63} & {38/83} & {\color{red} 40/89} & {39/85} && {17/37} & {\color{red} 41/90} & {29/63} & {\color{red} 26/57} && {\color{red}  1/99} & {\color{red} 22/57} & {\color{red} 26/57} & {\color{red}  7/23} && {\color{red} 25/77} & {28/61} & {\color{red} 41/90} & {\color{red} 28/61} &\\\hline
$56$ & {\color{red} 30/67} && {\color{red} 35/79} && {\color{red}  1/99} && {\color{red} 19/43} && { 7/15} && { 5/11} && {\color{red} 37/79} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 22/47} && { 5/11} && {43/89} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 33/73} && {\color{red}  1/99} && {16/33} && {\color{red}  1/99} && {41/88} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 29/62} && {\color{red}  1/99} && {\color{red} 29/79} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 23/58} && {\color{red}  1/99} && {\color{red} 23/72} && {\color{red}  1/99} &\\\hline
$57$ & {\color{red} 34/77} & {31/67} & {\color{red} 42/97} & {31/67} & {\color{red}  1/99} & {\color{red} 31/69} & {\color{red} 19/42} & {\color{red} 31/71} & { 9/19} & {\color{red} 37/77} & {\color{red} 41/92} & {\color{red} 35/79} & {\color{red}  1/99} & {\color{red} 19/46} & {\color{red}  1/99} & {\color{red}  1/99} & {22/47} & {\color{red} 37/85} & {41/86} & {\color{red} 41/87} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/87} & { 9/19} & {\color{red} 31/66} & {\color{red} 45/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 25/52} & {10/21} & {\color{red} 41/89} & {\color{red} 38/83} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {28/57} & {\color{red} 31/66} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {31/63} & {\color{red} 43/96} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$58$ & {\color{red} 39/88} && {32/71} && {\color{red}  1/99} && { 7/15} && {\color{red}  5/11} && {\color{red}  1/99} && {\color{red} 44/97} && {\color{red}  1/99} && { 8/17} && {14/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && { 8/17} && {47/97} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 41/86} && {29/62} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 33/91} && {\color{red} 12/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 27/83} &\\\hline
$59$ & {\color{red}  3/ 7} & {32/69} & {\color{red} 43/95} & {32/69} & {\color{red}  1/99} & {\color{red} 32/71} & {17/38} & {\color{red} 32/73} & {\color{red}  5/11} & {\color{red} 38/79} & {\color{red}  1/99} & {\color{red} 35/81} & {39/82} & {\color{red} 37/83} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {23/49} & {\color{red} 42/89} & {\color{red}  1/99} & {\color{red}  1/99} & {11/23} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 44/95} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/49} & {\color{red} 46/99} & {\color{red}  1/99} & {\color{red}  1/99} & {11/23} & {\color{red}  1/99} & {\color{red}  1/99} & {10/21} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 13/27} & {\color{red} 39/85} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {11/23} & {\color{red}  1/99} & {\color{red}  1/99} & {29/59} & {\color{red} 44/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 24/61} & {\color{red}  1/99} & {\color{red}  1/99} & {32/65} & {\color{red}  1/99} \\\hline
$60$ & {\color{red}  3/ 7} && {\color{red} 40/93} &&&& {\color{red} 42/97} && {\color{red} 43/99} && {\color{red} 27/62} && {\color{red} 38/87} &&&& {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &&&& {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g4-a01b02.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 5} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 2/ 9} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 3/13} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 4/17} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 5/21} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 6/25} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 7/29} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 8/33} & { 1/ 4} & { 1/ 4} & { 1/ 4} & { 9/37} & { 1/ 4} & { 1/ 4} & { 1/ 4} & {10/41} & { 1/ 4} & { 1/ 4} & { 1/ 4} & {11/45} & { 1/ 4} & { 1/ 4} & { 1/ 4} & {12/49} & { 1/ 4} & { 1/ 4} & { 1/ 4} & {13/53} & { 1/ 4} & { 1/ 4} & { 1/ 4} & {14/57} & { 1/ 4} & { 1/ 4} & { 1/ 4} & {15/61} & { 1/ 4} & { 1/ 4} & { 1/ 4} \\\hline
$2$ & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 3/11} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} \\\hline
$3$ & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} \\\hline
$4$ & { 1/ 4} & { 2/ 7} & { 2/ 7} & { 3/11} & {\color{red}  1/ 4} & { 2/ 7} & { 2/ 7} & { 4/15} & { 2/ 7} & { 2/ 7} & { 5/18} & {\color{red}  5/19} & { 2/ 7} & { 2/ 7} & { 3/11} & { 2/ 7} & { 2/ 7} & { 7/25} & {\color{red}  7/26} & { 2/ 7} & { 2/ 7} & { 8/29} & { 2/ 7} & { 2/ 7} & { 9/32} & {\color{red}  3/11} & { 2/ 7} & { 2/ 7} & { 5/18} & { 2/ 7} & { 2/ 7} & {11/39} & {\color{red} 11/40} & { 2/ 7} & { 2/ 7} & {12/43} & { 2/ 7} & { 2/ 7} & {13/46} & {\color{red} 13/47} & { 2/ 7} & { 2/ 7} & { 7/25} & { 2/ 7} & { 2/ 7} & {15/53} & {\color{red}  5/18} & { 2/ 7} & { 2/ 7} & {16/57} & { 2/ 7} & { 2/ 7} & {17/60} & {\color{red} 17/61} & { 2/ 7} & { 2/ 7} & { 9/32} & { 2/ 7} & { 2/ 7} & {19/67} \\\hline
$5$ & { 1/ 3} & { 3/11} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} \\\hline
$6$ & { 3/10} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} \\\hline
$7$ & { 3/11} & { 3/10} & { 3/10} & { 2/ 7} & {\color{red}  7/26} & { 3/10} & { 5/17} & {\color{red}  5/18} & { 3/10} & { 3/10} & { 2/ 7} & { 3/10} & { 3/10} & { 7/24} & {\color{red}  7/25} & { 3/10} & { 8/27} & {\color{red}  2/ 7} & { 3/10} & { 3/10} & { 9/31} & { 3/10} & { 3/10} & { 5/17} & {\color{red}  2/ 7} & { 3/10} & {11/37} & {\color{red} 11/38} & { 3/10} & { 3/10} & {12/41} & { 3/10} & { 3/10} & {13/44} & {\color{red} 13/45} & { 3/10} & {14/47} & {\color{red}  7/24} & { 3/10} & { 3/10} & { 5/17} & { 3/10} & { 3/10} & { 8/27} & {\color{red} 16/55} & { 3/10} & {17/57} & {\color{red} 17/58} & { 3/10} & { 3/10} & {18/61} & { 3/10} & { 3/10} & {19/64} & {\color{red} 19/65} & { 3/10} & {20/67} & {\color{red}  5/17} & { 3/10} & { 3/10} \\\hline
$8$ & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} \\\hline
$9$ & { 4/13} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} \\\hline
$10$ & { 2/ 7} & { 4/13} & { 4/13} & { 5/17} & { 9/32} & { 4/13} & { 3/10} & {\color{red}  2/ 7} & { 4/13} & { 7/23} & {\color{red}  7/24} & { 4/13} & { 4/13} & { 8/27} & { 4/13} & { 4/13} & { 3/10} & {\color{red}  9/31} & { 4/13} & {10/33} & {\color{red}  5/17} & { 4/13} & {11/36} & {\color{red} 11/37} & { 4/13} & { 4/13} & { 3/10} & { 4/13} & { 4/13} & {13/43} & {\color{red} 13/44} & { 4/13} & { 7/23} & {\color{red} 14/47} & { 4/13} & {15/49} & {\color{red}  3/10} & { 4/13} & { 4/13} & {16/53} & { 4/13} & { 4/13} & {17/56} & {\color{red} 17/57} & { 4/13} & {18/59} & {\color{red}  3/10} & { 4/13} & {19/62} & {\color{red} 19/63} & { 4/13} & { 4/13} & {10/33} & { 4/13} & { 4/13} & { 7/23} & {\color{red}  3/10} & { 4/13} & {11/36} & {\color{red} 22/73} \\\hline
$11$ & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} \\\hline
$12$ & { 5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} \\\hline
$13$ & { 5/17} & { 5/16} & { 5/16} & { 3/10} & {11/38} & { 5/16} & { 7/23} & {12/41} & { 5/16} & { 4/13} & {\color{red}  8/27} & { 5/16} & { 9/29} & {\color{red}  3/10} & { 5/16} & { 5/16} & {10/33} & { 5/16} & { 5/16} & {11/36} & {\color{red} 11/37} & { 5/16} & { 4/13} & {\color{red}  3/10} & { 5/16} & {13/42} & {\color{red} 13/43} & { 5/16} & {14/45} & {\color{red}  7/23} & { 5/16} & { 5/16} & {15/49} & { 5/16} & { 5/16} & { 4/13} & {\color{red} 16/53} & { 5/16} & {17/55} & {\color{red} 17/56} & { 5/16} & { 9/29} & {\color{red} 18/59} & { 5/16} & {19/61} & {\color{red} 19/62} & { 5/16} & { 5/16} & { 4/13} & { 5/16} & { 5/16} & {21/68} & {\color{red}  7/23} & { 5/16} & {22/71} & {\color{red} 11/36} & { 5/16} & {23/74} & {\color{red} 23/75} & { 5/16} \\\hline
$14$ & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} \\\hline
$15$ & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} \\\hline
$16$ & { 3/10} & { 6/19} & { 6/19} & { 7/23} & {13/44} & { 6/19} & { 4/13} & {14/47} & { 6/19} & { 9/29} & { 3/10} & { 6/19} & { 5/16} & {\color{red} 10/33} & { 6/19} & {11/35} & {\color{red} 11/36} & { 6/19} & { 6/19} & { 4/13} & { 6/19} & { 6/19} & {13/42} & {\color{red} 13/43} & { 6/19} & {14/45} & {\color{red}  7/23} & { 6/19} & { 5/16} & {\color{red} 15/49} & { 6/19} & {16/51} & {\color{red}  4/13} & { 6/19} & {17/54} & {\color{red} 17/55} & { 6/19} & { 6/19} & { 9/29} & { 6/19} & { 6/19} & {19/61} & {\color{red} 19/62} & { 6/19} & { 5/16} & {\color{red}  4/13} & { 6/19} & {21/67} & {\color{red} 21/68} & { 6/19} & {11/35} & {\color{red} 22/71} & { 6/19} & {23/73} & {\color{red} 23/74} & { 6/19} & { 6/19} & {24/77} & { 6/19} & { 6/19} \\\hline
$17$ & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} \\\hline
$18$ & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} \\\hline
$19$ & { 7/23} & { 7/22} & { 7/22} & { 4/13} & { 3/10} & { 7/22} & { 9/29} & {16/53} & { 7/22} & { 5/16} & {17/56} & { 7/22} & {11/35} & {11/36} & { 7/22} & { 6/19} & {\color{red}  4/13} & { 7/22} & {13/41} & {\color{red} 13/42} & { 7/22} & { 7/22} & {14/45} & { 7/22} & { 7/22} & { 5/16} & {\color{red} 15/49} & { 7/22} & {16/51} & {\color{red}  4/13} & { 7/22} & {17/54} & {\color{red} 17/55} & { 7/22} & { 6/19} & {\color{red}  9/29} & { 7/22} & {19/60} & {\color{red} 19/61} & { 7/22} & {20/63} & {\color{red}  5/16} & { 7/22} & { 7/22} & {21/67} & { 7/22} & { 7/22} & {11/35} & {\color{red} 22/71} & { 7/22} & {23/73} & {\color{red} 23/74} & { 7/22} & { 6/19} & {\color{red} 24/77} & { 7/22} & {25/79} & {\color{red}  5/16} & { 7/22} & {13/41} \\\hline
$20$ & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} \\\hline
$21$ & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} \\\hline
$22$ & { 4/13} & { 8/25} & { 8/25} & { 9/29} & {17/56} & { 8/25} & { 5/16} & {18/59} & { 8/25} & {11/35} & {19/62} & { 8/25} & { 6/19} & { 4/13} & { 8/25} & {13/41} & {13/42} & { 8/25} & { 7/22} & {\color{red} 14/45} & { 8/25} & {15/47} & {\color{red}  5/16} & { 8/25} & { 8/25} & {16/51} & { 8/25} & { 8/25} & {17/54} & {\color{red} 17/55} & { 8/25} & { 6/19} & {\color{red}  9/29} & { 8/25} & {19/60} & {\color{red} 19/61} & { 8/25} & {20/63} & {\color{red}  5/16} & { 8/25} & { 7/22} & {\color{red} 21/67} & { 8/25} & {22/69} & {\color{red} 11/35} & { 8/25} & {23/72} & {\color{red} 23/73} & { 8/25} & { 8/25} & { 6/19} & { 8/25} & { 8/25} & {25/79} & {\color{red}  5/16} & { 8/25} & {13/41} & {\color{red} 26/83} & { 8/25} & {27/85} \\\hline
$23$ & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} \\\hline
$24$ & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} \\\hline
$25$ & { 9/29} & { 9/28} & { 9/28} & { 5/16} & {19/62} & { 9/28} & {11/35} & { 4/13} & { 9/28} & { 6/19} & {21/68} & { 9/28} & {13/41} & {22/71} & { 9/28} & { 7/22} & {14/45} & { 9/28} & {15/47} & { 5/16} & { 9/28} & { 8/25} & {\color{red} 16/51} & { 9/28} & {17/53} & {\color{red} 17/54} & { 9/28} & { 9/28} & { 6/19} & { 9/28} & { 9/28} & {19/60} & {\color{red} 19/61} & { 9/28} & {20/63} & {\color{red}  5/16} & { 9/28} & { 7/22} & {\color{red} 21/67} & { 9/28} & {22/69} & {\color{red} 11/35} & { 9/28} & {23/72} & {\color{red} 23/73} & { 9/28} & { 8/25} & {\color{red}  6/19} & { 9/28} & {25/78} & {\color{red} 25/79} & { 9/28} & {26/81} & {\color{red} 13/41} & { 9/28} & { 9/28} & {27/85} & { 9/28} & { 9/28} & { 7/22} \\\hline
$26$ & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} \\\hline
$27$ & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} \\\hline
$28$ & { 5/16} & {10/31} & {10/31} & {11/35} & {21/68} & {10/31} & { 6/19} & {22/71} & {10/31} & {13/41} & {23/74} & {10/31} & { 7/22} & {24/77} & {10/31} & {15/47} & { 5/16} & {10/31} & { 8/25} & {16/51} & {10/31} & {17/53} & {17/54} & {10/31} & { 9/28} & {\color{red}  6/19} & {10/31} & {19/59} & {\color{red} 19/60} & {10/31} & {10/31} & {20/63} & {10/31} & {10/31} & { 7/22} & {\color{red} 21/67} & {10/31} & {22/69} & {\color{red} 11/35} & {10/31} & {23/72} & {\color{red} 23/73} & {10/31} & { 8/25} & {\color{red}  6/19} & {10/31} & {25/78} & {\color{red} 25/79} & {10/31} & {26/81} & {\color{red} 13/41} & {10/31} & { 9/28} & {\color{red} 27/85} & {10/31} & {28/87} & {\color{red}  7/22} & {10/31} & {29/90} & {\color{red} 29/91} \\\hline
$29$ & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} \\\hline
$30$ & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} \\\hline
$31$ & {11/35} & {11/34} & {11/34} & { 6/19} & {23/74} & {11/34} & {13/41} & {24/77} & {11/34} & { 7/22} & { 5/16} & {11/34} & {15/47} & {26/83} & {11/34} & { 8/25} & {27/86} & {11/34} & {17/53} & {17/54} & {11/34} & { 9/28} & { 6/19} & {11/34} & {19/59} & {19/60} & {11/34} & {10/31} & {\color{red} 20/63} & {11/34} & {21/65} & {\color{red}  7/22} & {11/34} & {11/34} & {22/69} & {11/34} & {11/34} & {23/72} & {\color{red} 23/73} & {11/34} & { 8/25} & {\color{red}  6/19} & {11/34} & {25/78} & {\color{red} 25/79} & {11/34} & {26/81} & {\color{red} 13/41} & {11/34} & { 9/28} & {\color{red} 27/85} & {11/34} & {28/87} & {\color{red}  7/22} & {11/34} & {29/90} & {\color{red} 29/91} & {11/34} & {10/31} & {\color{red} 15/47} \\\hline
$32$ & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} \\\hline
$33$ & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} \\\hline
$34$ & { 6/19} & {12/37} & {12/37} & {13/41} & { 5/16} & {12/37} & { 7/22} & {26/83} & {12/37} & {15/47} & {27/86} & {12/37} & { 8/25} & {28/89} & {12/37} & {17/53} & {29/92} & {12/37} & { 9/28} & { 6/19} & {12/37} & {19/59} & {19/60} & {12/37} & {10/31} & {20/63} & {12/37} & {21/65} & { 7/22} & {12/37} & {11/34} & {\color{red} 22/69} & {12/37} & {23/71} & {\color{red} 23/72} & {12/37} & {12/37} & { 8/25} & {12/37} & {12/37} & {25/78} & {\color{red} 25/79} & {12/37} & {26/81} & {\color{red} 13/41} & {12/37} & { 9/28} & {\color{red} 27/85} & {12/37} & {28/87} & {\color{red}  7/22} & {12/37} & {29/90} & {\color{red} 29/91} & {12/37} & {10/31} & {\color{red} 15/47} & {12/37} & {31/96} & {\color{red} 31/97} \\\hline
$35$ & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} \\\hline
$36$ & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$37$ & {13/41} & {13/40} & {13/40} & { 7/22} & {27/86} & {13/40} & {15/47} & {28/89} & {13/40} & { 8/25} & {29/92} & {13/40} & {17/53} & { 6/19} & {13/40} & { 9/28} & {31/98} & {13/40} & {19/59} & {19/60} & {13/40} & {10/31} & {20/63} & {13/40} & {21/65} & {\color{red}  7/22} & {13/40} & {11/34} & {22/69} & {13/40} & {23/71} & {23/72} & {13/40} & {12/37} & {\color{red}  8/25} & {13/40} & {25/77} & {\color{red} 25/78} & {13/40} & {13/40} & {26/81} & {\color{red} 13/41} & {13/40} & { 9/28} & {\color{red} 27/85} & {13/40} & {28/87} & {\color{red}  7/22} & {13/40} & {29/90} & {\color{red} 29/91} & {13/40} & {10/31} & {\color{red} 15/47} & {13/40} & {31/96} & {\color{red} 31/97} & {13/40} & {32/99} & {\color{red}  8/25} \\\hline
$38$ & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} \\\hline
$39$ & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$40$ & { 7/22} & {14/43} & {14/43} & {15/47} & {29/92} & {14/43} & { 8/25} & { 6/19} & {14/43} & {17/53} & {31/98} & {14/43} & { 9/28} & {19/60} & {14/43} & {19/59} & {20/63} & {14/43} & {10/31} & {27/85} & {14/43} & {21/65} & { 7/22} & {14/43} & {11/34} & {22/69} & {14/43} & {23/71} & {\color{red} 23/72} & {14/43} & {12/37} & { 8/25} & {14/43} & {25/77} & {25/78} & {14/43} & {13/40} & {\color{red} 26/81} & {14/43} & {27/83} & {\color{red}  9/28} & {14/43} & {14/43} & {28/87} & {\color{red}  7/22} & {14/43} & {29/90} & {\color{red} 29/91} & {14/43} & {10/31} & {\color{red} 15/47} & {14/43} & {31/96} & {\color{red} 31/97} & {14/43} & {32/99} & {\color{red}  8/25} & {14/43} & {11/34} & {\color{red} 25/78} \\\hline
$41$ & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} \\\hline
$42$ & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$43$ & {15/47} & {15/46} & {15/46} & { 8/25} & {31/98} & {15/46} & {17/53} & {19/60} & {15/46} & { 9/28} & {20/63} & {15/46} & {19/59} & {27/85} & {15/46} & {10/31} & { 7/22} & {15/46} & {21/65} & {29/91} & {15/46} & {11/34} & {22/69} & {15/46} & {23/71} & {23/72} & {15/46} & {12/37} & {\color{red}  8/25} & {15/46} & {25/77} & {\color{red} 25/78} & {15/46} & {13/40} & {26/81} & {15/46} & {27/83} & { 9/28} & {15/46} & {14/43} & {\color{red} 28/87} & {15/46} & {29/89} & {\color{red} 29/90} & {15/46} & {15/46} & {10/31} & {\color{red} 15/47} & {15/46} & {31/96} & {\color{red} 31/97} & {15/46} & {32/99} & {\color{red}  8/25} & {15/46} & {11/34} & {\color{red} 25/78} & {15/46} & {23/71} & {\color{red} 17/53} \\\hline
$44$ & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} \\\hline
$45$ & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$46$ & { 8/25} & {16/49} & {16/49} & {17/53} & {20/63} & {16/49} & { 9/28} & {27/85} & {16/49} & {19/59} & { 7/22} & {16/49} & {10/31} & {29/91} & {16/49} & {21/65} & {22/69} & {16/49} & {11/34} & {23/72} & {16/49} & {23/71} & {31/97} & {16/49} & {12/37} & { 8/25} & {16/49} & {25/77} & {25/78} & {16/49} & {13/40} & {\color{red} 26/81} & {16/49} & {27/83} & {\color{red}  9/28} & {16/49} & {14/43} & {\color{red} 28/87} & {16/49} & {29/89} & {\color{red} 29/90} & {16/49} & {15/46} & {\color{red} 10/31} & {16/49} & {31/95} & {\color{red} 31/96} & {16/49} & {16/49} & {32/99} & {\color{red}  8/25} & {\color{red} 31/95} & {11/34} & {\color{red} 25/78} & {16/49} & {23/71} & {\color{red} 17/53} & {16/49} & {23/71} & {\color{red} 26/81} \\\hline
$47$ & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} \\\hline
$48$ & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$49$ & {17/53} & {17/52} & {17/52} & { 9/28} & { 7/22} & {17/52} & {19/59} & {29/91} & {17/52} & {10/31} & {22/69} & {17/52} & {21/65} & {23/72} & {17/52} & {11/34} & {31/97} & {17/52} & {23/71} & { 8/25} & {17/52} & {12/37} & {25/78} & {17/52} & {25/77} & {25/78} & {17/52} & {13/40} & {26/81} & {17/52} & {27/83} & {\color{red}  9/28} & {17/52} & {14/43} & {\color{red} 28/87} & {17/52} & {29/89} & {\color{red} 29/90} & {17/52} & {15/46} & {\color{red} 10/31} & {17/52} & {31/95} & {\color{red} 31/96} & {17/52} & {16/49} & {\color{red} 32/99} & {17/52} & {17/52} & {\color{red} 11/34} & {17/52} & {17/52} & {23/71} & {\color{red} 17/53} & {\color{red} 17/52} & {23/71} & {\color{red} 26/81} & {17/52} & {12/37} & {\color{red}  9/28} \\\hline
$50$ & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} \\\hline
$51$ & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$52$ & { 9/28} & {\color{red} 27/85} & {18/55} & {19/59} & {22/69} & {18/55} & {10/31} & {23/72} & {18/55} & {21/65} & {31/97} & {18/55} & {11/34} & { 8/25} & {18/55} & {23/71} & {25/78} & {18/55} & {12/37} & {25/78} & {18/55} & {25/77} & {26/81} & {18/55} & {13/40} & {\color{red} 26/81} & {\color{red} 18/55} & {27/83} & { 9/28} & {18/55} & {14/43} & {\color{red} 28/87} & {18/55} & {29/89} & {\color{red} 29/90} & {18/55} & {15/46} & {\color{red} 10/31} & {18/55} & {31/95} & {\color{red} 31/96} & {18/55} & {16/49} & {\color{red} 32/99} & {18/55} & {17/52} & {\color{red} 11/34} & {18/55} & {17/52} & {\color{red} 23/71} & {18/55} & {18/55} & {\color{red} 23/71} & {18/55} & {18/55} & {12/37} & {\color{red}  9/28} & {\color{red} 18/55} & {25/77} & {\color{red} 28/87} \\\hline
$53$ & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} \\\hline
$54$ & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$55$ & {19/59} & {\color{red} 29/91} & {19/58} & {10/31} & {31/97} & {19/58} & {21/65} & { 8/25} & {19/58} & {11/34} & {25/78} & {19/58} & {23/71} & {25/78} & {19/58} & {12/37} & {26/81} & {19/58} & {25/77} & {26/81} & {19/58} & {13/40} & { 9/28} & {19/58} & {27/83} & {\color{red}  9/28} & {19/58} & {14/43} & {28/87} & {19/58} & {29/89} & {29/90} & {19/58} & {15/46} & {\color{red} 10/31} & {19/58} & {31/95} & {\color{red} 31/96} & {19/58} & {16/49} & {\color{red} 32/99} & {19/58} & {17/52} & {\color{red} 11/34} & {19/58} & {17/52} & {\color{red} 23/71} & {19/58} & {18/55} & {\color{red} 23/71} & {19/58} & {18/55} & {\color{red} 12/37} & {19/58} & {19/58} & {\color{red} 25/77} & {19/58} & {19/58} & {25/77} & {\color{red} 19/59} \\\hline
$56$ & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} \\\hline
$57$ & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
$58$ & {10/31} & {\color{red}  5/16} & {20/61} & {21/65} & {\color{red} 31/97} & {20/61} & {11/34} & {25/78} & {20/61} & {23/71} & {26/81} & {20/61} & {12/37} & {\color{red} 26/81} & {20/61} & {25/77} & { 9/28} & {20/61} & {13/40} & {\color{red} 13/41} & {20/61} & {27/83} & {28/87} & {20/61} & {14/43} & {\color{red}  7/22} & {20/61} & {29/89} & {\color{red} 29/90} & {\color{red} 20/61} & {15/46} & {\color{red} 10/31} & {20/61} & {31/95} & {\color{red} 31/96} & {20/61} & {16/49} & {\color{red} 32/99} & {20/61} & {17/52} & {\color{red} 11/34} & {20/61} & {17/52} & {\color{red} 23/71} & {20/61} & {18/55} & {\color{red} 23/71} & {20/61} & {18/55} & {\color{red} 12/37} & {20/61} & {19/58} & {\color{red} 25/77} & {20/61} & {19/58} & {\color{red} 25/77} & {20/61} & {20/61} & {\color{red} 13/40} & {20/61} \\\hline
$59$ & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} \\\hline
$60$ & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & {23/70} & { 1/ 3} & { 1/ 3} & {24/73} & { 1/ 3} & { 1/ 3} & {25/76} & { 1/ 3} & { 1/ 3} & {26/79} & { 1/ 3} & { 1/ 3} & {27/82} & { 1/ 3} & { 1/ 3} & {28/85} & { 1/ 3} & { 1/ 3} & {29/88} & { 1/ 3} & { 1/ 3} & {30/91} & { 1/ 3} & { 1/ 3} & {31/94} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} & {32/97} & { 1/ 3} & { 1/ 3} \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 2, 2+k, 2+k+i\}$.
\end{center}


==> tables/table-g4-a01b03.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 4} & { 2/ 7} & { 1/ 4} & { 2/ 7} & {\color{red}  1/ 4} & { 2/ 7} & { 2/ 7} & { 4/15} & { 2/ 7} & { 4/15} & { 2/ 7} & {\color{red}  4/15} & { 2/ 7} & { 2/ 7} & { 3/11} & { 2/ 7} & { 3/11} & { 2/ 7} & {\color{red}  3/11} & { 2/ 7} & { 2/ 7} & { 8/29} & { 2/ 7} & { 8/29} & { 2/ 7} & {\color{red}  8/29} & { 2/ 7} & { 2/ 7} & { 5/18} & { 2/ 7} & { 5/18} & { 2/ 7} & {\color{red}  5/18} & { 2/ 7} & { 2/ 7} & {12/43} & { 2/ 7} & {12/43} & { 2/ 7} & {\color{red} 12/43} & { 2/ 7} & { 2/ 7} & { 7/25} & { 2/ 7} & { 7/25} & { 2/ 7} & {\color{red}  7/25} & { 2/ 7} & { 2/ 7} & {16/57} & { 2/ 7} & {16/57} & { 2/ 7} & {\color{red} 16/57} & { 2/ 7} & { 2/ 7} & { 9/32} & { 2/ 7} & { 9/32} & { 2/ 7} \\\hline
$2$ & { 3/11} && { 4/13} && { 1/ 3} && { 6/17} && { 7/19} && { 8/21} && { 9/23} && { 2/ 5} && {11/27} && {12/29} && {13/31} && {14/33} && { 3/ 7} && {16/37} && {17/39} && {18/41} && {19/43} && { 4/ 9} && {21/47} && {22/49} && {23/51} && {24/53} && { 5/11} && {26/57} && {27/59} && {28/61} && {29/63} && { 6/13} && {31/67} && {32/69} &\\\hline
$3$ & { 1/ 4} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 5/16} & { 3/10} & { 1/ 3} & {\color{red}  3/11} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 7/23} & { 1/ 3} & { 8/25} & { 9/29} & { 1/ 3} & {\color{red}  9/31} & { 1/ 3} & { 3/10} & { 1/ 3} & { 5/16} & { 1/ 3} & {11/34} & { 6/19} & { 1/ 3} & {\color{red}  3/10} & { 1/ 3} & { 4/13} & { 1/ 3} & {13/41} & { 1/ 3} & {14/43} & {15/47} & { 1/ 3} & {\color{red} 15/49} & { 1/ 3} & { 5/16} & { 1/ 3} & { 8/25} & { 1/ 3} & {17/52} & { 9/28} & { 1/ 3} & {\color{red}  9/29} & { 1/ 3} & { 6/19} & { 1/ 3} & {19/59} & { 1/ 3} & {20/61} & {21/65} & { 1/ 3} & {\color{red} 21/67} & { 1/ 3} & { 7/22} & { 1/ 3} & {11/34} & { 1/ 3} \\\hline
$4$ & { 4/15} && { 5/17} && { 6/19} && { 1/ 3} && { 8/23} && { 9/25} && {10/27} && {11/29} && {12/31} && {13/33} && { 2/ 5} && {15/37} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} &\\\hline
$5$ & {\color{red}  1/ 4} & { 4/11} & { 2/ 7} & { 4/11} & { 5/16} & { 4/11} & { 1/ 3} & { 1/ 3} & { 7/20} & {\color{red}  4/13} & { 4/11} & {\color{red}  7/23} & { 4/11} & { 8/25} & { 4/11} & { 1/ 3} & { 4/11} & {10/29} & {12/35} & {11/31} & {\color{red} 12/37} & { 4/11} & {\color{red} 11/34} & { 4/11} & { 1/ 3} & { 4/11} & {13/38} & { 4/11} & { 7/20} & { 8/23} & { 5/14} & {\color{red}  1/ 3} & { 4/11} & {\color{red}  1/ 3} & { 4/11} & {16/47} & { 4/11} & {17/49} & { 4/11} & { 6/17} & {20/57} & {19/53} & {\color{red} 20/59} & { 4/11} & {\color{red} 19/56} & { 4/11} & {10/29} & { 4/11} & { 7/20} & { 4/11} & {11/31} & { 6/17} & {23/64} & {\color{red} 12/35} & { 4/11} & {\color{red} 23/67} & { 4/11} & { 8/23} & { 4/11} & {25/71} \\\hline
$6$ & {\color{red}  5/19} && { 2/ 7} && {\color{red}  7/23} && { 8/25} && { 1/ 3} && {10/29} && {11/31} && { 4/11} && {13/35} && {14/37} && { 5/13} && {16/41} && {17/43} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && {22/53} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} &\\\hline
$7$ & { 2/ 7} & { 5/13} & { 5/16} & { 5/13} & { 1/ 3} & { 5/13} & { 7/20} & { 5/14} & { 4/11} & { 1/ 3} & { 3/ 8} & { 8/25} & { 5/13} & { 1/ 3} & { 5/13} & {10/29} & { 5/13} & {11/31} & { 5/13} & { 4/11} & {15/41} & {13/35} & {15/43} & {14/37} & {13/38} & { 5/13} & { 7/20} & { 5/13} & { 5/14} & { 5/13} & { 4/11} & { 5/13} & {17/46} & {10/27} & { 3/ 8} & { 5/14} & {19/50} & { 6/17} & { 5/13} & {19/53} & { 5/13} & { 4/11} & { 5/13} & { 7/19} & { 5/13} & {22/59} & {25/67} & {23/61} & {25/69} & { 8/21} & {\color{red} 23/64} & { 5/13} & { 4/11} & { 5/13} & {25/68} & { 5/13} & {13/35} & { 5/13} & { 3/ 8} & { 3/ 8} \\\hline
$8$ & { 4/15} && {\color{red}  7/25} && {\color{red}  8/27} && {\color{red}  9/29} && {10/31} && { 1/ 3} && {12/35} && {13/37} && {14/39} && {15/41} && {16/43} && {17/45} && {18/47} && {19/49} && {20/51} && {21/53} && { 2/ 5} && {23/57} && {24/59} && {25/61} && {26/63} && {27/65} && {28/67} && {29/69} && {30/71} && {31/73} && {32/75} && { 3/ 7} && {34/79} && {35/81} &\\\hline
$9$ & { 7/25} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 7/20} & { 2/ 5} & { 4/11} & { 3/ 8} & { 3/ 8} & { 6/17} & { 5/13} & { 1/ 3} & {11/28} & {10/29} & { 2/ 5} & {11/31} & { 2/ 5} & { 4/11} & { 2/ 5} & {13/35} & { 2/ 5} & {14/37} & {18/47} & { 5/13} & {18/49} & {16/41} & { 5/14} & {17/43} & { 4/11} & { 2/ 5} & {17/46} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {19/50} & { 2/ 5} & { 5/13} & {12/31} & { 7/18} & { 3/ 8} & {11/28} & { 7/19} & {23/58} & {22/59} & { 2/ 5} & {23/61} & { 2/ 5} & { 8/21} & { 2/ 5} & { 5/13} & { 2/ 5} & {26/67} & {30/77} & { 9/23} & {30/79} & {28/71} & {\color{red}  3/ 8} & {29/73} & {14/37} & { 2/ 5} \\\hline
$10$ & {\color{red} 14/53} && {\color{red}  5/18} && {10/31} && {\color{red}  7/23} && {\color{red} 11/35} && {\color{red} 12/37} && { 1/ 3} && {14/41} && {15/43} && {16/45} && {17/47} && {18/49} && {19/51} && {20/53} && {21/55} && {22/57} && {23/59} && {24/61} && {25/63} && { 2/ 5} && {27/67} && {28/69} && {29/71} && {30/73} && {31/75} && {32/77} && {33/79} && {34/81} && {35/83} && {36/85} &\\\hline
$11$ & { 8/29} & { 7/17} & {10/31} & { 7/17} & { 4/11} & { 7/17} & { 3/ 8} & { 7/18} & { 5/13} & { 7/19} & {11/28} & { 7/20} & { 2/ 5} & { 1/ 3} & {13/32} & { 4/11} & { 7/17} & {13/35} & { 7/17} & {14/37} & { 7/17} & { 5/13} & { 7/17} & {16/41} & {21/53} & {17/43} & {21/55} & { 2/ 5} & {17/46} & {19/47} & { 3/ 8} & {20/49} & {19/50} & { 7/17} & { 5/13} & { 7/17} & { 7/18} & { 7/17} & {11/28} & { 7/17} & {23/58} & { 2/ 5} & { 2/ 5} & { 7/18} & {25/62} & {\color{red}  8/21} & {13/32} & { 5/13} & { 9/22} & {26/67} & { 7/17} & { 9/23} & { 7/17} & {28/71} & { 7/17} & {29/73} & { 7/17} & { 2/ 5} & {35/87} & {31/77} \\\hline
$12$ & {\color{red}  5/19} && { 2/ 7} && {\color{red} 11/35} && {\color{red} 12/37} && { 1/ 3} && {\color{red}  1/ 3} && { 1/ 3} && { 1/ 3} && {16/47} && {\color{red} 17/49} && { 6/17} && {\color{red} 19/53} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} &\\\hline
$13$ & {\color{red}  3/11} & { 8/19} & {11/35} & { 8/19} & {13/37} & { 8/19} & { 5/13} & { 2/ 5} & {11/28} & { 8/21} & { 2/ 5} & { 4/11} & {13/32} & { 8/23} & { 7/17} & { 1/ 3} & { 5/12} & { 9/25} & { 8/19} & { 5/13} & { 8/19} & {16/41} & { 8/19} & {17/43} & { 8/19} & { 2/ 5} & {24/59} & {19/47} & {24/61} & {20/49} & { 8/21} & { 7/17} & { 5/13} & {22/53} & { 7/18} & {23/55} & {11/28} & { 8/19} & {23/58} & { 8/19} & { 2/ 5} & { 8/19} & {25/62} & { 8/19} & {13/32} & {16/39} & { 9/22} & { 2/ 5} & { 7/17} & {\color{red}  9/23} & {29/70} & {28/71} & { 5/12} & {29/73} & {31/74} & { 2/ 5} & { 8/19} & {31/77} & { 8/19} & {32/79} \\\hline
$14$ & { 2/ 7} && { 7/23} && { 8/25} && {\color{red} 14/41} && {10/29} && { 7/20} && { 7/20} && { 7/20} && { 1/ 3} && {18/53} && {\color{red} 19/55} && {\color{red} 20/57} && {\color{red} 21/59} && {\color{red} 22/61} && {23/63} && {24/65} && {25/67} && {26/69} && {27/71} && {28/73} && {29/75} && {30/77} && {31/79} && {32/81} && {33/83} && { 2/ 5} && {35/87} && {36/89} && {37/91} && {38/93} &\\\hline
$15$ & { 3/11} & { 3/ 7} & { 4/13} & { 3/ 7} & {14/41} & { 3/ 7} & {16/43} & { 9/22} & { 2/ 5} & { 9/23} & {13/32} & { 3/ 8} & { 7/17} & { 9/25} & { 5/12} & { 9/26} & { 8/19} & { 1/ 3} & {17/40} & { 5/14} & { 3/ 7} & {11/29} & { 3/ 7} & { 2/ 5} & { 3/ 7} & {19/47} & { 3/ 7} & {20/49} & {27/65} & { 7/17} & {27/67} & {22/53} & { 9/23} & {23/55} & {27/71} & { 8/19} & {28/73} & {25/59} & { 2/ 5} & {26/61} & {25/62} & { 3/ 7} & {13/32} & { 3/ 7} & { 9/22} & { 3/ 7} & { 7/17} & { 3/ 7} & {29/70} & {18/43} & { 5/12} & { 9/22} & {31/74} & { 2/ 5} & { 8/19} & {31/77} & {11/26} & {32/79} & {17/40} & {11/27} \\\hline
$16$ & {11/39} && { 8/25} && { 1/ 3} && {10/29} && {11/31} && { 4/11} && { 4/11} && { 4/11} && { 4/11} && { 1/ 3} && {\color{red} 20/59} && {\color{red} 21/61} && {\color{red} 22/63} && {24/65} && {\color{red} 24/67} && {\color{red} 25/69} && {\color{red} 26/71} && {27/73} && {28/75} && {29/77} && {30/79} && {31/81} && {32/83} && {33/85} && {34/87} && {35/89} && {36/91} && {37/93} && { 2/ 5} && {39/97} &\\\hline
$17$ & {\color{red} 23/85} & {10/23} & {\color{red} 13/43} & {10/23} & {\color{red}  1/ 3} & {10/23} & {17/47} & { 5/12} & {19/49} & { 2/ 5} & { 7/17} & { 5/13} & { 5/12} & {10/27} & { 8/19} & { 5/14} & {17/40} & {10/29} & { 3/ 7} & { 1/ 3} & {19/44} & {11/31} & {10/23} & { 3/ 8} & {10/23} & {13/33} & {10/23} & { 7/17} & {10/23} & {22/53} & {30/71} & {23/55} & {30/73} & { 8/19} & { 2/ 5} & {25/59} & {30/77} & {26/61} & {30/79} & { 3/ 7} & {31/81} & {28/65} & {33/83} & {29/67} & { 7/17} & {10/23} & {29/70} & {10/23} & { 5/12} & {10/23} & {31/74} & {10/23} & { 8/19} & {20/47} & {11/26} & { 5/12} & {17/40} & {20/49} & {35/82} & { 2/ 5} \\\hline
$18$ & {12/43} && { 1/ 3} && {10/29} && {11/31} && { 4/11} && {13/35} && { 3/ 8} && { 3/ 8} && { 3/ 8} && {22/61} && { 1/ 3} && {\color{red} 16/47} && {\color{red} 17/49} && { 6/17} && {\color{red} 26/71} && {\color{red} 27/73} && { 7/19} && {22/59} && { 3/ 8} && { 3/ 8} && { 3/ 8} && {32/85} && {11/29} && {34/89} && {\color{red}  5/13} && {12/31} && {\color{red} 37/95} && {38/97} && {13/33} && {21/53} &\\\hline
$19$ & {\color{red}  7/26} & {11/25} & {\color{red} 14/47} & {11/25} & {\color{red} 16/49} & {11/25} & { 6/17} & {11/26} & {20/53} & {11/27} & { 2/ 5} & {11/28} & { 8/19} & {11/29} & {17/40} & {11/30} & { 3/ 7} & {\color{red} 11/31} & {19/44} & {11/32} & {10/23} & { 1/ 3} & { 7/16} & { 6/17} & {11/25} & {13/35} & {11/25} & { 7/18} & {11/25} & {15/37} & {11/25} & { 8/19} & { 3/ 7} & {25/59} & {33/79} & {26/61} & {11/27} & { 3/ 7} & {33/83} & {28/65} & {33/85} & {29/67} & {11/29} & {10/23} & {34/89} & {31/71} & {36/91} & {32/73} & {38/93} & {11/25} & { 8/19} & {11/25} & {11/26} & {11/25} & {17/40} & {11/25} & {35/82} & {22/51} & { 3/ 7} & {11/26} \\\hline
$20$ & {\color{red} 13/47} && {16/49} && {11/31} && { 4/11} && {13/35} && {14/37} && { 5/13} && { 5/13} && { 5/13} && { 5/13} && {24/67} && { 1/ 3} && { 6/17} && {19/53} && { 4/11} && {\color{red}  7/19} && {\color{red} 30/79} && {\color{red} 23/61} && { 8/21} && { 5/13} && { 5/13} && { 5/13} && { 5/13} && {35/93} && {\color{red} 35/93} && {\color{red} 36/95} && {\color{red} 37/97} && {\color{red} 38/99} && {\color{red} 33/85} && {\color{red} 33/85} &\\\hline
$21$ & { 2/ 7} & { 4/ 9} & { 3/10} & { 4/ 9} & {18/53} & { 4/ 9} & {\color{red} 19/55} & { 3/ 7} & { 7/19} & {12/29} & {23/59} & { 2/ 5} & {25/61} & {12/31} & { 3/ 7} & { 3/ 8} & {19/44} & { 4/11} & {10/23} & {\color{red}  6/17} & { 7/16} & {\color{red} 12/35} & {11/25} & { 1/ 3} & {23/52} & {13/37} & { 4/ 9} & { 7/19} & { 4/ 9} & { 5/13} & { 4/ 9} & { 2/ 5} & { 4/ 9} & {17/41} & {36/83} & { 3/ 7} & {36/85} & {28/65} & {12/29} & {29/67} & {36/89} & {10/23} & {36/91} & {31/71} & {12/31} & {32/73} & {36/95} & {11/25} & {37/97} & {34/77} & {13/33} & {35/79} & {28/69} & { 4/ 9} & {38/91} & { 4/ 9} & { 3/ 7} & { 4/ 9} & {37/86} & {\color{red} 36/85} \\\hline
$22$ & { 8/29} && {17/53} && { 4/11} && {13/35} && {14/37} && { 5/13} && {16/41} && {11/28} && {11/28} && {11/28} && {27/71} && {26/73} && { 1/ 3} && { 4/11} && { 7/19} && {22/59} && {23/61} && {\color{red}  8/21} && { 5/13} && {26/67} && { 9/23} && {11/28} && {11/28} && {11/28} && {38/99} && {\color{red} 37/99} && {\color{red} 37/99} && {\color{red} 35/93} && {\color{red} 25/66} && {\color{red}  8/21} &\\\hline
$23$ & {15/53} & {13/29} & { 5/16} & {13/29} & {\color{red}  1/ 3} & {13/29} & {\color{red} 20/59} & {13/30} & {22/61} & {13/31} & { 8/21} & {13/32} & { 2/ 5} & {13/33} & {28/67} & {13/34} & {10/23} & {\color{red} 13/35} & { 7/16} & {\color{red} 13/36} & {11/25} & {\color{red} 13/37} & {23/52} & {\color{red} 10/29} & { 4/ 9} & { 1/ 3} & {25/56} & { 7/20} & {13/29} & {15/41} & {13/29} & { 8/21} & {13/29} & {17/43} & {13/29} & { 9/22} & {39/89} & {19/45} & { 3/ 7} & {10/23} & {13/31} & {31/71} & {39/95} & {32/73} & {39/97} & {11/25} & {13/33} & {34/77} & {22/57} & {35/79} & {25/66} & { 4/ 9} & { 8/21} & {37/83} & {31/79} & {38/85} & {23/57} & {13/29} & {29/70} & {13/29} \\\hline
$24$ & {\color{red}  3/11} && { 6/19} && {21/59} && {14/37} && { 5/13} && {16/41} && {17/43} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {29/77} && {28/79} && { 1/ 3} && {30/83} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {\color{red} 35/92} && {\color{red} 32/85} && {\color{red} 11/29} && {\color{red}  1/99} &\\\hline
$25$ & {16/57} & {14/31} & {11/34} & {14/31} & { 1/ 3} & {14/31} & {\color{red} 22/63} & { 7/16} & {\color{red} 23/65} & {14/33} & {25/67} & { 7/17} & { 9/23} & { 2/ 5} & {29/71} & { 7/18} & {31/73} & {14/37} & {11/25} & {\color{red}  7/19} & {23/52} & {\color{red} 14/39} & { 4/ 9} & {\color{red} 11/31} & {25/56} & {\color{red} 11/31} & {13/29} & { 1/ 3} & { 9/20} & {15/43} & {14/31} & {\color{red}  4/11} & {14/31} & {17/45} & {14/31} & { 9/23} & {14/31} & {19/47} & {42/95} & { 5/12} & {42/97} & { 3/ 7} & {14/33} & {11/25} & {37/89} & {34/77} & {31/76} & {35/79} & { 2/ 5} & { 4/ 9} & {31/79} & {37/83} & {\color{red} 11/31} & {38/85} & {\color{red}  4/11} & {13/29} & {\color{red} 17/45} & {40/89} & { 9/23} & {41/91} \\\hline
$26$ & {\color{red}  3/11} && {\color{red} 19/61} && {22/63} && { 5/13} && {16/41} && {17/43} && { 2/ 5} && {19/47} && {13/32} && {13/32} && {13/32} && {32/81} && {31/83} && { 6/17} && {\color{red} 28/85} && {32/89} && { 5/13} && {26/67} && { 9/23} && {28/71} && {\color{red} 29/73} && {\color{red}  2/ 5} && {\color{red} 31/77} && {\color{red} 32/79} && {13/32} && {13/32} && {13/32} && {\color{red} 19/49} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$27$ & {\color{red} 17/61} & { 5/11} & { 1/ 3} & { 5/11} & {13/38} & { 5/11} & {\color{red} 24/67} & {15/34} & { 5/14} & { 3/ 7} & {\color{red} 26/71} & { 5/12} & {28/73} & {15/37} & { 2/ 5} & {15/38} & {32/77} & { 5/13} & {34/79} & {\color{red}  3/ 8} & { 4/ 9} & {31/82} & {25/56} & { 4/11} & {13/29} & { 4/11} & { 9/20} & { 4/11} & {14/31} & { 1/ 3} & {29/64} & {\color{red}  8/23} & { 5/11} & {\color{red} 17/47} & { 5/11} & { 3/ 8} & { 5/11} & {19/49} & { 5/11} & { 2/ 5} & {41/92} & { 7/17} & {38/87} & {11/26} & { 3/ 7} & {23/53} & {37/88} & { 4/ 9} & {26/63} & {37/83} & {\color{red} 31/82} & {38/85} & {\color{red} 31/86} & {13/29} & {\color{red}  4/11} & {40/89} & {\color{red}  4/11} & {41/91} & {\color{red}  1/99} & {14/31} \\\hline
$28$ & { 2/ 7} && {\color{red}  4/13} && {\color{red} 23/67} && {26/69} && {17/43} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && { 7/17} && { 7/17} && { 7/17} && {34/87} && {33/89} && {32/91} && {\color{red} 29/89} && {34/95} && {37/97} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && { 7/17} && { 7/17} && { 7/17} && {\color{red}  1/99} &\\\hline
$29$ & {\color{red}  5/18} & {16/35} & {22/67} & {16/35} & { 7/20} & {16/35} & { 5/14} & { 4/ 9} & { 4/11} & {16/37} & {17/46} & { 8/19} & {29/77} & {16/39} & {31/79} & { 2/ 5} & {11/27} & {16/41} & {35/83} & { 8/21} & {37/85} & {\color{red} 16/43} & {13/29} & {\color{red}  3/ 8} & { 9/20} & {13/35} & {14/31} & {13/35} & {29/64} & {17/47} & { 5/11} & { 1/ 3} & {31/68} & {\color{red}  8/23} & {16/35} & {\color{red}  9/25} & {16/35} & {\color{red} 19/51} & {16/35} & {\color{red}  5/13} & {16/35} & {21/53} & {35/78} & {11/27} & {37/84} & {23/55} & {16/37} & { 3/ 7} & {\color{red} 16/41} & {25/57} & {38/91} & {13/29} & {\color{red}  3/ 8} & {40/89} & {\color{red}  3/ 8} & {41/91} & {\color{red} 17/46} & {14/31} & {\color{red}  1/99} & {43/95} \\\hline
$30$ & {19/67} && {\color{red}  4/13} && {\color{red} 24/71} && {27/73} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && {22/53} && { 5/12} && { 5/12} && { 5/12} && {37/91} && {12/31} && { 7/19} && {\color{red}  9/26} && { 1/ 3} && {\color{red} 15/43} && {25/66} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {\color{red} 37/89} && {\color{red} 37/91} && {\color{red} 12/31} &\\\hline
$31$ & {\color{red} 19/69} & {17/37} & {23/71} & {17/37} & { 5/14} & {17/37} & { 4/11} & {17/38} & {17/46} & {17/39} & { 3/ 8} & {17/40} & {\color{red} 14/37} & {17/41} & {32/83} & {17/42} & { 2/ 5} & {17/43} & {12/29} & {17/44} & {38/89} & {\color{red} 17/45} & {40/91} & {\color{red} 35/92} & {14/31} & {14/37} & {29/64} & {14/37} & { 5/11} & {14/37} & {31/68} & { 9/25} & {16/35} & {\color{red} 25/77} & {11/24} & {\color{red} 26/73} & {17/37} & {\color{red}  9/25} & {17/37} & {\color{red} 10/27} & {17/37} & {\color{red} 31/83} & {17/37} & {11/28} & {\color{red} 17/40} & {23/57} & {43/97} & {12/29} & {17/39} & {\color{red} 37/89} & {\color{red} 17/43} & {\color{red} 38/89} & {\color{red} 17/44} & {27/61} & {\color{red} 35/92} & {14/31} & {\color{red} 35/92} & {43/95} & {\color{red}  3/ 8} & {44/97} \\\hline
$32$ & {20/71} && {\color{red} 13/41} && {26/75} && { 4/11} && {31/79} && {20/49} && { 7/17} && {22/53} && {23/55} && { 8/19} && { 8/19} && { 8/19} && { 8/19} && {39/97} && {38/99} && {\color{red} 26/71} && {\color{red} 13/38} && {\color{red}  1/99} && {\color{red}  8/23} && {\color{red}  4/11} && {23/58} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && { 8/19} &\\\hline
$33$ & {\color{red} 11/40} & { 6/13} & { 8/25} & { 6/13} & { 4/11} & { 6/13} & {17/46} & { 9/20} & { 3/ 8} & {18/41} & {19/50} & { 3/ 7} & { 5/13} & {18/43} & {\color{red}  5/13} & { 9/22} & {35/89} & { 2/ 5} & {37/91} & { 9/23} & {13/31} & {\color{red} 18/47} & {41/95} & { 8/21} & {43/97} & {\color{red} 19/49} & { 5/11} & { 5/13} & {31/68} & { 5/13} & {16/35} & { 5/13} & {11/24} & {\color{red} 11/31} & {17/37} & {\color{red}  1/99} & {35/76} & { 4/11} & { 6/13} & {\color{red} 29/79} & { 6/13} & {\color{red} 10/27} & { 6/13} & {\color{red} 11/29} & {\color{red} 18/41} & {\color{red} 34/89} & {\color{red}  3/ 7} & {\color{red} 35/89} & {\color{red} 18/43} & {\color{red} 37/91} & {\color{red}  9/22} & {13/31} & {\color{red}  2/ 5} & { 3/ 7} & {\color{red}  9/23} & {\color{red} 41/95} & {\color{red} 18/47} & {\color{red} 43/97} & {\color{red} 19/49} & { 5/11} \\\hline
$34$ & {\color{red}  7/25} && {14/43} && {\color{red} 27/79} && {\color{red} 29/81} && {32/83} && { 7/17} && {22/53} && {23/55} && { 8/19} && {25/59} && {17/40} && {17/40} && {17/40} && {37/89} && {39/98} && { 8/21} && {\color{red} 31/86} && {\color{red}  7/20} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 18/49} && {\color{red} 23/59} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} &\\\hline
$35$ & { 2/ 7} & {19/41} & {\color{red} 25/79} & {19/41} & {29/81} & {19/41} & { 3/ 8} & {19/42} & {19/50} & {19/43} & { 5/13} & {19/44} & { 7/18} & {19/45} & {16/41} & {19/46} & {\color{red} 16/41} & {19/47} & { 2/ 5} & {19/48} & {40/97} & {\color{red} 19/49} & {14/33} & {\color{red}  5/13} & {27/62} & {26/67} & {25/56} & {16/41} & {16/35} & {16/41} & {11/24} & {16/41} & {17/37} & {21/55} & {35/76} & { 5/14} & { 6/13} & {\color{red}  1/99} & {37/80} & {\color{red}  1/99} & {19/41} & {\color{red} 31/83} & {19/41} & {\color{red} 32/85} & {19/41} & {\color{red} 11/29} & {\color{red} 19/43} & {\color{red} 12/31} & {\color{red} 19/44} & {\color{red} 37/95} & {\color{red} 19/45} & {\color{red}  2/ 5} & {\color{red} 19/46} & {\color{red} 40/97} & {\color{red} 19/47} & {14/33} & {\color{red} 19/48} & {\color{red} 23/54} & {\color{red} 19/49} & {\color{red} 27/62} \\\hline
$36$ & {\color{red} 12/43} && { 1/ 3} && {\color{red} 16/47} && {\color{red}  6/17} && {11/29} && {36/89} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {37/90} && {28/71} && {\color{red} 11/30} && {\color{red}  5/14} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 11/29} && {\color{red} 36/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {23/54} &\\\hline
$37$ & {23/81} & {20/43} & {\color{red} 26/83} & {20/43} & { 6/17} & {20/43} & {19/50} & { 5/11} & { 5/13} & { 4/ 9} & { 7/18} & {10/23} & {11/28} & {20/47} & {17/43} & { 5/12} & {17/43} & {20/49} & {\color{red} 17/43} & { 2/ 5} & {28/69} & {\color{red} 20/51} & {38/91} & {\color{red} 26/67} & { 3/ 7} & { 9/23} & {29/66} & {28/71} & {40/89} & {17/43} & {17/37} & {17/43} & {35/76} & {17/43} & { 6/13} & {\color{red} 26/71} & {37/80} & {\color{red}  1/99} & {19/41} & {\color{red}  1/99} & {13/28} & {\color{red}  1/99} & {20/43} & {\color{red}  1/99} & {20/43} & {\color{red}  1/99} & {20/43} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} & {\color{red} 10/23} & {\color{red}  1/99} & {\color{red} 20/47} & {\color{red}  1/99} & {\color{red}  5/12} & {\color{red} 28/69} & {\color{red} 20/49} & {\color{red} 38/91} & {\color{red}  2/ 5} & { 3/ 7} \\\hline
$38$ & {\color{red} 23/83} && {28/85} && {17/49} && {\color{red} 32/89} && {34/91} && {37/93} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {19/44} && {19/44} && {19/44} && {36/85} && {\color{red}  2/ 5} && { 9/23} && {\color{red} 35/94} && {\color{red}  4/11} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 32/89} && {\color{red} 39/97} && { 8/19} && {41/97} && {14/33} && {23/54} && {41/96} &\\\hline
$39$ & {24/85} & { 7/15} & {\color{red}  5/16} & { 7/15} & {\color{red} 31/89} & { 7/15} & { 5/13} & {21/46} & { 7/18} & {21/47} & {11/28} & { 7/16} & {23/58} & { 3/ 7} & { 2/ 5} & {21/50} & { 2/ 5} & { 7/17} & { 2/ 5} & {21/52} & { 2/ 5} & {\color{red} 21/53} & {37/90} & {\color{red}  9/23} & {27/64} & {\color{red} 28/71} & {16/37} & {\color{red} 29/73} & {27/61} & { 2/ 5} & {33/73} & { 2/ 5} & { 6/13} & { 2/ 5} & {37/80} & { 2/ 5} & {19/41} & {\color{red} 37/99} & {13/28} & {\color{red}  1/99} & {20/43} & {\color{red}  1/99} & {41/88} & {\color{red}  1/99} & { 7/15} & {\color{red}  1/99} & { 7/15} & {\color{red}  1/99} & {\color{red} 21/46} & {\color{red}  1/99} & {\color{red} 21/47} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red}  1/99} & {\color{red} 21/50} & {\color{red}  1/99} & {\color{red}  7/17} & {\color{red}  1/99} \\\hline
$40$ & {\color{red} 13/47} && {29/89} && { 6/17} && {\color{red} 34/93} && {\color{red}  7/19} && {38/97} && {41/99} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {10/23} && {10/23} && {10/23} && {\color{red} 39/94} && {\color{red} 19/48} && {\color{red} 37/98} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 38/97} && {\color{red} 41/99} && {23/54} && {41/96} && { 3/ 7} &\\\hline
$41$ & {\color{red} 25/89} & {22/47} & {\color{red}  8/25} & {22/47} & {\color{red} 32/93} & {22/47} & {36/95} & {11/24} & {11/28} & {22/49} & {23/58} & {11/25} & { 2/ 5} & {22/51} & {25/62} & {11/26} & {19/47} & {22/53} & {\color{red} 19/47} & {11/27} & {\color{red} 19/47} & {\color{red}  9/23} & {15/37} & {\color{red} 28/71} & {37/89} & {\color{red} 29/73} & {26/61} & {\color{red}  2/ 5} & {17/39} & {\color{red} 31/77} & {\color{red}  7/16} & {19/47} & { 5/11} & {19/47} & {19/41} & {19/47} & {13/28} & {\color{red} 31/80} & {20/43} & {\color{red}  1/99} & {41/88} & {\color{red}  1/99} & { 7/15} & {\color{red}  1/99} & {43/92} & {\color{red}  1/99} & {22/47} & {\color{red}  1/99} & {22/47} & {\color{red}  1/99} & {\color{red} 11/24} & {\color{red}  1/99} & {\color{red} 22/49} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red}  1/99} & {\color{red} 22/51} & {\color{red}  1/99} & {\color{red} 11/26} & {\color{red}  1/99} \\\hline
$42$ & { 2/ 7} && {10/31} && {19/53} && {\color{red}  4/11} && {\color{red}  7/19} && {22/57} && {31/76} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && { 7/16} && { 7/16} && { 7/16} && {\color{red} 41/98} && {\color{red} 20/49} && { 2/ 5} && {\color{red}  3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 31/76} && { 3/ 7} && {40/93} &\\\hline
$43$ & {\color{red}  7/25} & {23/49} & {17/52} & {23/49} & {34/97} & {23/49} & {37/99} & {23/50} & {23/58} & {23/51} & { 2/ 5} & {23/52} & {25/62} & {23/53} & {13/32} & {23/54} & {20/49} & {23/55} & {20/49} & {23/56} & {\color{red} 20/49} & {\color{red} 11/28} & {\color{red} 15/38} & {\color{red} 29/73} & {16/39} & {\color{red}  2/ 5} & {29/69} & {\color{red} 31/77} & {40/93} & {32/79} & {18/41} & {11/27} & {\color{red} 37/84} & {20/49} & {\color{red} 19/42} & {20/49} & {20/43} & {20/49} & {41/88} & {\color{red} 31/81} & { 7/15} & {\color{red}  1/99} & {43/92} & {\color{red}  1/99} & {22/47} & {\color{red}  1/99} & {15/32} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {\color{red} 23/50} & {\color{red}  1/99} & {\color{red} 23/51} & {\color{red}  1/99} & {\color{red} 23/52} & {\color{red}  1/99} & {\color{red} 23/53} & {\color{red}  1/99} \\\hline
$44$ & {27/95} && {\color{red} 31/97} && { 4/11} && { 7/19} && {\color{red} 22/59} && {\color{red}  8/21} && {39/97} && {27/64} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {11/25} && {11/25} && {11/25} && {\color{red} 35/83} && {\color{red} 21/52} && {\color{red} 29/75} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 27/64} &\\\hline
$45$ & {\color{red} 27/97} & { 8/17} & { 1/ 3} & { 8/17} & {\color{red} 26/75} & { 8/17} & {31/84} & {\color{red} 11/25} & { 2/ 5} & {24/53} & {25/62} & { 4/ 9} & {13/32} & {24/55} & { 9/22} & { 3/ 7} & { 7/17} & { 8/19} & { 7/17} & {12/29} & { 7/17} & {\color{red} 23/58} & { 7/17} & { 2/ 5} & {\color{red}  2/ 5} & {\color{red} 31/77} & {17/41} & {\color{red} 32/79} & {39/92} & {11/27} & {\color{red}  3/ 7} & {34/83} & {19/43} & { 7/17} & {\color{red} 39/88} & { 7/17} & {\color{red}  5/11} & { 7/17} & { 7/15} & { 7/17} & {43/92} & {\color{red}  1/99} & {22/47} & {\color{red}  1/99} & {15/32} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {39/83} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {\color{red}  6/13} & {\color{red}  1/99} & {\color{red} 24/53} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} \\\hline
$46$ & {28/99} && {\color{red} 14/45} && {23/64} && {22/59} && {23/61} && {\color{red}  8/21} && {23/58} && {37/89} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} && {23/52} && {23/52} && {23/52} && {\color{red} 31/73} && {\color{red} 22/53} && {11/27} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$47$ & {\color{red}  5/18} & {25/53} & {\color{red}  9/28} & {25/53} & {\color{red} 10/29} & {25/53} & {\color{red} 35/96} & {\color{red} 23/52} & {28/71} & { 5/11} & {13/32} & {25/56} & { 9/22} & {25/57} & { 7/17} & {25/58} & {29/70} & {25/59} & {22/53} & {\color{red} 24/59} & {22/53} & {\color{red}  2/ 5} & {22/53} & {\color{red} 29/77} & {\color{red} 35/89} & {\color{red} 32/79} & {\color{red} 17/42} & {\color{red} 11/27} & {18/43} & {34/83} & {41/96} & { 7/17} & {\color{red} 19/44} & {12/29} & { 4/ 9} & {22/53} & {\color{red} 41/92} & {22/53} & {\color{red} 21/46} & {22/53} & {22/47} & {\color{red} 21/53} & {15/32} & {\color{red}  1/99} & {23/49} & {\color{red}  1/99} & {39/83} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {41/87} & {\color{red}  1/99} & {25/53} & {\color{red}  1/99} & {25/53} & {\color{red}  1/99} & {\color{red} 25/54} & {\color{red}  1/99} & {\color{red}  5/11} & {\color{red}  1/99} \\\hline
$48$ & {\color{red} 20/71} && {\color{red}  6/19} && {27/76} && {23/61} && { 8/21} && {\color{red}  5/13} && {\color{red}  9/23} && {16/39} && {\color{red} 30/71} && {32/73} && {11/25} && {34/77} && {35/79} && { 4/ 9} && { 4/ 9} && { 4/ 9} && { 4/ 9} && {\color{red} 41/96} && {\color{red} 23/56} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$49$ & { 2/ 7} & {26/55} & {\color{red} 25/78} & {26/55} & {\color{red}  7/20} & {\color{red} 24/53} & {\color{red} 31/86} & {\color{red} 23/53} & {37/95} & {26/57} & { 9/22} & {\color{red}  3/ 7} & { 7/17} & {26/59} & {29/70} & {\color{red} 23/57} & { 5/12} & {\color{red}  5/12} & {23/55} & {\color{red}  2/ 5} & {23/55} & {\color{red} 25/62} & {23/55} & {\color{red}  3/ 8} & {\color{red} 37/93} & {\color{red} 32/81} & {\color{red} 35/88} & {\color{red} 34/83} & {\color{red}  9/22} & { 7/17} & {19/45} & {12/29} & {\color{red} 39/92} & {37/89} & {\color{red} 10/23} & {38/91} & {21/47} & {23/55} & {\color{red} 43/96} & {23/55} & {\color{red} 11/24} & {23/55} & {23/49} & {\color{red}  4/11} & {39/83} & {\color{red}  1/99} & { 8/17} & {\color{red}  1/99} & {41/87} & {\color{red}  1/99} & {25/53} & {\color{red}  1/99} & {17/36} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {\color{red} 13/28} & {\color{red}  1/99} \\\hline
$50$ & {\color{red} 16/57} && {\color{red} 19/59} && {\color{red} 13/37} && { 8/21} && { 5/13} && {26/67} && {\color{red}  9/23} && {32/79} && {\color{red} 41/98} && {11/25} && {34/77} && {35/79} && { 4/ 9} && {37/83} && {25/56} && {25/56} && {25/56} && {\color{red} 40/93} && {\color{red}  8/19} && {12/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & {\color{red}  8/29} & { 9/19} & {\color{red} 29/91} & { 9/19} & {11/31} & {\color{red}  5/11} & {\color{red} 23/63} & {\color{red} 24/55} & { 5/13} & {\color{red} 25/57} & { 7/17} & {\color{red} 25/58} & {29/70} & {\color{red} 23/57} & { 5/12} & {\color{red} 23/58} & {31/74} & {\color{red} 27/73} & { 8/19} & {\color{red} 25/62} & { 8/19} & {\color{red} 29/79} & { 8/19} & {\color{red}  7/19} & { 8/19} & {\color{red} 19/50} & { 2/ 5} & { 7/17} & {\color{red} 37/92} & {12/29} & {\color{red} 19/46} & {37/89} & {20/47} & {38/91} & {\color{red} 41/96} & {13/31} & {\color{red}  7/16} & { 8/19} & {22/49} & { 8/19} & {\color{red}  9/20} & { 8/19} & {\color{red} 23/50} & { 8/19} & { 8/17} & {\color{red}  1/99} & {41/87} & {\color{red}  1/99} & {25/53} & {\color{red}  1/99} & {17/36} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {44/93} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} \\\hline
$52$ & {\color{red}  3/11} && {20/61} && {\color{red} 23/67} && { 5/13} && {26/67} && { 9/23} && {\color{red} 28/71} && {\color{red}  2/ 5} && {\color{red}  7/17} && {\color{red}  3/ 7} && {35/79} && { 4/ 9} && {37/83} && {38/85} && {13/29} && {13/29} && {13/29} && {13/29} && {\color{red} 35/81} && {\color{red}  5/12} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & {\color{red}  7/29} & {28/59} & {\color{red} 23/73} & {\color{red}  9/19} & {23/64} & {\color{red} 25/56} & {\color{red}  4/11} & {\color{red} 25/57} & {\color{red}  3/ 8} & {\color{red} 28/67} & {\color{red}  2/ 5} & {\color{red} 28/69} & { 5/12} & {\color{red} 28/71} & {31/74} & {\color{red} 28/73} & { 8/19} & {\color{red} 28/75} & {11/26} & {\color{red} 30/79} & {25/59} & {\color{red} 30/79} & {\color{red} 41/97} & {\color{red} 35/94} & {\color{red} 41/99} & {\color{red} 35/94} & {\color{red} 40/99} & {\color{red}  1/99} & {\color{red}  1/99} & {37/89} & {\color{red} 13/32} & {38/91} & {\color{red}  5/12} & {13/31} & { 3/ 7} & { 8/19} & {\color{red} 40/93} & {41/97} & {\color{red} 11/25} & {25/59} & {23/51} & {25/59} & {\color{red} 33/73} & {\color{red} 12/29} & {\color{red}  6/13} & {\color{red} 13/35} & {25/53} & {\color{red}  1/99} & {17/36} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {44/93} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {46/97} & {\color{red}  1/99} & {28/59} & {\color{red}  1/99} \\\hline
$54$ & {\color{red}  1/99} && { 1/ 3} && {\color{red} 18/53} && {\color{red} 25/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {\color{red} 32/79} && {\color{red} 33/79} && { 4/ 9} && {37/83} && {38/85} && {13/29} && {40/89} && { 9/20} && {\color{red} 40/91} && { 9/20} && {\color{red}  2/ 5} && {\color{red} 13/33} && {\color{red} 21/53} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & {\color{red}  1/99} & {29/61} & {\color{red}  1/99} & {\color{red} 29/63} & { 4/11} & {\color{red} 13/29} & {\color{red} 25/68} & {\color{red} 29/67} & {\color{red} 13/35} & {\color{red} 29/69} & {\color{red} 36/91} & {\color{red} 29/71} & {31/74} & {\color{red} 29/73} & { 8/19} & {\color{red} 29/75} & {11/26} & {\color{red} 29/77} & {17/40} & {\color{red} 10/27} & {\color{red} 23/54} & {\color{red} 31/83} & {\color{red} 23/54} & {\color{red} 32/85} & {\color{red} 23/54} & {\color{red} 32/85} & {\color{red} 31/76} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {13/31} & {\color{red} 25/61} & { 8/19} & {\color{red} 21/50} & {41/97} & {22/51} & {14/33} & {\color{red} 29/67} & {23/54} & {\color{red} 23/52} & {\color{red} 23/54} & {24/53} & {\color{red} 31/76} & {\color{red} 44/97} & {\color{red}  8/21} & {\color{red} 25/54} & {\color{red}  1/99} & {26/55} & {\color{red}  1/99} & {44/93} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {46/97} & {\color{red}  1/99} & {28/59} & {\color{red}  1/99} & {19/40} & {\color{red}  1/99} \\\hline
$56$ & {\color{red}  1/99} && {\color{red} 21/65} && {\color{red} 23/67} && {\color{red} 36/97} && {28/71} && {29/73} && { 2/ 5} && {\color{red} 31/77} && {\color{red} 11/27} && {\color{red} 23/55} && {\color{red} 36/83} && {38/85} && {13/29} && {40/89} && {41/91} && {14/31} && {14/31} && {\color{red} 41/95} && {\color{red} 40/97} && {\color{red} 21/53} && {\color{red} 39/98} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & {\color{red}  1/99} & {10/21} & {\color{red}  1/99} & {\color{red}  6/13} & {\color{red}  6/17} & {\color{red}  9/20} & {13/35} & {\color{red} 10/23} & {\color{red}  3/ 8} & {\color{red} 30/71} & {\color{red} 11/28} & {\color{red} 30/73} & { 8/19} & {\color{red}  2/ 5} & {11/26} & {\color{red} 30/77} & {17/40} & {\color{red} 30/79} & {35/82} & {\color{red} 31/83} & { 3/ 7} & {\color{red} 32/85} & { 3/ 7} & {\color{red} 11/29} & { 3/ 7} & {\color{red}  1/99} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/19} & {\color{red}  1/99} & {41/97} & {\color{red}  1/99} & {14/33} & {\color{red} 11/26} & {23/54} & {23/53} & {41/96} & {\color{red} 37/85} & { 3/ 7} & {\color{red}  4/ 9} & { 3/ 7} & { 5/11} & {\color{red} 39/97} & {\color{red} 41/90} & {\color{red} 14/37} & {\color{red} 13/28} & {\color{red}  1/99} & { 9/19} & {\color{red}  1/99} & {46/97} & {\color{red}  1/99} & {28/59} & {\color{red}  1/99} & {19/40} & {\color{red}  1/99} & {29/61} & {\color{red}  1/99} \\\hline
$58$ & {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  8/23} && {16/43} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {\color{red} 13/32} && {\color{red}  7/17} && {\color{red} 40/93} && {13/29} && {40/89} && {41/91} && {14/31} && {43/95} && {\color{red} 43/95} && {\color{red} 43/97} && {\color{red} 14/33} && {\color{red} 28/69} && {\color{red}  2/ 5} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & {\color{red}  1/99} & {31/65} & {\color{red}  1/99} & {\color{red} 31/67} & {\color{red} 33/94} & {\color{red} 31/69} & { 3/ 8} & {\color{red} 31/71} & {\color{red} 14/37} & {\color{red} 31/73} & {\color{red} 26/67} & {\color{red} 31/75} & {\color{red} 16/39} & {\color{red} 31/77} & {17/40} & {\color{red} 31/79} & {35/82} & {\color{red} 31/81} & { 3/ 7} & {\color{red} 32/85} & {37/86} & {\color{red} 11/29} & {\color{red} 37/86} & {\color{red} 34/89} & {\color{red} 40/93} & {\color{red}  1/99} & {\color{red} 27/64} & {\color{red}  1/99} & {\color{red} 20/51} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {14/33} & {\color{red}  1/99} & {23/54} & {\color{red}  1/99} & {41/96} & {\color{red} 23/54} & { 3/ 7} & {24/55} & {40/93} & {\color{red}  7/16} & {\color{red} 40/93} & {\color{red} 25/56} & {\color{red} 27/64} & {26/57} & {\color{red} 23/58} & {\color{red} 37/81} & {\color{red} 35/92} & {\color{red} 27/58} & {\color{red}  1/99} & {28/59} & {\color{red}  1/99} & {19/40} & {\color{red}  1/99} & {29/61} & {\color{red}  1/99} & {39/82} & {\color{red}  1/99} \\\hline
$60$ & {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 25/71} && {\color{red} 23/64} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {\color{red} 38/93} && {\color{red} 12/29} && {\color{red} 37/89} && {\color{red} 39/89} && {41/91} && {14/31} && {43/95} && {44/97} && { 5/11} && { 5/11} && {\color{red} 27/62} && {\color{red} 38/91} && {\color{red} 39/97} && {\color{red} 23/57} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 3, 3+k, 3+k+i\}$.
\end{center}


==> tables/table-g4-a01b04.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 2/ 9} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 5/19} & { 1/ 3} & { 1/ 3} & { 3/11} & { 1/ 3} & { 1/ 3} & { 7/25} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 9/31} & { 1/ 3} & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & {11/37} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & {13/43} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & {15/49} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {17/55} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & {19/61} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {21/67} & { 1/ 3} & { 1/ 3} \\\hline
$2$ & { 4/13} & { 1/ 3} & { 2/ 5} & { 2/ 7} & { 2/ 5} & { 1/ 3} & { 6/17} & { 2/ 5} & { 6/19} & { 2/ 5} & { 8/23} & { 4/11} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 5/14} & {10/27} & { 2/ 5} & {10/29} & { 2/ 5} & { 4/11} & { 3/ 8} & { 2/ 5} & { 6/17} & { 2/ 5} & { 7/19} & {14/37} & { 2/ 5} & {14/39} & { 2/ 5} & {16/43} & { 8/21} & { 2/ 5} & { 4/11} & { 2/ 5} & { 3/ 8} & {18/47} & { 2/ 5} & {18/49} & { 2/ 5} & {20/53} & { 5/13} & { 2/ 5} & {10/27} & { 2/ 5} & {11/29} & {22/57} & { 2/ 5} & {22/59} & { 2/ 5} & { 8/21} & {12/31} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {13/34} & {26/67} & { 2/ 5} & {26/69} & { 2/ 5} \\\hline
$3$ & { 1/ 3} & { 3/ 8} & { 4/11} & { 1/ 3} & { 3/ 8} & { 5/14} & { 1/ 3} & { 3/ 8} & { 6/17} & { 3/ 8} & { 7/19} & { 7/20} & { 3/ 8} & { 4/11} & { 8/23} & { 3/ 8} & { 9/25} & { 3/ 8} & {10/27} & { 5/14} & { 3/ 8} & {11/30} & {11/31} & { 3/ 8} & { 4/11} & { 3/ 8} & {13/35} & {13/36} & { 3/ 8} & { 7/19} & {14/39} & { 3/ 8} & {15/41} & { 3/ 8} & {16/43} & { 4/11} & { 3/ 8} & {17/46} & {17/47} & { 3/ 8} & {18/49} & { 3/ 8} & {19/51} & {19/52} & { 3/ 8} & {10/27} & { 4/11} & { 3/ 8} & { 7/19} & { 3/ 8} & {22/59} & {11/30} & { 3/ 8} & {23/62} & {23/63} & { 3/ 8} & {24/65} & { 3/ 8} & {25/67} & {25/68} \\\hline
$4$ & { 5/17} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} \\\hline
$5$ & { 6/19} & { 2/ 5} & { 5/13} & { 7/22} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 7/18} & { 1/ 3} & { 2/ 5} & { 8/21} & { 2/ 5} & { 9/23} & { 3/ 8} & { 2/ 5} & { 5/13} & { 2/ 5} & {11/28} & {11/29} & { 2/ 5} & {12/31} & { 2/ 5} & {13/33} & {13/34} & { 2/ 5} & { 7/18} & { 2/ 5} & {15/38} & { 5/13} & { 2/ 5} & {16/41} & { 2/ 5} & {17/43} & {17/44} & { 2/ 5} & { 9/23} & { 2/ 5} & {19/48} & {19/49} & { 2/ 5} & {20/51} & { 2/ 5} & {21/53} & { 7/18} & { 2/ 5} & {11/28} & { 2/ 5} & {23/58} & {23/59} & { 2/ 5} & {24/61} & { 2/ 5} & {25/63} & {25/64} & { 2/ 5} & {13/33} & { 2/ 5} & {27/68} & { 9/23} & { 2/ 5} \\\hline
$6$ & { 1/ 3} & { 4/11} & { 5/14} & { 1/ 3} & { 4/11} & { 6/17} & { 1/ 3} & { 4/11} & { 7/20} & { 1/ 3} & { 4/11} & { 8/23} & { 4/11} & { 9/25} & { 9/26} & { 4/11} & { 5/14} & {10/29} & { 4/11} & {11/31} & {11/32} & { 4/11} & { 6/17} & { 4/11} & {13/36} & {13/37} & { 4/11} & {14/39} & { 7/20} & { 4/11} & { 5/14} & {15/43} & { 4/11} & {16/45} & { 4/11} & {17/47} & {17/48} & { 4/11} & { 9/25} & { 6/17} & { 4/11} & {19/53} & {19/54} & { 4/11} & { 5/14} & { 4/11} & {21/58} & {21/59} & { 4/11} & {22/61} & {11/31} & { 4/11} & {23/64} & {23/65} & { 4/11} & {24/67} & { 4/11} & {25/69} & { 5/14} & { 4/11} \\\hline
$7$ & { 7/23} & { 6/17} & { 2/ 5} & { 6/19} & { 2/ 5} & { 1/ 3} & { 4/11} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 1/ 3} & {10/27} & { 2/ 5} & {10/29} & { 2/ 5} & {13/38} & { 3/ 8} & { 2/ 5} & { 6/17} & { 2/ 5} & {15/43} & {14/37} & { 2/ 5} & {14/39} & { 2/ 5} & {17/48} & { 8/21} & { 2/ 5} & { 4/11} & { 2/ 5} & {19/53} & {18/47} & { 2/ 5} & {18/49} & { 2/ 5} & {21/58} & { 5/13} & { 2/ 5} & {10/27} & { 2/ 5} & {23/63} & {22/57} & { 2/ 5} & {22/59} & { 2/ 5} & {25/68} & {12/31} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {27/73} & {26/67} & { 2/ 5} & {26/69} & { 2/ 5} & {29/78} & { 7/18} & { 2/ 5} & {14/37} & { 2/ 5} \\\hline
$8$ & { 8/25} & { 5/13} & { 3/ 8} & { 2/ 7} & { 5/13} & { 7/19} & {11/31} & { 8/21} & { 4/11} & { 5/13} & { 3/ 8} & { 1/ 3} & { 5/13} & {10/27} & { 5/13} & {11/29} & {11/30} & { 5/13} & { 3/ 8} & { 4/11} & {13/34} & {13/35} & { 5/13} & {14/37} & { 7/19} & { 5/13} & { 3/ 8} & { 5/13} & { 8/21} & {16/43} & { 5/13} & {17/45} & {17/46} & {18/47} & { 3/ 8} & { 5/13} & {19/50} & {19/51} & { 5/13} & {20/53} & { 5/13} & {21/55} & { 3/ 8} & { 5/13} & {11/29} & {22/59} & {23/60} & {23/61} & { 5/13} & { 8/21} & { 3/ 8} & { 5/13} & {25/66} & { 5/13} & {13/34} & {26/69} & { 5/13} & {27/71} & {\color{red}  3/ 8} & {28/73} \\\hline
$9$ & { 1/ 3} & { 5/14} & { 6/17} & { 1/ 3} & { 5/14} & { 7/20} & { 1/ 3} & { 5/14} & { 8/23} & { 6/17} & { 5/14} & { 9/26} & { 1/ 3} & { 5/14} & { 6/17} & { 5/14} & {11/31} & {11/32} & { 5/14} & { 6/17} & {12/35} & { 5/14} & {13/37} & {13/38} & { 5/14} & { 7/20} & { 6/17} & { 5/14} & {15/43} & { 5/14} & {16/45} & { 6/17} & { 5/14} & {17/48} & {17/49} & { 5/14} & { 6/17} & { 9/26} & { 5/14} & {19/54} & {19/55} & { 5/14} & {20/57} & { 5/14} & {21/59} & { 7/20} & { 5/14} & {11/31} & { 6/17} & { 5/14} & {23/65} & {23/66} & { 5/14} & { 6/17} & { 8/23} & { 5/14} & {25/71} & { 5/14} & {26/73} & {13/37} \\\hline
$10$ & { 9/29} & { 2/ 5} & { 7/18} & { 5/16} & { 2/ 5} & { 6/17} & { 2/ 5} & { 9/23} & { 1/ 3} & { 2/ 5} & { 5/13} & { 2/ 5} & {11/28} & { 1/ 3} & { 2/ 5} & {12/31} & { 2/ 5} & {13/33} & {17/47} & { 2/ 5} & { 7/18} & { 2/ 5} & {15/38} & { 5/13} & { 2/ 5} & {16/41} & { 2/ 5} & {17/43} & {17/44} & { 2/ 5} & { 9/23} & { 2/ 5} & {19/48} & {19/49} & { 2/ 5} & {20/51} & { 2/ 5} & {21/53} & { 7/18} & { 2/ 5} & {11/28} & { 2/ 5} & {23/58} & {23/59} & { 2/ 5} & {24/61} & { 2/ 5} & {25/63} & {25/64} & { 2/ 5} & {13/33} & { 2/ 5} & {27/68} & { 9/23} & { 2/ 5} & {28/71} & { 2/ 5} & {29/73} & {29/74} & { 2/ 5} \\\hline
$11$ & {10/31} & { 3/ 8} & { 7/19} & { 5/17} & { 3/ 8} & { 4/11} & {12/37} & { 3/ 8} & { 9/25} & { 3/ 8} & {10/27} & { 5/14} & { 3/ 8} & {11/30} & { 1/ 3} & { 3/ 8} & { 4/11} & { 3/ 8} & {13/35} & {13/36} & { 3/ 8} & { 7/19} & {14/39} & { 3/ 8} & {15/41} & { 3/ 8} & {16/43} & { 4/11} & { 3/ 8} & {17/46} & {17/47} & { 3/ 8} & {18/49} & { 3/ 8} & {19/51} & {19/52} & { 3/ 8} & {10/27} & { 4/11} & { 3/ 8} & { 7/19} & { 3/ 8} & {22/59} & {11/30} & { 3/ 8} & {23/62} & {23/63} & { 3/ 8} & {24/65} & { 3/ 8} & {25/67} & {25/68} & { 3/ 8} & {13/35} & {26/71} & { 3/ 8} & {27/73} & { 3/ 8} & {28/75} & { 7/19} \\\hline
$12$ & { 1/ 3} & { 4/11} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 8/23} & {10/27} & { 2/ 5} & { 9/26} & { 2/ 5} & { 6/17} & { 3/ 8} & { 2/ 5} & { 6/17} & { 2/ 5} & { 1/ 3} & {14/37} & { 2/ 5} & {14/39} & { 2/ 5} & {13/38} & { 8/21} & { 2/ 5} & { 4/11} & { 2/ 5} & {15/43} & {18/47} & { 2/ 5} & {18/49} & { 2/ 5} & { 6/17} & { 5/13} & { 2/ 5} & {10/27} & { 2/ 5} & { 5/14} & {22/57} & { 2/ 5} & {22/59} & { 2/ 5} & {22/61} & {12/31} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 4/11} & {26/67} & { 2/ 5} & {26/69} & { 2/ 5} & {26/71} & { 7/18} & { 2/ 5} & {14/37} & { 2/ 5} & { 7/19} & {30/77} & { 2/ 5} & {30/79} & { 2/ 5} \\\hline
$13$ & {11/35} & { 7/18} & { 8/21} & {\color{red} 11/38} & { 7/18} & { 3/ 8} & {15/41} & { 5/13} & { 1/ 3} & { 7/18} & {11/29} & { 8/23} & {12/31} & { 3/ 8} & { 7/18} & {13/34} & { 1/ 3} & { 7/18} & {14/37} & { 7/18} & { 5/13} & { 3/ 8} & { 7/18} & { 8/21} & {22/59} & {17/44} & {17/45} & { 7/18} & {18/47} & { 3/ 8} & {19/49} & {19/50} & { 7/18} & { 5/13} & {20/53} & { 7/18} & {21/55} & { 7/18} & {22/57} & {11/29} & { 7/18} & {23/60} & {\color{red} 23/61} & {12/31} & { 8/21} & { 7/18} & { 5/13} & {25/66} & {26/67} & {13/34} & { 7/18} & {27/70} & {27/71} & { 7/18} & {28/73} & { 7/18} & {29/75} & {29/76} & { 7/18} & { 5/13} \\\hline
$14$ & {12/37} & { 7/19} & { 4/11} & { 4/13} & { 7/19} & { 9/25} & {10/29} & { 7/19} & { 5/14} & { 4/11} & {11/30} & {11/31} & { 7/19} & { 4/11} & { 4/11} & { 7/19} & {13/36} & { 1/ 3} & { 7/19} & { 4/11} & { 7/19} & {15/41} & { 5/14} & { 7/19} & { 4/11} & {16/45} & { 7/19} & {17/47} & {\color{red} 17/48} & {18/49} & { 9/25} & { 7/19} & {19/52} & {19/53} & { 7/19} & { 4/11} & { 4/11} & { 7/19} & {21/58} & { 7/19} & {11/30} & { 4/11} & { 7/19} & {23/63} & {23/64} & { 7/19} & { 4/11} & {24/67} & {25/68} & {25/69} & { 7/19} & {26/71} & {13/36} & { 7/19} & {27/74} & { 9/25} & { 7/19} & { 4/11} & { 7/19} & {29/79} \\\hline
$15$ & { 1/ 3} & { 2/ 5} & { 9/23} & { 1/ 3} & { 2/ 5} & { 9/26} & { 2/ 5} & {11/28} & {10/29} & { 2/ 5} & {18/49} & { 2/ 5} & {13/33} & { 7/20} & { 2/ 5} & { 7/18} & { 2/ 5} & {15/38} & { 1/ 3} & { 2/ 5} & {16/41} & { 2/ 5} & {17/43} & {11/31} & { 2/ 5} & { 9/23} & { 2/ 5} & {19/48} & {25/67} & { 2/ 5} & {20/51} & { 2/ 5} & {21/53} & { 7/18} & { 2/ 5} & {11/28} & { 2/ 5} & {23/58} & {23/59} & { 2/ 5} & {24/61} & { 2/ 5} & {25/63} & {25/64} & { 2/ 5} & {13/33} & { 2/ 5} & {27/68} & { 9/23} & { 2/ 5} & {28/71} & { 2/ 5} & {29/73} & {29/74} & { 2/ 5} & {15/38} & { 2/ 5} & {31/78} & {31/79} & { 2/ 5} \\\hline
$16$ & {13/41} & { 8/21} & { 3/ 8} & { 2/ 7} & { 8/21} & {10/27} & {16/47} & {11/29} & {17/49} & { 8/21} & { 3/ 8} & { 1/ 3} & { 8/21} & {13/35} & { 4/11} & {14/37} & { 7/19} & { 8/21} & { 3/ 8} & { 1/ 3} & { 8/21} & {16/43} & { 8/21} & {17/45} & {17/46} & { 8/21} & { 3/ 8} & { 6/17} & {19/50} & {19/51} & { 8/21} & {20/53} & {10/27} & { 8/21} & { 3/ 8} & { 7/19} & {11/29} & {22/59} & { 8/21} & {23/61} & {23/62} & { 8/21} & { 3/ 8} & { 8/21} & {25/66} & {25/67} & { 8/21} & {26/69} & {13/35} & {27/71} & { 3/ 8} & { 8/21} & {14/37} & {28/75} & { 8/21} & {29/77} & {\color{red} 29/78} & {30/79} & { 3/ 8} & { 8/21} \\\hline
$17$ & {14/43} & {10/27} & { 2/ 5} & {15/46} & { 2/ 5} & { 5/14} & { 3/ 8} & { 2/ 5} & {11/31} & { 2/ 5} & { 4/11} & {14/37} & { 2/ 5} & {13/36} & { 2/ 5} & { 4/11} & { 8/21} & { 2/ 5} & { 4/11} & { 2/ 5} & { 1/ 3} & {18/47} & { 2/ 5} & {18/49} & { 2/ 5} & {17/48} & { 5/13} & { 2/ 5} & {10/27} & { 2/ 5} & {19/53} & {22/57} & { 2/ 5} & {22/59} & { 2/ 5} & {21/58} & {12/31} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 4/11} & {26/67} & { 2/ 5} & {26/69} & { 2/ 5} & {26/71} & { 7/18} & { 2/ 5} & {14/37} & { 2/ 5} & { 7/19} & {30/77} & { 2/ 5} & {30/79} & { 2/ 5} & {10/27} & {16/41} & { 2/ 5} & { 8/21} & { 2/ 5} \\\hline
$18$ & { 1/ 3} & { 9/23} & { 5/13} & { 1/ 3} & { 9/23} & { 9/25} & {19/51} & {12/31} & {11/32} & { 9/23} & {13/34} & { 5/14} & { 7/18} & { 8/23} & { 9/23} & { 5/13} & { 8/23} & {16/41} & { 8/21} & { 9/23} & {17/44} & { 1/ 3} & { 9/23} & {18/47} & { 9/23} & {19/49} & {26/71} & { 9/23} & { 5/13} & {14/37} & { 7/18} & {21/55} & { 9/23} & {22/57} & {29/79} & {23/59} & {23/60} & { 9/23} & {12/31} & { 8/21} & {25/64} & { 5/13} & { 9/23} & {26/67} & {13/34} & { 9/23} & {27/70} & { 9/23} & { 7/18} & {28/73} & { 9/23} & {29/75} & {\color{red} 29/76} & {30/77} & { 5/13} & { 9/23} & {31/80} & {31/81} & {16/41} & {32/83} \\\hline
$19$ & {15/47} & { 3/ 8} & {10/27} & {10/31} & { 3/ 8} & {11/30} & { 6/17} & { 3/ 8} & { 4/11} & { 3/ 8} & {13/35} & {14/39} & { 3/ 8} & { 7/19} & {10/27} & { 3/ 8} & {15/41} & { 3/ 8} & {16/43} & {10/27} & { 3/ 8} & {17/46} & { 1/ 3} & { 3/ 8} & {10/27} & { 3/ 8} & {19/51} & {19/52} & { 3/ 8} & {10/27} & { 4/11} & { 3/ 8} & { 7/19} & { 3/ 8} & {22/59} & {11/30} & { 3/ 8} & {23/62} & {23/63} & { 3/ 8} & {24/65} & { 3/ 8} & {25/67} & {25/68} & { 3/ 8} & {13/35} & {10/27} & { 3/ 8} & {27/73} & { 3/ 8} & {28/75} & {10/27} & { 3/ 8} & {\color{red} 29/78} & {29/79} & { 3/ 8} & {10/27} & { 3/ 8} & {31/83} & {31/84} \\\hline
$20$ & {16/49} & { 2/ 5} & {11/28} & { 4/13} & { 2/ 5} & {11/31} & { 2/ 5} & {13/33} & { 6/17} & { 2/ 5} & { 9/25} & { 2/ 5} & {15/38} & {14/39} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {17/43} & { 9/25} & { 2/ 5} & { 9/23} & { 2/ 5} & {19/48} & { 1/ 3} & { 2/ 5} & {20/51} & { 2/ 5} & {21/53} & {\color{red} 19/54} & { 2/ 5} & {11/28} & { 2/ 5} & {23/58} & {15/41} & { 2/ 5} & {24/61} & { 2/ 5} & {25/63} & {11/29} & { 2/ 5} & {13/33} & { 2/ 5} & {27/68} & { 9/23} & { 2/ 5} & {28/71} & { 2/ 5} & {29/73} & {29/74} & { 2/ 5} & {15/38} & { 2/ 5} & {31/78} & {31/79} & { 2/ 5} & {32/81} & { 2/ 5} & {33/83} & {11/28} & { 2/ 5} \\\hline
$21$ & { 1/ 3} & { 5/13} & {11/29} & { 1/ 3} & { 5/13} & { 3/ 8} & {20/57} & {13/34} & {12/35} & { 5/13} & {14/37} & {13/38} & { 5/13} & { 3/ 8} & { 5/13} & { 8/21} & { 9/26} & { 5/13} & {17/45} & { 5/14} & {18/47} & { 3/ 8} & { 5/13} & {19/50} & { 1/ 3} & { 5/13} & {20/53} & { 5/13} & {21/55} & { 3/ 8} & { 5/13} & {11/29} & {30/83} & {23/60} & {23/61} & { 5/13} & { 8/21} & { 3/ 8} & { 5/13} & {25/66} & { 5/13} & {13/34} & {26/69} & { 5/13} & {27/71} & { 3/ 8} & {28/73} & {14/37} & { 5/13} & {29/76} & {29/77} & { 5/13} & {30/79} & { 5/13} & {31/81} & {31/82} & { 5/13} & { 8/21} & {32/85} & {33/86} \\\hline
$22$ & {17/53} & { 3/ 8} & { 2/ 5} & { 9/28} & { 2/ 5} & { 4/11} & {14/37} & { 2/ 5} & {13/36} & { 2/ 5} & { 7/19} & { 8/21} & { 2/ 5} & {15/41} & { 2/ 5} & {10/27} & {18/47} & { 2/ 5} & {17/46} & { 2/ 5} & {10/27} & { 5/13} & { 2/ 5} & {10/27} & { 2/ 5} & { 1/ 3} & {22/57} & { 2/ 5} & {22/59} & { 2/ 5} & {21/58} & {12/31} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {23/63} & {26/67} & { 2/ 5} & {26/69} & { 2/ 5} & {25/68} & { 7/18} & { 2/ 5} & {14/37} & { 2/ 5} & {\color{red} 27/73} & {30/77} & { 2/ 5} & {30/79} & { 2/ 5} & {10/27} & {16/41} & { 2/ 5} & { 8/21} & { 2/ 5} & {16/43} & {34/87} & { 2/ 5} & {34/89} & { 2/ 5} \\\hline
$23$ & {18/55} & {11/28} & {12/31} & { 9/29} & {11/28} & { 6/17} & {23/61} & { 7/18} & {13/37} & {11/28} & { 5/13} & { 4/11} & {16/41} & { 5/14} & {11/28} & {17/44} & {16/45} & { 9/23} & { 5/14} & {11/28} & {19/49} & { 5/14} & {20/51} & { 5/13} & {11/28} & { 7/18} & { 1/ 3} & {11/28} & {22/57} & {11/28} & {23/59} & {31/86} & {11/28} & {12/31} & {34/89} & {25/64} & { 5/13} & {11/28} & {26/67} & {35/94} & { 9/23} & {27/70} & {11/28} & { 7/18} & { 4/11} & {29/74} & {29/75} & {11/28} & {30/77} & { 5/13} & {31/79} & {31/80} & {11/28} & {16/41} & {32/83} & {11/28} & {33/85} & {\color{red} 34/89} & {34/87} & {17/44} \\\hline
$24$ & { 1/ 3} & {11/29} & { 3/ 8} & { 1/ 3} & {11/29} & {13/35} & {14/39} & {14/37} & {13/38} & {11/29} & { 3/ 8} & { 4/11} & {11/29} & {16/43} & { 3/ 8} & {17/45} & {18/49} & {11/29} & { 3/ 8} & { 3/ 8} & {11/29} & {19/51} & {29/79} & {20/53} & { 3/ 8} & {11/29} & { 3/ 8} & { 1/ 3} & {11/29} & { 3/ 8} & {11/29} & {23/61} & {23/62} & {11/29} & { 3/ 8} & { 6/17} & {25/66} & {25/67} & {11/29} & {26/69} & {13/35} & {11/29} & { 3/ 8} & { 7/19} & {14/37} & {28/75} & {11/29} & {29/77} & {29/78} & {11/29} & { 3/ 8} & { 3/ 8} & {31/82} & {31/83} & {11/29} & {32/85} & { 3/ 8} & {11/29} & {\color{red}  3/ 8} & {\color{red} 33/89} \\\hline
$25$ & {19/59} & { 2/ 5} & {13/33} & {\color{red} 19/62} & { 2/ 5} & {13/36} & { 2/ 5} & {15/38} & {14/39} & { 2/ 5} & {15/41} & { 2/ 5} & {17/43} & { 4/11} & { 2/ 5} & {11/30} & { 2/ 5} & {19/48} & {11/30} & { 2/ 5} & {30/79} & { 2/ 5} & {21/53} & {11/30} & { 2/ 5} & {11/28} & { 2/ 5} & {23/58} & { 1/ 3} & { 2/ 5} & {24/61} & { 2/ 5} & {25/63} & {23/64} & { 2/ 5} & {13/33} & { 2/ 5} & {27/68} & {\color{red} 25/69} & { 2/ 5} & {28/71} & { 2/ 5} & {29/73} & {19/51} & { 2/ 5} & {15/38} & { 2/ 5} & {31/78} & {23/60} & { 2/ 5} & {32/81} & { 2/ 5} & {33/83} & {11/28} & { 2/ 5} & {17/43} & { 2/ 5} & {35/88} & {35/89} & { 2/ 5} \\\hline
$26$ & {20/61} & {12/31} & {13/34} & { 6/19} & {12/31} & { 4/11} & {24/67} & { 5/13} & { 7/20} & {12/31} & { 8/21} & {15/43} & {17/44} & {11/31} & {12/31} & {18/47} & {17/48} & {12/31} & {19/50} & { 3/ 8} & { 5/13} & {11/31} & {12/31} & {21/55} & {\color{red} 11/31} & {22/57} & {11/29} & {12/31} & {23/60} & { 1/ 3} & {12/31} & { 8/21} & {12/31} & { 5/13} & { 7/19} & {12/31} & {13/34} & {18/49} & {27/70} & {27/71} & {12/31} & {28/73} & {23/64} & {29/75} & {29/76} & {12/31} & { 5/13} & {30/79} & {12/31} & {31/81} & {14/37} & {32/83} & { 8/21} & {12/31} & {33/86} & {11/29} & {17/44} & {34/89} & {12/31} & { 5/13} \\\hline
$27$ & { 1/ 3} & {14/37} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 7/19} & { 8/21} & { 2/ 5} & {25/71} & { 2/ 5} & {16/43} & {18/47} & { 2/ 5} & {17/46} & { 2/ 5} & { 3/ 8} & { 5/13} & { 2/ 5} & {19/51} & { 2/ 5} & { 3/ 8} & {22/57} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 3/ 8} & {12/31} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 1/ 3} & {26/67} & { 2/ 5} & {26/69} & { 2/ 5} & {25/68} & { 7/18} & { 2/ 5} & {14/37} & { 2/ 5} & {27/73} & {30/77} & { 2/ 5} & {30/79} & { 2/ 5} & {\color{red} 29/78} & {16/41} & { 2/ 5} & { 8/21} & { 2/ 5} & {\color{red} 31/83} & {34/87} & { 2/ 5} & {34/89} & { 2/ 5} & { 3/ 8} & { 9/23} & { 2/ 5} & {18/47} & { 2/ 5} \\\hline
$28$ & {21/65} & {13/33} & { 7/18} & { 3/10} & {13/33} & {14/39} & {27/71} & {16/41} & { 5/14} & {13/33} & {28/75} & { 7/19} & { 9/23} & {17/47} & {13/33} & {19/49} & { 9/25} & {20/51} & { 4/11} & {13/33} & { 7/18} & { 4/11} & {11/28} & { 4/11} & {13/33} & {23/59} & { 4/11} & {24/61} & {12/31} & {13/33} & {25/64} & { 1/ 3} & {13/33} & {26/67} & {13/33} & { 9/23} & {\color{red}  5/14} & {13/33} & { 7/18} & {\color{red}  7/19} & {29/74} & {20/53} & {13/33} & {30/77} & {35/93} & {31/79} & {31/80} & {13/33} & {16/41} & { 7/19} & {11/28} & {33/85} & {13/33} & {34/87} & {27/73} & {35/89} & { 7/18} & {13/33} & { 9/23} & {12/31} \\\hline
$29$ & {22/67} & {13/34} & {14/37} & {23/70} & {13/34} & { 3/ 8} & { 4/11} & { 8/21} & {15/43} & {13/34} & {17/45} & {18/49} & {13/34} & { 3/ 8} & {14/37} & {19/50} & {10/27} & {13/34} & {20/53} & {14/37} & {21/55} & { 3/ 8} & {13/34} & {11/29} & {14/37} & {13/34} & {23/61} & {17/47} & { 8/21} & {14/37} & {13/34} & {25/66} & { 1/ 3} & {13/34} & {14/37} & {13/34} & {27/71} & { 3/ 8} & {13/34} & {14/37} & {14/39} & {29/76} & {29/77} & {13/34} & {30/79} & { 3/ 8} & {13/34} & {31/82} & {\color{red} 37/99} & { 8/21} & {32/85} & {13/34} & {11/29} & { 3/ 8} & {34/89} & {17/45} & {13/34} & {35/92} & {\color{red} 35/93} & {13/34} \\\hline
$30$ & { 1/ 3} & { 2/ 5} & {15/38} & { 1/ 3} & { 2/ 5} & {15/41} & { 2/ 5} & {17/43} & { 4/11} & { 2/ 5} & {17/46} & { 2/ 5} & {19/48} & {18/49} & { 2/ 5} & {13/35} & { 2/ 5} & {21/53} & {10/27} & { 2/ 5} & {\color{red} 13/35} & { 2/ 5} & {23/58} & {13/35} & { 2/ 5} & {18/47} & { 2/ 5} & {25/63} & {13/35} & { 2/ 5} & {13/33} & { 2/ 5} & {27/68} & { 1/ 3} & { 2/ 5} & {28/71} & { 2/ 5} & {29/73} & {27/74} & { 2/ 5} & {15/38} & { 2/ 5} & {31/78} & {29/79} & { 2/ 5} & {32/81} & { 2/ 5} & {33/83} & {\color{red} 31/84} & { 2/ 5} & {17/43} & { 2/ 5} & {35/88} & {23/61} & { 2/ 5} & {36/91} & { 2/ 5} & {37/93} & {27/70} & { 2/ 5} \\\hline
$31$ & {23/71} & { 7/18} & { 5/13} & {14/43} & { 7/18} & {\color{red}  5/14} & { 4/11} & {17/44} & {16/45} & { 7/18} & {18/47} & {17/48} & {19/49} & { 9/25} & { 7/18} & { 5/13} & {19/53} & { 7/18} & {33/89} & { 7/18} & {22/57} & {13/36} & { 7/18} & {23/60} & { 7/19} & {12/31} & {\color{red} 13/36} & { 7/18} & { 5/13} & {13/36} & {26/67} & {13/34} & { 7/18} & {27/70} & { 1/ 3} & { 7/18} & {28/73} & { 7/18} & {29/75} & { 4/11} & { 7/18} & { 5/13} & {29/78} & {31/80} & {31/81} & { 7/18} & {32/83} & {\color{red} 34/95} & {33/85} & {33/86} & { 7/18} & {17/44} & {\color{red} 33/89} & { 7/18} & { 5/13} & { 7/18} & {12/31} & {18/47} & { 7/18} & {37/96} \\\hline
$32$ & {24/73} & { 8/21} & { 2/ 5} & { 6/19} & { 2/ 5} & {16/43} & {18/47} & { 2/ 5} & { 8/23} & { 2/ 5} & { 3/ 8} & { 5/13} & { 2/ 5} & {19/51} & { 2/ 5} & {20/53} & {22/57} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {14/37} & {12/31} & { 2/ 5} & {23/61} & { 2/ 5} & {14/37} & {26/67} & { 2/ 5} & {14/37} & { 2/ 5} & {31/84} & { 7/18} & { 2/ 5} & {14/37} & { 2/ 5} & { 1/ 3} & {30/77} & { 2/ 5} & {30/79} & { 2/ 5} & {29/78} & {16/41} & { 2/ 5} & { 8/21} & { 2/ 5} & {31/83} & {34/87} & { 2/ 5} & {34/89} & { 2/ 5} & { 3/ 8} & { 9/23} & { 2/ 5} & {18/47} & { 2/ 5} & {\color{red} 35/93} & {38/97} & { 2/ 5} & {38/99} & { 2/ 5} \\\hline
$33$ & { 1/ 3} & {15/38} & {16/41} & { 1/ 3} & {15/38} & { 4/11} & {31/81} & { 9/23} & {17/47} & {15/38} & {18/49} & {16/43} & {20/51} & {19/52} & {15/38} & { 7/18} & { 4/11} & {11/28} & { 7/19} & {15/38} & {23/59} & {11/30} & {24/61} & { 7/19} & {15/38} & {25/64} & { 7/19} & {13/33} & {31/84} & {15/38} & { 9/23} & { 7/19} & {28/71} & { 7/18} & {15/38} & {29/74} & { 1/ 3} & {15/38} & {30/77} & {\color{red} 31/81} & {31/79} & {\color{red} 29/80} & {15/38} & {16/41} & {\color{red} 16/43} & {11/28} & {29/78} & {15/38} & {34/87} & {36/95} & {35/89} & { 7/18} & {15/38} & { 9/23} & {16/43} & {37/94} & {37/95} & {15/38} & {38/97} & {\color{red} 18/49} \\\hline
$34$ & {25/77} & { 5/13} & { 8/21} & {13/40} & { 5/13} & {15/41} & {18/49} & {18/47} & {17/48} & { 5/13} & {19/50} & {10/27} & { 5/13} & {\color{red} 19/53} & { 5/13} & {21/55} & {22/59} & { 5/13} & {11/29} & { 8/21} & {23/60} & { 3/ 8} & { 5/13} & { 8/21} & { 8/21} & { 5/13} & {25/66} & { 5/13} & {13/34} & { 8/21} & { 5/13} & {27/71} & {\color{red} 14/39} & {28/73} & { 8/21} & { 5/13} & {\color{red} 29/76} & { 1/ 3} & { 5/13} & { 8/21} & { 5/13} & {\color{red} 31/81} & {\color{red} 15/41} & { 5/13} & { 8/21} & {\color{red}  4/11} & {33/86} & {11/29} & { 5/13} & {34/89} & {34/93} & { 5/13} & {35/92} & { 5/13} & {18/47} & {36/95} & { 5/13} & {37/97} & {35/93} & {38/99} \\\hline
$35$ & {26/79} & { 2/ 5} & {17/43} & {13/41} & { 2/ 5} & {17/46} & { 2/ 5} & {19/48} & {\color{red} 17/49} & { 2/ 5} & {19/51} & { 2/ 5} & {21/53} & {10/27} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {23/58} & {22/59} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {25/63} & { 3/ 8} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {27/68} & { 3/ 8} & { 2/ 5} & {37/96} & { 2/ 5} & {29/73} & { 3/ 8} & { 2/ 5} & {15/38} & { 2/ 5} & {31/78} & {\color{red} 32/97} & { 2/ 5} & {32/81} & { 2/ 5} & {33/83} & {31/84} & { 2/ 5} & {17/43} & { 2/ 5} & {35/88} & {33/89} & { 2/ 5} & {36/91} & { 2/ 5} & {37/93} & {\color{red} 35/94} & { 2/ 5} & {19/48} & { 2/ 5} & {39/98} & {\color{red} 37/99} & { 2/ 5} \\\hline
$36$ & { 1/ 3} & {16/41} & {17/44} & { 1/ 3} & {16/41} & {17/47} & {32/87} & {19/49} & { 9/25} & {16/41} & { 5/13} & { 5/14} & { 7/18} & { 4/11} & {16/41} & {22/57} & {21/58} & {23/59} & {15/41} & {16/41} & {12/31} & {23/63} & {16/41} & { 5/13} & { 8/21} & {26/67} & {15/41} & {16/41} & {27/70} & {\color{red} 15/41} & { 7/18} & { 4/11} & {16/41} & {29/75} & {15/41} & {30/77} & { 5/13} & {16/41} & {31/80} & { 1/ 3} & {16/41} & {32/83} & {\color{red}  8/21} & {33/85} & {\color{red} 31/86} & {16/41} & {17/44} & {\color{red}  4/11} & { 7/18} & { 5/13} & {16/41} & {12/31} & {\color{red} 17/47} & {37/95} & {37/96} & {16/41} & {19/49} & {\color{red}  4/11} & {23/59} & {22/57} \\\hline
$37$ & {27/83} & {18/47} & { 2/ 5} & {\color{red} 27/86} & { 2/ 5} & { 3/ 8} & { 5/13} & { 2/ 5} & { 6/17} & { 2/ 5} & {20/53} & {22/57} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {11/29} & {12/31} & { 2/ 5} & {23/61} & { 2/ 5} & { 8/21} & {26/67} & { 2/ 5} & {25/66} & { 2/ 5} & { 8/21} & { 7/18} & { 2/ 5} & {\color{red} 27/71} & { 2/ 5} & { 8/21} & {30/77} & { 2/ 5} & { 8/21} & { 2/ 5} & {35/96} & {16/41} & { 2/ 5} & { 8/21} & { 2/ 5} & { 1/ 3} & {34/87} & { 2/ 5} & {34/89} & { 2/ 5} & { 3/ 8} & { 9/23} & { 2/ 5} & {18/47} & { 2/ 5} & {35/93} & {38/97} & { 2/ 5} & {38/99} & { 2/ 5} & {37/98} & {20/51} & { 2/ 5} & { 5/13} & { 2/ 5} \\\hline
$38$ & {28/85} & {17/43} & { 9/23} & {\color{red}  8/25} & {17/43} & {18/49} & { 5/13} & {20/51} & {11/31} & {17/43} & {10/27} & { 3/ 8} & {11/28} & { 7/19} & {17/43} & {19/50} & {\color{red} 11/30} & {24/61} & {23/62} & {17/43} & {25/64} & {24/65} & {13/33} & {16/43} & {17/43} & { 9/23} & {13/35} & {28/71} & {16/43} & {17/43} & {29/74} & {16/43} & {15/38} & {22/59} & {17/43} & {31/79} & {16/43} & {32/81} & {16/41} & {17/43} & {11/28} & { 1/ 3} & {17/43} & {34/87} & {\color{red}  5/13} & {35/89} & {11/30} & {17/43} & { 9/23} & {\color{red}  3/ 8} & {37/94} & {\color{red}  7/19} & {17/43} & {38/97} & {37/97} & {13/33} & {\color{red} 19/50} & {17/43} & {20/51} & { 3/ 8} \\\hline
$39$ & { 1/ 3} & {17/44} & {18/47} & { 1/ 3} & {17/44} & {\color{red}  9/25} & {10/27} & { 5/13} & {19/53} & {17/44} & {21/55} & {22/59} & {22/57} & {21/58} & {17/44} & {23/60} & { 3/ 8} & {17/44} & { 8/21} & {18/47} & { 5/13} & {26/69} & {17/44} & {13/34} & {18/47} & {27/70} & {14/37} & {17/44} & {28/73} & {18/47} & {17/44} & {\color{red} 29/76} & {31/82} & { 5/13} && {17/44} & {\color{red} 31/81} & { 4/11} & {32/83} & {18/47} & {17/44} & {\color{red} 33/86} & {\color{red}  1/99} & {17/44} & {18/47} & {\color{red} 31/82} & {\color{red}  5/13} & {\color{red} 33/91} & {17/44} & {18/47} & {\color{red} 18/49} & {37/96} & {37/97} & {17/44} & {38/99} & {\color{red} 31/84} & {22/57} & {13/34} & {17/44} & { 5/13} \\\hline
$40$ & {29/89} & { 2/ 5} & {19/48} & {\color{red}  4/13} & { 2/ 5} & {19/51} & { 2/ 5} & {21/53} & {19/54} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {23/58} & {22/59} & { 2/ 5} & {23/61} & { 2/ 5} & {25/63} & { 3/ 8} & { 2/ 5} & {17/45} & { 2/ 5} & {27/68} & {26/69} & { 2/ 5} & {17/45} & { 2/ 5} & {29/73} & {17/45} & { 2/ 5} & {31/82} & { 2/ 5} & {31/78} & {17/45} & { 2/ 5} & {12/31} & { 2/ 5} & {33/83} & {\color{red} 30/83} & { 2/ 5} & {17/43} & { 2/ 5} & {35/88} & {\color{red}  1/99} & { 2/ 5} & {36/91} & { 2/ 5} & {37/93} & {35/94} & { 2/ 5} & {19/48} & { 2/ 5} & {39/98} & {37/99} & { 2/ 5} & {21/53} & { 2/ 5} & {39/98} & { 3/ 8} & { 2/ 5} \\\hline
$41$ & {30/91} & { 9/23} & {19/49} & {31/94} & { 9/23} & {19/52} & {36/97} & { 7/18} & { 4/11} & { 9/23} & {35/93} & {22/61} & {23/59} & {11/30} & { 9/23} & {12/31} & {23/63} & {25/64} & {24/65} & { 9/23} & {26/67} & {25/68} & { 9/23} & {17/46} & { 9/23} & { 7/18} & {17/46} & { 9/23} & {29/75} & { 3/ 8} & {30/77} & {\color{red} 17/46} & { 9/23} & {31/80} & {17/46} & {16/41} & {18/49} & { 9/23} & {33/85} & {17/46} & {34/87} & {17/44} & { 9/23} & { 7/18} & {\color{red}  1/99} & { 9/23} & {12/31} & { 9/23} & {37/95} & {\color{red} 35/96} & { 9/23} & {19/49} & {\color{red}  3/ 8} & {23/59} & {\color{red} 35/93} & { 9/23} & {33/85} & {\color{red} 19/52} & {25/64} & {29/75} \\\hline
$42$ & { 1/ 3} & { 5/13} & { 2/ 5} & { 1/ 3} & { 2/ 5} & {18/49} & {22/57} & { 2/ 5} & { 5/14} & { 2/ 5} & {11/29} & {12/31} & { 2/ 5} & {\color{red} 22/61} & { 2/ 5} & { 8/21} & {26/67} & { 2/ 5} & {25/66} & { 2/ 5} & {13/34} & { 7/18} & { 2/ 5} & {27/71} & { 2/ 5} & {18/47} & {30/77} & { 2/ 5} & {29/76} & { 2/ 5} & {18/47} & {16/41} & { 2/ 5} & {\color{red} 31/81} & { 2/ 5} & {18/47} & {34/87} & { 2/ 5} & {18/47} & { 2/ 5} & {\color{red} 17/47} & { 9/23} & { 2/ 5} & {18/47} & { 2/ 5} & {\color{red}  1/99} & {38/97} & { 2/ 5} & {38/99} & { 2/ 5} & {\color{red} 18/49} & {20/51} & { 2/ 5} & { 5/13} & { 2/ 5} & {25/66} & {31/79} & { 2/ 5} & {37/96} & { 2/ 5} \\\hline
$43$ & {31/95} & {19/48} & {20/51} & {18/55} & {19/48} & {10/27} & {22/57} & {11/28} & {20/57} & {19/48} & {22/59} & {20/53} & {24/61} & {23/62} & {19/48} & { 3/ 8} & {24/65} & {13/33} & {25/67} & {19/48} & { 9/23} & {13/35} & {28/71} & { 3/ 8} & {19/48} & {29/74} & {28/75} & {15/38} & { 3/ 8} & {19/48} & {31/79} & { 3/ 8} & {32/81} & { 3/ 8} & {19/48} & {11/28} & { 3/ 8} & {17/43} & {35/93} & {19/48} & {35/89} & { 3/ 8} & {36/91} & { 9/23} & {19/48} & {37/94} & {\color{red}  1/99} & {19/48} & {38/97} & {\color{red} 22/57} & {13/33} & {27/73} & {19/48} & {20/51} & {\color{red} 20/53} & {28/71} & {\color{red} 13/35} & {19/48} & {31/79} & {\color{red} 10/27} \\\hline
$44$ & {32/97} & {19/49} & { 5/13} & { 8/25} & {19/49} & { 4/11} & {22/59} & {22/57} & {21/58} & {19/49} & {23/60} & { 3/ 8} & {12/31} & {23/63} & {19/49} & { 5/13} & {26/69} & {19/49} & {18/49} & { 5/13} & {27/70} & {14/37} & {19/49} & {28/73} & { 5/13} & {29/75} & {30/79} & {19/49} & { 5/13} & { 5/13} & {31/80} & { 8/21} & {19/49} & {32/83} & { 5/13} & {19/49} & {\color{red} 33/86} & {\color{red} 18/49} & {17/44} & { 5/13} & {19/49} & {\color{red}  5/13} & {18/49} & {12/31} & { 5/13} & {19/49} & {\color{red} 37/96} & {\color{red}  1/99} & {19/49} & { 5/13} & {\color{red} 11/29} & {\color{red} 22/57} & {\color{red} 33/91} & {19/49} & { 5/13} & {\color{red} 10/27} & {29/75} & {23/60} & {19/49} & {37/96} \\\hline
$45$ & { 1/ 3} & { 2/ 5} & {21/53} & { 1/ 3} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {23/58} & {21/59} & { 2/ 5} & {23/61} & { 2/ 5} & {25/63} & { 3/ 8} & { 2/ 5} & {25/66} & { 2/ 5} & {27/68} & {26/69} & { 2/ 5} & {19/50} & { 2/ 5} & {29/73} & {14/37} & { 2/ 5} & {19/50} & { 2/ 5} & {31/78} & {30/79} & { 2/ 5} & {19/50} & { 2/ 5} & {33/83} & {19/50} & { 2/ 5} & {35/92} & { 2/ 5} & {35/88} & {19/50} & { 2/ 5} & {\color{red}  5/13} & { 2/ 5} & {37/93} & {\color{red}  9/25} & { 2/ 5} & {19/48} & { 2/ 5} & {39/98} & {\color{red}  1/99} & { 2/ 5} & {21/53} & { 2/ 5} & {39/98} & { 3/ 8} & { 2/ 5} & {21/53} & { 2/ 5} & {39/98} & {35/93} & { 2/ 5} \\\hline
$46$ & {17/52} & {20/51} & { 7/18} & {\color{red}  8/25} & {20/51} & { 7/19} & {37/99} & {23/59} & {\color{red}  7/20} & {20/51} & {\color{red} 23/62} & { 4/11} & {25/64} & {24/65} & {20/51} & {26/67} & {25/68} & { 9/23} & {13/35} & {20/51} & { 7/18} & {27/73} & {29/74} & {19/51} & {\color{red} 37/97} & {30/77} & {\color{red} 29/78} & {20/51} & {\color{red}  3/ 8} & {\color{red} 37/99} & {16/41} & {19/51} & {20/51} & {33/85} & {\color{red} 16/43} & {34/87} & {\color{red} 19/51} & {20/51} & { 7/18} & {19/51} & { 9/23} & {10/27} & {20/51} & {37/95} & {19/51} & {38/97} & {19/49} & {20/51} & {23/59} & {\color{red}  1/99} & {20/51} & {33/85} & {\color{red}  5/13} & {25/64} & {32/87} & {\color{red} 29/74} & { 7/18} & {\color{red} 10/27} & {34/87} & {\color{red} 24/65} \\\hline
$47$ & {32/97} & {22/57} & { 2/ 5} & {\color{red} 18/59} & { 2/ 5} & {\color{red} 21/58} & {12/31} & { 2/ 5} & {22/61} & { 2/ 5} & { 8/21} & {26/67} & { 2/ 5} & { 4/11} & { 2/ 5} & {13/34} & { 7/18} & { 2/ 5} & {27/71} & { 2/ 5} & {28/73} & {30/77} & { 2/ 5} & {29/76} & { 2/ 5} & { 5/13} & {16/41} & { 2/ 5} & {31/81} & { 2/ 5} & { 5/13} & {34/87} & { 2/ 5} & {33/86} & { 2/ 5} & { 5/13} & { 9/23} & { 2/ 5} & { 5/13} & { 2/ 5} & { 5/13} & {38/97} & { 2/ 5} & { 5/13} & { 2/ 5} & {19/52} & {20/51} & { 2/ 5} & { 5/13} & { 2/ 5} & {\color{red}  1/99} & {31/79} & { 2/ 5} & {37/96} & { 2/ 5} & {\color{red} 13/36} & {11/28} & { 2/ 5} & {22/57} & { 2/ 5} \\\hline
$48$ & { 1/ 3} & {21/53} & {11/28} & { 1/ 3} & {21/53} & {22/59} & {31/80} & {24/61} & {11/31} & {21/53} & { 3/ 8} & {11/29} & {13/33} & {25/67} & {21/53} & {26/69} & {29/78} & {28/71} & { 3/ 8} & {21/53} & {38/99} & {28/75} & {15/38} & {29/77} & {21/53} & {31/79} & { 3/ 8} & {32/81} & {20/53} & {21/53} & {11/28} & {32/85} & {17/43} & {20/53} & {21/53} & {35/89} & {20/53} & {36/91} & {\color{red} 19/53} & {21/53} & {37/94} & {20/53} & {19/48} & {\color{red} 36/97} & {21/53} & {13/33} & {\color{red} 19/53} & {21/53} & {20/51} & {21/53} & {28/71} & {\color{red}  1/99} & {21/53} & {31/79} & {\color{red} 31/80} & {28/71} & {22/59} & {\color{red} 21/53} & {11/28} & {\color{red} 11/29} \\\hline
$49$ & {18/55} & { 7/18} & {22/57} & {\color{red}  7/22} & { 7/18} & {11/30} & { 3/ 8} & {12/31} & {31/87} & { 7/18} & { 5/13} & {26/69} & {26/67} & {25/68} & { 7/18} & {27/70} & {14/37} & { 7/18} & {\color{red} 27/73} & { 7/18} & {29/75} & {30/79} & { 7/18} & { 5/13} & {22/57} & {31/80} & { 8/21} & { 7/18} & {32/83} & {22/57} & {33/85} & {34/89} & { 7/18} & {17/44} & {22/57} & { 7/18} & { 5/13} & { 7/18} & {12/31} & {22/57} & { 7/18} & {\color{red} 37/96} & {\color{red} 10/27} & {19/49} & {22/57} & { 7/18} & {\color{red} 22/57} & {10/27} & {33/85} & {22/57} & { 7/18} & {\color{red} 29/75} & {\color{red}  1/99} & { 7/18} & {22/57} & { 7/18} & {\color{red} 31/80} & {\color{red} 26/71} & { 7/18} & {22/57} \\\hline
$50$ & {32/97} & { 2/ 5} & {23/58} & {\color{red} 10/31} & { 2/ 5} & { 7/19} & { 2/ 5} & {25/63} & {23/64} & { 2/ 5} & {25/66} & { 2/ 5} & {27/68} & {\color{red} 25/69} & { 2/ 5} & {27/71} & { 2/ 5} & {29/73} & {14/37} & { 2/ 5} & {29/76} & { 2/ 5} & {31/78} & {30/79} & { 2/ 5} & {21/55} & { 2/ 5} & {33/83} & { 8/21} & { 2/ 5} & {21/55} & { 2/ 5} & {35/88} & {21/55} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {37/93} & {21/55} & { 2/ 5} & {\color{red} 35/93} & { 2/ 5} & {39/98} & {21/55} & { 2/ 5} & {\color{red} 22/57} & { 2/ 5} & {39/98} & {\color{red}  4/11} & { 2/ 5} & {21/53} & { 2/ 5} & {39/98} & {\color{red}  1/99} & { 2/ 5} & {23/58} & { 2/ 5} & {39/98} & {\color{red}  7/19} & { 2/ 5} \\\hline
$51$ & { 1/ 3} & {11/28} & {23/59} & { 1/ 3} & {11/28} & {23/62} & {35/93} & {25/64} & {23/65} & {11/28} & {25/67} & {26/71} & { 9/23} & {13/35} & {11/28} & { 7/18} & { 7/19} & {29/74} & {28/75} & {11/28} & {30/77} & {\color{red} 29/78} & {31/79} & { 3/ 8} & {11/28} & {16/41} & {\color{red} 31/83} & {11/28} & { 3/ 8} & {11/28} & {34/87} & { 3/ 8} & {11/28} & { 7/18} & {\color{red} 35/93} & { 9/23} & { 3/ 8} & {11/28} & {37/95} & { 3/ 8} & {38/97} & { 3/ 8} & {11/28} & {23/59} & { 3/ 8} & {20/51} & {22/59} & {11/28} & {25/64} & { 3/ 8} & {31/79} & { 7/18} & {11/28} & {34/87} & {\color{red}  1/99} & {11/28} & {37/95} & {11/28} & { 9/23} & {33/89} \\\hline
$52$ & {19/58} & {12/31} & { 2/ 5} & {\color{red}  5/16} & { 2/ 5} & {23/63} & {26/67} & { 2/ 5} & { 4/11} & { 2/ 5} & {13/34} & { 7/18} & { 2/ 5} & {26/71} & { 2/ 5} & {28/73} & {30/77} & { 2/ 5} & {37/99} & { 2/ 5} & { 5/13} & {16/41} & { 2/ 5} & {31/81} & { 2/ 5} & {32/83} & {34/87} & { 2/ 5} & {33/86} & { 2/ 5} & {22/57} & { 9/23} & { 2/ 5} & { 5/13} & { 2/ 5} & {22/57} & {38/97} & { 2/ 5} & {37/96} & { 2/ 5} & {22/57} & {20/51} & { 2/ 5} & {22/57} & { 2/ 5} & {\color{red} 35/94} & {31/79} & { 2/ 5} & {22/57} & { 2/ 5} & { 7/19} & {11/28} & { 2/ 5} & {22/57} & { 2/ 5} & {\color{red}  1/99} & {35/89} & { 2/ 5} & {\color{red}  9/29} & { 2/ 5} \\\hline
$53$ & {32/97} & {23/58} & {24/61} & {\color{red} 21/65} & {23/58} & { 3/ 8} & {33/85} & {13/33} & {24/67} & {23/58} & {26/69} & { 8/21} & {28/71} & { 3/ 8} & {23/58} & {14/37} & {37/99} & {15/38} & {29/77} & {23/58} & {\color{red} 11/29} & { 3/ 8} & {32/81} & {31/82} & {23/58} & {11/28} & {32/85} & {17/43} & {11/29} & {23/58} & {35/89} & {17/45} & {36/91} & {11/29} & {23/58} & {37/94} & {36/95} & {19/48} & {11/29} & {23/58} & {13/33} & {11/29} & {21/53} & {\color{red} 21/58} & {23/58} & {28/71} & {11/29} & {21/53} & {\color{red} 37/99} & {23/58} & {28/71} & {\color{red} 21/58} & {23/58} & {11/28} & {23/58} & {15/38} & {\color{red}  1/99} & {23/58} & {35/89} & {\color{red} 33/85} \\\hline
$54$ & { 1/ 3} & {\color{red} 19/50} & {12/31} & { 1/ 3} & {23/59} & {24/65} & {26/69} & {26/67} & { 6/17} & {23/59} & {\color{red} 13/35} & {14/37} & { 7/18} & {27/73} & {23/59} & {29/75} & {30/79} & {30/77} & {\color{red} 29/78} & {23/59} & {31/80} & { 8/21} & {23/59} & {\color{red} 22/59} & {12/31} & {33/85} & {34/89} & {23/59} & {17/44} & {12/31} & { 7/18} & {18/47} & {23/59} & {12/31} & {12/31} & {37/95} & {38/99} & {23/59} & {19/49} & {12/31} & {23/59} & {\color{red} 22/57} & {\color{red} 22/59} & {33/85} & {12/31} & {23/59} & {\color{red} 29/75} & {22/59} & { 7/18} & {\color{red} 29/75} & {23/59} & {\color{red} 31/80} & {22/59} & {37/95} & {12/31} & {23/59} & {\color{red} 26/67} & {\color{red}  1/99} & {23/59} & {12/31} \\\hline
$55$ & {20/61} & { 2/ 5} & {25/63} & {22/67} & { 2/ 5} & {\color{red}  4/11} & { 2/ 5} & {27/68} & {25/69} & { 2/ 5} & {27/71} & { 2/ 5} & {29/73} & {27/74} & { 2/ 5} & {29/76} & { 2/ 5} & {31/78} & {30/79} & { 2/ 5} & {31/81} & { 2/ 5} & {33/83} & { 8/21} & { 2/ 5} & {23/60} & { 2/ 5} & {35/88} & {34/89} & { 2/ 5} & {23/60} & { 2/ 5} & {37/93} & {18/47} & { 2/ 5} & {23/60} & { 2/ 5} & {39/98} & {23/60} & { 2/ 5} & {20/53} & { 2/ 5} & {39/98} & {23/60} & { 2/ 5} & {\color{red} 14/37} & { 2/ 5} & {39/98} & {23/60} & { 2/ 5} & {\color{red} 31/80} & { 2/ 5} & {39/98} & {11/30} & { 2/ 5} & {23/58} & { 2/ 5} & {39/98} & {\color{red}  1/99} & { 2/ 5} \\\hline
$56$ & {32/97} & {\color{red} 18/47} & {25/64} & {\color{red}  1/99} & {24/61} & {25/67} & {31/82} & { 9/23} & { 5/14} & {24/61} & { 3/ 8} & { 7/19} & {29/74} & {28/75} & {24/61} & {\color{red} 29/77} & {10/27} & {31/79} & { 3/ 8} & {\color{red} 35/89} & {16/41} & {\color{red} 31/83} & {11/28} & {32/85} & {24/61} & {34/87} & {\color{red}  3/ 8} & {35/89} & {23/61} & {\color{red}  5/13} & { 9/23} & {\color{red} 35/93} & {24/61} & {\color{red} 23/61} & {\color{red} 31/82} & {38/97} & {\color{red} 23/61} & {24/61} & {23/59} & {\color{red} 35/93} & {20/51} & {\color{red} 23/61} & {24/61} & {25/64} & {23/61} & {31/79} & { 3/ 8} & {24/61} & {34/87} & {23/61} & {11/28} & {\color{red} 29/78} & {24/61} & { 9/23} & {\color{red}  9/29} & {35/89} & {23/59} & {24/61} & {38/97} & {\color{red}  1/99} \\\hline
$57$ & { 1/ 3} & {26/67} & { 2/ 5} & { 1/ 3} & { 2/ 5} & {25/68} & { 7/18} & { 2/ 5} & {\color{red} 25/71} & { 2/ 5} & {28/73} & {30/77} & { 2/ 5} & { 7/19} & { 2/ 5} & { 5/13} & {16/41} & { 2/ 5} & {10/27} & { 2/ 5} & {32/83} & {34/87} & { 2/ 5} & {33/86} & { 2/ 5} & {17/44} & { 9/23} & { 2/ 5} & { 5/13} & { 2/ 5} & {12/31} & {38/97} & { 2/ 5} & {37/96} & { 2/ 5} & {12/31} & {20/51} & { 2/ 5} & {22/57} & { 2/ 5} & {12/31} & {31/79} & { 2/ 5} & {29/75} & { 2/ 5} & {12/31} & {11/28} & { 2/ 5} & {12/31} & { 2/ 5} & {\color{red} 28/75} & {35/89} & { 2/ 5} & {12/31} & { 2/ 5} & {23/62} & {24/61} & { 2/ 5} & {12/31} & { 2/ 5} \\\hline
$58$ & {\color{red} 10/31} & {\color{red} 33/85} & {13/33} & {\color{red} 32/99} & {25/63} & {24/65} & {37/95} & {28/71} & {13/36} & {25/63} & {14/37} & {13/34} & {15/38} & {\color{red}  4/11} & {25/63} & {30/79} & {\color{red} 25/68} & {32/81} & {31/82} & {25/63} & { 8/21} & {27/73} & {17/43} & {11/29} & {25/63} & {\color{red} 34/89} & {17/45} & {36/91} & {35/92} & {25/63} & {37/94} & {36/95} & {19/48} & { 8/21} & {25/63} & {13/33} & {19/50} & {21/53} & { 8/21} & {25/63} & {28/71} & { 8/21} & {21/53} & { 8/21} & {25/63} & {28/71} & { 8/21} & {23/58} & {\color{red} 34/93} & {25/63} & {15/38} & { 8/21} & {23/58} & {\color{red} 35/93} & {25/63} & {32/81} & {\color{red} 23/63} & {25/63} & {24/61} & {25/63} \\\hline
$59$ & {\color{red} 21/65} & {\color{red}  8/21} & {26/67} & {\color{red}  1/99} & {25/64} & {13/35} & {14/37} & { 7/18} & {26/73} & {25/64} & {\color{red} 28/75} & {30/79} & {30/77} & {29/78} & {25/64} & {31/80} & { 8/21} & {16/41} & {31/83} & {25/64} & {33/85} & {34/89} & {25/64} & { 3/ 8} & {\color{red} 31/80} & { 7/18} & {18/47} & {25/64} & {12/31} & {26/67} & {37/95} & {38/99} & {25/64} & {19/49} & {26/67} & {23/59} & { 5/13} & {25/64} & {33/85} & {26/67} & {25/64} & {37/96} & {25/64} & { 7/18} & {26/67} & {25/64} & {\color{red} 31/80} & {\color{red}  3/ 8} & {37/95} & {\color{red} 31/80} & {25/64} & {\color{red} 26/67} & { 3/ 8} & {23/59} & {\color{red} 31/80} & {25/64} & {\color{red} 33/85} & { 3/ 8} & {16/41} & {26/67} \\\hline
$60$ & { 1/ 3} & { 2/ 5} & {27/68} & { 1/ 3} & { 2/ 5} & {26/71} & { 2/ 5} & {29/73} & {34/95} & { 2/ 5} & {29/76} & { 2/ 5} & {31/78} & {29/79} & { 2/ 5} & {31/81} & { 2/ 5} & {33/83} & { 8/21} & { 2/ 5} & {33/86} & { 2/ 5} & {35/88} & {34/89} & { 2/ 5} & { 5/13} & { 2/ 5} & {37/93} & {18/47} & { 2/ 5} & { 5/13} & { 2/ 5} & {39/98} & {38/99} & { 2/ 5} & { 5/13} & { 2/ 5} & {39/98} & { 5/13} & { 2/ 5} & { 5/13} & { 2/ 5} & {39/98} & { 5/13} & { 2/ 5} & {11/29} & { 2/ 5} & {39/98} & { 5/13} & { 2/ 5} & {\color{red} 27/71} & { 2/ 5} & {39/98} & { 5/13} & { 2/ 5} & {\color{red} 33/85} & { 2/ 5} & {39/98} & {24/65} & { 2/ 5} \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g4-a01b05.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 4} & { 2/ 7} & { 2/ 7} & { 3/11} & { 1/ 4} & { 2/ 7} & { 2/ 7} & { 3/11} & { 2/ 7} & { 2/ 7} & { 5/18} & { 5/19} & { 2/ 7} & { 2/ 7} & { 3/11} & { 2/ 7} & { 2/ 7} & { 7/25} & { 3/11} & { 2/ 7} & { 2/ 7} & { 8/29} & { 2/ 7} & { 2/ 7} & { 9/32} & { 3/11} & { 2/ 7} & { 2/ 7} & { 5/18} & { 2/ 7} & { 2/ 7} & {11/39} & {11/40} & { 2/ 7} & { 2/ 7} & {12/43} & { 2/ 7} & { 2/ 7} & {13/46} & {13/47} & { 2/ 7} & { 2/ 7} & { 7/25} & { 2/ 7} & { 2/ 7} & {15/53} & { 5/18} & { 2/ 7} & { 2/ 7} & {16/57} & { 2/ 7} & { 2/ 7} & {17/60} & {17/61} & { 2/ 7} & { 2/ 7} & { 9/32} & { 2/ 7} & { 2/ 7} & {19/67} \\\hline
$2$ & { 1/ 3} && { 1/ 3} && { 6/19} && { 1/ 3} && { 8/23} && { 9/25} && {10/27} && {11/29} && {12/31} && {13/33} && { 2/ 5} && {15/37} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} &\\\hline
$3$ & { 3/10} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {21/64} & { 1/ 3} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} \\\hline
$4$ & { 3/11} && { 3/10} && { 7/23} && {\color{red}  8/25} && { 1/ 3} && {10/29} && {11/31} && { 4/11} && {13/35} && {14/37} && { 5/13} && {16/41} && {17/43} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && {22/53} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} &\\\hline
$5$ & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red}  5/17} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & {\color{red} 15/49} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {\color{red}  5/16} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {\color{red} 25/79} & { 1/ 3} \\\hline
$6$ & { 4/13} && { 1/ 3} && { 1/ 3} && { 6/19} && { 1/ 3} && { 1/ 3} && {12/35} && {13/37} && {14/39} && {15/41} && {16/43} && {17/45} && {18/47} && {19/49} && {20/51} && {21/53} && { 2/ 5} && {23/57} && {24/59} && {25/61} && {26/63} && {27/65} && {28/67} && {29/69} && {30/71} && {31/73} && {32/75} && { 3/ 7} && {34/79} && {35/81} &\\\hline
$7$ & { 2/ 7} & { 6/17} & { 4/13} & { 6/17} & {\color{red}  5/18} & { 6/17} & { 1/ 3} & { 6/17} & {\color{red}  4/13} & { 6/17} & { 1/ 3} & { 1/ 3} & {\color{red}  1/ 3} & {\color{red} 10/31} & {11/32} & {\color{red}  4/13} & { 6/17} & {10/31} & { 6/17} & {\color{red} 12/37} & { 6/17} & {\color{red}  6/19} & { 6/17} & {14/41} & { 6/17} & {\color{red} 17/52} & { 6/17} & {14/41} & {18/53} & {\color{red} 14/41} & {\color{red}  1/ 3} & {17/49} & {\color{red}  8/25} & { 6/17} & { 1/ 3} & { 6/17} & {\color{red}  1/ 3} & { 6/17} & {\color{red} 17/52} & { 6/17} & {10/29} & { 6/17} & {\color{red}  1/ 3} & { 6/17} & {10/29} & {12/35} & {\color{red} 10/29} & {\color{red} 22/65} & {23/66} & {\color{red} 22/67} & { 6/17} & {22/65} & { 6/17} & {\color{red} 22/65} & { 6/17} & {\color{red}  1/ 3} & { 6/17} & {26/75} & { 6/17} & {\color{red} 26/77} \\\hline
$8$ & { 1/ 3} && { 1/ 3} && {\color{red}  9/31} && { 1/ 3} && { 1/ 3} && {\color{red} 12/37} && { 1/ 3} && {14/41} && {15/43} && {16/45} && {17/47} && {18/49} && {19/51} && {20/53} && {21/55} && {22/57} && {23/59} && {24/61} && {25/63} && { 2/ 5} && {27/67} && {28/69} && {29/71} && {30/73} && {31/75} && {32/77} && {33/79} && {34/81} && {35/83} && {36/85} &\\\hline
$9$ & { 5/16} & { 7/19} & { 1/ 3} & { 7/19} & { 1/ 3} & { 7/19} & { 7/22} & { 7/19} & { 1/ 3} & { 7/19} & { 1/ 3} & { 7/20} & {11/32} & { 1/ 3} & { 6/17} & {10/31} & {13/36} & { 1/ 3} & { 7/19} & { 1/ 3} & { 7/19} & {\color{red} 12/37} & { 7/19} & { 1/ 3} & { 7/19} & {\color{red}  1/ 3} & { 7/19} & {16/47} & { 7/19} & {17/49} & {21/59} & { 6/17} & {21/61} & {19/53} & {\color{red}  1/ 3} & { 4/11} & {\color{red} 17/52} & { 7/19} & {\color{red}  1/ 3} & { 7/19} & {\color{red}  1/ 3} & { 7/19} & {21/62} & { 7/19} & {\color{red} 11/32} & { 7/19} & {23/66} & { 7/19} & { 6/17} & {14/39} & { 5/14} & { 7/20} & {13/36} & {\color{red} 25/73} & {27/74} & {\color{red}  1/ 3} & { 7/19} & {\color{red} 25/73} & { 7/19} & {\color{red} 25/73} \\\hline
$10$ & { 5/17} && { 5/16} && { 2/ 7} && {\color{red} 12/37} && {\color{red}  5/16} && {\color{red} 13/41} && {\color{red} 14/43} && { 1/ 3} && {\color{red} 16/47} && {17/49} && { 6/17} && {\color{red} 19/53} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} &\\\hline
$11$ & { 1/ 3} & { 8/21} & { 1/ 3} & { 8/21} & { 4/13} & { 8/21} & { 1/ 3} & { 8/21} & { 1/ 3} & { 8/21} & {11/32} & { 4/11} & { 6/17} & { 8/23} & {13/36} & { 1/ 3} & { 7/19} & { 1/ 3} & { 3/ 8} & {\color{red} 13/41} & { 8/21} & { 1/ 3} & { 8/21} & { 1/ 3} & { 8/21} & {16/47} & { 8/21} & {17/49} & { 8/21} & { 6/17} & { 8/21} & {19/53} & {24/65} & { 4/11} & {24/67} & { 7/19} & { 8/23} & {22/59} & {\color{red} 24/71} & {23/61} & {\color{red} 21/62} & { 8/21} & {\color{red} 11/32} & { 8/21} & {\color{red} 23/66} & { 8/21} & { 6/17} & { 8/21} & { 5/14} & { 8/21} & {13/36} & { 8/21} & {27/74} & {16/43} & { 7/19} & { 4/11} & {29/78} & {16/45} & { 3/ 8} & {\color{red}  8/23} \\\hline
$12$ & { 6/19} && { 1/ 3} && { 1/ 3} && { 8/25} && { 1/ 3} && { 1/ 3} && {\color{red} 10/31} && { 1/ 3} && { 1/ 3} && {18/53} && {19/55} && {20/57} && {21/59} && {22/61} && {23/63} && {24/65} && {25/67} && {26/69} && {27/71} && {28/73} && {29/75} && {30/77} && {31/79} && {32/81} && {33/83} && { 2/ 5} && {35/87} && {36/89} && {37/91} && {38/93} &\\\hline
$13$ & { 3/10} & { 9/23} & { 6/19} & { 9/23} & { 9/28} & { 9/23} & {\color{red}  1/ 3} & { 9/23} & {11/32} & { 9/23} & { 6/17} & { 3/ 8} & {13/36} & { 9/25} & { 7/19} & { 9/26} & { 3/ 8} & { 1/ 3} & { 8/21} & {\color{red} 15/46} & {17/44} & {\color{red}  1/ 3} & { 9/23} & {\color{red} 16/47} & { 9/23} & {\color{red} 17/49} & { 9/23} & { 6/17} & { 9/23} & {\color{red} 19/53} & { 9/23} & { 4/11} & { 9/23} & { 7/19} & {27/71} & {22/59} & {27/73} & {23/61} & {\color{red}  9/25} & { 8/21} & {27/77} & { 5/13} & {\color{red} 23/66} & {26/67} & {\color{red}  6/17} & { 9/23} & {\color{red}  5/14} & { 9/23} & {\color{red} 13/36} & { 9/23} & {27/74} & { 9/23} & {\color{red}  7/19} & { 9/23} & {29/78} & { 9/23} & { 3/ 8} & {18/47} & {31/82} & { 3/ 8} \\\hline
$14$ & { 1/ 3} && { 1/ 3} && {\color{red}  7/25} && {\color{red}  1/ 3} && { 1/ 3} && {\color{red} 16/49} && {\color{red}  1/ 3} && { 1/ 3} && {\color{red}  1/ 3} && { 1/ 3} && {\color{red} 20/59} && {21/61} && {\color{red} 22/63} && {\color{red} 23/65} && {24/67} && {\color{red} 25/69} && {26/71} && {27/73} && {28/75} && {29/77} && {30/79} && {31/81} && {32/83} && {33/85} && {34/87} && {35/89} && {36/91} && {37/93} && { 2/ 5} && {39/97} &\\\hline
$15$ & { 7/22} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 1/ 3} & { 2/ 5} & {11/32} & { 2/ 5} & { 6/17} & { 2/ 5} & {13/36} & { 5/13} & { 7/19} & {10/27} & { 3/ 8} & { 5/14} & { 8/21} & {10/29} & {17/44} & { 1/ 3} & { 9/23} & {16/47} & {19/48} & {17/49} & { 2/ 5} & { 6/17} & { 2/ 5} & {19/53} & { 2/ 5} & { 4/11} & { 2/ 5} & { 7/19} & { 2/ 5} & {22/59} & { 2/ 5} & {23/61} & {30/77} & { 8/21} & {30/79} & { 5/13} & {10/27} & {26/67} & {30/83} & { 9/23} & {\color{red}  5/14} & {28/71} & {\color{red} 13/36} & {29/73} & {\color{red} 27/74} & { 2/ 5} & { 7/19} & { 2/ 5} & {\color{red} 29/78} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {31/82} & { 2/ 5} & { 8/21} & { 2/ 5} \\\hline
$16$ & { 7/23} && { 7/22} && {14/47} && {\color{red} 16/49} && {\color{red}  1/ 3} && {\color{red}  5/16} && {\color{red} 19/55} && {\color{red}  7/22} && {\color{red} 19/59} && {\color{red} 20/61} && { 1/ 3} && {\color{red} 22/65} && {\color{red} 23/67} && { 8/23} && {26/71} && {26/73} && {\color{red}  9/25} && {\color{red}  4/11} && {29/79} && {10/27} && {31/83} && {32/85} && {11/29} && {34/89} && { 5/13} && {12/31} && {37/95} && {38/97} && {13/33} && {21/53} &\\\hline
$17$ & { 1/ 3} & {11/27} & { 1/ 3} & {11/27} & {16/49} & {11/27} & { 6/17} & {11/27} & {13/36} & {11/27} & { 7/19} & {11/28} & { 3/ 8} & {11/29} & { 8/21} & {11/30} & {17/44} & {11/31} & { 9/23} & {\color{red} 11/32} & {19/48} & { 1/ 3} & { 2/ 5} & { 6/17} & {21/52} & {19/53} & {11/27} & { 4/11} & {11/27} & { 7/19} & {11/27} & {22/59} & {11/27} & {23/61} & {11/27} & { 8/21} & {11/27} & { 5/13} & {33/83} & {26/67} & {33/85} & { 9/23} & {11/29} & {28/71} & {33/89} & {29/73} & {\color{red} 27/74} & { 2/ 5} & {\color{red}  7/19} & {31/77} & {\color{red} 29/78} & {32/79} & { 3/ 8} & {11/27} & {31/82} & {11/27} & { 8/21} & {11/27} & {33/86} & {11/27} \\\hline
$18$ & { 8/25} && { 1/ 3} && { 1/ 3} && {\color{red} 10/31} && { 1/ 3} && {\color{red}  1/ 3} && {\color{red}  1/ 3} && { 1/ 3} && {\color{red} 27/80} && {\color{red} 14/43} && { 1/ 3} && { 1/ 3} && {\color{red} 24/71} && {25/73} && {\color{red} 26/75} && {\color{red} 27/77} && {\color{red} 28/79} && {\color{red} 29/81} && {30/83} && {\color{red} 31/85} && {32/87} && {33/89} && {34/91} && {35/93} && {36/95} && {\color{red} 36/95} && {\color{red} 37/97} && {\color{red} 38/99} && {\color{red} 22/57} && {\color{red} 33/85} &\\\hline
$19$ & { 4/13} & {12/29} & { 8/25} & {12/29} & {17/53} & {12/29} & {19/55} & {12/29} & { 7/19} & {12/29} & { 3/ 8} & { 2/ 5} & { 8/21} & {12/31} & {17/44} & { 3/ 8} & { 9/23} & { 4/11} & {19/48} & { 6/17} & { 2/ 5} & {12/35} & {21/52} & { 1/ 3} & {11/27} & {13/37} & {23/56} & { 7/19} & {12/29} & {22/59} & {12/29} & {23/61} & {12/29} & { 8/21} & {12/29} & { 5/13} & {12/29} & {26/67} & {12/29} & { 9/23} & {36/89} & {28/71} & {36/91} & {29/73} & {12/31} & { 2/ 5} & {36/95} & {31/77} & {\color{red} 29/78} & {32/79} & {\color{red}  3/ 8} & {11/27} & {\color{red} 31/82} & {34/83} & { 8/21} & { 7/17} & {33/86} & {12/29} & {17/44} & {12/29} \\\hline
$20$ & { 1/ 3} && { 1/ 3} && { 2/ 7} && {\color{red}  1/ 3} && { 1/ 3} && {\color{red}  1/ 3} && {\color{red} 22/63} && { 1/ 3} && {\color{red} 29/84} && {\color{red}  1/ 3} && {\color{red}  1/ 3} && {\color{red}  1/ 3} && { 1/ 3} && {\color{red} 26/77} && {\color{red} 27/79} && {\color{red} 28/81} && {\color{red} 30/83} && { 6/17} && {\color{red} 32/87} && {\color{red} 32/89} && {\color{red} 33/91} && {\color{red} 34/93} && {\color{red} 34/93} && {\color{red}  7/19} && {\color{red} 36/97} && {\color{red} 37/99} && {\color{red} 35/93} && {\color{red} 35/93} && {\color{red} 25/66} && {\color{red}  7/19} &\\\hline
$21$ & { 9/28} & {13/31} & { 1/ 3} & {13/31} & { 1/ 3} & {13/31} & {\color{red} 20/59} & {13/31} & {22/61} & {13/31} & { 8/21} & {13/32} & {17/44} & {13/33} & { 9/23} & {13/34} & {19/48} & {13/35} & { 2/ 5} & {13/36} & {21/52} & {13/37} & {11/27} & {\color{red} 13/38} & {23/56} & { 1/ 3} & {12/29} & { 7/20} & { 5/12} & {15/41} & {13/31} & { 8/21} & {13/31} & { 5/13} & {13/31} & {26/67} & {13/31} & { 9/23} & {13/31} & {28/71} & {13/31} & {29/73} & {39/95} & { 2/ 5} & {39/97} & {31/77} & {13/33} & {32/79} & {22/57} & {11/27} & {25/66} & {34/83} & { 8/21} & { 7/17} & {\color{red} 33/86} & {12/29} & {17/44} & {37/89} & { 7/18} & {38/91} \\\hline
$22$ & { 9/29} && { 9/28} && {\color{red} 18/59} && {\color{red} 20/61} && {\color{red}  1/ 3} && {\color{red} 22/65} && {\color{red} 23/67} && {\color{red} 16/47} && {\color{red} 11/32} && {\color{red} 11/32} && {\color{red} 11/32} && {\color{red} 11/32} && {11/32} && { 1/ 3} && {\color{red} 28/83} && {\color{red} 29/85} && {\color{red} 10/29} && {\color{red} 32/89} && {\color{red} 32/91} && {\color{red} 11/31} && {\color{red}  7/19} && {\color{red} 34/95} && {\color{red} 35/97} && {\color{red} 35/97} && {\color{red}  4/11} && {\color{red} 26/71} && {\color{red} 31/84} && {\color{red} 34/95} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$23$ & { 1/ 3} & {14/33} & { 1/ 3} & {14/33} & {\color{red} 19/61} & {14/33} & {\color{red}  1/ 3} & {14/33} & {23/65} & {14/33} & {25/67} & { 7/17} & { 9/23} & { 2/ 5} & {19/48} & { 7/18} & { 2/ 5} & {14/37} & {21/52} & {\color{red}  7/19} & {11/27} & {14/39} & {23/56} & { 7/20} & {12/29} & {\color{red} 14/41} & { 5/12} & { 1/ 3} & {13/31} & {15/43} & {27/64} & { 4/11} & {14/33} & {17/45} & {14/33} & { 9/23} & {14/33} & {28/71} & {14/33} & {29/73} & {14/33} & { 2/ 5} & {14/33} & {31/77} & {37/89} & {32/79} & {31/76} & {11/27} & { 2/ 5} & {34/83} & {31/79} & { 7/17} & {37/96} & {12/29} & {14/37} & {37/89} & {35/92} & {38/91} & { 9/23} & {13/31} \\\hline
$24$ & {10/31} && { 1/ 3} && { 1/ 3} && {14/41} && { 1/ 3} && {\color{red}  8/23} && {\color{red} 25/71} && {17/49} && {\color{red}  9/25} && { 6/17} && { 6/17} && {\color{red}  6/17} && { 6/17} && { 6/17} && { 1/ 3} && {\color{red} 22/65} && {\color{red} 30/89} && {\color{red} 11/31} && {\color{red} 34/95} && {\color{red}  8/23} && {\color{red} 37/99} && {\color{red} 35/99} && {\color{red}  9/25} && {\color{red} 35/99} && {\color{red} 35/99} && {\color{red} 23/64} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$25$ & { 5/16} & { 3/ 7} & {10/31} & { 3/ 7} & { 4/13} & { 3/ 7} & {\color{red} 22/67} & { 3/ 7} & {\color{red}  8/23} & { 3/ 7} & {26/71} & { 5/12} & {28/73} & {15/37} & { 2/ 5} & {15/38} & {21/52} & { 5/13} & {11/27} & { 3/ 8} & {23/56} & {15/41} & {12/29} & {\color{red}  5/14} & { 5/12} & {\color{red} 15/43} & {13/31} & {\color{red} 15/44} & {27/64} & { 1/ 3} & {14/33} & { 8/23} & {29/68} & {17/47} & { 3/ 7} & { 3/ 8} & { 3/ 7} & {19/49} & { 3/ 7} & { 2/ 5} & { 3/ 7} & {31/77} & { 3/ 7} & {32/79} & { 3/ 7} & {11/27} & {37/88} & {34/83} & {26/63} & { 7/17} & {15/37} & {12/29} & {39/98} & {37/89} & {\color{red} 15/43} & {38/91} & {\color{red} 33/94} & {13/31} & {\color{red} 17/47} & { 8/19} \\\hline
$26$ & { 1/ 3} && { 1/ 3} && {13/41} && {\color{red}  1/ 3} && {\color{red} 24/71} && {16/47} && {\color{red}  9/25} && { 6/17} && {\color{red} 19/53} && {\color{red} 13/36} && {13/36} && {\color{red} 13/36} && {13/36} && {13/36} && {32/91} && { 1/ 3} && {\color{red}  1/ 3} && {\color{red} 24/71} && {\color{red} 32/95} && {\color{red} 26/71} && {\color{red} 26/75} && {\color{red}  9/25} && {\color{red} 29/81} && {\color{red} 28/79} && {\color{red} 29/81} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$27$ & {11/34} & {16/37} & { 1/ 3} & {16/37} & { 1/ 3} & {16/37} & {\color{red} 24/71} & {16/37} & {25/73} & {16/37} & { 9/25} & { 8/19} & {29/77} & {16/39} & {31/79} & { 2/ 5} & {11/27} & {16/41} & {23/56} & { 8/21} & {12/29} & {16/43} & { 5/12} & {\color{red}  4/11} & {13/31} & {16/45} & {27/64} & { 8/23} & {14/33} & {\color{red}  1/ 3} & {29/68} & { 1/ 3} & { 3/ 7} & {\color{red} 17/49} & {31/72} & { 9/25} & {16/37} & {19/51} & {16/37} & { 5/13} & {16/37} & {21/53} & {16/37} & {11/27} & {16/37} & {34/83} & {16/37} & { 7/17} & {\color{red} 16/41} & {12/29} & {38/91} & {37/89} & {16/39} & {38/91} & {\color{red} 23/63} & {13/31} & {\color{red} 16/45} & { 8/19} & {\color{red}  8/23} & {41/97} \\\hline
$28$ & {11/35} && {11/34} && {14/43} && { 1/ 3} && {\color{red} 16/47} && {\color{red} 33/94} && { 6/17} && {19/53} && {\color{red}  4/11} && { 7/19} && { 7/19} && { 7/19} && { 7/19} && { 7/19} && { 7/19} && {34/97} && {\color{red} 13/40} && {\color{red}  1/ 3} && {\color{red}  1/ 3} && {\color{red} 27/77} && {\color{red} 27/79} && {\color{red} 27/77} && {\color{red} 30/83} && {\color{red}  6/17} && {\color{red} 30/83} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$29$ & { 1/ 3} & {17/39} & { 1/ 3} & {17/39} & {\color{red} 22/73} & {17/39} & {\color{red}  1/ 3} & {17/39} & {\color{red} 26/77} & {17/39} & {\color{red} 28/79} & {17/40} & {10/27} & {17/41} & {32/83} & {17/42} & { 2/ 5} & {17/43} & {12/29} & {17/44} & { 5/12} & {17/45} & {13/31} & {17/46} & {27/64} & {35/94} & {14/33} & {\color{red} 17/48} & {29/68} & {\color{red}  1/ 3} & { 3/ 7} & {\color{red} 31/96} & {31/72} & { 1/ 3} & {16/37} & {\color{red} 26/77} & {33/76} & {\color{red} 28/79} & {17/39} & {10/27} & {17/39} & {21/55} & {17/39} & {11/28} & {17/39} & {23/57} & {17/39} & {12/29} & {17/39} & {37/89} & { 3/ 7} & {38/91} & {\color{red} 17/44} & {13/31} & {\color{red} 17/45} & { 8/19} & {\color{red} 17/46} & {41/97} & {\color{red} 35/94} & {14/33} \\\hline
$30$ & {12/37} && { 1/ 3} && { 1/ 3} && {\color{red} 16/47} && {17/49} && { 6/17} && {\color{red} 30/83} && { 4/11} && {\color{red}  7/19} && {22/59} && { 3/ 8} && {\color{red}  3/ 8} && { 3/ 8} && { 3/ 8} && { 3/ 8} && {26/71} && {\color{red} 14/41} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 27/79} && {\color{red} 28/81} && {\color{red} 30/83} && {\color{red}  1/99} && {\color{red} 32/87} && {\color{red} 32/89} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$31$ & { 6/19} & {18/41} & {12/37} & {18/41} & {\color{red} 24/77} & {18/41} & {\color{red} 27/79} & {18/41} & {\color{red} 28/81} & {18/41} & {\color{red} 29/83} & { 3/ 7} & {31/85} & {18/43} & {11/29} & { 9/22} & {35/89} & { 2/ 5} & {37/91} & { 9/23} & {13/31} & {18/47} & {27/64} & {\color{red}  3/ 8} & {14/33} & {18/49} & {29/68} & {\color{red}  9/25} & { 3/ 7} & {\color{red} 17/50} & {31/72} & {\color{red}  8/25} & {16/37} & {\color{red} 14/41} & {33/76} & {\color{red}  1/99} & {17/39} & {\color{red} 27/79} & { 7/16} & {\color{red} 29/83} & {18/41} & {\color{red} 31/85} & {18/41} & {11/29} & {18/41} & {23/59} & {18/41} & { 2/ 5} & {\color{red} 18/43} & {25/61} & {18/41} & {13/31} & {\color{red}  2/ 5} & { 8/19} & {\color{red}  9/23} & {41/97} & {\color{red} 18/47} & {14/33} & {\color{red}  3/ 8} & {23/54} \\\hline
$32$ & { 1/ 3} && { 1/ 3} && {26/79} && {17/49} && { 6/17} && {19/53} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 8/21} && { 8/21} && { 8/21} && { 8/21} && { 8/21} && {35/96} && {\color{red} 15/44} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$33$ & {13/40} & {19/43} & { 1/ 3} & {19/43} & { 1/ 3} & {19/43} & {\color{red} 28/83} & {19/43} & {\color{red}  1/ 3} & {19/43} & {\color{red} 10/29} & {19/44} & {\color{red} 32/89} & {19/45} & {34/91} & {19/46} & {12/31} & {19/47} & { 2/ 5} & {19/48} & {40/97} & {19/49} & {14/33} & {19/50} & {29/68} & {\color{red} 19/51} & { 3/ 7} & {\color{red}  6/17} & {31/72} & {\color{red}  9/26} & {16/37} & {\color{red}  1/ 3} & {33/76} & {\color{red} 24/73} & {17/39} & {\color{red}  1/99} & { 7/16} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {19/43} & {\color{red} 34/91} & {19/43} & {12/31} & {\color{red} 19/44} & {\color{red} 37/95} & {\color{red} 19/45} & {13/32} & {\color{red} 19/46} & {27/65} & {\color{red} 19/47} & {14/33} & {\color{red} 19/48} & {23/54} & {\color{red} 19/49} & {41/96} \\\hline
$34$ & {13/41} && {13/40} && {27/83} && { 6/17} && {19/53} && { 4/11} && { 7/19} && {22/59} && {\color{red} 36/95} && { 8/21} && { 5/13} && {17/44} && {17/44} && {17/44} && {17/44} && {17/44} && {14/37} && {\color{red} 16/45} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$35$ & { 1/ 3} & { 4/ 9} & { 1/ 3} & { 4/ 9} & {\color{red}  3/10} & { 4/ 9} & {\color{red}  1/ 3} & { 4/ 9} & {\color{red} 31/89} & { 4/ 9} & {\color{red} 32/91} & {10/23} & {\color{red} 11/31} & {20/47} & { 7/19} & { 5/12} & {37/97} & {20/49} & {13/33} & {\color{red} 17/47} & {28/69} & {20/51} & {38/91} & { 5/13} & { 3/ 7} & {\color{red} 19/52} & {31/72} & {\color{red} 19/53} & {16/37} & {\color{red} 14/41} & {33/76} & {\color{red} 19/55} & {17/39} & {\color{red} 29/86} & { 7/16} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & { 4/ 9} & {\color{red} 37/97} & { 4/ 9} & {13/33} & {\color{red} 20/47} & {\color{red} 21/53} & {\color{red}  5/12} & {\color{red} 28/69} & {\color{red} 20/49} & {\color{red} 38/91} & {\color{red}  2/ 5} & { 3/ 7} \\\hline
$36$ & {14/43} && { 1/ 3} && { 1/ 3} && {31/89} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && { 9/23} && { 9/23} && { 9/23} && { 9/23} && { 9/23} && {\color{red} 35/94} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$37$ & { 7/22} & {21/47} & {14/43} & {21/47} & {\color{red} 28/89} & {21/47} & {\color{red} 31/91} & {21/47} & {\color{red} 32/93} & {21/47} & {\color{red} 14/41} & { 7/16} & {\color{red} 35/97} & { 3/ 7} & {\color{red}  4/11} & {21/50} & {35/93} & { 7/17} & {33/85} & {21/52} & { 2/ 5} & {21/53} & {37/90} & {\color{red} 20/53} & {27/64} & {\color{red} 10/27} & {16/37} & {\color{red} 25/71} & {33/76} & {\color{red}  5/14} & {17/39} & {\color{red} 16/47} & { 7/16} & {\color{red} 15/44} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red}  3/ 7} & { 2/ 5} & {\color{red} 21/50} & {\color{red} 39/97} & {\color{red}  7/17} & {\color{red} 37/90} \\\hline
$38$ & { 1/ 3} && { 1/ 3} && {\color{red} 29/91} && {\color{red} 32/93} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {19/48} && {19/48} && {19/48} && {19/48} && {19/48} && {\color{red} 37/98} && {\color{red} 18/49} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$39$ & {15/46} & {22/49} & { 1/ 3} & {22/49} & { 1/ 3} & {22/49} & {\color{red} 32/95} & {22/49} & {\color{red} 33/97} & {22/49} & {\color{red} 35/99} & {11/25} & {\color{red} 26/71} & {22/51} & {\color{red} 23/64} & {11/26} & {13/35} & {22/53} & {23/60} & {11/27} & {28/71} & { 2/ 5} & {15/37} & {\color{red} 19/53} & {37/89} & {\color{red}  3/ 8} & {26/61} & {\color{red} 27/77} & {17/39} & {\color{red}  9/25} & { 7/16} & {\color{red} 27/77} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red} 17/49} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red}  1/99} & {\color{red} 22/51} & {\color{red}  1/99} & {\color{red} 11/26} & {15/37} \\\hline
$40$ & {15/47} && {15/46} && { 6/19} && {\color{red} 33/97} && { 4/11} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {\color{red} 13/34} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$41$ & { 1/ 3} & {23/51} & { 1/ 3} & {23/51} & { 9/28} & {23/51} & {10/29} & {23/51} & {\color{red} 26/75} & {23/51} & {\color{red} 29/83} & {23/52} & {\color{red} 31/88} & {23/53} & {\color{red} 23/66} & {23/54} & {\color{red} 13/36} & {23/55} & {14/37} & {\color{red} 20/53} & {37/95} & {23/57} & {\color{red} 15/38} & {\color{red} 22/57} & {16/39} & {\color{red}  5/14} & {29/69} & {\color{red} 21/58} & {40/93} & {\color{red} 28/81} & {18/41} & {\color{red} 29/83} & {37/84} & {\color{red} 34/95} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {\color{red} 23/52} & {\color{red}  1/99} & {\color{red} 23/53} & {\color{red}  1/99} \\\hline
$42$ & {16/49} && { 1/ 3} && { 1/ 3} && {\color{red} 33/98} && {23/64} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {21/52} && {21/52} && {21/52} && {21/52} && {21/52} && {\color{red} 29/75} && {\color{red} 20/53} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$43$ & { 8/25} & {24/53} & {16/49} & {24/53} & {19/58} & {24/53} & {\color{red} 18/53} & {24/53} & {\color{red} 12/35} & {24/53} & {\color{red} 27/76} & { 4/ 9} & {\color{red} 29/79} & {24/55} & {\color{red}  6/17} & { 3/ 7} & {\color{red}  9/25} & { 8/19} & {\color{red}  7/19} & {12/29} & { 5/13} & {24/59} & {32/81} & {\color{red} 26/77} & {32/79} & {\color{red} 22/59} & {17/41} & {\color{red} 28/81} & {39/92} & {\color{red} 30/83} & {42/97} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} \\\hline
$44$ & { 1/ 3} && { 1/ 3} && {\color{red} 18/59} && {\color{red} 12/35} && {\color{red} 27/76} && {35/93} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {11/27} && {11/27} && {11/27} && {11/27} && {11/27} && {\color{red} 10/27} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$45$ & {17/52} & { 5/11} & { 1/ 3} & { 5/11} & { 1/ 3} & { 5/11} & {\color{red} 21/62} & { 5/11} & {\color{red} 23/66} & {\color{red} 11/26} & {\color{red} 31/86} & {25/56} & {\color{red} 33/91} & {25/57} & {\color{red}  5/14} & {\color{red}  2/ 5} & {\color{red} 13/36} & {25/59} & {\color{red}  4/11} & {\color{red} 22/57} & {\color{red}  3/ 8} & {\color{red}  2/ 5} & {16/41} & {\color{red} 22/59} & {\color{red} 11/28} & {\color{red} 11/30} & {\color{red} 17/42} & {\color{red} 30/83} & {18/43} & {\color{red} 29/81} & {\color{red} 37/88} & {\color{red}  1/99} & {\color{red} 19/44} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} \\\hline
$46$ & {17/53} && {17/52} && {\color{red} 13/43} && {\color{red} 19/56} && {13/37} && {29/78} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && {23/56} && {23/56} && {23/56} && {23/56} && {23/56} && {\color{red} 15/38} && {\color{red} 32/93} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$47$ & { 1/ 3} & {26/57} & { 1/ 3} & {26/57} & {\color{red} 10/31} & {26/57} & {\color{red} 11/32} & {26/57} & {\color{red} 23/66} & {\color{red} 23/54} & {\color{red}  6/17} & {13/29} & {\color{red} 25/68} & {26/59} & {\color{red} 13/36} & {13/30} & {\color{red} 19/52} & {26/61} & {\color{red}  7/19} & {\color{red} 23/59} & {\color{red} 31/84} & {\color{red} 26/75} & {\color{red}  8/21} & {\color{red} 21/59} & {17/43} & {\color{red} 29/83} & {\color{red} 35/88} & {\color{red}  6/17} & {\color{red}  9/22} & {\color{red}  1/99} & {19/45} & {\color{red}  1/99} & {\color{red} 39/92} & {\color{red}  1/99} & {\color{red} 10/23} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} \\\hline
$48$ & {18/55} && { 1/ 3} && { 1/ 3} && {\color{red} 29/84} && {\color{red}  8/23} && {\color{red} 17/47} && {29/75} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {12/29} && {12/29} && {12/29} && {12/29} && {12/29} && {\color{red} 11/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$49$ & { 9/28} & {27/59} & {18/55} & {27/59} & {\color{red} 26/81} & {27/59} & {23/66} & {27/59} & { 6/17} & {\color{red}  3/ 7} & {\color{red} 30/83} & { 9/20} & {\color{red} 29/78} & {\color{red} 12/29} & {\color{red}  1/99} & {\color{red} 24/59} & {\color{red}  7/19} & {\color{red} 27/73} & {\color{red} 29/78} & {\color{red}  9/25} & {\color{red} 16/43} & {\color{red} 27/77} & {\color{red}  3/ 8} & {\color{red} 29/83} & {\color{red} 17/44} & {\color{red}  6/17} & { 2/ 5} & {\color{red} 31/87} & {\color{red} 37/92} & {\color{red}  1/99} & {\color{red} 19/46} & {\color{red}  1/99} & {20/47} & {\color{red}  1/99} & {\color{red} 41/96} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} \\\hline
$50$ & { 1/ 3} && { 1/ 3} && {\color{red}  1/99} && {\color{red}  1/ 3} && {\color{red} 24/71} && {\color{red} 26/73} && {\color{red} 37/98} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && { 5/12} && { 5/12} && {\color{red} 27/65} && { 5/12} && { 5/12} && {\color{red}  2/ 5} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & {19/58} & {28/61} & { 1/ 3} & {28/61} & { 1/ 3} & {28/61} & { 6/17} & {\color{red} 25/57} & { 5/14} & {\color{red} 25/58} & {\color{red} 13/36} & {14/31} & {\color{red} 27/74} & {\color{red}  5/12} & {\color{red}  1/99} & {\color{red} 25/61} & {\color{red}  3/ 8} & {\color{red} 28/75} & {\color{red} 29/78} & {\color{red}  4/11} & {\color{red}  1/99} & {\color{red} 28/79} & {\color{red} 17/45} & {\color{red}  6/17} & {\color{red} 35/92} & {\color{red} 31/87} & {\color{red}  9/23} & {\color{red} 32/89} & {19/47} & {\color{red}  1/99} & {\color{red} 13/32} & {\color{red}  1/99} & {\color{red}  5/12} & {\color{red}  1/99} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 40/93} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} \\\hline
$52$ & {19/59} && {\color{red} 29/89} && {\color{red}  4/13} && {\color{red}  1/ 3} && {\color{red}  1/99} && {\color{red}  9/25} && {\color{red} 19/51} && {\color{red} 30/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && {13/31} && {13/31} && {\color{red}  5/12} && {13/31} && {\color{red}  4/11} && {\color{red} 26/71} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & { 1/ 3} & {29/63} & { 1/ 3} & {29/63} & {\color{red}  1/99} & {29/63} & {\color{red} 12/35} & {\color{red} 26/59} & {13/36} & {\color{red} 13/30} & {27/74} & {29/64} & {\color{red}  7/19} & {\color{red} 13/31} & {\color{red}  1/99} & {\color{red} 29/75} & {\color{red}  3/ 8} & {\color{red} 29/77} & {\color{red}  1/99} & {\color{red} 29/79} & {\color{red}  1/99} & {\color{red} 29/81} & {\color{red}  1/99} & {\color{red} 30/83} & {\color{red}  1/99} & {\color{red} 32/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/48} & {\color{red}  1/99} & {20/49} & {\color{red}  1/99} & {\color{red} 25/61} & {\color{red}  1/99} & {\color{red} 21/50} & {\color{red}  1/99} & {22/51} & {\color{red}  1/99} & {\color{red} 29/67} & {\color{red}  1/99} & {\color{red} 23/52} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} \\\hline
$54$ & {20/61} && { 1/ 3} && {\color{red}  1/99} && {\color{red} 24/71} && {\color{red} 25/73} && {\color{red} 27/77} && {\color{red} 29/79} && {\color{red} 29/75} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {27/64} && {27/64} && {\color{red} 37/88} && {\color{red} 13/33} && {\color{red} 35/93} && {\color{red} 23/64} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & {10/31} & { 6/13} & {\color{red} 13/40} & { 6/13} & {\color{red}  1/99} & { 6/13} & {\color{red} 31/91} & {\color{red} 27/61} & {27/74} & {\color{red} 27/62} & { 7/19} & {\color{red} 30/73} & {\color{red} 29/78} & {\color{red}  2/ 5} & {\color{red} 29/78} & {\color{red} 30/77} & {\color{red}  3/ 8} & {\color{red} 30/79} & {\color{red}  1/99} & {\color{red} 10/27} & {\color{red}  1/99} & {\color{red} 30/83} & {\color{red}  1/99} & {\color{red}  6/17} & {\color{red}  1/99} & {\color{red} 32/91} & {\color{red}  1/99} & {\color{red} 34/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 7/17} & {\color{red}  1/99} & {\color{red} 31/75} & {\color{red}  1/99} & {\color{red} 11/26} & {\color{red}  1/99} & {23/53} & {\color{red}  1/99} & {\color{red} 37/85} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {40/87} & {\color{red}  1/99} \\\hline
$56$ & { 1/ 3} && { 1/ 3} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 24/73} && {\color{red} 10/27} && {\color{red} 21/55} && {\color{red} 33/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {14/33} && {14/33} && {\color{red} 11/26} && {\color{red} 33/85} && {\color{red} 13/35} && {\color{red} 31/86} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & {21/64} & {31/67} & { 1/ 3} & {31/67} & {\color{red}  1/99} & {31/67} & {\color{red}  1/99} & {\color{red} 31/71} & { 7/19} & {\color{red}  7/16} & {29/78} & {\color{red} 31/75} & {\color{red}  3/ 8} & {\color{red} 31/77} & {\color{red}  3/ 8} & {\color{red} 31/79} & {\color{red}  8/21} & {\color{red} 31/81} & {\color{red}  1/99} & {\color{red} 31/83} & {\color{red}  1/99} & {\color{red} 31/85} & {\color{red}  1/99} & {\color{red} 32/87} & {\color{red}  1/99} & {\color{red} 32/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {22/53} & {\color{red}  1/99} & {\color{red}  5/12} & {\color{red}  1/99} & {\color{red} 23/54} & {\color{red}  1/99} & {24/55} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red} 25/56} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {40/87} & {\color{red}  1/99} & {29/63} & {\color{red}  1/99} \\\hline
$58$ & {21/65} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 23/71} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 32/85} && {\color{red} 15/38} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {23/54} && {\color{red} 23/54} && {\color{red} 23/54} && {\color{red} 38/91} && {\color{red}  2/ 5} && {\color{red} 23/60} && {\color{red} 29/79} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & { 1/ 3} & {32/69} & {\color{red}  1/99} & {32/69} & {\color{red}  1/99} & {32/69} & {\color{red}  1/99} & {\color{red} 32/73} & {\color{red} 14/39} & {\color{red} 32/75} & { 3/ 8} & {\color{red} 32/77} & {\color{red} 31/82} & {\color{red} 32/79} & {\color{red} 31/82} & {\color{red} 32/81} & {\color{red}  1/99} & {\color{red} 32/83} & {\color{red}  1/99} & {\color{red} 32/85} & {\color{red}  1/99} & {\color{red} 32/87} & {\color{red}  1/99} & {\color{red} 32/89} & {\color{red}  1/99} & {\color{red} 32/91} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 34/81} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red}  1/99} & {25/57} & {\color{red}  1/99} & {\color{red} 40/91} & {\color{red}  1/99} & {\color{red} 13/29} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {40/87} & {\color{red}  1/99} & {29/63} & {\color{red}  1/99} & {41/89} & {\color{red}  1/99} \\\hline
$60$ & {22/67} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 23/59} && {\color{red} 36/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {23/54} && {41/96} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 37/90} && {\color{red} 28/71} && {\color{red} 14/37} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g4-a02b03.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 2/ 7} & { 1/ 4} & {\color{red}  3/11} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 4/13} & { 2/ 7} & {\color{red}  5/17} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/19} & { 3/10} & {\color{red}  7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 8/25} & { 4/13} & {\color{red}  9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {10/31} & { 5/16} & {\color{red} 11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & {\color{red} 13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & { 7/22} & {\color{red} 15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 8/25} & {\color{red} 17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & {\color{red} 19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {\color{red} 21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} \\\hline
$2$ & { 1/ 4} & { 1/ 4} & {\color{red}  4/17} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 4/15} & { 1/ 4} & {\color{red}  1/ 4} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 3/11} & { 6/23} & {\color{red}  7/27} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 8/29} & { 4/15} & {\color{red}  9/34} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 5/18} & {10/37} & {\color{red} 11/41} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & {12/43} & { 3/11} & {\color{red} 13/48} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 7/25} & {14/51} & {\color{red}  3/11} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & {16/57} & { 8/29} & {\color{red} 17/62} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 9/32} & {18/65} & {\color{red} 19/69} & { 2/ 7} \\\hline
$3$ & { 1/ 3} & { 2/ 7} & { 1/ 4} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red}  5/19} & { 5/17} & { 1/ 3} & { 1/ 3} & { 7/23} & { 2/ 7} & { 7/22} & { 1/ 3} & { 1/ 3} & {\color{red}  2/ 7} & { 4/13} & { 1/ 3} & { 1/ 3} & { 5/16} & { 3/10} & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red} 11/37} & {11/35} & { 1/ 3} & { 1/ 3} & {13/41} & { 4/13} & {13/40} & { 1/ 3} & { 1/ 3} & {\color{red}  7/23} & { 7/22} & { 1/ 3} & { 1/ 3} & { 8/25} & { 5/16} & {16/49} & { 1/ 3} & { 1/ 3} & {\color{red} 17/55} & {17/53} & { 1/ 3} & { 1/ 3} & {19/59} & { 6/19} & {19/58} & { 1/ 3} & { 1/ 3} & {\color{red}  5/16} & {10/31} & { 1/ 3} & { 1/ 3} & {11/34} & { 7/22} & {22/67} & { 1/ 3} & { 1/ 3} \\\hline
$4$ & { 2/ 5} & { 5/16} & { 4/13} & { 5/14} & { 2/ 5} & { 2/ 5} & { 1/ 3} & { 1/ 3} & { 7/19} & { 2/ 5} & { 2/ 5} & { 9/26} & { 8/23} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {11/31} & { 5/14} & {11/29} & { 2/ 5} & { 2/ 5} & {13/36} & { 4/11} & {13/34} & { 2/ 5} & { 2/ 5} & {15/41} & { 7/19} & { 5/13} & { 2/ 5} & { 2/ 5} & {17/46} & {16/43} & {17/44} & { 2/ 5} & { 2/ 5} & {19/51} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {20/53} & { 7/18} & { 2/ 5} & { 2/ 5} & {23/61} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {25/66} & { 8/21} & {25/64} & { 2/ 5} & { 2/ 5} & {27/71} & {13/34} & { 9/23} & { 2/ 5} \\\hline
$5$ & { 4/11} & { 1/ 3} & { 6/19} & { 2/ 5} & { 2/ 5} & { 3/ 8} & { 6/17} & { 1/ 3} & { 2/ 5} & { 2/ 5} & { 8/21} & { 4/11} & { 8/23} & { 2/ 5} & { 2/ 5} & { 5/13} & {10/27} & { 5/14} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & { 4/11} & { 2/ 5} & { 2/ 5} & { 7/18} & {14/37} & { 7/19} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {16/43} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & { 2/ 5} & { 2/ 5} & {11/28} & {22/57} & {11/29} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & {\color{red}  8/21} & { 2/ 5} & { 2/ 5} & {13/33} & {26/67} & {\color{red} 13/34} & { 2/ 5} & { 2/ 5} \\\hline
$6$ & { 1/ 3} & { 4/13} & { 2/ 7} & { 4/11} & { 4/11} & { 6/17} & { 1/ 3} & { 6/19} & { 1/ 3} & { 4/11} & { 4/11} & { 8/23} & { 1/ 3} & { 8/25} & { 4/11} & { 4/11} & { 5/14} & {10/29} & { 1/ 3} & {13/38} & { 4/11} & { 4/11} & { 6/17} & {12/35} & { 1/ 3} & { 4/11} & { 4/11} & {14/39} & { 7/20} & {14/41} & {17/49} & { 4/11} & { 4/11} & {16/45} & { 8/23} & {16/47} & { 4/11} & { 4/11} & { 9/25} & { 6/17} & { 9/26} & { 7/20} & { 4/11} & { 4/11} & { 5/14} & {20/57} & {10/29} & { 4/11} & { 4/11} & {22/61} & {11/31} & {22/63} & {25/71} & { 4/11} & { 4/11} & {24/67} & { 6/17} & { 8/23} & { 4/11} & { 4/11} \\\hline
$7$ & { 4/13} & { 2/ 7} & {\color{red}  4/15} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/19} & {\color{red} 16/53} & { 4/13} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 8/25} & { 4/13} & {\color{red} 11/37} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {10/31} & {\color{red}  5/16} & {\color{red}  7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & {\color{red}  7/22} & {\color{red} 14/45} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 8/25} & {\color{red} 16/51} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & {\color{red}  9/28} & {\color{red}  6/19} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {\color{red} 20/63} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {\color{red} 11/34} & {\color{red} 22/69} & { 1/ 3} & { 1/ 3} & { 1/ 3} \\\hline
$8$ & { 5/14} & { 7/24} & { 5/17} & { 1/ 3} & { 5/14} & { 5/14} & { 3/10} & { 7/22} & { 8/23} & { 5/14} & { 1/ 3} & {\color{red}  4/13} & { 1/ 3} & { 5/14} & { 5/14} & { 6/19} & {10/31} & {11/32} & { 5/14} & { 5/14} & {\color{red} 11/35} & { 1/ 3} & {13/37} & { 5/14} & {16/47} & {\color{red} 13/40} & {14/41} & { 5/14} & { 5/14} & {17/52} & { 1/ 3} & { 8/23} & { 5/14} & { 5/14} & {\color{red} 16/49} & {17/50} & { 6/17} & { 5/14} & {21/61} & {\color{red}  1/ 3} & {19/55} & { 5/14} & { 5/14} & { 1/ 3} & {20/59} & { 7/20} & { 5/14} & { 5/14} & {\color{red}  1/ 3} & {11/32} & {23/65} & { 5/14} & {26/75} & {\color{red} 23/68} & { 8/23} & { 5/14} & { 5/14} & {27/80} & {25/73} & {13/37} \\\hline
$9$ & { 2/ 5} & { 4/13} & { 1/ 3} & { 7/19} & { 2/ 5} & { 2/ 5} & {10/31} & { 8/23} & { 3/ 8} & { 2/ 5} & { 2/ 5} & { 1/ 3} & { 5/14} & {11/29} & { 2/ 5} & { 2/ 5} & {11/32} & { 4/11} & {13/34} & { 2/ 5} & { 2/ 5} & {13/37} & { 7/19} & { 5/13} & { 2/ 5} & { 2/ 5} & { 5/14} & {16/43} & {17/44} & { 2/ 5} & { 2/ 5} & {17/47} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & {19/52} & {20/53} & { 7/18} & { 2/ 5} & { 2/ 5} & { 7/19} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {23/62} & { 8/21} & {25/64} & { 2/ 5} & { 2/ 5} & {\color{red} 25/67} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & {\color{red}  3/ 8} & {28/73} & {29/74} & { 2/ 5} \\\hline
$10$ & { 3/ 8} & { 9/28} & { 9/29} & { 2/ 5} & { 2/ 5} & { 8/21} & { 4/11} & {11/34} & { 2/ 5} & { 2/ 5} & { 5/13} & {10/27} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & { 4/11} & { 2/ 5} & { 2/ 5} & { 7/18} & {14/37} & { 7/19} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {16/43} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & { 2/ 5} & { 2/ 5} & {11/28} & {22/57} & {11/29} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 2/ 5} & { 2/ 5} & {13/33} & {26/67} & {13/34} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {28/73} & { 2/ 5} & { 2/ 5} \\\hline
$11$ & { 6/17} & { 1/ 3} & {\color{red}  9/31} & { 3/ 8} & { 3/ 8} & { 4/11} & { 8/23} & { 1/ 3} & {13/37} & { 3/ 8} & {10/27} & { 5/14} & {10/29} & { 1/ 3} & { 3/ 8} & { 3/ 8} & { 4/11} & { 6/17} & {12/35} & { 3/ 8} & { 3/ 8} & { 7/19} & {14/39} & { 7/20} & {19/53} & { 3/ 8} & {16/43} & { 4/11} & {16/45} & { 8/23} & { 3/ 8} & { 3/ 8} & {18/49} & { 9/25} & { 6/17} & { 3/ 8} & { 3/ 8} & {10/27} & { 4/11} & { 5/14} & {25/69} & { 3/ 8} & {22/59} & {11/30} & {22/61} & {\color{red} 11/31} & { 3/ 8} & { 3/ 8} & {24/65} & { 4/11} & {24/67} & { 3/ 8} & { 3/ 8} & {13/35} & {26/71} & {13/36} & {31/85} & { 3/ 8} & {28/75} & { 7/19} \\\hline
$12$ & { 1/ 3} & { 6/19} & { 2/ 7} & { 6/17} & { 6/17} & { 8/23} & { 1/ 3} & {\color{red}  8/25} & { 1/ 3} & { 6/17} & { 6/17} & {10/29} & {\color{red}  1/ 3} & { 1/ 3} & { 1/ 3} & { 6/17} & { 6/17} & {12/35} & { 1/ 3} & {\color{red} 12/37} & { 6/17} & { 6/17} & { 7/20} & {14/41} & {\color{red}  1/ 3} & {\color{red} 20/61} & { 6/17} & { 6/17} & { 8/23} & {\color{red} 16/47} & {\color{red}  1/ 3} & {21/62} & { 6/17} & { 6/17} & { 9/26} & {18/53} & {\color{red}  1/ 3} & { 6/17} & { 6/17} & {20/57} & {10/29} & {\color{red} 20/59} & {\color{red}  1/ 3} & { 6/17} & { 6/17} & {22/63} & {\color{red} 11/32} & {\color{red} 22/65} & {27/79} & { 6/17} & { 6/17} & { 8/23} & {12/35} & {\color{red} 24/71} & { 6/17} & { 6/17} & {13/37} & {26/75} & {\color{red} 13/38} & {\color{red} 26/77} \\\hline
$13$ & { 7/19} & { 3/10} & { 7/22} & { 8/23} & { 7/19} & { 7/19} & { 8/25} & { 1/ 3} & { 5/14} & { 7/19} & {15/43} & { 1/ 3} & {11/32} & { 4/11} & { 7/19} & { 1/ 3} & {\color{red}  1/ 3} & {13/37} & { 7/19} & { 7/19} & {\color{red} 13/40} & {14/41} & { 5/14} & { 7/19} & { 7/19} & {\color{red}  1/ 3} & { 8/23} & {17/47} & { 7/19} & {11/31} & {\color{red} 17/50} & { 6/17} & {19/52} & { 7/19} & {23/67} & {\color{red} 19/55} & { 5/14} & { 7/19} & { 7/19} & {\color{red} 20/59} & { 7/20} & {22/61} & { 7/19} & { 7/19} & {\color{red} 11/32} & {23/65} & { 4/11} & { 7/19} & {29/81} & {\color{red}  8/23} & { 5/14} & {26/71} & { 7/19} & {15/43} & {\color{red} 13/37} & { 9/25} & { 7/19} & { 7/19} & {\color{red}  9/26} & {28/79} \\\hline
$14$ & { 2/ 5} & {11/36} & {12/37} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {\color{red} 13/41} & { 5/14} & {11/29} & { 2/ 5} & { 2/ 5} & {15/46} & { 4/11} & {13/34} & { 2/ 5} & { 2/ 5} & { 1/ 3} & { 7/19} & { 5/13} & { 2/ 5} & { 2/ 5} & { 5/14} & {16/43} & {17/44} & { 2/ 5} & { 2/ 5} & {17/47} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & {19/52} & {20/53} & { 7/18} & { 2/ 5} & { 2/ 5} & { 7/19} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {23/62} & { 8/21} & {25/64} & { 2/ 5} & { 2/ 5} & {25/67} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {28/73} & {29/74} & { 2/ 5} & { 2/ 5} & {29/77} & { 5/13} & {31/79} & { 2/ 5} \\\hline
$15$ & { 8/21} & { 6/19} & { 4/13} & { 2/ 5} & { 2/ 5} & { 5/13} & {15/43} & {\color{red}  7/22} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & {16/49} & { 2/ 5} & { 2/ 5} & { 7/18} & {14/37} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {21/59} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & { 2/ 5} & { 2/ 5} & {11/28} & {22/57} & {11/29} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 2/ 5} & { 2/ 5} & {13/33} & {26/67} & {13/34} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {28/73} & { 2/ 5} & { 2/ 5} & {15/38} & {30/77} & { 5/13} & { 2/ 5} & { 2/ 5} \\\hline
$16$ & { 4/11} & {13/40} & {\color{red} 12/41} & { 8/21} & { 8/21} & {10/27} & { 5/14} & {\color{red} 13/42} & {17/47} & { 8/21} & { 3/ 8} & { 4/11} & { 6/17} & { 9/26} & { 8/21} & {14/37} & { 7/19} & {14/39} & { 1/ 3} & { 8/21} & { 8/21} & {16/43} & { 4/11} & {16/45} & { 8/21} & { 8/21} & { 3/ 8} & {18/49} & { 9/25} & {25/68} & { 8/21} & {20/53} & {10/27} & { 4/11} & { 5/14} & { 8/21} & {11/29} & {22/59} & {11/30} & {22/61} & { 8/21} & { 8/21} & { 3/ 8} & {24/65} & { 4/11} & { 8/21} & { 8/21} & {26/69} & {13/35} & {26/71} & {33/89} & { 8/21} & {14/37} & {28/75} & { 7/19} & {\color{red}  4/11} & { 8/21} & {30/79} & { 3/ 8} & {10/27} \\\hline
$17$ & { 8/23} & { 1/ 3} & { 4/13} & { 4/11} & { 4/11} & { 5/14} & {10/29} & { 1/ 3} & {11/32} & { 4/11} & { 4/11} & { 6/17} & {\color{red} 12/35} & { 8/23} & { 4/11} & { 4/11} & {14/39} & {\color{red}  7/20} & { 8/23} & { 1/ 3} & { 4/11} & { 4/11} & {16/45} & { 8/23} & {16/47} & { 4/11} & { 4/11} & { 9/25} & { 6/17} & {\color{red}  9/26} & {\color{red} 13/38} & { 4/11} & { 4/11} & { 5/14} & {\color{red} 20/57} & {\color{red} 28/81} & { 4/11} & { 4/11} & {22/61} & {\color{red} 11/31} & {\color{red} 22/63} & { 8/23} & { 4/11} & { 4/11} & {24/67} & { 6/17} & {\color{red}  8/23} & { 4/11} & { 4/11} & {13/36} & {26/73} & {\color{red} 13/37} & {\color{red} 17/49} & { 4/11} & { 4/11} & {14/39} & {\color{red} 28/79} & {\color{red}  7/20} & { 4/11} & { 4/11} \\\hline
$18$ & { 3/ 8} & { 8/25} & { 1/ 3} & { 5/14} & { 3/ 8} & { 3/ 8} & { 1/ 3} & {11/32} & { 4/11} & { 3/ 8} & {19/53} & {12/35} & {13/37} & { 7/19} & { 3/ 8} & { 8/23} & { 8/23} & { 5/14} & {16/43} & { 3/ 8} & { 1/ 3} & {\color{red}  8/23} & {17/47} & { 3/ 8} & { 3/ 8} & {17/50} & { 6/17} & {19/52} & { 3/ 8} & { 3/ 8} & {\color{red} 19/55} & { 5/14} & { 7/19} & { 3/ 8} & { 4/11} & {\color{red}  7/20} & {22/61} & {23/62} & { 3/ 8} & {29/82} & {\color{red} 23/65} & { 4/11} & {25/67} & { 3/ 8} & {\color{red}  8/23} & {\color{red}  5/14} & {26/71} & { 3/ 8} & { 3/ 8} & {\color{red} 13/37} & { 9/25} & { 7/19} & { 3/ 8} & { 3/ 8} & {\color{red} 28/79} & {29/80} & {10/27} & { 3/ 8} & {26/71} & {\color{red}  5/14} \\\hline
$19$ & { 2/ 5} & { 4/13} & {15/47} & {11/29} & { 2/ 5} & { 2/ 5} & {10/31} & { 9/26} & {13/34} & { 2/ 5} & { 2/ 5} & { 1/ 3} & { 7/19} & { 5/13} & { 2/ 5} & { 2/ 5} & {\color{red}  1/ 3} & {16/43} & {17/44} & { 2/ 5} & { 2/ 5} & { 1/ 3} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & {25/71} & {20/53} & { 7/18} & { 2/ 5} & { 2/ 5} & { 7/19} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {23/62} & { 8/21} & {25/64} & { 2/ 5} & { 2/ 5} & {25/67} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {28/73} & {29/74} & { 2/ 5} & { 2/ 5} & {29/77} & { 5/13} & {31/79} & { 2/ 5} & { 2/ 5} & {31/82} & {32/83} & {11/28} & { 2/ 5} \\\hline
$20$ & { 5/13} & { 5/16} & {\color{red} 15/49} & { 2/ 5} & { 2/ 5} & {12/31} & {18/53} & {\color{red} 29/92} & { 2/ 5} & { 2/ 5} & { 7/18} & {21/58} & {21/64} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {\color{red} 21/64} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {13/37} & { 2/ 5} & { 2/ 5} & {11/28} & {22/57} & {29/79} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 2/ 5} & { 2/ 5} & {13/33} & {26/67} & {13/34} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {28/73} & { 2/ 5} & { 2/ 5} & {15/38} & {30/77} & { 5/13} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {32/83} & { 2/ 5} & { 2/ 5} \\\hline
$21$ & {10/27} & { 8/25} & { 3/10} & { 5/13} & { 5/13} & { 3/ 8} & { 4/11} & {\color{red} 21/65} & { 7/19} & { 5/13} & {14/37} & { 7/19} & {\color{red}  1/ 3} & {11/31} & { 5/13} & { 8/21} & {16/43} & { 4/11} & {23/67} & { 5/13} & {18/47} & { 3/ 8} & {18/49} & { 1/ 3} & { 5/13} & { 5/13} & {20/53} & {10/27} & { 4/11} & { 5/13} & { 5/13} & {11/29} & {22/59} & {11/30} & {31/83} & { 5/13} & { 8/21} & { 3/ 8} & {24/65} & { 4/11} & { 5/13} & {13/34} & {26/69} & {13/35} & {26/71} & { 5/13} & {28/73} & {14/37} & {28/75} & { 7/19} & { 5/13} & { 5/13} & {30/79} & { 3/ 8} & {10/27} & { 5/13} & { 5/13} & { 8/21} & {32/85} & {16/43} \\\hline
$22$ & { 5/14} & {17/52} & {10/31} & {10/27} & {10/27} & { 4/11} & { 6/17} & { 1/ 3} & {13/37} & {10/27} & { 7/19} & {14/39} & { 7/20} & { 5/14} & {10/27} & {10/27} & { 4/11} & {\color{red} 16/45} & { 5/14} & { 5/14} & {10/27} & {18/49} & {\color{red}  9/25} & { 5/14} & { 1/ 3} & {10/27} & {10/27} & { 4/11} & { 5/14} & {20/57} & {10/27} & {10/27} & {11/30} & {22/61} & {11/31} & {\color{red} 32/91} & {10/27} & {24/65} & { 4/11} & {\color{red} 24/67} & {\color{red} 17/48} & {10/27} & {10/27} & {26/71} & {\color{red} 13/36} & {\color{red} 31/87} & {35/97} & {10/27} & { 7/19} & {\color{red}  4/11} & {\color{red} 14/39} & { 5/14} & {10/27} & {10/27} & {15/41} & {30/83} & {\color{red}  5/14} & {10/27} & {10/27} & {32/87} \\\hline
$23$ & {11/29} & { 1/ 3} & {18/55} & { 4/11} & {11/29} & {11/29} & {12/35} & {13/37} & { 7/19} & {11/29} & {23/63} & { 7/20} & { 5/14} & {16/43} & {11/29} & { 5/14} & {16/45} & {17/47} & { 3/ 8} & {11/29} & { 5/14} & { 5/14} & {19/52} & {20/53} & {11/29} & { 1/ 3} & {\color{red}  5/14} & { 7/19} & {11/29} & {11/29} & { 7/20} & {22/61} & {23/62} & {11/29} & {11/29} & {23/65} & { 4/11} & {25/67} & {11/29} & {17/46} & {\color{red}  5/14} & {26/71} & { 3/ 8} & {11/29} & {35/97} & {\color{red}  9/25} & { 7/19} & {29/77} & {11/29} & {\color{red}  5/14} & {\color{red} 29/80} & {10/27} & {31/82} & {11/29} & {\color{red}  5/14} & {\color{red} 31/85} & {16/43} & {11/29} & {11/29} & {\color{red} 32/89} \\\hline
$24$ & { 2/ 5} & {10/31} & { 6/19} & {13/34} & { 2/ 5} & { 2/ 5} & { 1/ 3} & {21/62} & { 5/13} & { 2/ 5} & { 2/ 5} & {14/41} & {24/67} & {17/44} & { 2/ 5} & { 2/ 5} & {\color{red} 10/29} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & {10/29} & {20/53} & { 7/18} & { 2/ 5} & { 2/ 5} & { 1/ 3} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {15/43} & { 8/21} & {25/64} & { 2/ 5} & { 2/ 5} & {33/91} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {28/73} & {29/74} & { 2/ 5} & { 2/ 5} & {29/77} & { 5/13} & {31/79} & { 2/ 5} & { 2/ 5} & {31/82} & {32/83} & {11/28} & { 2/ 5} & { 2/ 5} & {11/29} & {17/44} & {35/89} & { 2/ 5} \\\hline
$25$ & {12/31} & {\color{red}  5/16} & {\color{red} 18/59} & { 2/ 5} & { 2/ 5} & { 7/18} & {\color{red}  1/ 3} & {\color{red} 21/64} & { 2/ 5} & { 2/ 5} & {16/41} & { 6/17} & {\color{red} 33/98} & { 2/ 5} & { 2/ 5} & { 9/23} & {27/73} & {\color{red} 17/50} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {\color{red}  1/ 3} & { 2/ 5} & { 2/ 5} & {11/28} & {22/57} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & {31/89} & { 2/ 5} & { 2/ 5} & {13/33} & {26/67} & {17/47} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {37/99} & { 2/ 5} & { 2/ 5} & {15/38} & {30/77} & { 5/13} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {32/83} & { 2/ 5} & { 2/ 5} & {17/43} & {34/87} & {17/44} & { 2/ 5} & { 2/ 5} \\\hline
$26$ & { 3/ 8} & {19/60} & {11/35} & {12/31} & {12/31} & {14/37} & {23/65} & {\color{red}  1/ 3} & {25/67} & {12/31} & { 8/21} & {16/43} & {\color{red} 33/97} & {13/36} & {12/31} & {18/47} & { 3/ 8} & {\color{red} 28/81} & {27/77} & {12/31} & { 5/13} & {20/53} & {10/27} & {\color{red} 11/32} & {12/31} & {22/57} & {11/29} & {22/59} & { 1/ 3} & {12/31} & {12/31} & { 8/21} & { 3/ 8} & {33/92} & {12/31} & {12/31} & {13/34} & {26/69} & {13/35} & {37/98} & {12/31} & {28/73} & {14/37} & {28/75} & {31/84} & {12/31} & { 5/13} & {30/79} & { 3/ 8} & {10/27} & {12/31} & {32/83} & { 8/21} & {32/85} & {16/43} & {12/31} & {17/44} & {34/89} & {17/45} & {34/91} \\\hline
$27$ & { 4/11} & {10/31} & { 1/ 3} & { 3/ 8} & { 3/ 8} & { 7/19} & {14/39} & {14/41} & { 5/14} & { 3/ 8} & {16/43} & { 4/11} & { 8/23} & {17/47} & { 3/ 8} & { 3/ 8} & {18/49} & { 9/25} & { 4/11} & { 3/ 8} & { 3/ 8} & {10/27} & {\color{red}  4/11} & { 4/11} & { 6/17} & { 3/ 8} & {22/59} & {\color{red} 11/30} & { 4/11} & { 1/ 3} & { 3/ 8} & { 3/ 8} & {24/65} & { 4/11} & {24/67} & { 3/ 8} & { 3/ 8} & {13/35} & {26/71} & {13/36} & {\color{red} 19/53} & { 3/ 8} & {28/75} & { 7/19} & { 4/11} & {31/86} & { 3/ 8} & { 3/ 8} & {10/27} & {\color{red} 15/41} & {\color{red} 30/83} & { 3/ 8} & { 3/ 8} & {16/43} & {\color{red} 32/87} & {\color{red}  4/11} & { 4/11} & { 3/ 8} & {34/91} & {\color{red} 17/46} \\\hline
$28$ & {13/34} & {21/64} & {21/65} & { 7/19} & {13/34} & {13/34} & { 7/20} & { 5/14} & {16/43} & {13/34} & {27/73} & {16/45} & {17/47} & { 3/ 8} & {13/34} & { 4/11} & { 9/25} & {19/52} & {20/53} & {13/34} & { 4/11} & { 4/11} & { 7/19} & {11/29} & {13/34} & { 4/11} & { 4/11} & {23/62} & { 8/21} & {13/34} & { 1/ 3} & {\color{red}  4/11} & {25/67} & {13/34} & {13/34} & { 5/14} & {26/71} & { 3/ 8} & {13/34} & {13/34} & { 9/25} & { 7/19} & {29/77} & {13/34} & {37/99} & {29/80} & {10/27} & {31/82} & {13/34} & {26/71} & {\color{red} 31/85} & {16/43} & {11/29} & {13/34} & { 4/11} & {\color{red} 11/30} & {34/91} & {35/92} & {13/34} & {\color{red}  4/11} \\\hline
$29$ & { 2/ 5} & { 1/ 3} & {\color{red} 21/67} & { 5/13} & { 2/ 5} & { 2/ 5} & {14/41} & {\color{red}  1/ 3} & {17/44} & { 2/ 5} & { 2/ 5} & { 8/23} & {27/77} & {19/49} & { 2/ 5} & { 2/ 5} & { 6/17} & {15/41} & { 7/18} & { 2/ 5} & { 2/ 5} & {\color{red}  6/17} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & { 6/17} & { 8/21} & {25/64} & { 2/ 5} & { 2/ 5} & { 1/ 3} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & {26/75} & {28/73} & {29/74} & { 2/ 5} & { 2/ 5} & {19/53} & { 5/13} & {31/79} & { 2/ 5} & { 2/ 5} & {24/65} & {32/83} & {11/28} & { 2/ 5} & { 2/ 5} & {11/29} & {17/44} & {35/89} & { 2/ 5} & { 2/ 5} & {35/92} & {12/31} & {37/94} & { 2/ 5} \\\hline
$30$ & { 7/18} & {12/37} & {\color{red}  4/13} & { 2/ 5} & { 2/ 5} & {16/41} & {\color{red}  1/ 3} & {\color{red} 14/43} & { 2/ 5} & { 2/ 5} & { 9/23} & { 9/26} & {\color{red} 27/79} & { 2/ 5} & { 2/ 5} & {20/51} & {30/83} & {31/89} & { 2/ 5} & { 2/ 5} & {11/28} & { 3/ 8} & {\color{red} 31/89} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & {\color{red} 12/35} & { 2/ 5} & { 2/ 5} & {13/33} & {26/67} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & { 9/26} & { 2/ 5} & { 2/ 5} & {15/38} & {30/77} & {34/95} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {\color{red} 30/83} & { 2/ 5} & { 2/ 5} & {17/43} & {34/87} & {31/82} & { 2/ 5} & { 2/ 5} & {36/91} & { 9/23} & {12/31} & { 2/ 5} & { 2/ 5} \\\hline
$31$ & {14/37} & {\color{red}  6/19} & {13/40} & { 7/18} & { 7/18} & { 8/21} & {26/75} & { 1/ 3} & {29/77} & { 7/18} & {18/47} & { 3/ 8} & {\color{red} 28/81} & {15/41} & { 7/18} & { 5/13} & {20/53} & {\color{red} 32/91} & {\color{red} 31/87} & { 7/18} & {22/57} & {11/29} & {\color{red} 17/48} & {\color{red} 13/37} & { 7/18} & {12/31} & { 8/21} & { 3/ 8} & {13/37} & { 7/18} & {26/67} & {13/34} & {26/69} & { 1/ 3} & { 7/18} & { 7/18} & {28/73} & {14/37} & {\color{red} 32/91} & { 7/18} & { 7/18} & { 5/13} & {30/79} & { 3/ 8} & {35/92} & { 7/18} & {32/83} & { 8/21} & {32/85} & {22/59} & { 7/18} & {17/44} & {34/89} & {17/45} & {15/41} & { 7/18} & {12/31} & {18/47} & {36/95} & { 3/ 8} \\\hline
$32$ & { 7/19} & {23/72} & {24/73} & {14/37} & {14/37} & {16/43} & { 4/11} & { 8/23} & {17/47} & {14/37} & { 3/ 8} & {18/49} & { 6/17} & {19/52} & {14/37} & {20/53} & {10/27} & { 4/11} & { 7/19} & {14/37} & {14/37} & {22/59} & {11/30} & { 7/19} & { 7/19} & {14/37} & { 3/ 8} & {\color{red} 24/65} & { 7/19} & { 7/20} & {14/37} & {26/69} & {\color{red} 13/35} & { 7/19} & { 1/ 3} & {14/37} & {14/37} & {28/75} & { 7/19} & { 4/11} & {14/37} & {14/37} & { 3/ 8} & {10/27} & {15/41} & {\color{red}  4/11} & {14/37} & {32/85} & {16/43} & {32/87} & {23/63} & {14/37} & {17/45} & {34/91} & {17/46} & {\color{red} 34/93} & {14/37} & {14/37} & { 3/ 8} & {\color{red} 36/97} \\\hline
$33$ & { 5/13} & {12/37} & { 8/25} & {16/43} & { 5/13} & { 5/13} & {16/45} & { 7/20} & { 3/ 8} & { 5/13} & {31/83} & { 9/25} & {19/52} & {20/53} & { 5/13} & { 7/19} & { 4/11} & { 7/19} & {11/29} & { 5/13} & { 7/19} & {11/30} & {23/62} & { 8/21} & { 5/13} & { 7/19} & { 7/19} & {25/67} & {13/34} & { 5/13} & {23/64} & { 7/19} & { 3/ 8} & {28/73} & { 5/13} & { 1/ 3} & {\color{red}  7/19} & {29/77} & { 5/13} & { 5/13} & {\color{red} 28/79} & {10/27} & {31/82} & { 5/13} & {\color{red} 31/83} & {31/85} & {16/43} & {11/29} & { 5/13} & {23/61} & {11/30} & {34/91} & {35/92} & { 5/13} & {\color{red} 34/93} & {\color{red}  7/19} & { 3/ 8} & {37/97} & { 5/13} & {\color{red} 18/49} \\\hline
$34$ & { 2/ 5} & {25/76} & {\color{red} 24/77} & {17/44} & { 2/ 5} & { 2/ 5} & { 8/23} & {\color{red} 27/82} & {19/49} & { 2/ 5} & { 2/ 5} & { 6/17} & {\color{red}  9/26} & { 7/18} & { 2/ 5} & { 2/ 5} & { 5/14} & {33/92} & {23/59} & { 2/ 5} & { 2/ 5} & {\color{red} 14/39} & {36/97} & {25/64} & { 2/ 5} & { 2/ 5} & {14/39} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & {14/39} & {28/73} & {29/74} & { 2/ 5} & { 2/ 5} & {\color{red} 32/97} & { 5/13} & {31/79} & { 2/ 5} & { 2/ 5} & {\color{red} 28/81} & {32/83} & {11/28} & { 2/ 5} & { 2/ 5} & {\color{red} 15/43} & {17/44} & {35/89} & { 2/ 5} & { 2/ 5} & {\color{red} 33/92} & {12/31} & {37/94} & { 2/ 5} & { 2/ 5} & {\color{red} 36/97} & {19/49} & {13/33} & { 2/ 5} \\\hline
$35$ & {16/41} & { 1/ 3} & { 7/22} & { 2/ 5} & { 2/ 5} & { 9/23} & {16/47} & {\color{red}  1/ 3} & { 2/ 5} & { 2/ 5} & {20/51} & { 9/26} & {\color{red} 31/89} & { 2/ 5} & { 2/ 5} & {11/28} & {11/31} & {\color{red} 33/94} & { 2/ 5} & { 2/ 5} & {24/61} & {18/49} & {\color{red} 35/99} & { 2/ 5} & { 2/ 5} & {13/33} & {25/66} & {\color{red}  7/20} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & { 7/20} & { 2/ 5} & { 2/ 5} & {15/38} & {30/77} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {\color{red} 15/44} & { 2/ 5} & { 2/ 5} & {17/43} & {34/87} & {\color{red} 11/31} & { 2/ 5} & { 2/ 5} & {36/91} & { 9/23} & {\color{red}  5/14} & { 2/ 5} & { 2/ 5} & {19/48} & {38/97} & {\color{red} 18/49} & { 2/ 5} & { 2/ 5} \\\hline
$36$ & { 8/21} & {14/43} & { 1/ 3} & {16/41} & {16/41} & {18/47} & {\color{red} 29/85} & {17/50} & {11/29} & {16/41} & { 5/13} & {11/30} & {\color{red} 32/91} & {17/46} & {16/41} & {22/57} & {11/29} & {\color{red} 17/48} & {\color{red} 35/97} & {16/41} & {12/31} & { 8/21} & {\color{red} 19/53} & {\color{red}  5/14} & {16/41} & {26/67} & {13/34} & {\color{red} 31/86} & { 5/14} & {16/41} & { 7/18} & {28/73} & {14/37} & { 5/14} & {16/41} & {30/77} & { 5/13} & {30/79} & { 1/ 3} & {16/41} & {16/41} & {32/83} & { 8/21} & {\color{red} 29/85} & {\color{red} 11/29} & {16/41} & {17/44} & {34/89} & {\color{red} 11/30} & {\color{red} 17/46} & {16/41} & {12/31} & {18/47} & {36/95} & {\color{red} 35/97} & {16/41} & {19/49} & {38/99} & {19/50} & {\color{red} 31/87} \\\hline
$37$ & {16/43} & {\color{red}  7/22} & {27/83} & { 8/21} & { 8/21} & { 3/ 8} & {31/87} & { 6/17} & {19/52} & { 8/21} & {20/53} & {10/27} & { 5/14} & { 7/19} & { 8/21} & {11/29} & {22/59} & {22/61} & {23/62} & { 8/21} & { 8/21} & { 3/ 8} & {24/65} & {16/43} & { 8/21} & { 8/21} & {26/69} & {13/35} & {16/43} & { 4/11} & { 8/21} & {14/37} & {\color{red} 28/75} & {16/43} & { 8/23} & { 8/21} & {30/79} & {\color{red}  3/ 8} & {16/43} & { 1/ 3} & { 8/21} & { 8/21} & {32/85} & {16/43} & {\color{red} 31/87} & { 8/21} & { 8/21} & {17/45} & {34/91} & {17/46} & {\color{red} 23/63} & { 8/21} & {36/95} & { 3/ 8} & {36/97} & {\color{red} 26/71} & { 8/21} & {19/50} & {35/93} & {19/51} \\\hline
$38$ & {17/44} & { 9/28} & {\color{red} 27/85} & { 3/ 8} & {17/44} & {17/44} & { 9/25} & {31/90} & {20/53} & {17/44} & {35/93} & { 4/11} & { 7/19} & {11/29} & {17/44} & {16/43} & {11/30} & {23/62} & { 8/21} & {17/44} & {16/43} & {24/65} & {25/67} & {13/34} & {17/44} & {16/43} & {13/35} & { 3/ 8} & {28/73} & {17/44} & {16/43} & {16/43} & {29/77} & { 5/13} & {17/44} & {21/59} & {16/43} & {31/82} & {32/83} & {17/44} & {\color{red} 31/95} & {\color{red} 16/43} & {11/29} & {17/44} & {17/44} & {\color{red} 32/89} & {34/91} & {35/92} & {17/44} & {\color{red} 35/93} & { 7/19} & { 3/ 8} & {37/97} & {17/44} & {\color{red} 18/49} & {27/73} & {35/93} & {13/34} & {17/44} & {\color{red} 31/84} \\\hline
$39$ & { 2/ 5} & {14/43} & {\color{red}  5/16} & {19/49} & { 2/ 5} & { 2/ 5} & { 6/17} & {\color{red} 31/92} & { 7/18} & { 2/ 5} & { 2/ 5} & { 5/14} & {20/57} & {23/59} & { 2/ 5} & { 2/ 5} & {22/61} & {\color{red} 11/31} & {25/64} & { 2/ 5} & { 2/ 5} & { 4/11} & {35/96} & { 9/23} & { 2/ 5} & { 2/ 5} & {\color{red}  4/11} & { 3/ 8} & {29/74} & { 2/ 5} & { 2/ 5} & { 4/11} & { 5/13} & {31/79} & { 2/ 5} & { 2/ 5} & { 4/11} & {32/83} & {11/28} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {17/44} & {35/89} & { 2/ 5} & { 2/ 5} & {\color{red} 32/91} & {12/31} & {37/94} & { 2/ 5} & { 2/ 5} & {\color{red} 17/48} & {19/49} & {13/33} & { 2/ 5} & { 2/ 5} & {\color{red} 31/87} & {33/85} & {28/71} & { 2/ 5} \\\hline
$40$ & { 9/23} & {29/88} & {16/49} & { 2/ 5} & { 2/ 5} & {20/51} & { 9/26} & {\color{red} 16/47} & { 2/ 5} & { 2/ 5} & {11/28} & {\color{red} 20/57} & {\color{red} 10/29} & { 2/ 5} & { 2/ 5} & {24/61} & {\color{red} 11/31} & {\color{red} 21/59} & { 2/ 5} & { 2/ 5} & {13/33} & {13/36} & {\color{red} 34/95} & { 2/ 5} & { 2/ 5} & {28/71} & {29/78} & {\color{red} 32/89} & { 2/ 5} & { 2/ 5} & {15/38} & {37/97} & {\color{red} 16/45} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {16/45} & { 2/ 5} & { 2/ 5} & {17/43} & {34/87} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {36/91} & { 9/23} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {19/48} & {38/97} & {\color{red} 29/83} & { 2/ 5} & { 2/ 5} & {21/53} & {20/51} & {\color{red} 13/36} & { 2/ 5} & { 2/ 5} \\\hline
$41$ & {18/47} & { 1/ 3} & {\color{red}  8/25} & { 9/23} & { 9/23} & { 5/13} & {\color{red} 18/53} & {19/55} & {37/97} & { 9/23} & {22/57} & { 9/25} & {\color{red}  7/20} & {19/51} & { 9/23} & {12/31} & { 8/21} & {\color{red} 19/53} & {\color{red} 35/96} & { 9/23} & {26/67} & {13/34} & {\color{red} 31/86} & {\color{red} 17/47} & { 9/23} & { 7/18} & {28/73} & {\color{red}  4/11} & {\color{red} 17/47} & { 9/23} & {30/77} & { 5/13} & {\color{red}  4/11} & {17/47} & { 9/23} & {16/41} & {32/83} & { 8/21} & {\color{red}  8/23} & { 9/23} & {34/87} & {17/44} & {34/89} & {\color{red}  1/99} & { 9/23} & { 9/23} & {12/31} & {18/47} & {\color{red} 11/32} & {\color{red} 37/97} & { 9/23} & {19/49} & {38/99} & {\color{red}  4/11} & {\color{red} 19/51} & {\color{red} 34/87} & {33/85} & { 5/13} & { 8/21} & {\color{red} 35/96} \\\hline
$42$ & { 3/ 8} & {16/49} & {10/31} & {18/47} & {18/47} & {20/53} & {34/97} & { 5/14} & { 7/19} & {18/47} & {11/29} & {22/59} & {22/61} & {23/62} & {18/47} & { 8/21} & { 3/ 8} & { 4/11} & {25/67} & {18/47} & {13/34} & {26/69} & {\color{red} 26/71} & { 3/ 8} & {18/47} & {18/47} & {14/37} & {28/75} & { 3/ 8} & { 3/ 8} & {18/47} & {30/79} & {\color{red}  3/ 8} & { 3/ 8} & { 9/25} & {18/47} & { 8/21} & {\color{red} 32/85} & { 3/ 8} & {\color{red}  9/26} & {18/47} & {34/89} & {\color{red} 17/45} & { 3/ 8} & {\color{red}  1/99} & {18/47} & {18/47} & {36/95} & { 3/ 8} & { 5/14} & {\color{red}  3/ 8} & {18/47} & {19/50} & {35/93} & {19/51} & {\color{red} 19/52} & {\color{red} 31/81} & { 8/21} & {20/53} & {37/99} \\\hline
$43$ & {19/49} & {\color{red}  8/25} & {\color{red}  6/19} & {20/53} & {19/49} & {19/49} & { 4/11} & {\color{red} 17/50} & {11/29} & {19/49} & {25/66} & {11/30} & {21/58} & { 8/21} & {19/49} & { 3/ 8} & {24/65} & {25/67} & {13/34} & {19/49} & { 3/ 8} & {13/35} & { 3/ 8} & {28/73} & {19/49} & { 3/ 8} & {28/75} & {29/77} & { 5/13} & {19/49} & { 3/ 8} & { 3/ 8} & {31/82} & {32/83} & {19/49} & { 3/ 8} & { 3/ 8} & {11/29} & {17/44} & {19/49} & {\color{red} 26/75} & { 3/ 8} & {35/92} & {12/31} & {19/49} & {\color{red}  1/99} & {\color{red}  3/ 8} & {37/97} & {19/49} & {19/49} & { 4/11} & {35/93} & {13/34} & {\color{red} 31/80} & {\color{red} 25/66} & {\color{red} 19/52} & {20/53} & {23/60} & {\color{red} 31/80} & {\color{red} 10/27} \\\hline
$44$ & { 2/ 5} & {31/96} & {17/53} & { 7/18} & { 2/ 5} & { 2/ 5} & { 5/14} & {\color{red}  1/ 3} & {23/59} & { 2/ 5} & { 2/ 5} & {22/61} & {\color{red} 28/81} & {25/64} & { 2/ 5} & { 2/ 5} & { 4/11} & {\color{red} 24/67} & { 9/23} & { 2/ 5} & { 2/ 5} & {26/71} & {\color{red} 13/36} & {29/74} & { 2/ 5} & { 2/ 5} & {\color{red} 18/49} & {31/84} & {31/79} & { 2/ 5} & { 2/ 5} & {18/49} & {\color{red} 31/83} & {11/28} & { 2/ 5} & { 2/ 5} & {18/49} & {17/44} & {35/89} & { 2/ 5} & { 2/ 5} & {\color{red} 25/71} & {12/31} & {37/94} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {19/49} & {13/33} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {33/85} & {28/71} & { 2/ 5} & { 2/ 5} & {\color{red} 19/53} & { 7/18} & {28/71} & { 2/ 5} \\\hline
$45$ & {20/51} & {16/49} & { 1/ 3} & { 2/ 5} & { 2/ 5} & {11/28} & {20/57} & {\color{red} 20/59} & { 2/ 5} & { 2/ 5} & {24/61} & {11/31} & {\color{red} 22/63} & { 2/ 5} & { 2/ 5} & {13/33} & {24/67} & {\color{red}  6/17} & { 2/ 5} & { 2/ 5} & {28/71} & {\color{red}  9/25} & {\color{red} 32/89} & { 2/ 5} & { 2/ 5} & {15/38} & {\color{red} 15/41} & {\color{red} 33/91} & { 2/ 5} & { 2/ 5} & {32/81} & {\color{red} 32/87} & {\color{red}  9/25} & { 2/ 5} & { 2/ 5} & {17/43} & {\color{red} 11/29} & {\color{red}  9/25} & { 2/ 5} & { 2/ 5} & {36/91} & { 9/23} & { 9/25} & { 2/ 5} & { 2/ 5} & {19/48} & {38/97} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {21/53} & {20/51} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {21/53} & {31/79} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} \\\hline
$46$ & { 5/13} & {\color{red} 17/53} & {\color{red} 25/78} & {20/51} & {20/51} & {22/57} & {10/29} & { 7/20} & {23/60} & {20/51} & {12/31} & {\color{red} 22/63} & {23/65} & { 3/ 8} & {20/51} & {26/67} & {37/99} & {\color{red} 21/58} & {\color{red} 25/68} & {20/51} & { 7/18} & {28/73} & {\color{red} 21/58} & {\color{red} 19/52} & {20/51} & {30/77} & { 5/13} & {\color{red}  4/11} & {\color{red} 19/52} & {20/51} & {16/41} & {32/83} & {\color{red} 23/63} & {19/52} & {20/51} & {34/87} & {17/44} & {\color{red} 19/52} & {19/52} & {20/51} & { 9/23} & {12/31} & {18/47} & {\color{red}  6/17} & {20/51} & {38/97} & {19/49} & {38/99} & {\color{red}  1/99} & {20/51} & {20/51} & {33/85} & { 5/13} & {\color{red}  1/99} & {\color{red} 23/60} & {\color{red} 29/74} & { 7/18} & {37/96} & {\color{red} 28/79} & {\color{red}  3/ 8} \\\hline
$47$ & {20/53} & { 1/ 3} & {\color{red} 28/89} & { 5/13} & { 5/13} & {11/29} & {\color{red} 28/81} & {19/54} & {23/62} & { 5/13} & { 8/21} & { 3/ 8} & { 4/11} & {25/67} & { 5/13} & {13/34} & {26/69} & {26/71} & { 3/ 8} & { 5/13} & {28/73} & {14/37} & { 7/19} & {29/77} & { 5/13} & { 5/13} & {30/79} & { 3/ 8} & {20/53} & { 5/13} & { 5/13} & { 8/21} & {32/85} & {20/53} & {\color{red} 29/79} & { 5/13} & {34/89} & {\color{red} 17/45} & {20/53} & {\color{red} 13/37} & { 5/13} & {18/47} & {\color{red} 36/95} & {20/53} & {\color{red}  1/99} & { 5/13} & {38/99} & {\color{red} 19/50} & {20/53} & {\color{red}  1/99} & { 5/13} & { 5/13} & { 8/21} & {20/53} & {\color{red} 19/54} & {\color{red} 29/79} & { 5/13} & {21/55} & {14/37} & { 3/ 8} \\\hline
$48$ & { 7/18} & {18/55} & {\color{red}  6/19} & {11/29} & { 7/18} & {\color{red} 25/66} & {34/95} & {\color{red} 33/98} & { 8/21} & { 7/18} & {35/92} & {24/65} & {31/87} & {13/34} & { 7/18} & {26/69} & {13/35} & { 3/ 8} & {28/73} & { 7/18} & {20/53} & {28/75} & {29/77} & { 5/13} & { 7/18} & {20/53} & { 3/ 8} & {31/82} & {32/83} & { 7/18} & {20/53} & {32/85} & {11/29} & {17/44} & { 7/18} & {20/53} & {20/53} & {35/92} & {12/31} & { 7/18} & {\color{red} 19/53} & {20/53} & {37/97} & {19/49} & { 7/18} & {\color{red} 18/53} & {20/53} & {13/34} & {33/85} & { 7/18} & {\color{red}  1/99} & {\color{red} 20/53} & {23/60} & { 7/18} & { 7/18} & {\color{red} 34/95} & {14/37} & {38/99} & {\color{red} 33/85} & {\color{red} 35/92} \\\hline
$49$ & { 2/ 5} & {\color{red}  9/28} & {19/58} & {23/59} & { 2/ 5} & { 2/ 5} & {22/61} & {\color{red} 19/56} & {25/64} & { 2/ 5} & { 2/ 5} & { 4/11} & {\color{red} 34/97} & { 9/23} & { 2/ 5} & { 2/ 5} & {26/71} & {\color{red} 13/36} & {29/74} & { 2/ 5} & { 2/ 5} & { 7/19} & {\color{red}  4/11} & {31/79} & { 2/ 5} & { 2/ 5} & {10/27} & {\color{red} 15/41} & {11/28} & { 2/ 5} & { 2/ 5} & {\color{red} 10/27} & {\color{red} 32/87} & {35/89} & { 2/ 5} & { 2/ 5} & {10/27} & {\color{red} 35/93} & {37/94} & { 2/ 5} & { 2/ 5} & {10/27} & {19/49} & {13/33} & { 2/ 5} & { 2/ 5} & {\color{red} 19/55} & {33/85} & {28/71} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & { 7/18} & {28/71} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {37/95} & {15/38} & { 2/ 5} \\\hline
$50$ & {11/28} & {\color{red} 29/91} & {\color{red} 19/59} & { 2/ 5} & { 2/ 5} & {24/61} & {11/31} & {11/32} & { 2/ 5} & { 2/ 5} & {13/33} & {24/67} & {\color{red}  6/17} & { 2/ 5} & { 2/ 5} & {28/71} & {13/36} & {\color{red} 26/73} & { 2/ 5} & { 2/ 5} & {15/38} & { 4/11} & {\color{red} 14/39} & { 2/ 5} & { 2/ 5} & {32/81} & {\color{red}  4/11} & {\color{red} 30/83} & { 2/ 5} & { 2/ 5} & {17/43} & {\color{red} 17/46} & {\color{red}  4/11} & { 2/ 5} & { 2/ 5} & {36/91} & {\color{red} 36/97} & {\color{red}  4/11} & { 2/ 5} & { 2/ 5} & {19/48} & {\color{red} 37/97} & { 4/11} & { 2/ 5} & { 2/ 5} & {21/53} & {20/51} & { 4/11} & { 2/ 5} & { 2/ 5} & {21/53} & {31/79} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {23/58} & {11/28} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} \\\hline
$51$ & {22/57} & {\color{red} 26/81} & {12/37} & {\color{red} 23/60} & {11/28} & {12/31} & {22/63} & {23/65} & {\color{red}  3/ 8} & {11/28} & {26/67} & {\color{red}  6/17} & { 5/14} & {\color{red} 25/68} & {11/28} & { 7/18} & {\color{red}  4/11} & {\color{red}  9/25} & {\color{red} 27/73} & {11/28} & {30/77} & { 5/13} & {\color{red} 29/80} & {\color{red}  7/19} & {11/28} & {16/41} & {32/83} & {\color{red} 26/71} & { 7/19} & {11/28} & {34/87} & {17/44} & {\color{red} 11/30} & {\color{red}  7/19} & {11/28} & { 9/23} & {12/31} & {\color{red}  7/19} & { 7/19} & {11/28} & {38/97} & {19/49} & {\color{red} 29/79} & { 7/19} & {11/28} & {20/51} & {33/85} & { 5/13} & {\color{red}  1/99} & {11/28} & {31/79} & { 7/18} & {37/96} & {\color{red}  1/99} & {11/28} & {11/28} & {37/95} & {22/57} & {\color{red}  1/99} & {\color{red}  5/13} \\\hline
$52$ & {11/29} & {\color{red} 19/59} & {\color{red}  5/16} & {\color{red}  3/ 8} & {22/57} & { 8/21} & {\color{red} 11/32} & {\color{red} 29/85} & {25/67} & {22/57} & {13/34} & {\color{red} 25/69} & {26/71} & { 3/ 8} & {22/57} & {28/73} & {14/37} & { 7/19} & {29/77} & {22/57} & { 5/13} & {30/79} & {10/27} & {31/82} & {22/57} & {32/83} & { 8/21} & {16/43} & {11/29} & {22/57} & {\color{red} 37/96} & {34/89} & {17/45} & {11/29} & {11/29} & {22/57} & {18/47} & {36/95} & {11/29} & {\color{red} 34/97} & {22/57} & {38/99} & {\color{red} 19/50} & {\color{red} 14/37} & {\color{red} 29/83} & {22/57} & { 5/13} & {\color{red}  8/21} & {\color{red} 14/37} & {\color{red}  1/99} & {22/57} & {37/96} & {\color{red} 21/55} & {11/29} & {\color{red}  1/99} & {22/57} & {22/57} & {31/81} & {11/29} & {\color{red}  1/99} \\\hline
$53$ & {23/59} & { 1/ 3} & {10/31} & { 8/21} & {23/59} & {\color{red} 35/92} & {\color{red}  8/23} & {\color{red}  1/ 3} & {13/34} & {23/59} & {\color{red} 26/69} & {13/35} & {\color{red} 26/75} & {28/73} & {23/59} & {14/37} & {28/75} & {\color{red}  4/11} & { 5/13} & {23/59} & {11/29} & { 3/ 8} & {31/82} & {32/83} & {23/59} & {11/29} & {32/85} & {11/29} & {17/44} & {23/59} & {11/29} & {17/45} & {35/92} & {12/31} & {23/59} & {\color{red} 36/95} & {36/95} & {37/97} & {19/49} & {23/59} & {\color{red}  9/25} & {11/29} & {13/34} & {33/85} & {23/59} & {\color{red} 12/35} & {11/29} & {23/60} & { 7/18} & {\color{red} 37/95} & {\color{red}  1/99} & {11/29} & {38/99} & {37/95} & {23/59} & {\color{red}  1/99} & {\color{red} 11/29} & { 5/13} & {23/59} & {23/59} \\\hline
$54$ & { 2/ 5} & {20/61} & { 1/ 3} & {25/64} & { 2/ 5} & { 2/ 5} & { 4/11} & {\color{red} 23/68} & { 9/23} & { 2/ 5} & { 2/ 5} & {26/71} & {\color{red} 28/79} & {29/74} & { 2/ 5} & { 2/ 5} & { 7/19} & { 4/11} & {31/79} & { 2/ 5} & { 2/ 5} & {10/27} & {\color{red} 15/41} & {11/28} & { 2/ 5} & { 2/ 5} & {16/43} & {\color{red} 32/87} & {35/89} & { 2/ 5} & { 2/ 5} & {\color{red} 19/51} & {\color{red} 17/46} & {37/94} & { 2/ 5} & { 2/ 5} & {22/59} & {\color{red} 36/97} & {13/33} & { 2/ 5} & { 2/ 5} & {22/59} & {\color{red} 25/66} & {28/71} & { 2/ 5} & { 2/ 5} & {22/59} & { 7/18} & {28/71} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {37/95} & {15/38} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {23/59} & {32/81} & { 2/ 5} \\\hline
$55$ & {24/61} & {\color{red} 10/31} & {\color{red} 28/87} & { 2/ 5} & { 2/ 5} & {13/33} & {24/67} & { 8/23} & { 2/ 5} & { 2/ 5} & {28/71} & {13/36} & {\color{red} 31/87} & { 2/ 5} & { 2/ 5} & {15/38} & { 4/11} & {\color{red} 14/39} & { 2/ 5} & { 2/ 5} & {32/81} & {15/41} & {\color{red} 30/83} & { 2/ 5} & { 2/ 5} & {17/43} & {\color{red} 11/30} & {\color{red}  4/11} & { 2/ 5} & { 2/ 5} & {36/91} & {\color{red} 34/93} & {\color{red} 34/93} & { 2/ 5} & { 2/ 5} & {19/48} & {\color{red} 19/51} & {\color{red} 11/30} & { 2/ 5} & { 2/ 5} & {21/53} & {\color{red} 37/99} & {\color{red} 11/30} & { 2/ 5} & { 2/ 5} & {21/53} & {\color{red} 23/60} & {\color{red} 34/95} & { 2/ 5} & { 2/ 5} & {23/58} & {11/28} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {23/58} & {35/89} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} \\\hline
$56$ & {12/31} & {\color{red} 13/40} & {\color{red}  1/99} & {\color{red} 25/66} & {24/61} & {26/67} & { 6/17} & { 5/14} & {\color{red} 25/68} & {24/61} & { 7/18} & {\color{red} 26/73} & { 9/25} & {\color{red} 27/73} & {\color{red} 35/89} & {30/77} & {\color{red} 14/39} & {29/80} & {\color{red} 10/27} & {\color{red} 35/89} & {16/41} & {\color{red} 31/83} & {\color{red} 31/85} & {\color{red} 27/73} & {24/61} & {34/87} & {17/44} & {\color{red} 11/30} & {23/62} & {24/61} & { 9/23} & {12/31} & {\color{red}  7/19} & {\color{red} 27/73} & {24/61} & {38/97} & {19/49} & {\color{red} 27/73} & {23/62} & {\color{red} 35/89} & {20/51} & {33/85} & {\color{red}  7/19} & {\color{red} 21/58} & {24/61} & {31/79} & { 7/18} & {\color{red} 27/73} & {\color{red} 31/86} & {24/61} & {11/28} & {37/95} & {22/57} & {\color{red}  1/99} & {24/61} & {35/89} & {23/59} & {29/75} & {\color{red}  1/99} & {\color{red} 29/90} \\\hline
$57$ & { 8/21} & {\color{red} 10/31} & {\color{red}  1/99} & {12/31} & {12/31} & {13/34} & { 8/23} & {\color{red} 19/56} & { 3/ 8} & {12/31} & {28/73} & {\color{red} 34/95} & { 7/19} & {29/77} & {12/31} & { 5/13} & {30/79} & {10/27} & {31/82} & {12/31} & {32/83} & { 8/21} & {16/43} & {11/29} & {12/31} & {17/44} & {34/89} & {34/91} & {35/92} & {12/31} & {12/31} & {18/47} & {\color{red}  3/ 8} & { 8/21} & {12/31} & {\color{red} 29/75} & {38/99} & {19/50} & { 8/21} & {\color{red}  6/17} & {12/31} & { 5/13} & { 8/21} & { 8/21} & {\color{red} 23/65} & {12/31} & {37/96} & {\color{red} 21/55} & {\color{red} 27/71} & {\color{red}  1/99} & {\color{red} 29/75} & {22/57} & {\color{red} 31/81} & {\color{red} 27/71} & {\color{red}  1/99} & {12/31} & {29/75} & {\color{red} 23/60} & { 8/21} & {\color{red}  1/99} \\\hline
$58$ & {25/64} & {\color{red} 21/65} & {\color{red}  1/ 5} & {13/34} & {\color{red} 16/41} & {\color{red} 34/89} & {\color{red} 15/43} & {\color{red}  1/ 3} & {28/73} & {\color{red} 16/41} & {\color{red} 14/37} & {28/75} & {\color{red} 13/38} & { 5/13} & {\color{red} 16/41} & {30/79} & { 3/ 8} & {\color{red} 31/86} & {32/83} & {\color{red} 23/59} & { 8/21} & {32/85} & {11/29} & {17/44} & {\color{red}  7/18} & { 8/21} & {17/45} & {35/92} & {12/31} & {25/64} & { 8/21} & {36/95} & {37/97} & {19/49} & {\color{red} 16/41} & { 8/21} & {19/50} & {13/34} & {33/85} & {25/64} & { 8/21} & { 8/21} & {23/60} & { 7/18} & {\color{red} 16/41} & {\color{red} 28/79} & {\color{red} 27/71} & {38/99} & {37/95} & {\color{red} 23/59} & {\color{red}  8/23} & { 8/21} & { 5/13} & {23/59} & {\color{red} 16/41} & {\color{red}  1/99} & { 8/21} & {37/96} & {16/41} & {25/64} \\\hline
$59$ & { 2/ 5} & { 1/ 3} & {\color{red}  1/99} & { 9/23} & { 2/ 5} & { 2/ 5} & {\color{red} 25/71} & {\color{red} 25/73} & {29/74} & { 2/ 5} & { 2/ 5} & { 7/19} & {\color{red}  9/26} & {31/79} & { 2/ 5} & { 2/ 5} & {10/27} & {\color{red} 11/31} & {11/28} & { 2/ 5} & { 2/ 5} & {16/43} & {32/87} & {35/89} & { 2/ 5} & { 2/ 5} & {34/91} & {\color{red} 17/46} & {37/94} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {\color{red} 36/97} & {13/33} & { 2/ 5} & { 2/ 5} & {\color{red}  3/ 8} & {\color{red} 19/51} & {28/71} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {\color{red} 37/99} & {28/71} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {\color{red} 35/92} & {15/38} & { 2/ 5} & { 2/ 5} & {\color{red} 35/99} & {23/59} & {32/81} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {16/41} & {32/81} & { 2/ 5} \\\hline
$60$ & {13/33} & {\color{red} 22/67} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {28/71} & {13/36} & {13/37} & { 2/ 5} & { 2/ 5} & {15/38} & { 4/11} & {\color{red} 28/79} & { 2/ 5} & { 2/ 5} & {32/81} & {15/41} & {\color{red} 30/83} & { 2/ 5} & { 2/ 5} & {17/43} & {32/87} & {\color{red}  4/11} & { 2/ 5} & { 2/ 5} & {36/91} & {\color{red} 31/84} & {\color{red} 34/93} & { 2/ 5} & { 2/ 5} & {19/48} & {\color{red} 24/65} & {\color{red} 18/49} & { 2/ 5} & { 2/ 5} & {21/53} & {\color{red} 31/84} & {\color{red} 31/84} & { 2/ 5} & { 2/ 5} & {21/53} & {\color{red}  3/ 8} & {\color{red}  7/19} & { 2/ 5} & { 2/ 5} & {23/58} & {\color{red} 35/93} & {\color{red}  7/19} & { 2/ 5} & { 2/ 5} & {23/58} & {\color{red}  5/13} & {\color{red}  6/17} & { 2/ 5} & { 2/ 5} & {25/63} & {24/61} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 3, 3+k, 3+k+i\}$.
\end{center}


==> tables/table-g4-a02b04.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & {\color{red}  7/26} & { 1/ 3} & { 1/ 3} & {\color{red}  2/ 7} & { 1/ 3} & { 1/ 3} & {\color{red}  9/32} & { 1/ 3} & { 1/ 3} & {\color{red}  2/ 7} & { 1/ 3} & { 1/ 3} & {\color{red}  9/31} & { 1/ 3} & { 1/ 3} & {\color{red}  5/17} & { 1/ 3} & { 1/ 3} & {\color{red} 11/37} & { 1/ 3} & { 1/ 3} & {\color{red}  3/10} & { 1/ 3} & { 1/ 3} & {\color{red} 13/43} & { 1/ 3} & { 1/ 3} & {\color{red}  7/23} & { 1/ 3} & { 1/ 3} & {\color{red} 15/49} & { 1/ 3} & { 1/ 3} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & {\color{red} 17/55} & { 1/ 3} & { 1/ 3} & {\color{red}  9/29} & { 1/ 3} & { 1/ 3} & {\color{red} 19/61} & { 1/ 3} & { 1/ 3} & {\color{red}  5/16} & { 1/ 3} & { 1/ 3} & {\color{red} 21/67} & { 1/ 3} & { 1/ 3} \\\hline
$2$ & { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} && { 1/ 4} &\\\hline
$3$ & { 1/ 3} & { 3/11} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} \\\hline
$4$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$5$ & { 1/ 3} & { 4/13} & { 2/ 7} & { 5/17} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/19} & { 3/10} & { 7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 8/25} & { 4/13} & { 9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {10/31} & { 5/16} & {11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & {13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & { 7/22} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 8/25} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {11/34} & {23/71} & { 1/ 3} & { 1/ 3} \\\hline
$6$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$7$ & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & {\color{red} 11/38} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red} 13/44} & { 1/ 3} & { 1/ 3} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & {\color{red}  3/10} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red} 17/56} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red} 19/62} & { 1/ 3} & { 1/ 3} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & {\color{red} 17/55} & { 1/ 3} & { 1/ 3} & {\color{red}  9/29} & { 1/ 3} & { 1/ 3} & {\color{red} 19/61} & { 1/ 3} & { 1/ 3} & {\color{red}  5/16} & { 1/ 3} & { 1/ 3} & {\color{red} 21/67} & { 1/ 3} & { 1/ 3} & {\color{red} 11/35} & { 1/ 3} & { 1/ 3} & {\color{red} 23/73} & { 1/ 3} & { 1/ 3} \\\hline
$8$ & { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} && { 2/ 7} &\\\hline
$9$ & { 1/ 3} & { 5/17} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} \\\hline
$10$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$11$ & { 1/ 3} & { 6/19} & {\color{red}  5/17} & { 7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 8/25} & { 4/13} & { 9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {10/31} & { 5/16} & {11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & {13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & { 7/22} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 8/25} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {11/34} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {12/37} & {25/77} & { 1/ 3} & { 1/ 3} \\\hline
$12$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$13$ & { 3/10} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {17/56} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {\color{red} 19/62} & { 1/ 3} & { 1/ 3} & {\color{red}  6/19} & { 1/ 3} & { 1/ 3} & {\color{red} 21/68} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {\color{red} 23/74} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {\color{red}  5/16} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {\color{red} 27/86} & { 1/ 3} & { 1/ 3} & {\color{red}  6/19} & { 1/ 3} & { 1/ 3} & {\color{red} 29/92} & { 1/ 3} & { 1/ 3} & {\color{red}  6/19} & { 1/ 3} & { 1/ 3} & {\color{red} 25/79} & { 1/ 3} & { 1/ 3} \\\hline
$14$ & { 3/10} && { 3/10} && { 3/10} && {\color{red}  8/27} && { 3/10} && { 3/10} && { 3/10} && { 3/10} && {\color{red} 11/37} && { 3/10} && { 3/10} && { 3/10} && { 3/10} && {\color{red} 14/47} && { 3/10} && { 3/10} && { 3/10} && { 3/10} && {\color{red} 17/57} && { 3/10} && { 3/10} && { 3/10} && { 3/10} && {\color{red} 20/67} && { 3/10} && { 3/10} && { 3/10} && { 3/10} && {\color{red} 23/77} && { 3/10} &\\\hline
$15$ & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} \\\hline
$16$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$17$ & { 1/ 3} & { 8/25} & {\color{red}  7/23} & { 9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {10/31} & {\color{red}  7/23} & {11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & {13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & { 7/22} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 8/25} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {11/34} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {12/37} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {13/40} & {27/83} & { 1/ 3} & { 1/ 3} \\\hline
$18$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$19$ & { 4/13} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {19/62} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {21/68} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {23/74} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {\color{red}  5/16} & { 1/ 3} & { 1/ 3} & {\color{red}  8/25} & { 1/ 3} & { 1/ 3} & {\color{red} 27/86} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {\color{red} 29/92} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {\color{red} 31/98} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {\color{red} 20/63} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {\color{red}  7/22} & { 1/ 3} & { 1/ 3} \\\hline
$20$ & { 4/13} && { 4/13} && { 4/13} && {\color{red} 10/33} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && {\color{red} 15/49} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && {\color{red} 18/59} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && {\color{red} 23/75} && { 4/13} && { 4/13} && { 4/13} && { 4/13} && {\color{red} 26/85} &\\\hline
$21$ & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} \\\hline
$22$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$23$ & { 1/ 3} & {10/31} & {\color{red}  9/29} & {11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & {\color{red}  9/29} & {13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & {\color{red}  9/29} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 8/25} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {11/34} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {12/37} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {13/40} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {14/43} & {29/89} & { 1/ 3} & { 1/ 3} \\\hline
$24$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$25$ & { 5/16} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {23/74} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {27/86} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {29/92} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red} 31/98} & { 1/ 3} & { 1/ 3} & {\color{red} 10/31} & { 1/ 3} & { 1/ 3} & {\color{red} 20/63} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red}  7/22} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red} 22/69} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red} 31/97} & { 1/ 3} & { 1/ 3} \\\hline
$26$ & { 5/16} && { 5/16} && { 5/16} && {\color{red}  4/13} && { 5/16} && { 5/16} && {\color{red} 14/45} && { 5/16} && { 5/16} && { 5/16} && { 5/16} && {\color{red} 17/55} && { 5/16} && { 5/16} && {\color{red} 19/61} && { 5/16} && { 5/16} && { 5/16} && { 5/16} && {\color{red} 22/71} && { 5/16} && { 5/16} && {\color{red} 24/77} && { 5/16} && { 5/16} && { 5/16} && { 5/16} && {\color{red}  9/29} && { 5/16} && { 5/16} &\\\hline
$27$ & { 1/ 3} & {11/35} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} \\\hline
$28$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$29$ & { 1/ 3} & {12/37} & {\color{red} 11/35} & {13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {14/43} & {\color{red} 11/35} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & {\color{red} 11/35} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & {\color{red} 11/35} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {10/31} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {11/34} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {12/37} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {13/40} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {14/43} & {29/89} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {30/91} & {15/46} & {31/95} & { 1/ 3} & { 1/ 3} \\\hline
$30$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$31$ & { 6/19} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {27/86} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {29/92} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {31/98} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {20/63} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {\color{red} 22/69} & { 1/ 3} & { 1/ 3} & {\color{red} 12/37} & { 1/ 3} & { 1/ 3} & {\color{red} 31/97} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {\color{red} 25/78} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {\color{red} 31/97} & { 1/ 3} & { 1/ 3} \\\hline
$32$ & { 6/19} && { 6/19} && { 6/19} && {\color{red} 14/45} && { 6/19} && { 6/19} && {\color{red} 16/51} && { 6/19} && { 6/19} && { 6/19} && { 6/19} && { 6/19} && { 6/19} && { 6/19} && {\color{red} 21/67} && { 6/19} && { 6/19} && {\color{red} 23/73} && { 6/19} && { 6/19} && { 6/19} && { 6/19} && {\color{red} 26/83} && { 6/19} && { 6/19} && {\color{red} 28/89} && { 6/19} && { 6/19} && { 6/19} && { 6/19} &\\\hline
$33$ & { 1/ 3} & {13/41} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} \\\hline
$34$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$35$ & { 1/ 3} & {14/43} & {\color{red} 13/41} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & {\color{red} 13/41} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & {\color{red} 13/41} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {\color{red} 13/41} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {\color{red} 13/41} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {12/37} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {13/40} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {14/43} & {29/89} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {30/91} & {15/46} & {31/95} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {16/49} & {17/52} & { 1/ 3} & { 1/ 3} \\\hline
$36$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$37$ & { 7/22} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {31/98} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {20/63} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {22/69} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {31/97} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {25/78} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {\color{red} 25/78} & { 1/ 3} & { 1/ 3} & {\color{red} 14/43} & { 1/ 3} & { 1/ 3} & {\color{red} 26/81} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {\color{red}  9/28} & { 1/ 3} & { 1/ 3} \\\hline
$38$ & { 7/22} && { 7/22} && { 7/22} && {\color{red} 16/51} && { 7/22} && { 7/22} && {\color{red}  6/19} && { 7/22} && { 7/22} && {\color{red} 20/63} && { 7/22} && { 7/22} && { 7/22} && { 7/22} && {\color{red} 23/73} && { 7/22} && { 7/22} && {\color{red} 25/79} && { 7/22} && { 7/22} && {\color{red} 27/85} && { 7/22} && { 7/22} && { 7/22} && {\color{red} 27/85} && {\color{red}  6/19} && { 7/22} && { 7/22} && {\color{red} 19/60} && { 7/22} &\\\hline
$39$ & { 1/ 3} & {15/47} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} \\\hline
$40$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$41$ & { 1/ 3} & {16/49} & {\color{red} 15/47} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & {\color{red} 15/47} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {\color{red} 15/47} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {\color{red} 15/47} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {\color{red} 15/47} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {\color{red} 15/47} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {14/43} & {29/89} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {30/91} & {15/46} & {31/95} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {16/49} & {17/52} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {17/52} & {18/55} & { 1/ 3} & { 1/ 3} \\\hline
$42$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$43$ & { 8/25} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {22/69} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {31/97} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/78} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {26/81} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {\color{red}  9/28} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {\color{red}  9/28} & { 1/ 3} & { 1/ 3} & {\color{red} 31/95} & { 1/ 3} & { 1/ 3} & {\color{red} 26/81} & { 1/ 3} & { 1/ 3} \\\hline
$44$ & { 8/25} && { 8/25} && { 8/25} && {\color{red}  6/19} && { 8/25} && { 8/25} && {\color{red} 20/63} && { 8/25} && { 8/25} && {\color{red} 22/69} && { 8/25} && { 8/25} && { 8/25} && { 8/25} && { 8/25} && { 8/25} && { 8/25} && {\color{red} 27/85} && { 8/25} && { 8/25} && {\color{red} 29/91} && { 8/25} && { 8/25} && {\color{red} 31/97} && { 8/25} && { 8/25} && { 8/25} && { 8/25} && {\color{red} 27/85} && { 8/25} &\\\hline
$45$ & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 9/28} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} \\\hline
$46$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$47$ & { 1/ 3} & {18/55} & {\color{red} 17/53} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & {\color{red} 17/53} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {\color{red} 17/53} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {\color{red} 17/53} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {\color{red} 17/53} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {\color{red} 17/53} & {29/89} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {30/91} & {\color{red} 17/53} & {31/95} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {16/49} & {17/52} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {17/52} & {18/55} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {18/55} & {19/58} & { 1/ 3} & { 1/ 3} \\\hline
$48$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$49$ & { 9/28} & { 1/ 3} & { 1/ 3} & {\color{red} 20/63} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red}  7/22} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {\color{red} 31/97} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {\color{red} 25/78} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {\color{red} 26/81} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {28/87} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {29/90} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {\color{red} 29/90} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {\color{red} 29/90} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {\color{red} 31/96} & { 1/ 3} & { 1/ 3} \\\hline
$50$ & { 9/28} && { 9/28} && { 9/28} && {\color{red} 20/63} && { 9/28} && { 9/28} && {\color{red} 22/69} && { 9/28} && { 9/28} && {\color{red}  8/25} && { 9/28} && { 9/28} && {\color{red} 26/81} && {\color{red} 17/53} && { 9/28} && { 9/28} && { 9/28} && {\color{red} 29/91} && { 9/28} && { 9/28} && {\color{red} 31/97} && { 9/28} && { 9/28} && {\color{red} 25/78} && { 9/28} && { 9/28} && {\color{red} 26/81} && { 9/28} && { 9/28} && {\color{red} 26/81} &\\\hline
$51$ & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & {10/31} & { 1/ 3} & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} \\\hline
$52$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$53$ & { 1/ 3} & {20/61} & {\color{red} 19/59} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {22/67} & {\color{red} 19/59} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {\color{red} 19/59} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {\color{red} 19/59} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {\color{red} 19/59} & {29/89} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {30/91} & {\color{red} 19/59} & {31/95} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {\color{red} 19/59} & {17/52} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {\color{red} 19/59} & {18/55} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {18/55} & {19/58} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {19/58} & {20/61} & { 1/ 3} & { 1/ 3} \\\hline
$54$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$55$ & {10/31} & { 1/ 3} & { 1/ 3} & {\color{red} 21/67} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {\color{red} 31/97} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {\color{red} 25/78} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {\color{red} 26/81} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {\color{red} 29/91} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {\color{red} 28/87} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {\color{red} 31/96} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {\color{red} 26/81} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {\color{red} 28/87} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {\color{red} 11/34} & { 1/ 3} & { 1/ 3} \\\hline
$56$ & {10/31} && {10/31} && {10/31} && {\color{red} 22/69} && {10/31} && {10/31} && {\color{red}  8/25} && {10/31} && {10/31} && {\color{red} 26/81} && {\color{red} 17/53} && {10/31} && {\color{red} 28/87} && {10/31} && {10/31} && {10/31} && {10/31} && {10/31} && {10/31} && {10/31} && {\color{red} 25/78} && {10/31} && {10/31} && {\color{red} 26/81} && {10/31} && {10/31} && {\color{red} 28/87} && {10/31} && {10/31} && {\color{red} 29/90} &\\\hline
$57$ & { 1/ 3} & {21/65} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & {23/71} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & {25/77} & { 1/ 3} & { 1/ 3} & {13/40} & { 1/ 3} & { 1/ 3} & {27/83} & { 1/ 3} & { 1/ 3} & {14/43} & { 1/ 3} & { 1/ 3} & {29/89} & { 1/ 3} & { 1/ 3} & {15/46} & { 1/ 3} & { 1/ 3} & {31/95} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {18/55} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {19/58} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} \\\hline
$58$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
$59$ & { 1/ 3} & {22/67} & {\color{red} 21/65} & {23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {24/73} & {\color{red} 21/65} & {25/77} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {26/79} & {\color{red} 21/65} & {27/83} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {28/85} & {\color{red} 25/78} & {29/89} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {30/91} & {\color{red} 21/65} & {31/95} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {\color{red} 31/96} & {17/52} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {\color{red} 21/65} & {18/55} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {\color{red} 21/65} & {19/58} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {\color{red} 29/90} & {20/61} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {32/97} & {20/61} & {21/64} & { 1/ 3} & { 1/ 3} \\\hline
$60$ & { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} && { 1/ 3} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g4-a02b05.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & {\color{red}  1/ 4} & { 2/ 7} & { 4/11} & { 1/ 3} & {\color{red}  1/ 4} & { 1/ 3} & { 4/11} & { 6/19} & { 3/10} & { 4/11} & { 4/11} & {\color{red}  7/23} & { 8/25} & { 4/11} & { 9/26} & {\color{red}  3/10} & {10/29} & { 4/11} & { 1/ 3} & {10/31} & { 4/11} & { 4/11} & {\color{red} 11/34} & { 1/ 3} & { 4/11} & {13/37} & {\color{red} 10/31} & { 7/20} & { 4/11} & {14/41} & { 1/ 3} & { 4/11} & { 4/11} & {\color{red}  1/ 3} & {16/47} & { 4/11} & {17/48} & {\color{red}  1/ 3} & { 6/17} & { 4/11} & { 9/26} & {18/53} & { 4/11} & { 4/11} & {\color{red} 18/53} & {10/29} & { 4/11} & {21/59} & {\color{red} 18/53} & {11/31} & { 4/11} & {22/63} & {11/32} & { 4/11} & { 4/11} & {\color{red} 11/32} & { 8/23} & { 4/11} & { 5/14} & {\color{red} 23/68} \\\hline
$2$ & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & {\color{red}  9/37} & { 1/ 3} & { 1/ 3} & { 3/11} & { 1/ 3} & { 1/ 3} & { 6/23} & { 1/ 3} & { 1/ 3} & { 7/26} & { 1/ 3} & { 1/ 3} & {\color{red}  8/29} & { 1/ 3} & { 1/ 3} & { 9/32} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & {11/38} & { 1/ 3} & { 1/ 3} & {12/41} & { 1/ 3} & { 1/ 3} & {13/44} & { 1/ 3} & { 1/ 3} & {14/47} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & {16/53} & { 1/ 3} & { 1/ 3} & {17/56} & { 1/ 3} & { 1/ 3} & {18/59} & { 1/ 3} & { 1/ 3} & {19/62} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {21/68} & { 1/ 3} & { 1/ 3} & {22/71} & { 1/ 3} \\\hline
$3$ & { 6/17} & { 1/ 3} & { 5/13} & { 2/ 5} & { 1/ 3} & { 3/ 8} & { 2/ 5} & { 1/ 3} & { 7/19} & { 2/ 5} & {10/27} & { 4/11} & { 9/23} & { 2/ 5} & { 9/25} & { 5/13} & { 2/ 5} & { 5/14} & {11/29} & { 2/ 5} & {14/37} & { 3/ 8} & {13/33} & { 2/ 5} & {13/35} & { 7/18} & { 2/ 5} & { 7/19} & { 5/13} & { 2/ 5} & {18/47} & { 8/21} & {17/43} & { 2/ 5} & {17/45} & { 9/23} & { 2/ 5} & { 3/ 8} & {19/49} & { 2/ 5} & {22/57} & { 5/13} & {21/53} & { 2/ 5} & {21/55} & {11/28} & { 2/ 5} & {11/29} & {23/59} & { 2/ 5} & {26/67} & {12/31} & {25/63} & { 2/ 5} & { 5/13} & {13/33} & { 2/ 5} & {\color{red} 13/34} & { 9/23} & { 2/ 5} \\\hline
$4$ & { 1/ 3} & { 3/10} & { 3/ 7} & { 7/18} & { 6/19} & { 3/ 8} & { 3/ 7} & { 4/11} & { 1/ 3} & { 3/ 7} & { 2/ 5} & { 9/26} & {12/31} & { 3/ 7} & {11/29} & { 6/17} & { 3/ 7} & {13/32} & { 4/11} & {15/38} & { 3/ 7} & { 7/18} & {15/41} & { 3/ 7} & {16/39} & { 3/ 8} & { 2/ 5} & { 3/ 7} & {17/43} & { 3/ 8} & { 3/ 7} & {19/46} & {18/47} & {21/52} & { 3/ 7} & { 2/ 5} & {21/55} & { 3/ 7} & {22/53} & { 7/18} & {24/59} & { 3/ 7} & {23/57} & {12/31} & { 3/ 7} & { 5/12} & {24/61} & { 9/22} & { 3/ 7} & {13/32} & { 9/23} & { 3/ 7} & {28/67} & {27/68} & {30/73} & { 3/ 7} & {29/71} & {15/38} & { 3/ 7} & {31/74} \\\hline
$5$ & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & {\color{red}  7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 11/37} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 21/67} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} \\\hline
$6$ & { 8/23} & { 1/ 3} & { 3/ 8} & { 5/13} & { 1/ 3} & { 7/19} & { 5/13} & { 1/ 3} & { 4/11} & { 5/13} & { 1/ 3} & { 9/25} & { 5/13} & {13/36} & { 5/14} & {11/29} & { 5/13} & {11/31} & { 3/ 8} & { 5/13} & { 6/17} & {13/35} & { 5/13} & {13/37} & { 7/19} & { 5/13} & {18/49} & {15/41} & { 8/21} & { 5/13} & { 4/11} & {17/45} & { 5/13} & {17/47} & { 3/ 8} & { 5/13} & { 9/25} & {19/51} & { 5/13} & {23/62} & {10/27} & {21/55} & { 5/13} & { 7/19} & {11/29} & { 5/13} & {11/30} & {23/61} & { 5/13} & {23/63} & { 3/ 8} & { 5/13} & {28/75} & {25/67} & {13/34} & { 5/13} & {13/35} & {27/71} & { 5/13} & {27/73} \\\hline
$7$ & { 9/25} & { 4/13} & { 7/17} & { 3/ 7} & { 9/29} & { 2/ 5} & { 3/ 7} & { 3/ 8} & { 4/11} & { 5/12} & { 3/ 7} & { 1/ 3} & {11/27} & { 3/ 7} & { 5/13} & { 2/ 5} & {13/31} & { 3/ 7} & {16/43} & { 7/17} & { 3/ 7} & { 9/23} & {15/37} & { 8/19} & { 3/ 7} & { 2/ 5} & {17/41} & { 3/ 7} & {21/53} & { 9/22} & {19/45} & { 3/ 7} & {19/47} & { 5/12} & { 3/ 7} & { 2/ 5} & { 7/17} & {11/26} & { 3/ 7} & {11/27} & {23/55} & { 3/ 7} & {\color{red} 23/57} & {12/29} & {25/59} & { 3/ 7} & {25/61} & {13/31} & { 3/ 7} & {\color{red} 13/32} & {27/65} & {14/33} & { 3/ 7} & { 7/17} & {29/69} & { 3/ 7} & {\color{red} 29/71} & { 5/12} & {31/73} & { 3/ 7} \\\hline
$8$ & { 1/ 3} & {\color{red}  2/ 7} & { 7/18} & { 4/11} & { 7/23} & {11/32} & { 7/18} & { 9/26} & { 1/ 3} & { 7/18} & {11/29} & { 1/ 3} & { 1/ 3} & { 7/18} & { 4/11} & { 1/ 3} & {16/43} & { 7/18} & {13/37} & {15/46} & { 7/18} & { 3/ 8} & {14/41} & { 9/25} & { 7/18} & { 4/11} & {\color{red}  1/ 3} & { 7/18} & {18/47} & {17/48} & {20/57} & { 7/18} & {19/51} & {\color{red}  9/26} & {23/61} & { 7/18} & { 4/11} & {\color{red} 11/32} & { 7/18} & {11/29} & {21/59} & {25/68} & { 7/18} & {23/62} & {\color{red} 22/63} & { 7/18} & { 5/13} & { 4/11} & { 9/25} & { 7/18} & {26/69} & {\color{red}  5/14} & {30/79} & { 7/18} & {27/73} & {\color{red} 29/82} & { 7/18} & {29/76} & { 4/11} & {16/43} \\\hline
$9$ & {10/29} & { 1/ 3} & { 7/19} & { 3/ 8} & { 1/ 3} & { 4/11} & { 3/ 8} & { 1/ 3} & { 9/25} & { 3/ 8} & { 1/ 3} & { 5/14} & { 3/ 8} & { 1/ 3} & {11/31} & { 3/ 8} & {16/45} & { 6/17} & {13/35} & { 3/ 8} & {13/37} & { 7/19} & { 3/ 8} & { 7/20} & {15/41} & { 3/ 8} & {15/43} & { 4/11} & { 3/ 8} & { 8/23} & {17/47} & { 3/ 8} & {22/61} & { 9/25} & {19/51} & { 3/ 8} & {19/53} & {10/27} & { 3/ 8} & { 5/14} & { 7/19} & { 3/ 8} & {21/59} & {11/30} & { 3/ 8} & {11/31} & {23/63} & { 3/ 8} & { 4/11} & { 4/11} & {25/67} & { 3/ 8} & {25/69} & {13/35} & { 3/ 8} & {13/36} & {27/73} & { 3/ 8} & { 9/25} & { 7/19} \\\hline
$10$ & {11/31} & { 5/16} & { 2/ 5} & { 7/17} & { 2/ 7} & { 9/23} & { 7/17} & {13/38} & { 5/13} & {11/27} & {16/41} & { 5/14} & { 2/ 5} & { 7/17} & { 1/ 3} & {13/33} & { 7/17} & { 3/ 8} & { 7/18} & {15/37} & { 7/17} & { 5/13} & { 2/ 5} & { 7/17} & { 4/11} & {17/43} & { 9/22} & {23/58} & { 9/23} & {19/47} & { 7/17} & {19/49} & { 2/ 5} & { 7/17} & { 5/13} & {21/53} & {11/27} & { 7/17} & {11/28} & {23/57} & { 7/17} & {23/59} & { 2/ 5} & {25/61} & { 2/ 5} & {25/63} & {13/32} & { 7/17} & {13/33} & {27/67} & { 7/17} & {\color{red}  9/23} & { 2/ 5} & {29/71} & { 7/17} & {29/73} & {15/37} & { 7/17} & {15/38} & {31/77} \\\hline
$11$ & { 4/11} & {\color{red}  5/17} & { 3/ 7} & { 2/ 5} & {12/37} & { 7/19} & { 3/ 7} & {11/29} & { 1/ 3} & { 3/ 7} & {13/32} & { 4/11} & {17/45} & { 3/ 7} & { 7/18} & { 1/ 3} & { 3/ 7} & {16/39} & { 3/ 8} & { 5/13} & { 3/ 7} & {17/43} & { 4/11} & { 3/ 7} & {19/46} & {18/47} & {23/59} & { 3/ 7} & { 2/ 5} & {19/51} & { 3/ 7} & {22/53} & { 7/18} & {13/33} & { 3/ 7} & {23/57} & {11/29} & { 3/ 7} & { 5/12} & {24/61} & {29/73} & { 3/ 7} & {13/32} & { 5/13} & { 3/ 7} & {28/67} & {27/68} & { 2/ 5} & { 3/ 7} & {29/71} & { 7/18} & { 3/ 7} & {31/74} & { 2/ 5} & {35/87} & { 3/ 7} & {16/39} & {\color{red} 31/79} & { 3/ 7} & {34/81} \\\hline
$12$ & {12/35} & { 1/ 3} & { 4/11} & { 7/19} & { 1/ 3} & { 9/25} & { 7/19} & { 1/ 3} & { 5/14} & { 7/19} & { 4/11} & {11/31} & { 7/19} & { 4/11} & { 6/17} & { 7/19} & { 1/ 3} & { 4/11} & { 7/19} & {19/54} & { 4/11} & {15/41} & { 7/19} & {15/43} & { 4/11} & { 7/19} & { 8/23} & {17/47} & { 7/19} & {\color{red} 17/49} & { 9/25} & { 7/19} & { 4/11} & {19/53} & { 7/19} & { 4/11} & { 5/14} & { 7/19} & {26/73} & { 4/11} & {11/30} & { 7/19} & { 4/11} & {23/63} & { 7/19} & {23/65} & { 4/11} & { 7/19} & { 6/17} & {25/69} & { 7/19} & {\color{red} 25/71} & {13/36} & { 7/19} & { 4/11} & { 9/25} & { 7/19} & { 4/11} & {\color{red} 14/39} & {29/79} \\\hline
$13$ & {13/37} & { 6/19} & { 9/23} & { 2/ 5} & {12/41} & { 5/13} & { 2/ 5} & {\color{red}  7/22} & {11/29} & { 2/ 5} & {17/47} & { 3/ 8} & {13/33} & { 2/ 5} & { 6/17} & { 7/18} & { 2/ 5} & { 1/ 3} & { 5/13} & { 2/ 5} & { 7/19} & { 8/21} & {17/43} & { 2/ 5} & {17/45} & { 9/23} & { 2/ 5} & { 3/ 8} & {19/49} & { 2/ 5} & {25/67} & { 5/13} & {21/53} & { 2/ 5} & {21/55} & {11/28} & { 2/ 5} & {11/29} & {23/59} & { 2/ 5} & {\color{red} 23/61} & {12/31} & {25/63} & { 2/ 5} & { 5/13} & {13/33} & { 2/ 5} & {13/34} & { 9/23} & { 2/ 5} & {\color{red} 27/71} & { 7/18} & {29/73} & { 2/ 5} & {29/75} & {15/38} & { 2/ 5} & { 5/13} & {31/79} & { 2/ 5} \\\hline
$14$ & {14/39} & {\color{red}  3/10} & { 5/12} & { 3/ 7} & {\color{red} 13/43} & {17/44} & { 3/ 7} & {17/46} & {16/47} & {13/31} & { 3/ 7} & { 1/ 3} & { 7/17} & { 3/ 7} & {20/53} & {10/27} & { 8/19} & { 3/ 7} & { 1/ 3} & {17/41} & { 3/ 7} & {23/60} & {24/61} & {19/45} & { 3/ 7} & {23/64} & { 5/12} & { 3/ 7} & {26/67} & { 7/17} & {11/26} & { 3/ 7} & {27/71} & {23/55} & { 3/ 7} & {29/74} & {12/29} & {25/59} & { 3/ 7} & {31/78} & {13/31} & { 3/ 7} & {32/81} & {27/65} & {14/33} & { 3/ 7} & { 7/17} & {29/69} & { 3/ 7} & {35/88} & { 5/12} & {31/73} & { 3/ 7} & {31/75} & { 8/19} & { 3/ 7} & { 2/ 5} & {33/79} & {17/40} & { 3/ 7} \\\hline
$15$ & { 9/26} & { 1/ 3} & { 2/ 5} & {11/29} & { 1/ 3} & { 5/14} & { 2/ 5} & { 4/11} & {11/31} & { 2/ 5} & { 7/18} & { 6/17} & { 4/11} & { 2/ 5} & { 3/ 8} & { 4/11} & {22/57} & {17/43} & { 4/11} & { 1/ 3} & { 2/ 5} & {18/47} & {17/48} & { 3/ 8} & { 2/ 5} & {19/51} & {17/49} & { 2/ 5} & { 7/18} & { 4/11} & {26/71} & { 2/ 5} & {11/29} & { 5/14} & { 2/ 5} & {24/61} & {23/62} & { 4/11} & { 2/ 5} & { 5/13} & { 4/11} & {16/41} & {27/68} & {26/69} & {\color{red}  5/14} & { 2/ 5} & { 7/18} & {27/73} & {34/89} & { 2/ 5} & {29/76} & { 4/11} & { 2/ 5} & {31/79} & { 3/ 8} & { 3/ 8} & { 2/ 5} & {32/83} & {\color{red} 31/84} & { 2/ 5} \\\hline
$16$ & {15/43} & { 7/22} & { 5/13} & { 9/23} & {\color{red} 14/47} & {11/29} & { 9/23} & {\color{red} 20/61} & { 3/ 8} & { 9/23} & {\color{red}  9/26} & {13/35} & { 7/18} & { 3/ 8} & { 7/19} & { 5/13} & { 9/23} & { 7/20} & { 8/21} & { 9/23} & { 1/ 3} & {17/45} & { 9/23} & { 4/11} & { 3/ 8} & {19/49} & { 9/23} & {19/51} & { 5/13} & { 9/23} & {10/27} & {21/55} & { 9/23} & { 7/19} & {11/29} & {23/59} & {30/79} & {23/61} & {12/31} & { 9/23} & { 3/ 8} & { 5/13} & { 9/23} & {25/67} & {13/34} & { 9/23} & {\color{red} 13/35} & {27/71} & { 7/18} & { 9/23} & {14/37} & {29/75} & { 9/23} & {29/77} & { 5/13} & { 9/23} & {\color{red}  3/ 8} & {31/81} & {16/41} & {13/34} \\\hline
$17$ & {16/45} & {\color{red}  7/23} & {11/27} & { 5/12} & {\color{red}  2/ 7} & { 2/ 5} & { 5/12} & { 9/26} & {19/53} & { 7/17} & { 2/ 5} & { 1/ 3} & {15/37} & { 5/12} & {20/59} & { 2/ 5} & {17/41} & {12/31} & {23/63} & { 9/22} & { 5/12} & { 1/ 3} & {19/47} & { 5/12} & {26/69} & { 2/ 5} & { 7/17} & { 5/12} & {27/73} & {11/27} & { 5/12} & { 7/19} & {23/57} & {12/29} & {32/79} & { 2/ 5} & {25/61} & { 5/12} & {31/83} & {13/32} & {27/65} & {17/43} & {27/67} & { 7/17} & { 5/12} & { 2/ 5} & {29/71} & { 5/12} & {12/31} & {15/37} & {31/75} & { 5/12} & {31/77} & {16/39} & { 5/12} & { 2/ 5} & {11/27} & {17/41} & {31/76} & {17/42} \\\hline
$18$ & {17/47} & { 1/ 3} & { 3/ 7} & {13/32} & { 1/ 3} & {19/52} & { 3/ 7} & { 7/18} & { 6/17} & { 3/ 7} & {16/39} & {13/37} & {22/59} & { 3/ 7} & {17/43} & { 9/25} & { 3/ 7} & {19/46} & {24/65} & {25/66} & { 3/ 7} & { 2/ 5} & { 1/ 3} & { 3/ 7} & {22/53} & { 7/18} & {28/73} & { 3/ 7} & {23/57} & {27/76} & { 3/ 7} & { 5/12} & {24/61} & {31/80} & { 3/ 7} & {13/32} & {31/83} & { 3/ 7} & {28/67} & {27/68} & {34/87} & { 3/ 7} & {29/71} & { 7/18} & { 3/ 7} & {31/74} & { 2/ 5} & {37/94} & { 3/ 7} & {16/39} & {31/79} & { 3/ 7} & {34/81} & {33/82} & {21/53} & { 3/ 7} & { 7/17} & {17/43} & { 3/ 7} & {37/88} \\\hline
$19$ & {17/49} & { 8/25} & {11/29} & { 5/13} & {11/34} & { 3/ 8} & { 5/13} & {13/37} & {13/35} & { 5/13} & { 3/ 8} & { 7/19} & { 5/13} & {11/29} & {15/41} & { 8/21} & { 5/13} & {11/29} & {17/45} & { 5/13} & {11/29} & { 3/ 8} & { 5/13} & { 1/ 3} & {11/29} & { 5/13} & { 9/25} & {\color{red} 10/27} & {\color{red} 21/55} & { 5/13} & { 7/19} & {11/29} & { 5/13} & {11/30} & {23/61} & { 5/13} & {\color{red} 23/63} & { 3/ 8} & { 5/13} & {26/69} & {25/67} & {13/34} & { 5/13} & {\color{red} 13/35} & {27/71} & { 5/13} & {11/29} & {14/37} & { 5/13} & {11/29} & {\color{red} 29/77} & { 5/13} & {\color{red} 29/79} & {11/29} & {31/81} & { 5/13} & {\color{red} 31/83} & {\color{red}  8/21} & { 5/13} & {16/43} \\\hline
$20$ & { 6/17} & {\color{red}  4/13} & { 2/ 5} & {11/27} & { 2/ 7} & {13/33} & {11/27} & {10/29} & {22/59} & {15/37} & {23/61} & {21/62} & { 2/ 5} & {11/27} & { 1/ 3} & {17/43} & {11/27} & { 6/17} & { 9/23} & {19/47} & {28/71} & {13/36} & { 2/ 5} & {11/27} & { 1/ 3} & {21/53} & {11/27} & {29/78} & {11/28} & {23/57} & {11/27} & {31/82} & { 2/ 5} & {11/27} & { 6/17} & {25/63} & {13/32} & {17/44} & {13/33} & {27/67} & {11/27} & { 9/23} & { 2/ 5} & {11/27} & { 7/19} & {29/73} & {15/37} & {39/98} & {15/38} & {31/77} & {11/27} & {31/79} & { 2/ 5} & {11/27} & { 8/21} & {33/83} & {17/42} & {11/27} & {17/43} & {35/87} \\\hline
$21$ & {19/53} & { 1/ 3} & {13/31} & { 3/ 7} & { 1/ 3} & {11/29} & { 3/ 7} & {11/30} & {13/37} & { 8/19} & { 3/ 7} & { 7/20} & { 2/ 5} & { 3/ 7} & {25/67} & { 5/14} & {19/45} & { 3/ 7} & { 5/14} & { 5/12} & { 3/ 7} & {14/37} & {28/75} & {11/26} & { 3/ 7} & { 1/ 3} & {23/55} & { 3/ 7} & {31/81} & {16/41} & {25/59} & { 3/ 7} & { 6/17} & {13/31} & { 3/ 7} & {17/44} & {36/89} & {14/33} & { 3/ 7} & {17/46} & {29/69} & { 3/ 7} & {37/95} & { 5/12} & {31/73} & { 3/ 7} & {38/99} & { 8/19} & { 3/ 7} & {20/51} & {33/79} & {17/40} & { 3/ 7} & {21/53} & {35/83} & { 3/ 7} & {28/71} & {18/43} & {37/87} & { 3/ 7} \\\hline
$22$ & { 4/11} & { 9/28} & {13/32} & { 7/18} & {19/59} & {13/35} & {13/32} & { 3/ 8} & { 7/19} & {13/32} & {17/43} & {15/41} & {11/29} & {13/32} & {18/47} & {17/45} & {28/71} & { 2/ 5} & { 3/ 8} & {11/29} & {13/32} & { 7/18} & {11/29} & { 5/13} & {23/57} & {11/29} & { 1/ 3} & {13/32} & {24/61} & {23/62} & {32/85} & {13/32} & { 5/13} & {\color{red} 23/63} & {13/32} & {27/68} & {26/69} & {\color{red} 25/67} & {13/32} & { 7/18} & {\color{red} 13/35} & {13/32} & { 2/ 5} & {29/76} & {14/37} & {13/32} & {31/79} & {\color{red} 29/77} & {39/98} & {33/82} & {32/83} & {11/29} & {13/32} & {17/43} & {11/29} & {\color{red} 32/85} & {36/89} & { 7/18} & {\color{red} 34/91} & {13/32} \\\hline
$23$ & {20/57} & {\color{red}  9/29} & {13/33} & { 2/ 5} & { 6/19} & { 7/18} & { 2/ 5} & {14/41} & { 5/13} & { 2/ 5} & {\color{red}  4/11} & { 6/17} & {17/43} & { 2/ 5} & {17/48} & { 9/23} & { 2/ 5} & { 4/11} & {19/49} & { 2/ 5} & { 4/11} & { 5/13} & {21/53} & { 2/ 5} & { 4/11} & {11/28} & { 2/ 5} & { 1/ 3} & {23/59} & { 2/ 5} & {32/87} & {12/31} & {25/63} & { 2/ 5} & { 5/13} & {13/33} & { 2/ 5} & {17/47} & { 9/23} & { 2/ 5} & {36/97} & { 7/18} & {29/73} & { 2/ 5} & {29/75} & {15/38} & { 2/ 5} & { 5/13} & {31/79} & { 2/ 5} & {37/99} & {16/41} & {33/83} & { 2/ 5} & {33/85} & {17/43} & { 2/ 5} & {17/44} & {35/89} & { 2/ 5} \\\hline
$24$ & {21/59} & { 1/ 3} & { 7/17} & {13/31} & { 1/ 3} & {25/64} & {13/31} & {23/66} & { 7/20} & {17/41} & {28/69} & {15/43} & { 9/22} & {13/31} & { 8/23} & {14/37} & { 5/12} & {15/38} & {11/31} & { 7/17} & {13/31} & {11/31} & {11/27} & {23/55} & {32/83} & {31/84} & {12/29} & {13/31} & { 1/ 3} & {25/61} & {13/31} & {17/45} & {36/91} & {27/65} & {13/31} & {17/47} & { 7/17} & {13/31} & {36/97} & {29/71} & { 5/12} & {25/61} & {22/57} & {31/75} & {13/31} & {19/52} & {16/39} & {33/79} & {39/97} & {11/27} & {17/41} & {13/31} & {14/37} & { 7/17} & {18/43} & {\color{red} 17/45} & { 9/22} & {37/89} & {13/31} & {\color{red} 36/91} \\\hline
$25$ & {22/61} & {10/31} & { 3/ 7} & {16/39} & { 4/13} & { 7/19} & { 3/ 7} & {13/34} & {15/41} & { 3/ 7} & {19/46} & { 4/11} & { 3/ 8} & { 3/ 7} & { 2/ 5} & { 3/ 8} & { 3/ 7} & {22/53} & {19/51} & { 3/ 8} & { 3/ 7} & {23/57} & { 3/ 8} & { 3/ 7} & { 5/12} & {\color{red}  3/ 8} & {11/29} & { 3/ 7} & {13/32} & { 1/ 3} & { 3/ 7} & {28/67} & {12/31} & {18/47} & { 3/ 7} & {29/71} & {25/69} & { 3/ 7} & {31/74} & { 2/ 5} & {22/57} & { 3/ 7} & {16/39} & {\color{red}  7/19} & { 3/ 7} & {34/81} & {33/82} & { 7/18} & { 3/ 7} & { 7/17} & {14/37} & { 3/ 7} & {37/88} & {36/89} & {\color{red} 22/57} & { 3/ 7} & {19/46} & {\color{red} 12/31} & { 3/ 7} & { 8/19} \\\hline
$26$ & {13/37} & {\color{red}  5/16} & { 7/18} & {13/33} & {22/67} & { 5/13} & {13/33} & { 4/11} & { 8/21} & {13/33} & {18/47} & {27/74} & { 9/23} & { 7/18} & {19/51} & {19/49} & {13/33} & { 7/18} & { 5/13} & {13/33} & { 7/18} & {\color{red} 21/55} & {11/28} & {16/43} & { 7/18} & {23/59} & {13/33} & { 7/18} & {\color{red} 12/31} & {13/33} & { 1/ 3} & { 7/18} & {13/33} & {35/96} & {13/34} & {\color{red}  9/23} & {13/33} & {27/71} & { 7/18} & {13/33} & {31/84} & {29/75} & {13/33} & { 3/ 8} & { 5/13} & {31/79} & {\color{red} 32/83} & {31/81} & {16/41} & {13/33} & {\color{red}  8/21} & {33/85} & {13/33} & { 7/18} & {17/44} & {35/89} & { 7/18} & {\color{red}  5/13} & { 9/23} & {13/33} \\\hline
$27$ & {23/65} & { 1/ 3} & {15/37} & { 7/17} & { 1/ 3} & { 2/ 5} & { 7/17} & {\color{red} 25/72} & {26/73} & { 9/22} & {29/75} & { 8/23} & {19/47} & { 7/17} & {17/49} & { 2/ 5} & { 7/17} & {15/41} & {30/83} & {11/27} & { 7/17} & { 6/17} & {23/57} & { 7/17} & {\color{red}  6/17} & { 2/ 5} & {25/61} & { 9/23} & {34/93} & {13/32} & { 7/17} & { 1/ 3} & {27/67} & { 7/17} & {37/99} & { 2/ 5} & {29/71} & { 7/17} & {31/84} & {15/37} & { 7/17} & {\color{red} 19/53} & {31/77} & {16/39} & {28/71} & { 2/ 5} & {11/27} & { 7/17} & {\color{red} 31/84} & {17/42} & { 7/17} & {\color{red} 37/99} & {35/87} & { 9/22} & { 7/17} & { 2/ 5} & {37/91} & { 7/17} & {\color{red} 31/84} & {19/47} \\\hline
$28$ & {24/67} & {11/34} & { 8/19} & { 3/ 7} & {22/71} & { 3/ 8} & { 3/ 7} & {27/74} & { 4/11} & {19/45} & { 3/ 7} & {17/47} & {31/79} & { 3/ 7} & {10/27} & {13/35} & {11/26} & { 3/ 7} & {10/27} & {35/86} & { 3/ 7} & { 3/ 8} & {13/35} & {25/59} & { 3/ 7} & {13/35} & {13/31} & { 3/ 7} & {36/95} & { 3/ 8} & {14/33} & { 3/ 7} & {\color{red} 15/46} & {29/69} & { 3/ 7} & {13/34} & {33/85} & {31/73} & { 3/ 7} & {\color{red}  9/25} & { 8/19} & { 3/ 7} & {37/96} & { 2/ 5} & {17/40} & { 3/ 7} & {\color{red} 15/41} & {35/83} & { 3/ 7} & {26/67} & {\color{red} 35/86} & {37/87} & { 3/ 7} & { 3/ 8} & {19/45} & { 3/ 7} & {\color{red} 37/96} & {13/31} & {20/47} & { 3/ 7} \\\hline
$29$ & {25/69} & {\color{red} 11/35} & {16/39} & {17/43} & {\color{red} 23/73} & { 8/21} & {16/39} & {18/47} & {17/45} & {16/39} & { 2/ 5} & { 3/ 8} & {19/49} & {16/39} & { 7/18} & { 5/13} & { 2/ 5} & {23/57} & {\color{red} 21/55} & { 7/18} & {16/39} & {24/61} & { 7/18} & { 9/23} & {13/32} & {\color{red} 12/31} & {36/95} & {16/39} & {27/68} & { 7/18} & {38/99} & {29/71} & { 7/18} & { 1/ 3} & {16/39} & { 2/ 5} & {29/76} & {\color{red} 14/37} & {16/39} & {31/79} & {29/77} & {16/39} & {33/82} & {32/83} & {\color{red} 31/81} & {16/39} & {17/43} & {\color{red}  8/21} & {\color{red}  2/ 5} & {36/89} & { 7/18} & {17/44} & {\color{red}  9/22} & {37/93} & {\color{red}  5/13} & {25/62} & {13/32} & {38/97} & { 7/18} & {16/39} \\\hline
$30$ & {25/71} & { 1/ 3} & { 2/ 5} & {15/37} & { 1/ 3} & {17/43} & {15/37} & {17/48} & {29/79} & {19/47} & {\color{red} 19/51} & {\color{red} 17/49} & { 2/ 5} & {15/37} & { 4/11} & {21/53} & {15/37} & { 3/ 8} & {34/89} & {23/57} & { 5/13} & {23/62} & { 2/ 5} & {15/37} & { 3/ 8} & {25/63} & {15/37} & { 5/14} & {13/33} & {27/67} & {21/53} & { 3/ 8} & { 2/ 5} & {15/37} & { 1/ 3} & {29/73} & {15/37} & {10/27} & {15/38} & {31/77} & {15/37} & {\color{red} 29/79} & { 2/ 5} & {15/37} & {\color{red}  6/17} & {33/83} & {17/42} & {\color{red} 34/91} & {17/43} & {35/87} & {15/37} & {\color{red} 34/89} & { 2/ 5} & {15/37} & {\color{red}  7/19} & {37/93} & {19/47} & {\color{red} 35/93} & {19/48} & {39/97} \\\hline
$31$ & {26/73} & {12/37} & {17/41} & { 8/19} & {\color{red} 24/77} & { 5/13} & { 8/19} & {\color{red}  7/20} & {17/47} & { 5/12} & {34/83} & { 9/25} & { 7/17} & { 8/19} & {19/53} & { 7/19} & {23/55} & { 2/ 5} & { 7/19} & {12/29} & { 8/19} & {11/30} & {37/95} & {13/31} & {38/97} & { 7/19} & {27/65} & { 8/19} & { 7/19} & { 7/17} & {29/69} & { 5/13} & {13/35} & { 5/12} & { 8/19} & {\color{red}  1/99} & {31/75} & { 8/19} & {\color{red} 19/52} & {11/28} & {33/79} & {\color{red} 34/83} & {\color{red} 29/81} & {17/41} & { 8/19} & {\color{red} 31/86} & { 7/17} & {18/43} & {31/75} & {\color{red} 13/35} & {37/89} & {\color{red} 21/50} & {\color{red} 33/91} & {19/46} & {13/31} & {\color{red} 38/97} & {\color{red} 11/28} & { 5/12} & {\color{red} 37/88} & {\color{red}  1/99} \\\hline
$32$ & { 9/25} & {\color{red}  6/19} & { 3/ 7} & {19/46} & {\color{red} 24/79} & {17/45} & { 3/ 7} & {31/82} & { 3/ 8} & { 3/ 7} & {22/53} & {19/51} & { 5/13} & { 3/ 7} & {35/89} & {21/55} & { 3/ 7} & { 5/12} & {11/29} & { 5/13} & { 3/ 7} & {13/32} & { 5/13} & { 3/ 7} & {28/67} & { 5/13} & {35/93} & { 3/ 7} & {29/71} & { 5/13} & { 3/ 7} & {31/74} & { 5/13} & {30/79} & { 3/ 7} & {16/39} & {\color{red}  1/99} & { 3/ 7} & {34/81} & {\color{red} 31/82} & {\color{red} 30/79} & { 3/ 7} & { 7/17} & {31/83} & { 3/ 7} & {37/88} & {\color{red} 35/89} & {37/96} & { 3/ 7} & {19/46} & {\color{red} 17/45} & { 3/ 7} & { 8/19} & {13/32} & {\color{red} 18/47} & { 3/ 7} & {41/99} & {\color{red} 37/97} & { 3/ 7} & {35/83} \\\hline
$33$ & { 4/11} & { 1/ 3} & {17/43} & { 2/ 5} & { 1/ 3} & { 9/23} & { 2/ 5} & {19/51} & {32/85} & { 2/ 5} & { 7/18} & { 4/11} & {21/53} & { 2/ 5} & {11/29} & {11/28} & { 2/ 5} & {24/61} & {23/59} & { 2/ 5} & {17/43} & { 5/13} & {25/63} & { 2/ 5} & {17/43} & {13/33} & { 2/ 5} & {17/43} & {\color{red}  9/23} & { 2/ 5} & {35/96} & {17/43} & {29/73} & { 2/ 5} & {31/80} & {\color{red} 15/38} & { 2/ 5} & {\color{red}  1/99} & {17/43} & { 2/ 5} & {\color{red} 31/84} & {16/41} & {\color{red} 33/83} & { 2/ 5} & {\color{red} 32/85} & {17/43} & { 2/ 5} & {34/91} & {35/89} & { 2/ 5} & {18/47} & { 9/23} & {37/93} & { 2/ 5} & {37/95} & {19/48} & { 2/ 5} & {22/57} & {13/33} & { 2/ 5} \\\hline
$34$ & {28/79} & {13/40} & { 9/22} & {17/41} & {16/49} & {11/28} & {17/41} & {\color{red} 15/43} & { 9/25} & { 7/17} & {35/89} & {19/53} & {11/27} & {17/41} & {\color{red}  5/14} & {18/47} & {12/29} & { 3/ 8} & {15/41} & {25/61} & {17/41} & {\color{red} 23/63} & {13/32} & {17/41} & {\color{red}  4/11} & { 3/ 8} & { 7/17} & {28/69} & {15/41} & {29/71} & {17/41} & {15/41} & {15/37} & {31/75} & {37/95} & {\color{red}  4/11} & {16/39} & {17/41} & {\color{red}  1/99} & {11/27} & {17/41} & { 3/ 8} & {\color{red} 11/28} & { 7/17} & {\color{red} 28/69} & {\color{red}  1/99} & { 9/22} & {\color{red} 41/99} & {\color{red}  1/99} & {37/91} & {19/46} & {\color{red} 37/95} & {\color{red} 18/47} & {39/95} & {17/41} & {\color{red}  1/99} & {20/49} & {41/99} & {\color{red} 35/92} & {28/69} \\\hline
$35$ & {29/81} & {\color{red} 13/41} & {19/45} & { 3/ 7} & {\color{red}  3/10} & {\color{red}  3/ 8} & { 3/ 7} & { 4/11} & {19/51} & {11/26} & { 3/ 7} & {10/27} & {12/31} & { 3/ 7} & { 7/19} & {11/29} & {25/59} & { 3/ 7} & {23/61} & {\color{red}  9/23} & { 3/ 7} & {\color{red}  3/ 8} & { 8/21} & {14/33} & { 3/ 7} & { 8/21} & {37/90} & { 3/ 7} & {27/71} & { 4/11} & {31/73} & { 3/ 7} & { 8/21} & { 8/19} & { 3/ 7} & {\color{red}  8/21} & {\color{red} 16/43} & {17/40} & { 3/ 7} & {\color{red}  1/99} & {35/83} & { 3/ 7} & {\color{red} 35/93} & {12/31} & {37/87} & { 3/ 7} & {\color{red}  1/99} & {19/45} & { 3/ 7} & {\color{red} 19/51} & {\color{red} 23/59} & {20/47} & { 3/ 7} & {\color{red}  1/99} & {41/97} & { 3/ 7} & {\color{red} 35/93} & {\color{red}  2/ 5} & {23/54} & { 3/ 7} \\\hline
$36$ & {30/83} & { 1/ 3} & {19/46} & { 2/ 5} & { 1/ 3} & {19/49} & {19/46} & { 7/18} & { 5/13} & {19/46} & {23/57} & {33/94} & {11/28} & {19/46} & {24/61} & {23/59} & {40/99} & {13/32} & {12/31} & {17/43} & {19/46} & {27/68} & {13/33} & {21/53} & {29/71} & {\color{red}  9/23} & {17/43} & {19/46} & { 2/ 5} & {17/43} & {37/95} & {16/39} & {\color{red} 15/38} & {\color{red} 19/53} & {19/46} & {33/82} & {17/43} & {\color{red} 29/78} & { 7/17} & {17/43} & {\color{red}  1/99} & {19/46} & {36/89} & { 7/18} & {\color{red} 17/44} & {19/46} & {37/93} & { 5/13} & {19/46} & {13/32} & {38/97} & {37/95} & {\color{red} 37/90} & { 2/ 5} & {19/49} & {\color{red} 40/99} & {31/76} & {28/71} & {20/51} & {\color{red} 37/90} \\\hline
$37$ & {\color{red} 17/48} & {14/43} & {19/47} & { 9/22} & {29/89} & { 2/ 5} & { 9/22} & { 4/11} & {\color{red} 19/53} & {11/27} & {\color{red} 11/29} & {\color{red}  5/14} & {23/57} & { 9/22} & {23/62} & { 2/ 5} & { 9/22} & {18/47} & {\color{red}  4/11} & {13/32} & { 2/ 5} & {26/69} & {27/67} & { 9/22} & {18/47} & { 2/ 5} & {29/71} & { 3/ 8} & {29/76} & {15/37} & { 9/22} & {18/47} & {31/77} & { 9/22} & {\color{red}  1/99} & { 2/ 5} & {11/27} & {\color{red}  8/21} & {18/47} & {17/42} & { 9/22} & {\color{red}  1/99} & {35/87} & { 9/22} & {\color{red} 26/71} & { 2/ 5} & {37/91} & {\color{red}  2/ 5} & {\color{red}  1/99} & {19/47} & {\color{red} 38/93} & {\color{red}  1/99} & {39/97} & {20/49} & {\color{red}  3/ 8} & { 2/ 5} & {28/69} & {\color{red} 38/93} & {\color{red}  1/99} & {21/52} \\\hline
$38$ & {31/87} & {\color{red}  7/22} & { 5/12} & {19/45} & {17/53} & {35/92} & {19/45} & {17/47} & {10/27} & {23/55} & {40/97} & { 7/19} & {40/99} & {19/45} & {11/30} & {23/61} & {13/31} & {21/52} & { 3/ 8} & {27/65} & {19/45} & {25/67} & {\color{red} 17/45} & {29/69} & {\color{red}  5/13} & {17/45} & { 5/12} & {19/45} & {17/45} & {23/58} & { 8/19} & {\color{red} 14/37} & {\color{red}  9/26} & {33/79} & {19/45} & {17/45} & {17/41} & {35/83} & {\color{red} 17/45} & {\color{red} 29/79} & {18/43} & {19/45} & {\color{red}  1/99} & {37/89} & {19/45} & {\color{red} 17/47} & {\color{red} 35/92} & {13/31} & {\color{red} 40/97} & {\color{red}  1/99} & { 5/12} & {\color{red} 35/83} & {\color{red}  1/99} & {\color{red} 40/99} & {21/50} & {\color{red} 21/52} & {\color{red}  1/99} & {38/91} & {\color{red}  8/19} & {\color{red}  1/99} \\\hline
$39$ & {32/89} & { 1/ 3} & { 3/ 7} & {22/53} & { 1/ 3} & { 5/13} & { 3/ 7} & { 3/ 8} & {21/55} & { 3/ 7} & { 5/12} & { 9/25} & {23/59} & { 3/ 7} & {33/85} & {12/31} & { 3/ 7} & {28/67} & { 5/13} & { 9/23} & { 3/ 7} & {\color{red} 28/71} & { 9/23} & { 3/ 7} & {31/74} & { 7/18} & { 9/23} & { 3/ 7} & {16/39} & { 9/23} & { 3/ 7} & {34/81} & { 9/23} & {\color{red} 10/27} & { 3/ 7} & { 7/17} & {\color{red} 19/51} & { 3/ 7} & {37/88} & { 9/23} & {\color{red} 10/27} & { 3/ 7} & {19/46} & {\color{red}  1/99} & { 3/ 7} & { 8/19} & {\color{red} 25/66} & {\color{red} 18/47} & { 3/ 7} & {41/99} & {\color{red} 37/97} & { 3/ 7} & {35/83} & {\color{red} 33/85} & {\color{red} 22/57} & { 3/ 7} & {22/53} & {\color{red}  1/99} & { 3/ 7} & {27/64} \\\hline
$40$ & {33/91} & {15/46} & { 2/ 5} & {19/47} & {\color{red} 13/42} & {21/53} & {19/47} & {11/29} & { 4/11} & {23/57} & {24/61} & {\color{red} 21/59} & { 2/ 5} & {\color{red} 19/47} & { 5/13} & {25/63} & {19/47} & {27/68} & {\color{red} 26/69} & {27/67} & { 2/ 5} & { 7/18} & { 2/ 5} & {19/47} & { 2/ 5} & {29/73} & {19/47} & { 2/ 5} & {31/79} & {31/77} & {\color{red}  8/21} & { 2/ 5} & { 2/ 5} & {19/47} & { 2/ 5} & {\color{red} 33/83} & {19/47} & {\color{red}  1/99} & { 2/ 5} & {35/87} & {\color{red} 33/85} & {\color{red} 23/60} & {\color{red}  2/ 5} & {19/47} & {\color{red}  1/99} & { 2/ 5} & {19/47} & {\color{red} 37/98} & {19/48} & {\color{red} 39/97} & {\color{red} 33/85} & {\color{red}  1/99} & { 2/ 5} & {\color{red} 21/52} & { 8/21} & {39/98} & {21/52} & { 7/18} & {21/53} & {39/97} \\\hline
$41$ & {11/31} & {\color{red} 15/47} & { 7/17} & { 5/12} & {\color{red}  9/28} & {19/49} & { 5/12} & {\color{red} 21/59} & { 7/19} & {12/29} & {39/98} & {11/30} & {25/61} & { 5/12} & {\color{red} 23/63} & { 3/ 8} & {27/65} & {21/55} & {25/67} & { 7/17} & { 5/12} & {\color{red} 13/35} & {\color{red} 28/71} & { 5/12} & {\color{red} 19/51} & {\color{red}  3/ 8} & {31/75} & { 5/12} & { 3/ 8} & {16/39} & { 5/12} & {\color{red}  3/ 8} & {\color{red} 37/98} & {17/41} & {\color{red} 39/98} & { 3/ 8} & { 7/17} & { 5/12} & { 3/ 8} & { 9/22} & {37/89} & {\color{red} 21/55} & {\color{red} 19/51} & {19/46} & { 5/12} & {\color{red}  1/99} & {39/95} & { 5/12} & {\color{red}  1/99} & {\color{red} 19/49} & {41/99} & { 5/12} & {\color{red}  1/99} & { 7/17} & {\color{red} 37/89} & {\color{red}  1/99} & {34/83} & {22/53} & {\color{red} 21/55} & {\color{red}  1/99} \\\hline
$42$ & {34/95} & { 1/ 3} & {11/26} & { 3/ 7} & { 1/ 3} & {21/55} & { 3/ 7} & {33/91} & {11/29} & {25/59} & { 3/ 7} & {32/87} & {\color{red} 12/31} & { 3/ 7} & {29/79} & { 5/13} & {14/33} & { 3/ 7} & {13/34} & {15/38} & { 3/ 7} & {\color{red} 27/71} & {19/49} & {31/73} & { 3/ 7} & {29/75} & {\color{red} 33/83} & { 3/ 7} & {\color{red}  5/13} & {19/49} & {17/40} & { 3/ 7} & {19/49} & {\color{red} 34/83} & { 3/ 7} & {19/49} & {\color{red}  1/99} & {37/87} & { 3/ 7} & {\color{red} 18/49} & {19/45} & { 3/ 7} & {19/49} & {\color{red} 27/73} & {20/47} & { 3/ 7} & {\color{red}  1/99} & {41/97} & { 3/ 7} & {\color{red} 33/91} & {\color{red} 23/60} & {23/54} & { 3/ 7} & {\color{red}  1/99} & {11/26} & { 3/ 7} & {\color{red}  1/99} & {15/38} & {23/54} & { 3/ 7} \\\hline
$43$ & {35/97} & {\color{red}  6/19} & {22/53} & {23/57} & {\color{red} 25/83} & {11/28} & {22/53} & { 5/13} & {13/35} & {22/53} & {13/32} & {\color{red} 11/31} & {25/63} & {22/53} & {27/68} & {13/33} & {\color{red}  2/ 5} & {29/71} & { 9/23} & { 2/ 5} & {22/53} & { 2/ 5} & {29/73} & { 2/ 5} & {16/39} & {15/38} & { 2/ 5} & {22/53} & {33/82} & { 2/ 5} & {\color{red} 23/60} & { 7/17} & {\color{red} 33/83} & { 2/ 5} & {22/53} & {36/89} & { 2/ 5} & {\color{red}  4/11} & {19/46} & { 2/ 5} & {\color{red}  1/99} & {22/53} & {13/32} & { 2/ 5} & {\color{red} 34/95} & {41/99} & { 2/ 5} & {\color{red}  1/99} & {22/53} & {31/76} & {\color{red}  5/13} & {20/51} & {22/53} & {39/97} & {\color{red}  1/99} & {22/53} & { 9/22} & {23/58} & {28/71} & {\color{red} 40/97} \\\hline
$44$ & { 4/11} & {\color{red}  8/25} & {11/27} & { 7/17} & {\color{red} 29/92} & {28/71} & { 7/17} & {23/62} & {11/30} & {25/61} & {\color{red} 37/96} & {\color{red} 23/63} & {13/32} & { 7/17} & {26/69} & {22/57} & { 7/17} & { 7/18} & {\color{red} 13/35} & {29/71} & { 7/17} & {29/76} & {15/37} & { 7/17} & { 7/18} & {\color{red}  3/ 8} & {16/39} & { 7/18} & {32/83} & {11/27} & { 7/17} & { 7/18} & {17/42} & { 7/17} & {\color{red} 27/85} & { 7/18} & { 9/22} & { 7/17} & { 7/18} & {37/91} & { 7/17} & {\color{red}  1/99} & {19/47} & {39/95} & {\color{red} 37/96} & { 7/18} & {20/49} & { 7/17} & {\color{red}  1/99} & {28/69} & { 7/17} & {\color{red}  1/99} & {\color{red} 28/71} & {34/83} & { 7/17} & {\color{red}  1/99} & {11/27} & { 7/17} & {\color{red}  1/99} & {15/37} \\\hline
$45$ & {31/87} & { 1/ 3} & {23/55} & {\color{red} 40/97} & { 1/ 3} & {\color{red} 11/29} & {11/26} & {\color{red} 13/36} & {23/61} & {13/31} & {29/70} & { 3/ 8} & {\color{red} 35/89} & {11/26} & {\color{red}  5/14} & {13/34} & {29/69} & {\color{red} 23/58} & {27/71} & { 5/12} & {11/26} & {14/37} & { 5/13} & { 8/19} & {\color{red} 29/77} & { 5/13} & {33/79} & {11/26} & {31/81} & { 5/13} & {35/83} & {\color{red}  8/21} & { 5/13} & {18/43} & {11/26} & { 5/13} & {\color{red} 39/98} & {19/45} & {\color{red}  5/13} & {\color{red}  1/99} & {13/31} & {11/26} & { 5/13} & { 5/12} & {41/97} & {\color{red}  5/13} & {\color{red}  1/99} & {21/50} & {11/26} & {\color{red}  1/99} & {38/91} & {11/26} & {\color{red}  1/99} & {\color{red} 20/53} & {37/88} & {\color{red} 29/70} & {\color{red}  1/99} & {23/55} & {\color{red} 27/64} & {\color{red}  1/99} \\\hline
$46$ & {23/64} & {\color{red} 17/55} & { 3/ 7} & { 5/12} & {\color{red} 19/61} & {23/59} & { 3/ 7} & {\color{red} 26/71} & {14/37} & { 3/ 7} & {28/67} & {23/65} & {13/33} & { 3/ 7} & { 5/13} & { 9/23} & { 3/ 7} & {31/74} & { 7/18} & {21/53} & { 3/ 7} & {\color{red} 33/85} & {15/38} & { 3/ 7} & {34/81} & {31/79} & {\color{red} 19/48} & { 3/ 7} & {\color{red}  2/ 5} & {21/53} & { 3/ 7} & {37/88} & {17/43} & {\color{red}  1/99} & { 3/ 7} & {19/46} & {21/53} & { 3/ 7} & { 8/19} & {21/53} & {\color{red}  1/99} & { 3/ 7} & {41/99} & {\color{red}  1/99} & { 3/ 7} & {35/83} & {21/53} & {\color{red}  1/99} & { 3/ 7} & {22/53} & {\color{red}  1/99} & { 3/ 7} & {27/64} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 7} & {37/89} & {\color{red}  1/99} & { 3/ 7} & {30/71} \\\hline
$47$ & {21/58} & {\color{red} 25/81} & {23/57} & {11/27} & {\color{red}  1/99} & { 2/ 5} & {\color{red} 11/27} & { 5/13} & {23/63} & {13/32} & {27/68} & { 4/11} & {27/67} & {\color{red} 11/27} & { 7/18} & { 2/ 5} & {11/27} & { 2/ 5} & {\color{red} 27/73} & {15/37} & {23/57} & {31/79} & {31/77} & {11/27} & {33/82} & { 2/ 5} & {11/27} & {23/57} & {17/43} & {17/42} & {11/27} & {\color{red} 39/97} & {35/87} & {11/27} & {23/57} & { 2/ 5} & {37/91} & {\color{red} 17/46} & {23/57} & {19/47} & {11/27} & {\color{red}  3/ 8} & {\color{red} 39/97} & {11/27} & {\color{red}  1/99} & {23/57} & {28/69} & {\color{red} 29/74} & {\color{red} 23/64} & {\color{red} 21/52} & {11/27} & {\color{red}  1/99} & {23/57} & {11/27} & {\color{red}  1/99} & { 2/ 5} & {\color{red} 15/37} & {11/27} & {\color{red}  1/99} & {23/57} \\\hline
$48$ & {\color{red} 21/59} & { 1/ 3} & {12/29} & {\color{red} 35/86} & { 1/ 3} & {38/99} & {23/55} & { 4/11} & { 3/ 8} & {27/65} & {\color{red} 17/43} & {25/67} & { 7/17} & {23/55} & {27/73} & {27/71} & { 5/12} & {12/31} & {14/37} & {31/75} & {23/55} & {\color{red} 29/77} & {\color{red} 38/99} & {33/79} & {\color{red} 11/29} & {21/55} & {17/41} & {\color{red} 31/76} & {\color{red}  8/21} & { 7/17} & {23/55} & {\color{red} 11/29} & {\color{red}  1/ 3} & {37/89} & {\color{red}  2/ 5} & {\color{red} 21/55} & {19/46} & {23/55} & {\color{red} 33/94} & {\color{red} 36/95} & { 5/12} & {\color{red} 35/89} & {\color{red}  1/99} & {41/99} & {23/55} & {\color{red}  1/99} & { 7/17} & {38/91} & {\color{red} 21/55} & {\color{red}  1/99} & {22/53} & {23/55} & {\color{red}  1/99} & {26/63} & {23/55} & {\color{red}  1/99} & {\color{red} 38/99} & {37/89} & {\color{red} 27/67} & {\color{red}  1/99} \\\hline
$49$ & {34/95} & {\color{red}  9/29} & {25/59} & { 3/ 7} & {\color{red}  1/99} & {12/31} & { 3/ 7} & {\color{red} 34/95} & { 5/13} & {14/33} & { 3/ 7} & {\color{red}  6/17} & { 9/23} & { 3/ 7} & {\color{red} 21/58} & { 7/18} & {31/73} & { 3/ 7} & {29/75} & {\color{red} 11/28} & { 3/ 7} & { 5/13} & {31/79} & {17/40} & { 3/ 7} & {16/41} & { 2/ 5} & { 3/ 7} & {33/85} & {11/28} & {37/87} & { 3/ 7} & {11/28} & {\color{red} 39/97} & { 3/ 7} & { 9/23} & {\color{red}  1/99} & {20/47} & { 3/ 7} & {11/28} & {\color{red} 40/97} & { 3/ 7} & {\color{red} 20/51} & {\color{red}  1/99} & {23/54} & { 3/ 7} & {\color{red}  1/99} & {11/26} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {23/54} & { 3/ 7} & {\color{red}  1/99} & {36/85} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {26/61} & { 3/ 7} \\\hline
$50$ & {31/86} & {\color{red}  9/28} & { 5/12} & {13/32} & {\color{red}  1/99} & {25/63} & { 5/12} & {\color{red} 35/93} & {\color{red}  4/11} & {\color{red} 35/86} & {29/71} & {25/69} & { 2/ 5} & {\color{red} 37/89} & { 2/ 5} & {29/73} & {\color{red} 31/77} & {16/39} & {16/43} & {31/77} & {\color{red} 37/89} & {33/82} & { 2/ 5} & {\color{red} 23/57} & { 7/17} & {33/83} & {23/57} & { 5/12} & {36/89} & {35/87} & {\color{red} 18/47} & {19/46} & { 2/ 5} & {23/57} & {\color{red} 37/89} & {13/32} & {23/57} & {\color{red}  7/19} & {41/99} & {\color{red} 39/97} & {\color{red}  5/13} & { 5/12} & {31/76} & {23/57} & {\color{red}  7/19} & {22/53} & {23/57} & {\color{red}  1/99} & { 5/12} & { 9/22} & {\color{red} 22/57} & {\color{red}  1/99} & {37/89} & {23/57} & {\color{red}  1/99} & { 5/12} & {16/39} & {\color{red}  1/99} & {23/58} & { 5/12} \\\hline
$51$ & {33/91} & { 1/ 3} & {25/61} & {\color{red} 40/99} & {\color{red}  1/99} & {23/59} & {12/29} & {26/69} & {25/67} & { 7/17} & {\color{red} 16/41} & {13/35} & {29/71} & {12/29} & {29/76} & {\color{red} 14/37} & {31/75} & {31/79} & {\color{red} 29/77} & {16/39} & {12/29} & {32/83} & {11/27} & {12/29} & {\color{red} 38/97} & {11/29} & { 7/17} & {\color{red} 13/33} & { 7/18} & { 9/22} & {12/29} & {24/61} & {\color{red} 23/59} & {19/46} & {\color{red} 20/53} & {38/97} & {39/95} & {12/29} & {24/61} & {20/49} & {12/29} & {\color{red}  1/99} & {\color{red}  9/23} & { 7/17} & {\color{red} 23/58} & {\color{red}  5/13} & {34/83} & {12/29} & {\color{red}  1/99} & {11/27} & {26/63} & {\color{red} 11/29} & {\color{red}  1/99} & {23/56} & {12/29} & {\color{red}  1/99} & {38/93} & {12/29} & {\color{red}  1/99} & {\color{red} 23/59} \\\hline
$52$ & {31/87} & {\color{red} 19/61} & {13/31} & {\color{red} 29/70} & {\color{red}  1/99} & { 5/13} & {\color{red} 36/85} & {\color{red}  5/14} & {13/34} & {29/69} & {\color{red} 29/73} & {\color{red}  5/14} & {\color{red}  7/18} & {\color{red} 36/85} & {\color{red}  1/99} & {29/75} & { 8/19} & {\color{red}  2/ 5} & { 5/13} & {\color{red} 32/79} & {25/59} & {31/81} & {\color{red} 37/95} & {35/83} & {\color{red} 11/29} & {33/85} & {18/43} & {25/59} & {17/44} & {\color{red} 37/95} & {19/45} & {\color{red}  5/13} & {23/59} & {13/31} & {\color{red} 36/85} & {37/95} & {\color{red} 25/66} & {41/97} & {\color{red} 19/49} & {\color{red}  4/11} & {21/50} & {25/59} & {\color{red}  7/18} & {\color{red} 39/98} & {11/26} & {\color{red}  1/99} & {\color{red}  1/99} & {37/88} & {25/59} & {\color{red}  1/99} & {23/55} & {36/85} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/19} & {25/59} & {\color{red}  1/99} & {31/74} & {25/59} & {\color{red}  1/99} \\\hline
$53$ & {14/39} & {\color{red} 14/45} & { 3/ 7} & {28/67} & {\color{red}  1/99} & {13/33} & { 3/ 7} & {\color{red} 31/85} & {\color{red} 33/91} & { 3/ 7} & {31/74} & {\color{red}  1/99} & {29/73} & { 3/ 7} & {\color{red} 32/85} & {15/38} & { 3/ 7} & {34/81} & {\color{red} 30/79} & { 2/ 5} & { 3/ 7} & { 9/23} & {33/83} & { 3/ 7} & {37/88} & {17/43} & { 2/ 5} & { 3/ 7} & {\color{red} 13/33} & { 2/ 5} & { 3/ 7} & { 8/19} & {37/93} & { 2/ 5} & { 3/ 7} & {\color{red} 40/99} & { 2/ 5} & { 3/ 7} & {35/83} & { 2/ 5} & {\color{red}  1/99} & { 3/ 7} & {22/53} & { 2/ 5} & { 3/ 7} & {27/64} & { 2/ 5} & {\color{red}  1/99} & { 3/ 7} & {37/89} & {\color{red}  1/99} & { 3/ 7} & {30/71} & {\color{red} 14/39} & {\color{red}  1/99} & { 3/ 7} & { 5/12} & {\color{red}  1/99} & { 3/ 7} & {41/97} \\\hline
$54$ & {30/83} & { 1/ 3} & {13/32} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red} 26/67} & {\color{red} 34/83} & { 7/18} & {13/35} & {29/71} & { 2/ 5} & {27/73} & {15/37} & {\color{red} 25/61} & {31/79} & {\color{red} 29/77} & {\color{red} 34/83} & {33/82} & { 3/ 8} & {11/27} & {\color{red} 13/32} & {17/43} & {17/42} & {\color{red} 34/83} & {36/89} & { 7/18} & { 9/22} & {13/32} & {37/93} & {37/91} & {\color{red} 34/83} & {13/32} & {19/47} & {25/61} & {13/32} & { 2/ 5} & {20/49} & {\color{red} 38/99} & {\color{red} 39/97} & {28/69} & {25/61} & {\color{red} 33/85} & {\color{red} 21/52} & {34/83} & {\color{red}  1/99} & {\color{red} 23/57} & {11/27} & {\color{red} 38/99} & {\color{red} 22/59} & {\color{red} 15/37} & {25/61} & {\color{red}  1/99} & {13/32} & {38/93} & {\color{red} 23/61} & {\color{red}  1/99} & {\color{red} 24/59} & {25/61} & {\color{red}  1/99} & {13/32} \\\hline
$55$ & { 4/11} & {\color{red}  5/16} & {27/65} & {13/31} & {\color{red}  1/99} & {\color{red} 13/34} & {13/31} & {27/73} & {27/71} & { 5/12} & {\color{red}  2/ 5} & { 4/11} & {\color{red}  2/ 5} & {13/31} & { 3/ 8} & { 5/13} & {33/79} & {\color{red} 38/99} & {31/81} & {17/41} & {13/31} & {\color{red}  8/21} & {\color{red} 17/44} & {18/43} & {\color{red} 18/47} & {17/44} & {37/89} & {13/31} & {\color{red}  5/13} & {\color{red}  9/23} & {13/31} & {\color{red} 18/47} & {\color{red}  7/19} & { 5/12} & {\color{red}  2/ 5} & {\color{red} 12/31} & {41/99} & {\color{red} 38/91} & {\color{red}  1/99} & {\color{red}  1/99} & {38/91} & {\color{red}  5/13} & {\color{red}  1/99} & {22/53} & {13/31} & {\color{red}  1/99} & {\color{red} 37/96} & {23/55} & {\color{red} 22/57} & {\color{red}  1/99} & {37/89} & {\color{red} 31/74} & {\color{red}  1/99} & {12/29} & {31/74} & {\color{red}  1/99} & {\color{red}  1/99} & { 5/12} & {13/31} & {\color{red}  1/99} \\\hline
$56$ & {\color{red} 35/99} & {\color{red}  1/99} & {14/33} & { 3/ 7} & {\color{red}  1/99} & { 9/23} & { 3/ 7} & {\color{red} 13/37} & {\color{red}  7/19} & {31/73} & { 3/ 7} & {\color{red}  1/99} & {15/38} & { 3/ 7} & {\color{red}  1/99} & {31/79} & {17/40} & { 3/ 7} & {16/41} & {\color{red} 21/53} & { 3/ 7} & {\color{red}  1/99} & {17/43} & {37/87} & { 3/ 7} & {35/89} & {\color{red} 23/58} & { 3/ 7} & { 9/23} & {25/63} & {20/47} & { 3/ 7} & {19/48} & {21/52} & { 3/ 7} & {13/33} & {\color{red} 21/53} & {23/54} & { 3/ 7} & {25/63} & {\color{red} 15/37} & { 3/ 7} & {21/53} & {\color{red}  1/99} & {23/54} & { 3/ 7} & {\color{red} 23/58} & {\color{red} 29/70} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {26/61} & { 3/ 7} & {\color{red}  1/99} & {25/59} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {26/61} & { 3/ 7} \\\hline
$57$ & {\color{red}  9/25} & {\color{red}  1/99} & {28/67} & {29/71} & {\color{red}  1/99} & { 2/ 5} & {\color{red}  5/12} & {\color{red} 37/99} & {27/73} & {\color{red} 15/37} & {16/39} & { 7/19} & {31/77} & {\color{red} 38/91} & {\color{red} 16/41} & { 2/ 5} & {\color{red} 28/69} & { 7/17} & {\color{red}  1/99} & {17/42} & {\color{red}  5/12} & {36/89} & {35/87} & {\color{red} 28/69} & {19/46} & { 2/ 5} & {\color{red} 28/69} & {\color{red} 37/89} & {13/32} & {19/47} & {\color{red} 36/95} & {41/99} & {39/97} & {\color{red} 28/69} & {\color{red} 37/89} & {31/76} & {28/69} & {\color{red} 19/51} & {22/53} & {21/52} & {\color{red} 23/59} & {\color{red} 37/89} & { 9/22} & {\color{red} 15/37} & {\color{red}  3/ 8} & {37/89} & {\color{red} 15/37} & {\color{red}  1/99} & {\color{red}  5/12} & {16/39} & {\color{red} 23/59} & {\color{red}  1/99} & { 5/12} & {13/32} & {\color{red}  1/99} & {28/67} & {37/90} & {\color{red} 32/97} & {\color{red}  1/99} & {38/91} \\\hline
$58$ & {\color{red}  5/14} & {\color{red}  1/99} & { 7/17} & {\color{red} 28/69} & {\color{red}  1/99} & {17/44} & {\color{red} 22/53} & {29/76} & {14/37} & {31/75} & {\color{red} 31/79} & {\color{red}  4/11} & {16/39} & {\color{red} 22/53} & {32/83} & {31/81} & {17/41} & {17/43} & {\color{red}  8/21} & { 7/17} & {\color{red} 36/89} & { 7/18} & {\color{red} 25/64} & {\color{red} 22/53} & {\color{red} 23/58} & { 5/13} & {19/46} & {\color{red} 39/98} & {38/97} & {39/95} & {\color{red} 22/53} & {\color{red} 23/58} & {\color{red} 22/57} & {41/99} & {\color{red} 35/92} & {28/71} & { 7/17} & {\color{red} 22/53} & {\color{red} 23/58} & {\color{red}  2/ 5} & {22/53} & {\color{red}  1/99} & {23/58} & {26/63} & {\color{red} 39/98} & {\color{red} 23/58} & {23/56} & {27/65} & {\color{red}  1/99} & {\color{red}  9/23} & {12/29} & {\color{red}  5/13} & {\color{red} 37/97} & { 7/17} & {\color{red} 17/41} & {\color{red}  1/99} & {25/61} & {17/41} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$59$ & {\color{red}  5/14} & {\color{red}  1/99} & {29/69} & {\color{red} 37/89} & {\color{red}  1/99} & { 7/18} & {\color{red} 39/92} & {\color{red}  4/11} & {\color{red} 28/75} & { 8/19} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red} 31/79} & {\color{red} 25/59} & {\color{red}  1/99} & {16/41} & {35/83} & {\color{red} 13/33} & {33/85} & {\color{red} 17/43} & {\color{red} 39/92} & {\color{red}  1/99} & {35/89} & {19/45} & {\color{red} 18/47} & { 9/23} & {13/31} & {\color{red} 39/92} & {37/95} & {13/33} & {41/97} & {\color{red} 19/49} & {13/33} & {21/50} & {\color{red} 36/85} & {\color{red} 20/51} & {\color{red}  1/99} & {11/26} & {\color{red} 25/64} & {\color{red} 11/28} & {37/88} & {14/33} & {\color{red}  1/99} & {\color{red}  5/13} & {36/85} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/19} & {14/33} & {\color{red}  1/99} & {\color{red} 39/97} & {25/59} & {\color{red}  1/99} & {\color{red}  1/99} & {35/83} & {14/33} & {\color{red}  1/99} & {13/31} & {39/92} & {\color{red}  1/99} \\\hline
$60$ & {\color{red}  6/17} & {\color{red}  1/99} & { 3/ 7} & {31/74} & {\color{red}  1/99} & {29/73} & { 3/ 7} & {17/46} & {\color{red}  1/99} & { 3/ 7} & {34/81} & {\color{red}  1/99} & { 2/ 5} & { 3/ 7} & {\color{red} 37/99} & {33/83} & { 3/ 7} & {37/88} & {\color{red}  1/99} & {35/87} & { 3/ 7} & {\color{red} 38/99} & { 2/ 5} & { 3/ 7} & { 8/19} & {37/93} & {\color{red} 39/97} & { 3/ 7} & {21/53} & {39/97} & { 3/ 7} & {35/83} & { 2/ 5} & {\color{red} 31/79} & { 3/ 7} & {\color{red} 39/98} & {\color{red} 39/97} & { 3/ 7} & {27/64} & {39/97} & {\color{red}  1/99} & { 3/ 7} & {\color{red} 35/86} & {\color{red} 32/81} & { 3/ 7} & {30/71} & {\color{red} 39/97} & {\color{red}  1/99} & { 3/ 7} & { 5/12} & {\color{red}  1/99} & { 3/ 7} & {41/97} & {\color{red} 32/81} & {\color{red}  1/99} & { 3/ 7} & {38/91} & {\color{red}  1/99} & { 3/ 7} & {11/26} \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g4-a03b04.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 1/ 3} & { 3/10} & { 3/11} & {\color{red}  2/ 7} & { 1/ 3} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 6/17} & { 1/ 3} & { 6/19} & {\color{red}  7/22} & { 8/23} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 9/25} & { 9/26} & { 1/ 3} & {\color{red}  1/ 3} & {11/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 4/11} & { 6/17} & {12/35} & {\color{red} 13/38} & {14/39} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {15/41} & { 5/14} & {15/43} & {\color{red}  8/23} & {17/47} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {18/49} & { 9/25} & { 6/17} & {\color{red} 19/54} & { 4/11} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 7/19} & {21/58} & {21/59} & {\color{red} 11/31} & {23/63} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {24/65} & { 4/11} & {24/67} & {\color{red}  5/14} \\\hline
$2$ & { 3/10} & {\color{red}  2/ 7} & { 1/ 4} & { 2/ 7} & {\color{red}  5/17} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/19} & { 3/10} & { 2/ 7} & {\color{red}  9/32} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 9/28} & { 9/29} & { 3/10} & {\color{red}  5/17} & {\color{red} 11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & { 4/13} & {\color{red} 13/43} & {\color{red}  7/22} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {15/46} & {15/47} & { 5/16} & {\color{red}  4/13} & {\color{red} 17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & { 6/19} & {\color{red} 19/61} & {\color{red} 10/31} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {21/64} & {21/65} & { 7/22} & {\color{red} 11/35} & {\color{red} 23/71} & { 1/ 3} \\\hline
$3$ & { 3/11} & { 3/11} & {\color{red}  6/25} & { 1/ 4} & {\color{red}  5/19} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 2/ 7} & { 3/11} & { 3/11} & {\color{red} 15/58} & {\color{red}  8/29} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 9/31} & { 9/32} & { 3/11} & { 3/11} & {\color{red} 11/39} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & {12/41} & { 2/ 7} & {12/43} & {\color{red} 27/98} & {\color{red}  2/ 7} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 5/17} & {15/52} & {15/53} & {\color{red} 26/93} & {\color{red} 17/59} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & {18/61} & { 9/31} & { 2/ 7} & {\color{red} 13/46} & {\color{red} 20/69} & { 3/10} & { 3/10} & { 3/10} & { 3/10} & { 3/10} \\\hline
$4$ & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 4} & {\color{red}  5/17} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  2/ 7} & { 2/ 7} & { 7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  9/31} & { 2/ 7} & { 9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 11/37} & {\color{red}  5/17} & {11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 13/43} & { 3/10} & {13/41} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 15/49} & {\color{red}  7/23} & {15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 17/55} & { 4/13} & {17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 19/61} & {\color{red}  9/29} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 21/67} & { 5/16} & {21/65} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 23/73} & {\color{red} 11/35} & {23/71} & { 1/ 3} \\\hline
$5$ & { 5/13} & { 7/20} & { 2/ 7} & { 5/17} & { 1/ 3} & { 7/19} & { 5/13} & { 5/13} & { 1/ 3} & {\color{red}  7/23} & { 1/ 3} & { 9/25} & { 5/13} & { 5/13} & { 4/11} & {\color{red} 11/34} & { 1/ 3} & {11/31} & { 3/ 8} & { 5/13} & { 5/13} & { 7/20} & {\color{red}  1/ 3} & {13/37} & { 7/19} & { 5/13} & { 5/13} & {17/46} & {\color{red} 16/47} & {15/43} & { 4/11} & {17/45} & { 5/13} & { 5/13} & {19/53} & {\color{red} 17/49} & { 9/25} & {19/51} & { 5/13} & { 5/13} & {22/59} & {\color{red}  7/20} & { 5/14} & { 7/19} & {11/29} & { 5/13} & { 5/13} & { 4/11} & {\color{red} 11/31} & {23/63} & { 3/ 8} & { 5/13} & { 5/13} & { 3/ 8} & {\color{red} 26/73} & {25/69} & {13/35} & {27/71} & { 5/13} & { 5/13} \\\hline
$6$ & { 3/ 7} & { 4/11} & { 7/23} & { 1/ 3} & { 7/19} & { 2/ 5} & { 3/ 7} & { 3/ 7} & {11/29} & { 1/ 3} & { 9/25} & { 5/13} & {11/27} & { 3/ 7} & { 3/ 7} & { 7/18} & {11/31} & { 3/ 8} & {13/33} & { 7/17} & { 3/ 7} & { 3/ 7} & {17/43} & { 7/19} & { 5/13} & { 2/ 5} & {17/41} & { 3/ 7} & { 3/ 7} & { 2/ 5} & {17/45} & { 9/23} & {19/47} & { 5/12} & { 3/ 7} & { 3/ 7} & {23/57} & { 5/13} & {21/53} & {11/27} & {23/55} & { 3/ 7} & { 3/ 7} & {13/32} & {\color{red} 23/59} & { 2/ 5} & {25/61} & {13/31} & { 3/ 7} & { 3/ 7} & {29/71} & {\color{red} 13/33} & {27/67} & { 7/17} & {29/69} & { 3/ 7} & { 3/ 7} & {16/39} & {\color{red} 29/73} & {15/37} \\\hline
$7$ & { 2/ 5} & { 3/ 8} & { 8/25} & { 4/13} & {10/27} & { 3/ 7} & { 3/ 7} & { 9/22} & { 9/23} & { 3/ 8} & { 1/ 3} & {13/34} & { 3/ 7} & { 3/ 7} & {12/29} & { 2/ 5} & {12/31} & { 3/ 8} & {16/41} & { 3/ 7} & { 3/ 7} & { 5/12} & {15/37} & {15/38} & { 5/13} & {19/48} & { 3/ 7} & { 3/ 7} & {18/43} & { 9/22} & { 2/ 5} & { 9/23} & { 2/ 5} & { 3/ 7} & { 3/ 7} & {21/50} & { 7/17} & {21/52} & {21/53} & {25/62} & { 3/ 7} & { 3/ 7} & { 8/19} & {12/29} & {24/59} & { 2/ 5} & {28/69} & { 3/ 7} & { 3/ 7} & {27/64} & {27/65} & { 9/22} & {27/67} & {31/76} & { 3/ 7} & { 3/ 7} & {30/71} & { 5/12} & {30/73} & {15/37} \\\hline
$8$ & { 3/ 8} & { 6/17} & { 1/ 3} & { 2/ 7} & {10/29} & { 2/ 5} & { 2/ 5} & { 9/23} & { 3/ 8} & { 9/25} & { 9/26} & { 1/ 3} & {14/37} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & { 4/11} & { 6/17} & { 4/11} & { 2/ 5} & { 2/ 5} & {15/38} & { 5/13} & { 3/ 8} & {15/41} & { 5/14} & { 5/13} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & { 3/ 8} & {18/49} & {22/59} & { 2/ 5} & { 2/ 5} & {21/53} & { 7/18} & {21/55} & { 3/ 8} & {\color{red}  7/19} & {26/67} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 3/ 8} & {14/37} & { 2/ 5} & { 2/ 5} & {27/68} & { 9/23} & {27/70} & {27/71} & {\color{red}  3/ 8} & {16/41} & { 2/ 5} & { 2/ 5} \\\hline
$9$ & { 6/17} & { 1/ 3} & { 6/19} & { 3/10} & {10/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 9/25} & { 9/26} & { 1/ 3} & { 9/28} & { 1/ 3} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 4/11} & { 6/17} & {12/35} & { 1/ 3} & {\color{red} 16/47} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {15/41} & { 5/14} & {15/43} & {15/44} & {19/55} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {18/49} & { 9/25} & { 6/17} & { 9/26} & {\color{red} 22/63} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 7/19} & {21/58} & {21/59} & {\color{red}  7/20} & {25/71} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {24/65} & { 4/11} & {24/67} & { 6/17} & {\color{red} 28/79} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {27/73} & {27/74} & { 9/25} & {\color{red} 27/76} \\\hline
$10$ & { 1/ 3} & { 1/ 3} & { 3/10} & {\color{red}  2/ 7} & {\color{red}  4/13} & { 6/17} & { 6/17} & { 6/17} & { 9/26} & { 1/ 3} & {\color{red} 11/34} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/17} & { 6/17} & { 6/17} & {12/35} & { 1/ 3} & { 1/ 3} & {\color{red} 13/41} & {\color{red}  9/28} & { 6/17} & { 6/17} & { 6/17} & {15/43} & {15/44} & {\color{red}  1/ 3} & {\color{red} 18/55} & { 1/ 3} & {20/59} & { 6/17} & { 6/17} & { 6/17} & { 9/26} & {18/53} & { 1/ 3} & { 1/ 3} & {\color{red} 24/73} & { 6/17} & { 6/17} & { 6/17} & { 7/20} & {21/61} & {\color{red} 21/62} & {\color{red}  1/ 3} & {\color{red} 27/82} & {13/38} & { 6/17} & { 6/17} & { 6/17} & { 8/23} & {12/35} & {24/71} & {\color{red}  1/ 3} & {\color{red}  1/ 3} & { 6/17} & { 6/17} & { 6/17} & {27/77} \\\hline
$11$ & { 7/19} & {11/32} & { 2/ 7} & { 7/23} & { 1/ 3} & { 9/25} & { 7/19} & { 7/19} & { 1/ 3} & { 9/28} & { 1/ 3} & {11/31} & { 7/19} & { 7/19} & { 1/ 3} & { 1/ 3} & {\color{red}  1/ 3} & {13/37} & { 7/19} & { 7/19} & { 6/17} & {\color{red} 13/41} & { 1/ 3} & {15/43} & { 4/11} & { 7/19} & { 7/19} & {\color{red} 19/58} & {\color{red}  1/ 3} & {17/49} & { 9/25} & { 7/19} & { 7/19} & {11/32} & {\color{red}  1/ 3} & {\color{red} 19/55} & { 5/14} & { 7/19} & { 7/19} & { 5/14} & {\color{red}  1/ 3} & {21/61} & {11/31} & {23/63} & { 7/19} & { 7/19} & {\color{red} 26/77} & {\color{red} 23/67} & { 6/17} & {25/69} & { 7/19} & { 7/19} & {29/83} & {\color{red} 25/73} & {\color{red} 13/37} & { 9/25} & { 7/19} & { 7/19} & {32/89} & {\color{red} 27/79} \\\hline
$12$ & { 2/ 5} & { 6/17} & {\color{red}  2/ 7} & { 1/ 3} & { 9/25} & { 5/13} & { 2/ 5} & { 2/ 5} & {14/41} & { 1/ 3} & {11/31} & { 3/ 8} & {13/33} & { 2/ 5} & {18/47} & { 1/ 3} & {13/37} & { 7/19} & { 5/13} & { 2/ 5} & { 2/ 5} & {10/27} & {15/43} & { 4/11} & {17/45} & { 9/23} & { 2/ 5} & { 2/ 5} & {22/61} & { 9/25} & {19/51} & { 5/13} & {21/53} & { 2/ 5} & {26/67} & { 5/14} & { 7/19} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {14/37} & {23/63} & { 3/ 8} & { 5/13} & {13/33} & { 2/ 5} & { 2/ 5} & {\color{red} 10/27} & {13/35} & {27/71} & { 7/18} & {29/73} & { 2/ 5} & {34/87} & {\color{red}  7/19} & {29/77} & { 5/13} & {31/79} & { 2/ 5} \\\hline
$13$ & { 3/ 7} & {13/36} & {\color{red} 11/37} & { 6/19} & { 5/13} & {11/27} & { 3/ 7} & { 3/ 7} & {16/43} & {\color{red}  7/22} & {16/45} & {13/33} & { 7/17} & { 3/ 7} & { 3/ 7} & {19/50} & { 1/ 3} & { 5/13} & { 2/ 5} & {17/41} & { 3/ 7} & { 3/ 7} & {22/57} & {21/58} & { 9/23} & {19/47} & { 5/12} & { 3/ 7} & { 3/ 7} & {25/64} & { 5/13} & {21/53} & {11/27} & {23/55} & { 3/ 7} & { 3/ 7} & {28/71} & {23/59} & { 2/ 5} & {25/61} & {13/31} & { 3/ 7} & { 3/ 7} & {31/78} & {13/33} & {27/67} & { 7/17} & {29/69} & { 3/ 7} & { 3/ 7} & { 2/ 5} & {29/73} & {15/37} & {31/75} & { 8/19} & { 3/ 7} & { 3/ 7} & {37/92} & {\color{red}  2/ 5} & {11/27} \\\hline
$14$ & { 9/22} & { 7/19} & { 4/13} & {\color{red}  3/10} & {15/41} & { 3/ 7} & { 3/ 7} & {12/29} & { 2/ 5} & { 8/23} & {\color{red} 15/47} & { 3/ 8} & { 3/ 7} & { 3/ 7} & { 5/12} & {15/37} & {20/53} & { 1/ 3} & {21/55} & { 3/ 7} & { 3/ 7} & {18/43} & { 9/22} & { 2/ 5} & {22/61} & {12/31} & { 3/ 7} & { 3/ 7} & {21/50} & { 7/17} & {21/52} & {13/34} & { 9/23} & { 3/ 7} & { 3/ 7} & { 8/19} & {12/29} & {24/59} & { 2/ 5} & {15/38} & { 3/ 7} & { 3/ 7} & {27/64} & {27/65} & { 9/22} & {27/67} & {33/83} & { 3/ 7} & { 3/ 7} & {30/71} & { 5/12} & {30/73} & {15/37} & { 2/ 5} & { 3/ 7} & { 3/ 7} & {11/26} & {33/79} & {33/80} & {11/27} \\\hline
$15$ & { 9/23} & { 3/ 8} & {13/41} & {\color{red}  2/ 7} & {15/43} & { 9/22} & { 9/22} & { 2/ 5} & {12/31} & { 3/ 8} & {\color{red} 16/49} & {17/50} & {20/51} & { 9/22} & {15/37} & {15/38} & { 5/13} & { 3/ 8} & { 1/ 3} & {11/29} & { 9/22} & { 9/22} & { 2/ 5} & { 9/23} & {18/47} & { 3/ 8} & {24/65} & { 9/22} & { 9/22} & {21/52} & {21/53} & { 7/18} & {21/55} & { 3/ 8} & {29/73} & { 9/22} & {24/59} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & {31/80} & { 9/22} & { 9/22} & {27/67} & {27/68} & { 9/23} & {27/70} & {\color{red} 27/71} & { 9/22} & { 9/22} & {15/37} & { 2/ 5} & {15/38} & {30/77} & { 5/13} & { 2/ 5} & { 9/22} & {11/27} & {33/82} \\\hline
$16$ & { 3/ 8} & { 9/25} & {14/43} & { 2/ 7} & {\color{red}  1/ 3} & { 9/23} & { 9/23} & {12/31} & { 3/ 8} & { 4/11} & { 6/17} & { 1/ 3} & {19/53} & { 9/23} & { 9/23} & { 5/13} & { 3/ 8} & {15/41} & { 5/14} & { 1/ 3} & {23/61} & { 9/23} & { 9/23} & {18/47} & { 3/ 8} & {18/49} & { 9/25} & { 6/17} & { 9/23} & { 9/23} & { 7/18} & {21/55} & { 3/ 8} & { 7/19} & {21/58} & { 7/19} & { 9/23} & { 9/23} & {12/31} & { 8/21} & { 3/ 8} & {24/65} & { 4/11} & { 8/21} & { 9/23} & { 9/23} & {27/70} & {27/71} & { 3/ 8} & {27/73} & {\color{red} 27/74} & { 9/23} & { 9/23} & {30/77} & { 5/13} & {30/79} & { 3/ 8} & {\color{red} 10/27} & {\color{red} 37/99} & { 9/23} \\\hline
$17$ & { 9/25} & { 9/26} & { 1/ 3} & { 9/29} & { 1/ 3} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 4/11} & { 6/17} & {\color{red} 12/35} & {13/37} & { 9/25} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {15/41} & {\color{red} 34/95} & { 9/25} & { 9/25} & { 1/ 3} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {18/49} & { 9/25} & { 6/17} & {\color{red}  9/26} & {\color{red} 18/53} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 7/19} & {21/58} & {\color{red} 21/59} & {\color{red} 32/91} & {\color{red} 11/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {24/65} & {\color{red}  4/11} & {\color{red} 24/67} & { 9/25} & { 9/25} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {27/73} & {27/74} & { 9/25} & {\color{red} 27/76} & {\color{red} 27/77} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {10/27} & {15/41} & {\color{red} 30/83} & {\color{red}  5/14} \\\hline
$18$ & { 5/13} & { 8/23} & { 9/28} & { 1/ 3} & {11/31} & { 3/ 8} & { 5/13} & { 5/13} & { 6/17} & {12/35} & {13/37} & { 7/19} & { 5/13} & { 5/13} & { 9/25} & { 9/25} & { 5/14} & { 4/11} & {17/45} & { 5/13} & { 5/13} & { 1/ 3} & { 9/25} & {\color{red}  9/25} & {19/51} & { 5/13} & { 5/13} & {13/36} & {\color{red} 19/55} & { 5/14} & { 7/19} & {11/29} & { 5/13} & { 5/13} & { 7/20} & {\color{red} 11/31} & {23/63} & { 3/ 8} & { 5/13} & { 5/13} & {31/85} & {24/67} & {\color{red} 25/69} & {13/35} & {27/71} & { 5/13} & { 5/13} & { 9/25} & {\color{red}  9/25} & {\color{red}  7/19} & {29/77} & { 5/13} & { 5/13} & {18/49} & {\color{red} 29/81} & {15/41} & {31/83} & { 8/21} & { 5/13} & { 5/13} \\\hline
$19$ & {11/27} & {17/48} & { 9/29} & { 8/25} & { 3/ 8} & {13/33} & {11/27} & {11/27} & {\color{red} 19/55} & { 1/ 3} & { 7/19} & { 5/13} & { 2/ 5} & {11/27} & {24/61} & { 9/26} & {22/63} & {17/45} & { 9/23} & {19/47} & {11/27} & {13/34} & { 1/ 3} & {19/51} & { 5/13} & {21/53} & {11/27} & {11/27} & {28/75} & { 7/19} & {11/29} & {23/59} & { 2/ 5} & {11/27} & {11/27} & {15/41} & { 3/ 8} & { 5/13} & {13/33} & {27/67} & {11/27} & {35/88} & {13/35} & {27/71} & { 7/18} & {29/73} & {15/37} & {11/27} & {37/95} & {29/77} & { 5/13} & {31/79} & { 2/ 5} & {11/27} & {11/27} & {13/34} & { 8/21} & {33/85} & {17/43} & {35/87} \\\hline
$20$ & { 3/ 7} & { 9/25} & { 3/10} & { 4/13} & {20/53} & { 7/17} & { 3/ 7} & { 3/ 7} & { 7/19} & {\color{red} 19/58} & {\color{red} 20/59} & { 2/ 5} & {17/41} & { 3/ 7} & { 3/ 7} & { 3/ 8} & {\color{red}  1/ 3} & { 4/11} & {19/47} & { 5/12} & { 3/ 7} & { 3/ 7} & {27/71} & { 1/ 3} & {28/73} & {11/27} & {23/55} & { 3/ 7} & { 3/ 7} & { 5/13} & {28/79} & { 2/ 5} & {25/61} & {13/31} & { 3/ 7} & { 3/ 7} & {33/85} & {16/43} & {27/67} & { 7/17} & {29/69} & { 3/ 7} & { 3/ 7} & { 9/23} & {12/31} & {15/37} & {31/75} & { 8/19} & { 3/ 7} & { 3/ 7} & {13/33} & { 2/ 5} & {11/27} & {17/41} & {35/83} & { 3/ 7} & { 3/ 7} & {21/53} & {35/87} & { 9/22} \\\hline
$21$ & {12/29} & {19/52} & {\color{red} 16/53} & {\color{red}  8/27} & { 4/11} & { 3/ 7} & { 3/ 7} & { 5/12} & {23/59} & {\color{red}  1/ 3} & {\color{red} 20/61} & {23/62} & { 3/ 7} & { 3/ 7} & {18/43} & { 9/22} & {24/67} & {\color{red} 14/43} & {26/69} & { 3/ 7} & { 3/ 7} & {21/50} & { 7/17} & {14/37} & { 1/ 3} & {29/76} & { 3/ 7} & { 3/ 7} & { 8/19} & {12/29} & {32/81} & {29/82} & {32/83} & { 3/ 7} & { 3/ 7} & {27/64} & {27/65} & { 9/22} & {33/89} & { 7/18} & { 3/ 7} & { 3/ 7} & {30/71} & { 5/12} & {30/73} & {37/96} & {38/97} & { 3/ 7} & { 3/ 7} & {11/26} & {33/79} & {33/80} & {39/98} & {28/71} & { 3/ 7} & { 3/ 7} & {36/85} & {18/43} & {12/29} & { 9/22} \\\hline
$22$ & { 2/ 5} & {10/27} & {\color{red} 17/55} & {\color{red} 17/56} & {20/57} & {12/29} & {12/29} & {15/37} & {15/38} & {11/31} & {\color{red} 29/90} & {\color{red} 11/32} & { 2/ 5} & {12/29} & { 9/22} & { 2/ 5} & { 9/23} & {\color{red} 12/35} & {\color{red} 24/71} & { 7/18} & {12/29} & { 7/17} & {21/52} & {21/53} & {29/77} & { 1/ 3} & {30/79} & {12/29} & {12/29} & {24/59} & { 2/ 5} & {24/61} & {31/85} & {16/43} & {12/29} & {12/29} & { 9/22} & {27/67} & {27/68} & { 9/23} & {34/93} & {19/47} & {12/29} & {30/73} & {15/37} & { 2/ 5} & {15/38} & {19/50} & {21/53} & {12/29} & {33/80} & {11/27} & {33/82} & {33/83} & {11/28} & {\color{red} 16/43} & {12/29} & {12/29} & { 9/22} & {36/89} \\\hline
$23$ & {12/31} & { 3/ 8} & { 6/19} & {11/35} & {\color{red} 20/59} & { 2/ 5} & { 2/ 5} & {15/38} & { 5/13} & { 3/ 8} & { 1/ 3} & {15/43} & {25/67} & { 2/ 5} & { 2/ 5} & { 9/23} & {18/47} & { 3/ 8} & {11/31} & {11/31} & { 2/ 5} & { 2/ 5} & {21/53} & { 7/18} & {21/55} & { 3/ 8} & { 1/ 3} & {31/82} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 3/ 8} & {\color{red} 32/89} & { 2/ 5} & { 2/ 5} & {27/68} & { 9/23} & {27/70} & {27/71} & { 3/ 8} & {37/97} & { 2/ 5} & { 2/ 5} & {15/38} & {30/77} & { 5/13} & {30/79} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {33/83} & {11/28} & {33/85} & {33/86} & {11/29} & {\color{red} 37/97} & { 2/ 5} & { 2/ 5} \\\hline
$24$ & { 3/ 8} & { 4/11} & {19/59} & { 1/ 3} & {13/37} & {12/31} & {12/31} & { 5/13} & { 3/ 8} & {15/41} & {15/43} & { 4/11} & { 3/ 8} & {12/31} & {12/31} & {18/47} & { 3/ 8} & {\color{red} 18/49} & {19/51} & { 3/ 8} & { 4/11} & {12/31} & {12/31} & {21/55} & {\color{red}  3/ 8} & { 3/ 8} & { 3/ 8} & { 1/ 3} & {32/85} & {12/31} & {12/31} & { 8/21} & { 3/ 8} & {24/65} & { 4/11} & {\color{red}  6/17} & {12/31} & {12/31} & {27/70} & {27/71} & { 3/ 8} & {\color{red} 27/73} & {\color{red} 27/74} & {\color{red}  7/19} & {12/31} & {12/31} & { 5/13} & {30/79} & {\color{red}  3/ 8} & {\color{red} 10/27} & {31/83} & {\color{red}  3/ 8} & {12/31} & {12/31} & {33/86} & {\color{red} 11/29} & {\color{red}  3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 10/27} \\\hline
$25$ & {13/33} & {\color{red}  6/17} & {20/61} & {10/31} & { 7/19} & { 5/13} & {13/33} & {13/33} & {15/41} & { 5/14} & { 4/11} & {17/45} & { 9/23} & {13/33} & { 3/ 8} & { 3/ 8} & {18/49} & {19/51} & { 5/13} & {13/33} & {13/33} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {11/29} & {23/59} & {13/33} & {33/86} & { 1/ 3} & { 3/ 8} & {\color{red}  3/ 8} & { 5/13} & {13/33} & {13/33} & {\color{red} 34/93} & {25/69} & {13/35} & {27/71} & { 7/18} & {13/33} & {13/33} & {27/74} & {\color{red}  7/19} & {29/77} & { 5/13} & {31/79} & {13/33} & {\color{red} 20/53} & {\color{red} 10/27} & {\color{red} 31/83} & { 8/21} & {33/85} & {13/33} & {13/33} & { 3/ 8} & { 3/ 8} & {\color{red} 17/45} & { 5/13} & { 9/23} & {13/33} \\\hline
$26$ & { 7/17} & {11/31} & { 1/ 3} & {\color{red}  5/16} & { 5/13} & { 2/ 5} & { 7/17} & { 7/17} & { 5/14} & {15/43} & {25/71} & { 9/23} & {19/47} & { 7/17} & { 2/ 5} & { 4/11} & { 9/25} & { 5/13} & {21/53} & {11/27} & { 7/17} & {16/41} & { 4/11} & { 4/11} & {23/59} & { 2/ 5} & {25/61} & { 7/17} & {34/89} & { 1/ 3} & { 5/13} & {13/33} & {27/67} & { 7/17} & { 7/17} & { 3/ 8} & {35/97} & { 7/18} & {29/73} & {15/37} & { 7/17} & { 7/17} & {\color{red} 31/84} & { 5/13} & {31/79} & { 2/ 5} & {11/27} & { 7/17} & {23/57} & {\color{red}  4/11} & {33/85} & {17/43} & {35/87} & { 9/22} & { 7/17} & {23/58} & { 5/13} & { 9/23} & {37/93} & {19/47} \\\hline
$27$ & { 3/ 7} & {23/64} & {12/37} & {\color{red} 10/33} & {25/67} & {17/41} & { 3/ 7} & { 3/ 7} & {26/71} & {15/44} & {\color{red}  1/ 3} & {29/74} & { 5/12} & { 3/ 7} & { 3/ 7} & {29/78} & { 6/17} & {\color{red}  7/20} & {11/27} & {23/55} & { 3/ 7} & { 3/ 7} & {32/85} & {\color{red}  6/17} & {32/87} & {25/61} & {13/31} & { 3/ 7} & { 3/ 7} & {35/92} & { 1/ 3} & {18/47} & { 7/17} & {29/69} & { 3/ 7} & { 3/ 7} & {38/99} & {\color{red}  7/20} & {21/53} & {31/75} & { 8/19} & { 3/ 7} & { 3/ 7} & {29/75} & {\color{red} 35/96} & {11/27} & {17/41} & {35/83} & { 3/ 7} & { 3/ 7} & {37/95} & {\color{red} 32/87} & { 9/22} & {37/89} & {19/45} & { 3/ 7} & { 3/ 7} & {38/97} & {\color{red} 18/47} & {39/95} \\\hline
$28$ & { 5/12} & { 4/11} & { 6/19} & { 3/10} & {25/69} & { 3/ 7} & { 3/ 7} & {18/43} & {28/73} & {\color{red}  1/ 3} & {\color{red}  1/ 3} & { 7/19} & { 3/ 7} & { 3/ 7} & {21/50} & { 2/ 5} & {\color{red} 28/81} & {31/89} & {31/83} & { 3/ 7} & { 3/ 7} & { 8/19} & {12/29} & { 4/11} & {\color{red} 31/89} & {17/45} & { 3/ 7} & { 3/ 7} & {27/64} & {27/65} & {36/95} & { 1/ 3} & {37/97} & { 3/ 7} & { 3/ 7} & {30/71} & { 5/12} & {20/51} & {\color{red} 28/81} & {\color{red} 37/97} & { 3/ 7} & { 3/ 7} & {11/26} & {33/79} & {23/57} & {\color{red}  4/11} & {31/80} & { 3/ 7} & { 3/ 7} & {36/85} & {18/43} & {12/29} & {35/93} & {\color{red} 31/80} & { 3/ 7} & { 3/ 7} & {39/92} & {13/31} & {39/94} & {\color{red} 36/95} \\\hline
$29$ & {15/37} & {25/68} & {\color{red}  4/13} & {13/41} & {\color{red} 25/71} & { 5/12} & { 5/12} & { 9/22} & { 2/ 5} & {\color{red} 13/38} & {\color{red} 26/77} & {\color{red} 17/49} & {32/79} & { 5/12} & { 7/17} & {21/52} & {31/83} & {\color{red} 32/91} & {13/37} & {17/43} & { 5/12} & {12/29} & {24/59} & { 2/ 5} & {\color{red} 32/91} & {\color{red} 13/37} & {12/31} & { 5/12} & {27/65} & { 9/22} & {27/67} & {37/98} & { 1/ 3} & {19/50} & { 5/12} & { 5/12} & {30/73} & {15/37} & { 2/ 5} & {\color{red} 19/53} & {37/99} & { 5/12} & { 5/12} & {33/80} & {11/27} & {33/82} & {\color{red} 37/98} & {\color{red} 27/76} & {38/93} & { 5/12} & {12/29} & { 9/22} & {36/89} & { 2/ 5} & {\color{red} 19/53} & {39/97} & { 5/12} & {39/94} & {39/95} & {13/32} \\\hline
$30$ & {15/38} & {13/35} & {\color{red} 22/71} & { 1/ 3} & {\color{red} 15/43} & {15/37} & {15/37} & { 2/ 5} & { 9/23} & {14/39} & {17/49} & {\color{red}  9/25} & {31/81} & {15/37} & {21/52} & {21/53} & { 7/18} & { 5/14} & { 7/19} & { 7/19} & {15/37} & {15/37} & { 2/ 5} & {24/61} & {12/31} & { 7/19} & { 7/19} & {19/48} & {15/37} & {27/67} & {27/68} & { 9/23} & {35/93} & { 1/ 3} & {25/66} & {15/37} & {15/37} & { 2/ 5} & {15/38} & {30/77} & {\color{red} 14/39} & {\color{red}  4/11} & {15/37} & {15/37} & {33/82} & {33/83} & {11/28} & {33/85} & {\color{red} 31/86} & {23/59} & {15/37} & {36/89} & { 2/ 5} & {36/91} & { 9/23} & {12/31} & {\color{red} 31/84} & {15/37} & {15/37} & {39/97} \\\hline
$31$ & { 5/13} & { 3/ 8} & {\color{red} 23/73} & {12/37} & { 4/11} & {15/38} & {15/38} & { 9/23} & {18/47} & { 3/ 8} & { 9/25} & {19/51} & { 5/13} & {15/38} & {15/38} & { 7/18} & {21/55} & { 3/ 8} & {11/29} & { 5/13} & { 5/13} & {15/38} & {24/61} & {12/31} & {\color{red}  8/21} & { 5/13} & { 5/13} & { 5/14} & {15/38} & {15/38} & { 9/23} & {\color{red} 27/70} & { 5/13} & { 5/13} & { 1/ 3} & {20/53} & {15/38} & {15/38} & {30/77} & { 5/13} & {30/79} & { 3/ 8} & {\color{red} 15/41} & {15/38} & {15/38} & {11/28} & {33/85} & {33/86} & {\color{red} 11/29} & { 3/ 8} & {\color{red} 17/45} & {15/38} & {15/38} & { 9/23} & {12/31} & {\color{red} 18/47} & {\color{red} 36/95} & {37/97} & {\color{red}  5/13} & {15/38} \\\hline
$32$ & { 2/ 5} & {15/41} & { 8/25} & { 6/19} & {17/45} & { 9/23} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {18/49} & {30/83} & { 5/13} & {21/53} & { 2/ 5} & { 5/13} & {21/55} & { 3/ 8} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & { 5/13} & { 5/13} & { 8/21} & { 5/13} & {13/33} & { 2/ 5} & { 2/ 5} & {26/71} & { 5/13} & { 5/13} & { 7/18} & {29/73} & { 2/ 5} & {\color{red} 11/29} & {\color{red}  1/99} & {\color{red} 29/77} & {\color{red}  5/13} & {31/79} & { 2/ 5} & { 2/ 5} & {\color{red} 10/27} & {\color{red} 15/41} & { 8/21} & {33/85} & {17/43} & { 2/ 5} & { 2/ 5} & { 3/ 8} & {\color{red} 17/45} & { 5/13} & { 9/23} & {37/93} & { 2/ 5} & {\color{red} 23/60} & {36/95} & {\color{red} 37/97} & {19/49} & {13/33} & { 2/ 5} \\\hline
$33$ & {17/41} & {\color{red}  5/14} & {25/77} & {\color{red}  4/13} & {30/79} & {19/47} & {17/41} & {17/41} & {18/49} & { 9/25} & { 6/17} & {21/53} & {11/27} & {17/41} & {36/89} & { 3/ 8} & { 7/19} & {\color{red} 17/46} & { 2/ 5} & {25/61} & {17/41} & {19/48} & { 3/ 8} & { 3/ 8} & {13/33} & {27/67} & { 7/17} & {17/41} & {33/85} & { 3/ 8} & { 3/ 8} & {29/73} & {15/37} & {31/75} & {17/41} & {\color{red} 31/84} & {\color{red}  1/99} & {\color{red} 30/79} & { 2/ 5} & {11/27} & {17/41} & {17/41} & {\color{red} 30/83} & {\color{red}  5/14} & {17/43} & {35/87} & { 9/22} & {\color{red} 12/29} & {17/41} & {\color{red} 11/30} & {\color{red} 17/46} & {37/93} & {19/47} & {39/95} & {17/41} & {\color{red} 19/48} & {\color{red} 36/97} & {13/33} & { 2/ 5} & {28/69} \\\hline
$34$ & { 3/ 7} & {\color{red} 14/39} & {26/79} & {\color{red}  5/16} & {10/27} & { 5/12} & { 3/ 7} & { 3/ 7} & {\color{red} 31/85} & { 6/17} & {\color{red}  9/26} & {17/44} & {23/55} & { 3/ 7} & { 3/ 7} & {\color{red} 17/46} & {\color{red} 21/58} & {\color{red} 21/59} & { 2/ 5} & {13/31} & { 3/ 7} & { 3/ 7} & {\color{red} 37/99} & {\color{red} 15/41} & { 4/11} & { 7/17} & {29/69} & { 3/ 7} & { 3/ 7} & {20/53} & {15/41} & {\color{red} 10/27} & {31/75} & { 8/19} & { 3/ 7} & { 3/ 7} & {\color{red} 20/53} & {\color{red}  1/99} & {\color{red}  3/ 8} & {17/41} & {35/83} & { 3/ 7} & { 3/ 7} & {\color{red} 35/92} & {\color{red}  1/99} & {\color{red} 17/44} & {37/89} & {19/45} & { 3/ 7} & { 3/ 7} & {\color{red} 35/92} & {\color{red}  1/99} & {\color{red}  2/ 5} & { 5/12} & {41/97} & { 3/ 7} & { 3/ 7} & {\color{red} 35/92} & {\color{red}  1/99} & { 7/17} \\\hline
$35$ & {18/43} & {29/80} & { 1/ 3} & {15/47} & {30/83} & { 3/ 7} & { 3/ 7} & {21/50} & {11/29} & { 9/26} & {\color{red} 31/89} & {11/30} & { 3/ 7} & { 3/ 7} & { 8/19} & {37/94} & {\color{red} 21/59} & {\color{red} 27/76} & {36/97} & { 3/ 7} & { 3/ 7} & {27/64} & {28/69} & {\color{red}  5/14} & {\color{red} 23/64} & { 3/ 8} & { 3/ 7} & { 3/ 7} & {30/71} & { 5/12} & {\color{red} 29/79} & {\color{red}  5/14} & {14/37} & { 3/ 7} & { 3/ 7} & {11/26} & {33/79} & {11/29} & {\color{red}  1/99} & {\color{red} 14/37} & { 3/ 7} & { 3/ 7} & {36/85} & {18/43} & {\color{red} 18/47} & {\color{red}  1/99} & {\color{red} 14/37} & { 3/ 7} & { 3/ 7} & {39/92} & {13/31} & {\color{red} 37/94} & {\color{red}  1/99} & {\color{red} 14/37} & { 3/ 7} & { 3/ 7} & {14/33} & {21/50} & {\color{red} 28/69} & {\color{red}  1/99} \\\hline
$36$ & { 9/22} & {15/41} & {15/46} & { 1/ 3} & {\color{red}  6/17} & {18/43} & {18/43} & { 7/17} & {35/89} & {\color{red} 31/90} & {\color{red} 32/91} & {\color{red}  5/14} & {38/93} & {18/43} & {12/29} & {24/59} & {35/97} & {\color{red} 34/95} & { 4/11} & { 2/ 5} & {18/43} & {27/65} & { 9/22} & {\color{red} 25/67} & {\color{red} 25/69} & {\color{red}  4/11} & {31/79} & {18/43} & { 5/12} & {30/73} & {15/37} & {\color{red}  4/11} & { 4/11} & {\color{red} 37/99} & {18/43} & {33/79} & {33/80} & {11/27} & {\color{red} 15/41} & {\color{red}  1/99} & {\color{red} 27/76} & {18/43} & {18/43} & {12/29} & { 9/22} & {\color{red} 35/89} & {\color{red}  1/99} & {\color{red} 32/91} & {\color{red} 38/93} & {\color{red}  5/12} & {39/94} & {39/95} & {13/32} & {\color{red} 35/97} & {\color{red}  1/99} & {\color{red}  2/ 5} & {\color{red} 38/91} & {37/89} & { 7/17} & {31/76} \\\hline
$37$ & { 2/ 5} & {31/84} & {\color{red} 15/47} & {14/43} & { 9/25} & { 9/22} & { 9/22} & {21/52} & {21/53} & {\color{red}  8/23} & { 5/14} & {\color{red}  7/19} & {37/95} & { 9/22} & {24/59} & { 2/ 5} & {38/99} & {23/63} & { 3/ 8} & {\color{red} 17/45} & { 9/22} & { 9/22} & {27/67} & {27/68} & {\color{red} 13/35} & {17/45} & {17/45} & { 9/22} & { 9/22} & {15/37} & { 2/ 5} & {15/38} & {17/45} & {\color{red} 29/83} & {\color{red} 37/95} & { 9/22} & {11/27} & {33/82} & {33/83} & {\color{red} 17/45} & {\color{red}  1/99} & {\color{red} 19/51} & { 9/22} & { 9/22} & {36/89} & { 2/ 5} & {36/91} & {\color{red}  1/99} & {\color{red} 17/47} & { 9/22} & { 9/22} & {13/32} & {39/97} & {39/98} & {\color{red} 38/99} & {\color{red} 26/71} & {\color{red} 35/89} & { 9/22} & {31/76} & {21/52} \\\hline
$38$ & { 9/23} & {16/43} & {\color{red}  5/16} & {\color{red}  7/22} & {19/51} & { 2/ 5} & { 2/ 5} & {21/53} & { 7/18} & {17/47} & { 7/19} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 3/ 8} & { 5/13} & { 9/23} & { 2/ 5} & { 2/ 5} & {27/68} & { 9/23} & {\color{red} 27/70} & { 7/18} & { 9/23} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {15/38} & {\color{red} 30/77} & { 9/23} & { 9/23} & {\color{red} 15/43} & { 2/ 5} & { 2/ 5} & {33/83} & {\color{red} 11/28} & { 9/23} & {\color{red} 16/43} & {\color{red}  1/99} & {\color{red} 36/97} & { 2/ 5} & { 2/ 5} & {36/91} & { 9/23} & {12/31} & { 7/19} & { 3/ 8} & { 2/ 5} & { 2/ 5} & {39/98} & {13/33} & {23/59} & {22/57} & {\color{red} 25/66} & {\color{red}  5/13} & { 2/ 5} & { 2/ 5} \\\hline
$39$ & {19/47} & { 3/ 8} & {\color{red} 28/89} & {\color{red} 14/45} & { 5/13} & {21/53} & {19/47} & {19/47} & {21/55} & { 3/ 8} & {\color{red} 34/97} & {23/59} & { 2/ 5} & {19/47} & {\color{red}  9/23} & {12/31} & { 8/21} & { 5/13} & {13/33} & {27/67} & {19/47} & { 9/23} & { 9/23} & {27/70} & { 7/18} & {29/73} & {19/47} & {19/47} & { 9/23} & { 9/23} & {30/77} & {31/79} & { 2/ 5} & {19/47} & {\color{red} 22/57} & {\color{red} 35/99} & { 9/23} & { 9/23} & {17/43} & {35/87} & {19/47} & {\color{red} 35/93} & {\color{red}  1/99} & { 5/13} & {\color{red}  9/23} & {37/93} & {19/47} & {19/47} & {\color{red} 36/95} & { 3/ 8} & {19/49} & {13/33} & { 2/ 5} & {\color{red} 23/57} & {\color{red} 25/63} & {13/34} & { 5/13} & {25/64} & {21/53} & {39/97} \\\hline
$40$ & { 5/12} & {18/49} & {\color{red} 29/91} & {\color{red}  4/13} & {35/93} & {11/27} & { 5/12} & { 5/12} & { 3/ 8} & { 7/19} & {\color{red} 34/99} & { 2/ 5} & {25/61} & { 5/12} & {31/76} & { 8/21} & { 3/ 8} & {\color{red} 24/65} & {27/67} & { 7/17} & { 5/12} & {\color{red} 33/85} & {18/47} & {27/71} & {\color{red} 35/93} & {15/37} & {31/75} & { 5/12} & {\color{red} 21/55} & {18/47} & {18/47} & { 2/ 5} & {11/27} & {17/41} & { 5/12} & {\color{red}  4/11} & {\color{red} 31/86} & {18/47} & {35/87} & { 9/22} & {37/89} & { 5/12} & {\color{red} 11/30} & {\color{red}  1/99} & {\color{red} 35/93} & {19/47} & {39/95} & { 5/12} & { 5/12} & {\color{red} 36/97} & {\color{red}  1/99} & { 2/ 5} & {28/69} & { 7/17} & {\color{red} 12/29} & {\color{red} 31/76} & {\color{red}  1/99} & {\color{red}  1/99} & {39/97} & {11/27} \\\hline
$41$ & { 3/ 7} & {\color{red}  9/25} & {\color{red}  6/19} & {\color{red} 17/53} & { 7/19} & {23/55} & { 3/ 7} & { 3/ 7} & {\color{red}  7/19} & {21/58} & {\color{red} 26/75} & {13/34} & {13/31} & { 3/ 7} & { 3/ 7} & { 3/ 8} & {24/65} & {\color{red}  4/11} & {28/71} & {29/69} & { 3/ 7} & { 3/ 7} & {\color{red}  3/ 8} & { 3/ 8} & {\color{red} 27/73} & {\color{red}  2/ 5} & { 8/19} & { 3/ 7} & { 3/ 7} & { 3/ 8} & {\color{red}  3/ 8} & { 3/ 8} & {17/41} & {35/83} & { 3/ 7} & { 3/ 7} & {\color{red}  4/11} & { 3/ 8} & {\color{red}  3/ 8} & {37/89} & {19/45} & { 3/ 7} & { 3/ 7} & {\color{red} 32/87} & {\color{red}  1/99} & {13/34} & { 5/12} & {41/97} & { 3/ 7} & { 3/ 7} & {\color{red} 29/78} & {\color{red}  1/99} & {\color{red} 37/96} & {38/91} & {11/26} & { 3/ 7} & { 3/ 7} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red} 28/71} \\\hline
$42$ & {21/50} & {\color{red} 17/47} & {\color{red} 22/69} & { 1/ 3} & {\color{red} 35/97} & { 3/ 7} & { 3/ 7} & { 8/19} & {35/93} & {21/59} & {\color{red}  7/20} & {\color{red} 19/52} & { 3/ 7} & { 3/ 7} & {27/64} & { 7/18} & { 4/11} & {\color{red}  4/11} & {24/65} & { 3/ 7} & { 3/ 7} & {30/71} & {\color{red} 31/79} & {\color{red} 18/49} & {\color{red} 25/68} & {\color{red} 24/65} & { 3/ 7} & { 3/ 7} & {11/26} & {\color{red} 32/79} & {\color{red} 18/49} & {\color{red} 18/49} & {\color{red} 24/65} & { 3/ 7} & { 3/ 7} & {36/85} & {18/43} & {\color{red} 17/47} & {\color{red}  1/99} & {\color{red} 18/49} & { 3/ 7} & { 3/ 7} & {39/92} & {13/31} & {\color{red} 35/93} & {\color{red}  1/99} & {\color{red} 24/65} & { 3/ 7} & { 3/ 7} & {14/33} & {21/50} & { 7/18} & {\color{red}  1/99} & {\color{red} 24/65} & { 3/ 7} & { 3/ 7} & {31/73} & {37/88} & {\color{red}  9/23} & {\color{red}  1/99} \\\hline
$43$ & { 7/17} & {35/96} & {\color{red} 17/53} & {\color{red} 29/92} & {\color{red}  5/14} & {21/50} & {21/50} & {12/29} & {33/85} & {\color{red}  7/20} & {11/31} & {\color{red} 23/63} & {\color{red}  2/ 5} & {21/50} & {27/65} & { 9/22} & {\color{red} 24/67} & {\color{red} 25/69} & {\color{red} 13/35} & {\color{red} 27/71} & {21/50} & { 5/12} & {30/73} & {\color{red} 35/96} & {\color{red} 27/73} & {19/51} & {\color{red} 22/57} & {21/50} & {33/79} & {33/80} & {\color{red} 33/85} & {\color{red} 19/51} & {\color{red} 19/51} & {\color{red} 31/85} & {21/50} & {18/43} & {12/29} & { 9/22} & {19/51} & {\color{red}  1/99} & {\color{red}  9/25} & {21/50} & {13/31} & {39/94} & {39/95} & {\color{red} 19/51} & {\color{red}  1/99} & {\color{red}  9/25} & {21/50} & {21/50} & {37/89} & { 7/17} & {\color{red} 33/85} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/90} & {\color{red} 34/81} & { 5/12} & {26/63} & { 9/22} \\\hline
$44$ & {21/52} & {18/49} & { 1/ 3} & { 8/25} & { 7/19} & { 7/17} & { 7/17} & {24/59} & { 2/ 5} & {\color{red} 21/61} & {23/63} & { 3/ 8} & {\color{red} 31/80} & { 7/17} & { 9/22} & {27/67} & {\color{red} 18/49} & {13/35} & {27/71} & {\color{red}  5/13} & { 7/17} & {30/73} & {15/37} & { 2/ 5} & {29/77} & { 5/13} & { 5/13} & { 7/17} & { 7/17} & {11/27} & {33/82} & {\color{red}  8/21} & { 5/13} & { 5/13} & {\color{red} 28/71} & { 7/17} & { 9/22} & {36/89} & { 2/ 5} & { 5/13} & {\color{red}  1/99} & {\color{red} 17/47} & { 7/17} & {39/95} & {13/32} & {39/97} & { 5/13} & {\color{red}  1/99} & {\color{red} 26/71} & { 7/17} & { 7/17} & {31/76} & {21/52} & { 2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 32/81} & {\color{red} 37/90} & { 9/22} & {15/37} \\\hline
$45$ & {21/53} & {27/73} & {18/55} & {\color{red} 25/83} & {11/29} & {21/52} & {21/52} & { 2/ 5} & {24/61} & {\color{red} 19/54} & {\color{red} 27/77} & { 5/13} & {13/33} & {21/52} & {27/67} & {27/68} & { 9/23} & {27/71} & { 7/18} & {21/53} & {21/52} & {21/52} & { 2/ 5} & {15/38} & { 5/13} & {31/79} & {21/53} & {\color{red} 34/89} & {21/52} & {33/82} & {33/83} & {\color{red} 11/28} & {17/43} & {21/53} & {\color{red} 35/96} & {21/52} & {21/52} & { 2/ 5} & {\color{red} 36/91} & {21/53} & {21/53} & {\color{red}  1/99} & {\color{red}  5/13} & {21/52} & {39/97} & {\color{red} 39/98} & {21/53} & {\color{red} 29/78} & {\color{red}  1/99} & {\color{red} 16/51} & {21/52} & {21/52} & { 2/ 5} & {21/53} & {31/79} & {\color{red}  1/99} & {21/55} & {\color{red}  7/18} & {\color{red} 25/62} & {39/97} \\\hline
$46$ & {11/27} & {19/51} & {\color{red}  9/28} & {\color{red}  9/29} & { 8/21} & { 2/ 5} & {11/27} & {11/27} & {12/31} & {\color{red}  6/17} & {\color{red} 33/98} & {13/33} & {27/67} & {11/27} & {\color{red} 21/53} & { 9/23} & {27/70} & {\color{red} 21/58} & {29/73} & {15/37} & {11/27} & {21/53} & {15/38} & {30/77} & {31/79} & { 2/ 5} & {11/27} & {11/27} & {21/53} & {21/53} & {11/28} & {17/43} & {35/87} & {11/27} & {\color{red} 17/44} & {\color{red} 18/49} & {21/53} & {36/91} & {37/93} & {19/47} & {11/27} & {\color{red}  7/19} & {\color{red}  1/99} & {21/53} & {21/53} & { 2/ 5} & {28/69} & {11/27} & {\color{red} 19/51} & {\color{red}  1/99} & {\color{red} 20/63} & {\color{red} 21/53} & {39/97} & {11/27} & {11/27} & {37/96} & {\color{red}  1/99} & {11/28} & {39/98} & {23/57} \\\hline
$47$ & {23/55} & { 3/ 8} & {\color{red}  2/ 7} & {\color{red} 19/59} & {\color{red} 32/87} & {25/61} & {23/55} & {\color{red} 31/76} & { 8/21} & { 3/ 8} & {\color{red} 32/95} & {\color{red} 26/67} & { 7/17} & {\color{red} 38/91} & {\color{red}  9/23} & {27/70} & {27/71} & { 3/ 8} & {15/37} & {31/75} & {23/55} & {\color{red}  7/18} & {\color{red} 33/85} & { 5/13} & {\color{red} 30/79} & {11/27} & {17/41} & {23/55} & {\color{red} 31/83} & { 7/18} & {33/85} & {\color{red} 33/86} & { 9/22} & {37/89} & {23/55} & {\color{red} 11/30} & {\color{red} 27/73} & { 7/18} & {19/47} & {39/95} & { 5/12} & {23/55} & {\color{red} 35/97} & {\color{red}  1/99} & {\color{red} 27/73} & {28/69} & { 7/17} & {38/91} & {23/55} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red} 17/53} & {11/27} & {26/63} & {23/55} & {23/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 15/38} & {38/93} \\\hline
$48$ & { 3/ 7} & { 7/19} & {\color{red} 23/74} & { 1/ 3} & {\color{red}  9/25} & {13/31} & { 3/ 7} & { 3/ 7} & { 3/ 8} & {24/65} & {\color{red} 23/67} & {\color{red} 28/75} & {29/69} & { 3/ 7} & { 3/ 7} & {27/71} & { 3/ 8} & {\color{red} 27/73} & {16/41} & { 8/19} & { 3/ 7} & { 3/ 7} & {\color{red} 30/79} & {30/79} & {\color{red}  3/ 8} & {\color{red} 35/89} & {35/83} & { 3/ 7} & { 3/ 7} & {\color{red} 32/87} & {\color{red} 21/55} & {11/29} & {\color{red} 36/89} & {19/45} & { 3/ 7} & { 3/ 7} & {\color{red} 17/47} & {\color{red} 19/51} & {\color{red} 36/95} & { 5/12} & {41/97} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {38/91} & {11/26} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {23/55} & {36/85} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  8/23} \\\hline
$49$ & { 8/19} & {\color{red} 21/58} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 21/59} & { 3/ 7} & { 3/ 7} & {27/64} & {\color{red} 24/65} & { 4/11} & {\color{red}  6/17} & {\color{red} 25/69} & { 3/ 7} & { 3/ 7} & {30/71} & {\color{red} 30/79} & {27/73} & {\color{red} 27/74} & {\color{red}  7/19} & { 3/ 7} & { 3/ 7} & {11/26} & {17/43} & { 3/ 8} & {\color{red} 10/27} & {\color{red}  7/19} & { 3/ 7} & { 3/ 7} & {36/85} & {\color{red} 37/93} & {\color{red}  3/ 8} & {\color{red}  3/ 8} & {\color{red} 33/89} & { 3/ 7} & { 3/ 7} & {39/92} & {\color{red} 38/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {14/33} & {21/50} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {31/73} & {37/88} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {31/73} & { 8/19} & {\color{red} 37/96} & {\color{red}  1/99} \\\hline
$50$ & {12/29} & {\color{red}  4/11} & {\color{red}  1/99} & {\color{red}  1/99} & {23/63} & {\color{red} 37/90} & {\color{red} 37/88} & {27/65} & {\color{red} 36/95} & {24/67} & {25/69} & {\color{red} 13/35} & {\color{red} 23/57} & {\color{red} 37/88} & { 5/12} & {\color{red} 29/73} & {\color{red} 27/74} & {\color{red}  7/19} & {29/77} & {\color{red}  5/13} & {\color{red} 37/88} & {33/79} & {33/80} & {\color{red} 32/87} & {\color{red} 31/83} & {\color{red} 25/66} & {\color{red} 25/66} & {\color{red} 37/88} & {18/43} & {12/29} & {\color{red} 33/89} & {\color{red} 17/45} & {\color{red} 25/66} & {\color{red} 17/46} & { 8/19} & {13/31} & {39/94} & {\color{red} 37/95} & {\color{red} 25/66} & {\color{red} 25/66} & {\color{red} 18/49} & { 8/19} & {21/50} & {37/89} & { 7/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 11/35} & { 8/19} & {37/88} & { 5/12} & {26/63} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/19} & { 8/19} & {38/91} & {12/29} & {\color{red}  5/13} \\\hline
$51$ & {24/59} & {\color{red} 35/97} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 8} & {12/29} & {12/29} & { 9/22} & {\color{red} 26/67} & { 6/17} & {\color{red}  5/14} & {27/71} & {\color{red} 37/94} & {12/29} & {30/73} & {15/37} & {\color{red}  9/25} & {29/77} & { 5/13} & {\color{red} 33/85} & {12/29} & {33/80} & {11/27} & {\color{red} 31/82} & { 8/21} & {33/85} & {\color{red} 33/85} & {12/29} & {12/29} & { 9/22} & {36/89} & { 5/13} & {\color{red} 19/49} & {\color{red}  8/21} & {\color{red} 37/94} & {12/29} & {39/95} & {13/32} & {\color{red} 19/49} & {\color{red} 19/49} & {\color{red}  1/99} & {\color{red} 35/93} & {\color{red}  7/17} & { 7/17} & {31/76} & {21/52} & {\color{red}  8/21} & {\color{red}  1/99} & {\color{red} 17/53} & {12/29} & {26/63} & { 9/22} & {15/37} & {\color{red} 26/71} & {\color{red}  1/99} & {\color{red}  1/99} & {12/29} & {12/29} & {16/39} & {24/59} \\\hline
$52$ & { 2/ 5} & { 7/19} & {\color{red} 10/31} & {\color{red}  1/99} & { 5/13} & {\color{red} 19/48} & {\color{red} 13/32} & {27/67} & {27/68} & {\color{red}  8/23} & {\color{red} 12/35} & { 7/18} & {29/73} & {\color{red} 13/32} & {15/37} & { 2/ 5} & {\color{red} 34/91} & { 5/13} & {31/79} & { 2/ 5} & {\color{red} 13/32} & {\color{red} 13/32} & {33/82} & {33/83} & {33/85} & {17/43} & { 2/ 5} & { 2/ 5} & {\color{red} 13/32} & {36/89} & { 2/ 5} & {\color{red}  9/23} & {37/93} & { 2/ 5} & {\color{red} 37/99} & {\color{red} 13/32} & {13/32} & {39/97} & {\color{red} 39/98} & { 2/ 5} & { 2/ 5} & {\color{red}  1/99} & {\color{red} 33/85} & {\color{red} 21/52} & {21/52} & {\color{red}  2/ 5} & {\color{red} 39/98} & {\color{red} 37/99} & {\color{red}  1/99} & {\color{red}  1/ 3} & {\color{red} 15/37} & {15/37} & {\color{red} 39/97} & { 2/ 5} & {\color{red}  7/19} & {\color{red}  1/99} & {\color{red}  1/99} & {24/59} & {24/59} & {25/62} \\\hline
$53$ & {25/61} & {\color{red} 31/85} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 16/43} & {27/67} & {\color{red}  9/22} & {\color{red}  2/ 5} & { 9/23} & {\color{red} 11/31} & {\color{red} 24/71} & {29/73} & {15/37} & {\color{red}  9/22} & { 2/ 5} & {15/38} & {30/77} & {\color{red}  4/11} & { 2/ 5} & {11/27} & {\color{red}  9/22} & { 2/ 5} & {33/83} & {11/28} & {\color{red} 33/86} & {35/87} & { 9/22} & {\color{red}  9/22} & { 2/ 5} & { 2/ 5} & {36/91} & {37/93} & {19/47} & {\color{red} 38/93} & {\color{red}  2/ 5} & { 2/ 5} & { 2/ 5} & {39/98} & { 2/ 5} & {28/69} & {\color{red} 11/27} & {\color{red} 13/34} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & {39/97} & {11/27} & {\color{red} 38/93} & {\color{red} 29/79} & {\color{red}  1/99} & {\color{red} 26/71} & { 2/ 5} & {23/57} & {38/93} & {25/61} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  2/ 5} & {32/79} \\\hline
$54$ & {13/31} & {\color{red} 23/63} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 27/74} & { 7/17} & {\color{red} 31/74} & {\color{red} 16/39} & {27/70} & {\color{red} 25/71} & {\color{red} 25/73} & {\color{red} 22/57} & {31/75} & {\color{red} 31/74} & {\color{red} 15/38} & {30/77} & { 5/13} & {\color{red}  1/ 3} & {11/27} & {17/41} & {\color{red} 23/55} & {\color{red} 11/28} & {11/28} & {33/85} & {33/86} & { 9/22} & {37/89} & {\color{red} 23/55} & {\color{red} 38/99} & {\color{red} 31/79} & { 9/23} & {\color{red} 12/31} & {39/95} & { 5/12} & {\color{red} 23/55} & {\color{red} 36/97} & {\color{red} 31/79} & {\color{red} 31/79} & {\color{red} 23/59} & { 7/17} & {38/91} & {\color{red} 23/55} & {\color{red} 19/52} & {\color{red} 31/88} & {\color{red} 31/79} & {11/27} & {26/63} & {23/55} & {\color{red} 31/74} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/58} & {38/93} & {12/29} & {31/74} & {13/31} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {25/61} \\\hline
$55$ & { 3/ 7} & { 3/ 8} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 15/41} & {29/69} & { 3/ 7} & { 3/ 7} & {27/71} & { 3/ 8} & {\color{red} 13/37} & {\color{red} 33/89} & { 8/19} & { 3/ 7} & { 3/ 7} & { 5/13} & {30/79} & { 3/ 8} & {\color{red} 34/89} & {35/83} & { 3/ 7} & { 3/ 7} & {\color{red} 12/31} & {33/86} & {\color{red} 11/29} & {19/48} & {19/45} & { 3/ 7} & { 3/ 7} & {\color{red} 12/31} & {12/31} & {\color{red} 18/47} & {\color{red} 39/98} & {41/97} & { 3/ 7} & { 3/ 7} & {\color{red}  9/25} & {\color{red} 22/57} & {22/57} & {\color{red} 31/76} & {11/26} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 35/96} & {\color{red}  1/99} & {23/55} & {36/85} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {31/74} & {25/59} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$56$ & {27/64} & {24/65} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 25/69} & { 3/ 7} & { 3/ 7} & {30/71} & {\color{red}  3/ 8} & {27/73} & { 9/25} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {11/26} & {\color{red} 30/79} & { 3/ 8} & {\color{red} 10/27} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {36/85} & {\color{red} 12/31} & {11/29} & {\color{red}  3/ 8} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {39/92} & { 2/ 5} & {\color{red} 36/95} & {\color{red} 36/95} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {14/33} & {\color{red} 39/97} & {\color{red} 28/99} & {\color{red} 25/66} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {31/73} & {\color{red} 37/90} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {31/73} & { 8/19} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 7} & { 3/ 7} & {17/40} & {35/83} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$57$ & {27/65} & {\color{red}  4/11} & {\color{red}  1/99} & {\color{red}  1/99} & {13/35} & {\color{red} 31/75} & {\color{red} 35/83} & { 5/12} & {\color{red}  3/ 8} & {27/74} & { 7/19} & {\color{red} 29/77} & {\color{red} 31/78} & {\color{red}  8/19} & {33/79} & {\color{red} 28/71} & {\color{red} 10/27} & {\color{red} 31/83} & { 8/21} & {\color{red} 33/85} & {\color{red} 37/88} & {18/43} & {12/29} & {\color{red}  1/99} & {\color{red} 17/45} & { 5/13} & {\color{red}  5/13} & {\color{red}  8/19} & {13/31} & {39/94} & {\color{red}  1/99} & {\color{red} 37/97} & { 5/13} & {\color{red}  5/13} & {\color{red} 37/88} & {21/50} & {37/89} & {\color{red} 25/66} & {\color{red}  5/13} & {\color{red}  5/13} & {\color{red} 13/35} & {\color{red}  8/19} & {37/88} & { 5/12} & {\color{red} 28/71} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  8/19} & { 8/19} & {38/91} & {12/29} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 35/83} & {35/83} & {28/67} & {17/41} & {\color{red}  1/99} \\\hline
$58$ & { 9/22} & {\color{red} 32/89} & {\color{red}  1/99} & {\color{red}  1/99} & {27/71} & {\color{red} 28/69} & {\color{red} 39/94} & {30/73} & {\color{red} 37/96} & { 9/25} & {\color{red}  1/99} & { 5/13} & {\color{red} 21/53} & {\color{red} 39/94} & {33/80} & {11/27} & {\color{red} 15/41} & { 8/21} & {33/85} & {\color{red} 13/33} & {\color{red} 39/94} & {12/29} & { 9/22} & {\color{red} 32/87} & { 5/13} & { 9/23} & {13/33} & {\color{red} 39/94} & {39/94} & {39/95} & {\color{red} 19/48} & {19/49} & {13/33} & {13/33} & {\color{red} 28/69} & {\color{red} 17/41} & { 7/17} & {31/76} & {25/64} & {\color{red} 11/28} & {\color{red} 31/82} & {\color{red}  7/18} & {\color{red} 12/29} & {26/63} & { 9/22} & {\color{red} 11/28} & {\color{red} 11/28} & {\color{red}  1/99} & {\color{red} 37/99} & {\color{red} 12/29} & {12/29} & {16/39} & {24/59} & {\color{red} 31/82} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 17/41} & {17/41} & {37/90} & {31/76} \\\hline
$59$ & {27/67} & {\color{red} 33/91} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  3/ 8} & { 9/22} & { 9/22} & {15/37} & { 2/ 5} & {\color{red} 10/37} & {\color{red}  1/99} & {31/79} & { 2/ 5} & { 9/22} & {11/27} & {33/82} & {\color{red} 33/91} & {\color{red} 31/85} & {17/43} & {35/87} & { 9/22} & { 9/22} & {36/89} & { 2/ 5} & { 9/23} & {37/93} & {\color{red} 39/97} & { 9/22} & { 9/22} & {13/32} & {39/97} & {13/33} & { 2/ 5} & {\color{red} 39/97} & {\color{red} 22/57} & { 9/22} & {31/76} & {21/52} & { 2/ 5} & {39/97} & {\color{red} 39/97} & {\color{red}  1/99} & { 9/22} & { 9/22} & {15/37} & {\color{red} 39/97} & {\color{red}  2/ 5} & {\color{red} 15/38} & {\color{red}  1/99} & {\color{red}  5/13} & {\color{red} 24/59} & {24/59} & {\color{red} 25/62} & {\color{red}  2/ 5} & {\color{red} 29/78} & {\color{red}  1/99} & {\color{red} 20/61} & {\color{red} 31/76} & {31/76} & {\color{red} 17/42} \\\hline
$60$ & { 7/17} & {\color{red} 35/96} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 34/93} & {15/37} & { 7/17} & { 7/17} & {15/38} & {\color{red}  1/99} & {\color{red}  1/99} & { 2/ 5} & {11/27} & { 7/17} & {33/82} & {33/83} & {\color{red}  8/21} & {\color{red}  1/99} & {35/87} & { 9/22} & { 7/17} & {\color{red} 39/97} & { 2/ 5} & {36/91} & {\color{red} 29/78} & {19/47} & {39/95} & { 7/17} & {\color{red} 39/97} & {39/97} & {39/98} & { 2/ 5} & {28/69} & { 7/17} & { 7/17} & {\color{red} 11/28} & {\color{red} 39/97} & { 2/ 5} & {39/97} & {11/27} & {\color{red} 25/61} & {\color{red} 28/71} & {\color{red} 29/75} & {\color{red} 39/97} & {39/97} & {23/57} & {38/93} & {\color{red} 25/61} & {\color{red} 11/29} & {\color{red}  1/99} & {\color{red} 32/81} & {\color{red}  2/ 5} & {32/79} & {25/61} & {\color{red} 25/61} & {\color{red} 15/41} & {\color{red}  1/99} & {\color{red} 10/31} & {\color{red} 24/85} & {13/32} \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 3, 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g4-a03b05.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 3/10} & { 3/11} & { 1/ 4} & {\color{red}  3/11} & {\color{red}  5/17} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/19} & { 3/10} & { 2/ 7} & {\color{red}  7/25} & {\color{red}  4/13} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 9/28} & { 9/29} & { 3/10} & {\color{red}  5/17} & {\color{red} 11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 6/19} & { 4/13} & {\color{red} 13/43} & {\color{red}  7/22} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {15/46} & {15/47} & { 5/16} & {\color{red}  4/13} & {\color{red} 17/53} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {18/55} & { 9/28} & { 6/19} & {\color{red} 19/61} & {\color{red} 10/31} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {21/64} & {21/65} & { 7/22} & {\color{red} 11/35} & {\color{red} 23/71} & { 1/ 3} \\\hline
$2$ & {\color{red}  3/11} && { 5/17} && { 6/19} && { 1/ 3} && { 8/23} && { 9/25} && {10/27} && {11/29} && {12/31} && {13/33} && { 2/ 5} && {15/37} && {16/39} && {17/41} && {18/43} && {19/45} && {20/47} && { 3/ 7} && {22/51} && {23/53} && {24/55} && {25/57} && {26/59} && {27/61} && { 4/ 9} && {29/65} && {30/67} && {31/69} && {32/71} && {33/73} &\\\hline
$3$ & {\color{red}  6/23} & { 4/13} & { 1/ 4} & { 4/13} & { 1/ 4} & { 4/13} & { 3/11} & { 4/13} & {\color{red}  3/11} & { 4/13} & {\color{red}  7/24} & {\color{red}  2/ 7} & { 4/13} & {\color{red} 18/67} & { 4/13} & { 8/29} & { 4/13} & {\color{red}  8/29} & { 4/13} & {\color{red}  8/29} & { 4/13} & {\color{red}  2/ 7} & { 4/13} & {\color{red} 11/37} & {\color{red} 12/41} & { 4/13} & {\color{red} 26/93} & { 4/13} & { 2/ 7} & { 4/13} & { 2/ 7} & { 4/13} & {\color{red}  2/ 7} & { 4/13} & {\color{red}  7/24} & { 4/13} & {\color{red}  3/10} & {\color{red}  8/27} & { 4/13} & {\color{red}  2/ 7} & { 4/13} & {16/55} & { 4/13} & {16/55} & { 4/13} & {\color{red} 16/55} & { 4/13} & {\color{red} 18/61} & { 4/13} & {\color{red} 19/63} & {\color{red} 20/67} & { 4/13} & {\color{red} 20/69} & { 4/13} & { 5/17} & { 4/13} & { 5/17} & { 4/13} & {\color{red}  5/17} & { 4/13} \\\hline
$4$ & {\color{red}  2/ 7} && { 2/ 7} && { 7/23} && { 8/25} && { 1/ 3} && {10/29} && {11/31} && { 4/11} && {13/35} && {14/37} && { 5/13} && {16/41} && {17/43} && { 2/ 5} && {19/47} && {20/49} && { 7/17} && {22/53} && {23/55} && { 8/19} && {25/59} && {26/61} && { 3/ 7} && {28/65} && {29/67} && {10/23} && {31/71} && {32/73} && {11/25} && {34/77} &\\\hline
$5$ & { 1/ 3} & { 1/ 3} & { 7/23} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  4/13} & { 5/16} & { 9/28} & {\color{red}  9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 6/19} & { 1/ 3} & { 2/ 7} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {13/41} & {15/47} & {14/43} & {\color{red}  7/22} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {17/53} & { 1/ 3} & { 3/10} & { 1/ 3} & {17/52} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 9/28} & {10/31} & {19/58} & {\color{red} 19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {11/34} & { 1/ 3} & { 4/13} & { 1/ 3} & {22/67} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {23/71} & {25/77} & {24/73} & {12/37} & { 1/ 3} \\\hline
$6$ & { 3/ 8} && { 8/25} && { 8/27} && { 8/23} && { 3/ 8} && { 1/ 3} && {12/35} && {\color{red} 11/31} && { 3/ 8} && {15/41} && {16/43} && {17/45} && {18/47} && {19/49} && {20/51} && {21/53} && { 2/ 5} && {23/57} && {24/59} && {25/61} && {26/63} && {27/65} && {28/67} && {29/69} && {30/71} && {31/73} && {32/75} && { 3/ 7} && {34/79} && {35/81} &\\\hline
$7$ & { 3/ 8} & { 6/17} & { 1/ 3} & { 6/17} & { 7/22} & { 6/17} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 9/25} & { 9/26} & { 1/ 3} & { 1/ 3} & {11/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 4/11} & { 6/17} & {12/35} & { 6/17} & {14/39} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {15/41} & { 5/14} & {15/43} & { 8/23} & {17/47} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {18/49} & { 9/25} & { 6/17} & {19/54} & { 4/11} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 7/19} & {21/58} & {21/59} & {11/31} & {23/63} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {24/65} & { 4/11} & {24/67} & { 5/14} & {26/71} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {27/73} & {27/74} & { 9/25} \\\hline
$8$ & { 6/17} && { 6/19} && {10/31} && { 3/ 8} && { 9/25} && { 1/ 3} && { 1/ 3} && { 3/ 8} && { 4/11} && {16/45} && {17/47} && { 3/ 8} && {19/51} && {20/53} && {21/55} && {22/57} && {23/59} && {24/61} && {25/63} && { 2/ 5} && {27/67} && {28/69} && {29/71} && {30/73} && {31/75} && {32/77} && {33/79} && {34/81} && {35/83} && {36/85} &\\\hline
$9$ & { 1/ 3} & { 7/19} & { 3/10} & { 7/19} & {10/33} & { 7/19} & { 6/17} & { 7/19} & { 9/26} & { 7/19} & { 1/ 3} & { 7/20} & {11/32} & { 1/ 3} & { 6/17} & { 6/17} & {13/36} & {12/35} & { 7/19} & {\color{red} 12/37} & { 7/19} & {\color{red}  8/25} & { 7/19} & { 6/17} & { 7/19} & {15/43} & { 7/19} & {16/47} & { 7/19} & {17/49} & {21/59} & { 6/17} & { 6/17} & {19/53} & { 9/26} & { 4/11} & {\color{red}  1/ 3} & { 7/19} & {\color{red} 22/67} & { 7/19} & { 6/17} & { 7/19} & { 7/20} & { 7/19} & {11/32} & { 7/19} & {23/66} & { 7/19} & { 6/17} & {14/39} & { 5/14} & { 7/20} & {13/36} & {\color{red} 14/41} & {27/74} & {\color{red} 31/92} & { 7/19} & { 6/17} & { 7/19} & {27/77} \\\hline
$10$ & {\color{red} 10/31} && { 2/ 7} && { 2/ 7} && { 1/ 3} && { 1/ 3} && {14/41} && {\color{red} 14/43} && { 1/ 3} && {\color{red} 16/47} && {\color{red} 17/49} && { 6/17} && {19/53} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} &\\\hline
$11$ & {\color{red}  5/16} & { 8/21} & {\color{red}  7/24} & { 8/21} & { 4/13} & { 8/21} & { 9/28} & { 8/21} & { 1/ 3} & { 8/21} & {11/32} & { 4/11} & { 6/17} & { 8/23} & {13/36} & { 1/ 3} & { 7/19} & {\color{red} 10/31} & { 3/ 8} & {\color{red} 17/52} & { 8/21} & {\color{red} 14/43} & { 8/21} & {\color{red}  1/ 3} & { 8/21} & {16/47} & { 8/21} & {17/49} & { 8/21} & { 6/17} & { 8/21} & {19/53} & {24/65} & { 4/11} & {24/67} & { 7/19} & { 8/23} & {22/59} & {\color{red} 24/71} & {23/61} & {\color{red} 21/62} & { 8/21} & {\color{red} 11/32} & { 8/21} & {\color{red} 23/66} & { 8/21} & { 6/17} & { 8/21} & { 5/14} & { 8/21} & {13/36} & { 8/21} & {27/74} & {16/43} & { 7/19} & { 4/11} & {29/78} & {16/45} & { 3/ 8} & {\color{red}  8/23} \\\hline
$12$ & {\color{red}  7/22} && {11/37} && {\color{red} 11/39} && {\color{red}  5/16} && {\color{red}  7/22} && {\color{red} 14/45} && {16/47} && {\color{red} 16/49} && { 1/ 3} && {\color{red} 18/53} && {\color{red} 19/55} && {20/57} && {21/59} && {22/61} && {23/63} && {24/65} && {25/67} && {26/69} && {27/71} && {28/73} && {29/75} && {30/77} && {31/79} && {32/81} && {33/83} && { 2/ 5} && {35/87} && {36/89} && {37/91} && {38/93} &\\\hline
$13$ & { 8/23} & { 9/23} & { 4/13} & { 9/23} & { 9/28} & { 9/23} & { 1/ 3} & { 9/23} & { 8/23} & { 9/23} & { 6/17} & { 3/ 8} & {13/36} & { 9/25} & { 7/19} & {\color{red}  8/23} & { 3/ 8} & { 1/ 3} & { 8/21} & {\color{red} 14/43} & {17/44} & {\color{red}  1/ 3} & { 9/23} & { 8/23} & { 9/23} & {17/49} & { 9/23} & { 6/17} & { 9/23} & {19/53} & { 9/23} & { 4/11} & { 9/23} & { 7/19} & {27/71} & {22/59} & {27/73} & {23/61} & { 9/25} & { 8/21} & {27/77} & { 5/13} & {\color{red} 23/66} & {26/67} & {\color{red}  6/17} & { 9/23} & {\color{red}  5/14} & { 9/23} & {13/36} & { 9/23} & {27/74} & { 9/23} & { 7/19} & { 9/23} & {29/78} & { 9/23} & { 3/ 8} & {18/47} & {31/82} & { 3/ 8} \\\hline
$14$ & { 3/ 8} && {13/41} && { 9/29} && {11/31} && { 3/ 8} && {16/49} && {\color{red} 12/37} && {14/39} && { 3/ 8} && { 1/ 3} && {\color{red} 20/59} && {17/47} && { 3/ 8} && {23/65} && {24/67} && {\color{red}  4/11} && { 3/ 8} && {27/73} && {28/75} && {29/77} && {30/79} && {31/81} && {32/83} && {33/85} && {34/87} && {35/89} && {36/91} && {37/93} && { 2/ 5} && {39/97} &\\\hline
$15$ & { 3/ 8} & { 2/ 5} & {14/43} & { 2/ 5} & { 1/ 3} & { 2/ 5} & { 3/ 8} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {13/36} & { 5/13} & { 7/19} & {10/27} & { 3/ 8} & { 3/ 8} & { 8/21} & {15/41} & {17/44} & { 1/ 3} & { 9/23} & {17/47} & {19/48} & { 3/ 8} & { 2/ 5} & {18/49} & { 2/ 5} & {19/53} & { 2/ 5} & { 4/11} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {22/59} & { 2/ 5} & {23/61} & {30/77} & { 8/21} & {30/79} & { 5/13} & { 3/ 8} & {26/67} & {\color{red}  4/11} & { 9/23} & {\color{red}  5/14} & {28/71} & { 3/ 8} & {29/73} & { 3/ 8} & { 2/ 5} & { 7/19} & { 2/ 5} & {29/78} & { 2/ 5} & { 3/ 8} & { 2/ 5} & {\color{red} 31/82} & { 2/ 5} & { 8/21} & { 2/ 5} \\\hline
$16$ & { 9/25} && { 1/ 3} && {15/47} && { 3/ 8} && { 4/11} && {12/35} && {18/55} && { 3/ 8} && {15/41} && {15/43} && { 1/ 3} && { 3/ 8} && {18/49} && { 6/17} && {25/71} && { 3/ 8} && {\color{red}  7/19} && {\color{red}  4/11} && {29/79} && { 3/ 8} && {\color{red} 31/83} && {32/85} && {11/29} && {34/89} && { 5/13} && {12/31} && {37/95} && {38/97} && {\color{red} 38/97} && {21/53} &\\\hline
$17$ & { 9/26} & {11/27} & { 9/28} & {11/27} & {16/49} & {11/27} & { 9/25} & {11/27} & {13/36} & {11/27} & { 7/19} & {11/28} & { 3/ 8} & {11/29} & { 8/21} & {11/30} & {17/44} & {\color{red} 11/31} & { 9/23} & {\color{red} 11/32} & {19/48} & { 1/ 3} & { 2/ 5} & { 9/25} & {21/52} & {19/53} & {11/27} & { 4/11} & {11/27} & { 7/19} & {11/27} & {22/59} & {11/27} & {23/61} & {11/27} & { 8/21} & {11/27} & { 5/13} & {33/83} & {26/67} & {33/85} & { 9/23} & {11/29} & {28/71} & {33/89} & {29/73} & {\color{red} 27/74} & { 2/ 5} & {\color{red}  7/19} & {31/77} & {29/78} & {32/79} & { 3/ 8} & {11/27} & {31/82} & {11/27} & { 8/21} & {11/27} & {33/86} & {11/27} \\\hline
$18$ & {\color{red} 16/47} && { 9/29} && {\color{red}  5/17} && { 9/26} && {12/35} && {\color{red} 12/37} && {\color{red} 13/41} && { 9/26} && { 9/26} && {23/65} && {\color{red} 23/67} && { 1/ 3} && {\color{red}  9/26} && {\color{red} 26/73} && {\color{red} 26/75} && {27/77} && {28/79} && {\color{red} 29/81} && {\color{red} 30/83} && {31/85} && {32/87} && {33/89} && {34/91} && {35/93} && {\color{red} 35/93} && {\color{red} 36/95} && {\color{red} 37/97} && {\color{red} 38/99} && {\color{red} 38/99} && {\color{red} 35/93} &\\\hline
$19$ & {\color{red}  1/ 3} & {12/29} & { 3/10} & {12/29} & {17/53} & {12/29} & {19/55} & {12/29} & { 7/19} & {12/29} & { 3/ 8} & { 2/ 5} & { 8/21} & {12/31} & {17/44} & { 3/ 8} & { 9/23} & { 4/11} & {19/48} & {\color{red}  6/17} & { 2/ 5} & {\color{red} 12/35} & {21/52} & { 1/ 3} & {11/27} & {13/37} & {23/56} & { 7/19} & {12/29} & {22/59} & {12/29} & {23/61} & {12/29} & { 8/21} & {12/29} & { 5/13} & {12/29} & {26/67} & {12/29} & { 9/23} & {36/89} & {28/71} & {36/91} & {29/73} & {12/31} & { 2/ 5} & {36/95} & {31/77} & {\color{red} 29/78} & {32/79} & {\color{red}  3/ 8} & {11/27} & {\color{red} 31/82} & {34/83} & { 8/21} & { 7/17} & {33/86} & {12/29} & {17/44} & {12/29} \\\hline
$20$ & {\color{red}  1/ 3} && {\color{red} 16/53} && { 2/ 7} && {\color{red} 21/64} && {\color{red}  1/ 3} && {\color{red} 20/61} && {\color{red} 14/43} && { 1/ 3} && {\color{red}  1/ 3} && {\color{red}  1/ 3} && {25/71} && {\color{red} 25/73} && { 1/ 3} && {\color{red} 26/77} && {\color{red} 28/79} && {\color{red} 28/81} && {\color{red} 29/83} && {\color{red} 29/83} && {\color{red} 31/87} && {\color{red} 32/89} && {\color{red} 33/91} && {\color{red} 33/91} && {\color{red} 34/93} && {\color{red}  7/19} && {\color{red}  7/19} && {\color{red} 28/79} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$21$ & {11/31} & {13/31} & {17/55} & {13/31} & { 6/19} & {13/31} & {\color{red} 13/38} & {13/31} & {22/61} & {13/31} & { 8/21} & {13/32} & {17/44} & {13/33} & { 9/23} & {13/34} & {19/48} & {13/35} & { 2/ 5} & {13/36} & {21/52} & {\color{red} 13/37} & {11/27} & {11/31} & {23/56} & { 1/ 3} & {12/29} & { 7/20} & { 5/12} & {15/41} & {13/31} & { 8/21} & {13/31} & { 5/13} & {13/31} & {26/67} & {13/31} & { 9/23} & {13/31} & {28/71} & {13/31} & {29/73} & {39/95} & { 2/ 5} & {39/97} & {31/77} & {13/33} & {32/79} & {22/57} & {11/27} & {25/66} & {34/83} & { 8/21} & { 7/17} & {\color{red} 33/86} & {12/29} & {17/44} & {37/89} & { 7/18} & {38/91} \\\hline
$22$ & { 3/ 8} && { 6/19} && {12/37} && {14/39} && { 3/ 8} && {\color{red} 22/65} && {\color{red}  1/ 3} && {17/47} && { 3/ 8} && {\color{red} 11/32} && {\color{red} 11/32} && { 4/11} && { 3/ 8} && { 1/ 3} && {\color{red} 21/61} && {\color{red} 23/63} && { 3/ 8} && {\color{red} 31/89} && {\color{red} 32/91} && {\color{red} 26/71} && { 3/ 8} && {\color{red} 34/95} && {\color{red} 11/31} && {\color{red} 29/79} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$23$ & { 3/ 8} & {14/33} & {19/59} & {14/33} & {20/61} & {14/33} & { 3/ 8} & {14/33} & { 3/ 8} & {14/33} & {25/67} & { 7/17} & { 9/23} & { 2/ 5} & {19/48} & { 7/18} & { 2/ 5} & {14/37} & {21/52} & { 7/19} & {11/27} & {\color{red}  4/11} & {23/56} & { 3/ 8} & {12/29} & { 7/19} & { 5/12} & { 1/ 3} & {13/31} & {23/63} & {27/64} & { 3/ 8} & {14/33} & {17/45} & {14/33} & { 9/23} & {14/33} & {28/71} & {14/33} & {29/73} & {14/33} & { 2/ 5} & {14/33} & {31/77} & {37/89} & {32/79} & {31/76} & {11/27} & { 2/ 5} & {34/83} & {31/79} & { 7/17} & {37/96} & {12/29} & {14/37} & {37/89} & {35/92} & {38/91} & { 9/23} & {13/31} \\\hline
$24$ & { 4/11} && {20/61} && {20/63} && { 3/ 8} && {15/41} && {15/43} && {\color{red} 16/47} && { 3/ 8} && {18/49} && {\color{red}  6/17} && {\color{red}  6/17} && { 3/ 8} && { 7/19} && {\color{red} 21/59} && { 1/ 3} && { 3/ 8} && {\color{red} 24/65} && {\color{red} 24/67} && {\color{red}  8/23} && { 3/ 8} && {\color{red} 27/73} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$25$ & { 6/17} & { 3/ 7} & { 1/ 3} & { 3/ 7} & { 4/13} & { 3/ 7} & { 4/11} & { 3/ 7} & { 5/14} & { 3/ 7} & {26/71} & { 5/12} & {28/73} & {15/37} & { 2/ 5} & {15/38} & {21/52} & { 5/13} & {11/27} & { 3/ 8} & {23/56} & {15/41} & {12/29} & { 4/11} & { 5/12} & {\color{red} 31/86} & {13/31} & {\color{red} 21/61} & {27/64} & { 1/ 3} & {14/33} & { 4/11} & {29/68} & {\color{red} 17/47} & { 3/ 7} & { 3/ 8} & { 3/ 7} & {19/49} & { 3/ 7} & { 2/ 5} & { 3/ 7} & {31/77} & { 3/ 7} & {32/79} & { 3/ 7} & {11/27} & {37/88} & {34/83} & {26/63} & { 7/17} & {\color{red} 15/41} & {12/29} & {39/98} & {37/89} & {\color{red} 15/43} & {38/91} & {\color{red}  4/11} & {13/31} & {\color{red} 17/47} & { 8/19} \\\hline
$26$ & {\color{red} 22/63} && {12/37} && {13/41} && { 6/17} && {15/43} && {16/47} && {\color{red} 17/49} && { 6/17} && {19/53} && {13/36} && {13/36} && {13/36} && {13/36} && {\color{red} 13/36} && {\color{red} 32/91} && {\color{red} 25/76} && {\color{red}  6/17} && {\color{red} 35/97} && {\color{red} 31/91} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$27$ & {\color{red} 11/32} & {16/37} & { 6/19} & {16/37} & {\color{red}  7/23} & {16/37} & {12/35} & {16/37} & {\color{red} 25/73} & {16/37} & { 9/25} & { 8/19} & {29/77} & {16/39} & {31/79} & { 2/ 5} & {11/27} & {16/41} & {23/56} & { 8/21} & {12/29} & {16/43} & { 5/12} & { 4/11} & {13/31} & {\color{red} 16/45} & {27/64} & {\color{red} 33/92} & {14/33} & {\color{red} 16/47} & {29/68} & {\color{red} 12/37} & { 3/ 7} & {\color{red} 17/49} & {31/72} & {\color{red}  9/25} & {16/37} & {19/51} & {16/37} & {\color{red} 29/77} & {16/37} & {21/53} & {16/37} & {11/27} & {16/37} & {34/83} & {\color{red}  2/ 5} & { 7/17} & {\color{red} 16/41} & {12/29} & {38/91} & {37/89} & {\color{red} 16/43} & {38/91} & {\color{red}  4/11} & {13/31} & {\color{red} 33/92} & { 8/19} & {\color{red}  8/23} & {41/97} \\\hline
$28$ & {\color{red} 23/67} && {\color{red}  4/13} && {14/43} && {\color{red} 27/80} && {\color{red} 13/38} && {\color{red} 17/49} && { 6/17} && {19/53} && { 4/11} && { 7/19} && { 7/19} && { 7/19} && { 7/19} && { 7/19} && { 7/19} && {\color{red} 34/97} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 29/85} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$29$ & {14/39} & {17/39} & {\color{red} 22/71} & {17/39} & {\color{red}  7/22} & {17/39} & { 8/23} & {17/39} & {14/39} & {17/39} & {28/79} & {17/40} & {10/27} & {17/41} & {32/83} & {17/42} & { 2/ 5} & {17/43} & {12/29} & {17/44} & { 5/12} & {17/45} & {13/31} & {17/46} & {27/64} & {17/47} & {14/33} & {\color{red} 17/48} & {29/68} & {\color{red}  5/14} & { 3/ 7} & {\color{red} 14/39} & {31/72} & {\color{red}  1/99} & {16/37} & {\color{red} 26/77} & {33/76} & {\color{red} 28/79} & {17/39} & {10/27} & {17/39} & {\color{red} 31/83} & {17/39} & {11/28} & {17/39} & {23/57} & {17/39} & {12/29} & {\color{red} 17/42} & {37/89} & {\color{red} 17/43} & {38/91} & {\color{red} 17/44} & {13/31} & {17/41} & { 8/19} & {\color{red} 17/46} & {41/97} & {\color{red} 17/47} & {14/33} \\\hline
$30$ & { 3/ 8} && {23/73} && { 1/ 3} && {17/47} && { 3/ 8} && { 6/17} && {19/53} && { 4/11} && { 3/ 8} && {22/59} && { 3/ 8} && { 3/ 8} && { 3/ 8} && { 3/ 8} && { 3/ 8} && {\color{red} 26/71} && { 3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$31$ & { 3/ 8} & {18/41} & { 8/25} & {18/41} & {25/77} & {18/41} & { 3/ 8} & {18/41} & { 3/ 8} & {18/41} & {\color{red} 29/83} & { 3/ 7} & {31/85} & {18/43} & {11/29} & { 9/22} & {35/89} & { 2/ 5} & {37/91} & { 9/23} & {13/31} & {18/47} & {27/64} & { 3/ 8} & {14/33} & {24/65} & {29/68} & {\color{red} 17/49} & { 3/ 7} & {26/71} & {31/72} & { 3/ 8} & {16/37} & {27/73} & {33/76} & {\color{red}  1/99} & {17/39} & {\color{red} 29/79} & { 7/16} & { 3/ 8} & {18/41} & {\color{red} 10/27} & {18/41} & {11/29} & {18/41} & {\color{red} 34/89} & {\color{red}  3/ 7} & { 2/ 5} & {\color{red} 18/43} & {25/61} & {\color{red}  9/22} & {13/31} & {\color{red}  2/ 5} & { 8/19} & {\color{red}  9/23} & {41/97} & {\color{red} 18/47} & {14/33} & {\color{red}  3/ 8} & {23/54} \\\hline
$32$ & {15/41} && {25/77} && {26/79} && { 3/ 8} && {18/49} && {19/53} && { 4/11} && { 3/ 8} && {22/59} && {23/61} && { 8/21} && { 8/21} && { 8/21} && { 8/21} && { 8/21} && { 8/21} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$33$ & { 5/14} & {19/43} & {26/79} & {19/43} & {\color{red} 25/81} & {19/43} & {15/41} & {19/43} & { 9/25} & {19/43} & {\color{red}  9/26} & {19/44} & {32/89} & {19/45} & {34/91} & {19/46} & {12/31} & {19/47} & { 2/ 5} & {19/48} & {40/97} & {19/49} & {14/33} & {19/50} & {29/68} & {\color{red} 19/51} & { 3/ 7} & {\color{red}  6/17} & {31/72} & {\color{red}  1/ 3} & {16/37} & {\color{red} 15/41} & {33/76} & {\color{red}  9/25} & {17/39} & {\color{red}  1/99} & { 7/16} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {19/43} & {12/31} & {\color{red} 41/93} & {\color{red} 37/95} & {\color{red} 19/45} & {\color{red}  2/ 5} & {\color{red} 19/46} & {\color{red} 40/97} & {\color{red} 19/47} & {14/33} & {\color{red} 19/48} & {23/54} & {\color{red} 19/49} & {41/96} \\\hline
$34$ & {\color{red} 28/79} && { 1/ 3} && {27/83} && { 5/14} && {19/53} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {17/44} && {17/44} && {17/44} && {17/44} && {17/44} && {\color{red} 11/30} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$35$ & {\color{red}  7/20} & { 4/ 9} & {15/46} & { 4/ 9} & {\color{red}  3/10} & { 4/ 9} & {15/43} & { 4/ 9} & {\color{red} 31/89} & { 4/ 9} & {\color{red} 31/91} & {10/23} & {\color{red} 11/31} & {20/47} & { 7/19} & { 5/12} & {37/97} & {20/49} & {13/33} & {\color{red} 17/47} & {28/69} & {20/51} & {38/91} & {\color{red} 19/51} & { 3/ 7} & {\color{red} 19/52} & {31/72} & {\color{red}  9/26} & {16/37} & {\color{red}  1/ 3} & {33/76} & {\color{red}  1/99} & {17/39} & {\color{red}  1/99} & { 7/16} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {\color{red} 10/23} & {13/33} & {\color{red} 20/47} & {\color{red} 21/53} & {\color{red}  5/12} & {\color{red} 28/69} & {\color{red} 20/49} & {\color{red} 38/91} & {\color{red}  2/ 5} & { 3/ 7} \\\hline
$36$ & {\color{red} 29/83} && {15/47} && {28/87} && {\color{red} 31/89} && { 4/11} && { 7/19} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && { 9/23} && { 9/23} && { 9/23} && { 9/23} && { 9/23} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$37$ & {17/47} & {21/47} & {\color{red}  5/16} & {21/47} & {17/52} & {21/47} & {19/54} & {21/47} & {17/47} & {21/47} & {\color{red} 32/95} & { 7/16} & {\color{red} 34/97} & { 3/ 7} & { 4/11} & {21/50} & {35/93} & { 7/17} & {33/85} & {\color{red} 18/49} & { 2/ 5} & {21/53} & {37/90} & {\color{red} 19/52} & {\color{red}  5/12} & {\color{red} 10/27} & {16/37} & {\color{red} 16/47} & {33/76} & {\color{red} 27/77} & {17/39} & {\color{red}  1/99} & { 7/16} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red}  1/99} & {\color{red} 21/50} & {\color{red} 39/97} & {\color{red}  7/17} & {\color{red} 37/90} \\\hline
$38$ & { 3/ 8} && {\color{red} 28/89} && {30/91} && { 4/11} && { 3/ 8} && {22/59} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {19/48} && {19/48} && {19/48} && {19/48} && {19/48} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$39$ & { 3/ 8} & {22/49} & {29/91} & {22/49} & {\color{red} 10/31} & {22/49} & { 3/ 8} & {22/49} & { 3/ 8} & {22/49} & {\color{red} 34/99} & {11/25} & {\color{red} 15/44} & {22/51} & { 3/ 8} & {11/26} & { 3/ 8} & {22/53} & {23/60} & {11/27} & {28/71} & {\color{red} 26/71} & {15/37} & {\color{red}  3/ 8} & {37/89} & {\color{red} 27/73} & {\color{red}  8/19} & {\color{red} 26/75} & {17/39} & {\color{red}  1/99} & { 7/16} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red}  1/99} & {\color{red} 22/51} & {\color{red}  1/99} & {\color{red} 11/26} & {\color{red}  1/99} \\\hline
$40$ & {18/49} && {\color{red}  6/19} && { 6/19} && { 3/ 8} && {\color{red}  7/19} && {23/61} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && { 2/ 5} && {\color{red} 30/83} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$41$ & { 9/25} & {23/51} & {\color{red} 22/69} & {23/51} & { 9/28} & {\color{red}  9/20} & {18/49} & {23/51} & {21/58} & {23/51} & {\color{red}  7/20} & {\color{red} 20/49} & {\color{red}  1/99} & {23/53} & {\color{red} 18/49} & {\color{red} 20/51} & {\color{red}  4/11} & {23/55} & {14/37} & {\color{red} 20/53} & {37/95} & {\color{red} 21/55} & {\color{red} 15/38} & {\color{red} 18/49} & {16/39} & {\color{red}  9/25} & {\color{red} 33/80} & {\color{red} 27/77} & {\color{red} 17/40} & {\color{red}  1/99} & {18/41} & {\color{red}  1/99} & {37/84} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {\color{red} 23/52} & {\color{red}  1/99} & {\color{red} 23/53} & {\color{red}  1/99} \\\hline
$42$ & {\color{red} 34/95} && {\color{red} 17/53} && {\color{red}  1/99} && { 9/25} && {\color{red} 23/64} && { 8/21} && { 5/13} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {\color{red} 31/77} && {21/52} && {21/52} && {21/52} && {21/52} && {\color{red} 10/29} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$43$ & {\color{red} 17/48} & {24/53} & { 1/ 3} & {24/53} & {19/58} & {\color{red} 33/73} & { 6/17} & {24/53} & {\color{red} 31/88} & {24/53} & {\color{red} 11/32} & {\color{red}  7/17} & {\color{red}  1/99} & {\color{red} 21/52} & {\color{red}  1/99} & {\color{red} 21/53} & {\color{red}  5/14} & {\color{red}  7/18} & {\color{red}  7/19} & {\color{red}  8/23} & { 5/13} & {\color{red} 25/73} & {\color{red} 31/80} & {\color{red}  6/17} & {\color{red}  2/ 5} & {\color{red} 27/77} & {17/41} & {\color{red} 28/81} & {\color{red}  5/12} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red}  1/99} & {19/43} & {\color{red}  1/99} & {39/88} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} \\\hline
$44$ & {\color{red} 35/99} && {18/55} && {\color{red}  1/99} && {\color{red}  9/26} && {\color{red} 27/76} && {35/93} && {26/67} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {11/27} && {11/27} && {\color{red} 28/69} && {11/27} && {\color{red} 31/89} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$45$ & { 4/11} & { 5/11} & {\color{red}  1/99} & { 5/11} & { 1/ 3} & {\color{red} 23/51} & {11/31} & { 5/11} & { 4/11} & {\color{red} 11/26} & {\color{red} 23/66} & {\color{red} 21/52} & {\color{red}  1/99} & {\color{red} 11/27} & {\color{red}  1/99} & {\color{red} 23/56} & {\color{red} 33/91} & {\color{red} 11/28} & {\color{red}  1/99} & {\color{red} 26/73} & {\color{red}  3/ 8} & {\color{red} 27/77} & {16/41} & {\color{red}  4/11} & {\color{red} 11/28} & {\color{red} 28/81} & {\color{red} 17/42} & {\color{red}  1/99} & {18/43} & {\color{red}  1/99} & {\color{red} 37/88} & {\color{red}  1/99} & {\color{red} 19/44} & {\color{red}  1/99} & { 4/ 9} & {\color{red}  1/99} & {41/92} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} \\\hline
$46$ & { 3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {23/63} && { 3/ 8} && {\color{red} 11/30} && { 9/23} && {28/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && {\color{red} 34/83} && {\color{red} 34/83} && {\color{red} 11/27} && {\color{red} 11/29} && {\color{red} 32/89} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$47$ & { 3/ 8} & {26/57} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {\color{red} 24/53} & { 3/ 8} & {26/57} & { 3/ 8} & {\color{red} 23/54} & {\color{red}  1/99} & {\color{red} 11/27} & {\color{red}  1/99} & {\color{red} 26/67} & {\color{red}  6/17} & {\color{red} 26/69} & {\color{red}  1/99} & {\color{red} 27/73} & {\color{red}  1/99} & {\color{red} 26/73} & {\color{red}  1/99} & {\color{red} 29/79} & {\color{red}  1/99} & {\color{red}  3/ 8} & {17/43} & {\color{red} 10/27} & {\color{red} 35/88} & {\color{red}  6/17} & {\color{red}  9/22} & {\color{red}  1/99} & {19/45} & {\color{red}  1/99} & {\color{red} 39/92} & {\color{red}  1/99} & {\color{red} 10/23} & {\color{red}  1/99} & {21/47} & {\color{red}  1/99} & {43/96} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} \\\hline
$48$ & { 7/19} && {\color{red}  1/99} && {\color{red}  1/99} && { 3/ 8} && {24/65} && {\color{red} 17/47} && {\color{red} 27/71} && {29/73} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {12/29} && {12/29} && {\color{red}  2/ 5} && {\color{red} 34/91} && {\color{red}  3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$49$ & {21/58} & {27/59} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red} 18/49} & {27/59} & { 4/11} & {\color{red} 27/65} & {\color{red}  1/99} & {\color{red} 27/67} & {\color{red}  1/99} & {\color{red}  9/23} & {\color{red}  1/99} & {\color{red} 24/59} & {\color{red}  1/99} & {\color{red} 27/73} & {\color{red}  1/99} & {\color{red}  9/25} & {\color{red}  1/99} & {\color{red} 28/79} & {\color{red}  1/99} & {\color{red} 18/49} & {\color{red}  1/99} & {\color{red} 30/83} & { 2/ 5} & {\color{red}  1/99} & {\color{red} 37/92} & {\color{red}  1/99} & {\color{red} 19/46} & {\color{red}  1/99} & {20/47} & {\color{red}  1/99} & {\color{red} 41/96} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {22/49} & {\color{red}  1/99} & { 9/20} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} \\\hline
$50$ & {\color{red} 21/59} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 30/83} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 37/98} && { 2/ 5} && {31/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {\color{red} 37/89} && {\color{red} 37/89} && {\color{red} 37/91} && {\color{red} 12/31} && {\color{red}  7/19} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$51$ & {\color{red}  7/20} & {28/61} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {\color{red} 25/56} & {\color{red}  1/99} & {\color{red} 13/29} & {\color{red}  1/99} & {\color{red} 28/67} & {\color{red}  1/99} & {\color{red} 28/69} & {\color{red}  1/99} & {\color{red} 28/71} & {\color{red}  1/99} & {\color{red} 28/73} & {\color{red}  1/99} & {\color{red} 28/75} & {\color{red}  1/99} & {\color{red}  4/11} & {\color{red}  1/99} & {\color{red} 28/79} & {\color{red}  1/99} & {\color{red} 11/31} & {\color{red}  1/99} & {\color{red} 31/87} & {\color{red}  1/99} & {\color{red}  1/99} & {19/47} & {\color{red}  1/99} & {\color{red} 13/32} & {\color{red}  1/99} & {\color{red}  5/12} & {\color{red}  1/99} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 40/93} & {\color{red}  1/99} & {\color{red} 11/25} & {\color{red}  1/99} & {23/51} & {\color{red}  1/99} & {33/73} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} \\\hline
$52$ & {\color{red} 11/31} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 19/51} && {\color{red} 30/77} && {32/79} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && {13/31} && {13/31} && {\color{red}  2/ 5} && {\color{red} 37/97} && {\color{red}  4/11} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$53$ & {23/63} & {29/63} & {\color{red}  1/99} & {29/63} & {\color{red}  1/99} & {\color{red} 29/65} & {\color{red} 19/66} & {\color{red}  9/20} & {\color{red}  5/14} & {\color{red} 29/69} & {\color{red}  1/99} & {\color{red} 29/71} & {\color{red}  1/99} & {\color{red} 29/73} & {\color{red}  1/99} & {\color{red} 29/75} & {\color{red}  1/99} & {\color{red} 29/77} & {\color{red}  1/99} & {\color{red} 29/79} & {\color{red}  1/99} & {\color{red} 29/81} & {\color{red}  1/99} & {\color{red} 17/47} & {\color{red}  1/99} & {\color{red} 32/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {20/49} & {\color{red}  1/99} & {\color{red} 25/61} & {\color{red}  1/99} & {\color{red} 21/50} & {\color{red}  1/99} & {22/51} & {\color{red}  1/99} & {\color{red} 29/67} & {\color{red}  1/99} & {\color{red} 23/52} & {\color{red}  1/99} & {24/53} & {\color{red}  1/99} & {44/97} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} \\\hline
$54$ & { 3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {26/71} && { 3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 29/75} && {11/27} && {34/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {\color{red}  8/19} && {\color{red}  8/19} && {\color{red} 40/97} && {\color{red} 13/33} && {\color{red} 35/93} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$55$ & { 3/ 8} & { 6/13} & {\color{red}  1/99} & { 6/13} & {\color{red}  1/99} & {\color{red} 30/67} & { 3/ 8} & {\color{red} 10/23} & { 3/ 8} & {\color{red} 30/71} & {\color{red}  1/99} & {\color{red} 30/73} & {\color{red}  1/99} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red} 30/77} & {\color{red}  1/99} & {\color{red} 30/79} & {\color{red}  1/99} & {\color{red} 10/27} & {\color{red}  1/99} & {\color{red} 32/87} & {\color{red}  1/99} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red} 33/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/75} & {\color{red}  1/99} & {\color{red} 11/26} & {\color{red}  1/99} & {23/53} & {\color{red}  1/99} & {\color{red} 37/85} & {\color{red}  1/99} & {\color{red}  4/ 9} & {\color{red}  1/99} & { 5/11} & {\color{red}  1/99} & {41/90} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {40/87} & {\color{red}  1/99} \\\hline
$56$ & {24/65} && {\color{red}  1/99} && {\color{red}  1/99} && { 3/ 8} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 33/83} && { 7/17} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {14/33} && {14/33} && {\color{red} 28/69} && {\color{red} 33/85} && {\color{red} 13/35} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$57$ & { 4/11} & {31/67} & {\color{red}  1/99} & {31/67} & {\color{red}  1/99} & {\color{red} 31/69} & {\color{red}  1/99} & {\color{red} 31/71} & {\color{red}  1/99} & {\color{red} 31/73} & {\color{red}  1/99} & {\color{red} 31/75} & {\color{red}  1/99} & {\color{red} 31/77} & {\color{red}  1/99} & {\color{red} 31/79} & {\color{red}  1/99} & {\color{red} 31/81} & {\color{red}  1/99} & {\color{red} 31/83} & {\color{red}  1/99} & {\color{red} 31/85} & {\color{red}  1/99} & {\color{red} 18/49} & {\color{red}  1/99} & {\color{red} 33/91} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  5/12} & {\color{red}  1/99} & {\color{red} 23/54} & {\color{red}  1/99} & {24/55} & {\color{red}  1/99} & {\color{red}  7/16} & {\color{red}  1/99} & {\color{red} 25/56} & {\color{red}  1/99} & {26/57} & {\color{red}  1/99} & {37/81} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {40/87} & {\color{red}  1/99} & {29/63} & {\color{red}  1/99} \\\hline
$58$ & {\color{red} 24/67} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 15/38} && {12/29} && {37/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {23/54} && {\color{red} 23/54} && {\color{red} 23/54} && {\color{red} 38/91} && {\color{red}  2/ 5} && {\color{red} 23/60} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
$59$ & {\color{red}  6/17} & {32/69} & {\color{red}  1/99} & {32/69} & {\color{red}  1/99} & {\color{red} 32/71} & {\color{red}  1/99} & {\color{red} 32/73} & {\color{red}  1/99} & {\color{red} 32/75} & {\color{red}  1/99} & {\color{red} 32/77} & {\color{red}  1/99} & {\color{red} 32/79} & {\color{red}  1/99} & {\color{red} 32/81} & {\color{red}  1/99} & {\color{red} 32/83} & {\color{red}  1/99} & {\color{red} 32/85} & {\color{red}  1/99} & {\color{red} 32/87} & {\color{red}  1/99} & {\color{red} 32/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  3/ 7} & {\color{red}  1/99} & {25/57} & {\color{red}  1/99} & {\color{red} 40/91} & {\color{red}  1/99} & {\color{red} 13/29} & {\color{red}  1/99} & {27/59} & {\color{red}  1/99} & {11/24} & {\color{red}  1/99} & {28/61} & {\color{red}  1/99} & {40/87} & {\color{red}  1/99} & {29/63} & {\color{red}  1/99} & {41/89} & {\color{red}  1/99} \\\hline
$60$ & {\color{red}  5/14} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red} 36/89} && {38/91} && {13/31} && { 8/19} && {41/97} && {14/33} && {23/54} && {41/96} && { 3/ 7} && { 3/ 7} && { 3/ 7} && {\color{red} 37/90} && {\color{red} 28/71} && {\color{red} 14/37} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} && {\color{red}  1/99} &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 3, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g4-a04b05.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$& $51$& $52$& $53$& $54$& $55$& $56$& $57$& $58$& $59$& $60$\\\hline
$1$ & { 4/11} & { 1/ 3} & { 4/13} & { 2/ 7} & {\color{red}  5/17} & { 1/ 3} & { 7/19} & { 2/ 5} & { 2/ 5} & { 2/ 5} & { 8/21} & { 4/11} & { 8/23} & { 1/ 3} & {\color{red}  1/ 3} & { 5/14} & {11/29} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & { 4/11} & { 6/17} & {\color{red} 13/37} & { 7/19} & { 5/13} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {16/43} & { 4/11} & {\color{red} 17/47} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & {10/27} & {\color{red}  7/19} & {11/29} & {23/59} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 3/ 8} & {\color{red} 25/67} & {13/34} & { 9/23} & { 2/ 5} & { 2/ 5} & { 2/ 5} \\\hline
$2$ & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red}  5/19} & { 1/ 3} & { 1/ 3} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & { 8/23} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {\color{red} 10/31} & {11/32} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & { 6/17} & {12/35} & { 1/ 3} & {12/37} & { 1/ 3} & {\color{red}  1/ 3} & {15/43} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & {16/45} & { 8/23} & {16/47} & { 1/ 3} & {\color{red} 17/52} & {\color{red} 18/53} & {19/54} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & { 5/14} & {20/57} & {10/29} & {20/59} & {\color{red}  1/ 3} & {\color{red} 11/32} & {23/65} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & {24/67} & { 6/17} & { 8/23} & {12/35} & {\color{red} 24/71} \\\hline
$3$ & { 4/13} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & {\color{red}  7/23} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & {\color{red} 11/35} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & {\color{red} 15/47} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {16/49} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & {\color{red} 19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {20/61} & { 1/ 3} & { 1/ 3} & { 5/16} & { 1/ 3} & { 1/ 3} & {\color{red} 23/71} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} \\\hline
$4$ & { 2/ 7} & { 2/ 7} & { 2/ 7} & { 1/ 4} & {\color{red} 12/49} & {\color{red}  9/34} & {\color{red}  2/ 7} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 8/27} & { 2/ 7} & { 2/ 7} & { 2/ 7} & {\color{red} 14/53} & {\color{red} 10/37} & {\color{red} 11/38} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 3/10} & {12/41} & { 2/ 7} & { 2/ 7} & { 2/ 7} & {\color{red}  7/25} & {\color{red}  5/17} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & {16/53} & { 8/27} & {16/55} & { 2/ 7} & {\color{red}  2/ 7} & {\color{red}  2/ 7} & {\color{red} 19/64} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & { 4/13} & {10/33} & {20/67} & { 5/17} & {20/69} & {\color{red}  2/ 7} & {\color{red} 11/38} & {\color{red} 23/77} & { 4/13} \\\hline
$5$ & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 4} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  9/31} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  7/23} & { 1/ 3} & { 1/ 3} & { 7/22} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 3/10} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red} 19/61} & { 1/ 3} & { 1/ 3} & {19/59} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 4/13} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & { 1/ 3} & {\color{red}  6/19} & { 1/ 3} & { 1/ 3} & {12/37} & { 1/ 3} \\\hline
$6$ & { 3/ 8} & { 3/ 8} & { 1/ 3} & {\color{red}  8/29} & { 1/ 3} & { 1/ 3} & { 8/23} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 1/ 3} & { 1/ 3} & {\color{red} 11/35} & { 1/ 3} & {11/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 14/41} & { 1/ 3} & { 1/ 3} & {13/38} & {14/39} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {17/49} & {\color{red} 19/59} & {\color{red}  1/ 3} & { 8/23} & {17/47} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 20/57} & {\color{red}  1/ 3} & {18/53} & {19/54} & { 4/11} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {23/65} & {\color{red}  1/ 3} & {\color{red} 21/61} & {11/31} & {23/63} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 26/73} & {\color{red} 23/67} & { 8/23} & { 5/14} & {26/71} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {29/81} & {\color{red} 13/38} \\\hline
$7$ & { 7/17} & { 5/13} & { 1/ 3} & { 2/ 7} & { 7/22} & { 8/23} & { 3/ 8} & { 2/ 5} & { 7/17} & { 7/17} & {13/35} & { 1/ 3} & { 1/ 3} & {11/31} & { 3/ 8} & {13/33} & { 7/17} & { 7/17} & {17/43} & { 4/11} & {13/38} & {14/39} & { 3/ 8} & {16/41} & {17/42} & { 7/17} & { 7/17} & { 5/13} & {19/53} & {17/47} & { 3/ 8} & {19/49} & { 2/ 5} & { 7/17} & { 7/17} & { 2/ 5} & {23/61} & {\color{red}  4/11} & { 3/ 8} & {22/57} & {23/58} & {24/59} & { 7/17} & { 7/17} & { 9/23} & {\color{red} 13/35} & { 3/ 8} & { 5/13} & {13/33} & {27/67} & { 7/17} & { 7/17} & {31/77} & { 5/13} & {\color{red}  3/ 8} & {28/73} & {29/74} & { 2/ 5} & {31/76} & { 7/17} \\\hline
$8$ & { 4/ 9} & {11/28} & {10/29} & { 1/ 3} & {10/31} & { 3/ 8} & { 2/ 5} & {11/26} & { 4/ 9} & { 4/ 9} & {15/37} & { 7/19} & { 1/ 3} & { 3/ 8} & {13/33} & { 7/17} & { 3/ 7} & { 4/ 9} & { 4/ 9} & {19/46} & {18/47} & { 3/ 8} & {16/41} & {17/42} & {18/43} & {19/44} & { 4/ 9} & { 4/ 9} & {23/55} & {11/28} & {19/49} & { 2/ 5} & { 7/17} & {11/26} & {23/53} & { 4/ 9} & { 4/ 9} & {27/64} & { 2/ 5} & {\color{red} 23/58} & {24/59} & { 5/12} & {26/61} & {27/62} & { 4/ 9} & { 4/ 9} & {31/73} & {15/37} & {\color{red} 27/67} & { 7/17} & {29/69} & { 3/ 7} & {31/71} & { 4/ 9} & { 4/ 9} & {35/82} & {34/83} & {\color{red} 31/76} & {32/77} & {11/26} \\\hline
$9$ & { 8/19} & { 2/ 5} & {11/31} & { 5/16} & { 1/ 3} & { 6/17} & { 2/ 5} & { 4/ 9} & { 4/ 9} & { 3/ 7} & {12/29} & { 2/ 5} & {15/41} & { 1/ 3} & {16/43} & { 9/22} & { 4/ 9} & { 4/ 9} & {16/37} & { 8/19} & {16/39} & { 2/ 5} & {19/51} & { 5/13} & {22/53} & { 4/ 9} & { 4/ 9} & {10/23} & {20/47} & { 5/12} & {20/49} & { 2/ 5} & {24/61} & {13/31} & { 4/ 9} & { 4/ 9} & {24/55} & { 3/ 7} & { 8/19} & {12/29} & {24/59} & { 2/ 5} & {30/71} & { 4/ 9} & { 4/ 9} & { 7/16} & {28/65} & {14/33} & {28/67} & { 7/17} & {\color{red} 28/69} & {17/40} & { 4/ 9} & { 4/ 9} & {32/73} & {16/37} & {32/75} & { 8/19} & {\color{red} 32/77} & {\color{red} 16/39} \\\hline
$10$ & { 2/ 5} & { 8/21} & { 4/11} & {11/34} & { 2/ 7} & { 1/ 3} & {14/37} & { 8/19} & { 8/19} & {12/29} & { 2/ 5} & {12/31} & { 3/ 8} & { 4/11} & { 1/ 3} & {17/46} & {19/47} & { 8/19} & { 8/19} & {16/39} & { 2/ 5} & {16/41} & { 8/21} & {16/43} & { 4/11} & {11/28} & { 8/19} & { 8/19} & { 5/12} & {20/49} & { 2/ 5} & {20/51} & { 5/13} & {\color{red} 20/53} & { 5/13} & { 9/22} & { 8/19} & { 8/19} & {12/29} & {24/59} & { 2/ 5} & {24/61} & {12/31} & {\color{red}  8/21} & { 2/ 5} & { 8/19} & { 8/19} & {28/67} & { 7/17} & {28/69} & { 2/ 5} & {28/71} & {\color{red}  7/18} & {\color{red} 11/28} & { 7/17} & { 8/19} & { 8/19} & {32/77} & {16/39} & {32/79} \\\hline
$11$ & { 8/21} & { 4/11} & { 8/23} & { 1/ 3} & {11/37} & { 1/ 3} & {14/39} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {12/31} & { 3/ 8} & { 4/11} & { 6/17} & {12/35} & { 1/ 3} & {18/49} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {16/43} & { 4/11} & {16/45} & {\color{red}  8/23} & {22/59} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & {10/27} & { 4/11} & { 5/14} & {26/69} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 3/ 8} & {24/65} & {\color{red}  4/11} & {30/79} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {28/73} & {14/37} & {28/75} & {\color{red}  7/19} & {34/89} & { 2/ 5} & { 2/ 5} & { 2/ 5} \\\hline
$12$ & { 4/11} & { 8/23} & { 1/ 3} & { 8/25} & { 1/ 3} & { 1/ 3} & {14/41} & { 8/21} & { 8/21} & { 8/21} & { 3/ 8} & { 4/11} & { 6/17} & {12/35} & { 1/ 3} & {\color{red} 12/37} & { 1/ 3} & {19/52} & { 8/21} & { 8/21} & { 8/21} & {16/43} & { 4/11} & {16/45} & { 8/23} & {16/47} & {\color{red}  1/ 3} & {\color{red} 11/31} & { 8/21} & { 8/21} & { 8/21} & {20/53} & {10/27} & { 4/11} & { 5/14} & {20/57} & {\color{red} 10/29} & {\color{red} 25/72} & {27/73} & { 8/21} & { 8/21} & { 8/21} & { 3/ 8} & {24/65} & { 4/11} & {24/67} & { 6/17} & {\color{red}  8/23} & {\color{red} 30/83} & { 8/21} & { 8/21} & { 8/21} & {14/37} & {28/75} & { 7/19} & { 4/11} & {\color{red} 14/39} & {\color{red} 28/79} & {\color{red} 11/31} & {35/94} \\\hline
$13$ & { 8/23} & { 8/23} & {\color{red}  8/25} & { 4/13} & {\color{red}  8/27} & {\color{red}  9/29} & {\color{red}  1/ 3} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & { 6/17} & {12/35} & {\color{red}  1/ 3} & {\color{red} 13/38} & { 8/23} & { 8/23} & { 1/ 3} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & {16/45} & { 8/23} & { 8/23} & { 1/ 3} & {\color{red} 16/49} & {\color{red} 21/64} & {\color{red} 22/65} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & { 5/14} & {20/57} & {\color{red} 10/29} & {\color{red} 20/59} & {\color{red} 21/61} & { 8/23} & { 8/23} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & {24/67} & { 6/17} & { 8/23} & { 8/23} & {\color{red} 24/71} & {\color{red} 29/86} & {\color{red} 10/29} & { 4/11} & { 4/11} & { 4/11} & { 4/11} & {14/39} & {28/79} & {\color{red}  7/20} & {\color{red} 28/81} & {\color{red} 14/41} \\\hline
$14$ & { 3/ 8} & { 3/ 8} & { 1/ 3} & { 1/ 3} & { 9/29} & { 1/ 3} & {11/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 8/23} & {12/35} & { 1/ 3} & {13/38} & {14/39} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 1/ 3} & { 8/23} & { 8/23} & {\color{red}  8/23} & {17/47} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 22/65} & { 1/ 3} & {18/53} & {19/54} & { 4/11} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 10/29} & {\color{red} 20/59} & {\color{red} 21/61} & {11/31} & {23/63} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 8/23} & {\color{red}  8/23} & {\color{red}  8/23} & {\color{red}  5/14} & {26/71} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 31/89} & {\color{red} 13/38} & {27/77} & {14/39} & {29/79} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 34/97} & {\color{red} 17/49} \\\hline
$15$ & { 2/ 5} & { 8/21} & { 1/ 3} & { 2/ 7} & { 1/ 3} & {11/31} & { 3/ 8} & {13/33} & { 2/ 5} & { 2/ 5} & { 6/17} & { 1/ 3} & {13/38} & {14/39} & { 3/ 8} & {16/41} & { 2/ 5} & { 2/ 5} & {22/59} & { 1/ 3} & { 8/23} & {17/47} & { 3/ 8} & {19/49} & { 2/ 5} & { 2/ 5} & {26/67} & { 6/17} & {19/54} & { 4/11} & { 3/ 8} & {22/57} & {23/58} & { 2/ 5} & { 2/ 5} & { 7/19} & {11/31} & {23/63} & { 3/ 8} & { 5/13} & {13/33} & { 2/ 5} & { 2/ 5} & { 8/21} & {\color{red}  5/14} & {\color{red} 26/71} & { 3/ 8} & {28/73} & {29/74} & { 2/ 5} & { 2/ 5} & { 9/23} & {\color{red} 34/93} & {\color{red} 29/79} & { 3/ 8} & {31/81} & {16/41} & {33/83} & { 2/ 5} & { 2/ 5} \\\hline
$16$ & {11/26} & {17/44} & { 1/ 3} & {\color{red} 13/46} & {15/47} & { 3/ 8} & {13/33} & { 7/17} & {11/26} & {11/26} & {20/53} & {\color{red}  1/ 3} & {18/55} & { 3/ 8} & {16/41} & {17/42} & {18/43} & {11/26} & {25/61} & {23/62} & { 1/ 3} & { 3/ 8} & {19/49} & { 2/ 5} & { 7/17} & {11/26} & {11/26} & { 2/ 5} & {26/71} & { 3/ 8} & {22/57} & {23/58} & {24/59} & { 5/12} & {11/26} & {11/26} & {31/79} & { 3/ 8} & { 5/13} & {13/33} & {27/67} & { 7/17} & {29/69} & {11/26} & {12/29} & {17/44} & {28/73} & {29/74} & { 2/ 5} & {31/76} & {32/77} & {11/26} & {11/26} & {13/32} & {\color{red} 31/81} & {\color{red} 16/41} & {33/83} & {17/42} & { 7/17} & {18/43} \\\hline
$17$ & { 4/ 9} & { 9/23} & {16/47} & { 1/ 3} & {\color{red} 15/49} & { 9/25} & { 7/17} & { 3/ 7} & { 4/ 9} & { 4/ 9} & { 2/ 5} & { 5/14} & { 1/ 3} & {10/29} & {23/59} & {18/43} & {19/44} & { 4/ 9} & { 4/ 9} & {13/32} & {24/65} & { 1/ 3} & {25/67} & { 7/17} & {11/26} & {23/53} & { 4/ 9} & { 4/ 9} & {30/73} & {14/37} & { 9/25} & {15/38} & { 5/12} & {26/61} & {27/62} & { 4/ 9} & { 4/ 9} & {17/41} & {32/83} & { 8/21} & { 7/17} & {29/69} & { 3/ 7} & {31/71} & { 4/ 9} & { 4/ 9} & {38/91} & { 9/23} & {37/93} & {32/77} & {11/26} & {34/79} & { 7/16} & { 4/ 9} & { 4/ 9} & {21/50} & {21/53} & { 7/17} & {18/43} & {37/87} \\\hline
$18$ & { 3/ 7} & {19/48} & {17/49} & {\color{red}  3/10} & { 1/ 3} & { 9/26} & {21/53} & { 4/ 9} & { 4/ 9} & {16/37} & { 8/19} & {11/29} & {\color{red} 20/59} & { 1/ 3} & {22/61} & {25/62} & { 4/ 9} & { 4/ 9} & {10/23} & {20/47} & {27/67} & {25/68} & { 1/ 3} & {13/35} & {29/71} & { 4/ 9} & { 4/ 9} & {24/55} & { 3/ 7} & { 8/19} & {30/77} & {14/39} & {30/79} & {33/80} & { 4/ 9} & { 4/ 9} & { 7/16} & {28/65} & {14/33} & {35/86} & {11/29} & {17/44} & {37/89} & { 4/ 9} & { 4/ 9} & {32/73} & {16/37} & {32/75} & { 8/19} & {19/48} & {38/97} & {41/98} & { 4/ 9} & { 4/ 9} & {18/41} & {36/83} & { 3/ 7} & {36/85} & {34/83} & {21/53} \\\hline
$19$ & {12/29} & { 2/ 5} & { 6/17} & { 4/13} & {\color{red}  2/ 7} & {\color{red}  1/ 3} & {21/55} & { 3/ 7} & { 3/ 7} & { 8/19} & {16/39} & { 2/ 5} & {22/61} & {\color{red} 10/31} & {\color{red}  1/ 3} & { 3/ 8} & {27/65} & { 3/ 7} & {20/47} & { 5/12} & {20/49} & { 2/ 5} & {26/71} & { 1/ 3} & {27/73} & {15/37} & { 3/ 7} & { 3/ 7} & { 8/19} & {12/29} & {24/59} & { 2/ 5} & {10/27} & {15/41} & {33/83} & { 3/ 7} & { 3/ 7} & {14/33} & {28/67} & { 7/17} & {28/69} & { 2/ 5} & {34/91} & { 9/23} & {13/31} & { 3/ 7} & {32/75} & { 8/19} & {32/77} & {16/39} & {32/79} & { 2/ 5} & {22/57} & { 7/17} & { 3/ 7} & { 3/ 7} & {36/85} & {18/43} & {12/29} & { 9/22} \\\hline
$20$ & { 2/ 5} & {12/31} & {19/53} & { 1/ 3} & { 2/ 7} & { 1/ 3} & { 7/19} & {12/29} & {12/29} & {16/39} & { 2/ 5} & {16/41} & { 8/21} & {\color{red} 11/32} & { 1/ 3} & {23/66} & {26/67} & {12/29} & {12/29} & {20/49} & { 2/ 5} & {20/51} & { 5/13} & {27/74} & { 1/ 3} & { 7/19} & {31/77} & {12/29} & {12/29} & {24/59} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 6/17} & {33/86} & {12/29} & {12/29} & { 7/17} & {28/69} & { 2/ 5} & {28/71} & { 7/18} & {28/73} & { 7/19} & {19/48} & {12/29} & {12/29} & {16/39} & {32/79} & { 2/ 5} & {32/81} & {16/41} & {\color{red} 32/83} & { 8/21} & {28/69} & {12/29} & {12/29} & { 9/22} & {36/89} \\\hline
$21$ & {12/31} & { 3/ 8} & { 4/11} & { 9/28} & { 1/ 3} & { 1/ 3} & {\color{red} 21/59} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {16/41} & { 8/21} & {16/43} & { 4/11} & { 8/23} & {11/31} & {25/69} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & {10/27} & { 4/11} & { 1/ 3} & {29/79} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & { 8/21} & { 3/ 8} & {24/65} & { 4/11} & {33/89} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {28/73} & {14/37} & {28/75} & { 7/19} & {37/99} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {32/83} & { 8/21} & {32/85} & {\color{red} 16/43} & {\color{red} 37/99} & { 2/ 5} & { 2/ 5} & { 2/ 5} \\\hline
$22$ & { 3/ 8} & { 3/ 8} & { 6/17} & {19/58} & {12/37} & {13/38} & {14/39} & {12/31} & {12/31} & {12/31} & { 8/21} & {16/43} & { 4/11} & {\color{red} 16/45} & {17/47} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {12/31} & {12/31} & { 5/13} & {20/53} & {\color{red} 10/27} & { 3/ 8} & { 3/ 8} & { 3/ 8} & { 1/ 3} & {15/41} & {12/31} & {12/31} & {12/31} & { 8/21} & { 3/ 8} & { 3/ 8} & { 4/11} & {\color{red} 24/67} & {\color{red}  6/17} & {\color{red}  9/25} & {12/31} & {12/31} & {12/31} & {28/73} & {14/37} & {28/75} & {\color{red}  7/19} & {\color{red}  4/11} & {\color{red} 29/79} & { 3/ 8} & {\color{red} 25/66} & {12/31} & {12/31} & {32/83} & { 8/21} & {\color{red} 32/85} & {\color{red} 16/43} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 33/92} & {12/31} \\\hline
$23$ & {13/33} & {11/29} & {12/35} & { 1/ 3} & {20/61} & {14/39} & { 3/ 8} & {16/41} & {13/33} & {13/33} & {16/43} & { 4/11} & {16/45} & {17/47} & { 3/ 8} & {19/49} & {13/33} & {13/33} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {10/27} & { 3/ 8} & {22/57} & {13/33} & {13/33} & {31/83} & { 1/ 3} & {31/85} & { 3/ 8} & {\color{red}  3/ 8} & { 5/13} & {13/33} & {13/33} & { 5/13} & {\color{red}  6/17} & {\color{red}  5/14} & {26/71} & { 3/ 8} & {28/73} & {29/74} & {13/33} & {13/33} & {\color{red}  7/19} & {\color{red}  4/11} & {\color{red} 29/79} & { 3/ 8} & {31/81} & {16/41} & {13/33} & {13/33} & {\color{red}  3/ 8} & { 3/ 8} & {\color{red} 16/43} & {\color{red}  3/ 8} & {34/89} & { 7/18} & {13/33} & {13/33} & {\color{red} 10/27} \\\hline
$24$ & { 7/17} & {23/60} & {\color{red}  1/ 3} & {12/37} & { 1/ 3} & { 3/ 8} & {16/41} & {17/42} & { 7/17} & { 7/17} & {\color{red}  4/11} & {16/45} & { 8/23} & { 3/ 8} & {19/49} & { 2/ 5} & { 7/17} & { 7/17} & {30/77} & { 4/11} & { 4/11} & { 3/ 8} & {22/57} & {23/58} & {24/59} & { 7/17} & { 7/17} & {16/43} & { 1/ 3} & { 3/ 8} & { 5/13} & {13/33} & {27/67} & { 7/17} & { 7/17} & {37/94} & {34/95} & { 3/ 8} & {28/73} & {29/74} & { 2/ 5} & {31/76} & { 7/17} & { 7/17} & {25/66} & { 3/ 8} & {31/81} & {16/41} & {33/83} & {17/42} & { 7/17} & { 7/17} & {23/58} & { 3/ 8} & {34/89} & { 7/18} & {36/91} & {37/92} & {38/93} & { 7/17} \\\hline
$25$ & { 3/ 7} & {12/31} & {\color{red}  1/ 3} & { 6/19} & { 4/13} & { 4/11} & {17/42} & {18/43} & { 3/ 7} & { 3/ 7} & {27/71} & {\color{red}  8/23} & {16/47} & {\color{red} 13/37} & { 2/ 5} & { 7/17} & {11/26} & { 3/ 7} & {33/79} & { 3/ 8} & { 6/17} & { 6/17} & {32/83} & {24/59} & { 5/12} & {26/61} & { 3/ 7} & { 9/22} & {33/89} & { 1/ 3} & {34/91} & {27/67} & { 7/17} & {29/69} & { 3/ 7} & { 3/ 7} & {39/97} & {18/49} & { 4/11} & { 2/ 5} & {31/76} & {32/77} & {11/26} & { 3/ 7} & { 3/ 7} & {21/53} & {\color{red}  5/14} & {\color{red} 32/83} & {17/42} & { 7/17} & {18/43} & {37/87} & { 3/ 7} & { 8/19} & {\color{red} 33/89} & {\color{red} 34/91} & {37/92} & {38/93} & {39/94} & { 8/19} \\\hline
$26$ & { 4/ 9} & {25/64} & {22/65} & { 1/ 3} & {\color{red}  3/10} & { 6/17} & {28/69} & {19/44} & { 4/ 9} & { 4/ 9} & {29/73} & {\color{red} 13/37} & {\color{red}  1/ 3} & {\color{red} 13/38} & {29/77} & {11/26} & {23/53} & { 4/ 9} & { 4/ 9} & {33/82} & {30/83} & {\color{red} 12/35} & {\color{red}  6/17} & {17/43} & {26/61} & {27/62} & { 4/ 9} & { 4/ 9} & {37/91} & {17/46} & { 1/ 3} & {35/94} & {39/95} & { 3/ 7} & {31/71} & { 4/ 9} & { 4/ 9} & {25/61} & {35/93} & {\color{red}  6/17} & {33/85} & {11/26} & {34/79} & { 7/16} & { 4/ 9} & { 4/ 9} & {\color{red} 25/61} & {\color{red} 35/93} & {\color{red} 17/47} & {\color{red} 17/43} & {37/87} & {19/44} & {39/89} & { 4/ 9} & { 4/ 9} & {\color{red} 26/63} & {\color{red} 35/93} & {\color{red} 35/94} & {\color{red} 39/95} & {41/96} \\\hline
$27$ & {16/37} & {13/33} & {23/67} & {\color{red}  3/10} & { 1/ 3} & {12/35} & {28/71} & { 4/ 9} & { 4/ 9} & {10/23} & {31/75} & { 7/19} & {\color{red} 26/77} & {\color{red}  1/ 3} & {\color{red} 28/79} & { 2/ 5} & { 4/ 9} & { 4/ 9} & {24/55} & { 3/ 7} & {33/85} & {\color{red} 15/43} & {\color{red}  1/ 3} & { 4/11} & {36/89} & { 4/ 9} & { 4/ 9} & { 7/16} & {28/65} & {19/47} & { 7/19} & { 1/ 3} & {36/97} & {20/49} & { 4/ 9} & { 4/ 9} & {32/73} & {16/37} & {38/91} & {\color{red} 32/85} & {\color{red}  1/99} & {\color{red} 36/97} & {37/90} & { 4/ 9} & { 4/ 9} & {18/41} & {36/83} & { 3/ 7} & {\color{red} 33/85} & {\color{red}  7/19} & {\color{red} 20/53} & {\color{red} 37/90} & { 4/ 9} & { 4/ 9} & {40/91} & {10/23} & {40/93} & {\color{red} 19/47} & {\color{red}  1/99} & {\color{red}  1/ 3} \\\hline
$28$ & { 8/19} & {27/68} & { 8/23} & {\color{red}  3/10} & {\color{red} 22/71} & {\color{red}  1/ 3} & {28/73} & {16/37} & {16/37} & {20/47} & { 5/12} & { 5/13} & {\color{red} 27/79} & {\color{red} 32/97} & {\color{red} 28/81} & {31/82} & {35/83} & {16/37} & { 3/ 7} & { 8/19} & {12/29} & { 3/ 8} & {\color{red} 31/89} & {\color{red} 13/38} & {34/91} & {19/46} & {16/37} & {28/65} & {14/33} & {28/67} & {39/97} & {18/49} & {\color{red}  1/99} & {27/73} & {28/69} & {16/37} & {16/37} & {32/75} & { 8/19} & {32/77} & {\color{red}  5/13} & {\color{red} 17/49} & {\color{red}  9/25} & { 2/ 5} & {16/37} & {16/37} & { 3/ 7} & {36/85} & {18/43} & {12/29} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red} 21/55} & {\color{red} 19/46} & {16/37} & {40/93} & {20/47} & { 8/19} & { 5/12} & {\color{red} 39/97} \\\hline
$29$ & {16/39} & { 2/ 5} & {25/71} & { 1/ 3} & { 7/22} & {\color{red} 25/74} & {28/75} & { 8/19} & { 8/19} & { 5/12} & {20/49} & { 2/ 5} & {29/81} & {\color{red} 18/53} & {19/54} & {\color{red} 14/39} & { 2/ 5} & { 8/19} & { 8/19} & {12/29} & {24/59} & { 2/ 5} & {\color{red} 33/91} & {14/39} & {14/39} & {18/47} & { 8/19} & { 8/19} & {28/67} & { 7/17} & {28/69} & { 2/ 5} & {26/71} & {\color{red}  1/99} & {31/84} & {21/52} & { 8/19} & { 8/19} & {32/77} & {16/39} & {32/79} & { 2/ 5} & {\color{red} 26/71} & {\color{red}  5/14} & {37/95} & { 8/19} & { 8/19} & {18/43} & {12/29} & { 9/22} & {36/89} & { 2/ 5} & {\color{red} 26/71} & {\color{red} 31/84} & {37/91} & { 8/19} & { 8/19} & { 5/12} & {40/97} & {20/49} \\\hline
$30$ & { 2/ 5} & {16/41} & {26/73} & {\color{red} 23/74} & { 1/ 3} & { 8/23} & {\color{red}  4/11} & {16/39} & {16/39} & {20/49} & { 2/ 5} & {20/51} & {31/83} & {19/54} & { 4/11} & { 3/ 8} & {\color{red} 11/29} & {16/39} & {16/39} & {24/59} & { 2/ 5} & {24/61} & {12/31} & { 3/ 8} & { 3/ 8} & { 3/ 8} & {38/97} & {16/39} & {16/39} & {28/69} & { 2/ 5} & {28/71} & { 7/18} & { 3/ 8} & {\color{red}  1/99} & {\color{red}  4/11} & {39/97} & {16/39} & {16/39} & {32/79} & { 2/ 5} & {32/81} & {16/41} & {\color{red} 31/83} & {\color{red}  1/99} & {\color{red} 11/29} & {16/39} & {16/39} & { 9/22} & {36/89} & { 2/ 5} & {36/91} & { 9/23} & {12/31} & {\color{red}  1/99} & {\color{red} 37/97} & {16/39} & {\color{red} 20/49} & {20/49} & {40/99} \\\hline
$31$ & {16/41} & {\color{red}  8/21} & { 9/25} & { 6/19} & {25/77} & {17/47} & { 3/ 8} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {20/51} & { 5/13} & {20/53} & { 4/11} & { 3/ 8} & {22/57} & {16/41} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {24/61} & {12/31} & {\color{red}  8/21} & { 5/13} & {16/41} & {16/41} & { 4/11} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {28/71} & {\color{red}  7/18} & {16/41} & {16/41} & {\color{red} 27/74} & {\color{red}  1/99} & {\color{red}  4/11} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {32/81} & {16/41} & {\color{red} 32/83} & { 8/21} & {\color{red} 32/85} & {\color{red} 32/87} & {\color{red}  3/ 8} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {36/91} & { 9/23} & {12/31} & {\color{red} 18/47} & {\color{red} 36/95} & {\color{red} 37/97} & {19/49} & { 2/ 5} & { 2/ 5} & { 2/ 5} \\\hline
$32$ & {17/42} & {\color{red} 29/76} & { 4/11} & { 1/ 3} & {\color{red} 25/79} & { 3/ 8} & {19/49} & { 2/ 5} & {17/42} & {17/42} & { 5/13} & {20/53} & {10/27} & { 3/ 8} & {22/57} & {23/58} & {17/42} & {17/42} & {16/41} & {16/41} & {12/31} & { 8/21} & { 5/13} & {13/33} & {27/67} & {17/42} & {21/53} & {19/51} & {16/41} & {16/41} & { 7/18} & {29/74} & { 2/ 5} & {17/42} & {17/42} & {\color{red} 34/93} & {\color{red}  1/99} & { 3/ 8} & {16/41} & {\color{red} 16/41} & {33/83} & {17/42} & {17/42} & {\color{red} 32/85} & {\color{red} 16/43} & { 3/ 8} & {34/89} & { 7/18} & {36/91} & {37/92} & {17/42} & {\color{red} 21/53} & {\color{red} 18/47} & {\color{red} 36/95} & {\color{red} 37/97} & {19/49} & {13/33} & { 2/ 5} & {\color{red} 23/57} & {17/42} \\\hline
$33$ & {18/43} & { 5/13} & {16/45} & {13/40} & { 1/ 3} & {15/41} & { 2/ 5} & { 7/17} & {18/43} & {18/43} & {\color{red} 20/53} & {10/27} & { 4/11} & {\color{red}  5/14} & {23/58} & {24/59} & { 5/12} & {18/43} & { 2/ 5} & { 8/21} & { 8/21} & { 3/ 8} & {13/33} & {27/67} & { 7/17} & {18/43} & {18/43} & { 5/13} & { 8/21} & { 8/21} & {\color{red} 23/60} & { 2/ 5} & {31/76} & {32/77} & {18/43} & {\color{red}  2/ 5} & {\color{red} 32/87} & {\color{red}  1/99} & {\color{red} 15/41} & {33/83} & {17/42} & { 7/17} & {18/43} & {18/43} & {25/63} & {\color{red}  1/99} & {\color{red}  1/99} & {36/91} & {37/92} & {38/93} & {39/94} & {\color{red} 38/91} & {\color{red}  2/ 5} & {\color{red}  5/13} & {\color{red}  1/99} & {13/33} & { 2/ 5} & {28/69} & { 7/17} & {38/91} \\\hline
$34$ & {19/44} & {31/80} & {\color{red}  8/23} & {27/82} & {\color{red} 13/43} & { 5/14} & { 7/17} & {11/26} & {19/44} & {19/44} & {34/89} & {\color{red}  4/11} & { 5/14} & {\color{red} 20/57} & {12/31} & { 5/12} & {26/61} & {19/44} & {41/97} & {\color{red} 37/98} & {16/43} & {24/65} & {\color{red} 26/71} & { 7/17} & {29/69} & { 3/ 7} & {19/44} & {22/53} & {37/99} & {16/43} & {16/43} & {34/87} & {32/77} & {11/26} & {34/79} & {19/44} & {\color{red} 21/53} & {\color{red}  5/14} & {\color{red}  1/99} & {\color{red} 26/71} & { 7/17} & {18/43} & {37/87} & {19/44} & {19/44} & {\color{red}  9/23} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 34/87} & {39/94} & { 8/19} & {41/96} & {\color{red}  3/ 7} & {\color{red} 41/97} & {\color{red} 37/98} & {\color{red}  1/99} & {\color{red}  1/99} & { 7/17} & {38/91} & {11/26} \\\hline
$35$ & { 4/ 9} & {16/41} & {\color{red} 16/47} & { 1/ 3} & {\color{red}  3/10} & {\color{red} 15/43} & {35/87} & {23/53} & { 4/ 9} & { 4/ 9} & {36/91} & {\color{red}  5/14} & {\color{red} 20/57} & {\color{red} 10/29} & { 7/19} & { 5/12} & {27/62} & { 4/ 9} & { 4/ 9} & {\color{red} 36/91} & {\color{red}  4/11} & { 4/11} & {\color{red} 23/64} & { 5/13} & { 3/ 7} & {31/71} & { 4/ 9} & { 4/ 9} & {\color{red}  2/ 5} & { 4/11} & {\color{red}  4/11} & {\color{red}  4/11} & {\color{red} 34/87} & {34/79} & { 7/16} & { 4/ 9} & { 4/ 9} & {\color{red} 23/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 35/87} & {19/44} & {39/89} & { 4/ 9} & { 4/ 9} & {\color{red} 23/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  7/19} & {\color{red}  5/12} & {42/97} & {43/98} & { 4/ 9} & { 4/ 9} & {\color{red} 23/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/95} & { 3/ 7} \\\hline
$36$ & {10/23} & {11/28} & {\color{red} 29/85} & {16/49} & { 1/ 3} & {\color{red} 15/44} & {35/89} & { 4/ 9} & { 4/ 9} & {24/55} & {38/93} & {\color{red} 17/47} & {\color{red} 10/29} & {\color{red} 11/32} & {\color{red} 34/97} & {39/98} & { 4/ 9} & { 4/ 9} & { 7/16} & {\color{red} 27/65} & {25/66} & {\color{red} 21/59} & {\color{red}  6/17} & {\color{red} 19/53} & {\color{red} 39/98} & { 4/ 9} & { 4/ 9} & {32/73} & {16/37} & {11/28} & {\color{red} 16/45} & {\color{red}  1/99} & {\color{red} 19/53} & {32/79} & { 4/ 9} & { 4/ 9} & {18/41} & {36/83} & {\color{red} 37/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 32/79} & { 4/ 9} & { 4/ 9} & {40/91} & {10/23} & {\color{red} 38/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 32/79} & { 4/ 9} & { 4/ 9} & {11/25} & {27/62} & {\color{red} 35/83} & {\color{red} 25/66} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$37$ & {20/47} & {17/43} & {10/29} & {\color{red}  8/25} & {17/52} & {\color{red} 18/53} & { 5/13} & {10/23} & {10/23} & { 3/ 7} & { 8/19} & { 3/ 8} & {\color{red} 20/59} & {\color{red} 17/49} & {\color{red} 11/31} & {19/50} & {23/54} & {10/23} & {28/65} & {14/33} & {\color{red} 17/43} & {\color{red} 19/53} & {\color{red}  5/14} & {\color{red} 17/47} & {\color{red} 27/73} & {\color{red} 28/69} & {10/23} & {16/37} & {32/75} & { 8/19} & {\color{red}  3/ 8} & {\color{red} 17/47} & {\color{red}  1/99} & {\color{red} 29/79} & {\color{red}  2/ 5} & {10/23} & {36/83} & { 3/ 7} & {36/85} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 32/81} & {10/23} & {10/23} & {40/93} & {20/47} & { 8/19} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/50} & {\color{red} 23/54} & {\color{red} 33/76} & {22/51} & {41/96} & {11/26} & {\color{red}  2/ 5} & {\color{red}  1/99} \\\hline
$38$ & { 5/12} & {35/88} & {31/89} & { 1/ 3} & {30/91} & {19/54} & {\color{red} 35/93} & {20/47} & {20/47} & { 8/19} & {12/29} & {19/49} & {\color{red} 21/61} & {11/31} & {\color{red} 23/63} & {\color{red}  3/ 8} & {31/76} & {20/47} & {14/33} & {28/67} & { 7/17} & {30/79} & {\color{red} 26/71} & { 3/ 8} & {\color{red}  3/ 8} & {11/28} & {20/47} & {20/47} & { 8/19} & {32/77} & {16/39} & {\color{red}  3/ 8} & { 3/ 8} & { 3/ 8} & {\color{red} 35/93} & {\color{red} 31/76} & {20/47} & {36/85} & {18/43} & {12/29} & {\color{red} 35/88} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 39/98} & {20/47} & {20/47} & { 8/19} & { 5/12} & {40/97} & {\color{red} 19/49} & {\color{red}  1/99} & {\color{red}  1/99} & {11/28} & {\color{red} 28/67} & {\color{red} 31/73} & {11/26} & {31/74} & {22/53} & {37/90} \\\hline
$39$ & {20/49} & { 2/ 5} & {32/91} & {\color{red}  4/13} & { 1/ 3} & { 4/11} & {\color{red}  3/ 8} & { 5/12} & { 5/12} & {12/29} & {24/59} & { 2/ 5} & {\color{red} 31/87} & {23/63} & { 3/ 8} & { 5/13} & {\color{red} 19/49} & { 5/12} & { 5/12} & { 7/17} & {28/69} & { 2/ 5} & {\color{red}  3/ 8} & {28/73} & {19/49} & {\color{red} 19/49} & {38/93} & { 5/12} & {32/77} & {16/39} & {32/79} & { 2/ 5} & {19/49} & {19/49} & {\color{red}  1/99} & {\color{red}  8/21} & { 5/12} & { 5/12} & {12/29} & { 9/22} & {36/89} & { 2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 25/64} & { 5/12} & { 5/12} & {40/97} & {20/49} & {40/99} & { 2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  3/ 8} & {\color{red} 38/93} & {\color{red} 37/89} & {22/53} & {37/90} & {11/27} \\\hline
$40$ & { 2/ 5} & {20/51} & {11/31} & {\color{red} 16/53} & {\color{red}  9/29} & { 3/ 8} & {22/57} & {20/49} & {20/49} & {24/59} & { 2/ 5} & {24/61} & {31/84} & { 3/ 8} & { 5/13} & {13/33} & { 2/ 5} & {20/49} & {20/49} & {28/69} & { 2/ 5} & {28/71} & {\color{red} 28/73} & {29/74} & { 2/ 5} & { 2/ 5} & { 5/13} & {20/49} & {20/49} & {32/79} & { 2/ 5} & {\color{red} 32/81} & {33/83} & { 2/ 5} & {\color{red} 35/92} & {\color{red}  1/99} & {\color{red} 17/44} & {20/49} & {20/49} & {36/89} & {\color{red}  2/ 5} & { 2/ 5} & { 2/ 5} & {\color{red} 33/92} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/49} & {20/49} & {20/49} & {40/99} & { 2/ 5} & {21/53} & {20/51} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 29/75} & {\color{red} 31/79} & {\color{red} 11/27} & {11/27} & {23/57} \\\hline
$41$ & { 7/17} & {\color{red}  5/13} & {34/95} & { 1/ 3} & {\color{red} 17/56} & {18/49} & {23/58} & {24/59} & { 7/17} & { 7/17} & {24/61} & {12/31} & { 8/21} & {19/53} & {13/33} & {27/67} & { 7/17} & { 7/17} & {\color{red}  2/ 5} & { 2/ 5} & {28/71} & { 7/18} & {29/74} & { 2/ 5} & {31/76} & { 7/17} & { 7/17} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {32/81} & {33/83} & {17/42} & { 7/17} & { 7/17} & {\color{red} 18/47} & {\color{red}  1/99} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {37/92} & {38/93} & { 7/17} & { 7/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 2/ 5} & {\color{red}  2/ 5} & {28/69} & { 7/17} & { 7/17} & {\color{red} 33/85} & {\color{red}  1/99} & {\color{red}  1/99} & {31/79} & {39/98} & {23/57} & { 9/22} & { 7/17} \\\hline
$42$ & {11/26} & {\color{red} 37/96} & {35/97} & {\color{red}  9/29} & { 1/ 3} & { 9/25} & {24/59} & { 5/12} & {11/26} & {11/26} & {12/31} & { 8/21} & { 3/ 8} & {\color{red} 33/97} & {28/71} & { 7/17} & {29/69} & {11/26} & {\color{red} 35/87} & {20/51} & { 7/18} & {28/73} & {\color{red} 14/37} & {31/76} & {32/77} & {11/26} & {11/26} & {\color{red} 37/96} & {20/51} & {20/51} & {16/41} & {17/42} & { 7/17} & {18/43} & {11/26} & {11/26} & {\color{red}  3/ 8} & {\color{red}  1/99} & {20/51} & {\color{red} 20/51} & {38/93} & {39/94} & { 8/19} & {11/26} & {\color{red} 35/86} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {28/69} & { 7/17} & {38/91} & {11/26} & {11/26} & {\color{red} 24/61} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 28/71} & { 9/22} & {29/70} & {34/81} \\\hline
$43$ & {23/53} & {19/49} & { 4/11} & {\color{red} 28/89} & {\color{red} 16/55} & { 6/17} & {31/76} & {26/61} & {\color{red} 42/97} & {23/53} & {\color{red}  8/21} & { 3/ 8} & {24/65} & { 4/11} & {\color{red} 35/94} & {29/69} & { 3/ 7} & {23/53} & {\color{red} 22/53} & {\color{red} 28/73} & {28/73} & {14/37} & {\color{red} 28/75} & {\color{red} 30/77} & {11/26} & {34/79} & {23/53} & {\color{red}  2/ 5} & {\color{red}  5/13} & { 5/13} & { 5/13} & {\color{red}  8/21} & {18/43} & {37/87} & {19/44} & {23/53} & {\color{red} 35/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 30/91} & {\color{red}  5/13} & { 8/19} & {41/96} & {42/97} & {23/53} & {\color{red} 19/49} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/76} & {11/26} & { 3/ 7} & {23/53} & {23/53} & {\color{red} 23/60} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {34/81} & {31/73} \\\hline
$44$ & { 4/ 9} & {23/59} & { 5/14} & { 1/ 3} & {\color{red} 19/59} & {\color{red}  9/26} & { 2/ 5} & {27/62} & { 4/ 9} & { 4/ 9} & {\color{red} 23/59} & {24/65} & { 4/11} & {\color{red} 24/67} & {\color{red} 31/87} & {\color{red} 32/79} & {31/71} & { 4/ 9} & { 4/ 9} & {\color{red} 23/59} & {\color{red} 20/53} & {\color{red} 28/75} & {\color{red}  7/19} & {\color{red} 32/87} & {\color{red} 33/79} & { 7/16} & { 4/ 9} & { 4/ 9} & {\color{red} 23/59} & {\color{red}  1/99} & {\color{red} 20/53} & {\color{red}  1/99} & {\color{red} 37/96} & {19/44} & {39/89} & { 4/ 9} & { 4/ 9} & {\color{red} 28/71} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 2/ 5} & {42/97} & {43/98} & { 4/ 9} & { 4/ 9} & {\color{red} 39/98} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/57} & {23/53} & {29/66} & { 4/ 9} & { 4/ 9} & {\color{red} 39/98} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 40/97} \\\hline
$45$ & {24/55} & {20/51} & {\color{red} 20/57} & {\color{red} 26/81} & { 1/ 3} & {\color{red} 22/63} & {31/79} & { 4/ 9} & { 4/ 9} & { 7/16} & {15/37} & {\color{red} 26/71} & {24/67} & {\color{red}  6/17} & {\color{red}  1/99} & {\color{red} 19/49} & { 4/ 9} & { 4/ 9} & {32/73} & {\color{red} 34/83} & {\color{red}  7/19} & {\color{red}  7/19} & {\color{red}  4/11} & {\color{red}  1/99} & {\color{red} 19/49} & { 4/ 9} & { 4/ 9} & {18/41} & {\color{red} 35/83} & {\color{red} 35/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/49} & { 4/ 9} & { 4/ 9} & {40/91} & {10/23} & {\color{red} 20/51} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/79} & { 4/ 9} & { 4/ 9} & {11/25} & {27/62} & {15/37} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/79} & { 4/ 9} & { 4/ 9} & {37/84} & {24/55} & {\color{red} 15/37} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$46$ & { 3/ 7} & {28/71} & {\color{red} 10/29} & {\color{red} 19/59} & {\color{red} 19/61} & {11/31} & {37/96} & {\color{red} 23/54} & {24/55} & {28/65} & {\color{red}  9/22} & {\color{red}  7/19} & {\color{red}  6/17} & {\color{red}  5/14} & {\color{red} 26/71} & {\color{red}  3/ 8} & {\color{red} 30/73} & {24/55} & {16/37} & {32/75} & {\color{red}  5/13} & {\color{red}  1/99} & {\color{red} 29/79} & {\color{red}  1/99} & {\color{red}  3/ 8} & {\color{red} 33/82} & {24/55} & {36/83} & { 3/ 7} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 36/91} & {24/55} & {10/23} & {40/93} & {20/47} & {\color{red}  3/ 8} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/59} & {24/55} & {27/62} & {22/51} & {41/96} & {\color{red} 28/71} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/96} & {24/55} & {24/55} & {16/37} & { 3/ 7} & {\color{red} 37/89} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$47$ & { 8/19} & {21/53} & {\color{red} 20/59} & { 1/ 3} & {\color{red}  1/99} & {23/63} & {\color{red} 14/37} & { 3/ 7} & { 3/ 7} & {14/33} & {28/67} & {11/29} & {\color{red}  1/99} & {26/71} & {\color{red}  3/ 8} & {\color{red} 28/73} & {\color{red} 38/93} & { 3/ 7} & {32/75} & { 8/19} & {\color{red} 31/77} & {\color{red}  1/99} & {\color{red}  3/ 8} & {31/81} & {\color{red} 31/81} & {\color{red} 20/51} & { 3/ 7} & { 3/ 7} & {36/85} & {18/43} & {\color{red} 29/75} & {\color{red} 34/89} & {\color{red} 34/89} & {\color{red}  1/99} & {\color{red} 13/34} & { 3/ 7} & { 3/ 7} & {20/47} & { 8/19} & { 5/12} & {\color{red}  1/99} & {\color{red} 20/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 11/28} & { 3/ 7} & {41/96} & {11/26} & {31/74} & {\color{red} 21/53} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 33/85} & { 3/ 7} & { 3/ 7} & {31/73} & { 8/19} & {38/91} & {\color{red}  1/99} \\\hline
$48$ & {12/29} & {39/98} & {\color{red} 34/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 8} & { 5/13} & { 8/19} & { 8/19} & {28/67} & { 7/17} & {\color{red} 30/79} & {\color{red} 12/35} & { 3/ 8} & {28/73} & {29/74} & {\color{red} 36/91} & { 8/19} & { 8/19} & {32/77} & {16/39} & {\color{red}  3/ 8} & {31/81} & {16/41} & {\color{red} 36/91} & {\color{red} 36/91} & { 8/19} & { 8/19} & {18/43} & {12/29} & { 9/22} & {\color{red}  7/18} & {36/91} & {\color{red} 36/91} & {\color{red} 33/91} & {\color{red} 28/71} & { 8/19} & { 8/19} & { 5/12} & {40/97} & {20/49} & {\color{red} 13/33} & {\color{red}  4/11} & {\color{red}  1/99} & {\color{red}  1/99} & { 8/19} & { 8/19} & {31/74} & {22/53} & {37/90} & {\color{red} 39/98} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 39/98} & { 8/19} & { 8/19} & {38/91} & {12/29} & {16/39} \\\hline
$49$ & {24/59} & { 2/ 5} & {\color{red} 26/75} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/53} & {13/33} & {12/29} & {12/29} & { 7/17} & {28/69} & { 2/ 5} & {\color{red} 26/75} & {\color{red} 25/73} & {29/74} & { 2/ 5} & {\color{red} 28/69} & {12/29} & {12/29} & {16/39} & {32/79} & { 2/ 5} & {16/41} & {33/83} & {17/42} & {\color{red} 28/69} & {\color{red} 21/53} & {12/29} & {12/29} & { 9/22} & {36/89} & { 2/ 5} & {37/92} & {\color{red} 28/69} & {\color{red} 28/69} & {\color{red}  1/99} & {\color{red} 37/97} & {\color{red} 40/97} & {40/97} & {20/49} & {\color{red} 40/99} & {28/69} & {\color{red} 28/69} & {\color{red} 31/87} & {\color{red}  1/99} & {\color{red} 12/35} & {\color{red} 21/53} & {12/29} & {37/90} & {\color{red} 11/27} & {24/59} & {24/59} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  9/23} & {12/29} & {12/29} & {16/39} & {24/59} \\\hline
$50$ & { 5/12} & {24/61} & {\color{red} 25/72} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 32/91} & {27/67} & { 7/17} & {\color{red} 32/77} & {\color{red} 31/76} & { 2/ 5} & {28/71} & {15/41} & {\color{red} 25/74} & { 2/ 5} & {31/76} & {32/77} & {\color{red} 32/77} & {\color{red} 32/79} & {32/79} & { 2/ 5} & {32/81} & {\color{red} 31/83} & {17/42} & { 7/17} & {\color{red} 39/94} & {\color{red} 31/76} & {\color{red} 35/89} & {\color{red} 36/89} & {36/89} & { 2/ 5} & {37/92} & {38/93} & {39/94} & {\color{red} 39/94} & {\color{red} 39/98} & {\color{red} 33/95} & {\color{red} 39/98} & {\color{red} 40/99} & {40/99} & {28/69} & { 7/17} & { 5/12} & {\color{red} 31/76} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  7/18} & {\color{red} 39/98} & {24/59} & { 9/22} & {29/70} & { 5/12} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 39/97} & {\color{red} 24/59} & { 7/17} & { 5/12} \\\hline
$51$ & {26/61} & {\color{red} 12/31} & {\color{red} 33/94} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 26/75} & { 7/17} & {29/69} & {\color{red} 37/87} & {\color{red}  5/12} & {28/71} & { 7/18} & {\color{red} 27/73} & {\color{red}  1/99} & {\color{red} 21/55} & {32/77} & {11/26} & {\color{red} 37/87} & {\color{red} 13/32} & { 2/ 5} & {32/81} & {16/41} & {\color{red} 32/83} & { 7/17} & {18/43} & {37/87} & {\color{red} 37/87} & { 2/ 5} & { 2/ 5} & { 2/ 5} & {36/91} & {\color{red}  9/23} & {39/94} & { 8/19} & {\color{red} 31/73} & {\color{red}  5/12} & {\color{red} 13/35} & { 2/ 5} & { 2/ 5} & { 2/ 5} & { 7/17} & {38/91} & {11/26} & {\color{red} 31/73} & {\color{red}  2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/66} & {\color{red} 23/66} & {29/70} & {34/81} & {31/73} & {26/61} & {\color{red} 22/57} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 7/17} & { 5/12} & {35/83} \\\hline
$52$ & {27/62} & {\color{red} 23/60} & {\color{red}  6/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  2/ 5} & { 3/ 7} & {\color{red} 10/23} & {\color{red} 26/61} & {\color{red}  7/18} & {28/73} & {14/37} & {\color{red}  1/99} & {\color{red} 16/43} & {11/26} & {34/79} & {\color{red} 10/23} & {\color{red} 33/80} & {\color{red} 20/51} & {16/41} & {32/83} & {\color{red}  8/21} & {\color{red} 36/95} & {37/87} & {19/44} & {\color{red} 10/23} & {\color{red} 36/89} & {\color{red}  9/23} & {\color{red} 11/28} & { 9/23} & {\color{red} 12/31} & {\color{red}  2/ 5} & {41/96} & {42/97} & {\color{red} 10/23} & {\color{red} 39/98} & {\color{red}  1/99} & {\color{red} 20/51} & {\color{red} 20/51} & {\color{red}  1/99} & {11/26} & { 3/ 7} & {23/53} & {27/62} & {\color{red} 31/79} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {31/73} & {40/93} & {10/23} & {27/62} & {\color{red} 26/67} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  7/20} & {26/61} \\\hline
$53$ & { 4/ 9} & {\color{red} 37/96} & {\color{red} 23/65} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/79} & {31/71} & { 4/ 9} & { 4/ 9} & {\color{red} 37/96} & {14/37} & {28/75} & {\color{red}  1/99} & {\color{red}  1/99} & { 9/22} & { 7/16} & { 4/ 9} & { 4/ 9} & {\color{red} 12/31} & {32/83} & { 8/21} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 40/97} & {39/89} & { 4/ 9} & { 4/ 9} & {\color{red} 12/31} & {\color{red}  1/99} & {12/31} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 41/97} & {43/98} & { 4/ 9} & { 4/ 9} & {\color{red} 37/96} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {23/53} & {29/66} & { 4/ 9} & { 4/ 9} & {\color{red} 37/96} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {10/23} & {40/91} & { 4/ 9} & { 4/ 9} & {\color{red} 37/94} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 33/98} \\\hline
$54$ & { 7/16} & {\color{red} 32/83} & { 4/11} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/60} & { 4/ 9} & { 4/ 9} & {32/73} & {\color{red} 33/83} & {\color{red} 28/75} & { 7/19} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/60} & { 4/ 9} & { 4/ 9} & {18/41} & {19/46} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/60} & { 4/ 9} & { 4/ 9} & {40/91} & {\color{red} 37/89} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/98} & { 4/ 9} & { 4/ 9} & {11/25} & {\color{red} 23/54} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 23/60} & { 4/ 9} & { 4/ 9} & {37/84} & {24/55} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  9/28} & { 4/ 9} & { 4/ 9} & {26/59} & {38/87} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$55$ & {28/65} & {\color{red} 29/75} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {26/71} & {\color{red}  3/ 8} & {\color{red} 31/73} & {\color{red} 24/55} & {16/37} & {\color{red} 31/76} & {\color{red}  1/99} & {\color{red}  6/19} & {\color{red} 29/79} & {\color{red}  4/13} & {\color{red}  1/99} & {\color{red} 17/41} & {\color{red} 24/55} & {36/83} & { 3/ 7} & {\color{red} 18/47} & {\color{red}  1/99} & {\color{red} 32/87} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/91} & {\color{red} 24/55} & {10/23} & {40/93} & {\color{red} 33/85} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  2/ 5} & { 7/16} & {27/62} & {22/51} & {\color{red} 31/76} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 28/71} & { 7/16} & {24/55} & {16/37} & { 3/ 7} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 27/88} & { 7/16} & {38/87} & {13/30} & {40/93} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$56$ & {14/33} & {\color{red} 25/64} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 3/ 8} & {\color{red} 28/73} & {\color{red} 35/83} & {\color{red} 40/93} & {32/75} & { 8/19} & {\color{red}  4/11} & {\color{red}  1/99} & { 3/ 8} & {31/81} & {\color{red} 16/41} & {\color{red}  7/17} & {\color{red} 40/93} & { 3/ 7} & {36/85} & {\color{red} 25/64} & {\color{red}  1/99} & {\color{red} 34/89} & {\color{red}  7/18} & {\color{red} 13/33} & {15/37} & {\color{red} 40/93} & {40/93} & {20/47} & { 8/19} & {\color{red}  1/99} & {\color{red}  1/99} & {13/33} & {\color{red} 13/33} & {\color{red}  4/11} & {\color{red} 35/83} & {\color{red}  3/ 7} & {41/96} & {11/26} & {\color{red} 25/64} & {\color{red}  1/99} & {\color{red} 31/79} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 15/37} & {\color{red}  3/ 7} & { 3/ 7} & {31/73} & { 8/19} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/ 3} & {28/65} & {40/93} & {26/61} & {41/97} & {\color{red}  1/99} & {\color{red}  1/99} \\\hline
$57$ & {28/67} & {\color{red} 38/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 26/73} & {29/74} & {\color{red} 37/89} & {\color{red} 36/85} & { 8/19} & {32/77} & {\color{red} 37/99} & {\color{red}  1/99} & {\color{red}  1/99} & {16/41} & {33/83} & {\color{red} 19/47} & {\color{red} 36/85} & {36/85} & {18/43} & {12/29} & {\color{red}  1/99} & { 7/18} & {36/91} & {37/92} & {\color{red} 37/92} & {\color{red} 31/75} & {\color{red} 11/26} & { 8/19} & { 5/12} & {\color{red} 38/97} & {\color{red} 13/33} & { 2/ 5} & {\color{red} 39/97} & {\color{red} 28/71} & {\color{red} 35/86} & {\color{red} 11/26} & {11/26} & {31/74} & {22/53} & {\color{red} 39/98} & {\color{red} 39/97} & {\color{red} 39/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 37/89} & {\color{red}  8/19} & { 8/19} & {38/91} & {12/29} & {\color{red} 39/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 19/59} & {14/33} & {41/97} & {13/31} & {37/89} & {\color{red} 25/63} \\\hline
$58$ & { 7/17} & {\color{red}  9/23} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & { 2/ 5} & {\color{red} 38/93} & {\color{red}  5/12} & {32/77} & {16/39} & {\color{red} 30/79} & {\color{red}  1/99} & {\color{red}  1/99} & {33/83} & {17/42} & { 7/17} & {\color{red}  5/12} & {\color{red}  5/12} & {12/29} & { 9/22} & {\color{red} 33/89} & {\color{red}  5/13} & {37/92} & {38/93} & { 7/17} & { 7/17} & {\color{red}  5/12} & { 5/12} & {40/97} & {20/49} & { 2/ 5} & {28/69} & { 7/17} & { 7/17} & {\color{red}  1/99} & {\color{red}  2/ 5} & {\color{red} 38/91} & {22/53} & {37/90} & {\color{red} 11/27} & { 9/22} & { 7/17} & { 7/17} & {\color{red}  1/99} & {\color{red} 37/99} & {\color{red} 38/91} & {38/91} & {12/29} & {\color{red} 16/39} & { 7/17} & { 7/17} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 29/94} & {28/67} & {37/89} & {\color{red} 26/63} & { 7/17} \\\hline
$59$ & {29/69} & { 2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {31/76} & {32/77} & {\color{red} 34/81} & {\color{red} 23/56} & {32/79} & { 2/ 5} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 22/57} & { 7/17} & {18/43} & {\color{red} 18/43} & {\color{red} 37/90} & { 9/22} & {36/89} & { 2/ 5} & {\color{red}  1/99} & {38/93} & {39/94} & {\color{red} 38/91} & {\color{red} 39/95} & {\color{red} 39/97} & {\color{red} 37/90} & {20/49} & {40/99} & { 2/ 5} & { 7/17} & {38/91} & {\color{red} 34/81} & {\color{red} 11/28} & {\color{red} 23/60} & {\color{red} 37/90} & {37/90} & {11/27} & { 9/22} & {29/70} & {34/81} & {\color{red} 34/81} & {\color{red} 33/91} & {\color{red}  1/99} & {\color{red}  8/23} & {\color{red} 16/39} & {16/39} & { 7/17} & { 5/12} & {\color{red}  5/12} & {\color{red} 32/79} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/ 3} & { 7/17} & {41/99} & {18/43} \\\hline
$60$ & { 3/ 7} & {28/71} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 31/77} & {11/26} & { 3/ 7} & { 3/ 7} & { 2/ 5} & {32/81} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {18/43} & {37/87} & { 3/ 7} & {\color{red} 36/89} & {36/89} & { 2/ 5} & {36/91} & {\color{red}  1/99} & {\color{red} 37/94} & { 8/19} & {41/96} & { 3/ 7} & {\color{red} 13/33} & {\color{red} 40/99} & {40/99} & { 2/ 5} & {\color{red} 21/53} & {38/91} & {11/26} & { 3/ 7} & { 3/ 7} & {\color{red}  1/99} & {\color{red} 28/71} & {\color{red} 23/57} & {23/57} & {\color{red}  2/ 5} & {34/81} & {31/73} & {\color{red} 26/61} & {\color{red} 40/97} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red} 35/99} & {\color{red} 25/62} & { 5/12} & {35/83} & {26/61} & {\color{red} 41/96} & {\color{red} 39/98} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {\color{red}  1/99} & {18/43} & {11/26} \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 4, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a1b2c3.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 6 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  2/11 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  3/16 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  4/21 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  5/26 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  6/31 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  7/36 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  8/41 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 &  9/46 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 & 10/51 &  1/ 5 &  1/ 5 &  1/ 5 &  1/ 5 \\\hline
$2$ &  1/ 4 &  1/ 4 &  1/ 5 &  1/ 4 &  1/ 4 &  1/ 4 &  3/14 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  5/22 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$3$ &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 \\\hline
$4$ &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 \\\hline
$5$ &  1/ 5 &  2/ 9 &  2/ 9 &  2/ 9 &  3/14 &  1/ 5 &  2/ 9 &  2/ 9 &  2/ 9 &  4/19 &  2/ 9 &  2/ 9 &  2/ 9 &  5/23 &  5/24 &  2/ 9 &  2/ 9 &  2/ 9 &  3/14 &  2/ 9 &  2/ 9 &  2/ 9 &  7/32 &  7/33 &  2/ 9 &  2/ 9 &  2/ 9 &  8/37 &  2/ 9 &  2/ 9 &  2/ 9 &  9/41 &  3/14 &  2/ 9 &  2/ 9 &  2/ 9 &  5/23 &  2/ 9 &  2/ 9 &  2/ 9 & 11/50 & 11/51 &  2/ 9 &  2/ 9 &  2/ 9 & 12/55 &  2/ 9 &  2/ 9 &  2/ 9 & 13/59 \\\hline
$6$ &  1/ 4 &  1/ 4 &  3/14 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  5/22 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$7$ &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 \\\hline
$8$ &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 \\\hline
$9$ &  3/14 &  3/13 &  3/13 &  3/13 &  2/ 9 &  3/14 &  3/13 &  3/13 &  5/22 &  5/23 &  3/13 &  3/13 &  3/13 &  2/ 9 &  3/13 &  3/13 &  3/13 &  7/31 &  9/41 &  3/13 &  3/13 &  8/35 &  2/ 9 &  3/13 &  3/13 &  3/13 &  9/40 &  3/13 &  3/13 &  3/13 &  5/22 &  2/ 9 &  3/13 &  3/13 & 11/48 & 11/49 &  3/13 &  3/13 &  3/13 & 12/53 &  3/13 &  3/13 &  3/13 & 13/57 & 13/58 &  3/13 &  3/13 & 14/61 &  7/31 &  3/13 \\\hline
$10$ &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  5/22 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$11$ &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 \\\hline
$12$ &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 \\\hline
$13$ &  2/ 9 &  4/17 &  4/17 &  4/17 &  5/22 &  2/ 9 &  4/17 &  4/17 &  3/13 &  2/ 9 &  4/17 &  4/17 &  7/30 &  7/31 &  4/17 &  4/17 &  4/17 &  8/35 &  4/17 &  4/17 &  4/17 &  3/13 & 12/53 &  4/17 &  4/17 & 10/43 &  5/22 &  4/17 &  4/17 & 11/47 & 11/48 &  4/17 &  4/17 &  4/17 &  3/13 &  4/17 &  4/17 &  4/17 & 13/56 &  8/35 &  4/17 &  4/17 &  7/30 & 14/61 &  4/17 &  4/17 & 15/64 &  3/13 &  4/17 &  4/17 \\\hline
$14$ &  1/ 4 &  1/ 4 &  5/22 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$15$ &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 \\\hline
$16$ &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 \\\hline
$17$ &  5/22 &  5/21 &  5/21 &  5/21 &  3/13 &  5/22 &  5/21 &  5/21 &  7/30 &  5/22 &  5/21 &  5/21 &  4/17 &  8/35 &  5/21 &  5/21 &  9/38 &  3/13 &  5/21 &  5/21 &  5/21 & 10/43 &  5/21 &  5/21 &  5/21 & 11/47 &  3/13 &  5/21 &  5/21 &  4/17 &  3/13 &  5/21 &  5/21 & 13/55 & 13/56 &  5/21 &  5/21 & 14/59 &  7/30 &  5/21 &  5/21 &  5/21 & 15/64 &  5/21 &  5/21 &  5/21 &  4/17 & 10/43 &  5/21 &  5/21 \\\hline
$18$ &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$19$ &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 \\\hline
$20$ &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 \\\hline
$21$ &  3/13 &  6/25 &  6/25 &  6/25 &  7/30 &  3/13 &  6/25 &  6/25 &  4/17 &  3/13 &  6/25 &  6/25 &  9/38 &  3/13 &  6/25 &  6/25 &  5/21 & 10/43 &  6/25 &  6/25 & 11/46 & 11/47 &  6/25 &  6/25 &  6/25 &  4/17 &  6/25 &  6/25 &  6/25 & 13/55 & 18/77 &  6/25 &  6/25 & 14/59 & 18/77 &  6/25 &  6/25 &  5/21 & 15/64 &  6/25 &  6/25 & 16/67 &  4/17 &  6/25 &  6/25 & 17/71 & 17/72 &  6/25 &  6/25 &  6/25 \\\hline
$22$ &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$23$ &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 \\\hline
$24$ &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 \\\hline
$25$ &  7/30 &  7/29 &  7/29 &  7/29 &  4/17 &  7/30 &  7/29 &  7/29 &  9/38 &  7/30 &  7/29 &  7/29 &  5/21 &  7/30 &  7/29 &  7/29 & 11/46 & 11/47 &  7/29 &  7/29 &  6/25 &  4/17 &  7/29 &  7/29 & 13/54 & 13/55 &  7/29 &  7/29 &  7/29 & 14/59 &  7/29 &  7/29 &  7/29 &  5/21 & 21/89 &  7/29 &  7/29 & 16/67 & 21/89 &  7/29 &  7/29 & 17/71 & 17/72 &  7/29 &  7/29 &  6/25 &  9/38 &  7/29 &  7/29 & 19/79 \\\hline
$26$ &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$27$ &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 \\\hline
$28$ &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 \\\hline
$29$ &  4/17 &  8/33 &  8/33 &  8/33 &  9/38 &  4/17 &  8/33 &  8/33 &  5/21 &  4/17 &  8/33 &  8/33 & 11/46 &  4/17 &  8/33 &  8/33 &  6/25 &  4/17 &  8/33 &  8/33 & 13/54 & 13/55 &  8/33 &  8/33 &  7/29 & 14/59 &  8/33 &  8/33 & 15/62 &  5/21 &  8/33 &  8/33 &  8/33 & 16/67 &  8/33 &  8/33 &  8/33 & 17/71 & 19/80 &  8/33 &  8/33 &  6/25 & 19/80 &  8/33 &  8/33 & 19/79 & 19/80 &  8/33 &  8/33 & 20/83 \\\hline
$30$ &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$31$ &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 \\\hline
$32$ &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 \\\hline
$33$ &  9/38 &  9/37 &  9/37 &  9/37 &  5/21 &  9/38 &  9/37 &  9/37 & 11/46 &  9/38 &  9/37 &  9/37 &  6/25 &  9/38 &  9/37 &  9/37 & 13/54 &  9/38 &  9/37 &  9/37 &  7/29 & 14/59 &  9/37 &  9/37 & 15/62 &  5/21 &  9/37 &  9/37 &  8/33 & 16/67 &  9/37 &  9/37 & 17/70 & 17/71 &  9/37 &  9/37 &  9/37 &  6/25 &  9/37 &  9/37 &  9/37 & 19/79 & 16/67 &  9/37 &  9/37 & 20/83 & 16/67 &  9/37 &  9/37 &  7/29 \\\hline
$34$ &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 21/86 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$35$ &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 \\\hline
$36$ & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 \\\hline
$37$ &  5/21 & 10/41 & 10/41 & 10/41 & 11/46 &  5/21 & 10/41 & 10/41 &  6/25 &  5/21 & 10/41 & 10/41 & 13/54 &  5/21 & 10/41 & 10/41 &  7/29 &  5/21 & 10/41 & 10/41 & 15/62 &  5/21 & 10/41 & 10/41 &  8/33 & 16/67 & 10/41 & 10/41 & 17/70 & 17/71 & 10/41 & 10/41 &  9/37 &  6/25 & 10/41 & 10/41 & 19/78 & 19/79 & 10/41 & 10/41 & 10/41 & 20/83 & 10/41 & 10/41 & 10/41 &  7/29 &  6/25 & 10/41 & 10/41 & 22/91 \\\hline
$38$ &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 21/86 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$39$ &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 &  1/ 4 &  1/ 4 & 23/93 \\\hline
$40$ & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 &  1/ 4 &  1/ 4 & 23/93 &  1/ 4 \\\hline
$41$ & 11/46 & 11/45 & 11/45 & 11/45 &  6/25 & 11/46 & 11/45 & 11/45 & 13/54 & 11/46 & 11/45 & 11/45 &  7/29 & 11/46 & 11/45 & 11/45 & 15/62 & 11/46 & 11/45 & 11/45 &  8/33 & 11/46 & 11/45 & 11/45 & 17/70 & 17/71 & 11/45 & 11/45 &  9/37 &  6/25 & 11/45 & 11/45 & 19/78 & 19/79 & 11/45 & 11/45 & 10/41 & 20/83 & 11/45 & 11/45 & 21/86 &  7/29 & 11/45 & 11/45 & 11/45 & 22/91 & 11/45 & 11/45 & 11/45 & 23/95 \\\hline
$42$ &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 21/86 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 23/94 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$43$ &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 &  1/ 4 &  1/ 4 & 23/93 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 \\\hline
$44$ & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 &  1/ 4 &  1/ 4 & 23/93 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 &  1/ 4 \\\hline
$45$ &  6/25 & 12/49 & 12/49 & 12/49 & 13/54 &  6/25 & 12/49 & 12/49 &  7/29 &  6/25 & 12/49 & 12/49 & 15/62 &  6/25 & 12/49 & 12/49 &  8/33 &  6/25 & 12/49 & 12/49 & 17/70 &  6/25 & 12/49 & 12/49 &  9/37 &  6/25 & 12/49 & 12/49 & 19/78 & 19/79 & 12/49 & 12/49 & 10/41 & 20/83 & 12/49 & 12/49 & 21/86 &  7/29 & 12/49 & 12/49 & 11/45 & 22/91 & 12/49 & 12/49 & 23/94 & 23/95 & 12/49 & 12/49 & 12/49 &  8/33 \\\hline
$46$ &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 21/86 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 23/94 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$47$ &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 &  1/ 4 &  1/ 4 & 23/93 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 \\\hline
$48$ & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 & 19/77 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 & 21/85 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 &  1/ 4 &  1/ 4 & 23/93 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 &  1/ 4 \\\hline
$49$ & 13/54 & 13/53 & 13/53 & 13/53 &  7/29 & 13/54 & 13/53 & 13/53 & 15/62 & 13/54 & 13/53 & 13/53 &  8/33 & 13/54 & 13/53 & 13/53 & 17/70 & 13/54 & 13/53 & 13/53 &  9/37 & 13/54 & 13/53 & 13/53 & 19/78 & 13/54 & 13/53 & 13/53 & 10/41 & 20/83 & 13/53 & 13/53 & 21/86 &  7/29 & 13/53 & 13/53 & 11/45 & 22/91 & 13/53 & 13/53 & 23/94 & 23/95 & 13/53 & 13/53 & 12/49 &  8/33 & 13/53 & 13/53 & 13/53 & 17/70 \\\hline
$50$ &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 & 15/62 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 17/70 &  1/ 4 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 &  1/ 4 &  1/ 4 & 19/78 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 21/86 &  1/ 4 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  1/ 4 &  1/ 4 & 23/94 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 2, 3, 3+k, 3+k+i\}$.
\end{center}


==> tables/table-g5-a1b2c4.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 5 &  1/ 3 &  1/ 3 &  3/13 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 \\\hline
$2$ &  1/ 4 &  1/ 5 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  4/19 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  8/35 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  9/37 &  1/ 4 & 10/43 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 & 11/45 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 & 14/59 &  1/ 4 &  1/ 4 &  7/29 \\\hline
$3$ &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 \\\hline
$4$ &  3/13 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 \\\hline
$5$ &  3/11 &  3/13 &  3/11 &  3/11 &  1/ 4 &  3/11 &  6/25 &  5/19 &  3/11 &  5/21 &  3/11 &  3/11 &  1/ 4 &  3/11 &  3/11 &  7/27 &  3/11 &  1/ 4 &  4/15 &  3/11 &  1/ 4 &  3/11 &  3/11 &  9/35 &  3/11 &  3/11 &  5/19 &  3/11 & 12/47 & 11/41 &  3/11 & 11/43 &  3/11 &  3/11 &  6/23 &  3/11 &  3/11 & 13/49 &  3/11 & 15/58 &  7/26 &  3/11 &  7/27 &  3/11 &  3/11 &  5/19 &  3/11 &  3/11 &  4/15 &  3/11 \\\hline
$6$ &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 \\\hline
$7$ &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 \\\hline
$8$ &  2/ 7 &  1/ 4 &  2/ 7 &  2/ 7 &  5/19 &  2/ 7 &  8/31 &  3/11 &  2/ 7 &  1/ 4 &  7/25 &  2/ 7 &  7/27 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  5/18 &  2/ 7 &  5/19 & 11/39 &  2/ 7 & 11/41 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 13/47 &  2/ 7 & 16/59 &  7/25 &  2/ 7 &  7/26 & 15/53 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 & 17/61 &  2/ 7 & 20/73 &  9/32 \\\hline
$9$ &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 \\\hline
$10$ &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 \\\hline
$11$ &  5/17 &  5/19 &  5/17 &  5/17 &  3/11 &  5/17 & 10/37 &  7/25 &  5/17 &  6/23 &  2/ 7 &  5/17 &  4/15 &  9/31 &  5/17 &  3/11 &  5/17 &  5/17 &  5/18 &  5/17 &  5/17 & 11/39 &  5/17 &  5/18 &  2/ 7 &  5/17 &  3/11 & 13/45 &  5/17 & 13/47 &  7/24 &  5/17 &  7/25 &  5/17 &  5/17 & 15/53 &  5/17 &  5/17 &  2/ 7 &  5/17 & 20/71 & 17/59 &  5/17 & 17/61 &  9/31 &  5/17 &  9/32 & 19/65 &  5/17 & 19/67 \\\hline
$12$ &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 \\\hline
$13$ &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 \\\hline
$14$ &  3/10 &  3/11 &  3/10 &  3/10 &  7/25 &  3/10 & 12/43 &  2/ 7 &  3/10 &  7/26 &  9/31 &  3/10 &  3/11 &  5/17 &  3/10 &  5/18 & 11/37 &  3/10 & 11/39 &  3/10 &  3/10 &  2/ 7 &  3/10 &  3/10 & 13/45 &  3/10 &  2/ 7 &  7/24 &  3/10 &  7/25 &  5/17 &  3/10 & 15/53 &  8/27 &  3/10 &  2/ 7 & 17/57 &  3/10 & 17/59 &  3/10 &  3/10 &  9/31 &  3/10 &  3/10 & 19/65 &  3/10 & 24/83 &  5/17 &  3/10 &  2/ 7 \\\hline
$15$ &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 \\\hline
$16$ &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 \\\hline
$17$ &  7/23 &  7/25 &  7/23 &  7/23 &  2/ 7 &  7/23 &  2/ 7 &  9/31 &  7/23 &  8/29 &  5/17 &  7/23 & 17/61 & 11/37 &  7/23 & 11/39 &  3/10 &  7/23 &  2/ 7 & 13/43 &  7/23 & 13/45 &  7/23 &  7/23 &  7/24 &  7/23 &  7/23 &  5/17 &  7/23 &  7/24 &  8/27 &  7/23 &  2/ 7 & 17/57 &  7/23 & 17/59 &  3/10 &  7/23 &  9/31 & 19/63 &  7/23 & 19/65 & 10/33 &  7/23 &  5/17 &  7/23 &  7/23 & 21/71 &  7/23 &  7/23 \\\hline
$18$ &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 \\\hline
$19$ &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 \\\hline
$20$ &  4/13 &  2/ 7 &  4/13 &  4/13 &  9/31 &  4/13 & 16/55 &  5/17 &  4/13 &  9/32 & 11/37 &  4/13 & 19/67 &  3/10 &  4/13 &  2/ 7 & 13/43 &  4/13 & 13/45 &  7/23 &  4/13 &  7/24 & 15/49 &  4/13 &  5/17 &  4/13 &  4/13 &  8/27 &  4/13 &  4/13 & 17/57 &  4/13 &  8/27 &  3/10 &  4/13 &  9/31 & 19/63 &  4/13 & 19/65 & 10/33 &  4/13 &  5/17 &  7/23 &  4/13 & 21/71 & 11/36 &  4/13 & 11/37 & 23/75 &  4/13 \\\hline
$21$ &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 \\\hline
$22$ &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 \\\hline
$23$ &  9/29 &  9/31 &  9/29 &  9/29 &  5/17 &  9/29 & 18/61 & 11/37 &  9/29 &  2/ 7 &  3/10 &  9/29 & 21/73 & 13/43 &  9/29 & 11/38 &  7/23 &  9/29 &  7/24 & 15/49 &  9/29 &  5/17 &  4/13 &  9/29 &  8/27 & 17/55 &  9/29 & 17/57 &  9/29 &  9/29 &  3/10 &  9/29 &  9/29 & 19/63 &  9/29 &  3/10 & 10/33 &  9/29 &  5/17 &  7/23 &  9/29 & 21/71 & 11/36 &  9/29 & 11/37 & 23/75 &  9/29 & 23/77 &  4/13 &  9/29 \\\hline
$24$ &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 \\\hline
$25$ &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 \\\hline
$26$ &  5/16 &  5/17 &  5/16 &  5/16 & 11/37 &  5/16 & 20/67 &  3/10 &  5/16 & 11/38 & 13/43 &  5/16 & 23/79 &  7/23 &  5/16 & 12/41 & 15/49 &  5/16 &  5/17 &  4/13 &  5/16 &  8/27 & 17/55 &  5/16 & 17/57 &  9/29 &  5/16 &  3/10 & 19/61 &  5/16 & 19/63 &  5/16 &  5/16 & 10/33 &  5/16 &  5/16 &  7/23 &  5/16 & 10/33 & 11/36 &  5/16 & 11/37 & 23/75 &  5/16 & 23/77 &  4/13 &  5/16 &  3/10 & 25/81 &  5/16 \\\hline
$27$ &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 \\\hline
$28$ & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 \\\hline
$29$ & 11/35 & 11/37 & 11/35 & 11/35 &  3/10 & 11/35 & 22/73 & 13/43 & 11/35 & 12/41 &  7/23 & 11/35 &  5/17 & 15/49 & 11/35 & 13/44 &  4/13 & 11/35 & 27/91 & 17/55 & 11/35 & 17/57 &  9/29 & 11/35 &  3/10 & 19/61 & 11/35 & 19/63 &  5/16 & 11/35 & 10/33 & 21/67 & 11/35 &  7/23 & 11/35 & 11/35 & 11/36 & 11/35 & 11/35 & 23/75 & 11/35 & 11/36 &  4/13 & 11/35 &  3/10 & 25/81 & 11/35 & 25/83 & 13/42 & 11/35 \\\hline
$30$ &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 \\\hline
$31$ &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 \\\hline
$32$ &  6/19 &  3/10 &  6/19 &  6/19 & 13/43 &  6/19 & 24/79 &  7/23 &  6/19 & 13/44 & 15/49 &  6/19 & 27/91 &  4/13 &  6/19 & 14/47 & 17/55 &  6/19 & 29/97 &  9/29 &  6/19 &  3/10 & 19/61 &  6/19 & 19/63 &  5/16 &  6/19 & 10/33 & 21/67 &  6/19 &  7/23 & 11/35 &  6/19 & 11/36 & 23/73 &  6/19 & 23/75 &  6/19 &  6/19 &  4/13 &  6/19 &  6/19 & 25/81 &  6/19 &  4/13 & 13/42 &  6/19 & 13/43 &  9/29 &  6/19 \\\hline
$33$ &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 29/89 \\\hline
$34$ & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 \\\hline
$35$ & 13/41 & 13/43 & 13/41 & 13/41 &  7/23 & 13/41 & 26/85 & 15/49 & 13/41 & 14/47 &  4/13 & 13/41 & 29/97 & 17/55 & 13/41 &  3/10 &  9/29 & 13/41 & 28/93 & 19/61 & 13/41 & 16/53 &  5/16 & 13/41 & 10/33 & 21/67 & 13/41 &  7/23 & 11/35 & 13/41 & 11/36 & 23/73 & 13/41 & 23/75 &  6/19 & 13/41 &  4/13 & 25/79 & 13/41 & 25/81 & 13/41 & 13/41 & 13/42 & 13/41 & 13/41 &  9/29 & 13/41 & 13/42 & 14/45 & 13/41 \\\hline
$36$ &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 29/89 &  1/ 3 &  1/ 3 & 15/46 \\\hline
$37$ &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 \\\hline
$38$ &  7/22 &  7/23 &  7/22 &  7/22 & 15/49 &  7/22 &  4/13 &  4/13 &  7/22 &  3/10 & 17/55 &  7/22 & 28/93 &  9/29 &  7/22 & 16/53 & 19/61 &  7/22 & 23/76 &  5/16 &  7/22 & 17/56 & 21/67 &  7/22 &  7/23 & 11/35 &  7/22 & 11/36 & 23/73 &  7/22 & 23/75 &  6/19 &  7/22 &  4/13 & 25/79 &  7/22 & 25/81 & 13/41 &  7/22 & 13/42 & 27/85 &  7/22 &  9/29 &  7/22 &  7/22 & 14/45 &  7/22 &  4/13 & 29/93 &  7/22 \\\hline
$39$ &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 29/89 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 31/95 \\\hline
$40$ & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 \\\hline
$41$ & 15/47 & 15/49 & 15/47 & 15/47 &  4/13 & 15/47 & 30/97 & 17/55 & 15/47 & 16/53 &  9/29 & 15/47 & 23/76 & 19/61 & 15/47 & 17/56 &  5/16 & 15/47 &  7/23 & 21/67 & 15/47 & 18/59 & 11/35 & 15/47 & 26/85 & 23/73 & 15/47 & 23/75 &  6/19 & 15/47 &  4/13 & 25/79 & 15/47 & 25/81 & 13/41 & 15/47 & 13/42 & 27/85 & 15/47 &  9/29 &  7/22 & 15/47 & 14/45 & 29/91 & 15/47 & 29/93 & 15/47 & 15/47 &  5/16 & 15/47 \\\hline
$42$ &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 29/89 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 31/95 &  1/ 3 &  1/ 3 & 16/49 \\\hline
$43$ &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 \\\hline
$44$ &  8/25 &  4/13 &  8/25 &  8/25 & 17/55 &  8/25 & 23/74 &  9/29 &  8/25 & 17/56 & 19/61 &  8/25 &  7/23 &  5/16 &  8/25 & 18/59 & 21/67 &  8/25 & 26/85 & 11/35 &  8/25 & 19/62 & 23/73 &  8/25 & 27/88 &  6/19 &  8/25 &  4/13 & 25/79 &  8/25 & 25/81 & 13/41 &  8/25 & 13/42 & 27/85 &  8/25 &  9/29 &  7/22 &  8/25 & 14/45 & 29/91 &  8/25 & 29/93 & 15/47 &  8/25 &  5/16 & 31/97 &  8/25 & 31/99 &  8/25 \\\hline
$45$ &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 29/89 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 31/95 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 \\\hline
$46$ & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 \\\hline
$47$ & 17/53 & 17/55 & 17/53 & 17/53 &  9/29 & 17/53 & 29/93 & 19/61 & 17/53 & 18/59 &  5/16 & 17/53 & 26/85 & 21/67 & 17/53 & 19/62 & 11/35 & 17/53 & 27/88 & 23/73 & 17/53 &  4/13 &  6/19 & 17/53 & 29/94 & 25/79 & 17/53 & 21/68 & 13/41 & 17/53 & 13/42 & 27/85 & 17/53 &  9/29 &  7/22 & 17/53 & 14/45 & 29/91 & 17/53 & 29/93 & 15/47 & 17/53 &  5/16 & 31/97 & 17/53 & 31/99 &  8/25 & 17/53 & 16/51 & 25/78 \\\hline
$48$ &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 19/59 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 21/65 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 23/71 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 25/77 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 27/83 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 29/89 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 31/95 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 17/52 \\\hline
$49$ &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 \\\hline
$50$ &  9/28 &  9/29 &  9/28 &  9/28 & 19/61 &  9/28 & 31/99 &  5/16 &  9/28 & 26/85 & 21/67 &  9/28 & 27/88 & 11/35 &  9/28 &  4/13 & 23/73 &  9/28 & 29/94 &  6/19 &  9/28 & 21/68 & 25/79 &  9/28 & 30/97 & 13/41 &  9/28 & 22/71 & 27/85 &  9/28 &  9/29 &  7/22 &  9/28 & 14/45 & 29/91 &  9/28 & 29/93 & 15/47 &  9/28 &  5/16 & 31/97 &  9/28 & 31/99 &  8/25 &  9/28 & 16/51 & 25/78 &  9/28 & 11/35 & 17/53 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 2, 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g5-a1b2c5.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 4 &  2/ 7 &  2/ 7 &  3/11 &  1/ 4 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  2/ 7 &  5/18 &  5/19 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  7/25 &  7/26 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  9/32 &  3/11 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 11/39 & 11/40 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  2/ 7 & 13/46 & 13/47 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 15/53 &  5/18 &  2/ 7 &  2/ 7 & 16/57 \\\hline
$2$ &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  4/17 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  6/23 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 \\\hline
$3$ &  3/10 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 \\\hline
$4$ &  3/11 &  3/10 &  3/10 &  2/ 7 &  4/15 &  3/10 &  5/17 &  5/18 &  3/10 &  3/10 &  2/ 7 &  3/10 &  3/10 &  7/24 &  7/25 &  3/10 &  8/27 &  2/ 7 &  3/10 &  3/10 &  9/31 &  3/10 &  3/10 &  5/17 &  2/ 7 &  3/10 & 11/37 & 11/38 &  3/10 &  3/10 & 12/41 &  3/10 &  3/10 & 13/44 & 13/45 &  3/10 & 14/47 &  7/24 &  3/10 &  3/10 &  5/17 &  3/10 &  3/10 &  8/27 & 16/55 &  3/10 & 17/57 & 17/58 &  3/10 &  3/10 \\\hline
$5$ &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 \\\hline
$6$ &  4/13 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 \\\hline
$7$ &  2/ 7 &  4/13 &  4/13 &  5/17 &  5/18 &  4/13 &  3/10 &  2/ 7 &  4/13 &  7/23 &  7/24 &  4/13 &  4/13 &  8/27 &  4/13 &  4/13 &  3/10 &  9/31 &  4/13 & 10/33 &  5/17 &  4/13 & 11/36 & 11/37 &  4/13 &  4/13 &  3/10 &  4/13 &  4/13 & 13/43 & 13/44 &  4/13 &  7/23 & 14/47 &  4/13 & 15/49 &  3/10 &  4/13 &  4/13 & 16/53 &  4/13 &  4/13 & 17/56 & 17/57 &  4/13 & 18/59 &  3/10 &  4/13 & 19/62 & 19/63 \\\hline
$8$ &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 \\\hline
$9$ &  5/16 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 \\\hline
$10$ &  5/17 &  5/16 &  5/16 &  3/10 &  2/ 7 &  5/16 &  7/23 &  7/24 &  5/16 &  4/13 &  8/27 &  5/16 &  9/29 &  3/10 &  5/16 &  5/16 & 10/33 &  5/16 &  5/16 & 11/36 & 11/37 &  5/16 &  4/13 &  3/10 &  5/16 & 13/42 & 13/43 &  5/16 & 14/45 &  7/23 &  5/16 &  5/16 & 15/49 &  5/16 &  5/16 &  4/13 & 16/53 &  5/16 & 17/55 & 17/56 &  5/16 &  9/29 & 18/59 &  5/16 & 19/61 & 19/62 &  5/16 &  5/16 &  4/13 &  5/16 \\\hline
$11$ &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 \\\hline
$12$ &  6/19 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 \\\hline
$13$ &  3/10 &  6/19 &  6/19 &  7/23 & 12/41 &  6/19 &  4/13 &  8/27 &  6/19 &  9/29 &  3/10 &  6/19 &  5/16 & 10/33 &  6/19 & 11/35 & 11/36 &  6/19 &  6/19 &  4/13 &  6/19 &  6/19 & 13/42 & 13/43 &  6/19 & 14/45 &  7/23 &  6/19 &  5/16 & 15/49 &  6/19 & 16/51 &  4/13 &  6/19 & 17/54 & 17/55 &  6/19 &  6/19 &  9/29 &  6/19 &  6/19 & 19/61 & 19/62 &  6/19 &  5/16 &  4/13 &  6/19 & 21/67 & 21/68 &  6/19 \\\hline
$14$ &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 \\\hline
$15$ &  7/22 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 \\\hline
$16$ &  7/23 &  7/22 &  7/22 &  4/13 & 14/47 &  7/22 &  9/29 &  3/10 &  7/22 &  5/16 & 10/33 &  7/22 & 11/35 & 11/36 &  7/22 &  6/19 &  4/13 &  7/22 & 13/41 & 13/42 &  7/22 &  7/22 & 14/45 &  7/22 &  7/22 &  5/16 & 15/49 &  7/22 & 16/51 &  4/13 &  7/22 & 17/54 & 17/55 &  7/22 &  6/19 &  9/29 &  7/22 & 19/60 & 19/61 &  7/22 & 20/63 &  5/16 &  7/22 &  7/22 & 21/67 &  7/22 &  7/22 & 11/35 & 22/71 &  7/22 \\\hline
$17$ &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 \\\hline
$18$ &  8/25 &  1/ 3 &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 \\\hline
$19$ &  4/13 &  8/25 &  8/25 &  9/29 & 16/53 &  8/25 &  5/16 &  2/ 7 &  8/25 & 11/35 & 11/36 &  8/25 &  6/19 &  4/13 &  8/25 & 13/41 & 13/42 &  8/25 &  7/22 & 14/45 &  8/25 & 15/47 &  5/16 &  8/25 &  8/25 & 16/51 &  8/25 &  8/25 & 17/54 & 17/55 &  8/25 &  6/19 &  9/29 &  8/25 & 19/60 & 19/61 &  8/25 & 20/63 &  5/16 &  8/25 &  7/22 & 21/67 &  8/25 & 22/69 & 11/35 &  8/25 & 23/72 & 23/73 &  8/25 &  8/25 \\\hline
$20$ &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 \\\hline
$21$ &  9/28 &  1/ 3 &  1/ 3 & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 \\\hline
$22$ &  9/29 &  9/28 &  9/28 &  5/16 & 18/59 &  9/28 & 11/35 &  9/31 &  9/28 &  6/19 &  4/13 &  9/28 & 13/41 & 13/42 &  9/28 &  7/22 & 14/45 &  9/28 & 15/47 &  5/16 &  9/28 &  8/25 & 16/51 &  9/28 & 17/53 & 17/54 &  9/28 &  9/28 &  6/19 &  9/28 &  9/28 & 19/60 & 19/61 &  9/28 & 20/63 &  5/16 &  9/28 &  7/22 & 21/67 &  9/28 & 22/69 & 11/35 &  9/28 & 23/72 & 23/73 &  9/28 &  8/25 &  6/19 &  9/28 & 25/78 \\\hline
$23$ &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 \\\hline
$24$ & 10/31 &  1/ 3 &  1/ 3 & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 \\\hline
$25$ &  5/16 & 10/31 & 10/31 & 11/35 &  4/13 & 10/31 &  6/19 &  5/17 & 10/31 & 13/41 & 21/71 & 10/31 &  7/22 & 14/45 & 10/31 & 15/47 &  5/16 & 10/31 &  8/25 & 16/51 & 10/31 & 17/53 & 17/54 & 10/31 &  9/28 &  6/19 & 10/31 & 19/59 & 19/60 & 10/31 & 10/31 & 20/63 & 10/31 & 10/31 &  7/22 & 21/67 & 10/31 & 22/69 & 11/35 & 10/31 & 23/72 & 23/73 & 10/31 &  8/25 &  6/19 & 10/31 & 25/78 & 25/79 & 10/31 & 26/81 \\\hline
$26$ &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 \\\hline
$27$ & 11/34 &  1/ 3 &  1/ 3 & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 \\\hline
$28$ & 11/35 & 11/34 & 11/34 &  6/19 & 22/71 & 11/34 & 13/41 & 11/37 & 11/34 &  7/22 & 24/83 & 11/34 & 15/47 &  5/16 & 11/34 &  8/25 & 16/51 & 11/34 & 17/53 & 17/54 & 11/34 &  9/28 &  6/19 & 11/34 & 19/59 & 19/60 & 11/34 & 10/31 & 20/63 & 11/34 & 21/65 &  7/22 & 11/34 & 11/34 & 22/69 & 11/34 & 11/34 & 23/72 & 23/73 & 11/34 &  8/25 &  6/19 & 11/34 & 25/78 & 25/79 & 11/34 & 26/81 & 13/41 & 11/34 &  9/28 \\\hline
$29$ &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 28/89 \\\hline
$30$ & 12/37 &  1/ 3 &  1/ 3 & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 \\\hline
$31$ &  6/19 & 12/37 & 12/37 & 13/41 & 24/77 & 12/37 &  7/22 &  3/10 & 12/37 & 15/47 & 26/89 & 12/37 &  8/25 & 13/43 & 12/37 & 17/53 & 17/54 & 12/37 &  9/28 &  6/19 & 12/37 & 19/59 & 19/60 & 12/37 & 10/31 & 20/63 & 12/37 & 21/65 &  7/22 & 12/37 & 11/34 & 22/69 & 12/37 & 23/71 & 23/72 & 12/37 & 12/37 &  8/25 & 12/37 & 12/37 & 25/78 & 25/79 & 12/37 & 26/81 & 13/41 & 12/37 &  9/28 & 27/85 & 12/37 & 28/87 \\\hline
$32$ &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 &  6/19 \\\hline
$33$ & 13/40 &  1/ 3 &  1/ 3 & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 &  1/ 3 & 29/88 &  1/ 3 \\\hline
$34$ & 13/41 & 13/40 & 13/40 &  7/22 & 26/83 & 13/40 & 15/47 & 13/43 & 13/40 &  8/25 & 28/95 & 13/40 & 17/53 &  8/27 & 13/40 &  9/28 &  6/19 & 13/40 & 19/59 & 19/60 & 13/40 & 10/31 & 20/63 & 13/40 & 21/65 &  7/22 & 13/40 & 11/34 & 22/69 & 13/40 & 23/71 & 23/72 & 13/40 & 12/37 &  8/25 & 13/40 & 25/77 & 25/78 & 13/40 & 13/40 & 26/81 & 13/40 & 13/40 &  9/28 & 27/85 & 13/40 & 28/87 &  7/22 & 13/40 & 29/90 \\\hline
$35$ &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 13/41 \\\hline
$36$ & 14/43 &  1/ 3 &  1/ 3 & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 &  1/ 3 & 29/88 &  1/ 3 &  1/ 3 & 30/91 &  1/ 3 \\\hline
$37$ &  7/22 & 14/43 & 14/43 & 15/47 & 28/89 & 14/43 &  8/25 &  7/23 & 14/43 & 17/53 & 19/64 & 14/43 &  9/28 & 17/57 & 14/43 & 19/59 & 27/88 & 14/43 & 10/31 & 20/63 & 14/43 & 21/65 &  7/22 & 14/43 & 11/34 & 22/69 & 14/43 & 23/71 & 23/72 & 14/43 & 12/37 &  8/25 & 14/43 & 25/77 & 25/78 & 14/43 & 13/40 & 26/81 & 14/43 & 27/83 &  9/28 & 14/43 & 14/43 & 28/87 &  7/22 & 27/83 & 29/90 & 29/91 & 14/43 & 10/31 \\\hline
$38$ &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 &  7/22 \\\hline
$39$ & 15/46 &  1/ 3 &  1/ 3 & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 &  1/ 3 & 29/88 &  1/ 3 &  1/ 3 & 30/91 &  1/ 3 &  1/ 3 & 31/94 &  1/ 3 \\\hline
$40$ & 15/47 & 15/46 & 15/46 &  8/25 &  6/19 & 15/46 & 17/53 & 15/49 & 15/46 &  9/28 & 29/97 & 15/46 & 19/59 &  3/10 & 15/46 & 10/31 & 19/63 & 15/46 & 21/65 &  7/22 & 15/46 & 11/34 & 22/69 & 15/46 & 23/71 & 23/72 & 15/46 & 12/37 &  8/25 & 15/46 & 25/77 & 25/78 & 15/46 & 13/40 & 26/81 & 15/46 & 27/83 &  9/28 & 15/46 & 14/43 & 28/87 & 15/46 & 29/89 & 29/90 & 15/46 & 15/46 & 10/31 & 15/47 & 29/89 & 31/96 \\\hline
$41$ &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 22/69 \\\hline
$42$ & 16/49 &  1/ 3 &  1/ 3 & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 &  1/ 3 & 29/88 &  1/ 3 &  1/ 3 & 30/91 &  1/ 3 &  1/ 3 & 31/94 &  1/ 3 &  1/ 3 & 32/97 &  1/ 3 \\\hline
$43$ &  8/25 & 16/49 & 16/49 & 17/53 & 19/60 & 16/49 &  9/28 &  4/13 & 16/49 & 19/59 & 28/93 & 16/49 & 10/31 & 19/63 & 16/49 & 21/65 & 10/33 & 16/49 & 11/34 &  9/29 & 16/49 & 23/71 & 23/72 & 16/49 & 12/37 &  8/25 & 16/49 & 25/77 & 25/78 & 16/49 & 13/40 & 26/81 & 16/49 & 27/83 &  9/28 & 16/49 & 14/43 & 28/87 & 16/49 & 29/89 & 29/90 & 16/49 & 15/46 & 10/31 & 16/49 & 31/95 & 31/96 & 16/49 & 16/49 & 32/99 \\\hline
$44$ &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 \\\hline
$45$ & 17/52 &  1/ 3 &  1/ 3 & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 &  1/ 3 & 29/88 &  1/ 3 &  1/ 3 & 30/91 &  1/ 3 &  1/ 3 & 31/94 &  1/ 3 &  1/ 3 & 32/97 &  1/ 3 &  1/ 3 & 32/97 &  1/ 3 \\\hline
$46$ & 17/53 & 17/52 & 17/52 &  9/28 & 27/85 & 17/52 & 19/59 & 17/55 & 17/52 & 10/31 & 23/76 & 17/52 & 21/65 & 27/89 & 17/52 & 11/34 &  7/23 & 17/52 & 23/71 & 11/36 & 17/52 & 12/37 &  8/25 & 17/52 & 25/77 & 25/78 & 17/52 & 13/40 & 26/81 & 17/52 & 27/83 &  9/28 & 17/52 & 14/43 & 28/87 & 17/52 & 29/89 & 29/90 & 17/52 & 15/46 & 10/31 & 17/52 & 31/95 & 31/96 & 17/52 & 16/49 & 32/99 & 17/52 & 17/52 & 11/34 \\\hline
$47$ &  1/ 3 & 17/53 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 \\\hline
$48$ & 18/55 &  1/ 3 &  1/ 3 & 19/58 &  1/ 3 &  1/ 3 & 20/61 &  1/ 3 &  1/ 3 & 21/64 &  1/ 3 &  1/ 3 & 22/67 &  1/ 3 &  1/ 3 & 23/70 &  1/ 3 &  1/ 3 & 24/73 &  1/ 3 &  1/ 3 & 25/76 &  1/ 3 &  1/ 3 & 26/79 &  1/ 3 &  1/ 3 & 27/82 &  1/ 3 &  1/ 3 & 28/85 &  1/ 3 &  1/ 3 & 29/88 &  1/ 3 &  1/ 3 & 30/91 &  1/ 3 &  1/ 3 & 31/94 &  1/ 3 &  1/ 3 & 32/97 &  1/ 3 &  1/ 3 & 32/97 &  1/ 3 &  1/ 3 & 32/97 &  1/ 3 \\\hline
$49$ &  9/28 & 18/55 & 18/55 & 19/59 & 29/91 & 18/55 & 10/31 &  9/29 & 18/55 & 21/65 & 24/79 & 18/55 & 11/34 & 25/82 & 18/55 & 23/71 & 11/36 & 18/55 & 12/37 & 23/75 & 18/55 & 25/77 & 31/99 & 18/55 & 13/40 & 26/81 & 18/55 & 27/83 &  9/28 & 18/55 & 14/43 & 28/87 & 18/55 & 29/89 & 29/90 & 18/55 & 15/46 & 10/31 & 18/55 & 31/95 & 31/96 & 18/55 & 16/49 & 32/99 & 18/55 & 17/52 & 11/34 & 18/55 & 17/52 & 23/71 \\\hline
$50$ &  1/ 3 &  9/28 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 &  1/ 3 & 17/53 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 2, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a1b2c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 2, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a1b3c4.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  2/ 9 &  1/ 4 &  2/ 9 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  4/17 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  6/25 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  8/33 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 & 10/41 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 & 12/49 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 \\\hline
$2$ &  1/ 5 &  2/ 7 &  1/ 4 &  2/ 7 &  2/ 7 &  1/ 4 &  2/ 7 &  4/17 &  2/ 7 &  5/19 &  2/ 7 &  2/ 7 &  6/23 &  2/ 7 &  1/ 4 &  2/ 7 &  7/26 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  8/31 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 \\\hline
$3$ &  1/ 5 &  1/ 4 &  3/14 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  4/19 &  1/ 4 &  5/22 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  2/ 9 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  8/35 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 & 10/43 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  4/17 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 & 14/59 &  1/ 4 \\\hline
$4$ &  1/ 4 &  2/ 7 &  2/ 7 &  1/ 4 &  2/ 7 &  4/17 &  2/ 7 &  5/19 &  2/ 7 &  2/ 7 &  6/23 &  2/ 7 &  1/ 4 &  2/ 7 &  7/26 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  8/31 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 \\\hline
$5$ &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 13/53 &  1/ 4 &  1/ 4 &  1/ 4 & 18/73 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 17/69 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 22/89 &  1/ 4 \\\hline
$6$ &  2/ 7 &  1/ 4 &  2/ 7 &  8/33 &  2/ 7 &  1/ 4 &  2/ 7 &  2/ 7 &  6/23 &  2/ 7 & 12/47 &  2/ 7 &  7/27 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 & 16/61 &  2/ 7 &  9/34 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  4/15 &  2/ 7 & 11/41 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 & 24/89 &  2/ 7 & 13/48 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 25/92 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 \\\hline
$7$ &  4/15 &  2/ 7 &  4/15 &  2/ 7 &  4/15 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  3/11 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  8/29 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 \\\hline
$8$ &  1/ 4 &  4/15 &  1/ 4 &  4/15 &  1/ 4 &  4/15 &  4/15 &  6/23 &  1/ 4 &  6/23 &  1/ 4 &  6/23 &  1/ 4 &  4/15 &  4/15 &  8/31 &  4/15 &  8/31 &  4/15 &  8/31 &  4/15 &  4/15 &  5/19 & 10/39 &  5/19 & 10/39 &  5/19 & 10/39 &  4/15 &  4/15 &  6/23 &  4/15 &  6/23 &  4/15 &  6/23 &  4/15 &  4/15 & 14/53 &  7/27 & 14/53 &  7/27 & 14/53 &  7/27 &  4/15 &  4/15 & 16/61 &  4/15 & 16/61 &  4/15 & 16/61 \\\hline
$9$ &  4/17 &  2/ 7 &  5/19 &  2/ 7 &  2/ 7 &  6/23 &  2/ 7 &  1/ 4 &  2/ 7 &  7/26 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  8/31 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 \\\hline
$10$ &  2/ 9 &  4/15 & 10/41 &  4/15 &  4/15 &  1/ 4 &  1/ 4 &  8/33 &  8/33 &  1/ 4 &  1/ 4 &  4/15 &  4/15 &  1/ 4 &  4/15 &  8/33 &  4/15 & 18/71 &  4/15 &  4/15 & 12/47 & 12/47 &  1/ 4 & 12/49 & 11/43 & 11/43 &  4/15 &  4/15 & 12/47 &  4/15 &  1/ 4 &  4/15 & 17/66 &  4/15 &  4/15 &  8/31 &  8/31 & 14/55 &  1/ 4 & 15/58 & 15/58 &  4/15 &  4/15 &  8/31 &  4/15 & 16/63 &  4/15 & 20/77 &  4/15 &  4/15 \\\hline
$11$ &  5/19 &  2/ 7 &  2/ 7 &  6/23 &  2/ 7 &  1/ 4 &  2/ 7 &  7/26 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  8/31 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 \\\hline
$12$ &  1/ 4 &  4/15 &  4/15 &  5/19 & 10/39 &  5/19 &  9/34 &  7/27 &  5/19 &  4/15 &  4/15 &  6/23 &  4/15 &  9/34 &  4/15 &  5/19 &  4/15 &  4/15 &  9/34 &  7/27 &  9/34 & 13/49 &  5/19 & 20/77 &  4/15 &  4/15 & 16/61 &  4/15 & 13/49 &  4/15 & 11/42 &  4/15 &  4/15 & 13/49 &  5/19 & 13/49 & 17/64 & 14/53 & 25/96 &  4/15 &  4/15 &  5/19 &  4/15 & 17/64 &  4/15 & 26/99 &  4/15 &  4/15 & 17/64 & 16/61 \\\hline
$13$ &  2/ 7 &  6/23 &  2/ 7 & 12/47 &  2/ 7 &  7/27 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 & 16/61 &  2/ 7 &  9/34 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  4/15 &  2/ 7 & 11/41 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 & 24/89 &  2/ 7 & 13/48 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 25/92 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 25/91 &  2/ 7 & 19/69 &  2/ 7 &  2/ 7 \\\hline
$14$ &  3/11 &  2/ 7 &  3/11 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  8/29 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 20/71 \\\hline
$15$ &  6/23 &  3/11 &  6/23 &  3/11 &  6/23 &  3/11 &  3/11 &  4/15 &  7/27 &  4/15 &  8/31 &  4/15 & 15/58 &  3/11 & 10/37 &  5/19 & 10/37 &  5/19 & 10/37 &  5/19 &  3/11 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  3/11 &  7/26 & 14/53 &  7/26 & 14/53 &  7/26 & 14/53 &  3/11 & 16/59 &  4/15 & 16/59 &  4/15 & 16/59 &  4/15 &  3/11 &  3/11 & 18/67 &  3/11 & 18/67 &  3/11 & 18/67 &  3/11 \\\hline
$16$ &  1/ 4 &  2/ 7 &  7/26 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  8/31 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 \\\hline
$17$ &  6/25 &  3/11 & 21/82 &  3/11 &  3/11 &  9/35 &  6/23 &  1/ 4 & 12/47 & 11/42 &  1/ 4 &  3/11 & 14/55 &  6/23 &  7/27 & 12/47 & 16/61 & 11/42 &  3/11 &  3/11 &  6/23 &  3/11 & 12/47 &  3/11 & 24/91 &  3/11 &  3/11 &  5/19 &  9/34 &  7/27 &  9/35 & 17/64 & 13/51 &  3/11 & 20/77 &  9/34 &  5/19 &  8/31 & 17/64 & 17/64 &  3/11 &  3/11 &  9/34 &  3/11 &  6/23 &  3/11 & 17/64 &  3/11 &  3/11 & 21/79 \\\hline
$18$ &  7/26 &  2/ 7 &  2/ 7 &  4/15 &  2/ 7 &  1/ 4 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 \\\hline
$19$ &  7/27 &  3/11 &  3/11 &  7/26 & 14/53 &  7/26 & 13/48 &  9/34 &  7/26 &  3/11 &  7/26 &  4/15 & 17/66 & 13/48 & 11/41 &  7/26 &  3/11 &  3/11 & 18/67 &  3/11 & 13/48 &  3/11 &  7/26 &  3/11 &  3/11 & 13/48 &  4/15 & 13/48 & 19/70 &  7/26 &  4/15 &  3/11 & 10/37 & 11/41 &  7/26 & 19/70 & 17/63 & 15/56 &  3/11 &  3/11 & 17/63 &  3/11 & 19/70 &  3/11 & 25/93 &  3/11 &  3/11 & 19/70 &  7/26 & 19/70 \\\hline
$20$ &  2/ 7 &  4/15 &  2/ 7 & 16/61 &  2/ 7 &  9/34 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  4/15 &  2/ 7 & 11/41 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 & 24/89 &  2/ 7 & 13/48 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 25/92 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 25/91 &  2/ 7 & 19/69 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  8/29 &  2/ 7 & 21/76 &  2/ 7 &  2/ 7 \\\hline
$21$ &  8/29 &  2/ 7 &  8/29 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 &  2/ 7 & 11/39 \\\hline
$22$ &  4/15 &  8/29 &  4/15 &  8/29 &  4/15 &  8/29 &  8/29 & 10/37 &  9/34 & 10/37 &  5/19 & 10/37 & 19/72 &  8/29 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  4/15 &  8/29 & 14/51 &  7/26 & 14/51 &  7/26 & 14/51 &  7/26 &  8/29 &  8/29 & 16/59 &  8/29 & 16/59 &  8/29 & 16/59 &  8/29 &  8/29 &  3/11 & 18/67 &  3/11 & 18/67 &  3/11 & 18/67 &  8/29 & 20/73 & 10/37 & 20/73 & 10/37 & 20/73 & 10/37 &  8/29 \\\hline
$23$ &  8/31 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 \\\hline
$24$ &  1/ 4 &  8/29 & 26/99 &  8/29 &  8/29 & 16/61 &  4/15 & 10/39 & 16/61 & 22/83 & 22/85 &  8/29 &  6/23 &  4/15 & 16/61 & 16/61 & 15/56 &  7/27 &  8/29 &  5/19 &  4/15 &  4/15 & 16/61 & 11/41 & 15/56 &  8/29 &  8/29 &  4/15 &  8/29 & 16/61 &  8/29 & 15/56 &  8/29 &  8/29 &  4/15 & 24/89 &  9/34 & 24/91 & 24/89 & 17/65 &  8/29 & 13/49 & 24/89 &  4/15 & 24/91 & 23/85 &  5/19 &  8/29 &  4/15 & 24/89 \\\hline
$25$ &  3/11 &  2/ 7 &  2/ 7 & 10/37 &  2/ 7 & 10/39 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 &  2/ 7 & 23/82 \\\hline
$26$ &  9/34 &  8/29 &  8/29 &  3/11 & 18/67 &  3/11 & 17/62 & 11/41 &  3/11 &  8/29 &  3/11 & 10/37 & 21/80 & 17/62 & 13/48 &  3/11 &  8/29 &  3/11 & 22/81 &  9/34 & 17/62 &  3/11 &  3/11 &  8/29 &  8/29 &  3/11 &  8/29 & 17/62 &  8/29 &  3/11 &  8/29 &  8/29 & 17/62 & 13/48 & 17/62 & 25/91 &  3/11 & 23/85 &  8/29 & 26/95 & 25/92 &  3/11 & 25/91 &  3/11 & 19/70 &  8/29 & 26/95 &  3/11 &  3/11 & 25/91 \\\hline
$27$ &  2/ 7 & 10/37 &  2/ 7 &  4/15 &  2/ 7 & 11/41 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 & 24/89 &  2/ 7 & 13/48 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 25/92 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 25/91 &  2/ 7 & 19/69 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  8/29 &  2/ 7 & 21/76 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 13/47 &  2/ 7 & 23/83 &  2/ 7 &  2/ 7 \\\hline
$28$ &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 &  2/ 7 & 24/85 \\\hline
$29$ & 10/37 &  5/18 & 10/37 &  5/18 & 10/37 &  5/18 &  5/18 &  3/11 & 11/41 &  3/11 &  4/15 &  3/11 & 23/86 &  5/18 & 14/51 & 24/89 & 14/51 &  7/26 & 14/51 &  7/26 &  5/18 &  8/29 & 16/59 &  8/29 & 16/59 &  8/29 & 16/59 &  5/18 & 18/65 &  3/11 & 18/65 &  3/11 & 18/65 &  3/11 &  5/18 &  5/18 & 20/73 &  5/18 & 20/73 &  5/18 & 20/73 &  5/18 &  5/18 & 11/40 & 22/81 & 11/40 & 22/81 & 11/40 & 22/81 &  5/18 \\\hline
$30$ &  5/19 &  2/ 7 & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  8/29 \\\hline
$31$ & 10/39 &  5/18 &  4/15 &  5/18 &  5/18 &  5/19 & 10/37 &  6/23 &  4/15 &  7/26 &  5/19 &  5/18 & 22/83 & 10/37 &  9/34 &  4/15 & 19/70 & 14/53 &  5/18 &  4/15 & 10/37 & 11/41 &  4/15 & 19/70 &  9/34 &  5/18 & 26/97 & 10/37 & 13/48 &  4/15 & 25/92 & 19/70 &  5/18 &  5/18 & 10/37 &  5/18 &  4/15 &  5/18 & 19/70 &  5/18 &  5/18 & 10/37 &  3/11 & 11/41 & 15/56 &  3/11 & 21/79 &  5/18 & 25/93 &  3/11 \\\hline
$32$ & 11/40 &  2/ 7 &  2/ 7 &  3/11 &  2/ 7 &  6/23 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 14/53 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 10/37 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  8/29 &  2/ 7 & 25/89 \\\hline
$33$ & 11/41 &  5/18 &  5/18 & 11/40 & 22/81 & 11/40 & 21/76 & 13/48 & 11/40 &  5/18 & 11/40 &  3/11 & 25/94 & 21/76 &  3/11 & 11/40 &  5/18 & 11/40 & 26/95 & 23/86 & 21/76 & 17/62 & 11/40 &  5/18 & 11/40 & 14/51 &  7/26 & 21/76 & 27/98 & 11/40 &  5/18 &  5/18 & 19/69 &  5/18 & 21/76 &  5/18 & 11/40 &  5/18 &  5/18 & 21/76 & 26/95 & 21/76 & 18/65 & 11/40 & 26/95 &  5/18 &  8/29 & 17/62 & 11/40 & 18/65 \\\hline
$34$ &  2/ 7 &  3/11 &  2/ 7 & 24/89 &  2/ 7 & 13/48 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 25/92 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 25/91 &  2/ 7 & 19/69 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  8/29 &  2/ 7 & 21/76 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 13/47 &  2/ 7 & 23/83 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 \\\hline
$35$ & 12/43 &  2/ 7 & 12/43 &  2/ 7 & 12/43 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 &  2/ 7 & 24/85 &  2/ 7 & 24/85 &  2/ 7 & 24/85 &  2/ 7 &  2/ 7 & 13/46 \\\hline
$36$ &  3/11 & 12/43 &  3/11 & 12/43 &  3/11 & 12/43 & 12/43 & 14/51 & 13/48 & 14/51 & 11/41 & 14/51 & 17/63 & 12/43 &  8/29 & 25/92 &  8/29 & 16/59 &  8/29 & 16/59 & 12/43 & 18/65 &  3/11 & 18/65 &  3/11 & 18/65 &  3/11 & 12/43 &  5/18 & 20/73 &  5/18 & 20/73 &  5/18 & 20/73 & 12/43 & 22/79 & 11/40 & 22/79 & 11/40 & 11/40 & 11/40 & 12/43 & 12/43 &  8/29 & 12/43 &  8/29 & 12/43 &  8/29 & 12/43 & 12/43 \\\hline
$37$ &  4/15 &  2/ 7 & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  8/29 &  2/ 7 & 25/89 &  2/ 7 &  2/ 7 & 26/93 &  2/ 7 & 13/47 \\\hline
$38$ &  6/23 & 12/43 & 24/89 & 12/43 & 12/43 &  4/15 &  3/11 & 14/53 & 24/89 & 16/59 &  4/15 & 12/43 & 26/97 &  3/11 &  4/15 & 24/89 & 25/92 & 19/71 & 12/43 &  7/26 &  3/11 & 24/89 & 24/89 & 23/84 & 19/71 & 12/43 & 10/37 &  3/11 & 25/92 & 24/89 & 23/84 & 11/41 & 12/43 & 16/59 &  3/11 & 26/95 & 24/89 & 17/62 & 23/84 & 12/43 & 12/43 &  3/11 & 12/43 & 24/89 & 12/43 & 23/84 & 12/43 & 12/43 &  4/15 & 25/91 \\\hline
$39$ & 13/47 &  2/ 7 &  2/ 7 & 14/51 &  2/ 7 & 14/53 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  4/15 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  3/11 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  8/29 &  2/ 7 & 25/89 &  2/ 7 &  2/ 7 & 26/93 &  2/ 7 & 13/47 &  2/ 7 &  9/32 \\\hline
$40$ & 13/48 & 12/43 & 12/43 & 13/47 & 26/95 & 13/47 &  5/18 &  3/11 & 13/47 & 12/43 & 13/47 & 14/51 & 18/67 &  5/18 & 17/62 & 13/47 & 12/43 & 13/47 & 19/69 & 24/89 &  5/18 & 19/69 & 13/47 & 12/43 & 13/47 &  8/29 & 13/48 &  5/18 & 21/76 & 13/47 & 12/43 & 13/47 & 21/76 & 25/92 &  5/18 & 23/83 & 13/47 & 12/43 & 12/43 & 23/83 & 12/43 &  5/18 & 12/43 & 13/47 & 12/43 & 12/43 &  5/18 & 19/69 & 23/83 & 27/97 \\\hline
$41$ &  2/ 7 & 14/51 &  2/ 7 & 25/92 &  2/ 7 &  3/11 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 25/91 &  2/ 7 & 19/69 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  8/29 &  2/ 7 & 21/76 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 13/47 &  2/ 7 & 23/83 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 26/93 &  2/ 7 & 26/95 &  2/ 7 & 27/97 &  2/ 7 &  2/ 7 \\\hline
$42$ &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 &  2/ 7 & 24/85 &  2/ 7 & 24/85 &  2/ 7 & 24/85 &  2/ 7 &  2/ 7 & 13/46 &  2/ 7 & 13/46 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 28/99 \\\hline
$43$ & 14/51 &  7/25 & 14/51 &  7/25 & 14/51 &  7/25 &  7/25 &  8/29 &  3/11 &  8/29 & 13/48 &  8/29 & 25/92 &  7/25 & 18/65 & 26/95 & 18/65 &  3/11 & 18/65 &  3/11 &  7/25 &  5/18 & 17/62 &  5/18 & 20/73 &  5/18 & 20/73 &  7/25 & 22/79 & 11/40 & 22/79 & 11/40 & 22/79 & 11/40 &  7/25 & 12/43 &  8/29 & 12/43 &  8/29 & 12/43 &  8/29 &  7/25 & 26/93 & 13/47 & 26/93 & 13/47 & 27/98 & 27/98 &  7/25 &  7/25 \\\hline
$44$ &  7/26 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 & 16/59 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 &  3/11 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 20/73 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 11/40 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  8/29 &  2/ 7 & 25/89 &  2/ 7 &  2/ 7 & 26/93 &  2/ 7 & 13/47 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 & 23/83 \\\hline
$45$ & 14/53 &  7/25 & 25/92 &  7/25 &  7/25 &  7/26 & 14/51 &  4/15 & 25/92 &  3/11 &  7/26 &  7/25 & 10/37 & 14/51 & 18/67 & 25/92 & 20/73 & 24/89 &  7/25 & 16/59 & 14/51 & 13/48 & 25/92 & 27/98 & 10/37 &  7/25 & 25/92 & 14/51 &  3/11 & 25/92 & 27/98 & 10/37 &  7/25 &  3/11 & 14/51 & 17/62 & 25/92 & 27/98 & 13/48 &  7/25 & 26/95 & 14/51 & 19/69 & 25/92 &  8/29 & 27/98 &  7/25 &  7/25 & 14/51 &  7/25 \\\hline
$46$ &  5/18 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  4/15 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 18/67 &  2/ 7 & 19/68 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 & 10/37 &  2/ 7 &  7/25 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 14/51 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 & 14/51 &  2/ 7 & 25/89 &  2/ 7 &  2/ 7 & 26/93 &  2/ 7 & 13/47 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 & 23/83 &  2/ 7 & 20/71 \\\hline
$47$ &  3/11 &  7/25 &  7/25 &  5/18 & 19/69 &  5/18 & 17/61 & 17/62 &  5/18 &  7/25 &  5/18 &  8/29 & 23/85 & 17/61 & 19/69 &  5/18 &  7/25 &  5/18 & 21/76 & 19/70 & 17/61 & 21/76 &  5/18 &  7/25 &  5/18 & 18/65 & 25/92 & 17/61 & 23/83 &  5/18 &  7/25 &  5/18 & 23/83 & 26/95 & 17/61 &  5/18 &  5/18 &  7/25 &  5/18 &  5/18 & 17/62 & 17/61 & 22/79 &  5/18 &  7/25 &  7/25 &  5/18 &  7/25 & 17/61 &  7/25 \\\hline
$48$ &  2/ 7 &  8/29 &  2/ 7 & 26/95 &  2/ 7 & 17/62 &  2/ 7 &  2/ 7 & 18/65 &  2/ 7 & 25/91 &  2/ 7 & 19/69 &  2/ 7 &  2/ 7 &  5/18 &  2/ 7 &  8/29 &  2/ 7 & 21/76 &  2/ 7 &  2/ 7 & 22/79 &  2/ 7 & 13/47 &  2/ 7 & 23/83 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 &  5/18 &  2/ 7 &  5/18 &  2/ 7 &  2/ 7 & 26/93 &  2/ 7 & 27/97 &  2/ 7 & 27/97 &  2/ 7 &  2/ 7 &  7/25 &  2/ 7 & 14/51 &  2/ 7 & 17/61 &  2/ 7 &  2/ 7 \\\hline
$49$ & 16/57 &  2/ 7 & 16/57 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  9/32 &  2/ 7 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 & 20/71 &  2/ 7 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 & 11/39 &  2/ 7 &  2/ 7 & 24/85 &  2/ 7 & 24/85 &  2/ 7 & 25/89 &  2/ 7 &  2/ 7 & 13/46 &  2/ 7 & 13/46 &  2/ 7 & 13/46 &  2/ 7 &  2/ 7 & 28/99 &  2/ 7 & 28/99 &  2/ 7 & 20/71 &  2/ 7 &  2/ 7 & 15/53 \\\hline
$50$ &  8/29 & 16/57 &  8/29 & 16/57 &  8/29 & 16/57 & 16/57 & 18/65 & 17/62 & 18/65 &  3/11 & 18/65 & 26/95 & 16/57 &  5/18 & 25/91 &  5/18 &  3/11 &  5/18 & 20/73 & 16/57 & 22/79 & 19/69 & 22/79 & 11/40 & 22/79 & 25/91 & 16/57 & 12/43 &  8/29 & 12/43 &  8/29 & 12/43 &  8/29 & 16/57 & 26/93 & 13/47 & 26/93 & 13/47 & 23/83 & 13/47 & 16/57 &  7/25 & 23/83 &  7/25 & 23/83 & 18/65 & 21/76 & 16/57 & 23/82 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 3, 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g5-a1b3c5.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 4 &  3/11 &  1/ 4 &  3/11 &  1/ 4 &  3/11 &  1/ 4 &  3/11 &  1/ 4 &  3/11 &  3/11 &  6/23 &  3/11 &  6/23 &  3/11 &  6/23 &  3/11 &  6/23 &  3/11 &  6/23 &  3/11 &  3/11 &  9/34 &  3/11 &  9/34 &  3/11 &  9/34 &  3/11 &  9/34 &  3/11 &  9/34 &  3/11 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  4/15 &  3/11 &  3/11 & 15/56 &  3/11 & 15/56 &  3/11 & 15/56 &  3/11 \\\hline
$2$ &  4/15 &&  5/17 &&  6/19 &&  1/ 3 &&  8/23 &&  9/25 && 10/27 && 11/29 && 12/31 && 13/33 &&  2/ 5 && 15/37 && 16/39 && 17/41 && 18/43 && 19/45 && 20/47 &&  3/ 7 && 22/51 && 23/53 && 24/55 && 25/57 && 26/59 && 27/61 &&  4/ 9 &\\\hline
$3$ &  1/ 4 &  4/13 &  1/ 4 &  4/13 &  1/ 4 &  4/13 &  1/ 4 &  4/13 &  3/11 &  4/13 &  7/24 &  2/ 7 &  4/13 &  4/15 &  4/13 &  8/29 &  4/13 &  8/29 &  4/13 &  8/29 &  4/13 &  2/ 7 &  4/13 & 11/37 & 12/41 &  4/13 & 12/43 &  4/13 &  2/ 7 &  4/13 &  2/ 7 &  4/13 &  2/ 7 &  4/13 &  7/24 &  4/13 &  3/10 &  8/27 &  4/13 &  2/ 7 &  4/13 & 16/55 &  4/13 & 16/55 &  4/13 & 16/55 &  4/13 & 18/61 &  4/13 & 19/63 \\\hline
$4$ &  5/19 &&  2/ 7 &&  7/23 &&  8/25 &&  1/ 3 && 10/29 && 11/31 &&  4/11 && 13/35 && 14/37 &&  5/13 && 16/41 && 17/43 &&  2/ 5 && 19/47 && 20/49 &&  7/17 && 22/53 && 23/55 &&  8/19 && 25/59 && 26/61 &&  3/ 7 && 28/65 && 29/67 &\\\hline
$5$ &  1/ 4 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 4 &  1/ 3 &  3/11 &  1/ 3 &  7/24 &  1/ 3 &  4/13 &  5/16 &  9/28 &  5/17 &  1/ 3 &  5/18 &  1/ 3 &  3/11 &  1/ 3 &  2/ 7 &  1/ 3 & 11/37 &  1/ 3 &  4/13 &  1/ 3 & 13/41 & 15/47 & 14/43 & 15/49 &  1/ 3 &  5/17 &  1/ 3 &  7/24 &  1/ 3 &  3/10 &  1/ 3 &  4/13 &  1/ 3 & 17/54 &  1/ 3 &  9/28 & 10/31 & 19/58 &  5/16 &  1/ 3 & 10/33 &  1/ 3 & 19/63 &  1/ 3 &  4/13 \\\hline
$6$ &  6/23 &&  7/25 &&  8/27 &&  9/29 && 10/31 &&  1/ 3 && 12/35 && 13/37 && 14/39 && 15/41 && 16/43 && 17/45 && 18/47 && 19/49 && 20/51 && 21/53 &&  2/ 5 && 23/57 && 24/59 && 25/61 && 26/63 && 27/65 && 28/67 && 29/69 && 30/71 &\\\hline
$7$ &  1/ 4 &  6/17 &  1/ 4 &  6/17 &  3/11 &  6/17 &  7/24 &  6/17 &  4/13 &  6/17 &  9/28 &  1/ 3 &  1/ 3 &  6/19 & 11/32 &  3/10 &  6/17 &  2/ 7 &  6/17 & 11/37 &  6/17 &  4/13 &  6/17 & 13/41 &  6/17 & 14/43 &  6/17 &  1/ 3 & 18/53 & 16/47 & 18/55 & 17/49 &  6/19 &  6/17 &  4/13 &  6/17 & 17/54 &  6/17 &  9/28 &  6/17 & 19/58 &  6/17 &  1/ 3 &  6/17 & 21/62 & 12/35 & 11/32 &  1/ 3 & 23/66 & 12/37 \\\hline
$8$ &  7/27 &&  8/29 &&  9/31 && 10/33 && 11/35 && 12/37 &&  1/ 3 && 14/41 && 15/43 && 16/45 && 17/47 && 18/49 && 19/51 && 20/53 && 21/55 && 22/57 && 23/59 && 24/61 && 25/63 &&  2/ 5 && 27/67 && 28/69 && 29/71 && 30/73 && 31/75 &\\\hline
$9$ &  1/ 4 &  7/19 &  3/11 &  7/19 &  7/24 &  7/19 &  4/13 &  7/19 &  9/28 &  7/19 &  1/ 3 &  7/20 & 11/32 &  1/ 3 &  6/17 &  7/22 & 13/36 &  7/23 &  7/19 &  4/13 &  7/19 & 13/41 &  7/19 & 14/43 &  7/19 &  1/ 3 &  7/19 & 16/47 &  7/19 & 17/49 & 21/59 &  6/17 & 21/61 & 19/53 &  1/ 3 &  4/11 & 21/65 &  7/19 & 19/58 &  7/19 &  1/ 3 &  7/19 & 21/62 &  7/19 & 11/32 &  7/19 & 23/66 &  7/19 &  6/17 & 14/39 \\\hline
$10$ &  8/31 &&  3/11 &&  2/ 7 && 11/37 &&  4/13 && 13/41 && 14/43 &&  1/ 3 && 16/47 && 17/49 &&  6/17 && 19/53 &&  4/11 &&  7/19 && 22/59 && 23/61 &&  8/21 &&  5/13 && 26/67 &&  9/23 && 28/71 && 29/73 &&  2/ 5 && 31/77 && 32/79 &\\\hline
$11$ &  3/11 &  8/21 &  7/24 &  8/21 &  4/13 &  8/21 &  9/28 &  8/21 &  1/ 3 &  8/21 & 11/32 &  4/11 &  6/17 &  8/23 & 13/36 &  1/ 3 &  7/19 &  8/25 &  3/ 8 & 13/41 &  8/21 & 14/43 &  8/21 &  1/ 3 &  8/21 & 16/47 &  8/21 & 17/49 &  8/21 &  6/17 &  8/21 & 19/53 & 24/65 &  4/11 & 24/67 &  7/19 &  8/23 & 22/59 & 24/71 & 23/61 & 21/62 &  8/21 & 11/32 &  8/21 & 23/66 &  8/21 &  6/17 &  8/21 &  5/14 &  8/21 \\\hline
$12$ &  6/23 && 10/37 && 11/39 && 12/41 && 13/43 && 14/45 && 15/47 && 16/49 &&  1/ 3 && 18/53 && 19/55 && 20/57 && 21/59 && 22/61 && 23/63 && 24/65 && 25/67 && 26/69 && 27/71 && 28/73 && 29/75 && 30/77 && 31/79 && 32/81 && 33/83 &\\\hline
$13$ & 10/37 &  9/23 &  4/13 &  9/23 &  9/28 &  9/23 &  1/ 3 &  9/23 & 11/32 &  9/23 &  6/17 &  3/ 8 & 13/36 &  9/25 &  7/19 &  9/26 &  3/ 8 &  1/ 3 &  8/21 & 14/43 & 17/44 &  1/ 3 &  9/23 & 16/47 &  9/23 & 17/49 &  9/23 &  6/17 &  9/23 & 19/53 &  9/23 &  4/11 &  9/23 &  7/19 & 27/71 & 22/59 & 27/73 & 23/61 &  9/25 &  8/21 & 27/77 &  5/13 & 23/66 & 26/67 &  6/17 &  9/23 &  5/14 &  9/23 & 13/36 &  9/23 \\\hline
$14$ & 20/77 &&  7/26 && 12/43 && 14/45 && 14/47 && 15/49 && 16/51 && 17/53 && 18/55 &&  1/ 3 && 20/59 && 21/61 && 22/63 && 23/65 && 24/67 && 25/69 && 26/71 && 27/73 && 28/75 && 29/77 && 30/79 && 31/81 && 32/83 && 33/85 && 34/87 &\\\hline
$15$ & 11/41 &  2/ 5 & 13/43 &  2/ 5 &  1/ 3 &  2/ 5 & 11/32 &  2/ 5 &  6/17 &  2/ 5 & 13/36 &  5/13 &  7/19 & 10/27 &  3/ 8 &  5/14 &  8/21 & 10/29 & 17/44 &  1/ 3 &  9/23 & 16/47 & 19/48 & 17/49 &  2/ 5 &  6/17 &  2/ 5 & 19/53 &  2/ 5 &  4/11 &  2/ 5 &  7/19 &  2/ 5 & 22/59 &  2/ 5 & 23/61 & 30/77 &  8/21 & 30/79 &  5/13 & 10/27 & 26/67 & 30/83 &  9/23 &  5/14 & 28/71 & 13/36 & 29/73 & 27/74 &  2/ 5 \\\hline
$16$ & 22/85 &&  8/29 && 13/47 && 15/49 && 16/51 && 16/53 && 17/55 &&  6/19 && 19/59 && 20/61 &&  1/ 3 && 22/65 && 23/67 &&  8/23 && 25/71 && 26/73 &&  9/25 &&  4/11 && 29/79 && 10/27 && 31/83 && 32/85 && 11/29 && 34/89 &&  5/13 &\\\hline
$17$ &  4/15 & 11/27 & 14/47 & 11/27 & 16/49 & 11/27 &  6/17 & 11/27 & 13/36 & 11/27 &  7/19 & 11/28 &  3/ 8 & 11/29 &  8/21 & 11/30 & 17/44 & 11/31 &  9/23 & 11/32 & 19/48 &  1/ 3 &  2/ 5 &  6/17 & 21/52 & 19/53 & 11/27 &  4/11 & 11/27 &  7/19 & 11/27 & 22/59 & 11/27 & 23/61 & 11/27 &  8/21 & 11/27 &  5/13 & 33/83 & 26/67 & 33/85 &  9/23 & 11/29 & 28/71 & 33/89 & 29/73 & 27/74 &  2/ 5 &  7/19 & 31/77 \\\hline
$18$ &  8/31 && 26/95 &&  9/32 && 16/53 && 18/55 &&  6/19 && 13/41 &&  9/28 &&  9/28 && 21/65 && 22/67 &&  1/ 3 && 24/71 && 25/73 && 26/75 && 27/77 && 28/79 && 29/81 && 30/83 && 31/85 && 32/87 && 33/89 && 34/91 && 35/93 && 36/95 &\\\hline
$19$ & 13/49 & 12/29 &  5/17 & 12/29 & 17/53 & 12/29 & 19/55 & 12/29 &  7/19 & 12/29 &  3/ 8 &  2/ 5 &  8/21 & 12/31 & 17/44 &  3/ 8 &  9/23 &  4/11 & 19/48 &  6/17 &  2/ 5 & 12/35 & 21/52 &  1/ 3 & 11/27 & 13/37 & 23/56 &  7/19 & 12/29 & 22/59 & 12/29 & 23/61 & 12/29 &  8/21 & 12/29 &  5/13 & 12/29 & 26/67 & 12/29 &  9/23 & 36/89 & 28/71 & 36/91 & 29/73 & 12/31 &  2/ 5 & 36/95 & 31/77 & 29/78 & 32/79 \\\hline
$20$ &  8/31 &&  3/11 &&  2/ 7 &&  3/10 && 19/59 && 20/61 && 14/43 &&  1/ 3 &&  1/ 3 &&  1/ 3 &&  1/ 3 &&  1/ 3 &&  1/ 3 && 26/77 && 27/79 && 28/81 && 29/83 &&  6/17 && 31/87 && 32/89 && 33/91 && 34/93 &&  7/19 &&  7/19 && 36/97 &\\\hline
$21$ & 14/53 & 13/31 & 16/55 & 13/31 &  6/19 & 13/31 & 20/59 & 13/31 & 22/61 & 13/31 &  8/21 & 13/32 & 17/44 & 13/33 &  9/23 & 13/34 & 19/48 & 13/35 &  2/ 5 & 13/36 & 21/52 & 13/37 & 11/27 & 13/38 & 23/56 &  1/ 3 & 12/29 &  7/20 &  5/12 & 15/41 & 13/31 &  8/21 & 13/31 &  5/13 & 13/31 & 26/67 & 13/31 &  9/23 & 13/31 & 28/71 & 13/31 & 29/73 & 39/95 &  2/ 5 & 39/97 & 31/77 & 13/33 & 32/79 & 22/57 & 11/27 \\\hline
$22$ &  3/11 &&  2/ 7 && 11/37 &&  4/13 && 20/63 && 22/65 &&  1/ 3 && 16/47 && 11/32 && 11/32 && 11/32 && 11/32 && 11/32 &&  1/ 3 && 28/83 && 29/85 && 10/29 && 31/89 && 32/91 && 11/31 && 34/95 && 34/95 && 35/97 &&  4/11 &&  4/11 &\\\hline
$23$ &  9/34 & 14/33 & 17/59 & 14/33 & 19/61 & 14/33 &  1/ 3 & 14/33 & 23/65 & 14/33 & 25/67 &  7/17 &  9/23 &  2/ 5 & 19/48 &  7/18 &  2/ 5 & 14/37 & 21/52 &  7/19 & 11/27 & 14/39 & 23/56 &  7/20 & 12/29 & 14/41 &  5/12 &  1/ 3 & 13/31 & 15/43 & 27/64 &  4/11 & 14/33 & 17/45 & 14/33 &  9/23 & 14/33 & 28/71 & 14/33 & 29/73 & 14/33 &  2/ 5 & 14/33 & 31/77 & 37/89 & 32/79 & 31/76 & 11/27 &  2/ 5 & 34/83 \\\hline
$24$ & 16/59 && 11/37 &&  4/13 && 13/41 && 14/43 &&  1/ 3 && 16/47 && 17/49 &&  6/17 &&  6/17 &&  6/17 &&  6/17 &&  6/17 &&  6/17 &&  1/ 3 && 30/89 && 30/89 && 31/91 && 32/93 && 33/95 &&  4/11 && 35/99 && 35/99 && 31/87 && 35/99 &\\\hline
$25$ & 16/61 &  3/ 7 &  2/ 7 &  3/ 7 &  4/13 &  3/ 7 & 22/67 &  3/ 7 &  8/23 &  3/ 7 & 26/71 &  5/12 & 28/73 & 15/37 &  2/ 5 & 15/38 & 21/52 &  5/13 & 11/27 &  3/ 8 & 23/56 & 15/41 & 12/29 &  5/14 &  5/12 & 15/43 & 13/31 & 15/44 & 27/64 &  1/ 3 & 14/33 &  8/23 & 29/68 & 17/47 &  3/ 7 &  3/ 8 &  3/ 7 & 19/49 &  3/ 7 &  2/ 5 &  3/ 7 & 31/77 &  3/ 7 & 32/79 &  3/ 7 & 11/27 & 37/88 & 34/83 & 26/63 &  7/17 \\\hline
$26$ & 17/63 &&  4/13 && 13/41 && 14/43 &&  1/ 3 && 16/47 && 17/49 &&  6/17 && 19/53 && 13/36 && 13/36 && 13/36 && 13/36 && 13/36 && 32/91 && 30/91 &&  1/ 3 &&  1/ 3 && 32/95 && 26/75 && 26/75 && 29/83 && 29/83 && 29/83 &&  6/17 &\\\hline
$27$ & 17/65 & 16/37 & 19/67 & 16/37 &  7/23 & 16/37 & 23/71 & 16/37 & 25/73 & 16/37 &  9/25 &  8/19 & 29/77 & 16/39 & 31/79 &  2/ 5 & 11/27 & 16/41 & 23/56 &  8/21 & 12/29 & 16/43 &  5/12 &  4/11 & 13/31 & 16/45 & 27/64 &  8/23 & 14/33 & 16/47 & 29/68 & 23/71 &  3/ 7 & 17/49 & 31/72 &  9/25 & 16/37 & 19/51 & 16/37 &  5/13 & 16/37 & 21/53 & 16/37 & 11/27 & 16/37 & 34/83 & 16/37 &  7/17 & 31/73 & 12/29 \\\hline
$28$ & 18/67 &&  7/23 && 14/43 &&  1/ 3 && 16/47 && 17/49 &&  6/17 && 19/53 &&  4/11 &&  7/19 &&  7/19 &&  7/19 &&  7/19 &&  7/19 &&  7/19 && 34/97 && 31/95 && 32/97 &&  1/ 3 && 26/77 && 27/79 && 28/81 && 29/83 &&  6/17 && 31/87 &\\\hline
$29$ &  6/23 & 17/39 &  2/ 7 & 17/39 & 22/73 & 17/39 &  8/25 & 17/39 & 26/77 & 17/39 & 28/79 & 17/40 & 10/27 & 17/41 & 32/83 & 17/42 &  2/ 5 & 17/43 & 12/29 & 17/44 &  5/12 & 17/45 & 13/31 & 17/46 & 27/64 & 17/47 & 14/33 & 17/48 & 29/68 &  1/ 3 &  3/ 7 & 16/49 & 31/72 & 25/77 & 16/37 & 26/77 & 33/76 & 19/53 & 17/39 & 10/27 & 17/39 & 21/55 & 17/39 & 11/28 & 17/39 & 23/57 & 17/39 & 12/29 & 17/39 & 37/89 \\\hline
$30$ & 19/71 && 22/73 &&  1/ 3 && 16/47 && 17/49 &&  6/17 && 19/53 &&  4/11 &&  7/19 && 22/59 &&  3/ 8 &&  3/ 8 &&  3/ 8 &&  3/ 8 &&  3/ 8 && 26/71 && 14/41 &&  1/ 3 && 26/77 && 27/79 && 28/81 && 29/83 &&  1/99 && 31/87 && 32/89 &\\\hline
$31$ & 11/42 & 18/41 &  7/25 & 18/41 & 23/77 & 18/41 & 26/79 & 18/41 &  1/ 3 & 18/41 & 29/83 &  3/ 7 & 31/85 & 18/43 & 11/29 &  9/22 & 35/89 &  2/ 5 & 37/91 &  9/23 & 13/31 & 18/47 & 27/64 &  3/ 8 & 14/33 & 18/49 & 29/68 &  9/25 &  3/ 7 & 17/50 & 31/72 &  8/25 & 16/37 & 13/41 & 33/76 &  1/ 3 & 17/39 & 28/83 &  7/16 & 29/83 & 18/41 & 31/85 & 18/41 & 11/29 & 18/41 & 34/89 & 18/41 &  2/ 5 & 18/43 & 25/61 \\\hline
$32$ &  4/15 && 23/77 && 26/79 && 17/49 &&  6/17 && 19/53 &&  4/11 &&  7/19 && 22/59 && 23/61 &&  8/21 &&  8/21 &&  8/21 &&  8/21 &&  8/21 &&  8/21 && 35/96 && 15/44 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$33$ &  3/11 & 19/43 & 13/46 & 19/43 &  8/27 & 19/43 & 27/83 & 19/43 & 28/85 & 19/43 & 10/29 & 19/44 & 32/89 & 19/45 & 34/91 & 19/46 & 12/31 & 19/47 &  2/ 5 & 19/48 & 40/97 & 19/49 & 14/33 & 19/50 & 29/68 & 19/51 &  3/ 7 &  6/17 & 31/72 &  9/26 & 16/37 & 17/52 & 33/76 & 14/43 & 17/39 & 14/43 &  7/16 &  1/99 & 18/41 & 10/29 & 37/84 & 31/89 & 19/43 & 32/89 & 19/43 & 34/91 & 19/43 & 12/31 & 19/44 & 37/95 \\\hline
$34$ &  4/15 &&  8/27 && 27/83 &&  6/17 && 19/53 &&  4/11 &&  7/19 && 22/59 && 23/61 &&  8/21 &&  5/13 && 17/44 && 17/44 && 17/44 && 17/44 && 17/44 && 14/37 && 16/45 &&  8/23 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$35$ & 22/81 &  4/ 9 &  7/24 &  4/ 9 &  3/10 &  4/ 9 & 28/87 &  4/ 9 & 30/89 &  4/ 9 & 31/91 & 10/23 & 11/31 & 20/47 &  7/19 &  5/12 & 37/97 & 20/49 & 13/33 &  2/ 5 & 28/69 & 20/51 & 38/91 &  5/13 &  3/ 7 & 20/53 & 31/72 & 19/53 & 16/37 & 18/53 & 33/76 &  1/ 3 & 17/39 &  1/ 3 &  7/16 &  1/ 3 & 18/41 &  1/99 & 37/84 &  1/99 & 19/43 &  1/99 & 39/88 &  1/99 &  4/ 9 &  1/99 &  4/ 9 &  7/19 &  4/ 9 & 37/97 \\\hline
$36$ & 22/83 &&  5/17 && 28/87 && 31/89 &&  4/11 &&  7/19 && 22/59 && 23/61 &&  8/21 &&  5/13 && 26/67 &&  9/23 &&  9/23 &&  9/23 &&  9/23 &&  9/23 &&  9/23 && 35/94 && 17/48 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$37$ & 23/85 & 21/47 &  3/10 & 21/47 &  4/13 & 21/47 & 29/91 & 21/47 & 32/93 & 21/47 & 32/95 &  7/16 & 34/97 &  3/ 7 &  4/11 & 21/50 & 35/93 &  7/17 & 33/85 & 21/52 &  2/ 5 & 21/53 & 37/90 &  7/18 & 27/64 & 10/27 & 16/37 &  4/11 & 33/76 & 19/55 & 17/39 & 16/47 &  7/16 & 16/47 & 18/41 &  1/99 & 37/84 &  1/99 & 19/43 &  1/99 & 39/88 &  1/99 &  4/ 9 &  1/99 & 41/92 &  1/99 & 21/47 &  1/99 & 21/47 &  1/99 \\\hline
$38$ & 23/87 && 26/89 && 29/91 && 32/93 &&  7/19 && 22/59 && 23/61 &&  8/21 &&  5/13 && 26/67 &&  9/23 && 28/71 && 19/48 && 19/48 && 19/48 && 19/48 && 19/48 && 37/98 && 18/49 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$39$ & 24/89 & 22/49 &  4/13 & 22/49 & 17/54 & 22/49 &  9/28 & 22/49 & 33/97 & 22/49 & 34/99 & 11/25 & 26/75 & 22/51 & 23/64 & 11/26 & 13/35 & 22/53 & 23/60 & 11/27 & 28/71 &  6/17 & 15/37 & 10/27 & 37/89 & 19/54 & 26/61 &  5/14 & 17/39 & 20/57 &  7/16 & 28/81 & 18/41 & 17/49 & 37/84 &  1/99 & 19/43 &  1/99 & 39/88 &  1/99 &  4/ 9 &  1/99 & 41/92 &  1/99 & 21/47 &  1/99 & 43/96 &  1/99 & 22/49 &  1/99 \\\hline
$40$ & 24/91 &&  9/31 &&  6/19 && 33/97 &&  4/11 && 23/61 &&  8/21 &&  5/13 && 26/67 &&  9/23 && 28/71 && 29/73 &&  2/ 5 &&  2/ 5 &&  2/ 5 &&  2/ 5 &&  2/ 5 &&  2/ 5 && 13/34 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$41$ & 25/93 & 23/51 & 29/95 & 23/51 &  9/28 & 23/51 & 19/58 & 23/51 & 33/98 & 23/51 & 29/83 & 23/52 & 11/32 & 23/53 & 23/66 & 23/54 & 13/36 & 23/55 & 14/37 &  7/18 & 37/95 & 23/57 & 15/38 & 19/54 & 16/39 &  5/14 & 33/80 & 20/57 & 40/93 & 28/81 & 18/41 & 29/83 & 37/84 &  6/17 & 19/43 &  1/99 & 39/88 &  1/99 &  4/ 9 &  1/99 & 41/92 &  1/99 & 21/47 &  1/99 & 43/96 &  1/99 & 22/49 &  1/99 &  9/20 &  1/99 \\\hline
$42$ & 14/53 && 16/55 && 31/99 && 33/98 && 23/64 &&  8/21 &&  5/13 && 26/67 &&  9/23 && 28/71 && 29/73 &&  2/ 5 && 31/77 && 21/52 && 21/52 && 21/52 && 21/52 && 21/52 && 29/75 && 28/87 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$43$ & 26/97 & 24/53 & 10/33 & 24/53 & 19/58 & 24/53 &  1/ 3 & 24/53 & 21/62 & 24/53 & 27/76 &  4/ 9 & 23/66 & 24/55 &  6/17 &  3/ 7 &  5/14 &  8/19 &  7/19 & 12/29 &  5/13 &  4/11 & 31/80 & 26/77 & 32/79 & 27/79 & 17/41 & 28/81 &  5/12 & 29/83 &  3/ 7 &  6/17 & 19/43 &  1/99 & 39/88 &  1/99 &  4/ 9 &  1/99 & 41/92 &  1/99 & 21/47 &  1/99 & 43/96 &  1/99 & 22/49 &  1/99 &  9/20 &  1/99 & 23/51 &  1/99 \\\hline
$44$ &  3/11 && 16/57 && 23/74 &&  1/ 3 && 27/76 && 35/93 && 26/67 &&  9/23 && 28/71 && 29/73 &&  2/ 5 && 31/77 && 32/79 && 11/27 && 11/27 && 11/27 && 11/27 && 11/27 && 11/27 && 30/89 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$45$ & 15/56 &  5/11 & 28/93 &  5/11 &  1/ 3 &  5/11 & 21/62 &  5/11 & 11/32 &  5/11 & 13/37 & 25/56 & 23/65 & 25/57 &  5/14 & 25/58 & 13/36 & 25/59 &  4/11 &  3/ 8 &  3/ 8 &  7/19 & 16/41 & 27/79 & 11/28 & 28/81 & 17/42 & 29/83 & 18/43 &  6/17 & 37/88 &  1/99 & 19/44 &  1/99 &  4/ 9 &  1/99 & 41/92 &  1/99 & 21/47 &  1/99 & 43/96 &  1/99 & 22/49 &  1/99 &  9/20 &  1/99 & 23/51 &  1/99 & 33/73 &  1/99 \\\hline
$46$ & 25/92 && 17/59 && 13/43 && 21/65 && 13/37 && 29/78 &&  9/23 && 28/71 && 29/73 &&  2/ 5 && 31/77 && 32/79 && 11/27 && 34/83 && 23/56 && 23/56 && 23/56 && 23/56 && 23/56 && 32/93 && 32/93 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$47$ &  4/15 & 26/57 & 27/92 & 26/57 & 10/31 & 41/90 & 11/32 & 26/57 & 23/66 & 23/54 &  6/17 & 23/55 & 14/39 & 23/56 & 13/36 & 23/57 & 27/74 & 22/57 &  7/19 &  5/14 & 31/84 & 26/75 &  8/21 & 28/81 & 17/43 & 29/83 & 35/88 &  6/17 &  9/22 & 31/87 & 19/45 &  1/99 & 39/92 &  1/99 & 10/23 &  1/99 & 21/47 &  1/99 & 43/96 &  1/99 & 22/49 &  1/99 &  9/20 &  1/99 & 23/51 &  1/99 & 33/73 &  1/99 & 24/53 &  1/99 \\\hline
$48$ & 16/59 && 18/61 && 19/63 && 29/90 &&  8/23 && 25/68 && 29/75 && 29/73 &&  2/ 5 && 31/77 && 32/79 && 11/27 && 34/83 &&  7/17 && 12/29 && 12/29 && 12/29 && 12/29 && 12/29 && 11/31 && 33/97 &&  1/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
$49$ & 22/85 & 27/59 & 23/79 & 27/59 & 26/81 & 37/81 & 23/66 & 25/56 &  6/17 & 23/55 &  5/14 & 23/56 & 13/36 & 11/28 & 27/74 & 22/57 &  7/19 & 27/73 & 29/78 &  9/25 & 16/43 & 27/77 &  3/ 8 & 29/83 & 17/44 &  6/17 &  2/ 5 & 31/87 & 37/92 & 32/89 & 19/46 &  1/99 & 20/47 &  1/99 & 41/96 &  1/99 &  7/16 &  1/99 & 22/49 &  1/99 &  9/20 &  1/99 & 23/51 &  1/99 & 33/73 &  1/99 & 24/53 &  1/99 & 44/97 &  1/99 \\\hline
$50$ & 10/37 && 19/63 &&  4/13 && 15/47 && 24/71 && 26/73 && 37/98 &&  2/ 5 && 31/77 && 32/79 && 11/27 && 34/83 &&  7/17 && 12/29 && 37/89 && 37/89 &&  5/12 && 27/65 &&  5/12 &&  7/19 && 34/97 && 34/99 &&  1/99 &&  1/99 &&  1/99 &\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 3, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a1b3c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 3, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a1b4c5.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 5 &  2/ 9 &  1/ 5 &  2/ 9 &  4/19 &  2/ 9 &  2/ 9 &  2/ 9 &  2/ 9 &  4/19 &  2/ 9 &  4/19 &  2/ 9 &  3/14 &  2/ 9 &  2/ 9 &  2/ 9 &  2/ 9 &  3/14 &  2/ 9 &  3/14 &  2/ 9 &  8/37 &  2/ 9 &  2/ 9 &  2/ 9 &  2/ 9 &  8/37 &  2/ 9 &  8/37 &  2/ 9 &  5/23 &  2/ 9 &  2/ 9 &  2/ 9 &  2/ 9 &  5/23 &  2/ 9 &  5/23 &  2/ 9 & 12/55 &  2/ 9 &  2/ 9 &  2/ 9 &  2/ 9 & 12/55 &  2/ 9 & 12/55 &  2/ 9 &  7/32 \\\hline
$2$ &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  6/23 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 \\\hline
$3$ &  3/13 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 \\\hline
$4$ &  3/14 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  3/14 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  3/13 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  2/ 9 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  3/13 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  3/13 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  7/30 &  1/ 4 & 15/62 &  1/ 4 \\\hline
$5$ &  1/ 3 &  4/17 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  6/23 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 \\\hline
$6$ &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 \\\hline
$7$ &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 16/65 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$8$ &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  6/23 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 \\\hline
$9$ &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 \\\hline
$10$ &  1/ 4 &  5/19 &  5/19 &  1/ 4 &  5/19 &  5/19 &  1/ 4 &  5/19 &  5/19 &  1/ 4 & 17/69 &  5/19 &  1/ 4 &  1/ 4 &  5/19 &  9/35 &  1/ 4 &  5/19 &  5/19 & 10/39 &  5/19 &  5/19 & 10/39 &  5/19 &  5/19 & 10/39 &  5/19 &  5/19 & 10/39 &  1/ 4 &  5/19 & 23/90 &  1/ 4 &  5/19 &  7/27 & 14/55 &  5/19 &  5/19 & 15/58 &  5/19 &  5/19 & 15/58 &  5/19 &  5/19 & 15/58 &  5/19 &  5/19 & 15/58 & 15/59 &  5/19 \\\hline
$11$ &  1/ 3 &  6/23 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 \\\hline
$12$ &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 \\\hline
$13$ &  6/23 &  3/11 &  3/11 &  6/23 &  3/11 &  3/11 &  6/23 &  3/11 &  3/11 &  6/23 & 10/39 &  3/11 & 15/58 &  8/31 &  3/11 &  5/19 &  8/31 &  3/11 & 11/41 & 11/42 &  3/11 &  3/11 &  4/15 &  3/11 &  3/11 &  4/15 &  3/11 &  3/11 &  4/15 &  3/11 &  3/11 &  4/15 &  6/23 &  3/11 &  9/34 &  7/27 &  3/11 &  4/15 & 16/61 &  3/11 & 17/63 & 17/64 &  3/11 &  3/11 & 18/67 &  3/11 &  3/11 & 18/67 &  3/11 &  3/11 \\\hline
$14$ &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 \\\hline
$15$ &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 \\\hline
$16$ &  7/26 &  7/25 &  7/25 &  7/26 &  7/25 &  7/25 &  7/26 &  7/25 &  7/25 &  7/26 & 23/87 &  7/25 & 17/64 &  9/34 &  7/25 & 18/67 &  9/34 &  7/25 &  3/11 & 19/71 &  7/25 & 13/47 & 13/48 &  7/25 &  7/25 & 14/51 &  7/25 &  7/25 & 14/51 &  7/25 &  7/25 & 14/51 &  7/25 &  7/25 & 14/51 &  7/26 &  7/25 & 25/92 &  4/15 &  7/25 & 26/95 & 25/93 &  7/25 & 19/69 & 19/70 &  7/25 &  5/18 & 20/73 &  7/25 &  7/25 \\\hline
$17$ &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 \\\hline
$18$ &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 \\\hline
$19$ &  8/29 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  8/29 & 16/59 &  2/ 7 & 19/70 & 10/37 &  2/ 7 & 20/73 & 10/37 &  2/ 7 & 13/47 &  3/11 &  2/ 7 &  7/25 & 11/40 &  2/ 7 & 15/53 &  5/18 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  2/ 7 &  5/18 &  3/11 &  2/ 7 & 12/43 & 14/51 &  2/ 7 & 23/82 & 21/76 &  2/ 7 & 11/39 \\\hline
$20$ &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 \\\hline
$21$ &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 \\\hline
$22$ &  9/32 &  9/31 &  9/31 &  9/32 &  9/31 &  9/31 &  9/32 &  9/31 &  9/31 &  9/32 & 18/65 &  9/31 & 21/76 & 11/40 &  9/31 & 22/79 & 11/40 &  9/31 & 23/82 & 23/83 &  9/31 & 15/53 & 12/43 &  9/31 &  2/ 7 & 25/89 &  9/31 & 17/59 & 17/60 &  9/31 &  9/31 &  2/ 7 &  9/31 &  9/31 &  2/ 7 &  9/31 &  9/31 &  2/ 7 &  9/31 &  9/31 &  2/ 7 &  9/32 &  9/31 & 13/46 &  5/18 &  9/31 & 21/74 & 19/68 &  9/31 & 27/95 \\\hline
$23$ &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 \\\hline
$24$ &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 \\\hline
$25$ &  2/ 7 &  5/17 &  5/17 &  2/ 7 &  5/17 &  5/17 &  2/ 7 &  5/17 &  5/17 &  2/ 7 & 20/71 &  5/17 & 23/82 & 12/43 &  5/17 & 24/85 & 12/43 &  5/17 & 25/88 & 25/89 &  5/17 &  2/ 7 & 13/46 &  5/17 & 17/59 & 27/95 &  5/17 &  9/31 &  2/ 7 &  5/17 & 19/65 & 19/66 &  5/17 &  5/17 & 20/69 &  5/17 &  5/17 & 20/69 &  5/17 &  5/17 & 20/69 &  5/17 &  5/17 & 20/69 &  2/ 7 &  5/17 & 27/94 & 11/39 &  5/17 & 23/80 \\\hline
$26$ &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 \\\hline
$27$ & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 \\\hline
$28$ & 11/38 & 11/37 & 11/37 & 11/38 & 11/37 & 11/37 & 11/38 & 11/37 & 11/37 & 11/38 &  2/ 7 & 11/37 & 25/88 & 13/46 & 11/37 &  2/ 7 & 13/46 & 11/37 & 27/94 & 27/95 & 11/37 & 28/97 &  2/ 7 & 11/37 &  9/31 & 27/94 & 11/37 & 19/65 & 15/52 & 11/37 &  5/17 & 20/69 & 11/37 & 21/71 &  7/24 & 11/37 & 11/37 & 22/75 & 11/37 & 11/37 & 22/75 & 11/37 & 11/37 & 22/75 & 11/37 & 11/37 & 22/75 & 11/38 & 11/37 &  9/31 \\\hline
$29$ &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 \\\hline
$30$ &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 \\\hline
$31$ & 12/41 &  3/10 &  3/10 & 12/41 &  3/10 &  3/10 & 12/41 &  3/10 &  3/10 & 12/41 & 24/83 &  3/10 & 27/94 &  2/ 7 &  3/10 & 28/97 &  2/ 7 &  3/10 & 20/69 & 27/94 &  3/10 & 23/79 & 15/52 &  3/10 & 19/65 & 20/69 &  3/10 &  5/17 & 16/55 &  3/10 & 21/71 & 26/89 &  3/10 & 11/37 & 22/75 &  3/10 & 23/77 & 23/78 &  3/10 &  3/10 &  8/27 &  3/10 &  3/10 &  8/27 &  3/10 &  3/10 & 18/61 &  3/10 &  3/10 &  8/27 \\\hline
$32$ &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 \\\hline
$33$ & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 \\\hline
$34$ & 13/44 & 13/43 & 13/43 & 13/44 & 13/43 & 13/43 & 13/44 & 13/43 & 13/43 & 13/44 & 26/89 & 13/43 & 20/69 & 15/52 & 13/43 & 23/79 & 15/52 & 13/43 & 19/65 & 20/69 & 13/43 & 27/92 & 16/55 & 13/43 & 28/95 & 26/89 & 13/43 & 21/71 & 17/58 & 13/43 & 11/37 &  5/17 & 13/43 & 23/77 & 18/61 & 13/43 &  3/10 &  8/27 & 13/43 & 25/83 & 25/84 & 13/43 & 13/43 & 26/87 & 13/43 & 13/43 & 26/87 & 13/43 & 13/43 & 25/84 \\\hline
$35$ &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 \\\hline
$36$ &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 \\\hline
$37$ & 14/47 &  7/23 &  7/23 & 14/47 &  7/23 &  7/23 & 14/47 &  7/23 &  7/23 & 14/47 & 28/95 &  7/23 & 19/65 & 16/55 &  7/23 & 27/92 & 16/55 &  7/23 & 28/95 & 26/89 &  7/23 & 21/71 & 17/58 &  7/23 & 27/91 &  5/17 &  7/23 & 25/84 & 18/61 &  7/23 & 23/77 & 29/98 &  7/23 &  3/10 & 19/64 &  7/23 & 25/83 & 25/84 &  7/23 & 13/43 & 26/87 &  7/23 & 27/89 &  3/10 &  7/23 &  7/23 & 28/93 &  7/23 &  7/23 & 28/93 \\\hline
$38$ &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 \\\hline
$39$ & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 \\\hline
$40$ &  3/10 & 15/49 & 15/49 &  3/10 & 15/49 & 15/49 &  3/10 & 15/49 & 15/49 &  3/10 & 19/64 & 15/49 & 28/95 & 17/58 & 15/49 & 21/71 & 17/58 & 15/49 & 27/91 &  5/17 & 15/49 & 25/84 & 18/61 & 15/49 & 20/67 & 29/98 & 15/49 & 29/97 & 19/64 & 15/49 &  3/10 & 25/84 & 15/49 & 25/83 & 20/67 & 15/49 & 13/43 & 29/97 & 15/49 & 27/89 &  3/10 & 15/49 &  7/23 & 28/93 & 15/49 & 29/95 & 29/96 & 15/49 & 15/49 & 10/33 \\\hline
$41$ &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 \\\hline
$42$ &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 \\\hline
$43$ & 16/53 &  4/13 &  4/13 & 16/53 &  4/13 &  4/13 & 16/53 &  4/13 &  4/13 & 16/53 & 29/97 &  4/13 & 27/91 & 18/61 &  4/13 & 25/84 & 18/61 &  4/13 & 20/67 & 29/98 &  4/13 & 29/97 & 19/64 &  4/13 &  3/10 & 25/84 &  4/13 & 28/93 & 20/67 &  4/13 & 22/73 & 29/97 &  4/13 & 13/43 &  3/10 &  4/13 & 27/89 &  3/10 &  4/13 &  7/23 & 28/93 &  4/13 & 29/95 & 29/96 &  4/13 & 15/49 & 10/33 &  4/13 & 27/88 & 24/79 \\\hline
$44$ &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 &  1/ 3 &  1/ 3 & 20/63 \\\hline
$45$ & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 \\\hline
$46$ & 17/56 & 17/55 & 17/55 & 17/56 & 17/55 & 17/55 & 17/56 & 17/55 & 17/55 & 17/56 & 28/93 & 17/55 & 20/67 & 18/61 & 17/55 & 29/97 & 19/64 & 17/55 &  3/10 & 25/84 & 17/55 & 28/93 & 20/67 & 17/55 & 22/73 & 29/97 & 17/55 & 29/96 &  3/10 & 17/55 & 23/76 & 28/93 & 17/55 & 27/89 & 22/73 & 17/55 &  7/23 & 28/93 & 17/55 & 29/95 & 29/96 & 17/55 & 15/49 & 10/33 & 17/55 & 27/88 & 24/79 & 17/55 &  4/13 & 25/82 \\\hline
$47$ &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 &  1/ 3 &  1/ 3 & 20/63 &  1/ 3 &  1/ 3 & 27/85 \\\hline
$48$ &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 \\\hline
$49$ & 18/59 &  9/29 &  9/29 & 18/59 &  9/29 &  9/29 &  7/23 &  9/29 &  9/29 & 18/59 & 17/58 &  9/29 &  3/10 & 29/98 &  9/29 & 28/93 & 25/84 &  9/29 &  3/10 & 29/97 &  9/29 & 29/96 &  3/10 &  9/29 & 23/76 & 28/93 &  9/29 & 27/89 &  3/10 &  9/29 & 27/89 & 29/96 &  9/29 & 25/82 & 23/76 &  9/29 & 29/95 & 27/89 &  9/29 & 15/49 & 10/33 &  9/29 & 27/88 & 24/79 &  9/29 &  4/13 & 25/82 &  9/29 & 29/94 & 11/36 \\\hline
$50$ &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 &  1/ 3 &  1/ 3 & 20/63 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 4, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a1b4c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 4, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a1b5c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 1, 5, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a2b3c4.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 4 &  2/ 9 &  3/13 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  1/ 4 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  6/23 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 \\\hline
$2$ &  2/ 9 &  1/ 5 &  1/ 5 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  2/ 9 &  5/23 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  3/13 &  7/31 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  4/17 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  5/21 & 11/47 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  6/25 & 13/55 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  7/29 \\\hline
$3$ &  3/11 &  3/11 &  4/17 &  2/ 9 &  1/ 4 &  3/11 &  3/11 &  3/11 &  1/ 4 &  1/ 4 &  3/11 &  3/11 &  3/11 &  1/ 4 &  1/ 4 &  7/27 &  3/11 &  3/11 &  3/11 &  8/31 &  8/31 &  3/11 &  3/11 &  3/11 & 10/39 &  8/31 &  5/19 &  3/11 &  3/11 &  3/11 & 11/42 & 11/42 &  3/11 &  3/11 &  3/11 & 13/50 & 11/42 & 13/49 &  3/11 &  3/11 &  3/11 & 14/53 & 14/53 &  3/11 &  3/11 &  3/11 & 16/61 & 14/53 &  4/15 &  3/11 \\\hline
$4$ &  1/ 3 &  1/ 3 &  5/19 &  1/ 4 &  5/17 &  1/ 3 &  1/ 3 &  1/ 3 &  7/25 &  3/11 &  7/23 &  1/ 3 &  1/ 3 &  1/ 3 &  9/31 &  2/ 7 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 & 11/37 &  5/17 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 13/43 &  3/10 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 15/49 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 17/55 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 19/61 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$5$ &  1/ 3 &  4/13 &  2/ 7 &  5/17 &  1/ 3 &  1/ 3 &  1/ 3 &  6/19 &  3/10 &  7/23 &  1/ 3 &  1/ 3 &  1/ 3 &  8/25 &  4/13 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 & 10/31 &  5/16 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 \\\hline
$6$ &  4/13 &  2/ 7 &  4/15 &  1/ 3 &  1/ 3 &  1/ 3 &  6/19 &  3/10 &  2/ 7 &  1/ 3 &  1/ 3 &  1/ 3 &  8/25 &  4/13 &  8/27 &  1/ 3 &  1/ 3 &  1/ 3 & 10/31 &  5/16 & 10/33 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 14/45 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 16/51 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 \\\hline
$7$ &  2/ 7 &  4/15 &  1/ 4 &  4/13 &  4/13 &  4/13 &  3/10 &  2/ 7 &  3/11 &  9/32 &  4/13 &  4/13 &  4/13 &  8/27 &  2/ 7 &  8/29 &  4/13 &  4/13 &  4/13 & 10/33 &  5/17 &  2/ 7 & 13/45 &  4/13 &  4/13 &  4/13 &  3/10 & 12/41 &  2/ 7 &  4/13 &  4/13 &  4/13 &  7/23 & 14/47 &  7/24 & 17/58 &  4/13 &  4/13 &  4/13 & 16/53 &  8/27 & 16/55 &  4/13 &  4/13 &  4/13 & 18/59 &  3/10 & 18/61 & 21/71 &  4/13 \\\hline
$8$ &  4/15 &  1/ 4 &  4/17 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  6/23 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  8/31 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 &  5/19 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  4/15 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 \\\hline
$9$ &  5/17 &  5/17 &  1/ 4 &  4/15 &  3/11 &  5/17 &  5/17 &  5/17 &  7/26 &  7/26 &  2/ 7 &  5/17 &  5/17 & 11/40 &  9/32 &  9/32 &  5/17 &  5/17 &  5/17 & 10/37 &  9/32 & 11/39 &  5/17 &  5/17 &  5/17 & 12/43 & 12/43 & 13/45 &  5/17 &  5/17 & 16/57 &  2/ 7 &  2/ 7 &  5/17 &  5/17 &  5/17 &  5/18 &  2/ 7 &  2/ 7 &  5/17 &  5/17 &  5/17 & 17/60 & 17/60 &  9/31 &  5/17 &  5/17 & 21/74 & 19/66 & 19/66 \\\hline
$10$ &  1/ 3 &  1/ 3 &  8/31 &  3/11 &  7/23 &  1/ 3 &  1/ 3 &  1/ 3 & 10/37 &  2/ 7 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 & 12/43 &  5/17 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 &  2/ 7 &  3/10 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 16/55 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 18/61 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 20/67 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 19/63 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$11$ &  1/ 3 &  6/19 &  3/11 &  7/23 &  1/ 3 &  1/ 3 &  1/ 3 &  8/25 &  4/13 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 & 10/31 &  5/16 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 \\\hline
$12$ &  6/19 &  3/10 &  2/ 7 &  1/ 3 &  1/ 3 &  1/ 3 &  8/25 &  4/13 &  8/27 &  1/ 3 &  1/ 3 &  1/ 3 & 10/31 &  5/16 & 10/33 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 14/45 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 16/51 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 20/63 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 \\\hline
$13$ &  3/10 &  2/ 7 &  3/11 &  6/19 &  6/19 &  6/19 &  4/13 &  8/27 &  2/ 7 & 13/44 &  6/19 &  6/19 &  5/16 & 10/33 &  5/17 &  2/ 7 &  6/19 &  6/19 &  6/19 &  4/13 &  3/10 & 12/41 &  6/19 &  6/19 &  6/19 & 14/45 &  7/23 & 14/47 & 19/63 &  6/19 &  6/19 & 16/51 &  4/13 & 16/53 &  8/27 &  6/19 &  6/19 &  6/19 &  9/29 & 18/59 &  3/10 &  6/19 &  6/19 &  6/19 &  5/16 &  4/13 & 10/33 & 25/82 &  6/19 &  6/19 \\\hline
$14$ &  2/ 7 &  3/11 &  6/23 &  3/10 &  3/10 &  3/10 &  8/27 &  2/ 7 &  8/29 &  7/26 &  3/10 &  3/10 &  3/10 &  5/17 &  2/ 7 &  5/18 & 15/53 &  3/10 &  3/10 &  3/10 & 12/41 &  2/ 7 & 12/43 &  3/10 &  3/10 &  3/10 & 14/47 &  7/24 &  2/ 7 &  7/25 &  3/10 &  3/10 &  3/10 &  8/27 & 16/55 &  2/ 7 & 21/73 &  3/10 &  3/10 &  3/10 & 18/61 &  9/31 &  2/ 7 &  3/10 &  3/10 &  3/10 & 20/67 &  5/17 & 20/69 &  2/ 7 \\\hline
$15$ &  7/23 &  7/23 &  1/ 4 &  2/ 7 &  2/ 7 &  7/23 &  7/23 &  7/23 &  9/32 &  9/32 &  5/17 &  7/23 &  7/23 & 15/52 & 11/38 & 11/38 &  3/10 &  7/23 &  7/23 &  2/ 7 & 13/44 & 13/44 &  7/23 &  7/23 &  7/23 &  2/ 7 & 13/44 & 13/44 &  7/23 &  7/23 &  7/23 & 16/55 & 16/55 & 17/57 &  7/23 &  7/23 & 22/75 & 18/61 & 18/61 & 19/63 &  7/23 &  7/23 & 19/65 & 20/67 & 20/67 &  7/23 &  7/23 &  7/23 & 19/65 & 20/67 \\\hline
$16$ &  1/ 3 &  1/ 3 &  7/27 &  2/ 7 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 &  3/11 &  5/17 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 11/39 &  3/10 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 13/45 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 &  5/17 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 17/57 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 19/63 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$17$ &  1/ 3 &  8/25 &  4/15 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 & 10/31 &  5/17 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 \\\hline
$18$ &  8/25 &  4/13 & 13/47 &  1/ 3 &  1/ 3 &  1/ 3 & 10/31 &  5/16 & 10/33 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 14/45 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 16/51 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 20/63 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 22/69 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 \\\hline
$19$ &  4/13 &  8/27 &  2/ 7 &  8/25 &  8/25 &  8/25 &  5/16 & 10/33 &  5/17 & 17/56 &  8/25 &  8/25 &  6/19 &  4/13 &  3/10 & 12/41 &  8/25 &  8/25 &  7/22 & 14/45 &  7/23 & 14/47 &  8/25 &  8/25 &  8/25 & 16/51 &  4/13 & 16/53 &  8/25 &  8/25 &  8/25 &  6/19 &  9/29 & 18/59 & 25/81 &  8/25 &  8/25 & 20/63 &  5/16 &  4/13 & 10/33 &  8/25 &  8/25 & 22/69 & 11/35 & 22/71 & 11/36 &  8/25 &  8/25 &  8/25 \\\hline
$20$ &  8/27 &  2/ 7 &  8/29 &  4/13 &  4/13 &  4/13 & 10/33 &  5/17 &  2/ 7 &  9/32 &  4/13 &  4/13 &  4/13 &  3/10 & 12/41 &  2/ 7 &  4/13 &  4/13 &  4/13 &  7/23 & 14/47 &  7/24 &  2/ 7 &  4/13 &  4/13 &  4/13 & 16/53 &  8/27 & 16/55 &  4/13 &  4/13 &  4/13 & 18/59 &  3/10 & 18/61 &  9/31 &  4/13 &  4/13 &  4/13 & 10/33 & 20/67 &  5/17 &  4/13 &  4/13 &  4/13 & 11/36 & 22/73 & 11/37 & 22/75 &  4/13 \\\hline
$21$ &  9/29 &  9/29 &  4/15 &  8/27 &  8/27 &  9/29 &  9/29 &  9/29 &  5/18 & 19/66 &  3/10 &  9/29 &  9/29 & 19/64 & 13/44 & 13/44 &  7/23 &  9/29 &  9/29 &  8/27 &  3/10 &  3/10 &  4/13 &  9/29 &  9/29 &  8/27 & 17/56 & 17/56 &  9/29 &  9/29 &  9/29 &  8/27 & 17/56 & 17/56 &  9/29 &  9/29 &  9/29 & 20/67 & 20/67 &  7/23 &  9/29 &  9/29 & 28/93 & 22/73 & 22/73 & 23/75 &  9/29 &  9/29 & 23/77 & 24/79 \\\hline
$22$ &  1/ 3 &  1/ 3 &  3/11 &  5/17 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 11/39 &  3/10 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 13/45 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 &  5/17 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 17/57 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 19/63 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 23/75 &  6/19 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$23$ &  1/ 3 & 10/31 &  5/19 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  2/ 7 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 \\\hline
$24$ & 10/31 &  5/16 & 16/59 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 14/45 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 16/51 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 20/63 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 22/69 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 &  8/25 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 \\\hline
$25$ &  5/16 & 10/33 & 17/61 & 10/31 & 10/31 & 10/31 &  6/19 &  4/13 &  3/10 & 21/68 & 10/31 & 10/31 &  7/22 & 14/45 &  7/23 & 14/47 & 10/31 & 10/31 &  8/25 & 16/51 &  4/13 & 16/53 & 10/31 & 10/31 &  9/28 &  6/19 &  9/29 & 18/59 & 10/31 & 10/31 & 10/31 & 20/63 &  5/16 &  4/13 & 10/31 & 10/31 & 10/31 & 22/69 & 11/35 & 22/71 & 31/99 & 10/31 & 10/31 &  8/25 &  6/19 & 24/77 &  4/13 & 10/31 & 10/31 & 26/81 \\\hline
$26$ & 10/33 &  5/17 &  2/ 7 &  5/16 &  5/16 &  5/16 &  4/13 &  3/10 & 12/41 & 11/38 &  5/16 &  5/16 & 14/45 &  7/23 & 14/47 & 12/41 &  5/16 &  5/16 &  5/16 &  4/13 & 16/53 &  8/27 & 25/83 &  5/16 &  5/16 &  9/29 & 18/59 &  3/10 & 18/61 &  5/16 &  5/16 &  5/16 &  4/13 & 10/33 & 20/67 &  5/16 &  5/16 &  5/16 & 22/71 & 11/36 & 22/73 & 11/37 &  5/16 &  5/16 & 24/77 &  4/13 & 24/79 &  3/10 &  5/16 &  5/16 \\\hline
$27$ & 11/35 & 11/35 &  5/18 & 10/33 & 10/33 & 11/35 & 11/35 & 11/35 &  2/ 7 & 23/78 &  7/23 & 11/35 & 11/35 & 23/76 &  7/24 & 25/84 &  4/13 & 11/35 & 11/35 & 16/53 & 17/56 & 17/56 &  9/29 & 11/35 & 11/35 & 10/33 & 19/62 & 19/62 &  5/16 & 11/35 & 11/35 & 10/33 & 21/68 & 21/68 & 11/35 & 11/35 & 11/35 & 10/33 & 21/68 & 21/68 & 11/35 & 11/35 & 11/35 & 24/79 & 24/79 & 25/81 & 11/35 & 11/35 & 19/62 & 26/85 \\\hline
$28$ &  1/ 3 &  1/ 3 & 10/37 &  3/10 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 13/45 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 &  5/17 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 17/57 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 19/63 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 23/75 &  6/19 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 25/81 & 13/41 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$29$ &  1/ 3 & 12/37 &  5/19 & 13/41 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/25 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/27 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 \\\hline
$30$ & 12/37 &  6/19 & 19/71 &  1/ 3 &  1/ 3 &  1/ 3 & 14/43 &  7/22 & 23/77 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 16/51 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 20/63 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 22/69 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 &  8/25 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 & 26/81 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/43 \\\hline
$31$ &  6/19 &  4/13 & 20/73 & 12/37 & 12/37 & 12/37 &  7/22 & 14/45 &  7/23 &  5/16 & 12/37 & 12/37 &  8/25 & 16/51 &  4/13 & 13/43 & 12/37 & 12/37 &  9/28 &  6/19 &  9/29 & 18/59 & 12/37 & 12/37 & 10/31 & 20/63 &  5/16 &  4/13 & 12/37 & 12/37 & 11/34 & 22/69 & 11/35 & 22/71 & 12/37 & 12/37 & 12/37 &  8/25 &  6/19 & 24/77 & 12/37 & 12/37 & 12/37 & 26/81 & 13/41 & 26/83 & 31/98 & 12/37 & 12/37 & 28/87 \\\hline
$32$ &  4/13 &  3/10 &  7/25 &  6/19 &  6/19 &  6/19 & 14/45 &  7/23 & 14/47 & 13/44 &  6/19 &  6/19 & 16/51 &  4/13 & 16/53 & 14/47 &  6/19 &  6/19 &  6/19 &  9/29 & 18/59 &  3/10 &  6/19 &  6/19 &  6/19 &  5/16 &  4/13 & 10/33 &  3/10 &  6/19 &  6/19 & 11/35 & 22/71 & 11/36 & 22/73 &  6/19 &  6/19 &  6/19 & 24/77 &  4/13 & 24/79 &  6/19 &  6/19 &  6/19 & 26/83 & 13/42 & 26/85 & 13/43 &  6/19 &  6/19 \\\hline
$33$ & 13/41 & 13/41 &  2/ 7 &  4/13 &  4/13 & 13/41 & 13/41 & 13/41 &  7/24 &  3/10 &  4/13 & 13/41 & 13/41 & 27/88 &  8/27 & 29/96 &  9/29 & 13/41 & 13/41 & 18/59 &  3/10 & 24/79 &  5/16 & 13/41 & 13/41 &  4/13 & 21/68 & 21/68 & 11/35 & 13/41 & 13/41 &  4/13 & 23/74 & 23/74 &  6/19 & 13/41 & 13/41 &  4/13 &  5/16 &  5/16 & 13/41 & 13/41 & 13/41 &  4/13 & 23/74 &  5/16 & 13/41 & 13/41 & 13/41 &  4/13 \\\hline
$34$ &  1/ 3 &  1/ 3 & 12/43 &  7/23 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 &  5/17 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 17/57 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 19/63 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 23/75 &  6/19 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 25/81 & 13/41 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 &  9/29 &  7/22 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$35$ &  1/ 3 & 14/43 &  3/11 & 15/47 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 & 25/87 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 & 29/99 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/33 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/43 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 & 30/91 \\\hline
$36$ & 14/43 &  7/22 &  4/15 &  1/ 3 &  1/ 3 &  1/ 3 & 16/49 &  8/25 & 26/89 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 20/63 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 22/69 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 &  8/25 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 & 26/81 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/43 & 28/87 &  1/ 3 &  1/ 3 &  1/ 3 & 30/91 & 15/46 \\\hline
$37$ &  7/22 & 14/45 & 23/85 & 14/43 & 14/43 & 14/43 &  8/25 & 16/51 &  4/13 & 29/92 & 14/43 & 14/43 &  9/28 &  6/19 &  9/29 & 15/49 & 14/43 & 14/43 & 10/31 & 20/63 &  5/16 &  4/13 & 14/43 & 14/43 & 11/34 & 22/69 & 11/35 & 22/71 & 14/43 & 14/43 & 12/37 &  8/25 &  6/19 & 24/77 & 14/43 & 14/43 & 13/40 & 26/81 & 13/41 & 26/83 & 14/43 & 14/43 & 14/43 & 28/87 &  7/22 & 28/89 & 29/92 & 14/43 & 14/43 & 10/31 \\\hline
$38$ & 14/45 &  7/23 &  8/29 &  7/22 &  7/22 &  7/22 & 16/51 &  4/13 & 16/53 &  3/10 &  7/22 &  7/22 &  6/19 &  9/29 & 18/59 & 16/53 &  7/22 &  7/22 & 20/63 &  5/16 &  4/13 & 17/56 &  7/22 &  7/22 &  7/22 & 11/35 & 22/71 & 11/36 & 22/71 &  7/22 &  7/22 &  6/19 & 24/77 &  4/13 &  7/23 &  7/22 &  7/22 & 13/41 & 26/83 & 13/42 & 26/85 &  7/22 &  7/22 &  7/22 & 28/89 & 14/45 &  4/13 & 22/71 & 27/85 &  7/22 \\\hline
$39$ & 15/47 & 15/47 & 25/89 & 14/45 & 14/45 & 15/47 & 15/47 & 15/47 &  8/27 & 24/79 & 14/45 & 15/47 & 15/47 & 22/71 &  3/10 & 11/36 &  5/16 & 15/47 & 15/47 &  4/13 & 10/33 & 27/88 & 11/35 & 15/47 & 15/47 & 22/71 & 11/36 & 25/81 &  6/19 & 15/47 & 15/47 & 14/45 &  5/16 &  5/16 & 13/41 & 15/47 & 15/47 & 14/45 & 27/86 & 27/86 &  7/22 & 15/47 & 15/47 & 14/45 & 29/92 & 29/92 & 15/47 & 15/47 & 15/47 & 23/74 \\\hline
$40$ &  1/ 3 &  1/ 3 &  2/ 7 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 16/55 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 19/63 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 23/75 &  6/19 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 25/81 & 13/41 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 &  9/29 &  7/22 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 & 29/93 & 15/47 & 31/95 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$41$ &  1/ 3 & 16/49 &  7/25 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 & 29/99 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 18/61 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 29/97 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 &  4/13 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/41 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/43 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 & 30/91 & 15/46 & 31/95 &  1/ 3 &  1/ 3 &  1/ 3 & 32/97 \\\hline
$42$ & 16/49 &  8/25 & 14/51 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 & 27/94 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 29/94 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 22/69 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 &  8/25 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 & 26/81 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/43 & 28/87 &  1/ 3 &  1/ 3 &  1/ 3 & 30/91 & 15/46 & 10/31 &  1/ 3 &  1/ 3 &  1/ 3 & 32/97 & 16/49 \\\hline
$43$ &  8/25 & 16/51 &  7/26 & 16/49 & 16/49 & 16/49 &  9/28 &  6/19 & 28/93 & 20/63 & 16/49 & 16/49 & 10/31 & 20/63 &  5/16 & 17/55 & 16/49 & 16/49 & 11/34 & 22/69 & 11/35 &  3/10 & 16/49 & 16/49 & 12/37 &  8/25 &  6/19 & 24/77 & 16/49 & 16/49 & 13/40 & 26/81 & 13/41 & 26/83 & 16/49 & 16/49 & 14/43 & 28/87 &  7/22 & 28/89 & 16/49 & 16/49 & 15/46 & 10/31 & 15/47 &  6/19 & 16/49 & 16/49 & 16/49 & 32/99 \\\hline
$44$ & 16/51 &  4/13 &  3/11 &  8/25 &  8/25 &  8/25 &  6/19 &  9/29 & 18/59 & 16/53 &  8/25 &  8/25 & 20/63 &  5/16 &  4/13 & 18/59 &  8/25 &  8/25 & 22/69 & 11/35 & 22/71 & 19/62 &  8/25 &  8/25 &  8/25 &  6/19 & 24/77 &  4/13 &  8/25 &  8/25 &  8/25 & 13/41 & 26/83 & 13/42 &  4/13 &  8/25 &  8/25 &  7/22 & 28/89 & 14/45 &  4/13 &  8/25 &  8/25 & 15/47 &  6/19 &  5/16 & 30/97 &  8/25 &  8/25 &  8/25 \\\hline
$45$ & 17/53 & 17/53 & 23/83 & 16/51 & 16/51 & 17/53 & 17/53 & 17/53 &  3/10 & 27/88 & 16/51 & 17/53 & 17/53 &  5/16 & 10/33 & 29/94 & 11/35 & 17/53 & 17/53 & 22/71 & 11/36 & 13/42 &  6/19 & 17/53 & 17/53 & 24/77 &  4/13 & 25/81 & 13/41 & 17/53 & 17/53 & 26/83 & 13/42 &  9/29 &  7/22 & 17/53 & 17/53 & 16/51 & 29/92 & 29/92 & 15/47 & 17/53 & 17/53 & 16/51 & 31/98 & 31/98 &  8/25 & 17/53 & 17/53 & 16/51 \\\hline
$46$ &  1/ 3 &  1/ 3 & 20/71 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 18/61 &  5/16 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 & 11/35 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 23/75 &  6/19 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 25/81 & 13/41 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 &  9/29 &  7/22 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 & 29/93 & 15/47 & 31/95 &  1/ 3 &  1/ 3 &  1/ 3 & 31/99 &  8/25 & 17/52 &  1/ 3 &  1/ 3 &  1/ 3 \\\hline
$47$ &  1/ 3 & 18/55 &  2/ 7 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 &  9/31 & 21/65 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 29/97 & 23/71 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 13/43 & 25/77 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/43 & 27/83 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/45 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 & 30/91 & 15/47 & 31/95 &  1/ 3 &  1/ 3 &  1/ 3 & 32/97 & 16/49 & 17/52 &  1/ 3 &  1/ 3 &  1/ 3 & 32/97 \\\hline
$48$ & 18/55 &  9/28 & 16/57 &  1/ 3 &  1/ 3 &  1/ 3 & 20/61 & 10/31 & 26/89 &  1/ 3 &  1/ 3 &  1/ 3 & 22/67 & 11/34 & 23/76 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 &  8/25 &  1/ 3 &  1/ 3 &  1/ 3 & 26/79 & 13/40 & 26/81 &  1/ 3 &  1/ 3 &  1/ 3 & 28/85 & 14/43 & 28/87 &  1/ 3 &  1/ 3 &  1/ 3 & 30/91 & 15/46 & 10/31 &  1/ 3 &  1/ 3 &  1/ 3 & 32/97 & 16/49 & 32/99 &  1/ 3 &  1/ 3 &  1/ 3 & 32/97 & 17/52 \\\hline
$49$ &  9/28 &  6/19 &  8/29 & 20/63 & 18/55 & 18/55 & 10/31 & 20/63 & 21/71 & 22/69 & 18/55 & 18/55 & 11/34 & 22/69 & 11/35 & 19/61 & 18/55 & 18/55 & 12/37 &  8/25 &  6/19 & 26/85 & 18/55 & 18/55 & 13/40 & 26/81 & 13/41 & 25/82 & 18/55 & 18/55 & 14/43 & 28/87 &  7/22 & 28/89 & 18/55 & 18/55 & 15/46 & 10/31 & 15/47 &  6/19 & 18/55 & 18/55 & 16/49 & 32/99 &  8/25 & 19/60 & 18/55 & 18/55 & 17/52 & 23/71 \\\hline
$50$ &  6/19 &  9/29 & 16/59 &  9/29 &  9/28 &  9/28 & 20/63 &  5/16 &  4/13 & 17/56 &  9/28 &  9/28 & 22/69 & 11/35 & 22/71 & 19/62 &  9/28 &  9/28 &  8/25 &  6/19 & 24/77 & 21/68 &  9/28 &  9/28 & 26/81 & 13/41 & 26/83 & 13/42 &  9/28 &  9/28 &  9/28 &  7/22 & 28/89 & 14/45 & 28/89 &  9/28 &  9/28 & 15/47 &  6/19 &  5/16 &  9/29 &  9/28 &  9/28 &  8/25 & 19/60 & 16/51 & 23/74 &  9/28 &  9/28 & 17/53 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 3, 4, 4+k, 4+k+i\}$.
\end{center}


==> tables/table-g5-a2b3c5.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  1/ 4 &  1/ 5 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 \\\hline
$2$ &  1/ 5 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  5/22 &  1/ 4 &  1/ 4 &  1/ 4 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  7/30 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  9/38 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 & 11/46 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 & 13/54 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 \\\hline
$3$ &  4/17 &  3/13 &  3/13 &  4/17 &  2/ 9 &  4/17 &  4/17 &  3/13 &  3/13 &  3/13 &  4/17 &  4/17 &  7/30 &  4/17 &  3/13 &  3/13 &  4/17 &  4/17 &  7/30 &  7/30 &  4/17 &  3/13 &  4/17 &  4/17 &  7/30 & 10/43 &  7/30 &  4/17 &  4/17 & 11/47 &  4/17 & 10/43 & 10/43 &  4/17 &  4/17 & 11/47 & 11/47 &  4/17 & 13/56 &  4/17 &  4/17 & 11/47 &  7/30 & 11/47 &  4/17 &  4/17 & 15/64 &  4/17 &  7/30 &  7/30 \\\hline
$4$ &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  1/ 4 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/37 &  1/ 4 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  8/31 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/31 &  5/19 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/19 &  4/15 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  7/26 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/26 & 16/59 & 17/62 &  2/ 7 &  2/ 7 \\\hline
$5$ &  2/ 7 &  2/ 7 &  4/15 &  1/ 4 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  6/23 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$6$ &  2/ 7 &  4/15 &  1/ 4 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  6/23 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$7$ &  4/15 &  1/ 4 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  6/23 &  8/31 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  5/19 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 &  4/15 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 \\\hline
$8$ &  1/ 4 &  1/ 4 &  8/33 &  4/15 &  4/15 &  4/15 &  4/15 &  6/23 &  1/ 4 &  1/ 4 & 12/49 &  4/15 &  4/15 &  4/15 &  4/15 &  8/31 &  1/ 4 &  1/ 4 &  4/15 &  4/15 &  4/15 &  4/15 &  5/19 & 10/39 &  1/ 4 &  1/ 4 &  4/15 &  4/15 &  4/15 &  4/15 &  6/23 & 12/47 & 15/59 &  4/15 &  4/15 &  4/15 &  4/15 & 14/53 &  7/27 & 14/55 & 15/59 &  4/15 &  4/15 &  4/15 &  4/15 & 16/61 &  8/31 & 19/74 &  4/15 &  4/15 \\\hline
$9$ &  1/ 4 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 16/69 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  5/21 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  7/29 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 \\\hline
$10$ &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  1/ 4 &  1/ 4 &  1/ 4 & 15/61 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 24/97 &  1/ 4 &  1/ 4 &  1/ 4 & 20/81 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 \\\hline
$11$ &  2/ 7 &  2/ 7 &  2/ 7 &  8/33 &  6/25 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  1/ 4 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/39 & 10/39 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  6/23 &  6/23 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 14/53 & 14/53 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  4/15 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 & 18/67 & 19/69 &  2/ 7 &  2/ 7 \\\hline
$12$ &  2/ 7 &  2/ 7 &  3/11 &  1/ 4 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$13$ &  2/ 7 &  3/11 &  6/23 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$14$ &  3/11 &  6/23 &  8/31 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  5/19 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 &  4/15 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 20/73 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 \\\hline
$15$ &  6/23 &  1/ 4 &  1/ 4 &  3/11 &  3/11 &  3/11 &  3/11 &  4/15 &  8/31 & 25/99 & 13/51 &  3/11 &  3/11 &  3/11 & 10/37 &  5/19 & 10/39 & 13/51 &  3/11 &  3/11 &  3/11 &  3/11 &  4/15 &  6/23 & 15/58 &  3/11 &  3/11 &  3/11 &  3/11 &  7/26 & 14/53 &  7/27 & 19/73 &  3/11 &  3/11 &  3/11 & 16/59 &  4/15 & 16/61 & 19/73 &  3/11 &  3/11 &  3/11 &  3/11 & 18/67 &  9/34 & 21/80 &  3/11 &  3/11 &  3/11 \\\hline
$16$ &  1/ 4 &  1/ 4 & 12/49 &  6/23 &  6/23 &  6/23 &  6/23 &  8/31 &  1/ 4 &  1/ 4 & 16/65 &  6/23 &  6/23 &  6/23 &  6/23 & 10/39 &  1/ 4 &  1/ 4 & 20/81 &  6/23 &  6/23 &  6/23 &  6/23 & 12/47 &  1/ 4 &  1/ 4 &  6/23 &  6/23 &  6/23 &  6/23 &  7/27 & 14/55 &  1/ 4 &  1/ 4 &  6/23 &  6/23 &  6/23 &  6/23 &  8/31 & 16/63 &  1/ 4 &  1/ 4 &  6/23 &  6/23 &  6/23 &  6/23 &  9/35 & 18/71 & 23/91 &  6/23 \\\hline
$17$ &  7/27 &  7/27 &  7/27 &  8/31 & 14/55 &  8/31 &  7/27 &  7/27 &  7/27 &  7/27 &  8/31 &  8/31 & 18/71 &  7/27 &  7/27 &  7/27 & 19/75 &  8/31 &  1/ 4 & 10/39 &  7/27 &  7/27 &  7/27 & 21/82 & 13/51 & 13/51 &  7/27 &  7/27 &  7/27 &  7/27 & 15/58 & 19/74 & 15/58 &  7/27 &  7/27 &  7/27 &  7/27 & 15/58 & 15/58 & 21/82 &  7/27 &  7/27 &  7/27 & 13/51 & 15/58 & 18/71 & 17/66 &  7/27 &  7/27 &  7/27 \\\hline
$18$ &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  1/ 4 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/39 & 10/39 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  6/23 &  6/23 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 14/53 & 14/53 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  4/15 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 & 18/67 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/37 & 10/37 & 21/76 &  2/ 7 &  2/ 7 \\\hline
$19$ &  2/ 7 &  2/ 7 &  8/29 & 12/49 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 15/59 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$20$ &  2/ 7 &  8/29 &  4/15 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$21$ &  8/29 &  4/15 &  5/19 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 &  4/15 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 20/73 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 \\\hline
$22$ &  4/15 &  8/31 & 21/82 &  8/29 &  8/29 &  8/29 &  8/29 & 10/37 &  5/19 & 17/66 & 17/65 &  8/29 &  8/29 &  8/29 &  3/11 &  4/15 & 23/88 & 15/58 &  8/29 &  8/29 &  8/29 & 14/51 &  7/26 & 14/53 & 17/65 &  8/29 &  8/29 &  8/29 &  8/29 & 16/59 &  4/15 & 19/72 &  8/29 &  8/29 &  8/29 &  8/29 &  3/11 & 18/67 &  9/34 & 25/94 &  8/29 &  8/29 &  8/29 & 20/73 & 10/37 &  4/15 & 24/91 &  8/29 &  8/29 &  8/29 \\\hline
$23$ &  8/31 &  1/ 4 &  1/ 4 &  4/15 &  4/15 &  4/15 &  4/15 &  5/19 & 10/39 &  1/ 4 & 17/67 &  4/15 &  4/15 &  4/15 &  4/15 &  6/23 & 12/47 & 16/63 &  4/15 &  4/15 &  4/15 &  4/15 & 14/53 &  7/27 &  8/31 & 18/71 &  4/15 &  4/15 &  4/15 &  4/15 & 16/61 &  8/31 & 10/39 &  4/15 &  4/15 &  4/15 &  4/15 &  9/34 &  6/23 &  9/35 & 25/97 &  4/15 &  4/15 &  4/15 &  4/15 &  5/19 & 20/77 &  8/31 &  4/15 &  4/15 \\\hline
$24$ &  9/34 &  9/34 &  9/34 &  5/19 &  6/23 &  5/19 &  9/34 &  9/34 &  9/34 &  9/34 &  5/19 &  5/19 & 22/85 &  9/34 &  9/34 &  9/34 & 23/89 &  5/19 & 13/51 &  6/23 &  9/34 &  9/34 &  9/34 & 25/96 & 15/58 & 15/58 & 26/99 &  9/34 &  9/34 &  9/34 & 16/61 & 17/65 & 17/65 &  9/34 &  9/34 &  9/34 &  9/34 & 19/72 & 26/99 & 19/72 &  9/34 &  9/34 &  9/34 &  9/34 & 19/72 & 19/72 & 23/88 &  9/34 &  9/34 &  9/34 \\\hline
$25$ &  2/ 7 &  2/ 7 &  2/ 7 & 10/39 & 10/39 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  6/23 &  6/23 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 14/53 & 14/53 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  4/15 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 & 18/67 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/37 & 10/37 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 22/81 & 22/81 & 23/83 &  2/ 7 &  2/ 7 \\\hline
$26$ &  2/ 7 &  2/ 7 &  5/18 &  1/ 4 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 & 12/47 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 21/80 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$27$ &  2/ 7 &  5/18 & 10/37 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$28$ &  5/18 & 10/37 &  4/15 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 20/73 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 &  8/29 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 \\\hline
$29$ & 10/37 &  5/19 & 25/96 &  5/18 &  5/18 &  5/18 &  5/18 &  3/11 &  4/15 & 23/88 & 21/79 &  5/18 &  5/18 &  5/18 & 14/51 &  7/26 & 23/87 &  7/27 &  5/18 &  5/18 &  5/18 &  8/29 & 16/59 &  4/15 & 26/99 &  5/18 &  5/18 &  5/18 & 18/65 &  3/11 & 18/67 & 21/79 &  5/18 &  5/18 &  5/18 &  5/18 & 20/73 & 10/37 &  4/15 &  5/18 &  5/18 &  5/18 &  5/18 & 11/40 & 22/81 & 11/41 & 24/89 &  5/18 &  5/18 &  5/18 \\\hline
$30$ &  5/19 & 10/39 & 13/51 & 10/37 & 10/37 & 10/37 & 10/37 &  4/15 &  6/23 & 10/39 &  7/27 & 10/37 & 10/37 & 10/37 &  7/26 & 14/53 &  7/27 &  9/35 & 10/37 & 10/37 & 10/37 & 10/37 &  4/15 & 16/61 & 22/85 & 25/96 & 10/37 & 10/37 & 10/37 & 18/67 &  9/34 &  5/19 & 22/85 & 10/37 & 10/37 & 10/37 & 10/37 &  4/15 &  5/19 &  6/23 & 10/37 & 10/37 & 10/37 & 10/37 & 11/41 & 22/83 & 11/42 & 26/99 & 10/37 & 10/37 \\\hline
$31$ & 11/41 & 11/41 & 11/41 &  4/15 & 22/83 &  4/15 & 11/41 & 11/41 & 11/41 & 11/41 &  4/15 &  4/15 &  5/19 & 11/41 & 11/41 & 11/41 & 16/61 &  4/15 & 15/58 & 14/53 & 11/41 & 11/41 & 11/41 & 24/91 & 17/65 & 17/65 & 17/64 & 11/41 & 11/41 & 11/41 & 22/83 & 19/72 & 19/72 &  4/15 & 11/41 & 11/41 & 11/41 & 25/94 & 21/79 & 21/79 & 11/41 & 11/41 & 11/41 & 11/41 & 23/86 &  4/15 & 23/86 & 11/41 & 11/41 & 11/41 \\\hline
$32$ &  2/ 7 &  2/ 7 &  2/ 7 &  6/23 &  6/23 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 14/53 & 14/53 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  4/15 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 & 18/67 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/37 & 10/37 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 22/81 & 22/81 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  3/11 &  5/18 &  2/ 7 &  2/ 7 \\\hline
$33$ &  2/ 7 &  2/ 7 & 12/43 & 12/47 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 &  7/27 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 & 16/61 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 23/86 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$34$ &  2/ 7 & 12/43 &  3/11 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$35$ & 12/43 &  3/11 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 20/73 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 &  8/29 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 & 13/47 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 \\\hline
$36$ &  3/11 &  4/15 & 21/80 & 12/43 & 12/43 & 12/43 & 12/43 & 14/51 &  7/26 & 14/53 & 25/93 & 12/43 & 12/43 & 12/43 &  8/29 & 16/59 &  4/15 & 16/61 & 12/43 & 12/43 & 12/43 & 18/65 &  3/11 & 18/67 &  9/34 & 12/43 & 12/43 & 12/43 &  5/18 & 20/73 & 10/37 &  4/15 & 12/43 & 12/43 & 12/43 & 22/79 & 11/40 & 22/81 & 25/93 & 12/43 & 12/43 & 12/43 & 12/43 &  8/29 &  3/11 & 24/89 & 12/43 & 12/43 & 12/43 & 12/43 \\\hline
$37$ &  4/15 &  6/23 & 15/58 &  3/11 &  3/11 &  3/11 &  3/11 &  7/26 & 14/53 &  7/27 &  5/19 &  3/11 &  3/11 &  3/11 & 16/59 &  4/15 & 16/61 & 19/73 &  3/11 &  3/11 &  3/11 &  3/11 & 18/67 &  9/34 & 21/80 &  3/11 &  3/11 &  3/11 &  3/11 & 10/37 &  4/15 & 24/91 & 11/42 &  3/11 &  3/11 &  3/11 & 22/81 & 11/41 &  4/15 & 26/99 &  3/11 &  3/11 &  3/11 &  3/11 & 24/89 &  4/15 & 24/91 &  3/11 &  3/11 &  3/11 \\\hline
$38$ & 13/48 & 13/48 & 13/48 &  7/26 & 26/97 &  7/26 & 13/48 & 13/48 & 13/48 & 13/48 &  7/26 &  7/26 &  4/15 & 13/48 & 13/48 & 13/48 & 22/83 &  7/26 &  4/15 &  4/15 & 13/48 & 13/48 & 13/48 & 25/94 & 19/72 & 19/72 & 19/71 & 13/48 & 13/48 & 13/48 & 23/86 & 21/79 & 21/79 & 18/67 & 13/48 & 13/48 & 13/48 & 26/97 & 23/86 & 23/86 & 24/89 & 13/48 & 13/48 & 13/48 & 25/93 & 25/93 & 25/93 & 13/48 & 13/48 & 13/48 \\\hline
$39$ &  2/ 7 &  2/ 7 &  2/ 7 & 14/53 & 14/53 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  4/15 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 & 18/67 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/37 & 10/37 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 22/81 & 22/81 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  3/11 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 26/95 & 26/95 & 27/97 &  2/ 7 &  2/ 7 \\\hline
$40$ &  2/ 7 &  2/ 7 &  7/25 &  7/27 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 & 16/61 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 &  9/34 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  4/15 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 23/85 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 & 26/93 & 27/97 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$41$ &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 & 26/93 & 27/97 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$42$ &  7/25 & 14/51 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 20/73 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 &  8/29 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 & 13/47 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 & 26/93 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 28/99 \\\hline
$43$ & 14/51 &  7/26 & 14/53 &  7/25 &  7/25 &  7/25 &  7/25 &  8/29 & 16/59 &  4/15 & 16/59 &  7/25 &  7/25 &  7/25 & 18/65 &  3/11 & 18/67 &  9/34 &  7/25 &  7/25 &  7/25 &  5/18 & 20/73 & 10/37 &  4/15 &  7/25 &  7/25 &  7/25 & 22/79 & 11/40 & 22/81 & 11/41 &  7/25 &  7/25 &  7/25 & 12/43 &  8/29 &  3/11 & 24/89 &  7/25 &  7/25 &  7/25 & 26/93 & 13/47 & 26/95 & 13/48 &  7/25 &  7/25 &  7/25 &  7/25 \\\hline
$44$ &  7/26 & 14/53 & 17/65 & 14/51 & 14/51 & 14/51 & 14/51 & 16/59 &  4/15 & 16/61 & 25/94 & 14/51 & 14/51 & 14/51 &  3/11 & 18/67 &  9/34 &  6/23 & 14/51 & 14/51 & 14/51 & 20/73 & 10/37 &  4/15 &  5/19 & 14/51 & 14/51 & 14/51 & 14/51 & 22/81 & 11/41 & 13/49 & 23/86 & 14/51 & 14/51 & 14/51 &  3/11 & 24/89 &  4/15 & 13/49 & 14/51 & 14/51 & 14/51 & 26/95 & 13/48 &  7/26 & 17/64 & 14/51 & 14/51 & 14/51 \\\hline
$45$ &  3/11 &  3/11 &  3/11 & 16/59 & 10/37 & 16/59 &  3/11 &  3/11 &  3/11 &  3/11 & 16/59 & 16/59 &  7/26 &  3/11 &  3/11 &  3/11 & 23/86 & 16/59 &  7/26 &  7/26 &  3/11 &  3/11 &  3/11 & 26/97 & 25/94 & 23/87 & 24/89 &  3/11 &  3/11 &  3/11 & 25/93 & 23/86 & 23/86 & 24/89 &  3/11 &  3/11 &  3/11 & 24/89 & 25/93 & 25/93 & 13/48 &  3/11 &  3/11 &  3/11 & 23/85 & 17/63 & 17/63 & 25/92 &  3/11 &  3/11 \\\hline
$46$ &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 &  4/15 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 & 18/67 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/37 & 10/37 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 22/81 & 22/81 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  3/11 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 26/95 & 26/95 & 27/97 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 14/51 & 14/51 & 17/61 &  2/ 7 &  2/ 7 \\\hline
$47$ &  2/ 7 &  2/ 7 & 16/57 & 16/61 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 &  9/34 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  4/15 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 11/41 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 24/89 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 & 13/48 & 27/97 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 28/99 &  7/25 & 17/61 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$48$ &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 21/76 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 & 26/93 & 27/97 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 28/99 &  7/25 & 17/61 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$49$ & 16/57 &  8/29 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 20/73 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 20/71 &  5/18 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 11/39 & 22/79 &  8/29 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 24/85 & 12/43 & 13/47 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 13/46 & 26/93 & 23/83 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 28/99 &  7/25 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 15/53 \\\hline
$50$ &  8/29 & 16/59 &  4/15 & 16/57 & 16/57 & 16/57 & 16/57 & 18/65 &  3/11 & 18/67 &  3/11 & 16/57 & 16/57 & 16/57 &  5/18 & 20/73 & 10/37 &  4/15 & 16/57 & 16/57 & 16/57 & 22/79 & 11/40 & 22/81 & 11/41 & 16/57 & 16/57 & 16/57 & 12/43 &  8/29 &  3/11 & 24/89 & 16/57 & 16/57 & 16/57 & 26/93 & 13/47 & 26/95 & 13/48 & 16/57 & 16/57 & 16/57 &  7/25 & 23/83 & 14/51 & 25/92 & 16/57 & 16/57 & 16/57 & 23/82 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 3, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a2b3c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 3, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a2b4c5.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  2/ 9 &  1/ 5 &  2/ 9 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  4/17 &  2/ 9 &  5/23 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  6/25 &  3/13 &  7/31 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  8/33 &  4/17 &  3/13 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 10/41 &  5/21 & 11/47 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 12/49 &  6/25 & 13/55 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 &  1/ 4 & 14/57 &  7/29 \\\hline
$2$ &  1/ 3 &  3/14 &  1/ 3 &  1/ 3 &  4/17 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  6/23 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 \\\hline
$3$ &  3/13 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 \\\hline
$4$ &  2/ 7 &  2/ 7 &  2/ 7 &  6/25 &  3/13 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  6/25 &  7/27 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 10/39 &  1/ 4 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  6/23 & 10/39 & 11/41 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 14/53 &  6/23 & 13/48 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  4/15 & 14/53 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 18/67 &  4/15 & 17/62 &  2/ 7 &  2/ 7 \\\hline
$5$ &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 \\\hline
$6$ &  2/ 7 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 \\\hline
$7$ &  4/15 &  1/ 4 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  3/11 &  6/23 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  4/15 &  8/31 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 &  5/19 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  4/15 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 \\\hline
$8$ &  1/ 3 &  1/ 4 &  1/ 3 &  1/ 3 &  4/15 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 \\\hline
$9$ &  5/19 &  1/ 3 &  1/ 3 &  3/11 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 \\\hline
$10$ &  1/ 4 &  5/19 &  5/19 &  1/ 4 &  5/19 &  7/26 &  7/26 &  5/19 &  7/26 &  6/23 & 10/41 &  5/19 &  7/26 &  1/ 4 &  7/26 &  7/26 & 25/99 &  5/19 &  4/15 &  6/23 &  5/19 &  7/26 & 10/39 &  5/19 &  4/15 &  7/26 &  5/19 &  4/15 & 11/42 & 17/66 &  5/19 &  7/26 &  7/26 &  4/15 &  7/26 & 19/72 &  5/19 & 17/64 &  7/26 &  5/19 &  7/26 &  7/26 &  5/19 & 17/64 & 19/71 & 19/72 & 17/64 &  7/26 &  6/23 &  5/19 \\\hline
$11$ &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 \\\hline
$12$ &  2/ 7 &  1/ 3 &  1/ 3 &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 \\\hline
$13$ &  2/ 7 &  3/11 &  3/11 &  6/23 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  7/26 &  9/34 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/18 & 10/37 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  3/11 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/25 & 14/51 &  3/11 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  8/29 & 17/62 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 18/65 & 19/69 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$14$ &  1/ 3 &  7/26 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 \\\hline
$15$ &  7/25 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 \\\hline
$16$ &  7/26 &  7/25 &  7/25 &  7/26 &  7/25 &  9/32 &  9/32 &  7/25 &  9/32 &  8/29 & 14/53 &  7/25 &  9/32 & 17/65 &  9/32 &  9/32 & 13/49 &  7/25 & 21/76 &  7/26 &  7/25 &  9/32 &  3/11 &  7/25 & 16/57 &  8/29 &  7/25 &  7/25 & 14/51 &  7/25 & 16/57 &  9/32 &  7/25 & 16/57 &  5/18 & 23/84 &  7/25 &  9/32 &  9/32 & 16/57 &  9/32 &  5/18 &  7/25 &  5/18 &  9/32 &  7/25 &  9/32 &  9/32 &  7/25 & 23/82 \\\hline
$17$ &  1/ 3 &  8/29 &  1/ 3 &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 \\\hline
$18$ &  2/ 7 &  1/ 3 &  1/ 3 &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 \\\hline
$19$ &  2/ 7 &  2/ 7 &  2/ 7 &  8/29 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  9/32 & 16/59 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 12/43 &  2/ 7 & 23/82 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 15/53 & 17/61 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 16/57 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 17/60 & 26/93 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 & 28/99 &  2/ 7 & 13/46 &  2/ 7 &  2/ 7 &  2/ 7 \\\hline
$20$ &  1/ 3 &  9/32 &  1/ 3 &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 \\\hline
$21$ &  9/31 &  1/ 3 &  1/ 3 &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 \\\hline
$22$ &  9/32 &  9/31 &  9/31 &  9/32 &  9/31 &  9/31 & 11/38 &  9/31 &  9/31 &  2/ 7 & 18/65 &  9/31 & 11/38 &  8/29 &  9/31 & 11/38 & 11/40 &  9/31 & 25/88 & 23/83 &  9/31 & 11/38 & 12/43 &  9/31 & 27/94 &  9/32 &  9/31 & 17/59 & 19/67 &  9/31 &  9/31 &  2/ 7 &  9/31 &  9/31 &  2/ 7 &  9/31 &  9/31 & 20/69 &  9/31 &  9/31 & 19/66 & 27/95 &  9/31 & 20/69 & 11/38 &  9/31 & 20/69 & 27/94 &  9/31 & 27/94 \\\hline
$23$ &  1/ 3 &  2/ 7 &  1/ 3 &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 \\\hline
$24$ &  5/17 &  1/ 3 &  1/ 3 & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 \\\hline
$25$ &  2/ 7 &  5/17 &  5/17 &  2/ 7 &  5/17 &  5/17 & 12/41 &  5/17 &  5/17 & 11/38 & 20/71 &  5/17 & 12/41 &  2/ 7 &  5/17 & 12/41 &  2/ 7 &  5/17 & 27/94 & 25/89 &  5/17 & 12/41 &  2/ 7 &  5/17 & 20/69 & 27/95 &  5/17 & 23/79 &  2/ 7 &  5/17 & 19/65 & 19/66 &  5/17 &  5/17 & 20/69 &  5/17 &  5/17 & 20/69 &  5/17 &  5/17 & 22/75 &  5/17 &  5/17 &  7/24 & 17/59 &  5/17 & 22/75 & 12/41 &  5/17 & 22/75 \\\hline
$26$ &  1/ 3 & 11/38 &  1/ 3 &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 \\\hline
$27$ & 11/37 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 \\\hline
$28$ & 11/38 & 11/37 & 11/37 & 11/38 & 11/37 & 11/37 & 13/44 & 11/37 & 11/37 & 12/41 &  2/ 7 & 11/37 & 13/44 &  2/ 7 & 11/37 & 13/44 & 13/46 & 11/37 & 20/69 &  2/ 7 & 11/37 & 13/44 &  2/ 7 & 11/37 & 19/65 & 27/94 & 11/37 & 27/92 & 15/52 & 11/37 & 28/95 & 20/69 & 11/37 & 21/71 &  7/24 & 11/37 & 11/37 & 22/75 & 11/37 & 11/37 & 22/75 & 11/37 & 11/37 &  8/27 & 11/37 & 11/37 & 23/78 &  7/24 & 11/37 &  8/27 \\\hline
$29$ &  1/ 3 & 12/41 &  1/ 3 &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 \\\hline
$30$ &  3/10 &  1/ 3 &  1/ 3 & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 \\\hline
$31$ & 12/41 &  3/10 &  3/10 & 12/41 &  3/10 &  3/10 & 14/47 &  3/10 &  3/10 & 13/44 & 24/83 &  3/10 & 14/47 & 27/95 &  3/10 & 14/47 &  2/ 7 &  3/10 & 19/65 & 27/94 &  3/10 & 14/47 & 15/52 &  3/10 & 28/95 & 20/69 &  3/10 & 21/71 & 16/55 &  3/10 & 27/91 & 26/89 &  3/10 & 25/84 & 22/75 &  3/10 & 23/77 & 23/78 &  3/10 &  3/10 &  8/27 &  3/10 &  3/10 &  8/27 &  3/10 &  3/10 & 26/87 &  3/10 &  3/10 & 25/84 \\\hline
$32$ &  1/ 3 & 13/44 &  1/ 3 &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 \\\hline
$33$ & 13/43 &  1/ 3 &  1/ 3 &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 \\\hline
$34$ & 13/44 & 13/43 & 13/43 & 13/44 & 13/43 & 13/43 &  3/10 & 13/43 & 13/43 & 14/47 & 26/89 & 13/43 &  3/10 & 27/94 & 13/43 &  3/10 & 15/52 & 13/43 & 28/95 & 20/69 & 13/43 &  3/10 & 16/55 & 13/43 & 27/91 & 26/89 & 13/43 & 25/84 & 17/58 & 13/43 & 20/67 &  5/17 & 13/43 & 29/97 & 18/61 & 13/43 &  3/10 &  8/27 & 13/43 & 25/83 & 25/84 & 13/43 & 13/43 & 26/87 & 13/43 & 13/43 & 26/87 & 13/43 & 13/43 & 28/93 \\\hline
$35$ &  1/ 3 & 14/47 &  1/ 3 &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 \\\hline
$36$ &  7/23 &  1/ 3 &  1/ 3 & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 \\\hline
$37$ & 14/47 &  7/23 &  7/23 & 14/47 &  7/23 &  7/23 & 16/53 &  7/23 &  7/23 &  3/10 & 28/95 &  7/23 & 16/53 & 20/69 &  7/23 & 16/53 & 16/55 &  7/23 & 27/91 & 26/89 &  7/23 & 16/53 & 17/58 &  7/23 & 20/67 &  5/17 &  7/23 & 29/97 & 18/61 &  7/23 &  3/10 & 29/98 &  7/23 & 28/93 & 19/64 &  7/23 & 22/73 & 25/84 &  7/23 & 13/43 & 26/87 &  7/23 & 27/89 &  3/10 &  7/23 &  7/23 & 28/93 &  7/23 &  7/23 & 28/93 \\\hline
$38$ &  1/ 3 &  3/10 &  1/ 3 &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 \\\hline
$39$ & 15/49 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 \\\hline
$40$ &  3/10 & 15/49 & 15/49 &  3/10 & 15/49 & 15/49 & 17/56 & 15/49 & 15/49 & 16/53 & 19/64 & 15/49 & 17/56 & 26/89 & 15/49 & 17/56 & 17/58 & 15/49 & 20/67 &  5/17 & 15/49 & 17/56 & 18/61 & 15/49 &  3/10 & 29/98 & 15/49 & 28/93 & 19/64 & 15/49 & 22/73 & 25/84 & 15/49 & 29/96 & 20/67 & 15/49 & 23/76 & 26/87 & 15/49 & 27/89 &  3/10 & 15/49 &  7/23 & 28/93 & 15/49 & 29/95 & 29/96 & 15/49 & 15/49 & 10/33 \\\hline
$41$ &  1/ 3 & 16/53 &  1/ 3 &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 \\\hline
$42$ &  4/13 &  1/ 3 &  1/ 3 & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 \\\hline
$43$ & 16/53 &  4/13 &  4/13 & 16/53 &  4/13 &  4/13 & 18/59 &  4/13 &  4/13 & 17/56 & 29/97 &  4/13 & 18/59 &  5/17 &  4/13 & 18/59 & 18/61 &  4/13 &  3/10 & 29/98 &  4/13 & 18/59 & 19/64 &  4/13 & 22/73 & 25/84 &  4/13 & 29/96 & 20/67 &  4/13 & 23/76 & 29/97 &  4/13 & 27/89 &  3/10 &  4/13 & 24/79 & 28/93 &  4/13 &  7/23 & 28/93 &  4/13 & 29/95 & 29/96 &  4/13 & 15/49 & 10/33 &  4/13 & 27/88 & 24/79 \\\hline
$44$ &  1/ 3 & 17/56 &  1/ 3 &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 &  1/ 3 &  1/ 3 & 20/63 \\\hline
$45$ & 17/55 &  1/ 3 &  1/ 3 &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 \\\hline
$46$ & 17/56 & 17/55 & 17/55 & 17/56 & 17/55 & 17/55 & 19/62 & 17/55 & 17/55 & 18/59 & 28/93 & 17/55 & 19/62 & 29/98 & 17/55 & 19/62 & 19/64 & 17/55 &  3/10 & 25/84 & 17/55 & 19/62 & 19/64 & 17/55 & 22/73 & 29/97 & 17/55 & 27/89 &  3/10 & 17/55 & 23/76 & 28/93 & 17/55 & 25/82 & 22/73 & 17/55 &  7/23 & 28/93 & 17/55 & 26/85 & 29/96 & 17/55 & 15/49 & 10/33 & 17/55 & 27/88 & 24/79 & 17/55 &  4/13 & 25/82 \\\hline
$47$ &  1/ 3 & 18/59 &  1/ 3 &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 &  1/ 3 &  1/ 3 & 20/63 &  1/ 3 &  1/ 3 & 27/85 \\\hline
$48$ &  9/29 &  1/ 3 &  1/ 3 & 19/61 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 21/67 &  1/ 3 &  1/ 3 & 11/35 &  1/ 3 &  1/ 3 & 23/73 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 25/79 &  1/ 3 &  1/ 3 & 13/41 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 &  1/ 3 &  1/ 3 & 29/91 &  1/ 3 &  1/ 3 & 15/47 &  1/ 3 &  1/ 3 & 31/97 &  1/ 3 &  1/ 3 &  8/25 &  1/ 3 &  1/ 3 & 25/78 &  1/ 3 &  1/ 3 & 17/53 &  1/ 3 \\\hline
$49$ & 18/59 &  9/29 &  9/29 & 18/59 &  9/29 &  9/29 &  4/13 &  9/29 &  9/29 & 18/59 & 23/76 &  9/29 &  4/13 & 25/84 &  9/29 &  4/13 & 19/64 &  9/29 &  3/10 & 29/97 &  9/29 &  4/13 & 20/67 &  9/29 & 23/76 & 28/93 &  9/29 & 25/82 &  3/10 &  9/29 & 27/89 & 28/93 &  9/29 & 25/82 & 23/76 &  9/29 & 29/95 & 29/97 &  9/29 & 15/49 & 10/33 &  9/29 & 27/88 & 24/79 &  9/29 &  4/13 & 25/82 &  9/29 & 29/94 & 11/36 \\\hline
$50$ &  1/ 3 & 19/62 &  1/ 3 &  1/ 3 &  4/13 &  1/ 3 &  1/ 3 & 21/68 &  1/ 3 &  1/ 3 & 22/71 &  1/ 3 &  1/ 3 & 23/74 &  1/ 3 &  1/ 3 & 24/77 &  1/ 3 &  1/ 3 &  5/16 &  1/ 3 &  1/ 3 & 26/83 &  1/ 3 &  1/ 3 & 27/86 &  1/ 3 &  1/ 3 & 28/89 &  1/ 3 &  1/ 3 & 29/92 &  1/ 3 &  1/ 3 &  6/19 &  1/ 3 &  1/ 3 & 31/98 &  1/ 3 &  1/ 3 & 19/60 &  1/ 3 &  1/ 3 & 20/63 &  1/ 3 &  1/ 3 & 27/85 &  1/ 3 &  1/ 3 &  7/22 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 4, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a2b4c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 4, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a2b5c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 2, 5, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a3b4c5.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }c@{\ }}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &  3/10 &  3/11 &  1/ 4 &  1/ 4 &  5/17 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 &  6/19 &  3/10 &  2/ 7 &  7/25 &  4/13 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 &  9/28 &  9/29 &  3/10 &  5/17 & 11/35 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 & 13/43 &  7/22 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 15/46 & 15/47 &  5/16 &  4/13 & 17/53 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 & 19/61 & 10/31 \\\hline
$2$ &  3/11 &  1/ 4 &  3/13 &  1/ 4 &  5/19 &  3/10 &  3/10 &  3/10 &  3/10 &  3/10 &  2/ 7 &  3/11 &  6/23 &  1/ 4 &  8/29 &  3/10 &  3/10 &  3/10 &  3/10 &  3/10 &  9/31 &  9/32 &  3/11 &  9/34 & 11/39 &  3/10 &  3/10 &  3/10 &  3/10 &  3/10 & 12/41 &  2/ 7 & 12/43 &  3/11 &  2/ 7 &  3/10 &  3/10 &  3/10 &  3/10 &  3/10 &  5/17 & 15/52 & 15/53 &  5/18 & 17/59 &  3/10 &  3/10 &  3/10 &  3/10 &  3/10 \\\hline
$3$ &  1/ 4 &  3/13 &  3/13 &  2/ 9 &  5/21 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  6/23 &  1/ 4 &  6/25 &  3/13 &  1/ 4 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  9/34 &  9/35 &  1/ 4 &  9/37 & 11/43 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  4/15 &  6/23 & 12/47 &  1/ 4 &  7/27 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 &  3/11 & 15/56 &  5/19 & 15/58 & 15/59 & 17/65 &  3/11 \\\hline
$4$ &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  7/30 &  1/ 4 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 &  7/26 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  1/ 4 & 15/58 &  7/26 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/19 & 11/40 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  5/19 & 23/86 & 11/40 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/26 &  5/18 &  5/18 &  2/ 7 &  2/ 7 &  2/ 7 &  2/ 7 &  7/26 & 25/92 &  5/18 &  2/ 7 &  2/ 7 \\\hline
$5$ &  1/ 3 &  1/ 3 &  7/23 &  1/ 4 &  1/ 4 &  2/ 7 &  7/22 &  1/ 3 &  1/ 3 &  1/ 3 &  9/31 &  7/27 &  2/ 7 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 &  6/19 & 11/39 &  2/ 7 & 11/36 & 12/37 &  1/ 3 &  1/ 3 &  1/ 3 &  7/23 &  2/ 7 & 13/43 &  7/22 &  1/ 3 &  1/ 3 &  1/ 3 & 17/53 &  8/27 &  3/10 & 16/51 & 17/52 &  1/ 3 &  1/ 3 &  1/ 3 & 19/61 & 17/57 &  9/29 & 19/59 &  1/ 3 &  1/ 3 &  1/ 3 & 11/34 &  7/23 &  4/13 \\\hline
$6$ &  3/ 8 &  3/ 8 &  8/25 &  7/26 &  2/ 7 &  7/22 &  8/23 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 &  5/17 &  9/29 &  1/ 3 & 11/31 &  3/ 8 &  3/ 8 &  3/ 8 & 14/41 & 13/42 & 12/37 & 13/38 & 14/39 &  3/ 8 &  3/ 8 &  3/ 8 & 17/49 &  8/25 &  1/ 3 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 20/57 & 19/58 & 18/53 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 & 23/65 &  1/ 3 & 21/61 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 \\\hline
$7$ &  3/ 8 &  6/17 &  1/ 3 &  2/ 7 &  7/22 &  8/23 &  3/ 8 &  3/ 8 &  3/ 8 &  9/25 &  9/26 &  1/ 3 &  1/ 3 & 11/31 &  3/ 8 &  3/ 8 &  3/ 8 &  4/11 &  6/17 & 12/35 & 13/38 & 14/39 &  3/ 8 &  3/ 8 &  3/ 8 & 15/41 &  5/14 & 15/43 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/17 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 21/59 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 \\\hline
$8$ &  6/17 &  1/ 3 &  6/19 &  3/10 & 10/31 &  3/ 8 &  3/ 8 &  3/ 8 &  9/25 &  9/26 &  1/ 3 &  9/28 &  1/ 3 &  3/ 8 &  3/ 8 &  3/ 8 &  4/11 &  6/17 & 12/35 &  1/ 3 & 16/47 &  3/ 8 &  3/ 8 &  3/ 8 & 15/41 &  5/14 & 15/43 & 15/44 & 19/55 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/17 &  9/26 & 22/63 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 21/59 &  7/20 & 25/71 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 \\\hline
$9$ &  1/ 3 &  6/19 &  3/10 &  2/ 7 & 10/33 &  6/17 &  6/17 &  6/17 &  9/26 &  1/ 3 &  9/28 &  9/29 &  3/10 &  1/ 3 &  6/17 &  6/17 &  6/17 & 12/35 &  1/ 3 & 12/37 &  6/19 &  8/25 &  6/17 &  6/17 &  6/17 & 15/43 & 15/44 &  1/ 3 & 15/46 & 15/47 & 20/59 &  6/17 &  6/17 &  6/17 &  9/26 & 18/53 &  1/ 3 & 18/55 & 22/67 &  6/17 &  6/17 &  6/17 &  7/20 & 21/61 & 21/62 &  1/ 3 & 21/64 & 13/38 &  6/17 &  6/17 \\\hline
$10$ &  6/19 &  3/10 &  2/ 7 &  3/11 &  2/ 7 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 &  9/28 &  9/29 &  3/10 &  9/31 & 13/44 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 &  3/10 & 16/53 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 15/46 & 15/47 &  5/16 & 15/49 & 19/62 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  9/29 & 22/71 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 21/64 & 21/65 &  7/22 & 21/67 &  5/16 \\\hline
$11$ &  3/10 &  2/ 7 &  2/ 7 &  6/23 & 10/37 &  6/19 &  6/19 &  6/19 &  6/19 &  9/29 &  3/10 &  9/31 & 13/46 &  2/ 7 & 14/47 &  6/19 &  6/19 &  6/19 &  6/19 &  4/13 &  3/10 & 12/41 &  2/ 7 &  2/ 7 &  6/19 &  6/19 &  6/19 &  6/19 &  5/16 & 15/49 &  3/10 &  5/17 & 15/52 & 10/33 &  6/19 &  6/19 &  6/19 &  6/19 &  9/29 & 18/59 &  3/10 & 18/61 & 22/75 &  6/19 &  6/19 &  6/19 &  6/19 & 21/67 & 21/68 &  7/23 \\\hline
$12$ &  7/22 &  7/22 & 11/37 &  7/26 &  7/26 &  3/10 &  9/29 &  7/22 &  7/22 &  7/22 &  9/31 &  5/17 &  5/17 & 11/36 &  7/22 &  7/22 &  7/22 &  3/10 &  3/10 & 13/42 & 13/42 &  7/22 &  7/22 &  7/22 & 18/59 &  3/10 &  3/10 & 13/42 & 16/51 &  7/22 &  7/22 &  7/22 &  8/27 & 17/56 & 17/56 &  9/29 &  7/22 &  7/22 &  7/22 & 19/62 & 19/62 &  5/16 &  5/16 &  7/22 &  7/22 &  7/22 & 25/81 & 19/62 & 19/62 &  5/16 \\\hline
$13$ &  8/23 &  8/23 &  4/13 &  7/27 &  2/ 7 &  9/29 &  1/ 3 &  8/23 &  8/23 &  8/23 & 14/47 &  2/ 7 & 11/36 & 12/37 & 13/38 &  8/23 &  8/23 &  1/ 3 & 16/55 & 13/43 &  7/22 &  1/ 3 &  8/23 &  8/23 &  8/23 & 10/31 &  3/10 & 16/51 & 17/52 & 18/53 &  8/23 &  8/23 &  8/23 & 11/35 &  9/29 & 19/59 &  1/ 3 & 21/61 &  8/23 &  8/23 & 26/77 &  4/13 &  7/22 & 22/67 & 23/68 &  8/23 &  8/23 &  8/23 & 28/85 & 23/73 \\\hline
$14$ &  3/ 8 &  3/ 8 & 13/41 &  2/ 7 &  9/29 &  1/ 3 & 11/31 &  3/ 8 &  3/ 8 &  3/ 8 & 16/49 & 11/36 & 12/37 & 13/38 & 14/39 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 &  7/22 &  1/ 3 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 22/65 & 17/52 & 18/53 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 & 25/73 &  1/ 3 & 21/61 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 28/81 & 23/68 &  8/23 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 \\\hline
$15$ &  3/ 8 &  9/25 & 14/43 &  3/11 &  1/ 3 & 11/31 &  3/ 8 &  3/ 8 &  3/ 8 &  4/11 &  6/17 &  4/13 & 13/38 & 14/39 &  3/ 8 &  3/ 8 &  3/ 8 & 15/41 &  5/14 &  1/ 3 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/17 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 21/59 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 & 24/67 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 \\\hline
$16$ &  9/25 &  9/26 &  1/ 3 & 13/46 & 15/47 &  3/ 8 &  3/ 8 &  3/ 8 &  4/11 &  6/17 & 12/35 &  1/ 3 & 18/55 &  3/ 8 &  3/ 8 &  3/ 8 & 15/41 &  5/14 & 15/43 & 15/44 &  1/ 3 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/17 &  9/26 & 18/53 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 21/59 &  7/20 & 21/61 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 & 24/67 &  6/17 &  8/23 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 \\\hline
$17$ &  9/26 &  1/ 3 &  9/28 &  7/24 & 15/49 &  9/25 &  9/25 &  9/25 &  6/17 & 12/35 &  1/ 3 & 12/37 &  6/19 & 10/29 &  9/25 &  9/25 &  5/14 & 15/43 & 15/44 &  1/ 3 & 15/46 &  1/ 3 &  9/25 &  9/25 &  9/25 &  6/17 &  9/26 & 18/53 &  1/ 3 & 18/55 &  9/25 &  9/25 &  9/25 & 21/59 &  7/20 & 21/61 & 21/62 &  1/ 3 & 29/83 &  9/25 &  9/25 & 24/67 &  6/17 &  8/23 & 12/35 & 24/71 & 31/91 &  9/25 &  9/25 &  9/25 \\\hline
$18$ &  1/ 3 &  9/28 &  9/29 &  3/10 &  5/17 &  9/26 &  9/26 &  9/26 & 12/35 &  1/ 3 & 12/37 &  6/19 &  4/13 & 19/60 &  9/26 &  9/26 &  9/26 & 15/44 &  1/ 3 & 15/46 & 15/47 &  5/16 &  1/ 3 &  9/26 &  9/26 &  9/26 & 18/53 &  1/ 3 & 18/55 &  9/28 &  6/19 &  9/26 &  9/26 &  9/26 & 21/61 & 21/62 &  1/ 3 & 21/64 & 21/65 & 14/43 &  9/26 &  9/26 &  9/26 & 12/35 & 24/71 &  1/ 3 & 24/73 & 12/37 & 32/95 &  9/26 \\\hline
$19$ &  9/28 &  9/29 &  3/10 &  9/31 & 15/53 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 12/37 &  6/19 &  4/13 &  3/10 & 13/43 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 15/46 & 15/47 &  5/16 &  9/29 &  9/29 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 18/55 &  9/28 &  6/19 &  9/29 & 18/59 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 21/64 & 21/65 &  7/22 & 21/67 & 30/97 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 24/73 & 12/37 &  8/25 &  6/19 & 24/77 \\\hline
$20$ &  1/ 3 &  1/ 3 & 16/53 &  9/32 &  2/ 7 &  9/28 & 12/37 &  1/ 3 &  1/ 3 &  1/ 3 &  4/13 & 13/42 & 13/42 & 23/72 &  1/ 3 &  1/ 3 &  1/ 3 &  9/28 & 15/47 &  8/25 &  8/25 & 17/52 &  1/ 3 &  1/ 3 &  1/ 3 &  9/28 &  9/28 & 19/58 & 19/58 &  1/ 3 &  1/ 3 &  1/ 3 & 26/83 &  9/28 &  9/28 & 19/58 & 22/67 &  1/ 3 &  1/ 3 &  1/ 3 & 11/35 &  8/25 & 23/72 & 29/89 &  1/ 3 &  1/ 3 &  1/ 3 & 17/53 & 25/78 & 13/40 \\\hline
$21$ & 11/31 & 11/31 & 17/55 &  2/ 7 & 11/36 & 12/37 & 13/38 & 11/31 & 11/31 & 11/31 & 19/63 & 13/43 &  7/22 &  1/ 3 &  8/23 & 11/31 & 11/31 & 12/35 &  9/29 & 16/51 & 17/52 & 18/53 & 19/54 & 11/31 & 11/31 &  1/ 3 &  9/29 & 19/59 &  1/ 3 & 21/61 & 11/31 & 11/31 & 11/31 & 14/43 &  7/22 & 22/67 & 23/68 &  8/23 & 11/31 & 11/31 & 11/31 & 15/47 & 12/37 &  1/ 3 & 13/38 & 27/77 & 11/31 & 11/31 & 26/75 & 26/81 \\\hline
$22$ &  3/ 8 &  3/ 8 &  6/19 &  8/29 & 12/37 & 13/38 & 14/39 &  3/ 8 &  3/ 8 &  3/ 8 & 21/65 &  7/22 &  1/ 3 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 24/73 & 17/52 & 18/53 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 &  1/ 3 & 21/61 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 30/89 & 23/68 &  8/23 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 33/97 & 13/38 & 27/77 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 \\\hline
$23$ &  3/ 8 &  4/11 & 19/59 &  4/15 & 20/61 & 14/39 &  3/ 8 &  3/ 8 &  3/ 8 & 15/41 & 23/67 &  5/17 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/19 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 &  1/ 3 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 &  8/23 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 &  9/25 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 \\\hline
$24$ &  4/11 &  6/17 & 20/61 & 17/62 & 20/63 &  3/ 8 &  3/ 8 &  3/ 8 & 15/41 &  5/14 & 15/43 & 11/35 & 23/71 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/17 &  9/26 & 26/79 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 21/59 &  7/20 &  1/ 3 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 & 24/67 &  6/17 &  8/23 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 &  9/25 & 27/76 & 27/77 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 15/41 \\\hline
$25$ &  6/17 & 12/35 &  1/ 3 &  9/32 &  4/13 &  4/11 &  4/11 &  4/11 &  5/14 & 15/43 & 15/44 &  1/ 3 & 22/73 & 13/37 &  4/11 &  4/11 &  9/25 &  6/17 &  9/26 & 18/53 &  1/ 3 & 14/41 &  4/11 &  4/11 & 21/58 & 21/59 &  7/20 & 21/61 & 21/62 &  1/ 3 &  4/11 &  4/11 &  4/11 & 24/67 &  6/17 &  8/23 & 12/35 & 24/71 &  4/11 &  4/11 &  4/11 &  9/25 & 27/76 & 27/77 &  9/26 & 27/79 & 27/76 &  4/11 &  4/11 & 30/83 \\\hline
$26$ & 12/35 &  1/ 3 & 12/37 & 19/66 & 20/67 &  6/17 &  6/17 &  6/17 & 15/43 & 15/44 &  1/ 3 & 15/46 & 23/75 & 25/76 &  6/17 &  6/17 &  6/17 &  9/26 & 18/53 &  1/ 3 & 18/55 &  9/28 &  6/17 &  6/17 &  6/17 &  7/20 & 21/61 & 21/62 &  1/ 3 & 21/64 &  1/ 3 &  6/17 &  6/17 &  6/17 &  8/23 & 12/35 & 24/71 &  1/ 3 & 24/73 &  6/17 &  6/17 &  6/17 & 27/77 &  9/26 & 27/79 & 27/80 &  1/ 3 & 33/98 &  6/17 &  6/17 \\\hline
$27$ &  1/ 3 & 12/37 &  6/19 &  5/17 & 20/69 & 12/35 & 12/35 & 12/35 & 15/44 &  1/ 3 & 15/46 & 15/47 &  5/16 & 27/86 & 12/35 & 12/35 & 12/35 & 18/53 &  1/ 3 & 18/55 &  9/28 & 19/59 & 12/37 & 12/35 & 12/35 & 12/35 & 21/62 &  1/ 3 & 21/64 & 12/37 & 12/37 &  1/ 3 & 12/35 & 12/35 & 12/35 & 24/71 &  1/ 3 & 24/73 & 12/37 &  8/25 & 12/35 & 12/35 & 12/35 & 27/79 & 27/80 &  1/ 3 & 27/82 & 27/83 &  9/28 & 12/35 \\\hline
$28$ & 13/38 & 13/38 &  4/13 &  3/10 & 13/43 &  1/ 3 &  1/ 3 & 13/38 & 13/38 & 13/38 & 15/47 &  5/16 & 16/51 & 29/88 & 18/53 & 13/38 & 13/38 &  1/ 3 & 18/55 & 19/58 & 19/58 &  1/ 3 & 13/38 & 13/38 & 13/38 &  1/ 3 &  1/ 3 &  1/ 3 &  1/ 3 & 23/68 & 13/38 & 13/38 &  1/ 3 &  1/ 3 &  1/ 3 & 25/74 & 25/74 & 13/38 & 13/38 & 13/38 & 27/85 &  1/ 3 &  1/ 3 & 33/98 & 28/83 & 13/38 & 13/38 & 13/38 & 14/43 & 29/88 \\\hline
$29$ & 14/39 & 14/39 & 22/71 & 12/41 &  7/22 &  1/ 3 &  8/23 & 14/39 & 14/39 & 14/39 &  5/16 & 16/51 & 17/52 & 18/53 & 19/54 & 14/39 & 14/39 & 15/43 &  9/28 & 19/59 &  1/ 3 & 21/61 & 11/31 & 14/39 & 14/39 & 16/47 & 12/37 & 22/67 & 23/68 &  8/23 &  5/14 & 14/39 & 14/39 &  1/ 3 & 12/37 &  1/ 3 & 13/38 & 27/77 & 14/39 & 14/39 & 14/39 & 26/81 & 27/82 & 28/83 & 29/84 &  6/17 & 14/39 & 14/39 & 14/39 & 29/89 \\\hline
$30$ &  3/ 8 &  3/ 8 & 23/73 &  2/ 7 &  1/ 3 &  8/23 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 26/81 & 25/82 & 18/53 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 & 29/89 &  1/ 3 & 21/61 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 32/97 & 23/68 &  8/23 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 & 13/38 & 27/77 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 & 28/83 & 29/84 &  6/17 & 31/86 & 32/87 &  3/ 8 &  3/ 8 &  3/ 8 \\\hline
$31$ &  3/ 8 & 15/41 &  8/25 & 12/43 & 25/77 & 17/47 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 & 28/83 & 17/57 & 29/85 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 32/91 & 22/71 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 &  8/25 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 & 27/83 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 15/41 & 29/85 & 31/86 & 32/87 &  3/ 8 &  3/ 8 &  3/ 8 & 33/89 \\\hline
$32$ & 15/41 &  5/14 & 25/77 & 11/39 & 25/79 &  3/ 8 &  3/ 8 &  3/ 8 & 18/49 &  9/25 &  6/17 & 13/43 & 28/87 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 21/59 & 31/94 & 31/95 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 & 24/67 &  6/17 & 32/97 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 &  9/25 & 27/76 & 32/97 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 15/41 & 30/83 &  5/14 &  6/17 &  3/ 8 &  3/ 8 &  3/ 8 & 33/89 & 11/30 \\\hline
$33$ &  5/14 & 15/43 & 26/79 & 11/40 & 25/81 & 15/41 & 15/41 & 15/41 &  9/25 &  6/17 &  9/26 &  7/22 & 27/89 & 16/45 & 15/41 & 15/41 & 21/58 & 21/59 &  7/20 & 21/61 & 11/35 & 17/49 & 15/41 & 15/41 &  4/11 & 24/67 &  6/17 &  8/23 & 12/35 & 18/53 & 15/41 & 15/41 & 27/74 &  9/25 & 27/76 & 27/77 &  9/26 & 26/79 & 15/41 & 15/41 & 15/41 & 30/83 &  5/14 &  6/17 & 15/43 & 10/29 & 16/45 & 15/41 & 23/63 & 33/91 \\\hline
$34$ & 15/43 & 15/44 &  1/ 3 & 23/82 & 25/83 &  5/14 &  5/14 &  5/14 &  6/17 &  9/26 & 18/53 &  1/ 3 &  4/13 & 31/92 &  5/14 &  5/14 & 21/59 &  7/20 & 21/61 & 21/62 &  1/ 3 & 23/71 &  5/14 &  5/14 &  5/14 &  6/17 &  8/23 & 12/35 & 24/71 &  1/ 3 & 23/66 &  5/14 &  5/14 & 27/76 & 27/77 &  9/26 & 27/79 & 27/80 &  1/ 3 &  5/14 &  5/14 &  5/14 &  6/17 & 15/43 & 10/29 & 15/44 & 30/89 & 23/66 & 31/87 & 31/87 \\\hline
$35$ & 15/44 &  1/ 3 & 15/46 &  2/ 7 &  3/10 & 15/43 & 15/43 & 15/43 &  9/26 & 18/53 &  1/ 3 & 18/55 & 31/99 & 11/34 & 15/43 & 15/43 & 15/43 & 21/61 & 21/62 &  1/ 3 & 21/64 & 22/67 & 18/53 & 15/43 & 15/43 &  8/23 & 12/35 & 24/71 &  1/ 3 &  1/ 3 &  1/ 3 & 15/43 & 15/43 & 15/43 &  9/26 & 27/79 & 27/80 &  1/ 3 &  1/ 3 &  1/ 3 & 15/43 & 15/43 & 15/43 & 10/29 & 15/44 & 30/89 &  1/ 3 & 30/91 & 18/53 & 31/89 \\\hline
$36$ &  8/23 &  8/23 & 15/47 & 25/86 & 16/51 & 15/44 & 15/44 &  8/23 &  8/23 &  8/23 & 18/55 &  9/28 & 19/59 & 33/98 & 21/61 &  8/23 &  8/23 & 21/62 &  1/ 3 & 21/64 & 22/67 & 19/56 &  8/23 &  8/23 &  8/23 & 15/44 & 24/71 & 25/74 & 25/74 & 13/38 &  8/23 &  8/23 &  8/23 & 15/44 & 15/44 & 14/41 & 14/41 & 29/84 &  8/23 &  8/23 & 32/97 & 15/44 & 15/44 & 31/90 & 31/90 &  8/23 &  8/23 &  8/23 & 10/31 &  1/ 3 \\\hline
$37$ & 17/47 & 17/47 &  5/16 & 13/44 & 17/52 & 18/53 & 19/54 & 17/47 & 17/47 & 17/47 &  9/28 &  6/19 &  1/ 3 & 21/61 & 11/31 & 17/47 & 17/47 &  6/17 & 21/64 & 22/67 & 23/68 &  8/23 &  5/14 & 17/47 & 17/47 & 19/55 &  1/ 3 &  1/ 3 & 13/38 & 27/77 & 14/39 & 17/47 & 17/47 & 20/59 &  1/ 3 & 28/83 & 29/84 &  6/17 & 31/86 & 17/47 & 17/47 &  1/ 3 &  1/ 3 & 31/91 &  8/23 & 11/31 & 17/47 & 17/47 & 17/47 & 32/97 \\\hline
$38$ &  3/ 8 &  3/ 8 & 28/89 &  3/10 & 30/91 & 19/54 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 & 31/97 & 31/98 & 21/61 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 23/71 & 17/53 &  8/23 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 19/58 & 13/38 & 27/77 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 & 32/97 & 29/84 &  6/17 & 31/86 & 32/87 &  3/ 8 &  3/ 8 &  3/ 8 & 30/91 &  8/23 & 11/31 & 17/47 &  7/19 &  3/ 8 &  3/ 8 &  3/ 8 \\\hline
$39$ &  3/ 8 & 18/49 & 29/91 &  5/17 & 10/31 &  4/11 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 &  1/ 3 & 22/71 & 33/98 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 & 28/81 & 17/54 & 23/66 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 31/87 & 15/47 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 15/41 & 10/31 & 31/86 & 32/87 &  3/ 8 &  3/ 8 &  3/ 8 & 33/89 & 11/30 &  1/ 3 & 17/47 &  7/19 &  3/ 8 &  3/ 8 &  3/ 8 & 36/97 \\\hline
$40$ & 18/49 &  9/25 & 10/31 & 15/52 &  6/19 &  3/ 8 &  3/ 8 &  3/ 8 &  7/19 & 21/58 & 26/75 & 16/51 & 25/78 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 & 24/67 &  7/22 & 12/37 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 &  9/25 & 20/59 & 20/61 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 15/41 & 30/83 &  5/14 & 32/97 &  3/ 8 &  3/ 8 &  3/ 8 & 33/89 & 11/30 & 33/91 & 33/92 & 12/37 &  3/ 8 &  3/ 8 &  3/ 8 & 36/97 & 18/49 \\\hline
$41$ &  9/25 &  6/17 & 31/95 & 15/53 & 30/97 & 18/49 & 18/49 & 18/49 & 21/58 & 21/59 &  7/20 &  4/13 & 11/35 & 19/53 & 18/49 & 18/49 &  4/11 & 24/67 &  6/17 & 19/56 & 29/92 & 20/57 & 18/49 & 18/49 & 27/74 &  9/25 & 27/76 & 27/77 & 29/90 & 21/61 & 18/49 & 18/49 & 15/41 & 30/83 &  5/14 &  6/17 & 15/43 & 20/61 & 18/49 & 18/49 & 11/30 & 33/91 & 33/92 & 11/31 & 33/94 & 31/95 & 18/49 & 18/49 & 18/49 &  4/11 \\\hline
$42$ &  6/17 &  9/26 & 32/97 &  2/ 7 & 10/33 &  9/25 &  9/25 &  9/25 & 21/59 &  7/20 & 21/61 & 17/53 & 27/85 & 25/73 &  9/25 &  9/25 & 24/67 &  6/17 &  8/23 & 12/35 & 28/87 & 19/58 &  9/25 &  9/25 &  9/25 & 27/76 & 27/77 &  9/26 & 27/79 & 32/97 &  9/25 &  9/25 &  9/25 &  5/14 &  6/17 & 15/43 & 10/29 & 15/44 & 25/73 &  9/25 &  9/25 & 33/92 & 11/31 & 33/94 & 33/95 & 11/32 & 32/97 &  9/25 &  9/25 &  9/25 \\\hline
$43$ &  9/26 & 18/53 &  1/ 3 & 25/91 &  9/29 &  6/17 &  6/17 &  6/17 &  7/20 & 21/61 & 21/62 &  1/ 3 & 26/81 & 32/97 &  6/17 &  6/17 &  6/17 &  8/23 & 12/35 & 24/71 &  1/ 3 &  1/ 3 &  6/17 &  6/17 &  6/17 & 27/77 &  9/26 & 27/79 & 27/80 & 28/83 & 18/53 &  6/17 &  6/17 &  6/17 & 15/43 & 10/29 & 15/44 & 18/53 & 18/53 &  6/17 &  6/17 &  6/17 & 33/94 & 33/95 & 11/32 & 33/97 & 18/53 &  1/ 3 &  6/17 &  6/17 \\\hline
$44$ & 19/54 & 19/54 & 18/55 & 18/65 & 19/59 &  9/26 &  9/26 & 19/54 & 19/54 & 19/54 &  1/ 3 & 21/64 & 22/67 & 27/79 &  8/23 & 19/54 & 19/54 & 12/35 & 24/71 &  1/ 3 &  1/ 3 & 13/38 & 27/77 & 19/54 & 19/54 &  9/26 & 27/79 & 27/80 & 28/83 & 29/84 & 19/54 & 19/54 & 19/54 &  9/26 & 10/29 & 31/90 & 31/90 &  8/23 & 19/54 & 19/54 &  9/26 &  9/26 &  9/26 & 17/49 & 17/49 &  7/20 & 19/54 & 19/54 & 32/97 &  9/26 \\\hline
$45$ &  4/11 &  4/11 &  9/28 & 24/85 &  1/ 3 & 21/61 & 11/31 &  4/11 &  4/11 &  4/11 & 21/64 & 21/65 & 23/68 &  8/23 &  5/14 &  4/11 &  4/11 & 19/55 &  1/ 3 &  1/ 3 & 13/38 & 27/77 & 14/39 &  4/11 &  4/11 & 18/53 & 27/80 & 28/83 & 29/84 &  6/17 & 31/86 &  4/11 &  4/11 & 18/53 & 18/53 & 31/91 &  8/23 & 11/31 & 17/47 &  4/11 &  4/11 & 18/53 & 18/53 & 34/99 &  7/20 & 31/87 & 33/91 &  4/11 &  4/11 &  1/ 3 \\\hline
$46$ &  3/ 8 &  3/ 8 &  6/19 &  2/ 7 &  9/28 & 11/31 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 21/65 &  7/22 &  8/23 &  5/14 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 24/73 & 20/61 & 27/77 & 14/39 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 & 27/82 &  6/17 & 31/86 & 32/87 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 &  8/23 & 11/31 & 17/47 &  7/19 &  3/ 8 &  3/ 8 &  3/ 8 &  1/ 3 &  7/20 & 31/87 & 33/91 & 31/84 &  3/ 8 &  3/ 8 &  3/ 8 \\\hline
$47$ &  3/ 8 &  7/19 & 27/85 & 17/59 & 11/35 & 23/63 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 & 12/37 & 21/67 &  1/ 3 & 26/71 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 14/41 &  8/25 & 29/86 & 29/79 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 31/90 & 27/83 & 15/43 & 32/87 &  3/ 8 &  3/ 8 &  3/ 8 & 33/89 & 16/45 & 18/55 & 17/47 &  7/19 &  3/ 8 &  3/ 8 &  3/ 8 & 36/97 & 18/49 &  1/99 & 33/91 & 31/84 &  3/ 8 &  3/ 8 &  3/ 8 & 13/35 \\\hline
$48$ &  7/19 & 21/58 & 21/67 &  3/10 & 23/74 &  3/ 8 &  3/ 8 &  3/ 8 & 24/65 &  4/11 & 27/79 & 21/68 & 29/92 &  3/ 8 &  3/ 8 &  3/ 8 & 27/73 & 27/74 &  9/25 & 25/78 & 25/78 &  3/ 8 &  3/ 8 &  3/ 8 & 10/27 & 15/41 & 30/83 & 14/43 & 14/43 &  3/ 8 &  3/ 8 &  3/ 8 & 33/89 & 11/30 & 33/91 & 27/79 &  1/99 &  3/ 8 &  3/ 8 &  3/ 8 & 36/97 & 18/49 &  4/11 &  9/25 &  1/99 &  3/ 8 &  3/ 8 &  3/ 8 & 13/35 & 32/87 \\\hline
$49$ & 21/58 & 21/59 & 15/47 & 18/61 & 25/82 & 19/53 &  7/19 &  7/19 &  4/11 & 24/67 &  6/17 &  7/23 & 29/94 & 20/57 &  7/19 &  7/19 & 27/74 &  9/25 & 27/76 & 12/37 &  8/25 & 21/61 &  7/19 &  7/19 & 15/41 & 30/83 &  5/14 &  6/17 & 19/58 & 29/89 &  7/19 &  7/19 & 11/30 & 33/91 & 33/92 & 11/31 & 12/37 & 25/77 &  7/19 &  7/19 & 18/49 &  4/11 &  9/25 & 31/87 &  6/17 & 19/59 &  7/19 &  7/19 & 32/87 & 35/96 \\\hline
$50$ & 21/59 &  7/20 & 28/87 &  9/31 &  4/13 & 32/91 & 21/58 & 30/83 & 24/67 &  6/17 &  8/23 & 11/36 & 23/73 & 26/75 & 30/83 & 21/58 &  9/25 & 27/76 & 27/77 &  9/26 & 13/40 &  1/ 3 & 21/58 & 21/58 & 30/83 &  5/14 &  6/17 & 15/43 & 32/97 &  1/ 3 & 21/58 & 21/58 & 21/58 & 33/92 & 11/31 & 33/94 & 33/95 &  1/ 3 & 10/29 & 21/58 & 21/58 &  9/25 & 31/87 &  6/17 & 29/83 &  9/26 &  1/ 3 & 21/58 & 21/58 & 13/36 \\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 3, 4, 5, 5+k, 5+k+i\}$.
\end{center}


==> tables/table-g5-a3b4c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 3, 4, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a3b5c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 3, 5, 6, 6+k, 6+k+i\}$.
\end{center}


==> tables/table-g5-a4b5c6.tex <==
\begin{center}
\begin{longtable}[h]{r|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
 $k \setminus i$ & $1$& $2$& $3$& $4$& $5$& $6$& $7$& $8$& $9$& $10$& $11$& $12$& $13$& $14$& $15$& $16$& $17$& $18$& $19$& $20$& $21$& $22$& $23$& $24$& $25$& $26$& $27$& $28$& $29$& $30$& $31$& $32$& $33$& $34$& $35$& $36$& $37$& $38$& $39$& $40$& $41$& $42$& $43$& $44$& $45$& $46$& $47$& $48$& $49$& $50$\\\hline
$1$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$2$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$3$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$4$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$5$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$6$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$7$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$8$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$9$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$10$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$11$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$12$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$13$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$14$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$15$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$16$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$17$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$18$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$19$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$20$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$21$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$22$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$23$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$24$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$25$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$26$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$27$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$28$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$29$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$30$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$31$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$32$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$33$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$34$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$35$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$36$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$37$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$38$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$39$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$40$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$41$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$42$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$43$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$44$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$45$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$46$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$47$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$48$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$49$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
$50$ &&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&\\\hline
\end{longtable}
\textbf{Table.} Lower bounds on $\dalpha(S)$ for $S = \{ 4, 5, 6, 6+k, 6+k+i\}$.
\end{center}

